Magnetars

Magnetars are the most magnetic objects in the Universe, serving as unique laboratories to test physics under extreme magnetic conditions that cannot be replicated on Earth. They were discovered in the late 1970s through their powerful X-ray flares, and were subsequently identified as neutron stars characterized by steady and transient emission across the radio, infrared, optical, X-ray, and gamma-ray bands. In this chapter, we summarize the current state of our experimental and theoretical knowledge on magnetars, as well as briefly discussing their relationship with supernovae, gamma-ray bursts, fast radio bursts, and the transient multi-band sky at large.

==> reference2.tex <==
@book{Jaeger2023,
  title={Women of Genius in Science: Whose Frequently Overlooked Contributions Changed the World},
  author={Jaeger, L.},
  isbn={9783031239267},
  url={https://books.google.it/books?id=XWynEAAAQBAJ},
  year={2023},
  publisher={Springer International Publishing}
}

@article{abadie10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010CQGra..27q3001A},
	Archiveprefix = {arXiv},
	Author = {{Abadie}, J. and {Abbott}, B.~P. and {Abbott}, R. and {Abernathy}, M. and {Accadia}, T. and {Acernese}, F. and {Adams}, C. and {Adhikari}, R. and {Ajith}, P. and {Allen}, B. and et al.},
	Doi = {10.1088/0264-9381/27/17/173001},
	Eid = {173001},
	Eprint = {1003.2480},
	Journal = {Classical and Quantum Gravity},
	Month = sep,
	Number = 17,
	Pages = {173001},
	Primaryclass = {astro-ph.HE},
	Title = {{TOPICAL REVIEW: Predictions for the rates of compact binary coalescences observable by ground-based gravitational-wave detectors}},
	Volume = 27,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0264-9381/27/17/173001}}

@article{abazajian09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..182..543A},
	Archiveprefix = {arXiv},
	Author = {{Abazajian}, K.~N. and others},
	Doi = {10.1088/0067-0049/182/2/543},
	Eid = {543},
	Eprint = {0812.0649},
	Journal = {\apjs},
	Keywords = {atlases, catalogs, surveys},
	Month = jun,
	Pages = {543-558},
	Title = {{The Seventh Data Release of the Sloan Digital Sky Survey}},
	Volume = 182,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/182/2/543}}

@article{abbott16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016PhRvL.116f1102A},
	Archiveprefix = {arXiv},
	Author = {{Abbott}, B.~P. and {Abbott}, R. and {Abbott}, T.~D. and {Abernathy}, M.~R. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adams}, T. and {Addesso}, P. and {Adhikari}, R.~X. and et al.},
	Doi = {10.1103/PhysRevLett.116.061102},
	Eid = {061102},
	Eprint = {1602.03837},
	Journal = {\prl},
	Month = feb,
	Number = 6,
	Pages = {061102},
	Primaryclass = {gr-qc},
	Title = {{Observation of Gravitational Waves from a Binary Black Hole Merger}},
	Volume = 116,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.116.061102}}

@article{abeysekara18,
	Author = {{Abeysekara}, A.~U. and others},
	Doi = {10.1038/s41586-018-0565-5},
	Journal = {\nat},
	Pages = {82-85},
	Title = {Very-high-energy particle acceleration powered by the jets of the microquasar SS 433},
	Volume = 562,
	Year = 2018}

@article{aguilera08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...486..255A},
	Archiveprefix = {arXiv},
	Author = {{Aguilera}, D.~N. and {Pons}, J.~A. and {Miralles}, J.~A.},
	Doi = {10.1051/0004-6361:20078786},
	Eprint = {0710.0854},
	Journal = {\aap},
	Keywords = {stars: neutron, stars: magnetic fields, radiation mechanisms: thermal},
	Month = jul,
	Pages = {255-271},
	Title = {{2D Cooling of magnetized neutron stars}},
	Volume = 486,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078786}}

@article{aharonian04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004Natur.432...75A},
	Author = {{Aharonian}, F.~A. and {Akhperjanian}, A.~G. and {Aye}, K.-M. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Berghaus}, P. and {Bernl{\"o}hr}, K. and {Bolz}, O. and {Boisson}, C. and {Borgmeier}, C. and {Breitling}, F. and {Brown}, A.~M. and {Bussons Gordo}, J. and {Chadwick}, P.~M. and {Chitnis}, V.~R. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Djannati-Ata{\"\i}}, A. and {Drury}, L.~O. and {Ergin}, T. and {Espigat}, P. and {Feinstein}, F. and {Fleury}, P. and {Fontaine}, G. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Gillessen}, S. and {Goret}, P. and {Guy}, J. and {Hadjichristidis}, C. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {de Jager}, O.~C. and {Jung}, I. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemoine}, M. and {Lemi{\`e}re}, A. and {Leroy}, N. and {Lohse}, T. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {Pohl}, M. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Raux}, J. and {Rayner}, S.~M. and {Redondo}, I. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rivoal}, M. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schuster}, C. and {Schwanke}, U. and {Siewert}, M. and {Sol}, H. and {Steenkamp}, R. and {Stegmann}, C. and {Tavernet}, J.-P. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {van der Walt}, D.~J. and {Vasileiadis}, G. and {Vincent}, P. and {Visser}, B. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J.},
	Doi = {10.1038/nature02960},
	Eprint = {arXiv:astro-ph/0411533},
	Journal = {\nat},
	Month = nov,
	Pages = {75-77},
	Title = {{High-energy particle acceleration in the shell of a supernova remnant}},
	Volume = 432,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature02960}}

@article{aharonian05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005Sci...309..746A&db_key=AST},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Aye}, K.-M. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Berghaus}, P. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {Gordo}, J.~B. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Drury}, L.~O. and {Dubus}, G. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Fleury}, P. and {Fontaine}, G. and {Fuchs}, Y. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Gillessen}, S. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Leroy}, N. and {Lohse}, T. and {Marcowith}, A. and {Martin}, J.-M. and {Martineau-Huynh}, O. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Raux}, J. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schuster}, C. and {Schwanke}, U. and {Siewert}, M. and {Sol}, H. and {Spangler}, D. and {Steenkamp}, R. and {Stegmann}, C. and {Tavernet}, J.-P. and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J.},
	Doi = {10.1126/science.1113764},
	Eprint = {astro-ph/0508298},
	Journal = {Science},
	Month = jul,
	Pages = {746-749},
	Title = {{Discovery of Very High Energy Gamma Rays Associated with an X-ray Binary}},
	Volume = 309,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1113764}}

@article{aharonian_psrb1259_05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...442....1A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Aye}, K.-M. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Berghaus}, P. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {Bussons Gordo}, J. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Djannati-Ata{\"\i}}, A. and {O'C.~Drury}, L. and {Dubus}, G. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Fleury}, P. and {Fontaine}, G. and {Fuchs}, Y. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Gillessen}, S. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {de Jager}, O.~C. and {Johnston}, S. and {Kh{\'e}lifi}, B. and {Kirk}, J.~G. and {Komin}, N. and {Konopelko}, A. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Leroy}, N. and {Martineau-Huynh}, O. and {Lohse}, T. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Raux}, J. and {Rayner}, S.~M. and {Redondo}, I. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schuster}, C. and {Schwanke}, U. and {Siewert}, M. and {Skj{\ae}raasen}, O. and {Sol}, H. and {Steenkamp}, R. and {Stegmann}, C. and {Tavernet}, J.-P. and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J.},
	Doi = {10.1051/0004-6361:20052983},
	Eprint = {arXiv:astro-ph/0506280},
	Journal = {\aap},
	Month = oct,
	Pages = {1-10},
	Title = {{Discovery of the binary pulsar PSR B1259-63 in very-high-energy gamma rays around periastron with HESS}},
	Volume = 442,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052983}}

@article{aharonian05vjr,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437L...7A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {O'C.~Drury}, L. and {Dubus}, G. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Fontaine}, G. and {Fuchs}, Y. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Gillessen}, S. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Leroy}, N. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Raux}, J. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schuster}, C. and {Schwanke}, U. and {Siewert}, M. and {Sol}, H. and {Spangler}, D. and {Steenkamp}, R. and {Stegmann}, C. and {Tavernet}, J.-P. and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J.},
	Doi = {10.1051/0004-6361:200500130},
	Eprint = {arXiv:astro-ph/0505380},
	Journal = {\aap},
	Keywords = {gamma rays: observations, supernovae: individual:, RX J0852.0-4622 (G266.2-1.2)},
	Month = jul,
	Pages = {L7-L10},
	Title = {{Detection of TeV {$\gamma$}-ray emission from the shell-type supernova remnant RX J0852.0-4622 with HESS}},
	Volume = 437,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500130}}

@article{aharonian06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460..743A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Brown}, A.~M. and {B{\"u}hler}, R. and {B{\"u}sching}, I. and {Carrigan}, S. and {Chadwick}, P.~M. and {Chounet}, L.-M. and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {O'C.~Drury}, L. and {Dubus}, G. and {Egberts}, K. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Ferrero}, E. and {Fiasson}, A. and {Fontaine}, G. and {Funk}, S. and {Funk}, S. and {F{\"u}{\ss}ling}, M. and {Gallant}, Y.~A. and {Giebels}, B. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, D. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hoffmann}, A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kendziorra}, E. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Kosack}, K. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {Maurin}, G. and {McComb}, T.~J.~L. and {Moulin}, E. and {de Naurois}, M. and {Nedbal}, D. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Santangelo}, A. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schr{\"o}der}, R. and {Schwanke}, U. and {Schwarzburg}, S. and {Shalchi}, A. and {Sol}, H. and {Spangler}, D. and {Spanier}, F. and {Steenkamp}, R. and {Stegmann}, C. and {Superina}, G. and {Tavernet}, J.-P. and {Terrier}, R. and {Tluczykont}, M. and {van Eldik}, C. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J. and {Ward}, M.},
	Doi = {10.1051/0004-6361:20065940},
	Eprint = {arXiv:astro-ph/0607192},
	Journal = {\aap},
	Month = dec,
	Pages = {743-749},
	Title = {{3.9 day orbital modulation in the TeV {$\gamma$}-ray flux and spectrum from the X-ray binary LS 5039}},
	Volume = 460,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065940}}

@article{aab06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636..777A},
	Author = {{Aharonian}, F. and {Akhperjanian}, A.~G. and {Bazer-Bachi}, A.~R. and {Beilicke}, M. and {Benbow}, W. and {Berge}, D. and {Bernl{\"o}hr}, K. and {Boisson}, C. and {Bolz}, O. and {Borrel}, V. and {Braun}, I. and {Breitling}, F. and {Brown}, A.~M. and {Chadwick}, P.~M. and {Chounet}, {L.-M.} and {Cornils}, R. and {Costamante}, L. and {Degrange}, B. and {Dickinson}, H.~J. and {Djannati-Ata{\"\i}}, A. and {Drury}, L.~O. and {Dubus}, G. and {Emmanoulopoulos}, D. and {Espigat}, P. and {Feinstein}, F. and {Fontaine}, G. and {Fuchs}, Y. and {Funk}, S. and {Gallant}, Y.~A. and {Giebels}, B. and {Gillessen}, S. and {Glicenstein}, J.~F. and {Goret}, P. and {Hadjichristidis}, C. and {Hauser}, M. and {Heinzelmann}, G. and {Henri}, G. and {Hermann}, G. and {Hinton}, J.~A. and {Hofmann}, W. and {Holleran}, M. and {Horns}, D. and {Jacholkowska}, A. and {de Jager}, O.~C. and {Kh{\'e}lifi}, B. and {Komin}, N. and {Konopelko}, A. and {Latham}, I.~J. and {Le Gallou}, R. and {Lemi{\`e}re}, A. and {Lemoine-Goumard}, M. and {Leroy}, N. and {Lohse}, T. and {Martin}, J.~M. and {Martineau-Huynh}, O. and {Marcowith}, A. and {Masterson}, C. and {McComb}, T.~J.~L. and {de Naurois}, M. and {Nolan}, S.~J. and {Noutsos}, A. and {Orford}, K.~J. and {Osborne}, J.~L. and {Ouchrif}, M. and {Panter}, M. and {Pelletier}, G. and {Pita}, S. and {P{\"u}hlhofer}, G. and {Punch}, M. and {Raubenheimer}, B.~C. and {Raue}, M. and {Raux}, J. and {Rayner}, S.~M. and {Reimer}, A. and {Reimer}, O. and {Ripken}, J. and {Rob}, L. and {Rolland}, L. and {Rowell}, G. and {Sahakian}, V. and {Saug{\'e}}, L. and {Schlenker}, S. and {Schlickeiser}, R. and {Schuster}, C. and {Schwanke}, U. and {Siewert}, M. and {Sol}, H. and {Spangler}, D. and {Steenkamp}, R. and {Stegmann}, C. and {Tavernet}, {J.-P.} and {Terrier}, R. and {Th{\'e}oret}, C.~G. and {Tluczykont}, M. and {Vasileiadis}, G. and {Venter}, C. and {Vincent}, P. and {V{\"o}lk}, H.~J. and {Wagner}, S.~J.},
	Doi = {10.1086/498013},
	Eprint = {arXiv:astro-ph/0510397},
	Journal = {\apj},
	Keywords = {Catalogs, Gamma Rays: Observations, Stars: Pulsars: General, ISM: Supernova Remnants, Stars: Supernovae: General, Surveys},
	Month = jan,
	Pages = {777-797},
	Title = {{The H.E.S.S. Survey of the Inner Galaxy in Very High Energy Gamma Rays}},
	Volume = 636,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498013}}

@article{aizu73,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1973PThPh..49.1184A},
	Author = {{Aizu}, K.},
	Doi = {10.1143/PTP.49.1184},
	Journal = {Progress of Theoretical Physics},
	Month = apr,
	Pages = {1184-1194},
	Title = {{X-Ray Emission Region of a White Dwarf with Accretion}},
	Volume = 49,
	Year = 1973,
	Bdsk-Url-1 = {http://dx.doi.org/10.1143/PTP.49.1184}}

@article{albano10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722..788A},
	Archiveprefix = {arXiv},
	Author = {{Albano}, A. and {Turolla}, R. and {Israel}, G.~L. and {Zane}, S. and {Nobili}, L. and {Stella}, L.},
	Doi = {10.1088/0004-637X/722/1/788},
	Eprint = {1007.5466},
	Journal = {\apj},
	Keywords = {radiation mechanisms: non-thermal, stars: magnetic field, stars: neutron, X-rays: individual: XTE J1810{\ndash}197 CXOU J164710.2{\ndash}455216},
	Month = oct,
	Pages = {788-802},
	Primaryclass = {astro-ph.HE},
	Title = {{A Unified Timing and Spectral Model for the Anomalous X-ray Pulsars XTE J1810-197 and CXOU J164710.2-455216}},
	Volume = 722,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/722/1/788}}

@article{aaa06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...643L..53A},
	Author = {{Albert}, J. and {Aliu}, E. and {Anderhub}, H. and {Antoranz}, P. and {Armada}, A. and {Asensio}, M. and {Baixeras}, C. and {Barrio}, J.~A. and {Bartelt}, M. and {Bartko}, H. and {Bastieri}, D. and {Bavikadi}, S.~R. and {Bednarek}, W. and {Berger}, K. and {Bigongiari}, C. and {Biland}, A. and {Bisesi}, E. and {Bock}, R.~K. and {Bordas}, P. and {Bosch-Ramon}, V. and {Bretz}, T. and {Britvitch}, I. and {Camara}, M. and {Carmona}, E. and {Chilingarian}, A. and {Ciprini}, S. and {Coarasa}, J.~A. and {Commichau}, S. and {Contreras}, J.~L. and {Cortina}, J. and {Curtef}, V. and {Dame}, T.~M. and {Danielyan}, V. and {Dazzi}, F. and {De Angelis}, A. and {de los Reyes}, R. and {De Lotto}, B. and {Domingo-Santamar{\'{\i}}}, E. and {Dorner}, D. and {Doro}, M. and {Errando}, M. and {Fagiolini}, M. and {Ferenc}, D. and {Fern{\'a}ndez}, E. and {Firpo}, R. and {Flix}, J. and {Fonseca}, M.~V. and {Font}, L. and {Fuchs}, M. and {Galante}, N. and {Garczarczyk}, M. and {Gaug}, M. and {Giller}, M. and {Goebel}, F. and {Hakobyan}, D. and {Hayashida}, M. and {Hengstebeck}, T. and {H{\"o}hne}, D. and {Hose}, J. and {Hsu}, C.~C. and {Isar}, P.~G. and {Jacon}, P. and {Kalekin}, O. and {Kasyra}, R. and {Kranich}, D. and {Laatiaoui}, M. and {Laille}, A. and {Lenisa}, T. and {Liebing}, P. and {Lindfors}, E. and {Lombardi}, S. and {Longo}, F. and {L{\'o}pez}, J. and {L{\'o}pez}, M. and {Lorenz}, E. and {Lucarelli}, F. and {Majumdar}, P. and {Maneva}, G. and {Mannheim}, K. and {Mansutti}, O. and {Mariotti}, M. and {Mart{\'{\i}}nez}, M. and {Mase}, K. and {Mazin}, D. and {Merck}, C. and {Meucci}, M. and {Meyer}, M. and {Miranda}, J.~M. and {Mirzoyan}, R. and {Mizobuchi}, S. and {Moralejo}, A. and {Nilsson}, K. and {O{\~n}a-Wilhelmi}, E. and {Ordu{\~n}a}, R. and {Otte}, N. and {Oya}, I. and {Paneque}, D. and {Paoletti}, R. and {Paredes}, J.~M. and {Pasanen}, M. and {Pascoli}, D. and {Pauss}, F. and {Pavel}, N. and {Pegna}, R. and {Persic}, M. and {Peruzzo}, L. and {Piccioli}, A. and {Poller}, M. and {Prandini}, E. and {Raymers}, A. and {Rico}, J. and {Rhode}, W. and {Rib{\'o}}, M. and {Riegel}, B. and {Rissi}, M. and {Robert}, A. and {R{\"u}gamer}, S. and {Saggion}, A. and {S{\'a}nchez}, A. and {Sartori}, P. and {Scalzotto}, V. and {Scapin}, V. and {Schmitt}, R. and {Schweizer}, T. and {Shayduk}, M. and {Shinozaki}, K. and {Shore}, S.~N. and {Sidro}, N. and {Sillanp{\"a}{\"a}}, A. and {Sobczynska}, D. and {Stamerra}, A. and {Stark}, L.~S. and {Takalo}, L. and {Temnikov}, P. and {Tescaro}, D. and {Teshima}, M. and {Tonello}, N. and {Torres}, A. and {Torres}, D.~F. and {Turini}, N. and {Vankov}, H. and {Vitale}, V. and {Wagner}, R.~M. and {Wibig}, T. and {Wittek}, W. and {Zanin}, R. and {Zapatero}, J.},
	Date-Modified = {2016-08-31 09:22:36 am +0000},
	Doi = {10.1086/504917},
	Eprint = {arXiv:astro-ph/0604197},
	Journal = {\apjl},
	Keywords = {Gamma Rays: Observations, ISM: Supernova Remnants},
	Month = may,
	Pages = {L53-L56},
	Title = {{Observation of VHE Gamma Radiation from HESS J1834-087/W41 with the MAGIC Telescope}},
	Volume = 643,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/504917}}

@article{alcock86,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1986PhRvL..57.2088A&amp;db_key=AST},
	Author = {{Alcock}, C. and {Farhi}, E. and {Olinto}, A.},
	Journal = {Physical Review Letters},
	Month = oct,
	Pages = {2088-2091},
	Title = {{Model for the 5 March 1979 gamma-ray transient}},
	Volume = 57,
	Year = 1986}

@article{alcock01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001MNRAS.321..678A},
	Author = {{Alcock}, C. and {Allsman}, R.~A. and {Alves}, D.~R. and {Axelrod}, T.~S. and {Becker}, A.~C. and {Bennett}, D.~P. and {Charles}, P.~A. and {Cook}, K.~H. and {Drake}, A.~J. and {Freeman}, K.~C. and {Geha}, M. and {Griest}, K. and {Lehner}, M.~J. and {Marshall}, S.~L. and {McGowan}, K.~E. and {Minniti}, D. and {Nelson}, C.~A. and {Peterson}, B.~A. and {Popowski}, P. and {Pratt}, M.~R. and {Quinn}, P.~J. and {Stubbs}, C.~W. and {Sutherland}, W. and {Tomaney}, A.~B. and {Vandehei}, T. and {Welch}, D.~L.},
	Eprint = {arXiv:astro-ph/0009415},
	Journal = {\mnras},
	Month = mar,
	Pages = {678-684},
	Title = {{A 421-d activity cycle in the BeX recurrent transient A0538-66 from MACHO monitoring}},
	Volume = 321,
	Year = 2001}

@article{albert06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006Sci...312.1771A&db_key=AST},
	Author = {{Albert}, J. and {Aliu}, E. and {Anderhub}, H. and {Antoranz}, P. and {Armada}, A. and {Asensio}, M. and {Baixeras}, C. and {Barrio}, J.~A. and {Bartelt}, M. and {Bartko}, H. and {Bastieri}, D. and {Bavikadi}, S.~R. and {Bednarek}, W. and {Berger}, K. and {Bigongiari}, C. and {Biland}, A. and {Bisesi}, E. and {Bock}, R.~K. and {Bordas}, P. and {Bosch-Ramon}, V. and {Bretz}, T. and {Britvitch}, I. and {Camara}, M. and {Carmona}, E. and {Chilingarian}, A. and {Ciprini}, S. and {Coarasa}, J.~A. and {Commichau}, S. and {Contreras}, J.~L. and {Cortina}, J. and {Curtef}, V. and {Danielyan}, V. and {Dazzi}, F. and {De Angelis}, A. and {de los Reyes}, R. and {De Lotto}, B. and {Domingo-Santamar{\'{\i}}a}, E. and {Dorner}, D. and {Doro}, M. and {Errando}, M. and {Fagiolini}, M. and {Ferenc}, D. and {Fern{\'a}ndez}, E. and {Firpo}, R. and {Flix}, J. and {Fonseca}, M.~V. and {Font}, L. and {Fuchs}, M. and {Galante}, N. and {Garczarczyk}, M. and {Gaug}, M. and {Giller}, M. and {Goebel}, F. and {Hakobyan}, D. and {Hayashida}, M. and {Hengstebeck}, T. and {H{\"o}hne}, D. and {Hose}, J. and {Hsu}, C.~C. and {Isar}, P.~G. and {Jacon}, P. and {Kalekin}, O. and {Kosyra}, R. and {Kranich}, D. and {Laatiaoui}, M. and {Laille}, A. and {Lenisa}, T. and {Liebing}, P. and {Lindfors}, E. and {Lombardi}, S. and {Longo}, F. and {L{\'o}pez}, J. and {L{\'o}pez}, M. and {Lorenz}, E. and {Lucarelli}, F. and {Majumdar}, P. and {Maneva}, G. and {Mannheim}, K. and {Mansutti}, O. and {Mariotti}, M. and {Mart{\'{\i}}nez}, M. and {Mase}, K. and {Mazin}, D. and {Merck}, C. and {Meucci}, M. and {Meyer}, M. and {Miranda}, J.~M. and {Mirzoyan}, R. and {Mizobuchi}, S. and {Moralejo}, A. and {Nilsson}, K. and {O{\~n}a-Wilhelmi}, E. and {Ordu{\~n}a}, R. and {Otte}, N. and {Oya}, I. and {Paneque}, D. and {Paoletti}, R. and {Paredes}, J.~M. and {Pasanen}, M. and {Pascoli}, D. and {Pauss}, F. and {Pavel}, N. and {Pegna}, R. and {Persic}, M. and {Peruzzo}, L. and {Piccioli}, A. and {Poller}, M. and {Pooley}, G. and {Prandini}, E. and {Raymers}, A. and {Rhode}, W. and {Rib{\'o}}, M. and {Rico}, J. and {Riegel}, B. and {Rissi}, M. and {Robert}, A. and {Romero}, G.~E. and {R{\"u}gamer}, S. and {Saggion}, A. and {S{\'a}nchez}, A. and {Sartori}, P. and {Scalzotto}, V. and {Scapin}, V. and {Schmitt}, R. and {Schweizer}, T. and {Shayduk}, M. and {Shinozaki}, K. and {Shore}, S.~N. and {Sidro}, N. and {Sillanp{\"a}{\"a}}, A. and {Sobczynska}, D. and {Stamerra}, A. and {Stark}, L.~S. and {Takalo}, L. and {Temnikov}, P. and {Tescaro}, D. and {Teshima}, M. and {Tonello}, N. and {Torres}, A. and {Torres}, D.~F. and {Turini}, N. and {Vankov}, H. and {Vitale}, V. and {Wagner}, R.~M. and {Wibig}, T. and {Wittek}, W. and {Zanin}, R. and {Zapatero}, J.},
	Doi = {10.1126/science.1128177},
	Eprint = {astro-ph/0605549},
	Journal = {Science},
	Month = jun,
	Pages = {1771-1773},
	Title = {{Variable Very-High-Energy Gamma-Ray Emission from the Microquasar LS I +61 303}},
	Volume = 312,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1128177}}

@ARTICLE{alekseev87,
   author = {{Alekseev}, E.~N. and {Alekseeva}, L.~N. and {Volchenko}, V.~I. and 
	{Krivosheina}, I.~V.},
    title = "{Possible detection of a neutrino signal on 23 February 1987 at the Baksan underground scintillation telescope of the Institute of Nuclear Research}",
  journal = {Soviet Journal of Experimental and Theoretical Physics Letters},
     year = 1987,
    month = may,
   volume = 45,
    pages = {589},
   adsurl = {http://adsabs.harvard.edu/abs/1987JETPL..45..589A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{aleksic13,
   author = {{Aleksi{\'c}}, J. and {Antonelli}, L.~A. and {Antoranz}, P. and 
	{Asensio}, M. and {Barres de Almeida}, U. and {Barrio}, J.~A. and 
	{Becerra Gonz{\'a}lez}, J. and {Bednarek}, W. and {Berger}, K. and 
	{Bernardini}, E. and {Biland}, A. and {Blanch}, O. and {Bock}, R.~K. and 
	{Boller}, A. and {Bonnoli}, G. and {Borla Tridon}, D. and {Bretz}, T. and 
	{Carmona}, E. and {Carosi}, A. and {Colin}, P. and {Colombo}, E. and 
	{Contreras}, J.~L. and {Cortina}, J. and {Cossio}, L. and {Covino}, S. and 
	{Da Vela}, P. and {Dazzi}, F. and {De Angelis}, A. and {De Caneva}, G. and 
	{De Cea del Pozo}, E. and {De Lotto}, B. and {Delgado Mendez}, C. and 
	{Diago Ortega}, A. and {Doert}, M. and {Dominis Prester}, D. and 
	{Dorner}, D. and {Doro}, M. and {Eisenacher}, D. and {Elsaesser}, D. and 
	{Ferenc}, D. and {Fonseca}, M.~V. and {Font}, L. and {Fruck}, C. and 
	{Garc{\'{\i}}a L{\'o}pez}, R.~J. and {Garczarczyk}, M. and {Garrido Terrats}, D. and 
	{Gaug}, M. and {Giavitto}, G. and {Godinovi{\'c}}, N. and {Gonz{\'a}lez Mu{\~n}oz}, A. and 
	{Gozzini}, S.~R. and {Hadamek}, A. and {Hadasch}, D. and {H{\"a}fner}, D. and 
	{Herrero}, A. and {Hose}, J. and {Hrupec}, D. and {Huber}, B. and 
	{Jankowski}, F. and {Jogler}, T. and {Kadenius}, V. and {Klepser}, S. and 
	{Knoetig}, M.~L. and {Kr{\"a}henb{\"u}hl}, T. and {Krause}, J. and 
	{Kushida}, J. and {La Barbera}, A. and {Lelas}, D. and {Leonardo}, E. and 
	{Lewandowska}, N. and {Lindfors}, E. and {Lombardi}, S. and 
	{L{\'o}pez}, M. and {L{\'o}pez-Coto}, R. and {L{\'o}pez-Oramas}, A. and 
	{Lorenz}, E. and {Makariev}, M. and {Maneva}, G. and {Mankuzhiyil}, N. and 
	{Mannheim}, K. and {Maraschi}, L. and {Marcote}, B. and {Mariotti}, M. and 
	{Mart{\'{\i}}nez}, M. and {Mazin}, D. and {Meucci}, M. and {Miranda}, J.~M. and 
	{Mirzoyan}, R. and {Mold{\'o}n}, J. and {Moralejo}, A. and {Munar-Adrover}, P. and 
	{Niedzwiecki}, A. and {Nieto}, D. and {Nilsson}, K. and {Nowak}, N. and 
	{Orito}, R. and {Paiano}, S. and {Palatiello}, M. and {Paneque}, D. and 
	{Paoletti}, R. and {Paredes}, J.~M. and {Partini}, S. and {Persic}, M. and 
	{Pilia}, M. and {Pochon}, J. and {Prada}, F. and {Prada Moroni}, P.~G. and 
	{Prandini}, E. and {Puljak}, I. and {Reichardt}, I. and {Reinthal}, R. and 
	{Rhode}, W. and {Rib{\'o}}, M. and {Rico}, J. and {R{\"u}gamer}, S. and 
	{Saggion}, A. and {Saito}, K. and {Saito}, T.~Y. and {Salvati}, M. and 
	{Satalecka}, K. and {Scalzotto}, V. and {Scapin}, V. and {Schultz}, C. and 
	{Schweizer}, T. and {Shore}, S.~N. and {Sillanp{\"a}{\"a}}, A. and 
	{Sitarek}, J. and {Snidaric}, I. and {Sobczynska}, D. and {Spanier}, F. and 
	{Spiro}, S. and {Stamatescu}, V. and {Stamerra}, A. and {Steinke}, B. and 
	{Storz}, J. and {Sun}, S. and {Suri{\'c}}, T. and {Takalo}, L. and 
	{Takami}, H. and {Tavecchio}, F. and {Temnikov}, P. and {Terzi{\'c}}, T. and 
	{Tescaro}, D. and {Teshima}, M. and {Tibolla}, O. and {Torres}, D.~F. and 
	{Toyama}, T. and {Treves}, A. and {Uellenbeck}, M. and {Vogler}, P. and 
	{Wagner}, R.~M. and {Weitzel}, Q. and {Zabalza}, V. and {Zandanel}, F. and 
	{Zanin}, R. and {Rea}, N. and {Backes}, M.},
    title = "{Observations of the magnetars 4U 0142+61 and 1E 2259+586 with the MAGIC telescopes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.1173},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetars, stars: individual: 4U 0142+61, stars: individual: 1E 2259+586, radiation mechanisms: non-thermal, gamma rays: stars},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A23},
    pages = {A23},
      doi = {10.1051/0004-6361/201220275},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A..23A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{alfven58,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1958Tell...10..104A},
	Author = {{Alfv{\'e}n}, H.},
	Journal = {Tellus},
	Month = feb,
	Pages = {104},
	Title = {{On the Theory of Magnetic Storms and Aurorae}},
	Volume = 10,
	Year = 1958}

@article{alfven86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986ITPS...14..779A},
	Author = {{Alfv{\'e}n}, H.},
	Doi = {10.1109/TPS.1986.4316626},
	Journal = {IEEE Transactions on Plasma Science},
	Keywords = {ASTRONOMICAL MODELS, CIRCUITS, COSMIC PLASMA, PLASMA LAYERS, AURORAL IONIZATION, EDUCATION, EXTRAGALACTIC RADIO SOURCES, GAMMA RAY BURSTS, SOLAR FLARES},
	Month = dec,
	Pages = {779-793},
	Title = {{Double layers and circuits in astrophysics}},
	Volume = 14,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1109/TPS.1986.4316626}}

@article{allan98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.295..167A},
	Author = {{Allan}, A. and {Hellier}, C. and {Beardmore}, A.},
	Doi = {10.1046/j.1365-8711.1998.29511353.x},
	Journal = {\mnras},
	Keywords = {White Dwarf Stars, X Ray Astronomy, Spectral Resolution, Astronomical Spectroscopy, Accretion Disks, Astronomical Models, Temperature Distribution, Shock Waves},
	Month = mar,
	Pages = {167},
	Title = {{ASCA X-ray observations of EX Hya - Spin-resolved spectroscopy}},
	Volume = 295,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.29511353.x}}

@ARTICLE{allen04,
   author = {{Allen}, M.~P. and {Horvath}, J.~E.},
    title = "{Influence of an Internal Magnetar on Supernova Remnant Expansion}",
  journal = {\apj},
   eprint = {astro-ph/0311570},
 keywords = {Stars: Magnetic Fields, Stars: Neutron, ISM: Supernova Remnants},
     year = 2004,
    month = nov,
   volume = 616,
    pages = {346-356},
      doi = {10.1086/424836},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616..346A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{allen12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750..125A},
	Archiveprefix = {arXiv},
	Author = {{Allen}, T.~S. and {Gutermuth}, R.~A. and {Kryukova}, E. and {Megeath}, S.~T. and {Pipher}, J.~L. and {Naylor}, T. and {Jeffries}, R.~D. and {Wolk}, S.~J. and {Spitzbart}, B. and {Muzerolle}, J.},
	Doi = {10.1088/0004-637X/750/2/125},
	Eid = {125},
	Eprint = {1203.5089},
	Journal = {\apj},
	Keywords = {infrared: stars, stars: formation, stars: pre-main sequence},
	Month = may,
	Pages = {125},
	Primaryclass = {astro-ph.SR},
	Title = {{Spitzer Imaging of the nearby Rich Young Cluster, Cep OB3b}},
	Volume = 750,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/750/2/125}}

@article{alpar01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554.1245A},
	Author = {{Alpar}, M.~A.},
	Doi = {10.1086/321393},
	Eprint = {arXiv:astro-ph/0005211},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Magnetic Fields, Stars: Neutron, Stars: Supernovae: General},
	Month = jun,
	Pages = {1245-1254},
	Title = {{On Young Neutron Stars as Propellers and Accretors with Conventional Magnetic Fields}},
	Volume = 554,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321393}}

@article{alpar11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732L...4A},
	Archiveprefix = {arXiv},
	Author = {{Alpar}, M.~A. and {Ertan}, {\"U}. and {{\c C}al{\i}{\c s}kan}, {\c S}.},
	Doi = {10.1088/2041-8205/732/1/L4},
	Eid = {L4},
	Eprint = {1102.1336},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, pulsars: individual: AXPs, stars: neutron, X-rays: bursts},
	Month = may,
	Pages = {L4},
	Primaryclass = {astro-ph.HE},
	Title = {{SGR 0418+5729{\mdash}How does a Young Neutron Star Spin Down to a 9 s Period with a Dipole Field Less Than 10$^{13}$ G?}},
	Volume = 732,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/732/1/L4}}

@ARTICLE{alton04,
   author = {{Alton}, P.~B. and {Xilouris}, E.~M. and {Misiriotis}, A. and 
	{Dasyra}, K.~M. and {Dumke}, M.},
    title = "{The emissivity of dust grains in spiral galaxies}",
  journal = {\aap},
 keywords = {ISM: dust, extinction, galaxies: ISM, galaxies: spiral, infrared: galaxies, submillimeter},
     year = 2004,
    month = oct,
   volume = 425,
    pages = {109-120},
      doi = {10.1051/0004-6361:20040438},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425..109A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{an14,
   author = {{An}, H. and {Kaspi}, V.~M. and {Archibald}, R. and {Bachetti}, M. and 
	{Bhalerao}, V. and {Bellm}, E.~C. and {Beloborodov}, A.~M. and 
	{Boggs}, S.~E. and {Chakrabarty}, D. and {Christensen}, F.~E. and 
	{Craig}, W.~W. and {Dufour}, F. and {Forster}, K. and {Gotthelf}, E.~V. and 
	{Grefenstette}, B.~W. and {Hailey}, C.~J. and {Harrison}, F.~A. and 
	{Hasco{\"e}t}, R. and {Kitaguchi}, T. and {Kouveliotou}, C. and 
	{Madsen}, K.~K. and {Mori}, K. and {Pivovaroff}, M.~J. and {Rana}, V.~R. and 
	{Stern}, D. and {Tendulkar}, S. and {Tomsick}, J.~A. and {Vogel}, J.~K. and 
	{Zhang}, W.~W. and {NuSTAR Team}},
    title = "{NuSTAR results and future plans for magnetar and rotation-powered pulsar observations}",
  journal = {Astronomische Nachrichten},
archivePrefix = "arXiv",
   eprint = {1402.1079},
 primaryClass = "astro-ph.HE",
 keywords = {space vehicles, stars: neutron, telescopes, X-rays: stars},
     year = 2014,
    month = mar,
   volume = 335,
    pages = {280-284},
      doi = {10.1002/asna.201312032},
   adsurl = {http://adsabs.harvard.edu/abs/2014AN....335..280A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{anders89,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1989GeCoA..53..197A},
	Author = {{Anders}, E. and {Grevesse}, N.},
	Doi = {10.1016/0016-7037(89)90286-X},
	Journal = {\gca},
	Month = jan,
	Pages = {197-214},
	Title = {{Abundances of the elements - Meteoritic and solar}},
	Volume = 53,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/0016-7037(89)90286-X}}

@article{anderson12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...53A},
	Archiveprefix = {arXiv},
	Author = {{Anderson}, G.~E. and {Gaensler}, B.~M. and {Slane}, P.~O. and {Rea}, N. and {Kaplan}, D.~L. and {Posselt}, B. and {Levin}, L. and {Johnston}, S. and {Murray}, S.~S. and {Brogan}, C.~L. and {Bailes}, M. and {Bates}, S. and {Benjamin}, R.~A. and {Bhat}, N.~D.~R. and {Burgay}, M. and {Burke-Spolaor}, S. and {Chakrabarty}, D. and {D'Amico}, N. and {Drake}, J.~J. and {Esposito}, P. and {Grindlay}, J.~E. and {Hong}, J. and {Israel}, G.~L. and {Keith}, M.~J. and {Kramer}, M. and {Lazio}, T.~J.~W. and {Lee}, J.~C. and {Mauerhan}, J.~C. and {Milia}, S. and {Possenti}, A. and {Stappers}, B. and {Steeghs}, D.~T.~H.},
	Doi = {10.1088/0004-637X/751/1/53},
	Eid = {53},
	Eprint = {1203.2719},
	Journal = {\apj},
	Keywords = {ISM: individual objects: G333.9+0.0, ISM: supernova remnants, pulsars: individual: PSR J1622-4950, radio continuum: stars, stars: neutron, X-rays: stars},
	Month = may,
	Pages = {53},
	Primaryclass = {astro-ph.HE},
	Title = {{Multi-wavelength Observations of the Radio Magnetar PSR J1622-4950 and Discovery of Its Possibly Associated Supernova Remnant}},
	Volume = 751,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/751/1/53}}

@article{antoniou09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697.1695A},
	Archiveprefix = {arXiv},
	Author = {{Antoniou}, V. and {Zezas}, A. and {Hatzidimitriou}, D. and {McDowell}, J.~C.},
	Doi = {10.1088/0004-637X/697/2/1695},
	Eprint = {0812.1226},
	Journal = {\apj},
	Keywords = {Magellanic Clouds, pulsars: general, stars: early-type, stars: emission-line, Be, stars: formation, X-rays: binaries},
	Month = jun,
	Pages = {1695-1716},
	Title = {{The Chandra Survey of the Small Magellanic Cloud ''Bar''. II. Optical Counterparts of X-ray Sources}},
	Volume = 697,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/697/2/1695}}

@article{ahz09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707.1080A},
	Archiveprefix = {arXiv},
	Author = {{Antoniou}, V. and {Hatzidimitriou}, D. and {Zezas}, A. and {Reig}, P.},
	Doi = {10.1088/0004-637X/707/2/1080},
	Eprint = {0912.1876},
	Journal = {\apj},
	Keywords = {galaxies: individual: Galaxy, Magellanic Clouds, stars: emission-line, Be, X-rays: binaries},
	Month = dec,
	Pages = {1080-1097},
	Primaryclass = {astro-ph.HE},
	Title = {{Optical Spectroscopy of 20 Be/X-ray Binaries in the Small Magellanic Cloud}},
	Volume = 707,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/707/2/1080}}

@article{antoniou10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716L.140A},
	Archiveprefix = {arXiv},
	Author = {{Antoniou}, V. and {Zezas}, A. and {Hatzidimitriou}, D. and {Kalogera}, V.},
	Doi = {10.1088/2041-8205/716/2/L140},
	Eprint = {1006.2381},
	Journal = {\apjl},
	Keywords = {Magellanic Clouds, pulsars: general, stars: early-type, stars: emission-line, Be, stars: formation, X-rays: binaries},
	Month = jun,
	Pages = {L140-L145},
	Primaryclass = {astro-ph.HE},
	Title = {{Star Formation History and X-ray Binary Populations: The Case of the Small Magellanic Cloud}},
	Volume = 716,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/716/2/L140}}

@article{antonopolou15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.3924A},
	Archiveprefix = {arXiv},
	Author = {{Antonopoulou}, D. and {Weltevrede}, P. and {Espinoza}, C.~M. and {Watts}, A.~L. and {Johnston}, S. and {Shannon}, R.~M. and {Kerr}, M.},
	Doi = {10.1093/mnras/stu2710},
	Eprint = {1412.5853},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, pulsars: individual: PSR J1119-6127},
	Month = mar,
	Pages = {3924-3935},
	Primaryclass = {astro-ph.HE},
	Title = {{The unusual glitch recoveries of the high-magnetic-field pulsar J1119-6127}},
	Volume = 447,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu2710}}

@article{anzolin08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489.1243A},
	Archiveprefix = {arXiv},
	Author = {{Anzolin}, G. and {de Martino}, D. and {Bonnet-Bidaud}, J.-M. and {Mouchet}, M. and {G{\"a}nsicke}, B.~T. and {Matt}, G. and {Mukai}, K.},
	Doi = {10.1051/0004-6361:200810402},
	Eprint = {0808.1499},
	Journal = {\aap},
	Keywords = {stars: binaries: close, stars: individual: 1RXS J070407.9+262501, stars: individual: 1RXS 180340.0+401214, stars: novae, cataclysmic variables, X-rays: stars, accretion, accretion disks},
	Month = oct,
	Pages = {1243-1254},
	Title = {{Two new intermediate polars with a soft X-ray component}},
	Volume = 489,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810402}}

@article{anzolin09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501.1047A},
	Archiveprefix = {arXiv},
	Author = {{Anzolin}, G. and {de Martino}, D. and {Falanga}, M. and {Mukai}, K. and {Bonnet-Bidaud}, J.-M. and {Mouchet}, M. and {Terada}, Y. and {Ishida}, M.},
	Doi = {10.1051/0004-6361/200911816},
	Eprint = {0905.1080},
	Journal = {\aap},
	Keywords = {stars: binaries: close, stars: individual: IGR J00234+6141, stars: individual: 1RXS J213344.1+510725, stars: novae, cataclysmic variables, X-rays: stars, accretion, accretion disks},
	Month = jul,
	Pages = {1047-1058},
	Primaryclass = {astro-ph.SR},
	Title = {{Broad-band properties of the hard X-ray cataclysmic variables IGR J00234+6141 and 1RXS J213344.1+510725}},
	Volume = 501,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200911816}}

@article{aptekar01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJS..137..227A&amp;db_key=AST},
	Author = {{Aptekar}, R.~L. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Il'inskii}, V.~N. and {Mazets}, E.~P. and {Pal'shin}, V.~D. and {Butterworth}, P.~S. and {Cline}, T.~L.},
	Journal = {\apjs},
	Month = dec,
	Pages = {227-277},
	Title = {{Konus Catalog of Soft Gamma Repeater Activity: 1978 to 2000}},
	Volume = 137,
	Year = 2001}

@ARTICLE{arcasedda18,
       author = {{Arca Sedda}, Manuel and {Askar}, Abbas and {Giersz}, Mirek},
        title = "{MOCCA-Survey Database - I. Unravelling black hole subsystems in globular clusters}",
      journal = {\mnras},
     keywords = {black hole physics, stars: kinematics and dynamics, globular clusters: general, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {479},
       number = {4},
        pages = {4652-4664},
          doi = {10.1093/mnras/sty1859},
archivePrefix = {arXiv},
       eprint = {1801.00795},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479.4652A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{arcasedda21,
       author = {{Arca-Sedda}, Manuel and {Rizzuto}, Francesco Paolo and {Naab}, Thorsten and {Ostriker}, Jeremiah and {Giersz}, Mirek and {Spurzem}, Rainer},
        title = "{Breaching the Limit: Formation of GW190521-like and IMBH Mergers in Young Massive Clusters}",
      journal = {\apj},
     keywords = {Astrophysical black holes, Black holes, Intermediate-mass black holes, Stellar mass black holes, Young star clusters, Globular star clusters, Galaxy nuclei, Gravitational wave astronomy, Gravitational wave detectors, Gravitational wave sources, 98, 162, 816, 1611, 1833, 656, 609, 675, 676, 677, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.3847/1538-4357/ac1419},
archivePrefix = {arXiv},
       eprint = {2105.07003},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920..128A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{archibald17,
   author = {{Archibald}, R.~F. and {Burgay}, M. and {Lyutikov}, M. and {Kaspi}, V.~M. and 
	{Esposito}, P. and {Israel}, G. and {Kerr}, M. and {Possenti}, A. and 
	{Rea}, N. and {Sarkissian}, J. and {Scholz}, P. and {Tendulkar}, S.~P.
	},
    title = "{Magnetar-like X-Ray Bursts Suppress Pulsar Radio Emission}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1710.03718},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, pulsars: individual: PSR J1119{\ndash}6127, stars: magnetars},
     year = 2017,
    month = nov,
   volume = 849,
      eid = {L20},
    pages = {L20},
      doi = {10.3847/2041-8213/aa9371},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...849L..20A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{arcodia21,
       author = {{Arcodia}, R. and {Merloni}, A. and {Nandra}, K. and {Buchner}, J. and {Salvato}, M. and {Pasham}, D. and {Remillard}, R. and {Comparat}, J. and {Lamer}, G. and {Ponti}, G. and {Malyali}, A. and {Wolf}, J. and {Arzoumanian}, Z. and {Bogensberger}, D. and {Buckley}, D.~A.~H. and {Gendreau}, K. and {Gromadzki}, M. and {Kara}, E. and {Krumpe}, M. and {Markwardt}, C. and {Ramos-Ceja}, M.~E. and {Rau}, A. and {Schramm}, M. and {Schwope}, A.},
        title = "{X-ray Quasi-Periodic Eruptions from two previously quiescent galaxies}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
          volume = 592,
        pages = {704-707},
archivePrefix = {arXiv},
       eprint = {2104.13388},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210413388A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{arevalo14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791...81A},
	Archiveprefix = {arXiv},
	Author = {{Ar{\'e}valo}, P. and {Bauer}, F.~E. and {Puccetti}, S. and {Walton}, D.~J. and {Koss}, M. and {Boggs}, S.~E. and {Brandt}, W.~N. and {Brightman}, M. and {Christensen}, F.~E. and {Comastri}, A. and {Craig}, W.~W. and {Fuerst}, F. and {Gandhi}, P. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Harrison}, F.~A. and {Luo}, B. and {Madejski}, G. and {Madsen}, K.~K. and {Marinucci}, A. and {Matt}, G. and {Saez}, C. and {Stern}, D. and {Stuhlinger}, M. and {Treister}, E. and {Urry}, C.~M. and {Zhang}, W.~W.},
	Doi = {10.1088/0004-637X/791/2/81},
	Eid = {81},
	Eprint = {1406.3345},
	Journal = {\apj},
	Keywords = {galaxies: active, galaxies: individual: Circinus, galaxies: Seyfert, X-rays: galaxies},
	Month = aug,
	Pages = {81},
	Primaryclass = {astro-ph.HE},
	Title = {{The 2-79 keV X-Ray Spectrum of the Circinus Galaxy with NuSTAR, XMM-Newton, and Chandra: A Fully Compton-thick Active Galactic Nucleus}},
	Volume = 791,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/791/2/81}}

@inproceedings{arnaud96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
	Author = {{Arnaud}, K.~A.},
	Booktitle = {Astronomical Data Analysis Software and Systems V},
	Editor = {{Jacoby}, G.~H. and {Barnes}, J.},
	Pages = {17-20},
	Publisher = {ASP, San Francisco},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{XSPEC: The First Ten Years}},
	Volume = 101,
	Year = 1996}

@ARTICLE{arnett89,
   author = {{Arnett}, W.~D. and {Bahcall}, J.~N. and {Kirshner}, R.~P. and 
	{Woosley}, S.~E.},
    title = "{Supernova 1987A}",
  journal = {\araa},
 keywords = {Stellar Evolution, Supernova 1987a, Blue Stars, Gamma Ray Spectra, Light Curve, Metallicity, Neutrinos, Nuclear Fusion, Stellar Color, X Ray Spectra},
     year = 1989,
   volume = 27,
    pages = {629-700},
      doi = {10.1146/annurev.aa.27.090189.003213},
   adsurl = {http://adsabs.harvard.edu/abs/1989ARA%26A..27..629A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{arons93,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...403..249A},
	Author = {{Arons}, J. and {Tavani}, M.},
	Doi = {10.1086/172198},
	Journal = {\apj},
	Month = jan,
	Pages = {249-255},
	Title = {{High-energy emission from the eclipsing millisecond pulsar PSR 1957+20}},
	Volume = 403,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/172198}}

@inproceedings{arons05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ASPC..328...95A},
	Author = {{Arons}, J. and {Backer}, D.~C. and {Spitkovsky}, A. and {Kaspi}, V.~M.},
	Booktitle = {Binary Radio Pulsars},
	Editor = {{Rasio}, F.~A. and {Stairs}, I.~H.},
	Month = jul,
	Pages = {95},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{Probing Relativistic Winds: The Case of PSR J0737-3039 A and B}},
	Volume = 328,
	Year = 2005}

@article{arzoumanian94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994ApJ...422..671A&db_key=AST},
	Author = {{Arzoumanian}, Z. and {Nice}, D.~J. and {Taylor}, J.~H. and {Thorsett}, S.~E.},
	Journal = {\apj},
	Month = feb,
	Pages = {671-680},
	Title = {{Timing behavior of 96 radio pulsars}},
	Volume = 422,
	Year = 1994}

@article{asano05,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005astro.ph..3335A&db_key=PRE},
	Author = {{Asano}, K. and {Yamazaki}, R. and {Sugiyama}, N.},
	Eprint = {astro-ph/0503335},
	Journal = {ArXiv Astrophysics e-prints (astro-ph/0503335)},
	Month = mar,
	Title = {{Possibility of Ultra High-Energy Cosmic Rays from the Giant Flare in SGR 1806-20}},
	Year = 2005}

@article{aschenbach91,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1991RvMA....4..173A&db_key=AST},
	Author = {{Aschenbach}, B.},
	Journal = {Reviews of Modern Astronomy},
	Pages = {173-187},
	Title = {{First Results from the X-Ray Astronomy Mission ROSAT.}},
	Volume = 4,
	Year = 1991}

@article{aschenbach98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1998Natur.396..141A},
	Author = {{Aschenbach}, B.},
	Doi = {10.1038/24103},
	Journal = {\nat},
	Month = nov,
	Pages = {141-142},
	Title = {{Discovery of a young nearby supernova remnant}},
	Volume = 396,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/24103}}

@BOOK{aschwanden13,
    title = "{Self-Organized Criticality Systems}",
 keywords = {astrophysics },
editor = {M.J.~Aschwanden},
     year = 2013,
    month = jul,
publisher = {Open Academic Press, Berlin, Warsaw, 483pp.},
   adsurl = {http://adsabs.harvard.edu/abs/2013socs.book.....A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{asplund09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
	Archiveprefix = {arXiv},
	Author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.},
	Doi = {10.1146/annurev.astro.46.060407.145222},
	Eprint = {0909.0948},
	Journal = {\araa},
	Month = sep,
	Pages = {481-522},
	Primaryclass = {astro-ph.SR},
	Title = {{The Chemical Composition of the Sun}},
	Volume = 47,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.46.060407.145222}}

@article{atteia87,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1987ApJ...320L.105A&amp;db_key=AST},
	Author = {{Atteia}, J.-L. and {Boer}, M. and {Hurley}, K. and {Niel}, M. and {Vedrenne}, G. and {Fenimore}, E.~E. and {Klebesadel}, R.~W. and {Laros}, J.~G. and {Kuznetsov}, A.~V. and {Sunyaev}, R.~A. and {Terekhov}, O.~V. and {Kouveliotou}, C. and {Cline}, T. and {Dennis}, B. and {Desai}, U. and {Orwig}, L.},
	Journal = {\apjl},
	Month = sep,
	Pages = {L105-L110},
	Title = {{Localization, time histories, and energy spectra of a new type of recurrent high-energy transient source}},
	Volume = 320,
	Year = 1987}

@article{aungwerojwit12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758...79A},
	Archiveprefix = {arXiv},
	Author = {{Aungwerojwit}, A. and {G{\"a}nsicke}, B.~T. and {Wheatley}, P.~J. and {Pyrzas}, S. and {Staels}, B. and {Krajci}, T. and {Rodr{\'{\i}}guez-Gil}, P.},
	Doi = {10.1088/0004-637X/758/2/79},
	Eid = {79},
	Eprint = {1209.0719},
	Journal = {\apj},
	Keywords = {novae, cataclysmic variables, stars: individual: IPHAS J062746.41+014811.3},
	Month = oct,
	Pages = {79},
	Primaryclass = {astro-ph.SR},
	Title = {{IPHAS J062746.41+014811.3: A Deeply Eclipsing Intermediate Polar}},
	Volume = 758,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/758/2/79}}

@article{bachetti14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014Natur.514..202B},
	Archiveprefix = {arXiv},
	Author = {{Bachetti}, M. and {Harrison}, F.~A. and {Walton}, D.~J. and {Grefenstette}, B.~W. and {Chakrabarty}, D. and {F{\"u}rst}, F. and {Barret}, D. and {Beloborodov}, A. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Hailey}, C.~J. and {Hornschemeier}, A. and {Kaspi}, V. and {Kulkarni}, S.~R. and {Maccarone}, T. and {Miller}, J.~M. and {Rana}, V. and {Stern}, D. and {Tendulkar}, S.~P. and {Tomsick}, J. and {Webb}, N.~A. and {Zhang}, W.~W.},
	Doi = {10.1038/nature13791},
	Journal = {\nat},
	Month = oct,
	Pages = {202-204},
	Title = {{An ultraluminous X-ray source powered by an accreting neutron star}},
	Volume = 514,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature13791}}

@article{baganoff03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591..891B},
	Author = {{Baganoff}, F.~K. and {Maeda}, Y. and {Morris}, M. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Cui}, W. and {Doty}, J.~P. and {Feigelson}, E.~D. and {Garmire}, G.~P. and {Pravdo}, S.~H. and {Ricker}, G.~R. and {Townsley}, L.~K.},
	Doi = {10.1086/375145},
	Eprint = {arXiv:astro-ph/0102151},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Black Hole Physics, Galaxies: Active, Galaxy: Center, X-Rays: ISM, X-Rays: Stars},
	Month = jul,
	Pages = {891-915},
	Title = {{Chandra X-Ray Spectroscopic Imaging of Sagittarius A* and the Central Parsec of the Galaxy}},
	Volume = 591,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375145}}

@ARTICLE{bahramian17,
       author = {{Bahramian}, Arash and {Heinke}, Craig O. and {Tudor}, Vlad and
         {Miller-Jones}, James C.~A. and {Bogdanov}, Slavko and
         {Maccarone}, Thomas J. and {Knigge}, Christian and
         {Sivakoff}, Gregory R. and {Chomiuk}, Laura and {Strader}, Jay and
         {Garcia}, Javier A. and {Kallman}, Timothy},
        title = "{The ultracompact nature of the black hole candidate X-ray binary 47 Tuc X9}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, stars: Black holes, stars: neutron, globular clusters: individual: 47 Tuc, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = may,
       volume = {467},
       number = {2},
        pages = {2199-2216},
          doi = {10.1093/mnras/stx166},
archivePrefix = {arXiv},
       eprint = {1702.02167},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.467.2199B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bailer18,
       author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and
         {Mantelet}, G. and {Andrae}, R.},
        title = "{Estimating Distance from Parallaxes. IV. Distances to 1.33 Billion Stars in Gaia Data Release 2}",
      journal = {\aj},
     keywords = {catalogs, Galaxy: structure, methods: statistical, stars: distances, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {156},
       number = {2},
          eid = {58},
        pages = {58},
          doi = {10.3847/1538-3881/aacb21},
archivePrefix = {arXiv},
       eprint = {1804.10121},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156...58B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bak91,
   author = {{Bak}, P. and {Chen}, K.},
    title = "{Self-Organized Criticality}",
  journal = {Scientific American},
     year = 1991,
    month = jan,
   volume = 264,
    pages = {46-53},
      doi = {10.1038/scientificamerican0191-46},
   adsurl = {http://adsabs.harvard.edu/abs/1991SciAm.264a..46B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balega02,
       author = {{Balega}, I.~I. and {Balega}, Y.~Y. and {Hofmann}, K. -H. and
         {Maksimov}, A.~F. and {Pluzhnik}, E.~A. and {Schertl}, D. and
         {Shkhagosheva}, Z.~U. and {Weigelt}, G.},
        title = "{Speckle interferometry of nearby multiple stars}",
      journal = {\aap},
     keywords = {STARS: BINARIES: VISUAL, STARS: FUNDAMENTAL PARAMETERS, TECHNIQUES: INTERFEROMETRIC},
         year = "2002",
        month = "Apr",
       volume = {385},
        pages = {87-93},
          doi = {10.1051/0004-6361:20020005},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...385...87B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{balucinska92,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1992ApJ...400..699B},
	Author = {{Balucinska-Church}, M. and {McCammon}, D.},
	Doi = {10.1086/172032},
	Journal = {\apj},
	Month = dec,
	Pages = {699},
	Title = {{Photoelectric absorption cross sections with variable abundances}},
	Volume = 400,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/172032}}

@article{bamba07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007PASJ...59S.209B},
	Author = {{Bamba}, A. and {Koyama}, K. and {Hiraga}, J.~S. and {Hughes}, J.~P. and {Kohmura}, T. and {Kokubun}, M. and {Maeda}, Y. and {Matsumoto}, H. and {Senda}, A. and {Takahashi}, T. and {Tsuboi}, Y. and {Yamauchi}, S. and {Yuasa}, T.},
	Eprint = {arXiv:astro-ph/0608310},
	Journal = {\pasj},
	Month = jan,
	Pages = {209-214},
	Title = {{Discovery of a Possible X-Ray Counterpart to HESS J1804-216}},
	Volume = 59,
	Year = 2007}

@article{bandyopadhyay11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3502....1B},
	Author = {{Bandyopadhyay}, R.~M. and {Lucas}, P.~W. and {Maccarone}, T.},
	Journal = {Astron. Tel.},
	Keywords = {Infra-Red, X-ray, Binary, Neutron Star, Transient},
	Month = jul,
	Title = {{Search for an IR counterpart to the newly discovered transient Swift J11822.3-1606}},
	Volume = 3502,
	Year = 2011}

@ARTICLE{barat83,
   author = {{Barat}, C. and {Hayles}, R.~I. and {Hurley}, K. and {Niel}, M. and 
	{Vedrenne}, G. and {Desai}, U. and {Kurt}, V.~G. and {Zenchenko}, V.~M. and 
	{Estulin}, I.~V.},
    title = "{Fine time structure in the 1979 March 5 gamma ray burst}",
  journal = {\aap},
 keywords = {Fine Structure, Gamma Ray Bursts, Neutron Stars, Power Spectra, Prognoz Satellites, Stellar Oscillations, Stellar Rotation, Torsional Vibration, Venera Satellites},
     year = 1983,
    month = oct,
   volume = 126,
    pages = {400-402},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...126..400B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{barbon89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26AS...81..421B},
	Author = {{Barbon}, R. and {Cappellaro}, E. and {Turatto}, M.},
	Journal = {\aaps},
	Month = dec,
	Pages = {421},
	Title = {{The Asiago Supernova Catalogue}},
	Volume = 81,
	Year = 1989}

@article{barnard08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488..697B},
	Archiveprefix = {arXiv},
	Author = {{Barnard}, R. and {Clark}, J.~S. and {Kolb}, U.~C.},
	Doi = {10.1051/0004-6361:20077975},
	Eprint = {0807.0606},
	Journal = {\aap},
	Keywords = {X-rays: binaries, X-rays: general, galaxies: individual: NGC 300, galaxies: individual: IC 10},
	Month = sep,
	Pages = {697-703},
	Title = {{NGC 300 X-1 and IC 10 X-1: a new breed of black hole binary?}},
	Volume = 488,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077975}}

@article{barros07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.374.1334B},
	Author = {{Barros}, S.~C.~C. and {Marsh}, T.~R. and {Dhillon}, V.~S. and {Groot}, P.~J. and {Littlefair}, S. and {Nelemans}, G. and {Roelofs}, G. and {Steeghs}, D. and {Wheatley}, P.~J.},
	Doi = {10.1111/j.1365-2966.2006.11244.x},
	Eprint = {arXiv:astro-ph/0611117},
	Journal = {\mnras},
	Keywords = {astrometry, binaries: close, stars: individual: V407 Vul, stars: individual: HM Cnc, stars: magnetic fields, white dwarfs, X-rays: stars},
	Month = feb,
	Pages = {1334-1346},
	Title = {{ULTRACAM photometry of the ultracompact binaries V407 Vul and HM Cnc}},
	Volume = 374,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.11244.x}}

@article{bartko08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.1105B},
	Archiveprefix = {arXiv},
	Author = {{Bartko}, H. and {Bednarek}, W.},
	Doi = {10.1111/j.1365-2966.2008.12870.x},
	Eprint = {0712.2964},
	Journal = {\mnras},
	Keywords = {pulsars: general , ISM: individual: IC 443 , ISM: individual: W41 , supernova remnants , gamma-rays: theory},
	Month = apr,
	Pages = {1105-1109},
	Title = {{{$\gamma$}-ray emission from PWNe interacting with molecular clouds}},
	Volume = 385,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.12870.x}}

@article{bauer04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...601L..67B},
	Author = {{Bauer}, F.~E. and {Brandt}, W.~N.},
	Doi = {10.1086/380107},
	Eprint = {arXiv:astro-ph/0310039},
	Journal = {\apjl},
	Keywords = {Galaxies: Individual: Alphanumeric: IC 10, Stars: Wolf-Rayet, X-Rays: Binaries, X-Rays: ISM},
	Month = jan,
	Pages = {L67-L70},
	Title = {{Chandra and Hubble Space Telescope Confirmation of the Luminous and Variable X-Ray Source IC 10 X-1 as a Possible Wolf-Rayet, Black Hole Binary}},
	Volume = 601,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/380107}}

@article{baykal06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2006MNRAS.369.1760B&db_key=AST},
	Author = {{Baykal}, A. and {{\.I}nam}, S.~{\c C}. and {Beklen}, E.},
	Doi = {10.1111/j.1365-2966.2006.10412.x},
	Eprint = {astro-ph/0512176},
	Journal = {\mnras},
	Month = jul,
	Pages = {1760-1764},
	Title = {{Evidence of a change in the long-term spin-down rate of the X-ray pulsar 4U 1907+09}},
	Volume = 369,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10412.x}}

@article{baring01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...547..929B&db_key=AST},
	Author = {{Baring}, M.~G. and {Harding}, A.~K.},
	Journal = {\apj},
	Month = feb,
	Pages = {929-948},
	Title = {{Photon Splitting and Pair Creation in Highly Magnetized Pulsars}},
	Volume = 547,
	Year = 2001}

@article{barnard12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.3937....1B},
	Author = {{Barnard}, R. and {Garcia}, M.~R. and {Murray}, S.~S.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Binary, Black Hole, Transient},
	Month = feb,
	Title = {{A Chandra/ACIS observation of the transient M31 ULX XMMU J004243.6+412519}},
	Volume = 3937,
	Year = 2012}

@article{barthelmy05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005SSRv..120..143B},
	Author = {{Barthelmy}, S.~D. and {Barbier}, L.~M. and {Cummings}, J.~R. and {Fenimore}, E.~E. and {Gehrels}, N. and {Hullinger}, D. and {Krimm}, H.~A. and {Markwardt}, C.~B. and {Palmer}, D.~M. and {Parsons}, A. and {Sato}, G. and {Suzuki}, M. and {Takahashi}, T. and {Tashiro}, M. and {Tueller}, J.},
	Doi = {10.1007/s11214-005-5096-3},
	Eprint = {arXiv:astro-ph/0507410},
	Journal = {Space Science Reviews},
	Keywords = {gamma-ray, GRB, hard X-ray, survey, burst, afterglow, CZT, coded aperture, astrophysics, cosmology},
	Month = oct,
	Pages = {143-164},
	Title = {{The Burst Alert Telescope (BAT) on the SWIFT Midex Mission}},
	Volume = 120,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-005-5096-3}}

@article{barthelmy10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010GCN.10528....1B},
	Author = {{Barthelmy}, S.~D. and {Sakamoto}, T. and {Baumgartner}, W.~H. and {Cummings}, J.~R. and {Gehrels}, N. and {Gelbord}, J.~M. and {Krimm}, H.~A. and {Markwardt}, C.~B. and {Palmer}, D.~M. and {Stamatikos}, M. and {Tueller}, J. and {Ukwatta}, T.~N.},
	Journal = {GCN Circ.},
	Title = {{Swift-BAT refined analysis of the probable new Sgr 1833-0832.}},
	Volume = 10528,
	Year = 2010}

@article{bauer01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122..182B},
	Author = {{Bauer}, F.~E. and {Brandt}, W.~N. and {Sambruna}, R.~M. and {Chartas}, G. and {Garmire}, G.~P. and {Kaspi}, S. and {Netzer}, H.},
	Doi = {10.1086/321123},
	Eprint = {astro-ph/0104035},
	Journal = {\aj},
	Keywords = {Galaxies: Active, Galaxies: Individual: Name: Circinus, X-Rays},
	Month = jul,
	Pages = {182-193},
	Title = {{A Chandra Study of the Circinus Galaxy Point-Source Population}},
	Volume = 122,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321123}}

@article{bauer08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...688.1210B},
	Archiveprefix = {arXiv},
	Author = {{Bauer}, F.~E. and {Dwarkadas}, V.~V. and {Brandt}, W.~N. and {Immler}, S. and {Smartt}, S. and {Bartel}, N. and {Bietenholz}, M.~F.},
	Doi = {10.1086/589761},
	Eprint = {0804.3597},
	Journal = {\apj},
	Keywords = {Stars: Circumstellar Matter, Stars: Supernovae: General, supernovae: individual (SN 1996cr), X-rays: individual (SN 1996cr)},
	Month = dec,
	Pages = {1210-1234},
	Title = {{Supernova 1996cr: SN 1987A's Wild Cousin?}},
	Volume = 688,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/589761}}

@ARTICLE{baumgartner13,
   author = {{Baumgartner}, W.~H. and {Tueller}, J. and {Markwardt}, C.~B. and 
	{Skinner}, G.~K. and {Barthelmy}, S. and {Mushotzky}, R.~F. and 
	{Evans}, P.~A. and {Gehrels}, N.},
    title = "{The 70 Month Swift-BAT All-sky Hard X-Ray Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1212.3336},
 primaryClass = "astro-ph.HE",
 keywords = {catalogs, surveys, X-rays: general},
     year = 2013,
    month = aug,
   volume = 207,
      eid = {19},
    pages = {19},
      doi = {10.1088/0067-0049/207/2/19},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..207...19B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bayless10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...709..251B},
	Archiveprefix = {arXiv},
	Author = {{Bayless}, A.~J. and {Robinson}, E.~L. and {Hynes}, R.~I. and {Ashcraft}, T.~A. and {Cornell}, M.~E.},
	Doi = {10.1088/0004-637X/709/1/251},
	Eprint = {0911.4492},
	Journal = {\apj},
	Keywords = {binaries: eclipsing, pulsars: individual: 4U 1822{\ndash}371, X-rays: binaries},
	Month = jan,
	Pages = {251-262},
	Primaryclass = {astro-ph.HE},
	Title = {{The Structure of the Accretion Disk in the Accretion Disk Corona X-ray Binary 4U 1822-371 at Optical and Ultraviolet Wavelengths}},
	Volume = 709,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/709/1/251}}

@ARTICLE{baym69,
   author = {{Baym}, G. and {Pethick}, C. and {Pines}, D.},
    title = "{Superfluidity in Neutron Stars}",
  journal = {\nat},
     year = 1969,
    month = nov,
   volume = 224,
    pages = {673-674},
      doi = {10.1038/224673a0},
   adsurl = {http://adsabs.harvard.edu/abs/1969Natur.224..673B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{beardmore00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315..307B},
	Author = {{Beardmore}, A.~P. and {Osborne}, J.~P. and {Hellier}, C.},
	Doi = {10.1046/j.1365-8711.2000.03477.x},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, STARS: INDIVIDUAL: V1223 SGR, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
	Month = jun,
	Pages = {307-315},
	Title = {{The multi-temperature X-ray spectrum of the intermediate polar V1223 Sagittarii}},
	Volume = 315,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03477.x}}

@article{becker97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...326..682B&db_key=AST},
	Author = {{Becker}, W. and {Truemper}, J.},
	Eprint = {astro-ph/9708169},
	Journal = {\aap},
	Month = oct,
	Pages = {682-691},
	Title = {{The X-ray luminosity of rotation-powered neutron stars.}},
	Volume = 326,
	Year = 1997}

@article{becker99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...341..803B},
	Author = {{Becker}, W. and {Tr{\"u}mper}, J.},
	Eprint = {arXiv:astro-ph/9806381},
	Journal = {\aap},
	Month = jan,
	Pages = {803-817},
	Title = {{The X-ray emission properties of millisecond pulsars}},
	Volume = 341,
	Year = 1999}

@inproceedings{becker02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002nsps.conf...64B},
	Author = {{Becker}, W. and {Aschenbach}, B.},
	Booktitle = {{Becker} W., {Lesch} H., \& {Tr{\"u}mper} J., eds., Proc. of the 270 WE-Heraeus Seminar, Neutron Stars, Pulsars, and Supernova Remnants},
	Eprint = {arXiv:astro-ph/0208466},
	Pages = {64-86},
	Series = {MPE Report, Garching},
	Title = {{X-ray Observations of Neutron Stars and Pulsars: First Results from XMM-Newton}},
	Volume = 278,
	Year = 2002}

@article{becker06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006astro.ph..7081B},
	Author = {{Becker}, W. and {Hui}, C.~Y. and {Aschenbach}, B. and {Iyudin}, A.},
	Journal = {preprint (astro-ph/0607081)},
	Month = jul,
	Title = {{Exploring the Central Compact Object in the RX J0852.0-4622 Supernova Remnant with XMM-Newton}},
	Year = 2006}

@article{becker07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654..435B},
	Author = {{Becker}, P.~A. and {Wolff}, M.~T.},
	Doi = {10.1086/509108},
	Eprint = {arXiv:astro-ph/0609035},
	Journal = {\apj},
	Keywords = {Methods: Analytical, Stars: Pulsars: General, Radiation Mechanisms: Nonthermal, Shock Waves, Stars: Neutron, X-Rays: Stars},
	Month = jan,
	Pages = {435-457},
	Title = {{Thermal and Bulk Comptonization in Accretion-powered X-Ray Pulsars}},
	Volume = 654,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/509108}}

@article{begelman02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...568L..97B},
	Author = {{Begelman}, M.~C.},
	Doi = {10.1086/340457},
	Eprint = {arXiv:astro-ph/0203030},
	Journal = {\apjl},
	Keywords = {Accretion, Accretion Disks, Black Hole Physics, Hydrodynamics, Magnetohydrodynamics: MHD, X-Rays: Binaries},
	Month = apr,
	Pages = {L97-L100},
	Title = {{Super-Eddington Fluxes from Thin Accretion Disks?}},
	Volume = 568,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340457}}

@article{begelman06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370..399B},
	Author = {{Begelman}, M.~C. and {King}, A.~R. and {Pringle}, J.~E.},
	Doi = {10.1111/j.1365-2966.2006.10469.x},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs: black hole physics: X-rays: binaries, accretion discs, black hole physics, X-rays: binaries},
	Month = jul,
	Pages = {399-404},
	Title = {{The nature of SS433 and the ultraluminous X-ray sources}},
	Volume = 370,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10469.x}}

@article{belczynski10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714.1217B},
	Archiveprefix = {arXiv},
	Author = {{Belczynski}, K. and {Bulik}, T. and {Fryer}, C.~L. and {Ruiter}, A. and {Valsecchi}, F. and {Vink}, J.~S. and {Hurley}, J.~R.},
	Doi = {10.1088/0004-637X/714/2/1217},
	Eprint = {0904.2784},
	Journal = {\apj},
	Keywords = {binaries: close, black hole physics, gravitational waves, stars: evolution, stars: neutron},
	Month = may,
	Pages = {1217-1226},
	Primaryclass = {astro-ph.SR},
	Title = {{On the Maximum Mass of Stellar Black Holes}},
	Volume = 714,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/2/1217}}

@article{belczynski13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...764...96B},
	Archiveprefix = {arXiv},
	Author = {{Belczynski}, K. and {Bulik}, T. and {Mandel}, I. and {Sathyaprakash}, B.~S. and {Zdziarski}, A.~A. and {Miko{\l}ajewska}, J.},
	Doi = {10.1088/0004-637X/764/1/96},
	Eid = {96},
	Eprint = {1209.2658},
	Journal = {\apj},
	Keywords = {binaries: general, stars: neutron, X-rays: binaries},
	Month = feb,
	Pages = {96},
	Primaryclass = {astro-ph.HE},
	Title = {{Cyg X-3: A Galactic Double Black Hole or Black-hole-Neutron-star Progenitor}},
	Volume = 764,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/764/1/96}}

@article{belloni11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011BASI...39..409B},
	Archiveprefix = {arXiv},
	Author = {{Belloni}, T.~M. and {Motta}, S.~E. and {Mu{\~n}oz-Darias}, T.},
	Eprint = {1109.3388},
	Journal = {Bulletin of the Astronomical Society of India},
	Keywords = {accretion, accretion discs, black hole physics, X-rays: binaries},
	Month = sep,
	Pages = {409-428},
	Primaryclass = {astro-ph.HE},
	Title = {{Black hole transients}},
	Volume = 39,
	Year = 2011}

@article{beloborodov02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...566L..85B},
	Author = {{Beloborodov}, A.~M.},
	Doi = {10.1086/339511},
	Eprint = {arXiv:astro-ph/0201117},
	Journal = {\apjl},
	Keywords = {Gravitation, Stars: Pulsars: General, Radiation Mechanisms: General, Relativity, Stars: Neutron, X-Rays: Binaries},
	Month = feb,
	Pages = {L85-L88},
	Title = {{Gravitational Bending of Light Near Compact Objects}},
	Volume = 566,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/339511}}

@article{beloborodov07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...657..967B},
	Author = {{Beloborodov}, A.~M. and {Thompson}, C.},
	Doi = {10.1086/508917},
	Eprint = {arXiv:astro-ph/0602417},
	Journal = {\apj},
	Month = mar,
	Pages = {967-993},
	Title = {{Corona of Magnetars}},
	Volume = 657,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/508917}}

@ARTICLE{beloborodov13,
   author = {{Beloborodov}, A.~M.},
    title = "{On the Mechanism of Hard X-Ray Emission from Magnetars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.0664},
 primaryClass = "astro-ph.HE",
 keywords = {plasmas, stars: magnetic field, stars: neutron},
     year = 2013,
    month = jan,
   volume = 762,
      eid = {13},
    pages = {13},
      doi = {10.1088/0004-637X/762/1/13},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...762...13B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{b13,
   author = {{Beloborodov}, A.~M.},
    title = "{Electron-Positron Flows around Magnetars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.4063},
 primaryClass = "astro-ph.HE",
 keywords = {plasmas, stars: magnetic field, stars: neutron },
     year = 2013,
    month = nov,
   volume = 777,
      eid = {114},
    pages = {114},
      doi = {10.1088/0004-637X/777/2/114},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...777..114B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{berghea08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687..471B},
	Archiveprefix = {arXiv},
	Author = {{Berghea}, C.~T. and {Weaver}, K.~A. and {Colbert}, E.~J.~M. and {Roberts}, T.~P.},
	Doi = {10.1086/591722},
	Eprint = {0807.1547},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Galaxies: General, Surveys, X-Rays: Binaries},
	Month = nov,
	Pages = {471-487},
	Title = {{Testing the Paradigm that Ultraluminous X-Ray Sources as a Class Represent Accreting Intermediate-Mass Black Holes}},
	Volume = 687,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591722}}

@phdthesis{berghea09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009PhDT.........8B},
	Author = {{Berghea}, C.~T.},
	Keywords = {Ultraluminous X-ray sources, Intermediate-mass black holes, Accretion discs, Black holes},
	Month = June,
	School = {The Catholic University of America; Washington, DC},
	Title = {{Ultraluminous X-ray sources and their environment}},
	Year = 2009}

@article{beri14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.1940B},
	Archiveprefix = {arXiv},
	Author = {{Beri}, A. and {Jain}, C. and {Paul}, B. and {Raichur}, H.},
	Doi = {10.1093/mnras/stu087},
	Eprint = {1401.2936},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, pulsars: individual: 4U 1626-67},
	Month = apr,
	Pages = {1940-1947},
	Primaryclass = {astro-ph.HE},
	Title = {{Torque reversals and pulse profile of the pulsar 4U 1626-67}},
	Volume = 439,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu087}}

@article{bernardini09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...498..195B},
	Archiveprefix = {arXiv},
	Author = {{Bernardini}, F. and {Israel}, G.~L. and {Dall'Osso}, S. and {Stella}, L. and {Rea}, N. and {Zane}, S. and {Turolla}, R. and {Perna}, R. and {Falanga}, M. and {Campana}, S. and {G{\"o}tz}, D. and {Mereghetti}, S. and {Tiengo}, A.},
	Doi = {10.1051/0004-6361/200810779},
	Eprint = {0901.2241},
	Journal = {\aap},
	Keywords = {moon, stars: magnetic fields, stars: neutron, X-rays: stars},
	Month = apr,
	Pages = {195-207},
	Title = {{From outburst to quiescence: the decay of the transient AXP XTE J1810-197}},
	Volume = 498,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200810779}}

@article{bernardini11,
	Author = {{Bernardini}, F. and {Israel}, G.~L. and {Stella}, L. and {Turolla}, R. and {Esposito}, P. and {Rea}, N. and {Zane}, S. and {Tiengo}, A. and {Campana}, S. and {G\"otz}, D. and {Mereghetti}, S. and {Romano}, P.},
	Doi = {10.1051/0004-6361/201016197},
	Journal = {\aap},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = may,
	Pages = {A19},
	Title = {{Multi-instrument X-ray monitoring of the January 2009 outburst from the recurrent magnetar candidate 1E 1547.0-5408}},
	Volume = 529,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201016197}}

@article{bernardini12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...542A..22B},
	Archiveprefix = {arXiv},
	Author = {{Bernardini}, F. and {de Martino}, D. and {Falanga}, M. and {Mukai}, K. and {Matt}, G. and {Bonnet-Bidaud}, J.-M. and {Masetti}, N. and {Mouchet}, M.},
	Doi = {10.1051/0004-6361/201219233},
	Eid = {A22},
	Eprint = {1204.3758},
	Journal = {\aap},
	Keywords = {binaries: close, X-rays: binaries, accretion, accretion disks, novae, cataclysmic variables},
	Month = jun,
	Pages = {A22},
	Primaryclass = {astro-ph.HE},
	Title = {{Characterization of new hard X-ray cataclysmic variables}},
	Volume = 542,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201219233}}

@article{bernardini14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.tmpL..12B},
	Archiveprefix = {arXiv},
	Author = {{Bernardini}, M.~G. and {Campana}, S. and {Ghisellini}, G. and {D'Avanzo}, P. and {Calderone}, G. and {Covino}, S. and {Cusumano}, G. and {Ghirlanda}, G. and {La Parola}, V. and {Maselli}, A. and {Melandri}, A. and {Salvaterra}, R. and {Burlon}, D. and {D'Elia}, V. and {Fugazza}, D. and {Sbarufatti}, B. and {Vergani}, S.~D. and {Tagliaferri}, G.},
	Doi = {10.1093/mnrasl/slu003},
	Eprint = {1401.1972},
	Journal = {\mnras, in press (DOI: 10.1093/mnrasl/slu003)},
	Keywords = {gamma-ray bursts: individual: GRB 130427A, stars: magnetars},
	Month = jan,
	Primaryclass = {astro-ph.HE},
	Title = {{A magnetar powering the ordinary monster GRB 130427A?}},
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnrasl/slu003}}

@article{bertin96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..117..393B},
	Author = {{Bertin}, E. and {Arnouts}, S.},
	Doi = {10.1051/aas:1996164},
	Journal = {\aaps},
	Keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
	Month = jun,
	Pages = {393-404},
	Title = {{SExtractor: Software for source extraction.}},
	Volume = 117,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/aas:1996164}}

@inproceedings{bertin02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ASPC..281..228B},
	Author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and {Didelon}, P. and {Morin}, B.},
	Booktitle = {Astronomical Data Analysis Software and Systems XI},
	Editor = {{D.~A.~Bohlender, D.~Durand, \& T.~H.~Handley}},
	Keywords = {astronomy: optical, astronomy: software, pipelines: data reduction, software: package, software: development, software: data analysis, data analysis, databases, distributed processing},
	Pages = {228},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{The TERAPIX Pipeline}},
	Volume = 281,
	Year = 2002}

@article{bertotti69,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1969Natur.221..624B&db_key=AST},
	Author = {{Bertotti}, B. and {Cavaliere}, A. and {Pacini}, F.},
	Journal = {\nat},
	Month = feb,
	Pages = {624},
	Title = {{Rotating Neutron Stars and Pulsar Emission}},
	Volume = 221,
	Year = 1969}

@article{beuermann99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...347...47B},
	Author = {{Beuermann}, K. and {Thomas}, {H.-C.} and {Reinsch}, K. and {Schwope}, A.~D. and {Tr{\"u}mper}, J. and {Voges}, W.},
	Journal = {\aap},
	Keywords = {STARS: NOVAE, CATACLYSMIC VARIABLES, GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: QUASARS: GENERAL, GALAXIES: SEYFERT, X-RAYS: GENERAL},
	Month = jul,
	Pages = {47-54},
	Title = {{Identification of soft high galactic latitude RASS X-ray sources. II. Sources with PSPC count rate CR {\lt}0.5 cts/s}},
	Volume = 347,
	Year = 1999}

@book{bevington69,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1969drea.book.....B},
	Author = {{Bevington}, P.~R.},
	Publisher = {New York: McGraw-Hill, 1969},
	Title = {{Data reduction and error analysis for the physical sciences}},
	Year = 1969}

@book{bevington92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992drea.book.....B},
	Author = {{Bevington}, P.~R. and {Robinson}, D.~K.},
	Publisher = {New York: McGraw-Hill, 1992, 2nd ed.},
	Title = {{Data reduction and error analysis for the physical sciences}},
	Year = 1992}

@article{bhadkamkar09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...506.1297B},
	Archiveprefix = {arXiv},
	Author = {{Bhadkamkar}, H. and {Ghosh}, P.},
	Doi = {10.1051/0004-6361/200912552},
	Eprint = {0909.0159},
	Journal = {\aap},
	Keywords = {X-rays: binaries, stars: neutron, stars: evolution, accretion, accretion disks, ISM: supernova remnants, X-rays: general},
	Month = nov,
	Pages = {1297-1307},
	Primaryclass = {astro-ph.SR},
	Title = {{Young pre-low-mass X-ray binaries in the propeller phase. Nature of the 6.7-h periodic X-ray source 1E 161348-5055 in RCW 103}},
	Volume = 506,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200912552}}

@article{bianchi02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...396..793B},
	Author = {{Bianchi}, S. and {Matt}, G. and {Fiore}, F. and {Fabian}, A.~C. and {Iwasawa}, K. and {Nicastro}, F.},
	Doi = {10.1051/0004-6361:20021414},
	Eprint = {astro-ph/0209583},
	Journal = {\aap},
	Keywords = {galaxies: individual: Circinus, galaxies: Seyfert, X-rays: galaxies, X-rays: individuals: CG X-1, X-rays: individuals: CG X-2},
	Month = dec,
	Pages = {793-799},
	Title = {{Flux and spectral variations in the Circinus Galaxy}},
	Volume = 396,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20021414}}

@article{bignami81,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...247L..85B&db_key=AST},
	Author = {{Bignami}, G.~F. and {Caraveo}, P.~A. and {Lamb}, R.~C. and {Markert}, T.~H. and {Paul}, J.~A.},
	Doi = {10.1086/183595},
	Journal = {\apjl},
	Month = jul,
	Pages = {L85-L88},
	Title = {{Einstein X-ray identification of the variable radio star LSI plus 61 deg 303}},
	Volume = 247,
	Year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/183595}}

@article{bignami83,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ARA%26A..21...67B},
	Author = {{Bignami}, G.~F. and {Hermsen}, W.},
	Doi = {10.1146/annurev.aa.21.090183.000435},
	Journal = {\araa},
	Pages = {67-108},
	Title = {{Galactic gamma-ray sources}},
	Volume = 21,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.21.090183.000435}}

@article{bildsten97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJS..113..367B},
	Author = {{Bildsten}, L. and {Chakrabarty}, D. and {Chiu}, J. and {Finger}, M.~H. and {Koh}, D.~T. and {Nelson}, R.~W. and {Prince}, T.~A. and {Rubin}, B.~C. and {Scott}, D.~M. and {Stollberg}, M. and {Vaughan}, B.~A. and {Wilson}, C.~A. and {Wilson}, R.~B.},
	Doi = {10.1086/313060},
	Eprint = {astro-ph/9707125},
	Journal = {\apjs},
	Keywords = {ACCRETION, ACCRETION DISKS, STARS: BINARIES: CLOSE, STARS: PULSARS: GENERAL, STARS: MAGNETIC FIELDS, X-RAYS: STARS, Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Pulsars: General, Stars: Magnetic Fields, Stars: Neutron, X-rays: stars},
	Month = dec,
	Pages = {367-408},
	Title = {{Observations of Accreting Pulsars}},
	Volume = 113,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/313060}}

@article{bilir08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1569B},
	Archiveprefix = {arXiv},
	Author = {{Bilir}, S. and {Karaali}, S. and {Ak}, S. and {Yaz}, E. and {Cabrera-Lavers}, A. and {Co{\c s}kuno{\v g}lu}, K.~B.},
	Doi = {10.1111/j.1365-2966.2008.13839.x},
	Eprint = {0808.1848},
	Journal = {\mnras},
	Keywords = {stars: distances , Galaxy: disc , solar neighbourhood},
	Month = nov,
	Pages = {1569-1576},
	Title = {{Luminosity-colour relations for thin-disc main-sequence stars}},
	Volume = 390,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13839.x}}
	
@ARTICLE{bionta87,
   author = {{Bionta}, R.~M. and {Blewitt}, G. and {Bratton}, C.~B. and {Casper}, D. and 
	{Ciocio}, A.},
    title = "{Observation of a neutrino burst in coincidence with supernova 1987A in the Large Magellanic Cloud}",
  journal = {Physical Review Letters},
 keywords = {Magellanic Clouds, Neutrinos, Supernova 1987a, Cerenkov Radiation, Radiation Detectors, Underground Structures},
     year = 1987,
    month = apr,
   volume = 58,
    pages = {1494-1496},
      doi = {10.1103/PhysRevLett.58.1494},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhRvL..58.1494B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bird10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186....1B},
	Archiveprefix = {arXiv},
	Author = {{Bird}, A.~J. and {Bazzano}, A. and {Bassani}, L. and {Capitanio}, F. and {Fiocchi}, M. and {Hill}, A.~B. and {Malizia}, A. and {McBride}, V.~A. and {Scaringi}, S. and {Sguera}, V. and {Stephen}, J.~B. and {Ubertini}, P. and {Dean}, A.~J. and {Lebrun}, F. and {Terrier}, R. and {Renaud}, M. and {Mattana}, F. and {G{\"o}tz}, D. and {Rodriguez}, J. and {Belanger}, G. and {Walter}, R. and {Winkler}, C.},
	Doi = {10.1088/0067-0049/186/1/1},
	Eprint = {0910.1704},
	Journal = {\apjs},
	Keywords = {Galaxy: general, gamma rays: observations, surveys},
	Month = jan,
	Pages = {1-9},
	Primaryclass = {astro-ph.HE},
	Title = {{The Fourth IBIS/ISGRI Soft Gamma-ray Survey Catalog}},
	Volume = 186,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/1/1}}

@article{bisnovatyi91,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...245..528B},
	Author = {{Bisnovatyi-Kogan}, G.~S.},
	Journal = {\aap},
	Keywords = {PULSARS, STELLAR ROTATION, X RAY BINARIES, STELLAR MAGNETOSPHERES, STELLAR WINDS},
	Month = may,
	Pages = {528-530},
	Title = {{Rotational equilibrium of long-periodic X-ray pulsars}},
	Volume = 245,
	Year = 1991}

@inproceedings{blackburn95,
	Author = {{Blackburn}, J.~K.},
	Booktitle = {{Shaw}, R.~A. and {Payne}, H.~E. and {Hayes}, J.~J.~E., eds., Astronomical Data Analysis Software and Systems IV.},
	Pages = {367},
	Series = {ASP Conf. Ser., (San Francisco, CA: ASP)},
	Title = {{FTOOLS: A FITS Data Processing and Analysis Software Package}},
	Volume = 77,
	Year = 1995}

@article{blandford76,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...205..580B},
	Author = {{Blandford}, R. and {Teukolsky}, S.~A.},
	Journal = {\apj},
	Month = apr,
	Pages = {580-591},
	Title = {{Arrival-time analysis for a pulsar in a binary system.}},
	Volume = 205,
	Year = 1976}

@article{blandford77,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1977MNRAS.179..433B&db_key=AST},
	Author = {{Blandford}, R.~D. and {Znajek}, R.~L.},
	Journal = {\mnras},
	Month = may,
	Pages = {433-456},
	Title = {{Electromagnetic extraction of energy from Kerr black holes}},
	Volume = 179,
	Year = 1977}

@article{blandford82,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.199..883B&db_key=AST},
	Author = {{Blandford}, R.~D. and {Payne}, D.~G.},
	Journal = {\mnras},
	Month = jun,
	Pages = {883-903},
	Title = {{Hydromagnetic flows from accretion discs and the production of radio jets}},
	Volume = 199,
	Year = 1982}

@ARTICLE{blinnikov00,
   author = {{Blinnikov}, S. and {Lundqvist}, P. and {Bartunov}, O. and {Nomoto}, K. and 
	{Iwamoto}, K.},
    title = "{Radiation Hydrodynamics of SN 1987A. I. Global Analysis of the Light Curve for the First 4 Months}",
  journal = {\apj},
   eprint = {astro-ph/9911205},
 keywords = {HYDRODYNAMICS, RADIATIVE TRANSFER, SCATTERING, SHOCK WAVES, STARS: INTERIORS, SUPERNOVAE: INDIVIDUAL (SN 1987A)},
     year = 2000,
    month = apr,
   volume = 532,
    pages = {1132-1149},
      doi = {10.1086/308588},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...532.1132B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{blondin90,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..591B},
	Author = {{Blondin}, J.~M. and {Kallman}, T.~R. and {Fryxell}, B.~A. and {Taam}, R.~E.},
	Doi = {10.1086/168865},
	Journal = {\apj},
	Keywords = {Hydrodynamics, Stellar Mass Accretion, Stellar Winds, X Ray Binaries, Black Holes (Astronomy), Neutron Stars, O Stars, Photoionization, Stellar Gravitation, Stellar Luminosity},
	Month = jun,
	Pages = {591-608},
	Title = {{Hydrodynamic simulations of stellar wind disruption by a compact X-ray source}},
	Volume = 356,
	Year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/168865}}

@ARTICLE{blum16,
   author = {{Blum}, K. and {Kushnir}, D.},
    title = "{Neutrino Signal of Collapse-induced Thermonuclear Supernovae: The Case for Prompt Black Hole Formation in SN 1987A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1601.03422},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, stars: black holes, supernovae: general, 95.35.+d, 98.35.Gi},
     year = 2016,
    month = sep,
   volume = 828,
      eid = {31},
    pages = {31},
      doi = {10.3847/0004-637X/828/1/31},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...828...31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bochanski11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AJ....141...98B},
	Archiveprefix = {arXiv},
	Author = {{Bochanski}, J.~J. and {Hawley}, S.~L. and {West}, A.~A.},
	Doi = {10.1088/0004-6256/141/3/98},
	Eid = {98},
	Eprint = {1101.3549},
	Journal = {\aj},
	Keywords = {Galaxy: kinematics and dynamics, methods: statistical, solar neighborhood, stars: fundamental parameters, stars: kinematics and dynamics, stars: low-mass},
	Month = mar,
	Pages = {98},
	Primaryclass = {astro-ph.SR},
	Title = {{The Sloan Digital Sky Survey Data Release 7 Spectroscopic M Dwarf Catalog. II. Statistical Parallax Analysis}},
	Volume = 141,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/141/3/98}}

@article{boella97,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997A%26AS..122..299B&db_key=AST},
	Author = {{Boella}, G. and {Butler}, R.~C. and {Perola}, G.~C. and {Piro}, L. and {Scarsi}, L. and {Bleeker}, J.~A.~M.},
	Journal = {\aaps},
	Month = apr,
	Pages = {299-307},
	Title = {{BeppoSAX, the wide band mission for X-ray astronomy}},
	Volume = 122,
	Year = 1997}

@article{boella97_mecs,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26AS..122..327B&db_key=AST},
	Author = {{Boella}, G. and {Chiappetti}, L. and {Conti}, G. and {Cusumano}, G. and {del Sordo}, S. and {La Rosa}, G. and {Maccarone}, M.~C. and {Mineo}, T. and {Molendi}, S. and {Re}, S. and {Sacco}, B. and {Tripiciano}, M.},
	Journal = {\aaps},
	Month = apr,
	Pages = {327-340},
	Title = {{The medium-energy concentrator spectrometer on board the BeppoSAX X-ray astronomy satellite}},
	Volume = 122,
	Year = 1997}

@article{boggs05,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005GCN..2936....1B&db_key=AST},
	Author = {{Boggs}, S. and {Hurley}, K. and {Smith}, D.~M. and {Lin}, R.~P. and {Hurford}, G. and {Hajdas}, W. and {Wigger}, C.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR 1806-20, RHESSI observations of the 041227 giant flare.}},
	Volume = 2936,
	Year = 2005}

@article{boggs07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...661..458B},
	Author = {{Boggs}, S.~E. and {Zoglauer}, A. and {Bellm}, E. and {Hurley}, K. and {Lin}, R.~P. and {Smith}, D.~M. and {Wigger}, C. and {Hajdas}, W.},
	Doi = {10.1086/516732},
	Eprint = {arXiv:astro-ph/0611318},
	Journal = {\apj},
	Month = may,
	Pages = {458-467},
	Title = {{The Giant Flare of 2004 December 27 from SGR 1806-20}},
	Volume = 661,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/516732}}

@ARTICLE{boggs15,
   author = {{Boggs}, S.~E. and {Harrison}, F.~A. and {Miyasaka}, H. and 
	{Grefenstette}, B.~W. and {Zoglauer}, A. and {Fryer}, C.~L. and 
	{Reynolds}, S.~P. and {Alexander}, D.~M. and {An}, H. and {Barret}, D. and 
	{Christensen}, F.~E. and {Craig}, W.~W. and {Forster}, K. and 
	{Giommi}, P. and {Hailey}, C.~J. and {Hornstrup}, A. and {Kitaguchi}, T. and 
	{Koglin}, J.~E. and {Madsen}, K.~K. and {Mao}, P.~H. and {Mori}, K. and 
	{Perri}, M. and {Pivovaroff}, M.~J. and {Puccetti}, S. and {Rana}, V. and 
	{Stern}, D. and {Westergaard}, N.~J. and {Zhang}, W.~W.},
    title = "{$^{44}$Ti gamma-ray emission lines from SN1987A reveal an asymmetric explosion}",
  journal = {Science},
     year = 2015,
    month = may,
   volume = 348,
    pages = {670-671},
      doi = {10.1126/science.aaa2259},
   adsurl = {http://adsabs.harvard.edu/abs/2015Sci...348..670B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bondi52,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1952MNRAS.112..195B},
	Author = {{Bondi}, H.},
	Journal = {\mnras},
	Pages = {195},
	Title = {{On spherically symmetrical accretion}},
	Volume = 112,
	Year = 1952}

@article{borkowski04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2920....1B&db_key=AST},
	Author = {{Borkowski}, J. and {G{\"o}tz}, D. and {Mereghetti}, S. and {Mowlavi}, N. and {Shaw}, S. and {Turler}, M.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Giant flare from Sgr 1806-20 detected by INTEGRAL.}},
	Volume = 2920,
	Year = 2004}

@article{bosch05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...628..388B},
	Author = {{Bosch-Ramon}, V. and {Paredes}, J.~M. and {Rib{\'o}}, M. and {Miller}, J.~M. and {Reig}, P. and {Mart{\'{\i}}}, J.},
	Doi = {10.1086/429901},
	Eprint = {arXiv:astro-ph/0507412},
	Journal = {\apj},
	Month = jul,
	Pages = {388-394},
	Title = {{Orbital X-Ray Variability of the Microquasar LS 5039}},
	Volume = 628,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429901}}

@article{boshkayev13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...762..117B},
	Archiveprefix = {arXiv},
	Author = {{Boshkayev}, K. and {Rueda}, J.~A. and {Ruffini}, R. and {Siutsou}, I.},
	Doi = {10.1088/0004-637X/762/2/117},
	Eid = {117},
	Eprint = {1204.2070},
	Journal = {\apj},
	Keywords = {dense matter, instabilities, stars: rotation, white dwarfs},
	Month = jan,
	Pages = {117},
	Primaryclass = {astro-ph.SR},
	Title = {{On General Relativistic Uniformly Rotating White Dwarfs}},
	Volume = 762,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/762/2/117}}

@ARTICLE{bower15,
   author = {{Bower}, G.~C. and {Deller}, A. and {Demorest}, P. and {Brunthaler}, A. and 
	{Falcke}, H. and {Moscibrodzka}, M. and {O'Leary}, R.~M. and 
	{Eatough}, R.~P. and {Kramer}, M. and {Lee}, K.~J. and {Spitler}, L. and 
	{Desvignes}, G. and {Rushton}, A.~P. and {Doeleman}, S. and 
	{Reid}, M.~J.},
    title = "{The Proper Motion of the Galactic Center Pulsar Relative to Sagittarius A*}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1411.0399},
 primaryClass = "astro-ph.HE",
 keywords = {black hole physics, Galaxy: center, proper motions, pulsars: general, pulsars: individual: J1745{\ndash}2900},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {120},
    pages = {120},
      doi = {10.1088/0004-637X/798/2/120},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798..120B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bozzo08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...683.1031B},
	Archiveprefix = {arXiv},
	Author = {{Bozzo}, E. and {Falanga}, M. and {Stella}, L.},
	Doi = {10.1086/589990},
	Eprint = {0805.1849},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Neutron, Stars: Supergiants, X-Rays: Binaries, X-Rays: Stars},
	Month = aug,
	Pages = {1031-1044},
	Title = {{Are There Magnetars in High-Mass X-Ray Binaries? The Case of Supergiant Fast X-Ray Transients}},
	Volume = 683,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/589990}}

@ARTICLE{bozzo09,
   author = {{Bozzo}, E. and {Stella}, L. and {Vietri}, M. and {Ghosh}, P.
	},
    title = "{Can disk-magnetosphere interaction models and beat frequency models for quasi-periodic oscillation in accreting X-ray pulsars be reconciled?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0811.0049},
 keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries},
     year = 2009,
    month = jan,
   volume = 493,
    pages = {809-818},
      doi = {10.1051/0004-6361:200810658},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...493..809B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bradt93,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1993A%26AS...97..355B&db_key=AST},
	Author = {{Bradt}, H.~V. and {Rothschild}, R.~E. and {Swank}, J.~H.},
	Journal = {\aaps},
	Month = jan,
	Pages = {355-360},
	Title = {{X-ray timing explorer mission}},
	Volume = 97,
	Year = 1993}

@article{brady08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008PASP..120..301B},
	Archiveprefix = {arXiv},
	Author = {{Brady}, S. and {Thorstensen}, J.~R. and {Koppelman}, M.~D. and {Prieto}, J.~L. and {Garnavich}, P.~M. and {Hirschauer}, A. and {Florack}, M.},
	Doi = {10.1086/529209},
	Eprint = {0801.3856},
	Journal = {\pasp},
	Keywords = {Stars},
	Month = mar,
	Pages = {301-310},
	Title = {{The Eclipsing Cataclysmic Variable Lanning 386: Dwarf Nova, SW Sextantis Star, or Both?}},
	Volume = 120,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/529209}}

@article{brazier99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.305..671B},
	Author = {{Brazier}, K.~T.~S. and {Johnston}, S.},
	Eprint = {arXiv:astro-ph/9803176},
	Journal = {\mnras},
	Month = may,
	Pages = {671-679},
	Title = {{The implications of radio-quiet neutron stars}},
	Volume = 305,
	Year = 1999}

@article{breeveld10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.1687B},
	Archiveprefix = {arXiv},
	Author = {{Breeveld}, A.~A. and {Curran}, P.~A. and {Hoversten}, E.~A. and {Koch}, S. and {Landsman}, W. and {Marshall}, F.~E. and {Page}, M.~J. and {Poole}, T.~S. and {Roming}, P. and {Smith}, P.~J. and {Still}, M. and {Yershov}, V. and {Blustin}, A.~J. and {Brown}, P.~J. and {Gronwall}, C. and {Holland}, S.~T. and {Kuin}, N.~P.~M. and {McGowan}, K. and {Rosen}, S. and {Boyd}, P. and {Broos}, P. and {Carter}, M. and {Chester}, M.~M. and {Hancock}, B. and {Huckle}, H. and {Immler}, S. and {Ivanushkina}, M. and {Kennedy}, T. and {Mason}, K.~O. and {Morgan}, A.~N. and {Oates}, S. and {de Pasquale}, M. and {Schady}, P. and {Siegel}, M. and {vanden Berk}, D.},
	Doi = {10.1111/j.1365-2966.2010.16832.x},
	Eprint = {1004.2448},
	Journal = {\mnras},
	Keywords = {instrumentation: detectors, instrumentation: photometers, astrometry, ultraviolet: general},
	Month = aug,
	Pages = {1687-1700},
	Primaryclass = {astro-ph.IM},
	Title = {{Further calibration of the Swift ultraviolet/optical telescope}},
	Volume = 406,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16832.x}}

@inproceedings{breeveld11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AIPC.1358..373B},
	Archiveprefix = {arXiv},
	Author = {{Breeveld}, A.~A. and {Landsman}, W. and {Holland}, S.~T. and {Roming}, P. and {Kuin}, N.~P.~M. and {Page}, M.~J.},
	Booktitle = {Gamma Ray Bursts 2010.},
	Doi = {10.1063/1.3621807},
	Editor = {{J.~E.~McEnery, J.~L.~Racusin, \& N.~Gehrels}},
	Eprint = {1102.4717},
	Keywords = {astrometry, spectrophotometry, gamma-ray sources (astronomical), colour, Astrometric and interferometric instruments, Spectroscopy and spectrophotometry, gamma-ray sources; gamma-ray bursts, Magnitudes and colors; luminosities},
	Month = aug,
	Pages = {373-376},
	Primaryclass = {astro-ph.IM},
	Publisher = {AIP, Melville},
	Series = {AIP Conference Proceedings},
	Title = {{An Updated Ultraviolet Calibration for the Swift/UVOT}},
	Volume = 1358,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.3621807}}

@article{brocksopp05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005MNRAS.356..125B},
	Author = {{Brocksopp}, C. and {Corbel}, S. and {Fender}, R.~P. and {Rupen}, M. and {Sault}, R. and {Tingay}, S.~J. and {Hannikainen}, D. and {O'Brien}, K.},
	Doi = {10.1111/j.1365-2966.2004.08427.x},
	Eprint = {astro-ph/0410353},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, stars: individual: XTE J1720-318, radio continuum: stars, X-rays: binaries},
	Month = jan,
	Pages = {125-130},
	Title = {{The 2003 radio outburst of a new X-ray transient: XTE J1720-318}},
	Volume = 356,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08427.x}}

@article{brogan00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...537..875B},
	Author = {{Brogan}, C.~L. and {Frail}, D.~A. and {Goss}, W.~M. and {Troland}, T.~H.},
	Doi = {10.1086/309068},
	Eprint = {arXiv:astro-ph/0002398},
	Journal = {\apj},
	Keywords = {ISM: Clouds, ISM: individual (W51, G349.7+0.2, CTB 37A, CTB 33, G357.7-0.1), ISM: Magnetic Fields, Masers, Polarization, Radio Lines: ISM},
	Month = jul,
	Pages = {875-890},
	Title = {{OH Zeeman Magnetic Field Detections toward Five Supernova Remnants Using the VLA}},
	Volume = 537,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/309068}}

@article{buccheri83,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...128..245B},
	Author = {{Buccheri}, R. and {Bennett}, K. and {Bignami}, G.~F. and {Bloemen}, J.~B.~G.~M. and {Boriakoff}, V. and {Caraveo}, P.~A. and {Hermsen}, W. and {Kanbach}, G. and {Manchester}, R.~N. and {Masnou}, J.~L. and {Mayer-Hasselwander}, H.~A. and {Ozel}, M.~E. and {Paul}, J.~A. and {Sacco}, B. and {Scarsi}, L. and {Strong}, A.~W.},
	Journal = {\aap},
	Month = nov,
	Pages = {245-251},
	Title = {{Search for pulsed gamma-ray emission from radio pulsars in the COS-B data}},
	Volume = 128,
	Year = 1983}

@article{bucciantini05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...434..189B},
	Author = {{Bucciantini}, N. and {Amato}, E. and {Del Zanna}, L.},
	Doi = {10.1051/0004-6361:20042205},
	Eprint = {arXiv:astro-ph/0412534},
	Journal = {\aap},
	Keywords = {ISM: jets and outflows, stars: pulsars: general, magnetohydrodynamics (MHD), shock waves, relativity},
	Month = apr,
	Pages = {189-199},
	Title = {{Relativistic MHD simulations of pulsar bow-shock nebulae}},
	Volume = 434,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20042205}}

@ARTICLE{bucciantini07,
   author = {{Bucciantini}, N. and {Quataert}, E. and {Arons}, J. and {Metzger}, B.~D. and 
	{Thompson}, T.~A.},
    title = "{Magnetar-driven bubbles and the origin of collimated outflows in gamma-ray bursts}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0705.1742},
 keywords = {magnetic fields, MHD, stars: neutron, supernovae: general, stars: winds, outflows, gamma-rays: bursts},
     year = 2007,
    month = oct,
   volume = 380,
    pages = {1541-1553},
      doi = {10.1111/j.1365-2966.2007.12164.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.380.1541B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{buckley06,
       author = {{Buckley}, David A.~H. and {Swart}, Gerhard P. and {Meiring}, Jacobus G.},
        title = "{Completion and commissioning of the Southern African Large Telescope}",
    booktitle = {Ground-based and Airborne Telescopes.  Edited by Stepp, Larry M..  Proceedings of the SPIE, Volume 6267, id. 62670Z (2006).},
    editor = {Stepp, Larry M.},
         year = "2006",
       volume = {6267},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
          eid = {62670Z},
        pages = {62670Z},
          doi = {10.1117/12.673750},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006SPIE.6267E..0ZB},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bulik11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...730..140B},
	Archiveprefix = {arXiv},
	Author = {{Bulik}, T. and {Belczynski}, K. and {Prestwich}, A.},
	Doi = {10.1088/0004-637X/730/2/140},
	Eid = {140},
	Eprint = {0803.3516},
	Journal = {\apj},
	Keywords = {binaries: close, black hole physics, gravitational waves, stars: evolution},
	Month = apr,
	Pages = {140},
	Title = {{IC10 X-1/NGC300 X-1: The Very Immediate Progenitors of BH-BH Binaries}},
	Volume = 730,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/730/2/140}}

@article{burderi06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...653L.133B},
	Author = {{Burderi}, L. and {Di Salvo}, T. and {Menna}, M.~T. and {Riggio}, A. and {Papitto}, A.},
	Doi = {10.1086/510666},
	Eprint = {arXiv:astro-ph/0612093},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: SAX J1808.4-3658, Stars: Magnetic Fields, Stars: Neutron, X-Rays: Binaries},
	Month = dec,
	Pages = {L133-L136},
	Title = {{Order in the Chaos: Spin-up and Spin-down during the 2002 Outburst of SAX J1808.4-3658}},
	Volume = 653,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/510666}}

@article{burgay03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003Natur.426..531B},
	Author = {{Burgay}, M. and {D'Amico}, N. and {Possenti}, A. and {Manchester}, R.~N. and {Lyne}, A.~G. and {Joshi}, B.~C. and {McLaughlin}, M.~A. and {Kramer}, M. and {Sarkissian}, J.~M. and {Camilo}, F. and {Kalogera}, V. and {Kim}, C. and {Lorimer}, D.~R.},
	Eprint = {arXiv:astro-ph/0312071},
	Journal = {\nat},
	Month = dec,
	Pages = {531-533},
	Title = {{An increased estimate of the merger rate of double neutron stars from observations of a highly relativistic system}},
	Volume = 426,
	Year = 2003}

@article{burgay05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...624L.113B},
	Author = {{Burgay}, M. and {Possenti}, A. and {Manchester}, R.~N. and {Kramer}, M. and {McLaughlin}, M.~A. and {Lorimer}, D.~R. and {Stairs}, I.~H. and {Joshi}, B.~C. and {Lyne}, A.~G. and {Camilo}, F. and {D'Amico}, N. and {Freire}, P.~C.~C. and {Sarkissian}, J.~M. and {Hotan}, A.~W. and {Hobbs}, G.~B.},
	Doi = {10.1086/430668},
	Eprint = {arXiv:astro-ph/0502512},
	Journal = {\apjl},
	Month = may,
	Pages = {L113-L116},
	Title = {{Long-Term Variations in the Pulse Emission from PSR J0737-3039B}},
	Volume = 624,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430668}}

@article{burgay06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..410B},
	Author = {{Burgay}, M. and {Rea}, N. and {Israel}, G.~L. and {Possenti}, A. and {Burderi}, L. and {di Salvo}, T. and {D'Amico}, N. and {Stella}, L.},
	Doi = {10.1111/j.1365-2966.2006.10872.x},
	Eprint = {arXiv:astro-ph/0607614},
	Journal = {\mnras},
	Keywords = {stars: neutron: pulsars: general},
	Month = oct,
	Pages = {410-416},
	Title = {{Search for radio pulsations in four Anomalous X-ray Pulsars and discovery of two new pulsars}},
	Volume = 372,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10872.x}}

@article{burgay09,
	Author = {{Burgay}, M. and {Israel}, G.~L. and {Possenti}, A. and {Rea}, N. and {Esposito}, P. and {Mereghetti}, S. and {Tiengo}, A. and {G\"otz}, D.},
	Journal = {Astron. Tel.},
	Title = {{Back to radio: Parkes detection of radio pulses from the transient AXP 1E1547.0-5408}},
	Volume = 1913,
	Year = 2009}

@article{burgay10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ATel.2515....1B},
	Author = {{Burgay}, M. and {Possenti}, A. and {Esposito}, P. and {Israel}, G.~L. and {Rea}, N. and {Sarkissian}, J. and {Tiengo}, A. and {Turolla}, R. and {Zane}, S. and {G\"otz}, D. and {Stella}, L. and {Mereghetti}, S.},
	Journal = {Astron. Tel.},
	Keywords = {Radio, Pulsars, Supernova Remnants},
	Month = mar,
	Title = {{Upper limit on the radio emission from the soft gamma-ray repeater SGR 1833-0832}},
	Volume = 2515,
	Year = 2010}

@ARTICLE{burgay16,
   author = {{Burgay}, M. and {Possenti}, A. and {Kerr}, M. and {Esposito}, P. and 
	{Rea}, N. and {Zelati}, F.~C. and {Israel}, G.~L. and {Johnston}, S.
	},
    title = "{Pulsed Radio Emission from PSR J1119-6127 disappeared}",
  journal = {Astron. Tel.},
 keywords = {Neutron Star, Soft Gamma-ray Repeater, Transient, Pulsar},
     year = 2016,
    month = jul,
   volume = 9286,
   adsurl = {http://adsabs.harvard.edu/abs/2016ATel.9286....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bpk16,
   author = {{Burgay}, M. and {Possenti}, A. and {Kerr}, M. and {Esposito}, P. and 
	{Rea}, N. and {Zelati}, F.~C. and {Israel}, G.~L. and {Johnston}, S.
	},
    title = "{Pulsed Radio Emission from PSR J1119-6127 re-activated}",
  journal = {Astron. Tel.},
 keywords = {Neutron Star, Soft Gamma-ray Repeater, Transient, Pulsar},
     year = 2016,
    month = aug,
   volume = 9366,
   adsurl = {http://adsabs.harvard.edu/abs/2016ATel.9366....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{burrows05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005SSRv..120..165B},
	Author = {{Burrows}, D.~N. and {Hill}, J.~E. and {Nousek}, J.~A. and {Kennea}, J.~A. and {Wells}, A. and {Osborne}, J.~P. and {Abbey}, A.~F. and {Beardmore}, A. and {Mukerjee}, K. and {Short}, A.~D.~T. and {Chincarini}, G. and {Campana}, S. and {Citterio}, O. and {Moretti}, A. and {Pagani}, C. and {Tagliaferri}, G. and {Giommi}, P. and {Capalbi}, M. and {Tamburelli}, F. and {Angelini}, L. and {Cusumano}, G. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Hartner}, G.~D.},
	Doi = {10.1007/s11214-005-5097-2},
	Journal = {Space Science Reviews},
	Month = oct,
	Pages = {165-195},
	Title = {{The Swift X-Ray Telescope}},
	Volume = 120,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-005-5097-2}}

@article{burrows11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011Natur.476..421B},
	Archiveprefix = {arXiv},
	Author = {{Burrows}, D.~N. and {Kennea}, J.~A. and {Ghisellini}, G. and {Mangano}, V. and {Zhang}, B. and {Page}, K.~L. and {Eracleous}, M. and {Romano}, P. and {Sakamoto}, T. and {Falcone}, A.~D. and {Osborne}, J.~P. and {Campana}, S. and {Beardmore}, A.~P. and {Breeveld}, A.~A. and {Chester}, M.~M. and {Corbet}, R. and {Covino}, S. and {Cummings}, J.~R. and {D'Avanzo}, P. and {D'Elia}, V. and {Esposito}, P. and {Evans}, P.~A. and {Fugazza}, D. and {Gelbord}, J.~M. and {Hiroi}, K. and {Holland}, S.~T. and {Huang}, K.~Y. and {Im}, M. and {Israel}, G. and {Jeon}, Y. and {Jeon}, Y.-B. and {Jun}, H.~D. and {Kawai}, N. and {Kim}, J.~H. and {Krimm}, H.~A. and {Marshall}, F.~E. and {P.~M{\'e}sz{\'a}ros} and {Negoro}, H. and {Omodei}, N. and {Park}, W.-K. and {Perkins}, J.~S. and {Sugizaki}, M. and {Sung}, H.-I. and {Tagliaferri}, G. and {Troja}, E. and {Ueda}, Y. and {Urata}, Y. and {Usui}, R. and {Antonelli}, L.~A. and {Barthelmy}, S.~D. and {Cusumano}, G. and {Giommi}, P. and {Melandri}, A. and {Perri}, M. and {Racusin}, J.~L. and {Sbarufatti}, B. and {Siegel}, M.~H. and {Gehrels}, N.},
	Doi = {10.1038/nature10374},
	Eprint = {1104.4787},
	Journal = {\nat},
	Month = aug,
	Pages = {421-424},
	Primaryclass = {astro-ph.HE},
	Title = {{Relativistic jet activity from the tidal disruption of a star by a massive black hole}},
	Volume = 476,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature10374}}

@ARTICLE{burrows12,
   author = {{Burrows}, D.~N. and {Chester}, M.~M. and {D'Elia}, V. and {Palmer}, D.~M. and 
	{Romano}, P. and {Saxton}, C.~J. and {Sonbas}, E. and {Stamatikos}, M. and 
	{Stratta}, G.},
    title = "{Swift detection of a burst from LS I +61$^\circ$ 303.}",
  journal = {GCN Circ.},
     year = 2012,
   volume = 12914,
   adsurl = {http://adsabs.harvard.edu/abs/2012GCN.12914....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{burwitz04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..123B},
	Author = {{Burwitz}, V. and {Haberl}, F. and {Freyberg}, M.~J. and {Dennerl}, K. and {Kendziorra}, E. and {Kirsch}, M.~G.~F.},
	Booktitle = {X-Ray and Gamma-Ray Instrumentation for Astronomy XIII},
	Doi = {10.1117/12.506363},
	Editor = {{Flanagan}, K.~A. and {Siegmund}, O.~H.~W.},
	Month = feb,
	Pages = {123-130},
	Publisher = {SPIE, Bellingham},
	Series = {Proceedings of the SPIE.},
	Title = {{Effect of soft flares on XMM-Newton EPIC-pn timing mode data}},
	Volume = 5165,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.506363}}

@ARTICLE{camero10,
   author = {{Camero-Arranz}, A. and {Finger}, M.~H. and {Ikhsanov}, N.~R. and 
	{Wilson-Hodge}, C.~A. and {Beklen}, E.},
    title = "{New Torque Reversal and Spin-up of 4U 1626-67 Observed by Fermi/Gamma-ray Burst Monitor and Swift/Burst Alert Telescope}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0906.4224},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, binaries: close, pulsars: individual: 4U 1626-67, stars: neutron, X-rays: stars},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {1500-1506},
      doi = {10.1088/0004-637X/708/2/1500},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708.1500C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{cameron05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005Natur.434.1112C&db_key=AST},
	Author = {{Cameron}, P.~B. and {Chandra}, P. and {Ray}, A. and {Kulkarni}, S.~R. and {Frail}, D.~A. and {Wieringa}, M.~H. and {Nakar}, E. and {Phinney}, E.~S. and {Miyazaki}, A. and {Tsuboi}, M. and {Okumura}, S. and {Kawai}, N. and {Menten}, K.~M. and {Bertoldi}, F.},
	Doi = {10.1038/nature03605},
	Journal = {\nat},
	Month = apr,
	Pages = {1112-1115},
	Title = {{Detection of a radio counterpart to the 27 December 2004 giant flare from SGR 1806 - 20}},
	Volume = 434,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03605}}

@article{camilo00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000ApJ...541..367C&db_key=AST},
	Author = {{Camilo}, F. and {Kaspi}, V.~M. and {Lyne}, A.~G. and {Manchester}, R.~N. and {Bell}, J.~F. and {D'Amico}, N. and {McKay}, N.~P.~F. and {Crawford}, F.},
	Journal = {\apj},
	Month = sep,
	Pages = {367-373},
	Title = {{Discovery of Two High Magnetic Field Radio Pulsars}},
	Volume = 541,
	Year = 2000}

@article{camilo04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...611L..25C&db_key=AST},
	Author = {{Camilo}, F. and {Manchester}, R.~N. and {Lyne}, A.~G. and {Gaensler}, B.~M. and {Possenti}, A. and {D'Amico}, N. and {Stairs}, I.~H. and {Faulkner}, A.~J. and {Kramer}, M. and {Lorimer}, D.~R. and {McLaughlin}, M.~A. and {Hobbs}, G.},
	Doi = {10.1086/423620},
	Eprint = {astro-ph/0406528},
	Journal = {\apjl},
	Month = aug,
	Pages = {L25-L28},
	Title = {{The Very Young Radio Pulsar J1357-6429}},
	Volume = 611,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423620}}

@article{ccr07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..497C},
	Author = {{Camilo}, F. and {Cognard}, I. and {Ransom}, S.~M. and {Halpern}, J.~P. and {Reynolds}, J. and {Zimmerman}, N. and {Gotthelf}, E.~V. and {Helfand}, D.~J. and {Demorest}, P. and {Theureau}, G. and {Backer}, D.~C.},
	Doi = {10.1086/518226},
	Eprint = {arXiv:astro-ph/0610685},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron},
	Month = jul,
	Pages = {497-504},
	Title = {{The Magnetar XTE J1810-197: Variations in Torque, Radio Flux Density, and Pulse Profile Morphology}},
	Volume = 663,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518226}}

@article{crj07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...659L..37C},
	Author = {{Camilo}, F. and {Reynolds}, J. and {Johnston}, S. and {Halpern}, J.~P. and {Ransom}, S.~M. and {van Straten}, W.},
	Doi = {10.1086/516630},
	Eprint = {arXiv:astro-ph/0702616},
	Journal = {\apjl},
	Keywords = {pulsars: individual (XTE J1810-197), Stars: Neutron},
	Month = apr,
	Pages = {L37-L40},
	Title = {{Polarized Radio Emission from the Magnetar XTE J1810-197}},
	Volume = 659,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/516630}}

@article{camilo08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...679..681C},
	Archiveprefix = {arXiv},
	Author = {{Camilo}, F. and {Reynolds}, J. and {Johnston}, S. and {Halpern}, J.~P. and {Ransom}, S.~M.},
	Doi = {10.1086/587054},
	Eprint = {0802.0494},
	Journal = {\apj},
	Keywords = {ISM: individual (G327.24-0.13), pulsars: individual (1E 1547.0-5408), pulsars: individual (PSR J1550-5418), Stars: Pulsars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron},
	Month = may,
	Pages = {681-686},
	Title = {{The Magnetar 1E 1547.0-5408: Radio Spectrum, Polarimetry, and Timing}},
	Volume = 679,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587054}}

@article{camilo08atel1558,
	Author = {{Camilo}, F. and {Sarkissian}, J.},
	Journal = {Astron. Tel.},
	Title = {{No radio pulsations detected from SGR 1627-41 following renewed X-ray activity}},
	Volume = 1558,
	Year = 2008}

@ARTICLE{camilo16,
   author = {{Camilo}, F. and {Ransom}, S.~M. and {Halpern}, J.~P. and {Alford}, J.~A.~J. and 
	{Cognard}, I. and {Reynolds}, J.~E. and {Johnston}, S. and {Sarkissian}, J. and 
	{van Straten}, W.},
    title = "{Radio Disappearance of the Magnetar XTE J1810-197 and Continued X-ray Timing}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1603.02170},
 primaryClass = "astro-ph.SR",
 keywords = {pulsars: individual: XTE J1810{\ndash}197, PSR J1809{\ndash}1943, stars: neutron},
     year = 2016,
    month = apr,
   volume = 820,
      eid = {110},
    pages = {110},
      doi = {10.3847/0004-637X/820/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...820..110C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{campana95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...297..385C},
	Author = {{Campana}, S. and {Stella}, L. and {Mereghetti}, S. and {Colpi}, M.},
	Eprint = {arXiv:astro-ph/9411064},
	Journal = {\aap},
	Month = may,
	Pages = {385},
	Title = {{Radio pulsar and accretion regimes of rapidly rotating magnetic neutron stars in early-type eccentric binaries.}},
	Volume = 297,
	Year = 1995}

@article{campana02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...580..389C},
	Author = {{Campana}, S. and {Stella}, L. and {Israel}, G.~L. and {Moretti}, A. and {Parmar}, A.~N. and {Orlandini}, M.},
	Doi = {10.1086/343074},
	Eprint = {arXiv:astro-ph/0207422},
	Journal = {\apj},
	Month = nov,
	Pages = {389-393},
	Title = {{The Quiescent X-Ray Emission of Three Transient X-Ray Pulsars}},
	Volume = 580,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/343074}}

@article{csg02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...575L..15C},
	Author = {{Campana}, S. and {Stella}, L. and {Gastaldello}, F. and {Mereghetti}, S. and {Colpi}, M. and {Israel}, G.~L. and {Burderi}, L. and {Di Salvo}, T. and {Robba}, R.~N.},
	Doi = {10.1086/342505},
	Eprint = {arXiv:astro-ph/0206376},
	Journal = {\apjl},
	Month = aug,
	Pages = {L15-L19},
	Title = {{An XMM-Newton Study of the 401 Hz Accreting Pulsar SAX J1808.4-3658 in Quiescence}},
	Volume = 575,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342505}}

@article{campana04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613L..53C},
	Author = {{Campana}, S. and {Possenti}, A. and {Burgay}, M.},
	Doi = {10.1086/424926},
	Eprint = {arXiv:astro-ph/0408157},
	Journal = {\apjl},
	Month = sep,
	Pages = {L53-L56},
	Title = {{XMM-Newton Observation of the Double Pulsar System J0737-3039}},
	Volume = 613,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/424926}}

@article{campana07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...463.1047C},
	Author = {{Campana}, S. and {Rea}, N. and {Israel}, G.~L. and {Turolla}, R. and {Zane}, S.},
	Doi = {10.1051/0004-6361:20065482},
	Eprint = {arXiv:astro-ph/0611216},
	Journal = {\aap},
	Month = mar,
	Pages = {1047-1051},
	Title = {{Swift and Chandra confirm the intensity-hardness correlation of the AXP 1RXS J170849.0-400910}},
	Volume = 463,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065482}}
    
@ARTICLE{campana18,
  author = {{Campana}, S. and {Stella}, L. and {Mereghetti}, S. and {de Martino}, D.
},
   title = "{A universal relation for the propeller mechanisms in magnetic rotating stars at different scales}",
 journal = {\aap},
archivePrefix = "arXiv",
  eprint = {1711.08233},
primaryClass = "astro-ph.HE",
keywords = {stars: neutron, X-rays: binaries, accretion, accretion discs, magnetic fields},
    year = 2018,
   month = feb,
  volume = 610,
     eid = {A46},
   pages = {A46},
     doi = {10.1051/0004-6361/201730769},
  adsurl = {http://cdsads.u-strasbg.fr/abs/2018A%26A...610A..46C},
 adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{campbell05,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005GCN..2932....1C&db_key=AST},
	Author = {{Campbell}, P. and {Hill}, M. and {Howe}, R. and {Kielkopf}, J.~F. and {Lewis}, N. and {Mandaville}, J. and {McWilliams}, A. and {Moos}, W. and {Samouce}, D. and {Winkler}, J. and {Fishman}, G.~J. and {Price}, A. and {Welch}, D.~L. and {Schnoor}, P. and {Clerkin}, A. and {Saum}, D.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR1806: detection of a sudden ionospheric disturbance.}},
	Volume = 2932,
	Year = 2005}

@article{canizares73,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1973NPhS..241...28C},
	Author = {{Canizares}, C.~R. and {McClintock}, J.~E. and {Clark}, G.~W. and {Lewin}, W.~H.~G. and {Schnopper}, H.~W. and {Sprott}, G.~F.},
	Doi = {10.1038/physci241028a0},
	Journal = {Nature Physical Science},
	Month = jan,
	Pages = {28-30},
	Title = {{Observations of Periodic Variations in the X-ray Intensity of Cygnus X-3}},
	Volume = 241,
	Year = 1973,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/physci241028a0}}

@article{cardelli89,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1989ApJ...345..245C},
	Author = {{Cardelli}, J.~A. and {Clayton}, G.~C. and {Mathis}, J.~S.},
	Doi = {10.1086/167900},
	Journal = {\apj},
	Month = oct,
	Pages = {245-256},
	Title = {{The relationship between infrared, optical, and ultraviolet extinction}},
	Volume = 345,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/167900}}

@ARTICLE{carpano05,
   author = {{Carpano}, S. and {Wilms}, J. and {Schirmer}, M. and {Kendziorra}, E.
	},
    title = "{X-ray properties of NGC 300. I. Global properties of X-ray point sources and their optical counterparts}",
  journal = {\aap},
   eprint = {astro-ph/0509383},
 keywords = {galaxies:, individual: NGC 300, X-rays: galaxies},
     year = 2005,
    month = nov,
   volume = 443,
    pages = {103-114},
      doi = {10.1051/0004-6361:20042162},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2005A%26A...443..103C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{carpano07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...461L...9C},
	Author = {{Carpano}, S. and {Pollock}, A.~M.~T. and {Wilms}, J. and {Ehle}, M. and {Schirmer}, M.},
	Doi = {10.1051/0004-6361:20066527},
	Eprint = {arXiv:astro-ph/0611424},
	Journal = {\aap},
	Keywords = {galaxies: individual: NGC 300, X-rays: binaries, stars: Wolf-Rayet},
	Month = jan,
	Pages = {L9-L12},
	Title = {{A Wolf-Rayet/black-hole X-ray binary candidate in NGC 300}},
	Volume = 461,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066527}}

@article{cpp07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...466L..17C},
	Author = {{Carpano}, S. and {Pollock}, A.~M.~T. and {Prestwich}, A. and {Crowther}, P. and {Wilms}, J. and {Yungelson}, L. and {Ehle}, M.},
	Doi = {10.1051/0004-6361:20077363},
	Eprint = {arXiv:astro-ph/0703270},
	Journal = {\aap},
	Keywords = {X-rays: individuals: NGC 300 X-1, X-rays: binaries, stars: Wolf-Rayet},
	Month = may,
	Pages = {L17-L20},
	Title = {{A 33 hour period for the Wolf-Rayet/black hole X-ray binary candidate NGC 300 X-1}},
	Volume = 466,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077363}}

@ARTICLE{carpano18,
   author = {{Carpano}, S. and {Haberl}, F. and {Maitra}, C. and {Vasilopoulos}, G.
	},
    title = "{Discovery of pulsations from NGC 300 ULX1 and its fast period evolution}",
  journal = {\mnras},
 keywords = {stars: neutron, pulsars: individual: NGC 300 ULX1- galaxies: individual: NGC 300, X-rays: binaries},
     year = 2018,
    month = may,
   volume = 476,
    pages = {L45-L49},
      doi = {10.1093/mnrasl/sly030},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.476L..45C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{carter97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997PASP..109..990C},
	Author = {{Carter}, L.~M. and {Dickel}, J.~R. and {Bomans}, D.~J.},
	Doi = {10.1086/133971},
	Journal = {\pasp},
	Month = sep,
	Pages = {990-997},
	Title = {{Expansion of the Supernova Remnant RCW 103}},
	Volume = 109,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133971}}

@inproceedings{carter03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ASPC..295..477C},
	Author = {{Carter}, C. and {Karovska}, M. and {Jerius}, D. and {Glotfelty}, K. and {Beikman}, S.},
	Booktitle = {Astronomical Data Analysis Software and Systems XII},
	Editor = {{H.~E.~Payne, R.~I.~Jedrzejewski, \& R.~N.~Hook (San Francisco, CA: ASP)}},
	Pages = {477},
	Series = {ASP Conf. Ser.},
	Title = {{ChaRT: The Chandra Ray Tracer}},
	Volume = 295,
	Year = 2003}

@article{casali07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467..777C},
	Author = {{Casali}, M. and {Adamson}, A. and {Alves de Oliveira}, C. and {Almaini}, O. and {Burch}, K. and {Chuter}, T. and {Elliot}, J. and {Folger}, M. and {Foucaud}, S. and {Hambly}, N. and {Hastie}, M. and {Henry}, D. and {Hirst}, P. and {Irwin}, M. and {Ives}, D. and {Lawrence}, A. and {Laidlaw}, K. and {Lee}, D. and {Lewis}, J. and {Lunney}, D. and {McLay}, S. and {Montgomery}, D. and {Pickup}, A. and {Read}, M. and {Rees}, N. and {Robson}, I. and {Sekiguchi}, K. and {Vick}, A. and {Warren}, S. and {Woodward}, B.},
	Doi = {10.1051/0004-6361:20066514},
	Journal = {\aap},
	Keywords = {instrumentation: miscellaneous, infrared: general},
	Month = may,
	Pages = {777-784},
	Title = {{The UKIRT wide-field camera}},
	Volume = 467,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066514}}

@article{crr05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.364..899C},
	Author = {{Casares}, J. and {Rib{\'o}}, M. and {Ribas}, I. and {Paredes}, J.~M. and {Mart{\'{\i}}}, J. and {Herrero}, A.},
	Doi = {10.1111/j.1365-2966.2005.09617.x},
	Eprint = {arXiv:astro-ph/0507549},
	Journal = {\mnras},
	Month = dec,
	Pages = {899-908},
	Title = {{A possible black hole in the {$\gamma$}-ray microquasar LS 5039}},
	Volume = 364,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09617.x}}

@article{casares05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360.1105C},
	Author = {{Casares}, J. and {Ribas}, I. and {Paredes}, J.~M. and {Mart{\'{\i}}}, J. and {Allende Prieto}, C.},
	Doi = {10.1111/j.1365-2966.2005.09106.x},
	Eprint = {arXiv:astro-ph/0504332},
	Journal = {\mnras},
	Month = jul,
	Pages = {1105-1109},
	Title = {{Orbital parameters of the microquasar LS I +61 303}},
	Volume = 360,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09106.x}}

@article{casella05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..403C},
	Author = {{Casella}, P. and {Belloni}, T. and {Stella}, L.},
	Doi = {10.1086/431174},
	Eprint = {arXiv:astro-ph/0504318},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Black Hole Physics, Stars: Oscillations, X-Rays: Binaries},
	Month = aug,
	Pages = {403-407},
	Title = {{The ABC of Low-Frequency Quasi-periodic Oscillations in Black Hole Candidates: Analogies with Z Sources}},
	Volume = {629},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/431174}}

@article{cassam04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004A%26A...427..199C},
	Author = {{Cassam-Chena{\"\i}}, G. and {Decourchelle}, A. and {Ballet}, J. and {Sauvageot}, J.-L. and {Dubner}, G. and {Giacani}, E.},
	Doi = {10.1051/0004-6361:20041154},
	Eprint = {arXiv:astro-ph/0407333},
	Journal = {\aap},
	Month = nov,
	Pages = {199-216},
	Title = {{XMM-Newton observations of the supernova remnant RX J1713.7-3946 and its central source}},
	Volume = 427,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041154}}

@inproceedings{cassam04iaus,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004IAUS..218...73C},
	Author = {{Cassam-Chena{\"\i}}, G. and {Decourchelle}, A. and {Ballet}, J. and {Sauvageot}, J.-L. and {Dubner}, G.},
	Booktitle = {{Camilo}, F. and {Gaensler}, B.~M., eds., IAU Symposium no. 218: Young Neutron Stars and Their Environments.},
	Pages = {73},
	Series = {Astronom. Soc. Pac. San Francisco CA},
	Title = {{XMM-Newton Observation of SNR RX J1713.7-3946}},
	Volume = 218,
	Year = 2004}

@ARTICLE{castor75,
   author = {{Castor}, J. and {McCray}, R. and {Weaver}, R.},
    title = "{Interstellar bubbles}",
  journal = {\apjl},
 keywords = {Bubbles, Early Stars, Interstellar Gas, Stellar Winds, Density Distribution, Gas Dynamics, Hydrogen Clouds, Interstellar Matter, Space Density, Stellar Envelopes, Stellar Evolution},
     year = 1975,
    month = sep,
   volume = 200,
    pages = {L107-L110},
      doi = {10.1086/181908},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...200L.107C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{castrotirado98,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998A%26A...330.1067C&db_key=AST},
	Author = {{Castro-Tirado}, A.~J. and {Gorosabel}, J. and {Hammersley}, P.},
	Journal = {\aap},
	Month = feb,
	Pages = {1067-1069},
	Title = {{IR observations of SGR 1806-20 during the November 1996 active period}},
	Volume = 330,
	Year = 1998}

@ARTICLE{caswell75,
   author = {{Caswell}, J.~L. and {Murray}, J.~D. and {Roger}, R.~S. and 
	{Cole}, D.~J. and {Cooke}, D.~J.},
    title = {{Neutral hydrogen absorption measurements yielding kinematic distances for 42 continuum sources in the galactic plane}},
  journal = {\aap},
     year = 1975,
    month = dec,
   volume = 45,
    pages = {239-258}
}

@article{caswell04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.352.1405C},
	Author = {{Caswell}, J.~L. and {McClure-Griffiths}, N.~M. and {Cheung}, M.~C.~M.},
	Doi = {10.1111/j.1365-2966.2004.08030.x},
	Journal = {\mnras},
	Keywords = {pulsars: individual: PSR J1119-6127, ISM: individual: G292.2-0.5, supernova remnants, Galaxy: structure, galaxies: magnetic fields, radio continuum: ISM},
	Month = aug,
	Pages = {1405-1412},
	Title = {{Supernova remnant G292.2-0.5, its pulsar, and the Galactic magnetic field}},
	Volume = 352,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08030.x}}

@ARTICLE{cavallo78,
   author = {{Cavallo}, G. and {Rees}, M.~J.},
    title = "{A qualitative study of cosmic fireballs and gamma-ray bursts}",
  journal = {\mnras},
 keywords = {Bursts, Cosmic Rays, Fireballs, Gamma Rays, Electron-Positron Pairs, Luminosity, Pair Production},
     year = 1978,
    month = may,
   volume = 183,
    pages = {359-365},
      doi = {10.1093/mnras/183.3.359},
   adsurl = {http://adsabs.harvard.edu/abs/1978MNRAS.183..359C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cavecchi11,
   author = {{Cavecchi}, Y. and {Patruno}, A. and {Haskell}, B. and {Watts}, A.~L. and 
	{Levin}, Y. and {Linares}, M. and {Altamirano}, D. and {Wijnands}, R. and 
	{van der Klis}, M.},
    title = "{Implications of Burst Oscillations from the Slowly Rotating Accreting Pulsar IGR J17480-2446 in the Globular Cluster Terzan 5}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1102.1548},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: IGR J17480-2446, stars: magnetic field, stars: neutron, stars: rotation, X-rays: bursts},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {L8},
    pages = {L8},
      doi = {10.1088/2041-8205/740/1/L8},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740L...8C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chadwick1932,
       author = {{Chadwick}, J.},
        title = "{Possible Existence of a Neutron}",
      journal = {\nat},
         year = 1932,
        month = feb,
       volume = {129},
       number = {3252},
        pages = {312},
          doi = {10.1038/129312a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1932Natur.129Q.312C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chakrabarty98,
   author = {{Chakrabarty}, D.},
    title = "{High-Speed Optical Photometry of the Ultracompact X-Ray Binary 4U 1626-67}",
  journal = {\apj},
   eprint = {astro-ph/9706049},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: BINARIES: CLOSE, STARS: PULSARS: INDIVIDUAL ALPHANUMERIC: 4U 1626-67, STARS: NEUTRON, STARS: LOW-MASS, BROWN DWARFS, Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Pulsars: Individual: Alphanumeric: 4U 1626-67, Stars: Low-Mass, Brown Dwarfs, Stars: Neutron},
     year = 1998,
    month = jan,
   volume = 492,
    pages = {342-351},
      doi = {10.1086/305035},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...492..342C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chakraborty21,
       author = {{Chakraborty}, Joheen and {Kara}, Erin and {Masterson}, Megan and {Giustini}, Margherita and {Miniutti}, Giovanni and {Saxton}, Richard},
        title = "{Possible X-ray Quasi-Periodic Eruptions in a Tidal Disruption Event Candidate}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = oct,
          eid = {arXiv:2110.10786},
        pages = {arXiv:2110.10786},
archivePrefix = {arXiv},
       eprint = {2110.10786},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv211010786C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chandrasekhar1931,
       author = {{Chandrasekhar}, S.},
        title = "{The Maximum Mass of Ideal White Dwarfs}",
      journal = {\apj},
         year = 1931,
        month = jul,
       volume = {74},
        pages = {81},
          doi = {10.1086/143324},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1931ApJ....74...81C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chashkina12,
   author = {{Chashkina}, A. and {Popov}, S.~B.},
    title = "{Magnetic field estimates for accreting neutron stars in massive binary systems and models of magnetic field decay}",
  journal = {\na},
archivePrefix = "arXiv",
   eprint = {1112.1123},
 primaryClass = "astro-ph.HE",
     year = 2012,
    month = aug,
   volume = 17,
    pages = {594-602},
      doi = {10.1016/j.newast.2012.01.004},
   adsurl = {http://adsabs.harvard.edu/abs/2012NewA...17..594C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{chatterjee00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...534..373C},
	Author = {{Chatterjee}, P. and {Hernquist}, L. and {Narayan}, R.},
	Doi = {10.1086/308748},
	Eprint = {arXiv:astro-ph/9912137},
	Journal = {\apj},
	Keywords = {ACCRETION, ACCRETION DISKS, STARS: PULSARS: GENERAL, STARS: NEUTRON, X-RAYS: STARS},
	Month = may,
	Pages = {373-379},
	Title = {{An Accretion Model for Anomalous X-Ray Pulsars}},
	Volume = 534,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308748}}

@article{chatterjee07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...670.1301C},
	Author = {{Chatterjee}, S. and {Gaensler}, B.~M. and {Melatos}, A. and {Brisken}, W.~F. and {Stappers}, B.~W.},
	Doi = {10.1086/522298},
	Eprint = {arXiv:astro-ph/0703181},
	Journal = {\apj},
	Month = dec,
	Pages = {1301-1306},
	Title = {{Pulsed X-Ray Emission from Pulsar A in the Double Pulsar System J0737-3039}},
	Volume = 670,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/522298}}

@article{cheng96,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1996Natur.382..518C&db_key=AST},
	Author = {{Cheng}, B. and {Epstein}, R.~I. and {Guyer}, R.~A. and {Young}, C.},
	Journal = {\nat},
	Pages = {518-520},
	Title = {{Earthquake-like behaviour of soft gamma-ray repeaters.}},
	Volume = 382,
	Year = 1996}

@article{cheng04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...617..480C&db_key=AST},
	Author = {{Cheng}, K.~S. and {Taam}, R.~E. and {Wang}, W.},
	Doi = {10.1086/425295},
	Eprint = {astro-ph/0408460},
	Journal = {\apj},
	Month = dec,
	Pages = {480-489},
	Title = {{Pulsar Wind Nebulae and the X-Ray Emission of Nonaccreting Neutron Stars}},
	Volume = 617,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/425295}}

@article{chernyakova06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006MNRAS.372.1585C&db_key=AST},
	Author = {{Chernyakova}, M. and {Neronov}, A. and {Walter}, R.},
	Doi = {10.1111/j.1365-2966.2006.10946.x},
	Eprint = {astro-ph/0606070},
	Journal = {\mnras},
	Month = nov,
	Pages = {1585-1592},
	Title = {{INTEGRAL and XMM-Newton observations of LSI +61{\deg} 303}},
	Volume = 372,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10946.x}}

@ARTICLE{chevalier92,
   author = {{Chevalier}, R.~A. and {Fransson}, C.},
    title = "{Pulsar nebulae in supernovae}",
  journal = {\apj},
 keywords = {Pulsars, Stellar Evolution, Supernova Remnants, Supernovae, Crab Nebula, Ionizing Radiation, Nebulae, Photoionization, Supernova 1987a, Taylor Instability},
     year = 1992,
    month = aug,
   volume = 395,
    pages = {540-552},
      doi = {10.1086/171674},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...395..540C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chevalier94,
   author = {{Chevalier}, R.~A. and {Fransson}, C.},
    title = "{Emission from circumstellar interaction in normal Type II supernovae}",
  journal = {\apj},
 keywords = {Emission Spectra, Galactic Evolution, Interstellar Matter, Photoionization, Stellar Envelopes, Stellar Winds, Supernova Remnants, Chronology, Hydrodynamics, Protostars, Shock Waves, Stellar Mass Ejection, Stellar Models, Stellar Spectra},
     year = 1994,
    month = jan,
   volume = 420,
    pages = {268-285},
      doi = {10.1086/173557},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...420..268C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{chevalier00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539L..45C},
	Author = {{Chevalier}, R.~A.},
	Doi = {10.1086/312835},
	Journal = {\apjl},
	Month = aug,
	Pages = {L45-L48},
	Title = {{A Model for the X-Ray Luminosity of Pulsar Nebulae}},
	Volume = 539,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312835}}

@article{chevalier05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005ApJ...619..839C&db_key=AST},
	Author = {{Chevalier}, R.~A.},
	Doi = {10.1086/426584},
	Eprint = {astro-ph/0409013},
	Journal = {\apj},
	Month = feb,
	Pages = {839-855},
	Title = {{Young Core-Collapse Supernova Remnants and Their Supernovae}},
	Volume = 619,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426584}}

@ARTICLE{chita08,
   author = {{Chita}, S.~M. and {Langer}, N. and {van Marle}, A.~J. and {Garc{\'{\i}}a-Segura}, G. and 
	{Heger}, A.},
    title = "{Multiple ring nebulae around blue supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0807.3049},
 keywords = {hydrodynamics, ISM: bubbles, stars: winds, outflows, stars: supergiants},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {L37-L41},
      doi = {10.1051/0004-6361:200810087},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488L..37C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clark05,
   author = {{Clark}, J.~S. and {Negueruela}, I. and {Crowther}, P.~A. and 
	{Goodwin}, S.~P.},
    title = "{On the massive stellar population of the super star cluster <ASTROBJ>Westerlund 1</ASTROBJ>}",
  journal = {\aap},
   eprint = {astro-ph/0504342},
 keywords = {stars: evolution, open clusters and associations: individual: Westerlund 1, galaxies: starburst},
     year = 2005,
    month = may,
   volume = 434,
    pages = {949-969},
      doi = {10.1051/0004-6361:20042413},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...434..949C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clark08,
   author = {{Clark}, J.~S. and {Muno}, M.~P. and {Negueruela}, I. and {Dougherty}, S.~M. and 
	{Crowther}, P.~A. and {Goodwin}, S.~P. and {de Grijs}, R.},
    title = "{Unveiling the X-ray point source population of the Young Massive Cluster Westerlund 1}",
  journal = {\aap},
 keywords = {stars: evolution, open clusters and associations: individual:, Westerlund 1, X rays: stars},
     year = 2008,
    month = jan,
   volume = 477,
    pages = {147-163},
      doi = {10.1051/0004-6361:20077186},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...477..147C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clark14,
   author = {{Clark}, J.~S. and {Ritchie}, B.~W. and {Najarro}, F. and {Langer}, N. and 
	{Negueruela}, I.},
    title = "{A VLT/FLAMES survey for massive binaries in Westerlund 1. IV. Wd1-5 - binary product and a pre-supernova companion for the magnetar CXOU J1647-45?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1405.3109},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: CXOU J1647-45, binaries: close, stars: evolution, stars: magnetars, stars: fundamental parameters, stars: abundances},
     year = 2014,
    month = may,
   volume = 565,
      eid = {A90},
    pages = {A90},
      doi = {10.1051/0004-6361/201321771},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...565A..90C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{clarke96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996Sci...274..404C},
	Author = {{Clarke}, J.~T. and {Ballester}, G.~E. and {Trauger}, J. and {Evans}, R. and {Connerney}, J.~E.~P. and {Stapelfeldt}, K. and {Crisp}, D. and {Feldman}, P.~D. and {Burrows}, C.~J. and {Casertano}, S. and {Gallagher}, III, J.~S. and {Griffiths}, R.~E. and {Hester}, J.~J. and {Hoessel}, J.~G. and {Holtzman}, J.~A. and {Krist}, J.~E. and {Meadows}, V. and {Mould}, J.~R. and {Scowen}, P.~A. and {Watson}, A.~M. and {Westphal}, J.~A.},
	Doi = {10.1126/science.274.5286.404},
	Journal = {Science},
	Month = oct,
	Pages = {404-409},
	Title = {{Far-Ultraviolet Imaging of Jupiter's Aurora and the lo ''Footprint''}},
	Volume = 274,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.274.5286.404}}

@ARTICLE{clausen11,
       author = {{Clausen}, Drew and {Eracleous}, Michael},
        title = "{Probing Intermediate-mass Black Holes with Optical Emission Lines from Tidally Disrupted White Dwarfs}",
      journal = {\apj},
     keywords = {black hole physics, globular clusters: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = jan,
       volume = {726},
       number = {1},
          eid = {34},
        pages = {34},
          doi = {10.1088/0004-637X/726/1/34},
archivePrefix = {arXiv},
       eprint = {1010.6087},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...726...34C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clausen12,
       author = {{Clausen}, Drew and {Sigurdsson}, Steinn and {Eracleous}, Michael and
         {Irwin}, Jimmy A.},
        title = "{Luminous [O III] and [N II] from tidally disrupted horizontal branch stars}",
      journal = {\mnras},
     keywords = {black hole physics, globular clusters: general, galaxies: individual: NGC 1399, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = aug,
       volume = {424},
       number = {2},
        pages = {1268-1274},
          doi = {10.1111/j.1365-2966.2012.21305.x},
archivePrefix = {arXiv},
       eprint = {1205.3053},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.424.1268C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{clemens98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.297.1015C},
	Author = {{Clemens}, M.~S. and {Alexander}, P. and {Green}, D.~A.},
	Doi = {10.1046/j.1365-8711.1998.01510.x},
	Journal = {\mnras},
	Keywords = {GALAXIES: EVOLUTION, GALAXIES: INDIVIDUAL: NGC 4485, GALAXIES: INDIVIDUAL: NGC 4490, GALAXIES: INTERACTIONS, RADIO LINES: GALAXIES},
	Month = jul,
	Pages = {1015-1020},
	Title = {{Possible formation scenarios for the giant HI envelope around the NGC 4490/4485 system}},
	Volume = 297,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.01510.x}}

@article{clemens99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.307..481C},
	Author = {{Clemens}, M.~S. and {Alexander}, P. and {Green}, D.~A.},
	Doi = {10.1046/j.1365-8711.1999.02594.x},
	Journal = {\mnras},
	Month = aug,
	Pages = {481-490},
	Title = {{The star formation history in the interacting galaxies NGC 4490 and 4485}},
	Volume = 307,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02594.x}}

@article{clemens02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.333...39C},
	Author = {{Clemens}, M.~S. and {Alexander}, P.},
	Doi = {10.1046/j.1365-8711.2002.05444.x},
	Journal = {\mnras},
	Keywords = {galaxies: individual: NGC 4490, galaxies: interactions, galaxies: ISM},
	Month = jun,
	Pages = {39-46},
	Title = {{H{$\alpha$}, SCUBA and MERLIN imaging of NGC 4490}},
	Volume = 333,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05444.x}}

@article{cline80,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1980ApJ...237L...1C&db_key=AST},
	Author = {{Cline}, T.~L. and {Desai}, U.~D. and {Pizzichini}, G. and {Teegarden}, B.~J. and {Evans}, W.~D. and {Klebesadel}, R.~W. and {Laros}, J.~G. and {Hurley}, K. and {Niel}, M. and {Vedrenne}, G.},
	Doi = {10.1086/183221},
	Journal = {\apjl},
	Month = apr,
	Pages = {L1-L5},
	Title = {{Detection of a fast, intense and unusual gamma-ray transient}},
	Volume = 237,
	Year = 1980,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/183221}}

@article{cline82,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...255L..45C},
	Author = {{Cline}, T.~L. and {Desai}, U.~D. and {Teegarden}, B.~J. and {Evans}, W.~D. and {Klebesadel}, R.~W. and {Laros}, J.~G. and {Barat}, C. and {Hurley}, K. and {Niel}, M. and {Weisskopf}, M.~C.},
	Doi = {10.1086/183766},
	Journal = {\apjl},
	Keywords = {ERROR ANALYSIS, GAMMA RAY BURSTS, RADIATION SOURCES, ASTRONOMICAL MODELS, PROPORTIONAL COUNTERS, SPECTRAL SENSITIVITY, TIME MEASUREMENT},
	Month = apr,
	Pages = {L45-L48},
	Title = {{Precise source location of the anomalous 1979 March 5 gamma-ray transient}},
	Volume = 255,
	Year = 1982,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/183766}}

@article{cline00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...531..407C&db_key=AST},
	Author = {{Cline}, T. and {Frederiks}, D.~D. and {Golenetskii}, S. and {Hurley}, K. and {Kouveliotou}, C. and {Mazets}, E. and {van Paradijs}, J.},
	Journal = {\apj},
	Month = mar,
	Pages = {407-410},
	Title = {{Observations of a Possible New Soft Gamma Repeater, SGR 1801-23}},
	Volume = 531,
	Year = 2000}

@article{coe05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.356..502C},
	Author = {{Coe}, M.~J. and {Edge}, W.~R.~T. and {Galache}, J.~L. and {McBride}, V.~A.},
	Doi = {10.1111/j.1365-2966.2004.08467.x},
	Eprint = {arXiv:astro-ph/0410074},
	Journal = {\mnras},
	Keywords = {stars: emission-line, Be, Magellanic Clouds, X-rays: binaries},
	Month = jan,
	Pages = {502-514},
	Title = {{Optical properties of Small Magellanic Cloud X-ray binaries}},
	Volume = 356,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08467.x}}

@article{colbert99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...519...89C},
	Author = {{Colbert}, E.~J.~M. and {Mushotzky}, R.~F.},
	Doi = {10.1086/307356},
	Eprint = {arXiv:astro-ph/9901023},
	Journal = {\apj},
	Keywords = {GALAXIES: ACTIVE, X-RAYS: GALAXIES},
	Month = jul,
	Pages = {89-107},
	Title = {{The Nature of Accreting Black Holes in Nearby Galaxy Nuclei}},
	Volume = 519,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307356}}

@article{coleiro13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1310.0451C},
	Archiveprefix = {arXiv},
	Author = {{Coleiro}, A. and {Chaty}, S. and {Zurita Heras}, J.~A. and {Rahoui}, F. and {Tomsick}, J.~A.},
	Eprint = {1310.0451},
	Journal = {ArXiv e-prints},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Galaxy Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
	Month = oct,
	Primaryclass = {astro-ph.HE},
	Title = {{Infrared identification of high-mass X-ray binaries discovered by INTEGRAL}},
	Year = 2013}

@article{cominsky84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...283..765C},
	Author = {{Cominsky}, L.~R. and {Wood}, K.~S.},
	Doi = {10.1086/162361},
	Journal = {\apj},
	Keywords = {ECLIPSING BINARY STARS, PERIODIC VARIATIONS, STELLAR FLARES, X RAY SOURCES, COMPANION STARS, HEAO 1, LIGHT CURVE, NEUTRON STARS, ORBITAL ELEMENTS, STELLAR LUMINOSITY, STELLAR MASS, X RAY SPECTRA},
	Month = aug,
	Pages = {765-773},
	Title = {{Discovery of a 7.1 hour period and eclipses from MXB 1659-29}},
	Volume = 283,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/162361}}

@article{condon83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJS...53..459C},
	Author = {{Condon}, J.~J.},
	Doi = {10.1086/190898},
	Journal = {\apjs},
	Keywords = {Astronomical Photometry, Brightness Temperature, Galactic Structure, Radio Sources (Astronomy), Spiral Galaxies, Stellar Evolution, Astronomical Maps, Disk Galaxies, High Resolution, Radiant Flux Density, Radio Spectra, Ubv Spectra},
	Month = oct,
	Pages = {459-495},
	Title = {{Strong radio sources in bright spiral galaxies. III - Disk emission}},
	Volume = 53,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/190898}}

@article{contopoulos02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...566..336C},
	Author = {{Contopoulos}, I. and {Kazanas}, D.},
	Doi = {10.1086/324778},
	Eprint = {arXiv:astro-ph/0110183},
	Journal = {\apj},
	Month = feb,
	Pages = {336-342},
	Title = {{Toward Resolving the Crab {$\sigma$}-Problem: A Linear Accelerator?}},
	Volume = 566,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324778}}

@article{corbel97,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...478..624C&db_key=AST},
	Author = {{Corbel}, S. and {Wallyn}, P. and {Dame}, T.~M. and {Durouchoux}, P. and {Mahoney}, W.~A. and {Vilhu}, O. and {Grindlay}, J.~E.},
	Journal = {\apj},
	Month = mar,
	Pages = {624},
	Title = {{The Distance of the Soft Gamma Repeater SGR 1806-20}},
	Volume = 478,
	Year = 1997}

@article{corbel99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...526L..29C&db_key=AST},
	Author = {{Corbel}, S. and {Chapuis}, C. and {Dame}, T.~M. and {Durouchoux}, P.},
	Journal = {\apjl},
	Month = nov,
	Pages = {L29-L32},
	Title = {{The Distance to the Soft Gamma Repeater SGR 1627-41}},
	Volume = 526,
	Year = 1999}

@article{corbel04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004A%26A...419..191C&db_key=AST},
	Author = {{Corbel}, S. and {Eikenberry}, S.~S.},
	Doi = {10.1051/0004-6361:20034054},
	Eprint = {astro-ph/0311313},
	Journal = {\aap},
	Month = may,
	Pages = {191-201},
	Title = {{The connection between W31, SGR 1806-20, and LBV 1806-20: Distance, extinction, and structure}},
	Volume = 419,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20034054}}

@article{corbet86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.220.1047C},
	Author = {{Corbet}, R.~H.~D.},
	Journal = {\mnras},
	Keywords = {ACCRETION DISKS, BINARY STARS, MASS TRANSFER, PULSARS, STELLAR MASS, X RAY STARS, ANGULAR MOMENTUM, B STARS, ORBITAL ELEMENTS, STELLAR ENVELOPES, STELLAR MASS ACCRETION, STELLAR ROTATION, SUPERGIANT STARS, WHITE DWARF STARS},
	Month = jun,
	Pages = {1047-1056},
	Title = {{The three types of high-mass X-ray pulsator}},
	Volume = 220,
	Year = 1986}

@article{corbet97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1997ApJ...476..833C},
	Author = {{Corbet}, R.~H.~D. and {Charles}, P.~A. and {Southwell}, K.~A. and {Smale}, A.~P.},
	Doi = {10.1086/303644},
	Journal = {\apj},
	Month = feb,
	Pages = {833},
	Title = {{A Low-Amplitude X-Ray and Optical Outburst from the Periodic Transient A0538-66: Accretion onto a Magnetosphere?}},
	Volume = 476,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/303644}}

@article{corbet04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ATel..273....1C},
	Author = {{Corbet}, R.~H.~D. and {Markwardt}, C.~B. and {Coe}, M.~J. and {Edge}, W.~R.~T. and {Laycock}, S. and {Marshall}, F.~E.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Binaries, Neutron Stars, Pulsars, Transients},
	Month = apr,
	Title = {{A New Transient X-ray Pulsar in the SMC (XTE J0051-727)}},
	Volume = 273,
	Year = 2004}

@article{chr04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ATel..269....1C},
	Author = {{Corbet}, R.~H.~D. and {Hannikainen}, D.~C. and {Remillard}, R.},
	Journal = {The Astronomer's Telegram},
	Keywords = {X-ray, Binaries, Black Holes, Neutron Stars, Transients},
	Month = apr,
	Title = {{The Orbital Period of IGR J19140+098}},
	Volume = 269,
	Year = 2004}

@article{corbet08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...675.1424C},
	Archiveprefix = {arXiv},
	Author = {{Corbet}, R.~H.~D. and {Sokoloski}, J.~L. and {Mukai}, K. and {Markwardt}, C.~B. and {Tueller}, J.},
	Doi = {10.1086/526337},
	Eprint = {0711.1519},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Symbiotic, Stars: Individual: Alphanumeric: GX 1+4, stars: individual (4U 1954+31), stars: individual (4U 1700+24), Stars: Neutron, X-Rays: Binaries},
	Month = mar,
	Pages = {1424-1435},
	Title = {{A Comparison of the Variability of the Symbiotic X-Ray Binaries GX 1+4, 4U 1954+31, and 4U 1700+24 from Swift BAT and RXTE ASM Observations}},
	Volume = 675,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/526337}}

@article{cordes02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002astro.ph..7156C&db_key=PRE},
	Author = {{Cordes}, J.~M. and {Lazio}, T.~J.~W.},
	Eprint = {astro-ph/0207156},
	Journal = {eprint (astro-ph/0207156)},
	Month = jul,
	Title = {{NE2001.I. A New Model for the Galactic Distribution of Free Electrons and its Fluctuations}},
	Year = 2002}

@ARTICLE{corrales16,
   author = {{Corrales}, L.~R. and {Garc{\'{\i}}a}, J. and {Wilms}, J. and 
	{Baganoff}, F.},
    title = "{The dust-scattering component of X-ray extinction: effects on continuum fitting and high-resolution absorption edge structure}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1602.01100},
 primaryClass = "astro-ph.HE",
 keywords = {scattering, dust, extinction, quasars: absorption lines, X-rays: binaries, X-rays: ISM},
     year = 2016,
    month = may,
   volume = 458,
    pages = {1345-1351},
      doi = {10.1093/mnras/stw376},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.458.1345C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{cortina05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005Ap%26SS.297..245C&db_key=AST},
	Author = {{Cortina}, J.},
	Doi = {10.1007/s10509-005-7627-5},
	Eprint = {astro-ph/0407475},
	Journal = {\apss},
	Month = jun,
	Pages = {245-255},
	Title = {{Status and First Results of the Magic Telescope}},
	Volume = 297,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-005-7627-5}}

@ARTICLE{cotizelati15,
   author = {{Coti Zelati}, F. and {Rea}, N. and {Papitto}, A. and {Vigan{\`o}}, D. and 
	{Pons}, J.~A. and {Turolla}, R. and {Esposito}, P. and {Haggard}, D. and 
	{Baganoff}, F.~K. and {Ponti}, G. and {Israel}, G.~L. and {Campana}, S. and 
	{Torres}, D.~F. and {Tiengo}, A. and {Mereghetti}, S. and {Perna}, R. and 
	{Zane}, S. and {Mignani}, R.~P. and {Possenti}, A. and {Stella}, L.
	},
    title = "{The X-ray outburst of the Galactic Centre magnetar SGR J1745-2900 during the first 1.5 year}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1503.01307},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetars, Galaxy: centre, X-rays: individual: SGR J1745-2900},
     year = 2015,
    month = may,
   volume = 449,
    pages = {2685-2699},
      doi = {10.1093/mnras/stv480},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.2685C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cotizelati17,
   author = {{Coti Zelati}, F. and {Rea}, N. and {Turolla}, R. and {Pons}, J.~A. and 
	{Papitto}, A. and {Esposito}, P. and {Israel}, G.~L. and {Campana}, S. and 
	{Zane}, S. and {Tiengo}, A. and {Mignani}, R.~P. and {Mereghetti}, S. and 
	{Baganoff}, F.~K. and {Haggard}, D. and {Ponti}, G. and {Torres}, D.~F. and 
	{Borghese}, A. and {Elfritz}, J.},
    title = "{Chandra monitoring of the Galactic Centre magnetar SGR J1745-2900 during the initial 3.5 years of outburst decay}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1707.01514},
 primaryClass = "astro-ph.HE",
 keywords = {methods: data analysis, methods: observational, stars: magnetars, Galaxy: centre, X-rays: individual: SGR J1745-2900},
     year = 2017,
    month = oct,
   volume = 471,
    pages = {1819-1829},
      doi = {10.1093/mnras/stx1700},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.471.1819C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{courvoisier03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003A%26A...411L..53C},
	Author = {{Courvoisier}, T.~J.-L. and {Walter}, R. and {Beckmann}, V. and {Dean}, A.~J. and {Dubath}, P. and {Hudec}, R. and {Kretschmar}, P. and {Mereghetti}, S. and {Montmerle}, T. and {Mowlavi}, N. and {Paltani}, S. and {Preite Martinez}, A. and {Produit}, N. and {Staubert}, R. and {Strong}, A.~W. and {Swings}, J.-P. and {Westergaard}, N.~J. and {White}, N. and {Winkler}, C. and {Zdziarski}, A.~A.},
	Doi = {10.1051/0004-6361:20031172},
	Eprint = {arXiv:astro-ph/0308047},
	Journal = {\aap},
	Month = nov,
	Pages = {L53-L57},
	Title = {{The INTEGRAL Science Data Centre (ISDC)}},
	Volume = 411,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031172}}

@article{coward12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2668C},
	Archiveprefix = {arXiv},
	Author = {{Coward}, D.~M. and {Howell}, E.~J. and {Piran}, T. and {Stratta}, G. and {Branchesi}, M. and {Bromberg}, O. and {Gendre}, B. and {Burman}, R.~R. and {Guetta}, D.},
	Doi = {10.1111/j.1365-2966.2012.21604.x},
	Eprint = {1202.2179},
	Journal = {\mnras},
	Keywords = {gravitational waves, techniques: miscellaneous, gamma-ray burst: individual, stars: neutron},
	Month = oct,
	Pages = {2668-2673},
	Primaryclass = {astro-ph.CO},
	Title = {{The Swift short gamma-ray burst rate density: implications for binary neutron star merger rates}},
	Volume = 425,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21604.x}}

@book{cox00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000asqu.book.....C},
	Author = {{Cox}, A.~N.},
	Publisher = {4th ed.~Publisher: New York: AIP Press; Springer, 2000.~Editedy by Arthur N.~Cox.~ ISBN: 0387987460},
	Title = {{Allen's astrophysical quantities}},
	Year = 2000}

@article{craig97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...488..307C},
	Author = {{Craig}, W.~W. and {Hailey}, C.~J. and {Pisarski}, R.~L.},
	Doi = {10.1086/304666},
	Journal = {\apj},
	Month = oct,
	Pages = {307},
	Title = {{ROSAT Observations of the Supernova Remnant CTB 1}},
	Volume = 488,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/304666}}

@article{crawfor07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662.1183C},
	Author = {{Crawford}, F. and {Hessels}, J.~W.~T. and {Kaspi}, V.~M.},
	Doi = {10.1086/517991},
	Eprint = {arXiv:astro-ph/0703246},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General, Stars: Neutron},
	Month = jun,
	Pages = {1183-1187},
	Title = {{Deep Searches for Radio Pulsations and Bursts from Four Southern Anomalous X-Ray Pulsars}},
	Volume = 662,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/517991}}

@article{crivellari09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501..445C},
	Archiveprefix = {arXiv},
	Author = {{Crivellari}, E. and {Wolter}, A. and {Trinchieri}, G.},
	Doi = {10.1051/0004-6361/200810707},
	Eprint = {0905.1230},
	Journal = {\aap},
	Keywords = {galaxies: individual: Cartwheel, X-rays: binaries, X-rays: galaxies, X-rays: ISM},
	Month = jul,
	Pages = {445-453},
	Primaryclass = {astro-ph.CO},
	Title = {{The Cartwheel galaxy with XMM-Newton}},
	Volume = 501,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200810707}}

@article{cropper98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.293L..57C},
	Author = {{Cropper}, M. and {Harrop-Allin}, M.~K. and {Mason}, K.~O. and {Mittaz}, J.~P.~D. and {Potter}, S.~B. and {Ramsay}, G.},
	Doi = {10.1046/j.1365-8711.1998.01297.x},
	Journal = {\mnras},
	Keywords = {ACCRETION DISKS, NOVAE, CATACLYSMIC VARIABLES, X RAY STARS, LIGHT CURVE, WHITE DWARF STARS},
	Month = jan,
	Pages = {L57-L60},
	Title = {{RX J1914.4+2456 - The first double-degenerate polar?}},
	Volume = 293,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.01297.x}}

@inproceedings{cropper04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ASPC..315..324C},
	Author = {{Cropper}, M. and {Ramsay}, G. and {Wu}, K. and {Hakala}, P.},
	Booktitle = {IAU Colloq. 190: Magnetic Cataclysmic Variables},
	Editor = {{S.~Vrielmann \& M.~Cropper}},
	Month = dec,
	Pages = {324},
	Publisher = {ASP, San Francisco},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{REVIEW: Ultra-Short Period Double-Degenerate Binaries}},
	Volume = 315,
	Year = 2004}

@article{crowther07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..177C},
	Author = {{Crowther}, P.~A.},
	Doi = {10.1146/annurev.astro.45.051806.110615},
	Eprint = {arXiv:astro-ph/0610356},
	Journal = {\araa},
	Month = sep,
	Pages = {177-219},
	Title = {{Physical Properties of Wolf-Rayet Stars}},
	Volume = 45,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.45.051806.110615}}

@article{crowther10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403L..41C},
	Archiveprefix = {arXiv},
	Author = {{Crowther}, P.~A. and {Barnard}, R. and {Carpano}, S. and {Clark}, J.~S. and {Dhillon}, V.~S. and {Pollock}, A.~M.~T.},
	Doi = {10.1111/j.1745-3933.2010.00811.x},
	Eprint = {1001.4616},
	Journal = {\mnras},
	Keywords = {stars: Wolf-Rayet, galaxies: individual: NGC 300, X-rays: binaries, X-rays: individual: NGC 300 X-1},
	Month = mar,
	Pages = {L41-L45},
	Primaryclass = {astro-ph.SR},
	Title = {{NGC 300 X-1 is a Wolf-Rayet/black hole binary}},
	Volume = 403,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2010.00811.x}}

@ARTICLE{cseh12,
   author = {{Cseh}, D. and {Corbel}, S. and {Kaaret}, P. and {Lang}, C. and 
	{Gris{\'e}}, F. and {Paragi}, Z. and {Tzioumis}, A. and {Tudose}, V. and 
	{Feng}, H.},
    title = "{Black Hole Powered Nebulae and a Case Study of the Ultraluminous X-Ray Source IC 342 X-1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.4473},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, ISM: bubbles, ISM: jets and outflows, X-rays: binaries},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {17},
    pages = {17},
      doi = {10.1088/0004-637X/749/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...749...17C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{cummings09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2127....1C},
	Author = {{Cummings}, J.~R. and {Page}, K.~L. and {Beardmore}, A.~P. and {Gehrels}, N.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Soft Gamma-ray Repeaters},
	Month = jul,
	Title = {{Swift Observations of SGR 0418+4729}},
	Volume = 2127,
	Year = 2009}

@article{cummings11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3488....1C},
	Author = {{Cummings}, J.~R. and {Burrows}, D. and {Campana}, S. and {Kennea}, J.~A. and {Krimm}, H.~A. and {Palmer}, D.~M. and {Sakamoto}, T. and {Zane}, S.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Gamma Ray, Soft Gamma-ray Repeater},
	Month = jul,
	Title = {{Swift J1822.3-1606: A Probable New SGR in Ground Analysis of BAT Data}},
	Volume = 3488,
	Year = 2011}

@article{currie09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.3210C},
	Archiveprefix = {arXiv},
	Author = {{Currie}, T. and {Evans}, N.~R. and {Spitzbart}, B.~D. and {Irwin}, J. and {Wolk}, S.~J. and {Hernandez}, J. and {Kenyon}, S.~J. and {Pasachoff}, J.~M.},
	Doi = {10.1088/0004-6256/137/2/3210},
	Eprint = {0811.1753},
	Journal = {\aj},
	Keywords = {open clusters and associations: individual: NGC 869, planetary systems: formation, stars: pre-main sequence, X-rays: stars},
	Month = feb,
	Pages = {3210-3221},
	Title = {{The X-Ray Environment During the Epoch of Terrestrial Planet Formation: Chandra Observations of h Persei}},
	Volume = 137,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/137/2/3210}}

@ARTICLE{dage18,
       author = {{Dage}, Kristen C. and {Zepf}, Stephen E. and {Bahramian}, Arash and
         {Kundu}, Arunav and {Maccarone}, Thomas J. and {Peacock}, Mark B.},
        title = "{X-Ray Variability from the Ultraluminous Black Hole Candidate X-Ray Binary in the Globular Cluster RZ 2109}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 4472, galaxies: star clusters: individual: RZ 2109, globular clusters: general, X-rays: binaries, X-rays: galaxies: clusters, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = aug,
       volume = {862},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.3847/1538-4357/aacb2b},
archivePrefix = {arXiv},
       eprint = {1806.01848},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...862..108D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dage19,
       author = {{Dage}, Kristen C. and {Zepf}, Stephen E. and {Bahramian}, Arash and
         {Strader}, Jay and {Maccarone}, Thomas J. and {Peacock}, Mark B. and
         {Kundu}, Arunav and {Steele}, Matthew M. and {Britt}, Christopher T.},
        title = "{Slow decline and rise of the broad [O III] emission line in globular cluster black hole candidate RZ2109}",
      journal = {\mnras},
     keywords = {white dwarfs, globular clusters: individual: RZ2109, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = nov,
       volume = {489},
       number = {4},
        pages = {4783-4790},
          doi = {10.1093/mnras/stz2514},
archivePrefix = {arXiv},
       eprint = {1909.02683},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.4783D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dallosso03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...599..485D},
	Author = {{Dall'Osso}, S. and {Israel}, G.~L. and {Stella}, L. and {Possenti}, A. and {Perozzi}, E.},
	Doi = {10.1086/379213},
	Journal = {\apj},
	Month = dec,
	Pages = {485-497},
	Title = {{The Glitches of the Anomalous X-Ray Pulsar 1RXS J170849.0-400910}},
	Volume = 599,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379213}}

@article{dallosso06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...447..785D},
	Author = {{Dall'Osso}, S. and {Israel}, G.~L. and {Stella}, L.},
	Doi = {10.1051/0004-6361:20052843},
	Eprint = {arXiv:astro-ph/0507474},
	Journal = {\aap},
	Keywords = {gravitational waves, magnetic fields, stars: binaries: close, stars: dwarfs novae, X-rays: individuals: RX J0806.3+1527, X-rays: individuals: RX J1914.4+2456},
	Month = mar,
	Pages = {785-796},
	Title = {{Astrophysical unipolar inductors powered by GW emission}},
	Volume = 447,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052843}}

@article{dallosso07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...464..417D},
	Author = {{Dall'Osso}, S. and {Israel}, G.~L. and {Stella}, L.},
	Doi = {10.1051/0004-6361:20064862},
	Eprint = {arXiv:astro-ph/0603795},
	Journal = {\aap},
	Keywords = {gravitational waves, magnetic fields, binaries: close, white dwarfs, X-rays: individuals: RX J0806+15, X-rays: individuals: RX J1914+24},
	Month = mar,
	Pages = {417-427},
	Title = {{Unipolar inductor model coupled to GW emission: energy budget and model application to RX J0806+15 and RX J1914+24}},
	Volume = 464,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20064862}}

@ARTICLE{dallosso09,
   author = {{Dall'Osso}, S. and {Shore}, S.~N. and {Stella}, L.},
    title = "{Early evolution of newly born magnetars with a strong toroidal field}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0811.4311},
 keywords = {gravitational waves , magnetic fields , stars: neutron , X-rays: stars},
     year = 2009,
    month = oct,
   volume = 398,
    pages = {1869-1885},
      doi = {10.1111/j.1365-2966.2008.14054.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398.1869D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dallosso11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1110.2498D},
	Author = {{Dall'Osso}, S. and {Granot}, J. and {Piran}, T.},
	Journal = {\mnras, in press (astro-ph/1110.2498)},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = oct,
	Title = {{Magnetic field decay in neutron stars: from Soft Gamma Repeaters to ''weak field magnetars''}},
	Year = 2011}

@ARTICLE{dallosso15,
   author = {{Dall'Osso}, S. and {Perna}, R. and {Stella}, L.},
    title = "{NuSTAR J095551+6940.8: a highly magnetized neutron star with super-Eddington mass accretion}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1412.1823},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, stars: magnetic field, stars: neutron, pulsars: general},
     year = 2015,
    month = may,
   volume = 449,
    pages = {2144-2150},
      doi = {10.1093/mnras/stv170},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.2144D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dall'Osso2021,
       author = {{Dall'Osso}, Simone and {Stella}, Luigi},
        title = "{Millisecond Magnetars}",
      journal = {Astrophysics and Space Science Library (in press), arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = mar,
          eid = {arXiv:2103.10878},
        pages = {arXiv:2103.10878},
archivePrefix = {arXiv},
       eprint = {2103.10878},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210310878D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dame01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...547..792D},
	Author = {{Dame}, T.~M. and {Hartmann}, D. and {Thaddeus}, P.},
	Doi = {10.1086/318388},
	Eprint = {arXiv:astro-ph/0009217},
	Journal = {\apj},
	Keywords = {Galaxy: Structure, ISM: Clouds, ISM: Molecules, Radio Lines: ISM, Galaxy: Solar Neighborhood, Stars: Formation},
	Month = feb,
	Pages = {792-813},
	Title = {{The Milky Way in Molecular Clouds: A New Complete CO Survey}},
	Volume = 547,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/318388}}

@article{dantona06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653.1429D},
	Author = {{D'Antona}, F. and {Ventura}, P. and {Burderi}, L. and {Teodorescu}, A.},
	Doi = {10.1086/507408},
	Eprint = {arXiv:astro-ph/0606577},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Symbiotic, Gravitational Waves, Stars: Individual: Alphanumeric: RX J0806.3+1527, Stars: Individual: Alphanumeric: RX J1914.4+2456, Stars: White Dwarfs},
	Month = dec,
	Pages = {1429-1434},
	Title = {{Modeling the Closest Double Degenerate System RX J0806.3+1527 and Its Decreasing Period}},
	Volume = 653,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507408}}

@article{davidge95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995AJ....110.1177D},
	Author = {{Davidge}, T.~J.},
	Doi = {10.1086/117597},
	Eprint = {astro-ph/9505114},
	Journal = {\aj},
	Keywords = {GLOBULAR CLUSTERS: INDIVIDUAL: NGC 5946, GLOBULAR CLUSTERS: INDIVIDUAL: NGC 7099, STARS: GIANT},
	Month = sep,
	Pages = {1177},
	Title = {{Near-Infrared Photometry of the Core-Collapsed Metal-Poor Globular Cluster NGC 5946 and NGC 7099}},
	Volume = 110,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/117597}}

@article{davidson73,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...179..585D},
	Author = {{Davidson}, K. and {Ostriker}, J.~P.},
	Doi = {10.1086/151897},
	Journal = {\apj},
	Month = jan,
	Pages = {585-598},
	Title = {{Neutron-Star Accretion in a Stellar Wind: Model for a Pulsed X-Ray Source}},
	Volume = 179,
	Year = 1973,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/151897}}

@article{davies79,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1979MNRAS.186..779D},
	Author = {{Davies}, R.~E. and {Fabian}, A.~C. and {Pringle}, J.~E.},
	Journal = {\mnras},
	Keywords = {BINARY STARS, MAGNETIC STARS, NEUTRON STARS, STELLAR EVOLUTION, STELLAR ROTATION, ANGULAR VELOCITY, RATES (PER TIME), STELLAR ENVELOPES, X RAY STARS},
	Month = mar,
	Pages = {779-782},
	Title = {{Spindown of neutron stars in close binary systems}},
	Volume = 186,
	Year = 1979}

@article{davies81,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1981MNRAS.196..209D},
	Author = {{Davies}, R.~E. and {Pringle}, J.~E.},
	Journal = {\mnras},
	Keywords = {BINARY STARS, MAGNETIC STARS, NEUTRON STARS, SPIN DYNAMICS, STELLAR ROTATION, STELLAR MODELS, X RAY SOURCES},
	Month = jul,
	Pages = {209-224},
	Title = {{Spindown of neutron stars in close binary systems. II}},
	Volume = 196,
	Year = 1981}

@ARTICLE{davies09,
   author = {{Davies}, B. and {Figer}, D.~F. and {Kudritzki}, R.-P. and {Trombley}, C. and 
	{Kouveliotou}, C. and {Wachter}, S.},
    title = "{The Progenitor Mass of the Magnetar SGR1900+14}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0910.4859},
 primaryClass = "astro-ph.SR",
 keywords = {open clusters and associations: individual: Cl 1900+14, stars: evolution, stars: individual: SGR1900+14, stars: neutron},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {844-851},
      doi = {10.1088/0004-637X/707/1/844},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707..844D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{davis96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...460..601D},
	Author = {{Davis}, D.~S. and {Mulchaey}, J.~S. and {Mushotzky}, R.~F. and {Burstein}, D.},
	Doi = {10.1086/176995},
	Journal = {\apj},
	Keywords = {COSMOLOGY: DIFFUSE RADIATION, GALAXIES: CLUSTERS: INDIVIDUAL NGC NUMBER: NGC 2300, GALAXIES: INTERGALACTIC MEDIUM, X-RAYS: GALAXIES},
	Month = apr,
	Pages = {601},
	Title = {{Spectral and Spatial Analysis of the Intragroup Medium in the NGC 2300 Group}},
	Volume = 460,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176995}}

@article{davis97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997AJ....114..613D},
	Author = {{Davis}, D.~S. and {Keel}, W.~C. and {Mulchaey}, J.~S. and {Henning}, P.~A.},
	Doi = {10.1086/118497},
	Eprint = {astro-ph/9705220},
	Journal = {\aj},
	Keywords = {GALAXIES: INTERACTIONS},
	Month = aug,
	Pages = {613-625},
	Title = {{Gravitational Interactions in Poor Galaxy Groups.}},
	Volume = 114,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/118497}}

@article{davis01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562..575D},
	Author = {{Davis}, J.~E.},
	Doi = {10.1086/323488},
	Journal = {\apj},
	Keywords = {Instrumentation: Detectors, Methods: Analytical, Methods: Data Analysis, X-Rays: General},
	Month = nov,
	Pages = {575-582},
	Title = {{Event Pileup in Charge-coupled Devices}},
	Volume = 562,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323488}}

@article{davis04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...604..653D},
	Author = {{Davis}, D.~S. and {Mushotzky}, R.~F.},
	Doi = {10.1086/381929},
	Eprint = {astro-ph/0312211},
	Journal = {\apj},
	Keywords = {Galaxies: Individual: NGC Number: NGC 2276, Galaxies: Spiral, X-Rays: Binaries, X-Rays: Galaxies},
	Month = apr,
	Pages = {653-661},
	Title = {{XMM-Newton Observations of an Intermediate X-Ray Object in NGC 2276}},
	Volume = 604,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/381929}}

@article{davis11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734..111D},
	Archiveprefix = {arXiv},
	Author = {{Davis}, S.~W. and {Narayan}, R. and {Zhu}, Y. and {Barret}, D. and {Farrell}, S.~A. and {Godet}, O. and {Servillat}, M. and {Webb}, N.~A.},
	Doi = {10.1088/0004-637X/734/2/111},
	Eid = {111},
	Eprint = {1104.2614},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, X-rays: binaries, X-rays: individual: ESO 243-49 HLX-1},
	Month = jun,
	Pages = {111},
	Primaryclass = {astro-ph.HE},
	Title = {{The Cool Accretion Disk in ESO 243-49 HLX-1: Further Evidence of an Intermediate-mass Black Hole}},
	Volume = 734,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/734/2/111}}

@INPROCEEDINGS{davis12,
   author = {{Davis}, J.~E. and {Bautz}, M.~W. and {Dewey}, D. and {Heilmann}, R.~K. and 
	{Houck}, J.~C. and {Huenemoerder}, D.~P. and {Marshall}, H.~L. and 
	{Nowak}, M.~A. and {Schattenburg}, M.~L. and {Schulz}, N.~S. and 
	{Smith}, R.~K.},
    title = "{Raytracing with MARX: x-ray observatory design, calibration, and support}",
booktitle = {Space Telescopes and Instrumentation 2012: Ultraviolet to Gamma Ray},
     year = 2012,
   series = {\procspie},
   volume = 8443,
    month = sep,
      eid = {84431A},
    pages = {84431A},
	Publisher = {SPIE, Bellingham},
      doi = {10.1117/12.926937},
   adsurl = {http://adsabs.harvard.edu/abs/2012SPIE.8443E..1AD},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dedeo01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...559..346D},
	Author = {{DeDeo}, S. and {Psaltis}, D. and {Narayan}, R.},
	Doi = {10.1086/322283},
	Eprint = {arXiv:astro-ph/0004266},
	Journal = {\apj},
	Month = sep,
	Pages = {346-352},
	Title = {{General Relativistic Constraints on Emission Models of Anomalous X-Ray Pulsars}},
	Volume = 559,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/322283}}

@ARTICLE{drm13,
   author = {{Degenaar}, N. and {Reynolds}, M.~T. and {Miller}, J.~M. and 
	{Kennea}, J.~A. and {Wijnands}, R.},
    title = "{Large Flare from Sgr A* Detected by Swift}",
  journal = {The Astronomer's Telegram},
 keywords = {Radio, Infra-Red, X-ray, AGN, Black Hole, Transient},
     year = 2013,
    month = apr,
   volume = 5006,
   adsurl = {http://adsabs.harvard.edu/abs/2013ATel.5006....1D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{degenaar13,
   author = {{Degenaar}, N. and {Miller}, J.~M. and {Kennea}, J. and {Gehrels}, N. and 
	{Reynolds}, M.~T. and {Wijnands}, R.},
    title = "{The X-Ray Flaring Properties of Sgr A* during Six Years of Monitoring with Swift}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1210.7237},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, black hole physics, Galaxy: center, X-rays: individual: Sgr A*},
     year = 2013,
    month = jun,
   volume = 769,
      eid = {155},
    pages = {155},
      doi = {10.1088/0004-637X/769/2/155},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769..155D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{delgado01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001ApJ...546..455D},
	Author = {{Delgado-Mart{\'{\i}}}, H. and {Levine}, A.~M. and {Pfahl}, E. and {Rappaport}, S.~A.},
	Doi = {10.1086/318236},
	Eprint = {arXiv:astro-ph/0004258},
	Journal = {\apj},
	Keywords = {Stars: Individual: Constellation Name: X Persei, Stars: Individual: Alphanumeric: 4U 0352+30, Stars: Neutron, Stars: Supernovae: General, X-Rays: Stars},
	Month = jan,
	Pages = {455-468},
	Title = {{The Orbit of X Persei and Its Neutron Star Companion}},
	Volume = 546,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/318236}}

@article{delia11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011GCN..12253...1D},
	Author = {{D'Elia}, V. and {Barthelmy}, S.~D. and {Baumgartner}, W.~H. and {Beardmore}, A.~P. and {Chester}, M.~M. and {Guidorzi}, C. and {Holland}, S.~T. and {Kuin}, N.~P.~M. and {Markwardt}, C.~B. and {Marshall}, F.~E. and {Melandri}, A. and {Palmer}, D.~M. and {Saxton}, C.~J. and {Stratta}, G. and {Swenson}, C.~A. and {Ukwatta}, T.~N.},
	Journal = {GCN Circ.},
	Title = {{GRB 110807A: Swift detection of a burst or a posible new Sgr.}},
	Volume = 12253,
	Year = 2011}

@ARTICLE{deller12,
   author = {{Deller}, A.~T. and {Camilo}, F. and {Reynolds}, J.~E. and {Halpern}, J.~P.
	},
    title = "{The Proper Motion of PSR J1550-5418 Measured with VLBI: A Second Magnetar Velocity Measurement}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1201.4684},
 primaryClass = "astro-ph.SR",
 keywords = {astrometry, pulsars: individual: PSR J1550-5418 1E 1547.0-5408, stars: neutron},
     year = 2012,
    month = mar,
   volume = 748,
      eid = {L1},
    pages = {L1},
      doi = {10.1088/2041-8205/748/1/L1},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748L...1D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{deloye06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649L..99D},
	Author = {{Deloye}, C.~J. and {Taam}, R.~E.},
	Doi = {10.1086/508372},
	Eprint = {arXiv:astro-ph/0608442},
	Journal = {\apjl},
	Keywords = {Stars: Binaries: Close, Gravitational Waves, stars: individual (RX J0806+1527), stars: individual (RX J1914+2456), Stars: White Dwarfs},
	Month = oct,
	Pages = {L99-L102},
	Title = {{The Turn-On of Mass Transfer in AM CVn Binaries: Implications for RX J0806+1527 and RX J1914+2456}},
	Volume = 649,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/508372}}

@article{deloye07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381..525D},
	Archiveprefix = {arXiv},
	Author = {{Deloye}, C.~J. and {Taam}, R.~E. and {Winisdoerffer}, C. and {Chabrier}, G.},
	Doi = {10.1111/j.1365-2966.2007.12262.x},
	Eprint = {0708.0220},
	Journal = {\mnras},
	Keywords = {gravitational waves, binaries: close, stars: individual: RX J0806+1527, stars: individual: RX J1914+2456, stars: individual: SDSS J0926+3624, white dwarfs},
	Month = oct,
	Pages = {525-542},
	Title = {{The thermal evolution of the donors in AM Canum Venaticorum binaries}},
	Volume = 381,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12262.x}}

@inproceedings{deluca08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008AIPC..983..311D},
	Author = {{De Luca}, A.},
	Booktitle = {{Bassa} C., {Wang} Z., {Cumming} A., {Kaspi} V.~M., eds., 40 years of pulsars: Millisecond Pulsars, Magnetars and More.},
	Doi = {10.1063/1.2900173},
	Keywords = {supernova remnants, neutron stars, X-ray sources (astronomical), pulsars},
	Month = feb,
	Pages = {311},
	Series = {AIP Conference Proceedings, Melville NY},
	Title = {{Central Compact Objects in Supernova Remnants}},
	Volume = 983,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2900173}}

@article{dmz08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682.1185D},
	Archiveprefix = {arXiv},
	Author = {{De Luca}, A. and {Mignani}, R.~P. and {Zaggia}, S. and {Beccari}, G. and {Mereghetti}, S. and {Caraveo}, P.~A. and {Bignami}, G.~F.},
	Doi = {10.1086/588600},
	Eprint = {0803.2885},
	Journal = {\apj},
	Keywords = {Stars: Individual: Alphanumeric: 1E 161348-5055, Stars: Neutron},
	Month = aug,
	Pages = {1185-1194},
	Title = {{Deep Infrared Observations of the Puzzling Central X-Ray Source in RCW 103}},
	Volume = 682,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588600}}

@article{deluca12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421L..72D},
	Archiveprefix = {arXiv},
	Author = {{De Luca}, A. and {Salvetti}, D. and {Sartori}, A. and {Esposito}, P. and {Tiengo}, A. and {Zane}, S. and {Turolla}, R. and {Pizzolato}, F. and {Mignani}, R.~P. and {Caraveo}, P.~A. and {Mereghetti}, S. and {Bignami}, G.~F.},
	Doi = {10.1111/j.1745-3933.2011.01209.x},
	Eprint = {1112.4602},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, X-rays: individual: RX J0822-4300},
	Month = mar,
	Pages = {L72-L76},
	Primaryclass = {astro-ph.HE},
	Title = {{A time-variable, phase-dependent emission line in the X-ray spectrum of the isolated neutron star RX J0822-4300}},
	Volume = 421,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2011.01209.x}}

@inproceedings{deluca15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150301497D},
	Archiveprefix = {arXiv},
	Author = {{De Luca}, A. and {Salvaterra}, R. and {Tiengo}, A. and {D'Agostino}, D. and {Watson}, M.~G. and {Haberl}, F. and {Wilms}, J.},
	Booktitle = {Swift: 10 Years of Discovery},
	Editor = {{Caraveo}, P. and {D'Avanzo}, P. and {Gehrels}, N. and {Tagliaferri}, G.},
	Eid = {135},
	Eprint = {1503.01497},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
	Month = mar,
	Pages = {135},
	Primaryclass = {astro-ph.HE},
	Publisher = {Proc. Sci.},
	Title = {{An overview of the EXTraS project: Exploring the X-ray Transient and Variable Sky}},
	Volume = 233,
	Year = 2015}
   
@inproceedings{deluca16,
   author = {{De Luca}, A. and {Salvaterra}, R. and {Tiengo}, A. and {D'Agostino}, D. and 
	{Watson}, M.~G. and {Haberl}, F. and {Wilms}, J.},
    title = "{Science with the EXTraS Project: Exploring the X-Ray Transient and Variable Sky}",
  Booktitle = {The Universe of Digital Sky Surveys},
archivePrefix = "arXiv",
series = {Astrophysics and Space Science Proceedings},
   eprint = {1503.01497},
 primaryClass = "astro-ph.HE",
 Editor = {{Napolitano}, N. and {Longo}, G. and {Marconi}, M. and {Paolillo}, M. and {Iodice}, E.},
 Publisher = {Springer International Publishing, Cham},
 keywords = {Physics},
     year = 2016,
   volume = 42,
    pages = {291},
      doi = {10.1007/978-3-319-19330-4_46},
   adsurl = {http://adsabs.harvard.edu/abs/2016ASSP...42..291D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deluca21extras,
       author = {{De Luca}, A. and {Salvaterra}, R. and {Belfiore}, A. and {Carpano}, S. and {D'Agostino}, D. and {Haberl}, F. and {Israel}, G.~L. and {Law-Green}, D. and {Lisini}, G. and {Marelli}, M. and {Novara}, G. and {Read}, A.~M. and {Rodriguez-Castillo}, G. and {Rosen}, S.~R. and {Salvetti}, D. and {Tiengo}, A. and {Vianello}, G. and {Watson}, M.~G. and {Delvaux}, C. and {Dickens}, T. and {Esposito}, P. and {Greiner}, J. and {H{\"a}mmerle}, H. and {Kreikenbohm}, A. and {Kreykenbohm}, S. and {Oertel}, M. and {Pizzocaro}, D. and {Pye}, J.~P. and {Sandrelli}, S. and {Stelzer}, B. and {Wilms}, J. and {Zagaria}, F.},
        title = "{The EXTraS project: Exploring the X-ray transient and variable sky}",
      journal = {\aap},
     keywords = {X-rays: general, methods: data analysis, astronomical databases: miscellaneous, catalogs, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = jun,
       volume = {650},
          eid = {A167},
        pages = {A167},
          doi = {10.1051/0004-6361/202039783},
archivePrefix = {arXiv},
       eprint = {2105.02895},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...650A.167D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

       author = {{De Luca}, A. and {Salvaterra}, R. and {Belfiore}, A. and {Carpano}, S. and {D'Agostino}, D. and {Haberl}, F. and {Israel}, G.~L. and {Law-Green}, D. and {Lisini}, G. and {Marelli}, M. and {Novara}, G. and {Read}, A.~M. and {Rodriguez-Castillo}, G. and {Rosen}, S.~R. and {Salvetti}, D. and {Tiengo}, A. and {Vianello}, G. and {Watson}, M.~G. and {Delvaux}, C. and {Dickens}, T. and {Esposito}, P. and {Greiner}, J. and {Haemmerle}, H. and {Kreikenbohm}, A. and {Kreykenbohm}, S. and {Oertel}, M. and {Pizzocaro}, D. and {Pye}, J.~P. and {Sandrelli}, S. and {Stelzer}, B. and {Wilms}, J. and {Zagaria}, F.},
        title = "{The EXTraS Project: Exploring the X-ray transient and variable sky}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.02895},
        pages = {arXiv:2105.02895},
archivePrefix = {arXiv},
       eprint = {2105.02895},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210502895D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{gourgouliatos18,
   author = {{Gourgouliatos}, K.~N. and {Esposito}, P.},
    title = "{Strongly magnetized pulsars: explosive events and evolution}",
    volume = 457,
    pages = {57-93},
    year = {2018},
  Publisher={Springer Nature Switzerland, Basel},
Booktitle = {The Physics and Astrophysics of Neutron Stars},
	Editor = {{Rezzolla}, L. and {Pizzochero}, P.~M. and {Jones}, D.~I. and {Rea}, N. and {Vida\~na}, I},
}

@article{demartino04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...415.1009D},
	Author = {{de Martino}, D. and {Matt}, G. and {Belloni}, T. and {Haberl}, F. and {Mukai}, K.},
	Doi = {10.1051/0004-6361:20034160},
	Eprint = {astro-ph/0311557},
	Journal = {\aap},
	Keywords = {accretion, accretion discs, binaries: close, stars: individual: RE 0751+144 (PQ Gem), RX J0558.0+5353 (V405 Aur), RX J1712.6-2414 (V2400 Oph), X-rays: binaries},
	Month = mar,
	Pages = {1009-1019},
	Title = {{BeppoSAX observations of soft X-ray intermediate polars}},
	Volume = 415,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20034160}}

@article{demartino05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..935D},
	Author = {{de Martino}, D. and {Matt}, G. and {Mukai}, K. and {Bonnet-Bidaud}, J.-M. and {G{\"a}nsicke}, B.~T. and {Gonzalez Perez}, J.~M. and {Haberl}, F. and {Mouchet}, M. and {Solheim}, J.-E.},
	Doi = {10.1051/0004-6361:20052761},
	Eprint = {astro-ph/0503470},
	Journal = {\aap},
	Keywords = {stars: binaries: close, stars: individual: HT Cam, stars: novae, cataclysmic variables},
	Month = jul,
	Pages = {935-945},
	Title = {{X-ray confirmation of the intermediate polar HT Cam}},
	Volume = 437,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052761}}

@article{demorest04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...615L.137D},
	Author = {{Demorest}, P. and {Ramachandran}, R. and {Backer}, D.~C. and {Ransom}, S.~M. and {Kaspi}, V. and {Arons}, J. and {Spitkovsky}, A.},
	Doi = {10.1086/426429},
	Eprint = {arXiv:astro-ph/0402025},
	Journal = {\apjl},
	Month = nov,
	Pages = {L137-L140},
	Title = {{Orientations of Spin and Magnetic Dipole Axes of Pulsars in the J0737-3039 Binary Based on Polarimetry Observations at the Green Bank Telescope}},
	Volume = 615,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426429}}

@article{deneva09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702L.177D},
	Archiveprefix = {arXiv},
	Author = {{Deneva}, J.~S. and {Cordes}, J.~M. and {Lazio}, T.~J.~W.},
	Doi = {10.1088/0004-637X/702/2/L177},
	Eprint = {0908.1331},
	Journal = {\apjl},
	Keywords = {pulsars: general, pulsars: individual: J1746{\ndash}2850I J1746{\ndash}2850II J1745{\ndash}2910},
	Month = sep,
	Pages = {L177-L181},
	Primaryclass = {astro-ph.SR},
	Title = {{Discovery of Three Pulsars from a Galactic Center Pulsar Population}},
	Volume = 702,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/702/2/L177}}

@article{denhartog06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2006A%26A...451..587D&db_key=AST},
	Author = {{den Hartog}, P.~R. and {Hermsen}, W. and {Kuiper}, L. and {Vink}, J. and {in't Zand}, J.~J.~M. and {Collmar}, W.},
	Doi = {10.1051/0004-6361:20054711},
	Journal = {\aap},
	Month = may,
	Pages = {587-602},
	Title = {{INTEGRAL survey of the Cassiopeia region in hard X rays}},
	Volume = 451,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054711}}

@ARTICLE{denhartog08,
   author = {{den Hartog}, P.~R. and {Kuiper}, L. and {Hermsen}, W. and {Kaspi}, V.~M. and 
	{Dib}, R. and {Kn{\"o}dlseder}, J. and {Gavriil}, F.~P.},
    title = "{Detailed high-energy characteristics of AXP 4U 0142+61. Multi-year observations with INTEGRAL, RXTE, XMM-Newton, and ASCA}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0804.1640},
 keywords = {stars: neutron, stars: pulsars: individual: <ASTROBJ>4U 0142+61</ASTROBJ>, gamma rays: observations},
     year = 2008,
    month = oct,
   volume = 489,
    pages = {245-261},
      doi = {10.1051/0004-6361:200809390},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489..245D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dkh08,
   author = {{den Hartog}, P.~R. and {Kuiper}, L. and {Hermsen}, W.},
    title = "{Detailed high-energy characteristics of AXP 1RXS J170849-400910. Probing the magnetosphere using INTEGRAL, RXTE, and XMM-Newton}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0804.1641},
 keywords = {stars: neutron, X-rays: individuals:, 1RXS J170849-400910, gamma rays:, observations, X-rays: individuals: 4U 0142+61},
     year = 2008,
    month = oct,
   volume = 489,
    pages = {263-279},
      doi = {10.1051/0004-6361:200809772},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489..263D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{denherder01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L...7D},
	Author = {{den Herder}, J.~W. and {Brinkman}, A.~C. and {Kahn}, S.~M. and {Branduardi-Raymont}, G. and {Thomsen}, K. and {Aarts}, H. and {Audard}, M. and {Bixler}, J.~V. and {den Boggende}, A.~J. and {Cottam}, J. and {Decker}, T. and {Dubbeldam}, L. and {Erd}, C. and {Goulooze}, H. and {G{\"u}del}, M. and {Guttridge}, P. and {Hailey}, C.~J. and {Janabi}, K.~A. and {Kaastra}, J.~S. and {de Korte}, P.~A.~J. and {van Leeuwen}, B.~J. and {Mauche}, C. and {McCalden}, A.~J. and {Mewe}, R. and {Naber}, A. and {Paerels}, F.~B. and {Peterson}, J.~R. and {Rasmussen}, A.~P. and {Rees}, K. and {Sakelliou}, I. and {Sako}, M. and {Spodek}, J. and {Stern}, M. and {Tamura}, T. and {Tandy}, J. and {de Vries}, C.~P. and {Welch}, S. and {Zehnder}, A.},
	Doi = {10.1051/0004-6361:20000058},
	Journal = {\aap},
	Keywords = {SPACE VEHICLES: INSTRUMENTS, REFLECTION GRATINGS, $\backslash$TEXTIT$\{$XMM-NEWTON$\}$},
	Month = jan,
	Pages = {L7-L17},
	Title = {{The Reflection Grating Spectrometer on board XMM-Newton}},
	Volume = 365,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000058}}

@ARTICLE{dessart10,
   author = {{Dessart}, L. and {Hillier}, D.~J.},
    title = "{Supernova radiative-transfer modelling: a new approach using non-local thermodynamic equilibrium and full time dependence}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.2557},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, stars: atmospheres, supernovae: general, supernovae: individual: SN 1987A},
     year = 2010,
    month = jul,
   volume = 405,
    pages = {2141-2160},
      doi = {10.1111/j.1365-2966.2010.16611.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.2141D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{deugarte11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3518....1D},
	Author = {{de Ugarte Postigo}, A. and {Munoz-Darias}, T.},
	Journal = {Astron. Tel.},
	Keywords = {Optical, Soft Gamma-ray Repeater},
	Month = jul,
	Title = {{Swift J1822.3-1606: Optical spectroscopy of the counterpart candidates from the 10.4m GTC}},
	Volume = 3518,
	Year = 2011}

@book{devaucouleurs76,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1976srcb.book.....D},
	Author = {{de Vaucouleurs}, G. and {de Vaucouleurs}, A. and {Corwin}, Jr., H.~G.},
	Publisher = {University of Texas Press, Austin},
	Title = {{Second reference catalogue of bright galaxies}},
	Year = 1976}

@book{devaucouleurs91,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1991rc3..book.....D},
	Author = {{de Vaucouleurs}, G. and {de Vaucouleurs}, A. and {Corwin}, Jr., H.~G. and {Buta}, R.~J. and {Paturel}, G. and {Fouqu{\'e}}, P.},
	Publisher = {Springer, New York},
	Title = {{Third Reference Catalogue of Bright Galaxies}},
	Year = 1991}

@article{devillard97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997Msngr..87...19D},
	Author = {{Devillard}, N.},
	Journal = {The Messenger},
	Keywords = {Methods of Reduction: Image Processing},
	Month = mar,
	Pages = {19-20},
	Title = {{The eclipse software.}},
	Volume = 87,
	Year = 1997}

@inproceedings{dhawan06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006smqw.confE..52D},
	Author = {{Dhawan}, V. and {Mioduszewski}, A. and {Rupen}, M.},
	Booktitle = {VI Microquasar Workshop: Microquasars and Beyond},
	Title = {{LS I +61 303 is a Be-Pulsar binary, not a Microquasar}},
	Year = 2006}

@article{diaztrigo06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..179D},
	Author = {{D{\'{\i}}az Trigo}, M. and {Parmar}, A.~N. and {Boirin}, L. and {M{\'e}ndez}, M. and {Kaastra}, J.~S.},
	Doi = {10.1051/0004-6361:20053586},
	Eprint = {arXiv:astro-ph/0509342},
	Journal = {\aap},
	Keywords = {X-rays: individual: EXO 0748-676, , XB 1254-690, X 1624-490, MXB 1659-298, 4U 1746-371, XB 1916-053, X-rays binaries, accretion, accretion disks},
	Month = jan,
	Pages = {179-195},
	Title = {{Spectral changes during dipping in low-mass X-ray binaries due to highly-ionized absorbers}},
	Volume = 445,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053586}}

@article{dib08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673.1044D},
	Author = {{Dib}, R. and {Kaspi}, V.~M. and {Gavriil}, F.~P.},
	Doi = {10.1086/524653},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: 1E 1841-045, pulsars: individual (RXS J170849.0-400910), Stars: Neutron, X-Rays: Stars},
	Month = feb,
	Pages = {1044-1061},
	Title = {{Glitches in Anomalous X-Ray Pulsars}},
	Volume = 673,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/524653}}

@ARTICLE{dib14,
   author = {{Dib}, R. and {Kaspi}, V.~M.},
    title = "{16 yr of RXTE Monitoring of Five Anomalous X-Ray Pulsars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1401.3085},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: 1E 1841{\ndash}045 RXS J170849.0{\ndash}400910 1E 2259+586 4U 0142+61 1E 1048.1{\ndash}5937, stars: neutron, X-rays: stars},
     year = 2014,
    month = mar,
   volume = 784,
      eid = {37},
    pages = {37},
      doi = {10.1088/0004-637X/784/1/37},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...784...37D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dickey90,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1990ARA%26A..28..215D&db_key=AST},
	Author = {{Dickey}, J.~M. and {Lockman}, F.~J.},
	Doi = {10.1146/annurev.aa.28.090190.001243},
	Journal = {\araa},
	Pages = {215-261},
	Title = {{H I in the Galaxy}},
	Volume = 28,
	Year = 1990,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.28.090190.001243}}

@article{dimai05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005IAUC.8588....2D},
	Author = {{Dimai}, A. and {Migliardi}, M. and {Manzini}, F.},
	Journal = {\iaucirc},
	Month = aug,
	Pages = {2},
	Title = {{Supernova 2005dl in NGC 2276}},
	Volume = 8588,
	Year = 2005}

@article{distefano94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...423..274D},
	Author = {{Di Stefano}, R. and {Rappaport}, S.},
	Doi = {10.1086/173805},
	Journal = {\apj},
	Keywords = {Accretion Disks, Astronomical Models, Binary Stars, Cataclysmic Variables, Globular Clusters, Stellar Evolution, Monte Carlo Method, Stellar Luminosity, Two Body Problem, X Ray Sources},
	Month = mar,
	Pages = {274-293},
	Title = {{Predictions of a population of cataclysmic variables in globular clusters}},
	Volume = 423,
	Year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/173805}}

@inproceedings{distefano97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ASIC..486..147D},
	Author = {{Di Stefano}, R. and {Nelson}, L.~A. and {Lee}, W. and {Wood}, H.~T. and {Rappaport}, S.},
	Booktitle = {NATO Advanced Science Institutes (ASI) Series C},
	Editor = {{Ruiz-Lapuente}, P. and {Canal}, R. and {Isern}, J.},
	Pages = {147},
	Publisher = {Kluwer Academic Publishers (Dordrecht)},
	Series = {Series C},
	Title = {{Luminous supersoft X-ray sources as Type Ia progenitors}},
	Volume = 486,
	Year = 1997}

@article{dobrotka14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.1714D},
	Archiveprefix = {arXiv},
	Author = {{Dobrotka}, A. and {Mineshige}, S. and {Ness}, J.-U.},
	Doi = {10.1093/mnras/stt2311},
	Eprint = {1311.7487},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, turbulence, stars: dwarf novae, stars: individual: RU Peg, X-rays: binaries},
	Month = feb,
	Pages = {1714-1723},
	Primaryclass = {astro-ph.SR},
	Title = {{Resolving different sources of fast X-ray variability of the dwarf nova RU Peg in quiescence}},
	Volume = 438,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt2311}}

@ARTICLE{dopita12,
   author = {{Dopita}, M.~A. and {Payne}, J.~L. and {Filipovi{\'c}}, M.~D. and 
	{Pannuti}, T.~G.},
    title = "{The physical parameters of the microquasar S26 in the Sculptor Group galaxy NGC 7793}",
  journal = {\mnras},
 keywords = {stars: winds, outflows, ISM: abundances, ISM: bubbles, ISM: jets and outflows, galaxies: individual: NGC 7793, X-rays: binaries},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {956-967},
      doi = {10.1111/j.1365-2966.2012.21947.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427..956D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{doroshenko11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A..52D},
	Archiveprefix = {arXiv},
	Author = {{Doroshenko}, V. and {Santangelo}, A. and {Suleimanov}, V.},
	Doi = {10.1051/0004-6361/201116482},
	Eid = {A52},
	Eprint = {1102.5254},
	Journal = {\aap},
	Keywords = {X-rays: binaries, pulsars: individual: Vela X-1},
	Month = may,
	Pages = {A52},
	Primaryclass = {astro-ph.HE},
	Title = {{Witnessing the magnetospheric boundary at work in Vela X-1}},
	Volume = 529,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201116482}}

@article{doroshenko12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...540L...1D},
	Archiveprefix = {arXiv},
	Author = {{Doroshenko}, V. and {Santangelo}, A. and {Kreykenbohm}, I. and {Doroshenko}, R.},
	Doi = {10.1051/0004-6361/201218878},
	Eid = {L1},
	Eprint = {1202.6271},
	Journal = {\aap},
	Keywords = {X-rays: binaries, pulsars: individual: X Persei, stars: neutron},
	Month = apr,
	Pages = {L1},
	Primaryclass = {astro-ph.HE},
	Title = {{The hard X-ray emission of X Persei}},
	Volume = 540,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201218878}}

@article{dsdk12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A..19D},
	Archiveprefix = {arXiv},
	Author = {{Doroshenko}, V. and {Santangelo}, A. and {Ducci}, L. and {Klochkov}, D.},
	Doi = {10.1051/0004-6361/201220085},
	Eid = {A19},
	Eprint = {1210.4428},
	Journal = {\aap},
	Keywords = {stars: neutron, pulsars: individual: 4U 1907+09, X-rays: binaries},
	Month = dec,
	Pages = {A19},
	Primaryclass = {astro-ph.HE},
	Title = {{Supergiant, fast, but not so transient 4U 1907+09}},
	Volume = 548,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201220085}}
	
@ARTICLE{dosopoulou16,
       author = {{Dosopoulou}, Fani and {Kalogera}, Vicky},
        title = "{Orbital Evolution of Mass-transferring Eccentric Binary Systems. II. Secular Evolution}",
      journal = {\apj},
     keywords = {binaries: close, binaries: general, planets and satellites: dynamical evolution and stability, stars: kinematics and dynamics, stars: mass-loss, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = jul,
       volume = {825},
       number = {1},
          eid = {71},
        pages = {71},
          doi = {10.3847/0004-637X/825/1/71},
archivePrefix = {arXiv},
       eprint = {1603.06593},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...825...71D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{downes01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001PASP..113..764D},
	Author = {{Downes}, R.~A. and {Webbink}, R.~F. and {Shara}, M.~M. and {Ritter}, H. and {Kolb}, U. and {Duerbeck}, H.~W.},
	Doi = {10.1086/320802},
	Eprint = {astro-ph/0102302},
	Journal = {\pasp},
	Keywords = {Atlases, Catalogs, cataclysmic variables},
	Month = jun,
	Pages = {764-768},
	Title = {{A Catalog and Atlas of Cataclysmic Variables: The Living Edition}},
	Volume = 113,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320802}}

@article{draine03,
   author = {{Draine}, B.~T.},
    title = "{Scattering by Interstellar Dust Grains. II. X-Rays}",
  journal = {\apj},
 keywords = {ISM: Dust, Extinction, Polarization, Scattering, Ultraviolet: ISM, X-Rays: ISM},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1026-1037},
      doi = {10.1086/379123},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598.1026D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{drake14,
       author = {{Drake}, A.~J. and {G{\"a}nsicke}, B.~T. and {Djorgovski}, S.~G. and
         {Wils}, P. and {Mahabal}, A.~A. and {Graham}, M.~J. and {Yang}, T. -C. and
         {Williams}, R. and {Catelan}, M. and {Prieto}, J.~L. and {Donalek}, C. and
         {Larson}, S. and {Christensen}, E.},
        title = "{Cataclysmic variables from the Catalina Real-time Transient Survey}",
      journal = {\mnras},
     keywords = {stars: distances, stars: dwarf novae, novae, cataclysmic variables, galaxies: stellar content, Astrophysics - Solar and Stellar Astrophysics},
         year = "2014",
        month = "Jun",
       volume = {441},
       number = {2},
        pages = {1186-1200},
          doi = {10.1093/mnras/stu639},
archivePrefix = {arXiv},
       eprint = {1404.3732},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.441.1186D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{drave13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433..528D},
	Archiveprefix = {arXiv},
	Author = {{Drave}, S.~P. and {Bird}, A.~J. and {Sidoli}, L. and {Sguera}, V. and {McBride}, V.~A. and {Hill}, A.~B. and {Bazzano}, A. and {Goossens}, M.~E.},
	Doi = {10.1093/mnras/stt754},
	Eprint = {1305.0430},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, stars: winds, outflows, X-rays: binaries, X-rays: individual: IGR J16418-4532},
	Month = jul,
	Pages = {528-542},
	Primaryclass = {astro-ph.HE},
	Title = {{INTEGRAL and XMM-Newton observations of IGR J16418-4532: evidence of accretion regime transitions in a supergiant fast X-ray transient}},
	Volume = 433,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt754}}

@article{drave14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1401.3570D},
	Archiveprefix = {arXiv},
	Author = {{Drave}, S.~P. and {Bird}, A.~J. and {Sidoli}, L. and {Sguera}, V. and {Bazzano}, A. and {Hill}, A.~B. and {Goossens}, M.~E.},
	Eprint = {1401.3570},
	Journal = {\mnras},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = apr,
	Pages = {2175-2185},
	Primaryclass = {astro-ph.HE},
	Title = {{New insights on accretion in Supergiant Fast X-ray Transients from XMM-Newton and INTEGRAL observations of IGR J17544\$-\$2619}},
	Volume = 439,
	Year = 2014}

@article{drew14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.440.2036D},
	Archiveprefix = {arXiv},
	Author = {{Drew}, J.~E. and {Gonzalez-Solares}, E. and {Greimel}, R. and {Irwin}, M.~J. and {K{\"u}pc{\"u} Yoldas}, A. and {Lewis}, J. and {Barentsen}, G. and {Eisl{\"o}ffel}, J. and {Farnhill}, H.~J. and {Martin}, W.~E. and {Walsh}, J.~R. and {Walton}, N.~A. and {Mohr-Smith}, M. and {Raddi}, R. and {Sale}, S.~E. and {Wright}, N.~J. and {Groot}, P. and {Barlow}, M.~J. and {Corradi}, R.~L.~M. and {Drake}, J.~J. and {Fabregat}, J. and {Frew}, D.~J. and {G{\"a}nsicke}, B.~T. and {Knigge}, C. and {Mampaso}, A. and {Morris}, R.~A.~H. and {Naylor}, T. and {Parker}, Q.~A. and {Phillipps}, S. and {Ruhland}, C. and {Steeghs}, D. and {Unruh}, Y.~C. and {Vink}, J.~S. and {Wesson}, R. and {Zijlstra}, A.~A.},
	Doi = {10.1093/mnras/stu394},
	Eprint = {1402.7024},
	Journal = {\mnras},
	Keywords = {surveys, stars: general, H II regions, planetary nebulae: general, Galaxy: bulge, Galaxy: disc},
	Month = may,
	Pages = {2036-3058},
	Primaryclass = {astro-ph.GA},
	Title = {{The VST Photometric H{$\alpha$} Survey of the Southern Galactic Plane and Bulge (VPHAS+)}},
	Volume = 440,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu394}}

@ARTICLE{drury12,
   author = {{Drury}, L.~O.~'.},
    title = "{Origin of cosmic rays}",
  journal = {Astroparticle Physics},
 primaryClass = "astro-ph.HE",
     year = 2012,
    month = dec,
   volume = 39,
    pages = {52-60},
      doi = {10.1016/j.astropartphys.2012.02.006},
   adsurl = {http://adsabs.harvard.edu/abs/2012APh....39...52D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{dubus99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.303..139D},
	Author = {{Dubus}, G. and {Lasota}, J.-P. and {Hameury}, J.-M. and {Charles}, P.},
	Doi = {10.1046/j.1365-8711.1999.02212.x},
	Eprint = {arXiv:astro-ph/9809036},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, INSTABILITIES, BINARIES : CLOSE, X-RAYS: GENERAL},
	Month = feb,
	Pages = {139-147},
	Title = {{X-ray irradiation in low-mass binary systems}},
	Volume = 303,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02212.x}}

@article{dubus06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006A%26A...456..801D},
	Author = {{Dubus}, G.},
	Doi = {10.1051/0004-6361:20054779},
	Eprint = {arXiv:astro-ph/0605287},
	Journal = {\aap},
	Month = sep,
	Pages = {801-817},
	Title = {{Gamma-ray binaries: pulsars in disguise?}},
	Volume = 456,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054779}}

@ARTICLE{dubus13,
   author = {{Dubus}, G.},
    title = "{Gamma-ray binaries and related systems}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1307.7083},
 primaryClass = "astro-ph.HE",
 keywords = {Acceleration of particles, Radiation mechanisms: non-thermal, Stars: massive, Novae, Pulsars: general, ISM: jets and outflows, Gamma rays: stars, X-rays: binaries},
     year = 2013,
    month = aug,
   volume = 21,
      eid = {64},
    pages = {64},
      doi = {10.1007/s00159-013-0064-5},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26ARv..21...64D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{duncan97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997MNRAS.287..722D&db_key=AST},
	Author = {{Duncan}, A.~R. and {Stewart}, R.~T. and {Haynes}, R.~F. and {Jones}, K.~L.},
	Journal = {\mnras},
	Month = jun,
	Pages = {722-738},
	Title = {{Supernova remnant candidates from the Parkes 2.4-GHz survey}},
	Volume = 287,
	Year = 1997}

@ARTICLE{duncan98,
   author = {{Duncan}, R.~C.},
    title = "{Global Seismic Oscillations in Soft Gamma Repeaters}",
  journal = {\apjl},
   eprint = {astro-ph/9803060},
 keywords = {STARS: MAGNETIC FIELDS, STARS: NEUTRON, STARS: OSCILLATIONS, X-RAYS: STARS, Stars: Magnetic Fields, Stars: Neutron, Stars: Oscillations, X-Rays: Stars},
     year = 1998,
    month = may,
   volume = 498,
    pages = {L45-L49},
      doi = {10.1086/311303},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...498L..45D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{duplain08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7019E..45D},
	Author = {{DuPlain}, R. and {Ransom}, S. and {Demorest}, P. and {Brandt}, P. and {Ford}, J. and {Shelton}, A.~L.},
	Booktitle = {Advanced Software and Control for Astronomy II, eds. {Bridger}, A. and {Radzwill}, N. Proceedings of the SPIE. SPIE, Bellingham WA},
	Doi = {10.1117/12.790003},
	Month = aug,
	Pages = {70191D1-70191D10},
	Series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	Title = {{Launching GUPPI: the Green Bank Ultimate Pulsar Processing Instrument}},
	Volume = 7019,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.790003}}

@article{durant05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...628L.135D},
	Author = {{Durant}, M. and {van Kerkwijk}, M.~H.},
	Doi = {10.1086/432882},
	Eprint = {arXiv:astro-ph/0506512},
	Journal = {\apjl},
	Month = aug,
	Pages = {L135-L138},
	Title = {{Possible Optical Detection of the Anomalous X-Ray Pulsar CXOU J010043.1-721134}},
	Volume = 628,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432882}}

@ARTICLE{dk05,
   author = {{Durant}, M. and {van Kerkwijk}, M.~H.},
    title = "{The Broadband Spectrum and Infrared Variability of the Magnetar AXP 1E 1048.1-5937}",
  journal = {\apj},
   eprint = {astro-ph/0502027},
 keywords = {Stars: Pulsars: Individual: Alphanumeric: 1E 1048.1-5937},
     year = 2005,
    month = jul,
   volume = 627,
    pages = {376-382},
      doi = {10.1086/429714},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...627..376D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{durant08,
	Author = {{Durant}, M. and {van Kerkwijk}, M.~H.},
	Eprint = {0711.3985},
	Journal = {ApJ preprint doi:10.1086/'529017'},
	Title = {{A search for the optical counterpart to the magnetar CXOU J010043.1-721134}},
	Year = 2008}

@article{durant11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...742...77D},
	Archiveprefix = {arXiv},
	Author = {{Durant}, M. and {Kargaltsev}, O. and {Pavlov}, G.~G.},
	Doi = {10.1088/0004-637X/742/2/77},
	Eid = {77},
	Eprint = {1108.3340},
	Journal = {\apj},
	Keywords = {stars: neutron, X-rays: individual: SGR 0418+5729},
	Month = dec,
	Pages = {77},
	Primaryclass = {astro-ph.HE},
	Title = {{Search for the Optical Counterpart to SGR 0418+5729}},
	Volume = 742,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/742/2/77}}

@article{duval81,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1981A%26A....98..352D},
	Author = {{Duval}, M.~F.},
	Journal = {\aap},
	Keywords = {ASTRONOMICAL PHOTOGRAPHY, ASTRONOMICAL PHOTOMETRY, ASTRONOMICAL SPECTROSCOPY, GALACTIC ROTATION, GALAXIES, GALACTIC RADIATION, H ALPHA LINE, LUMINOUS INTENSITY, VELOCITY DISTRIBUTION},
	Month = may,
	Pages = {352-366},
	Title = {{Photometric and kinematic study of the double system NGC 4485-4490}},
	Volume = 98,
	Year = 1981}

@book{eddington26,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1926ics..book.....E&db_key=AST},
	Author = {{Eddington}, A.~S.},
	Publisher = {Cambridge: Cambridge University Press},
	Title = {{The Internal Constitution of the Stars}},
	Year = 1926}

@article{edgar04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004NewAR..48..843E},
	Author = {{Edgar}, R.},
	Doi = {10.1016/j.newar.2004.06.001},
	Eprint = {astro-ph/0406166},
	Journal = {\nar},
	Month = sep,
	Pages = {843-859},
	Title = {{A review of Bondi-Hoyle-Lyttleton accretion}},
	Volume = 48,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.newar.2004.06.001}}

@article{edge04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353.1286E},
	Author = {{Edge}, W.~R.~T. and {Coe}, M.~J. and {Galache}, J.~L. and {McBride}, V.~A. and {Corbet}, R.~H.~D. and {Markwardt}, C.~B. and {Laycock}, S.},
	Doi = {10.1111/j.1365-2966.2004.08150.x},
	Eprint = {arXiv:astro-ph/0406580},
	Journal = {\mnras},
	Keywords = {stars: emission-line, Be, Magellanic Clouds, X-rays: binaries},
	Month = oct,
	Pages = {1286-1292},
	Title = {{Three new X-ray pulsars detected in the Small Magellanic Cloud and the positions of two other known pulsars determined}},
	Volume = 353,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08150.x}}

@article{edmonds03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...596.1177E},
	Author = {{Edmonds}, P.~D. and {Gilliland}, R.~L. and {Heinke}, C.~O. and {Grindlay}, J.~E.},
	Doi = {10.1086/378193},
	Eprint = {astro-ph/0307187},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Galaxy: Globular Clusters: Individual: Name: 47 Tucanae, Stars: Novae, Cataclysmic Variables, Stars: Chromospheres, Techniques: Photometric, X-Rays: Binaries},
	Month = oct,
	Pages = {1177-1196},
	Title = {{An Extensive Census of Hubble Space Telescope Counterparts to Chandra X-Ray Sources in the Globular Cluster 47 Tucanae. I. Astrometry and Photometry}},
	Volume = 596,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378193}}

@article{egh03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...596.1197E},
	Author = {{Edmonds}, P.~D. and {Gilliland}, R.~L. and {Heinke}, C.~O. and {Grindlay}, J.~E.},
	Doi = {10.1086/378194},
	Eprint = {astro-ph/0307189},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Galaxy: Globular Clusters: Individual: Name: 47 Tucanae, Stars: Novae, Cataclysmic Variables, Techniques: Photometric, X-Rays: Binaries},
	Month = oct,
	Pages = {1197-1219},
	Title = {{An Extensive Census of Hubble Space Telescope Counterparts to Chandra X-Ray Sources in the Globular Cluster 47 Tucanae. II. Time Series and Analysis}},
	Volume = 596,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378194}}

@article{eggleton83,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983ApJ...268..368E&db_key=AST},
	Author = {{Eggleton}, P.~P.},
	Doi = {10.1086/160960},
	Journal = {\apj},
	Month = may,
	Pages = {368},
	Title = {{Approximations to the radii of Roche lobes}},
	Volume = 268,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160960}}

@article{eichler89,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1989ApJ...336..360E},
	Author = {{Eichler}, D. and {Cheng}, A.~F.},
	Doi = {10.1086/167015},
	Journal = {\apj},
	Month = jan,
	Pages = {360-366},
	Title = {{Thermal afterglow from transient energy release in neutron stars}},
	Volume = 336,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/167015}}

@article{eichler06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006astro.ph.11747E},
	Author = {{Eichler}, D. and {Lyubarsky}, Y. and {Kouveliotou}, C. and {Wilson}, C.~A.},
	Eprint = {astro-ph/0611747},
	Journal = {preprint (astro-ph/0611747)},
	Keywords = {Astrophysics},
	Month = nov,
	Title = {{Long Term Cooling of Magnetar Crusts}},
	Year = 2006}

@article{eikenberry01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...563L.133E&db_key=AST},
	Author = {{Eikenberry}, S.~S. and {Garske}, M.~A. and {Hu}, D. and {Jackson}, M.~A. and {Patel}, S.~G. and {Barry}, D.~J. and {Colonno}, M.~R. and {Houck}, J.~R.},
	Journal = {\apjl},
	Month = dec,
	Pages = {L133-L137},
	Title = {{Possible Infrared Counterparts to the Soft Gamma-Ray Repeater SGR 1806-20}},
	Volume = 563,
	Year = 2001}

@ARTICLE{elfritz16,
   author = {{Elfritz}, J.~G. and {Pons}, J.~A. and {Rea}, N. and {Glampedakis}, K. and 
	{Vigan{\`o}}, D.},
    title = "{Simulated magnetic field expulsion in neutron star cores}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1512.07151},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: magnetars, stars: magnetic field, stars: neutron},
     year = 2016,
    month = mar,
   volume = 456,
    pages = {4461-4474},
      doi = {10.1093/mnras/stv2963},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.4461E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{elmegreen91,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...244...52E},
	Author = {{Elmegreen}, D.~M. and {Sundin}, M. and {Sundelius}, B. and {Elmegreen}, B.},
	Journal = {\aap},
	Keywords = {Codes, Computerized Simulation, Galactic Structure, Spiral Galaxies, Star Formation, H Alpha Line, Infrared Astronomy Satellite},
	Month = apr,
	Pages = {52-63},
	Title = {{Properties and simulations of interacting spiral galaxies with transient 'ocular' shapes}},
	Volume = 244,
	Year = 1991}

@article{enoto09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...693L.122E},
	Archiveprefix = {arXiv},
	Author = {{Enoto}, T. and {Nakagawa}, Y.~E. and {Rea}, N. and {Esposito}, P. and {G{\"o}tz}, D. and {Hurley}, K. and {Israel}, G.~L. and {Kokubun}, M. and {Makishima}, K. and {Mereghetti}, S. and {Murakami}, H. and {Nakazawa}, K. and {Sakamoto}, T. and {Stella}, L. and {Tiengo}, A. and {Turolla}, R. and {Yamada}, S. and {Yamaoka}, K. and {Yoshida}, A. and {Zane}, S.},
	Doi = {10.1088/0004-637X/693/2/L122},
	Eprint = {0901.3453},
	Journal = {\apjl},
	Keywords = {pulsars: individual: SGR 0501+4516, stars: magnetic fields, X-rays: stars},
	Month = mar,
	Pages = {L122-L126},
	Title = {{Suzaku Observation of the New Soft Gamma Repeater SGR 0501+4516 in Outburst}},
	Volume = 693,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/693/2/L122}}

@article{enoto14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...786..127E},
	Archiveprefix = {arXiv},
	Author = {{Enoto}, T. and {Sasano}, M. and {Yamada}, S. and {Tamagawa}, T. and {Makishima}, K. and {Pottschmidt}, K. and {Marcu}, D. and {Corbet}, R.~H.~D. and {Fuerst}, F. and {Wilms}, J.},
	Doi = {10.1088/0004-637X/786/2/127},
	Eid = {127},
	Eprint = {1404.0134},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, binaries: symbiotic, magnetic fields, stars: individual: 3A 1954+319 4U 1954+319, stars: neutron, X-rays : binaries},
	Month = may,
	Pages = {127},
	Primaryclass = {astro-ph.HE},
	Title = {{Spectral and Timing Nature of the Symbiotic X-Ray Binary 4U 1954+319: The Slowest Rotating Neutron Star in an X-Ray Binary System}},
	Volume = 786,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/786/2/127}}

@ARTICLE{enoto17,
   author = {{Enoto}, T. and {Shibata}, S. and {Kitaguchi}, T. and {Suwa}, Y. and 
	{Uchide}, T. and {Nishioka}, H. and {Kisaka}, S. and {Nakano}, T. and 
	{Murakami}, H. and {Makishima}, K.},
    title = "{Magnetar Broadband X-Ray Spectra Correlated with Magnetic Fields: Suzaku Archive of SGRs and AXPs Combined with NuSTAR, Swift, and RXTE}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1704.07018},
 primaryClass = "astro-ph.HE",
 keywords = {catalogs, pulsars: general, stars: magnetars, stars: magnetic field, stars: neutron, X-rays: stars},
     year = 2017,
    month = jul,
   volume = 231,
      eid = {8},
    pages = {8},
      doi = {10.3847/1538-4365/aa6f0a},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJS..231....8E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ertan09,
   author = {{Ertan}, {\"U}. and {Ek{\c s}i}, K.~Y. and {Erkut}, M.~H. and 
	{Alpar}, M.~A.},
    title = "{On the Evolution of Anomalous X-ray Pulsars and Soft Gamma-ray Repeaters with Fall Back Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0907.3222},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, pulsars: individual: AXPs, stars: neutron, X-rays: bursts},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {1309-1320},
      doi = {10.1088/0004-637X/702/2/1309},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702.1309E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{esposito07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2007A%26A...461..605E&db_key=AST},
	Author = {{Esposito}, P. and {Mereghetti}, S. and {Tiengo}, A. and {Sidoli}, L. and {Feroci}, M. and {Woods}, P.},
	Doi = {10.1051/0004-6361:20065529},
	Eprint = {astro-ph/0609078},
	Journal = {\aap},
	Month = jan,
	Pages = {605-612},
	Title = {{Five years of SGR 1900+14 observations with BeppoSAX}},
	Volume = 461,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065529}}

@article{etdm07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...467L..45E},
	Author = {{Esposito}, P. and {Tiengo}, A. and {De Luca}, A. and {Mattana}, F.},
	Doi = {10.1051/0004-6361:20077480},
	Eprint = {arXiv:0704.0205},
	Journal = {\aap},
	Month = may,
	Pages = {L45-L48},
	Title = {{Discovery of X-ray emission from the young radio pulsar PSR J1357-6429}},
	Volume = 467,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077480}}

@article{ecp07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...474..575E},
	Author = {{Esposito}, P. and {Caraveo}, P.~A. and {Pellizzoni}, A. and {De Luca}, A. and {Gehrels}, N. and {Marelli}, M.~A.},
	Doi = {10.1051/0004-6361:20078334},
	Eprint = {arXiv:0708.3330},
	Journal = {\aap},
	Month = nov,
	Pages = {575-578},
	Title = {{Swift/XRT monitoring of five orbital cycles of LS I +61{\deg} 303}},
	Volume = 474,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078334}}

@article{emt07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...476..321E},
	Author = {{Esposito}, P. and {Mereghetti}, S. and {Tiengo}, A. and {Zane}, S. and {Turolla}, R. and {G{\"o}tz}, D. and {Rea}, N. and {Kawai}, N. and {Ueno}, M. and {Israel}, G.~L. and {Stella}, L. and {Feroci}, M.},
	Doi = {10.1051/0004-6361:20078562},
	Eprint = {arXiv:0710.2789},
	Journal = {\aap},
	Month = dec,
	Pages = {321-330},
	Title = {{SGR 1806-20 about two years after the giant flare: Suzaku, XMM-Newton and INTEGRAL observations}},
	Volume = 476,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078562}}

@article{esposito08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.384..225E},
	Author = {{Esposito}, P. and {De Luca}, A. and {Tiengo}, A. and {Paizis}, A. and {Mereghetti}, S. and {Caraveo}, P.~A.},
	Doi = {10.1111/j.1365-2966.2007.12677.x},
	Eprint = {arXiv:0711.0827},
	Journal = {\mnras},
	Month = feb,
	Pages = {225-229},
	Title = {{Unveiling the nature of RXJ0002+6246 with XMM-Newton}},
	Volume = 384,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12677.x}}

@article{esposito08gcn,
	Author = {{Esposito}, P. and {Luca}, A.~D. and {Tiengo}, A. and {Vianello}, G. and {Page}, K.~L.},
	Journal = {GCN Circ. 7750},
	Title = {{GRB 080514B: second epoch Swift XRT data confirms the X-ray afterglow}},
	Year = 2008}

@article{eiz08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390L..34E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Zane}, S. and {Senziani}, F. and {Starling}, R.~L.~C. and {Rea}, N. and {Palmer}, D.~M. and {Gehrels}, N. and {Tiengo}, A. and {De Luca}, A. and {G{\"o}tz}, D. and {Mereghetti}, S. and {Romano}, P. and {Sakamoto}, T. and {Barthelmy}, S.~D. and {Stella}, L. and {Turolla}, R. and {Feroci}, M. and {Mangano}, V.},
	Doi = {10.1111/j.1745-3933.2008.00530.x},
	Eprint = {0807.1658},
	Journal = {\mnras},
	Keywords = {stars: neutron , X-rays: bursts , X-rays: individual: SGR1627-41},
	Month = oct,
	Pages = {L34-L38},
	Title = {{The 2008 May burst activation of SGR1627-41}},
	Volume = 390,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2008.00530.x}}

@article{esposito08_atel,
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Rea}, N. and {Krimm}, H.~A. and {Palmer}, D.~M. and {Gehrels}, N. and {Helmy}, S.~D.~B. and {Mereghetti}, S. and {Tiengo}, A. and {G\"otz}, D.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients, Variables},
	Month = oct,
	Title = {{Swift XRT follow-up of the transient AXP 1E1547.0-5408 in outburst}},
	Volume = 1763,
	Year = 2008}

@article{esposito09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690L.105E},
	Author = {{Esposito}, P. and {Tiengo}, A. and {Mereghetti}, S. and {Israel}, G.~L. and {De Luca}, A. and {G{\"o}tz}, D. and {Rea}, N. and {Turolla}, R. and {Zane}, S.},
	Doi = {10.1088/0004-637X/690/2/L105},
	Journal = {\apjl},
	Keywords = {ISM: individual: G337.0{\ndash}0.1, stars: neutron, supernova remnants, X-rays: individual: SGR 1627{\ndash}41, X-rays: stars},
	Month = jan,
	Pages = {L105-L109},
	Title = {{Xmm-Newton Discovery of 2.6 s Pulsations in the Soft Gamma-Ray Repeater SGR{\nbsp}1627{\ndash}41}},
	Volume = 690,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/2/L105}}

@article{ebp09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399L..44E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Burgay}, M. and {Possenti}, A. and {Turolla}, R. and {Zane}, S. and {De Luca}, A. and {Tiengo}, A. and {Israel}, G.~L. and {Mattana}, F. and {Mereghetti}, S. and {Bailes}, M. and {Romano}, P. and {G{\"o}tz}, D. and {Rea}, N.},
	Doi = {10.1111/j.1745-3933.2009.00723.x},
	Eprint = {0907.2873},
	Journal = {\mnras},
	Keywords = {stars: neutron , pulsars: general , X-rays: individual: SGR1627-41},
	Month = oct,
	Pages = {L44-L48},
	Title = {{Spin-down rate and inferred dipole magnetic field of the soft gamma-ray repeater SGR1627-41}},
	Volume = 399,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2009.00723.x}}

@article{esposito10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.1787E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Turolla}, R. and {Tiengo}, A. and {G{\"o}tz}, D. and {De Luca}, A. and {Mignani}, R.~P. and {Zane}, S. and {Rea}, N. and {Testa}, V. and {Caraveo}, P.~A. and {Chaty}, S. and {Mattana}, F. and {Mereghetti}, S. and {Pellizzoni}, A. and {Romano}, P.},
	Doi = {10.1111/j.1365-2966.2010.16551.x},
	Eprint = {1002.3506},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, X-rays: individual: SGR0418+5729},
	Month = jul,
	Pages = {1787-1795},
	Title = {{Early X-ray and optical observations of the soft gamma-ray repeater SGR 0418+5729}},
	Volume = 405,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16551.x}}

@article{eis10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ATel.2494....1E},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Stella}, L. and {Rea}, N. and {Tiengo}, A.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Soft Gamma-ray Repeaters},
	Month = mar,
	Title = {{Possible pulsation period in SGR 1833-0832}},
	Volume = 2494,
	Year = 2010}

@article{eib10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ATel.2550....1E},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Burgay}, M. and {Possenti}, A. and {G\"otz}, D. and {Rea}, N. and {Mereghetti}, S. and {Tiengo}, A. and {Stella}, L. and {Turolla}, R. and {Zane}, S.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Pulsars, Soft Gamma-ray Repeaters},
	Month = apr,
	Title = {{Spin down rate and inferred dipole magnetic field of the new soft gamma-ray repeater SGR 1833-0832}},
	Volume = 2550,
	Year = 2010}

@article{esposito11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416..205E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Turolla}, R. and {Mattana}, F. and {Tiengo}, A. and {Possenti}, A. and {Zane}, S. and {Rea}, N. and {Burgay}, M. and {G{\"o}tz}, D. and {Mereghetti}, S. and {Stella}, L. and {Wieringa}, M.~H. and {Sarkissian}, J.~M. and {Enoto}, T. and {Romano}, P. and {Sakamoto}, T. and {Nakagawa}, Y.~E. and {Makishima}, K. and {Nakazawa}, K. and {Nishioka}, H. and {Fran{\c c}ois-Martin}, C.},
	Doi = {10.1111/j.1365-2966.2011.19022.x},
	Eprint = {1105.1323},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, X-rays: individual: PSR B1830-08 (J1833-0827), X-rays: individual: SGR 1833-0832},
	Month = sep,
	Pages = {205-215},
	Primaryclass = {astro-ph.HE},
	Title = {{Long-term spectral and timing properties of the soft gamma-ray repeater SGR 1833-0832 and detection of extended X-ray emission around the radio pulsar PSR B1830-08}},
	Volume = 416,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19022.x}}

@article{eri11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3490....1E},
	Author = {{Esposito}, P. and {Rea}, N. and {Israel}, G.~L.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Star, Soft Gamma-ray Repeater, Transient, Pulsar},
	Month = jul,
	Title = {{SGR 1822-1606 (Swift J1822.3-1606): X-ray spectrum and refined spin period from Swift XRT analysis}},
	Volume = 3490,
	Year = 2011}

@article{erit11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3495....1E},
	Author = {{Esposito}, P. and {Rea}, N. and {Israel}, G.~L. and {Tiengo}, A.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Transient},
	Month = jul,
	Title = {{Swift J1822.3-1606: pre-outburst ROSAT limits (plus erratum)}},
	Volume = 3495,
	Year = 2011}

@article{etdl11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418..170E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Turolla}, R. and {De Luca}, A. and {Israel}, G.~L. and {Possenti}, A. and {Burrows}, D.~N.},
	Doi = {10.1111/j.1365-2966.2011.19473.x},
	Eprint = {1107.3770},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, X-rays: individual: 1E 161348-5055},
	Month = nov,
	Pages = {170-175},
	Primaryclass = {astro-ph.HE},
	Title = {{Swift monitoring of the central X-ray source in RCW 103}},
	Volume = 418,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19473.x}}

@article{esposito13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.tmp..186E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Motta}, S.~E. and {Pintore}, F. and {Zampieri}, L. and {Tomasella}, L.},
	Doi = {10.1093/mnras/sts248},
	Eprint = {1210.5099},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, galaxies: individual: M31, X-rays: binaries, X-rays: galaxies, X-rays: individual: XMMU J004243.6+412519},
	Month = jan,
	Pages = {2480-2488},
	Primaryclass = {astro-ph.HE},
	Title = {{Swift observations of the ultraluminous X-ray source XMMU J004243.6+412519 in M31}},
	Volume = 428,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts248}}

@article{etr13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.429.3123E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Tiengo}, A. and {Rea}, N. and {Turolla}, R. and {Fenzi}, A. and {Giuliani}, A. and {Israel}, G.~L. and {Zane}, S. and {Mereghetti}, S. and {Possenti}, A. and {Burgay}, M. and {Stella}, L. and {G{\"o}tz}, D. and {Perna}, R. and {Mignani}, R.~P. and {Romano}, P.},
	Doi = {10.1093/mnras/sts569},
	Eprint = {1212.1079},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, dust, extinction, X-rays: individual: Swift J1834.9-0846},
	Month = mar,
	Pages = {3123-3132},
	Primaryclass = {astro-ph.HE},
	Title = {{X-ray and radio observations of the magnetar Swift J1834.9-0846 and its dust-scattering halo}},
	Volume = 429,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts569}}

@article{eis13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.2028E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Sidoli}, L. and {Mason}, E. and {Rodr{\'{\i}}guez Castillo}, G.~A. and {Halpern}, J.~P. and {Moretti}, A. and {G{\"o}tz}, D.},
	Doi = {10.1093/mnras/stt870},
	Eprint = {1305.3439},
	Journal = {\mnras},
	Keywords = {stars: emission-line, Be, stars: individual: 2MASS J22535512+6243368, X-rays: binaries, X-rays: individual: 1RXS J225352.8+624354, X-rays: individual: CXOU J225355.1+624336, X-rays: individual: IGR J22534+6243},
	Month = aug,
	Pages = {2028-2035},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of 47-s pulsations in the X-ray source 1RXS J225352.8+624354}},
	Volume = 433,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt870}}

@article{eisrc13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.3464E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Sidoli}, L. and {Rodr{\'{\i}}guez Castillo}, G.~A. and {Masetti}, N. and {D'Avanzo}, P. and {Campana}, S.},
	Doi = {10.1093/mnras/stt1010},
	Eprint = {1306.1106},
	Journal = {\mnras},
	Keywords = {stars: emission-line, Be, Magellanic Clouds, X-rays: binaries, X-rays: individual: CXOU J005047.9-731817},
	Month = aug,
	Pages = {3464-3471},
	Primaryclass = {astro-ph.HE},
	Title = {{CXOU J005047.9-731817: a 292-s X-ray binary pulsar in the Small Magellanic Cloud}},
	Volume = 433,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt1010}}

@article{eism13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.tmp.2479E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Sidoli}, L. and {Mapelli}, M. and {Zampieri}, L. and {Motta}, S.~E.},
	Doi = {10.1093/mnras/stt1819},
	Eprint = {1309.6328},
	Journal = {\mnras},
	Keywords = {galaxies: individual: NGC 4490, X-rays: binaries, X-rays: individual: CXOU J123030.3+413853},
	Month = dec,
	Pages = {3380-3387},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of a 6.4 h black hole binary in NGC 4490}},
	Volume = 436,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt1819}}

@article{esposito14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A.117E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Dall'Osso}, S. and {Covino}, S.},
	Doi = {10.1051/0004-6361/201322719},
	Eid = {A117},
	Eprint = {1311.6973},
	Journal = {\aap},
	Keywords = {stars: individual: RX J0806.3+1527 (HM Cnc), X-rays: binaries, ultraviolet: stars, binaries: close, white dwarfs},
	Month = jan,
	Pages = {A117},
	Primaryclass = {astro-ph.HE},
	Title = {{Swift X-ray and ultraviolet observations of the shortest orbital period double-degenerate system RX J0806.3+1527 (HM Cnc)}},
	Volume = 561,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201322719}}

@article{eis14,
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Sidoli}, L. and {Tiengo}, A. and {Campana}, S. and {Moretti}, A.},
	Journal = {\mnras},
	Number = {2},
	Pages = {1126--1133},
	Publisher = {Oxford University Press},
	Title = {The X-ray emission of the high-mass X-ray binary IGR J17200--3116},
	Volume = {441},
	Year = {2014}}

@article{esposito15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.450.1705E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {de Martino}, D. and {D'Avanzo}, P. and {Testa}, V. and {Sidoli}, L. and {Di Stefano}, R. and {Belfiore}, A. and {Mapelli}, M. and {Piranomonte}, S. and {Rodr{\'{\i}}guez Castillo}, G.~A. and {Moretti}, A. and {D'Elia}, V. and {Verrecchia}, F. and {Campana}, S. and {Rea}, N.},
	Doi = {10.1093/mnras/stv724},
	Eprint = {1503.08830},
	Journal = {\mnras},
	Keywords = {novae, cataclysmic variables, white dwarfs, X-rays: binaries, X-rays: individual: Swift J201424.9+152930},
	Month = jun,
	Pages = {1705-1715},
	Primaryclass = {astro-ph.HE},
	Title = {{Swift J201424.9+152930: discovery of a new deeply eclipsing binary with 491-s and 3.4-h modulations}},
	Volume = 450,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv724}}

@article{eimm15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.452.1112E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Milisavljevic}, D. and {Mapelli}, M. and {Zampieri}, L. and {Sidoli}, L. and {Fabbiano}, G. and {Rodr{\'{\i}}guez Castillo}, G.~A.},
	Doi = {10.1093/mnras/stv1379},
	Eprint = {1506.05808},
	Journal = {\mnras},
	Keywords = {novae, cataclysmic variables, galaxies: individual: Circinus, X-rays: binaries, X-rays: individual: CG X-1 (CXOU J141312.3-652013), X-rays: individual: CXOU J141332.9-651756, X-rays: individual: CXO J141430.1-651621},
	Month = sep,
	Pages = {1112-1127},
	Primaryclass = {astro-ph.HE},
	Title = {{Periodic signals from the Circinus region: two new cataclysmic variables and the ultraluminous X-ray source candidate GC X-1}},
	Volume = 452,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stv1379}}

@article{esposito16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.457L...5E},
	Archiveprefix = {arXiv},
	Author = {{Esposito}, P. and {Israel}, G.~L. and {Belfiore}, A. and {Novara}, G. and {Sidoli}, L. and {Rodr{\'{\i}}guez Castillo}, G.~A. and {De Luca}, A. and {Tiengo}, A. and {Haberl}, F. and {Salvaterra}, R. and {Read}, A.~M. and {Salvetti}, D. and {Sandrelli}, S. and {Marelli}, M. and {Wilms}, J. and {D'Agostino}, D.},
	Doi = {10.1093/mnrasl/slv194},
	Eprint = {1512.00467},
	Journal = {\mnras},
	Keywords = {galaxies: individual: M 31, X-rays: binaries, X-rays: individual: 3XMM J004301.4+413017},
	Month = mar,
	Pages = {L5-L9},
	Primaryclass = {astro-ph.HE},
	Title = {{EXTraS discovery of an 1.2-s X-ray pulsar in M 31}},
	Volume = 457,
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnrasl/slv194}}

@ARTICLE{esposito18,
   author = {{Esposito}, P. and {Rea}, N. and {Lazzati}, D. and {Matsuura}, M. and 
	{Perna}, R. and {Pons}, J.~A.},
    title = "{Can a Bright and Energetic X-Ray Pulsar Be Hiding Amid the Debris of SN 1987A?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1803.04692},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, supernovae: individual: SN 1987A},
     year = 2018,
    month = apr,
   volume = 857,
      eid = {58},
    pages = {58},
      doi = {10.3847/1538-4357/aab6b6},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...857...58E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{Esposito2021,
       author = {{Esposito}, Paolo and {Rea}, Nanda and {Israel}, Gian Luca},
        title = "{Magnetars: A Short Review and Some Sparse Considerations}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {Astrophysics and Space Science Library},
         year = 2021,
       editor = {{Belloni}, Tomaso M. and {M{\'e}ndez}, Mariano and {Zhang}, Chengmin},
       series = {Astrophysics and Space Science Library},
       volume = {461},
        month = jan,
        pages = {97-142},
          doi = {10.1007/978-3-662-62110-3\_3},
archivePrefix = {arXiv},
       eprint = {1803.05716},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ASSL..461...97E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{evans79,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1979IAUC.3356....1E&db_key=AST},
	Author = {{Evans}, D. and {Kiebesadel}, R. and {Baros}, J. and {Cline}, T. and {Desai}, U. and {Teegarden}, B. and {Pizzichini}, G. and {Hurley}, K. and {Niel}, M. and {Vedrenne}, G. and {Estulin}, I.~V. and {Mazets}, E.~P.},
	Journal = {\iaucirc},
	Month = may,
	Pages = {1},
	Title = {{Gamma-ray Burst 79-03-05}},
	Volume = 3356,
	Year = 1979}

@article{evans07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..379E},
	Author = {{Evans}, P.~A. and {Beardmore}, A.~P. and {Page}, K.~L. and {Tyler}, L.~G. and {Osborne}, J.~P. and {Goad}, M.~R. and {O'Brien}, P.~T. and {Vetere}, L. and {Racusin}, J. and {Morris}, D. and {Burrows}, D.~N. and {Capalbi}, M. and {Perri}, M. and {Gehrels}, N. and {Romano}, P.},
	Doi = {10.1051/0004-6361:20077530},
	Eprint = {arXiv:0704.0128},
	Journal = {\aap},
	Keywords = {gamma rays: bursts, gamma rays: observations, methods: data analysis, catalogs},
	Month = jul,
	Pages = {379-385},
	Title = {{An online repository of Swift/XRT light curves of {$\gamma$}-ray bursts}},
	Volume = 469,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077530}}

@article{evans10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..189...37E},
	Archiveprefix = {arXiv},
	Author = {{Evans}, I.~N. and {Primini}, F.~A. and {Glotfelty}, K.~J. and {Anderson}, C.~S. and {Bonaventura}, N.~R. and {Chen}, J.~C. and {Davis}, J.~E. and {Doe}, S.~M. and {Evans}, J.~D. and {Fabbiano}, G. and {Galle}, E.~C. and {Gibbs}, II, D.~G. and {Grier}, J.~D. and {Hain}, R.~M. and {Hall}, D.~M. and {Harbo}, P.~N. and {(Helen He}, X. and {Houck}, J.~C. and {Karovska}, M. and {Kashyap}, V.~L. and {Lauer}, J. and {McCollough}, M.~L. and {McDowell}, J.~C. and {Miller}, J.~B. and {Mitschang}, A.~W. and {Morgan}, D.~L. and {Mossman}, A.~E. and {Nichols}, J.~S. and {Nowak}, M.~A. and {Plummer}, D.~A. and {Refsdal}, B.~L. and {Rots}, A.~H. and {Siemiginowska}, A. and {Sundheim}, B.~A. and {Tibbetts}, M.~S. and {Van Stone}, D.~W. and {Winkelman}, S.~L. and {Zografou}, P.},
	Doi = {10.1088/0067-0049/189/1/37},
	Eid = {37},
	Eprint = {1005.4665},
	Journal = {\apjs},
	Keywords = {catalogs, X-rays: general},
	Month = jul,
	Pages = {37-82},
	Primaryclass = {astro-ph.HE},
	Title = {{The Chandra Source Catalog}},
	Volume = 189,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/189/1/37}}
	
@ARTICLE{evans18,
       author = {{Evans}, D.~W. and {Riello}, M. and {De Angeli}, F. and
         {Carrasco}, J.~M. and {Montegriffo}, P. and {Fabricius}, C. and
         {Jordi}, C. and {Palaversa}, L. and {Diener}, C. and {Busso}, G. and
         {Cacciari}, C. and {van Leeuwen}, F. and {Burgess}, P.~W. and
         {Davidson}, M. and {Harrison}, D.~L. and {Hodgkin}, S.~T. and
         {Pancino}, E. and {Richards}, P.~J. and {Altavilla}, G. and
         {Balaguer-N{\'u}{\~n}ez}, L. and {Barstow}, M.~A. and {Bellazzini}, M. and
         {Brown}, A.~G.~A. and {Castellani}, M. and {Cocozza}, G. and
         {De Luise}, F. and {Delgado}, A. and {Ducourant}, C. and {Galleti}, S. and
         {Gilmore}, G. and {Giuffrida}, G. and {Holl}, B. and {Kewley}, A. and
         {Koposov}, S.~E. and {Marinoni}, S. and {Marrese}, P.~M. and
         {Osborne}, P.~J. and {Piersimoni}, A. and {Portell}, J. and
         {Pulone}, L. and {Ragaini}, S. and {Sanna}, N. and {Terrett}, D. and
         {Walton}, N.~A. and {Wevers}, T. and {Wyrzykowski}, {\L}.},
        title = "{Gaia Data Release 2. Photometric content and validation}",
      journal = {\aap},
     keywords = {catalogs, surveys, instrumentation: photometers, techniques: photometric, galaxies: general, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {616},
          eid = {A4},
        pages = {A4},
          doi = {10.1051/0004-6361/201832756},
archivePrefix = {arXiv},
       eprint = {1804.09368},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...4E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{evans19,
       author = {{Evans}, P.~A. and {Page}, K.~L. and {Osborne}, J.~P. and
         {Beardmore}, A.~P. and {Willingale}, R. and {Burrows}, D.~N. and
         {Kennea}, J.~A. and {Perri}, M. and {Capalbi}, M. and
         {Tagliaferri}, G. and {Cenko}, S.~B.},
        title = "{2SXPS: An improved and expanded Swift X-ray telescope point source catalog}",
      journal = {\apjs, submitted},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Nov",
          eid = {arXiv:1911.11710},
        pages = {arXiv:1911.11710},
archivePrefix = {arXiv},
       eprint = {1911.11710},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191111710E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{fabbiano89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989ARA%26A..27...87F},
	Author = {{Fabbiano}, G.},
	Doi = {10.1146/annurev.aa.27.090189.000511},
	Journal = {\araa},
	Keywords = {SPIRAL GALAXIES, X RAY ASTRONOMY, BRIGHTNESS DISTRIBUTION, GALACTIC NUCLEI, HEAO 2, LOCAL GROUP (ASTRONOMY), MAGELLANIC CLOUDS, STARBURST GALAXIES},
	Pages = {87-138},
	Title = {{X rays from normal galaxies}},
	Volume = 27,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.27.090189.000511}}

@article{fabbiano05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005Sci...307..533F},
	Author = {{Fabbiano}, G.},
	Doi = {10.1126/science.1107110},
	Journal = {Science},
	Month = jan,
	Pages = {533-534},
	Title = {{The hunt for intermediate-mass black holes.}},
	Volume = 307,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1107110}}

@article{fabbiano06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ARA%26A..44..323F},
	Author = {{Fabbiano}, G.},
	Doi = {10.1146/annurev.astro.44.051905.092519},
	Eprint = {arXiv:astro-ph/0511481},
	Journal = {\araa},
	Month = sep,
	Pages = {323-366},
	Title = {{Populations of X-Ray Sources in Galaxies}},
	Volume = 44,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.44.051905.092519}}

@ARTICLE{fabian79,
   author = {{Fabian}, A.~C.},
    title = "{Theories of the nuclei of active galaxies}",
  journal = {Proceedings of the Royal Society of London Series A},
 keywords = {Active Galaxies, Astrophysics, Galactic Nuclei, Quasars, Stellar Luminosity, X Ray Astronomy, Active Galactic Nuclei, Astronomical Models, Black Holes (Astronomy), Bremsstrahlung, Flux Density, Graphs (Charts), Radio Astronomy, Stellar Mass Accretion, X Ray Sources, X Ray Spectra},
     year = 1979,
    month = jun,
   volume = 366,
    pages = {449-459},
      doi = {10.1098/rspa.1979.0064},
   adsurl = {http://adsabs.harvard.edu/abs/1979RSPSA.366..449F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{farrell09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009Natur.460...73F},
	Archiveprefix = {arXiv},
	Author = {{Farrell}, S.~A. and {Webb}, N.~A. and {Barret}, D. and {Godet}, O. and {Rodrigues}, J.~M.},
	Doi = {10.1038/nature08083},
	Eprint = {1001.0567},
	Journal = {\nat},
	Month = jul,
	Pages = {73-75},
	Primaryclass = {astro-ph.HE},
	Title = {{An intermediate-mass black hole of over 500 solar masses in the galaxy ESO243-49}},
	Volume = 460,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature08083}}

@article{farrell15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813...28F},
	Archiveprefix = {arXiv},
	Author = {{Farrell}, S.~A. and {Murphy}, T. and {Lo}, K.~K.},
	Doi = {10.1088/0004-637X/813/1/28},
	Eid = {28},
	Eprint = {1509.03714},
	Journal = {\apj},
	Keywords = {catalogs, methods: statistical},
	Month = nov,
	Pages = {28},
	Primaryclass = {astro-ph.IM},
	Title = {{Autoclassification of the Variable 3XMM Sources Using the Random Forest Machine Learning Algorithm}},
	Volume = 813,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/813/1/28}}

@article{fasano87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.225..155F},
	Author = {{Fasano}, G. and {Franceschini}, A.},
	Journal = {\mnras},
	Keywords = {ASTRONOMICAL MODELS, GALACTIC EVOLUTION, GALACTIC NUCLEI, KOLMOGOROFF-SMIRNOFF TEST, RANDOM SAMPLING, X RAY SPECTRA, ACTIVE GALACTIC NUCLEI, DATA CORRELATION, MONTE CARLO METHOD, PROBABILITY DENSITY FUNCTIONS, RUN TIME (COMPUTERS)},
	Month = mar,
	Pages = {155-170},
	Title = {{A multidimensional version of the Kolmogorov-Smirnov test}},
	Volume = 225,
	Year = 1987}

@article{faucher06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...643..332F},
	Author = {{Faucher-Gigu{\`e}re}, C.-A. and {Kaspi}, V.~M.},
	Doi = {10.1086/501516},
	Eprint = {arXiv:astro-ph/0512585},
	Journal = {\apj},
	Keywords = {Galaxy: Structure, Methods: Statistical, Stars: Pulsars: General, Stars: Kinematics, Stars: Neutron},
	Month = may,
	Pages = {332-355},
	Title = {{Birth and Evolution of Isolated Radio Pulsars}},
	Volume = 643,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/501516}}

@article{fegan97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997JPhG...23.1013F&db_key=PHY},
	Author = {{Fegan}, D.~J.},
	Journal = {Journal of Physics G Nuclear Physics},
	Month = sep,
	Pages = {1013-1060},
	Title = {{$\gamma$/hadron separation at TeV energies}},
	Volume = 23,
	Year = 1997}

@article{fender06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006MNRAS.367L...6F},
	Author = {{Fender}, R.~P. and {Muxlow}, T.~W.~B. and {Garrett}, M.~A. and {Kouveliotou}, C. and {Gaensler}, B.~M. and {Garrington}, S.~T. and {Paragi}, Z. and {Tudose}, V. and {Miller-Jones}, J.~C.~A. and {Spencer}, R.~E. and {Wijers}, R.~A.~M. and {Taylor}, G.~B.},
	Doi = {10.1111/j.1745-3933.2006.00123.x},
	Eprint = {arXiv:astro-ph/0511214},
	Journal = {\mnras},
	Month = mar,
	Pages = {L6-L10},
	Title = {{Structure in the radio counterpart to the 2004 December 27 giant flare from SGR 1806-20}},
	Volume = 367,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2006.00123.x}}

@article{feng05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...633.1052F},
	Author = {{Feng}, H. and {Kaaret}, P.},
	Doi = {10.1086/491597},
	Eprint = {arXiv:astro-ph/0507562},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Black Hole Physics, X-Rays: Binaries, X-Rays: Galaxies},
	Month = nov,
	Pages = {1052-1063},
	Title = {{XMM-Newton Observations of Ultraluminous X-Ray Sources in Nearby Galaxies}},
	Volume = 633,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/491597}}

@article{feng10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710L.137F},
	Archiveprefix = {arXiv},
	Author = {{Feng}, H. and {Rao}, F. and {Kaaret}, P.},
	Doi = {10.1088/2041-8205/710/2/L137},
	Eprint = {1001.3456},
	Journal = {\apjl},
	Keywords = {accretion, accretion disks, black hole physics, X-rays: individual: CXOM82 J095551.1+694045{\amp}equalsX42.3+59},
	Month = feb,
	Pages = {L137-L141},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of Millihertz X-Ray Oscillations in a Transient Ultraluminous X-Ray Source in M82}},
	Volume = 710,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/710/2/L137}}

@article{feng11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011NewAR..55..166F},
	Archiveprefix = {arXiv},
	Author = {{Feng}, H. and {Soria}, R.},
	Doi = {10.1016/j.newar.2011.08.002},
	Journal = {\nar},
	Month = nov,
	Pages = {166-183},
	Title = {{Ultraluminous X-ray sources in the Chandra and XMM-Newton era}},
	Volume = 55,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.newar.2011.08.002}}

@article{fenimore94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994ApJ...432..742F&amp;db_key=AST},
	Author = {{Fenimore}, E.~E. and {Laros}, J.~G. and {Ulmer}, A.},
	Journal = {\apj},
	Month = sep,
	Pages = {742-752},
	Title = {{The X-ray spectrum of the soft gamma repeater 1806-20}},
	Volume = 432,
	Year = 1994}

@article{fernandez07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660..615F},
	Author = {{Fern{\'a}ndez}, R. and {Thompson}, C.},
	Doi = {10.1086/511810},
	Eprint = {arXiv:astro-ph/0608281},
	Journal = {\apj},
	Month = may,
	Pages = {615-640},
	Title = {{Resonant Cyclotron Scattering in Three Dimensions and the Quiescent Nonthermal X-ray Emission of Magnetars}},
	Volume = 660,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/511810}}

@article{feroci98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998IAUC.6945....3F&db_key=AST},
	Author = {{Feroci}, M. and {Costa}, E. and {Amati}, L. and {Piro}, L. and {Martino}, B. and {di Ciolo}, L. and {Coletta}, A. and {Frontera}, F.},
	Journal = {\iaucirc},
	Month = jun,
	Pages = {3},
	Title = {{SGR 1627-41}},
	Volume = 6945,
	Year = 1998}

@article{feroci99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...515L...9F&db_key=AST},
	Author = {{Feroci}, M. and {Frontera}, F. and {Costa}, E. and {Amati}, L. and {Tavani}, M. and {Rapisarda}, M. and {Orlandini}, M.},
	Doi = {10.1086/311964},
	Eprint = {astro-ph/9902096},
	Journal = {\apjl},
	Month = apr,
	Pages = {L9-L12},
	Title = {{A Giant Outburst from SGR 1900+14 Observed with the BeppoSAX Gamma-Ray Burst Monitor}},
	Volume = 515,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311964}}

@article{feroci01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...549.1021F&db_key=AST},
	Author = {{Feroci}, M. and {Hurley}, K. and {Duncan}, R.~C. and {Thompson}, C.},
	Doi = {10.1086/319441},
	Journal = {\apj},
	Month = mar,
	Pages = {1021-1038},
	Title = {{The Giant Flare of 1998 August 27 from SGR 1900+14. I. An Interpretive Study of BeppoSAX and Ulysses Observations}},
	Volume = 549,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/319441}}

@article{feroci01_gcn,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001GCN..1060....1F&db_key=AST},
	Author = {{Feroci}, M. and {in't Zand}, J.~J.~M. and {Soffitta}, P. and {Hurley}, K. and {Frontera}, F. and {Mazets}, E.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{X-ray precursors to the large flare from Sgr 1900+14.}},
	Volume = 1060,
	Year = 2001}

@inproceedings{feroci02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ASPC..271..285F&db_key=AST},
	Author = {{Feroci}, M. and {Mereghetti}, S. and {Costa}, E. and {in't Zand}, J.~J.~M. and {Soffitta}, P. and {Cline}, T. and {Duncan}, R. and {Finger}, M. and {Golenetskii}, S.~V. and {Hurley}, K. and {Kouveliotou}, C. and {Li}, P. and {Mazets}, E. and {Tavani}, M. and {Thompson}, C. and {Woods}, P.},
	Booktitle = {ASP Conf. Ser. 271: Neutron Stars in Supernova Remnants, ed. P.~O. Slane \& B.~M. Gaensler},
	Title = {{The BeppoSAX View on the 2001 Reactivation of SGR 1900+14}},
	Year = 2002}

@article{feroci03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003ApJ...596..470F&db_key=AST},
	Author = {{Feroci}, M. and {Mereghetti}, S. and {Woods}, P. and {Kouveliotou}, C. and {Costa}, E. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Hurley}, K. and {Mazets}, E. and {Soffitta}, P. and {Tavani}, M.},
	Doi = {10.1086/377513},
	Journal = {\apj},
	Month = oct,
	Pages = {470-476},
	Title = {{The 2001 April Burst Activation of SGR 1900+14: X-Ray Afterglow Emission}},
	Volume = 596,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/377513}}

@article{feroci04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...612..408F&amp;db_key=AST},
	Author = {{Feroci}, M. and {Caliandro}, G.~A. and {Massaro}, E. and {Mereghetti}, S. and {Woods}, P.~M.},
	Journal = {\apj},
	Month = sep,
	Pages = {408-413},
	Title = {{Broadband X-Ray Spectra of Short Bursts from SGR 1900+14}},
	Volume = 612,
	Year = 2004}

@INPROCEEDINGS{feroci16,
   author = {{Feroci}, M. and {Bozzo}, E. and {Brandt}, S. and {Hernanz}, M. and 
	{van der Klis}, M. and {Liu}, L.-P. and {Orleanski}, P. and 
	{Pohl}, M. and {Santangelo}, A. and {Schanne}, S. and et al.},
    title = "{The LOFT mission concept: a status update}",
booktitle = {Space Telescopes and Instrumentation 2016: Ultraviolet to Gamma Ray},
     year = 2016,
   series = {\procspie},
   volume = 9905,
    month = jul,
      eid = {99051R},
    pages = {99051R},
      doi = {10.1117/12.2233161},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9905E..1RF},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ferrario06,
   author = {{Ferrario}, L. and {Wickramasinghe}, D.},
    title = "{Modelling of isolated radio pulsars and magnetars on the fossil field hypothesis}",
  journal = {\mnras},
   eprint = {astro-ph/0601258},
 keywords = {stars: early-type, stars: magnetic fields, stars: neutron, pulsars: general},
     year = 2006,
    month = apr,
   volume = 367,
    pages = {1323-1328},
      doi = {10.1111/j.1365-2966.2006.10058.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367.1323F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ferrario08,
   author = {{Ferrario}, L. and {Wickramasinghe}, D.},
    title = "{Origin and evolution of magnetars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0807.2106},
 keywords = {stars: early-type, stars: magnetic fields, stars: neutron, pulsars: general},
     year = 2008,
    month = sep,
   volume = 389,
    pages = {L66-L70},
      doi = {10.1111/j.1745-3933.2008.00527.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.389L..66F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{figer05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...622L..49F&db_key=AST},
	Author = {{Figer}, D.~F. and {Najarro}, F. and {Geballe}, T.~R. and {Blum}, R.~D. and {Kudritzki}, R.~P.},
	Doi = {10.1086/429159},
	Eprint = {astro-ph/0501560},
	Journal = {\apjl},
	Month = mar,
	Pages = {L49-L52},
	Title = {{Massive Stars in the SGR 1806-20 Cluster}},
	Volume = 622,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429159}}

@article{fitzpatrick99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999PASP..111...63F},
	Author = {{Fitzpatrick}, E.~L.},
	Doi = {10.1086/316293},
	Eprint = {arXiv:astro-ph/9809387},
	Journal = {\pasp},
	Keywords = {ISM: DUST, EXTINCTION},
	Month = jan,
	Pages = {63-75},
	Title = {{Correcting for the Effects of Interstellar Extinction}},
	Volume = 111,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/316293}}

@article{fitzpatrick07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..320F},
	Archiveprefix = {arXiv},
	Author = {{Fitzpatrick}, E.~L. and {Massa}, D.},
	Doi = {10.1086/518158},
	Eprint = {0705.0154},
	Journal = {\apj},
	Keywords = {ISM: Dust, Extinction, Methods: Data Analysis},
	Month = jul,
	Pages = {320-341},
	Title = {{An Analysis of the Shapes of Interstellar Extinction Curves. V. The IR-through-UV Curve Morphology}},
	Volume = 663,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518158}}

@article{fong12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...756..189F},
	Archiveprefix = {arXiv},
	Author = {{Fong}, W. and {Berger}, E. and {Margutti}, R. and {Zauderer}, B.~A. and {Troja}, E. and {Czekala}, I. and {Chornock}, R. and {Gehrels}, N. and {Sakamoto}, T. and {Fox}, D.~B. and {Podsiadlowski}, P.},
	Doi = {10.1088/0004-637X/756/2/189},
	Eid = {189},
	Eprint = {1204.5475},
	Journal = {\apj},
	Keywords = {gamma-ray burst: general, gamma-ray burst: individual: 111020A},
	Month = sep,
	Pages = {189},
	Primaryclass = {astro-ph.HE},
	Title = {{A Jet Break in the X-Ray Light Curve of Short GRB 111020A: Implications for Energetics and Rates}},
	Volume = 756,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/756/2/189}}

@article{foster96,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996ApJ...467L..81F&db_key=AST},
	Author = {{Foster}, R.~S. and {Waltman}, E.~B. and {Tavani}, M. and {Harmon}, B.~A. and {Zhang}, S.~N. and {Paciesas}, W.~S. and {Ghigo}, F.~D.},
	Doi = {10.1086/310199},
	Journal = {\apjl},
	Month = aug,
	Pages = {L81},
	Title = {{Radio and X-Ray Variability of the Galactic Superluminal Source GRS 1915+105}},
	Volume = 467,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310199}}

@article{fragos09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697.1057F},
	Archiveprefix = {arXiv},
	Author = {{Fragos}, T. and {Willems}, B. and {Kalogera}, V. and {Ivanova}, N. and {Rockefeller}, G. and {Fryer}, C.~L. and {Young}, P.~A.},
	Doi = {10.1088/0004-637X/697/2/1057},
	Eprint = {0809.1588},
	Journal = {\apj},
	Keywords = {binaries: close, X-rays: binaries, X-rays: individual: XTEJ1118+480},
	Month = jun,
	Pages = {1057-1070},
	Title = {{Understanding Compact Object Formation and Natal Kicks. II. The Case of XTE J1118 + 480}},
	Volume = 697,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/697/2/1057}}

@article{fragos15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...802L...5F},
	Archiveprefix = {arXiv},
	Author = {{Fragos}, T. and {Linden}, T. and {Kalogera}, V. and {Sklias}, P.},
	Doi = {10.1088/2041-8205/802/1/L5},
	Eid = {L5},
	Eprint = {1501.02679},
	Journal = {\apjl},
	Keywords = {binaries: close, stars: neutron, X-rays: binaries},
	Month = mar,
	Pages = {L5},
	Primaryclass = {astro-ph.HE},
	Title = {{On the Formation of Ultraluminous X-Ray Sources with Neutron Star Accretors: The Case of M82 X-2}},
	Volume = 802,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/802/1/L5}}

@article{frail91,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991AJ....101.2126F&db_key=AST},
	Author = {{Frail}, D.~A. and {Hjellming}, R.~M.},
	Doi = {10.1086/115833},
	Journal = {\aj},
	Month = jun,
	Pages = {2126-2130},
	Title = {{Distance and total column density to the periodic radio star LSI + 61 deg 303}},
	Volume = 101,
	Year = 1991,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/115833}}

@article{frail96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1651F},
	Author = {{Frail}, D.~A. and {Goss}, W.~M. and {Reynoso}, E.~M. and {Giacani}, E.~B. and {Green}, A.~J. and {Otrupcek}, R.},
	Doi = {10.1086/117904},
	Journal = {\aj},
	Keywords = {SUPERNOVA REMNANTS, MASERS, CIRCUMSTELLAR MATTER, ISM: CLOUDS},
	Month = apr,
	Pages = {1651},
	Title = {{A Survey for OH(1720 MHz) Maser Emission Toward Supernova Remnants}},
	Volume = 111,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/117904}}

@article{frail97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...480L.129F&db_key=AST},
	Author = {{Frail}, D.~A. and {Vasisht}, G. and {Kulkarni}, S.~R.},
	Doi = {10.1086/310635},
	Journal = {\apjl},
	Month = may,
	Pages = {L129+},
	Title = {{The Changing Stucture of the Radio Nebula around the Soft Gamma-Ray Repeater SGR 1806-20}},
	Volume = 480,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310635}}

@article{frank87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...178..137F},
	Author = {{Frank}, J. and {King}, A.~R. and {Lasota}, J.-P.},
	Journal = {\aap},
	Keywords = {LIGHT CURVE, STELLAR CORONAS, STELLAR MASS ACCRETION, X RAY BINARIES, DIPPING, ECLIPSES, IONIZATION, STELLAR MODELS},
	Month = may,
	Pages = {137-142},
	Title = {{The light curves of low-mass X-ray binaries}},
	Volume = 178,
	Year = 1987}

@book{frank02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002apa..book.....F&db_key=AST},
	Author = {{Frank}, J. and {King}, A. and {Raine}, D.~J.},
	Publisher = {Cambridge: Cambridge University Press},
	Title = {{Accretion Power in Astrophysics: Third Edition}},
	Year = 2002}

@ARTICLE{frank16,
   author = {{Frank}, K.~A. and {Zhekov}, S.~A. and {Park}, S. and {McCray}, R. and 
	{Dwek}, E. and {Burrows}, D.~N.},
    title = "{Chandra Observes the End of an Era in SN 1987A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.02160},
 primaryClass = "astro-ph.HE",
 keywords = {circumstellar matter, ISM: supernova remnants, X-rays: individual: SN 1987A, X-rays: ISM},
     year = 2016,
    month = sep,
   volume = 829,
      eid = {40},
    pages = {40},
      doi = {10.3847/0004-637X/829/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...829...40F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{frederiks07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2007AstL...33....1F&db_key=AST},
	Author = {{Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Palshin}, V.~D. and {Aptekar}, R.~L. and {Ilyinskii}, V.~N. and {Oleinik}, F.~P. and {Mazets}, E.~P. and {Cline}, T.~L.},
	Doi = {10.1134/S106377370701001X},
	Eprint = {astro-ph/0612289},
	Journal = {Astron.~Lett.},
	Month = jan,
	Pages = {1-18},
	Title = {{Giant flare in SGR 1806-20 and its Compton reflection from the Moon}},
	Volume = 33,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1134/S106377370701001X}}

@article{freeman77,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1977A%26A....55..445F},
	Author = {{Freeman}, K.~C. and {Karlsson}, B. and {Lynga}, G. and {Burrell}, J.~F. and {van Woerden}, H. and {Goss}, W.~M. and {Mebold}, U.},
	Journal = {\aap},
	Keywords = {Astronomical Photometry, Galactic Radiation, Radio Sources (Astronomy), Spiral Galaxies, Brightness, Color, Galactic Nuclei, Galactic Rotation, Hydrogen, Interstellar Extinction},
	Month = mar,
	Pages = {445-458},
	Title = {{A large new galaxy in Circinus}},
	Volume = 55,
	Year = 1977}

@inproceedings{freeman01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001SPIE.4477...76F},
	Author = {{Freeman}, P. and {Doe}, S. and {Siemiginowska}, A.},
	Booktitle = {Astronomical Data Analysis},
	Doi = {10.1117/12.447161},
	Editor = {{Starck}, J.-L. and {Murtagh}, F.~D.},
	Eprint = {astro-ph/0108426},
	Month = nov,
	Pages = {76-87},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{Sherpa: a mission-independent data analysis application}},
	Volume = 4477,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.447161}}

@article{freitag06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649...91F},
	Author = {{Freitag}, M. and {Amaro-Seoane}, P. and {Kalogera}, V.},
	Doi = {10.1086/506193},
	Eprint = {arXiv:astro-ph/0603280},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Galaxies: Nuclei, Galaxies: Star Clusters, Gravitational Waves, Methods: n-Body Simulations, Stellar Dynamics},
	Month = sep,
	Pages = {91-117},
	Title = {{Stellar Remnants in Galactic Nuclei: Mass Segregation}},
	Volume = 649,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506193}}

@article{fridriksson08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..177..465F},
	Archiveprefix = {arXiv},
	Author = {{Fridriksson}, J.~K. and {Homan}, J. and {Lewin}, W.~H.~G. and {Kong}, A.~K.~H. and {Pooley}, D.},
	Doi = {10.1086/588817},
	Eprint = {0804.1411},
	Journal = {\apjs},
	Keywords = {Galaxies: Individual: NGC Number: NGC 6946, Galaxies: Individual: NGC Number: NGC 4485, Galaxies: Individual: NGC Number: NGC 4490, X-Rays: Binaries, X-Rays: Galaxies},
	Month = aug,
	Pages = {465-492},
	Title = {{The Long-Term Variability of the X-Ray Sources in NGC 6946 and NGC 4485/4490}},
	Volume = 177,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588817}}

@article{frontera97,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26AS..122..357F&db_key=AST},
	Author = {{Frontera}, F. and {Costa}, E. and {dal Fiume}, D. and {Feroci}, M. and {Nicastro}, L. and {Orlandini}, M. and {Palazzi}, E. and {Zavattini}, G.},
	Journal = {\aaps},
	Month = apr,
	Pages = {357-369},
	Title = {{The high energy instrument PDS on-board the BeppoSAX X--ray astronomy satellite}},
	Volume = 122,
	Year = 1997}

@inproceedings{fruscione06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6270E..60F},
	Author = {{Fruscione}, A. and {McDowell}, J.~C. and {Allen}, G.~E. and {Brickhouse}, N.~S. and {Burke}, D.~J. and {Davis}, J.~E. and {Durham}, N. and {Elvis}, M. and {Galle}, E.~C. and {Harris}, D.~E. and {Huenemoerder}, D.~P. and {Houck}, J.~C. and {Ishibashi}, B. and {Karovska}, M. and {Nicastro}, F. and {Noble}, M.~S. and {Nowak}, M.~A. and {Primini}, F.~A. and {Siemiginowska}, A. and {Smith}, R.~K. and {Wise}, M.},
	Booktitle = {Observatory Operations: Strategies, Processes, and Systems},
	Doi = {10.1117/12.671760},
	Editor = {{Silva}, D.~R. and {Doxsey}, R.~E.},
	Eid = {62701V},
	Month = jul,
	Pages = {62701V},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{CIAO: Chandra's data analysis system}},
	Volume = 6270,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.671760}}

@article{fryer99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...522..413F&db_key=AST},
	Author = {{Fryer}, C.~L.},
	Journal = {\apj},
	Month = sep,
	Pages = {413-418},
	Title = {{Mass Limits For Black Hole Formation}},
	Volume = 522,
	Year = 1999}

@article{fuchs99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999A%26A...350..891F&db_key=AST},
	Author = {{Fuchs}, Y. and {Mirabel}, F. and {Chaty}, S. and {Claret}, A. and {Cesarsky}, C.~J. and {Cesarsky}, D.~A.},
	Journal = {\aap},
	Month = oct,
	Pages = {891-899},
	Title = {{ISO observations of the environment of the soft gamma-ray repeater SGR 1806-20}},
	Volume = 350,
	Year = 1999}

@article{fukui03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003PASJ...55L..61F},
	Author = {{Fukui}, Y. and {Moriguchi}, Y. and {Tamura}, K. and {Yamamoto}, H. and {Tawara}, Y. and {Mizuno}, N. and {Onishi}, T. and {Mizuno}, A. and {Uchiyama}, Y. and {Hiraga}, J. and {Takahashi}, T. and {Yamashita}, K. and {Ikeuchi}, S.},
	Journal = {\pasj},
	Keywords = {cosmic rays, ISM: cloud, molecules, supernova remnants},
	Month = oct,
	Pages = {L61-L64},
	Title = {{Discovery of Interacting Molecular Gas toward the TeV Gamma-Ray Peak of the SNR G 347.3--0.5}},
	Volume = 55,
	Year = 2003}

@article{furst13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779...69F},
	Author = {{F{\"u}rst}, F. and {Grefenstette}, B.~W. and {Staubert}, R. and {Tomsick}, J.~A. and {Bachetti}, M. and {Barret}, D. and {Bellm}, E.~C. and {Boggs}, S.~E. and {Chenevez}, J. and {Christensen}, F.~E. and {Craig}, W.~W. and {Hailey}, C.~J. and {Harrison}, F. and {Klochkov}, D. and {Madsen}, K.~K. and {Pottschmidt}, K. and {Stern}, D. and {Walton}, D.~J. and {Wilms}, J. and {Zhang}, W.},
	Doi = {10.1088/0004-637X/779/1/69},
	Eid = {69},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, pulsars: individual: Her X-1, stars: neutron, X-rays: binaries},
	Month = dec,
	Pages = {69},
	Title = {{The Smooth Cyclotron Line in Her X-1 as Seen with Nuclear Spectroscopic Telescope Array}},
	Volume = 779,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/779/1/69}}

@ARTICLE{furst16,
   author = {{F{\"u}rst}, F. and {Walton}, D.~J. and {Harrison}, F.~A. and 
	{Stern}, D. and {Barret}, D. and {Brightman}, M. and {Fabian}, A.~C. and 
	{Grefenstette}, B. and {Madsen}, K.~K. and {Middleton}, M.~J. and 
	{Miller}, J.~M. and {Pottschmidt}, K. and {Ptak}, A. and {Rana}, V. and 
	{Webb}, N.},
    title = "{Discovery of Coherent Pulsations from the Ultraluminous X-Ray Source NGC 7793 P13}",
  journal = {\apjl},
 keywords = {accretion, accretion disks, pulsars: individual: NGC 7793 P13, stars: neutron, X-rays: binaries},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {L14},
    pages = {L14},
      doi = {10.3847/2041-8205/831/2/L14},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831L..14F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gabriel04,
   author = {{Gabriel}, C. and {Denby}, M. and {Fyfe}, D.~J. and {Hoar}, J. and 
	{Ibarra}, A. and {Ojero}, E. and {Osborne}, J. and {Saxton}, R.~D. and 
	{Lammers}, U. and {Vacanti}, G.},
    title = "{The XMM-Newton SAS - Distributed Development and Maintenance of a Large Science Analysis System: A Critical Analysis}",
booktitle = {Astronomical Data Analysis Software and Systems (ADASS) XIII},
     year = 2004,
   series = {ASP Conf. Ser. (San Francisco, CA: ASP)},
   volume = 314,
   editor = {{Ochsenbein}, F. and {Allen}, M.~G. and {Egret}, D.},
    month = jul,
    pages = {759},
   adsurl = {http://adsabs.harvard.edu/abs/2004ASPC..314..759G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gaensler95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.275L..73G},
	Author = {{Gaensler}, B.~M. and {Johnston}, S.},
	Journal = {\mnras},
	Keywords = {PULSARS: GENERAL, PULSARS: INDIVIDUAL: B1830-08, STARS: STATISTICS, SUPERNOVA REMNANTS},
	Month = aug,
	Pages = {L73-L75},
	Title = {{The case for associations between old pulsars and supernova remnants}},
	Volume = 275,
	Year = 1995}

@article{gaensler01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...559..963G&db_key=AST},
	Author = {{Gaensler}, B.~M. and {Slane}, P.~O. and {Gotthelf}, E.~V. and {Vasisht}, G.},
	Journal = {\apj},
	Month = oct,
	Pages = {963-972},
	Title = {{Anomalous X-Ray Pulsars and Soft Gamma-Ray Repeaters in Supernova Remnants}},
	Volume = 559,
	Year = 2001}

@article{gaensler04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616..383G},
	Author = {{Gaensler}, B.~M. and {van der Swaluw}, E. and {Camilo}, F. and {Kaspi}, V.~M. and {Baganoff}, F.~K. and {Yusef-Zadeh}, F. and {Manchester}, R.~N.},
	Doi = {10.1086/424906},
	Eprint = {arXiv:astro-ph/0312362},
	Journal = {\apj},
	Keywords = {ISM: Individual: Alphanumeric: G359.23-0.82, Stars: Pulsars: Individual: Alphanumeric: PSR J1747-2958, Stars: Neutron, Stars: Winds, Outflows},
	Month = nov,
	Pages = {383-402},
	Title = {{The Mouse that Soared: High-Resolution X-Ray Imaging of the Pulsar-powered Bow Shock G359.23-0.82}},
	Volume = 616,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/424906}}

@article{gmo05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...620L..95G},
	Author = {{Gaensler}, B.~M. and {McClure-Griffiths}, N.~M. and {Oey}, M.~S. and {Haverkorn}, M. and {Dickey}, J.~M. and {Green}, A.~J.},
	Doi = {10.1086/428725},
	Eprint = {arXiv:astro-ph/0501563},
	Journal = {\apjl},
	Keywords = {ISM: Bubbles, ISM: Individual: Alphanumeric: GSH 288.3-0.5-28, Stars: Pulsars: Individual: Alphanumeric: 1E 1048.1-5937, Radio Lines: ISM, Stars: Neutron, Stars: Winds, Outflows},
	Month = feb,
	Pages = {L95-L98},
	Title = {{A Stellar Wind Bubble Coincident with the Anomalous X-Ray Pulsar 1E 1048.1-5937: Are Magnetars Formed from Massive Progenitors?}},
	Volume = 620,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/428725}}

@article{gaensler06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006ARA%26A..44...17G&db_key=AST},
	Author = {{Gaensler}, B.~M. and {Slane}, P.~O.},
	Doi = {10.1146/annurev.astro.44.051905.092528PDF: http://arjournals.annualreviews.org/doi/pdf/10.1146/annurev.astro.44.051905.092528},
	Eprint = {astro-ph/0601081},
	Journal = {\araa},
	Month = sep,
	Pages = {17-47},
	Title = {{The Evolution and Structure of Pulsar Wind Nebulae}},
	Volume = 44,
	Year = 2006,
	Bdsk-Url-1 = {10.1146/annurev.astro.44.051905.092528PDF:%20http://arjournals.annualreviews.org/doi/pdf/10.1146/annurev.astro.44.051905.092528}}

@ARTICLE{gaia18,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and
         {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and
         {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and
         {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and
         {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and
         {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and
         {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and
         {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and
         {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and
         {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and
         {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and
         {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and
         {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and
         {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and
         {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and
         {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and
         {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and
         {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and
         {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and
         {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and
         {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and
         {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and
         {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and
         {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and
         {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and
         {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and
         {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and
         {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and
         {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and
         {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and
         {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and
         {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and
         {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and
         {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and
         {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and
         {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and
         {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and
         {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and
         {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and
         {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and
         {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and
         {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and
         {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and
         {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and
         {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and
         {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and
         {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and
         {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and
         {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and
         {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and
         {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and
         {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and
         {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and
         {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and
         {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and
         {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and
         {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and
         {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and
         {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and
         {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and
         {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and
         {De Luise}, F. and {De March}, R. and {de Martino}, D. and
         {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and
         {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and
         {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and
         {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and
         {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and
         {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and
         {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and
         {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and
         {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and
         {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and
         {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and
         {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and
         {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and
         {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and
         {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and
         {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and
         {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and
         {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and
         {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and
         {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and
         {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and
         {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and
         {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and
         {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and
         {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and
         {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and
         {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and
         {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and
         {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and
         {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and
         {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and
         {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and
         {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and
         {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and
         {Marton}, G. and {Mary}, N. and {Massari}, D. and
         {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and
         {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and
         {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and
         {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and
         {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and
         {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and
         {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and
         {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and
         {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and
         {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and
         {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and
         {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and
         {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and
         {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and
         {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and
         {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and
         {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and
         {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and
         {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and
         {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and
         {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and
         {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and
         {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and
         {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and
         {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and
         {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and
         {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and
         {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssand
        ier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and
         {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and
         {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and
         {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and
         {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and
         {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and
         {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and
         {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and
         {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and
         {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and
         {Zwitter}, T.},
        title = "{Gaia Data Release 2. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, techniques: radial velocities, stars: fundamental parameters, stars: variables: general, minor planets, asteroids: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {616},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201833051},
archivePrefix = {arXiv},
       eprint = {1804.09365},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaia19,
       author = {{Gaia Collaboration} and {Eyer}, L. and {Rimoldini}, L. and
         {Audard}, M. and {Anderson}, R.~I. and {Nienartowicz}, K. and
         {Glass}, F. and {Marchal}, O. and {Grenon}, M. and {Mowlavi}, N. and
         {Holl}, B. and {Clementini}, G. and {Aerts}, C. and {Mazeh}, T. and
         {Evans}, D.~W. and {Szabados}, L. and {Brown}, A.~G.~A. and
         {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and
         {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and
         {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and
         {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and
         {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and
         {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and
         {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and
         {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and
         {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and
         {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and
         {Masana}, E. and {Messineo}, R. and {Panuzzo}, P. and {Portell}, J. and
         {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and
         {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and
         {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and
         {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and
         {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and
         {Carry}, B. and {Cellino}, A. and {Clotet}, M. and {Creevey}, O. and
         {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and
         {Dell'Oro}, A. and {Ducourant}, C. and
         {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and
         {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and
         {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and
         {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and
         {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and
         {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and
         {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and
         {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and
         {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and
         {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and
         {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and
         {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and
         {Richards}, P.~J. and {Robin}, A.~C. and {Sarro}, L.~M. and
         {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and
         {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and
         {Abreu Aramburu}, A. and {Accart}, S. and {Altavilla}, G. and
         {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and
         {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and
         {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and
         {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and
         {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and
         {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and
         {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and
         {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and
         {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and
         {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and
         {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and
         {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and
         {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and
         {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and
         {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and
         {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and
         {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and
         {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and
         {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and
         {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and
         {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and
         {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and
         {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and
         {De Luise}, F. and {De March}, R. and {de Martino}, D. and
         {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and
         {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and
         {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and
         {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and
         {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and
         {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and
         {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and
         {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and
         {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and
         {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and
         {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and
         {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and
         {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and
         {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and
         {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and
         {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and
         {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and
         {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and
         {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and
         {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and
         {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and
         {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and
         {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and
         {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and
         {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and
         {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and
         {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and
         {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and
         {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and
         {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Lorenz}, D. and
         {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and
         {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and
         {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and
         {Marton}, G. and {Mary}, N. and {Massari}, D. and
         {Matijevi{\v{c}}}, G. and {McMillan}, P.~J. and {Messina}, S. and
         {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and
         {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and
         {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and
         {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and
         {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and
         {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and
         {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and
         {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and
         {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and
         {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and
         {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and
         {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and
         {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and
         {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and
         {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and
         {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and
         {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and
         {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and
         {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and
         {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and
         {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and
         {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and
         {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and
         {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and
         {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szegedi-Elek}, E. and
         {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and
         {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and
         {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and
         {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and
         {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and
         {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and
         {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and
         {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and
         {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and
         {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and
         {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and
         {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and
         {Zwitter}, T.},
        title = "{Gaia Data Release 2. Variable stars in the colour-absolute magnitude diagram}",
      journal = {\aap},
     keywords = {stars: general, stars: variables: general, stars: oscillations, binaries: eclipsing, surveys, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics},
         year = "2019",
        month = "Mar",
       volume = {623},
          eid = {A110},
        pages = {A110},
          doi = {10.1051/0004-6361/201833304},
archivePrefix = {arXiv},
       eprint = {1804.09382},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...623A.110G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{galache08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..177..189G},
	Archiveprefix = {arXiv},
	Author = {{Galache}, J.~L. and {Corbet}, R.~H.~D. and {Coe}, M.~J. and {Laycock}, S. and {Schurch}, M.~P.~E. and {Markwardt}, C. and {Marshall}, F.~E. and {Lochner}, J.},
	Doi = {10.1086/587743},
	Eprint = {0802.2118},
	Journal = {\apjs},
	Keywords = {Galaxies: Individual: Name: Small Magellanic Cloud, Stars: Pulsars: General, X-Rays: Binaries},
	Month = jul,
	Pages = {189-215},
	Title = {{A Long Look at the Be/X-Ray Binaries of the Small Magellanic Cloud}},
	Volume = 177,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587743}}

@article{galloway08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..179..360G},
	Author = {{Galloway}, D.~K. and {Muno}, M.~P. and {Hartman}, J.~M. and {Psaltis}, D. and {Chakrabarty}, D.},
	Doi = {10.1086/592044},
	Eprint = {astro-ph/0608259},
	Journal = {\apjs},
	Keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Distances, Stars: Neutron, X-Rays: Bursts},
	Month = dec,
	Pages = {360-422},
	Title = {{Thermonuclear (Type I) X-Ray Bursts Observed by the Rossi X-Ray Timing Explorer}},
	Volume = 179,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/592044}}

@inproceedings{garmire00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000HEAD....5.3211G},
	Author = {{Garmire}, G.~P. and {Garmire}, A.~B. and {Pavlov}, G. and {Burrows}, D.~N.},
	Booktitle = {AAS/HEAD Fifth Meeting,},
	Month = oct,
	Pages = {1237},
	Series = {Bulletin of the American Astronomical Society, Washington DC},
	Title = {{A High State in the Central Object of RCW103}},
	Volume = 32,
	Year = 2000}

@article{gpg00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000IAUC.7350....2G},
	Author = {{Garmire}, G.~P. and {Pavlov}, G.~G. and {Garmire}, A.~B. and {Zavlin}, V.~E.},
	Journal = {\iaucirc},
	Month = jan,
	Pages = {2},
	Title = {{1E 161348-5055}},
	Volume = 7350,
	Year = 2000}

@inproceedings{garmire03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003SPIE.4851...28G},
	Author = {{Garmire}, G.~P. and {Bautz}, M.~W. and {Ford}, P.~G. and {Nousek}, J.~A. and {Ricker}, Jr., G.~R.},
	Booktitle = {X-Ray and Gamma-Ray Telescopes and Instruments for Astronomy.},
	Doi = {10.1117/12.461599},
	Editor = {{Truemper}, J.~E. and {Tananbaum}, H.~D.},
	Month = mar,
	Pages = {28-44},
	Publisher = {SPIE, Bellingham},
	Series = {Proceedings of the SPIE.},
	Title = {{Advanced CCD imaging spectrometer (ACIS) instrument on the Chandra X-ray Observatory}},
	Volume = 4851,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.461599}}

@article{gavriil02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002Natur.419..142G&db_key=AST},
	Author = {{Gavriil}, F.~P. and {Kaspi}, V.~M. and {Woods}, P.~M.},
	Journal = {\nat},
	Month = sep,
	Pages = {142-144},
	Title = {{Magnetar-like X-ray bursts from an anomalous X-ray pulsar}},
	Volume = 419,
	Year = 2002}

@article{gk02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...567.1067G},
	Author = {{Gavriil}, F.~P. and {Kaspi}, V.~M.},
	Doi = {10.1086/338698},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General- pulsars: individual (4U 0142+61, 1RXS J170849.0-400910, 1E 2259.1+586)- X-Rays: General},
	Month = mar,
	Pages = {1067-1076},
	Title = {{Long-Term Rossi X-Ray Timing Explorer Monitoring of Anomalous X-Ray Pulsars}},
	Volume = 567,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338698}}

@article{gavriil04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...609L..67G},
	Author = {{Gavriil}, F.~P. and {Kaspi}, V.~M.},
	Doi = {10.1086/422751},
	Eprint = {arXiv:astro-ph/0404113},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: 1E 1048.1-5937, X-Rays: General},
	Month = jul,
	Pages = {L67-L70},
	Title = {{Anomalous X-Ray Pulsar 1E 1048.1-5937: Pulsed Flux Flares and Large Torque Variations}},
	Volume = 609,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422751}}

@article{gkw04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607..959G},
	Author = {{Gavriil}, F.~P. and {Kaspi}, V.~M. and {Woods}, P.~M.},
	Doi = {10.1086/383564},
	Eprint = {arXiv:astro-ph/0310852},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: 1E 2259+586, X-Rays: Bursts, X-Rays: General},
	Month = jun,
	Pages = {959-969},
	Title = {{A Comprehensive Study of the X-Ray Bursts from the Magnetar Candidate 1E 2259+586}},
	Volume = 607,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/383564}}

@article{gehrels86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...303..336G},
	Author = {{Gehrels}, N.},
	Doi = {10.1086/164079},
	Journal = {\apj},
	Keywords = {ASTROPHYSICS, BINOMIAL THEOREM, CONFIDENCE LIMITS, DATA PROCESSING, POISSON DENSITY FUNCTIONS, APPROXIMATION, TABLES (DATA)},
	Month = apr,
	Pages = {336-346},
	Title = {{Confidence limits for small numbers of events in astrophysical data}},
	Volume = 303,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/164079}}

@article{gehrels04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611.1005G},
	Author = {{Gehrels}, N. and {Chincarini}, G. and {Giommi}, P. and {Mason}, K.~O. and {Nousek}, J.~A. and {Wells}, A.~A. and {White}, N.~E. and {Barthelmy}, S.~D. and {Burrows}, D.~N. and {Cominsky}, L.~R. and {Hurley}, K.~C. and {Marshall}, F.~E. and {M{\'e}sz{\'a}ros}, P. and {Roming}, P.~W.~A. and {Angelini}, L. and {Barbier}, L.~M. and {Belloni}, T. and {Campana}, S. and {Caraveo}, P.~A. and {Chester}, M.~M. and {Citterio}, O. and {Cline}, T.~L. and {Cropper}, M.~S. and {Cummings}, J.~R. and {Dean}, A.~J. and {Feigelson}, E.~D. and {Fenimore}, E.~E. and {Frail}, D.~A. and {Fruchter}, A.~S. and {Garmire}, G.~P. and {Gendreau}, K. and {Ghisellini}, G. and {Greiner}, J. and {Hill}, J.~E. and {Hunsberger}, S.~D. and {Krimm}, H.~A. and {Kulkarni}, S.~R. and {Kumar}, P. and {Lebrun}, F. and {Lloyd-Ronning}, N.~M. and {Markwardt}, C.~B. and {Mattson}, B.~J. and {Mushotzky}, R.~F. and {Norris}, J.~P. and {Osborne}, J. and {Paczynski}, B. and {Palmer}, D.~M. and {Park}, H.-S. and {Parsons}, A.~M. and {Paul}, J. and {Rees}, M.~J. and {Reynolds}, C.~S. and {Rhoads}, J.~E. and {Sasseen}, T.~P. and {Schaefer}, B.~E. and {Short}, A.~T. and {Smale}, A.~P. and {Smith}, I.~A. and {Stella}, L. and {Tagliaferri}, G. and {Takahashi}, T. and {Tashiro}, M. and {Townsley}, L.~K. and {Tueller}, J. and {Turner}, M.~J.~L. and {Vietri}, M. and {Voges}, W. and {Ward}, M.~J. and {Willingale}, R. and {Zerbi}, F.~M. and {Zhang}, W.~W.},
	Doi = {10.1086/422091},
	Eprint = {arXiv:astro-ph/0405233},
	Journal = {\apj},
	Month = aug,
	Pages = {1005-1020},
	Title = {{The Swift Gamma-Ray Burst Mission}},
	Volume = 611,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422091}}

@article{gelbord10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010GCN.10526....1G},
	Author = {{Gelbord}, J.~M. and {Barthelmy}, S.~D. and {Baumgartner}, W.~H. and {Burrows}, D.~N. and {Gehrels}, N. and {Grupe}, D. and {Holland}, S.~T. and {Kennea}, J.~A. and {Marshall}, F.~E. and {O'Brien}, P.~T. and {Osborne}, J.~P. and {Palmer}, D.~M. and {Romano}, P. and {Sakamoto}, T. and {Siegel}, M.~H. and {Stamatikos}, M. and {Stark}, M.~A. and {Troja}, E. and {Ukwatta}, T.~N.},
	Journal = {GCN Circ.},
	Title = {{GRB 100319A: Swift detection of a burst; possible Sgr.}},
	Volume = 10526,
	Year = 2010}

@article{gv10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010GCN.10531....1G},
	Author = {{Gelbord}, J.~M. and {Vetere}, L.},
	Journal = {GCN Circ.},
	Title = {{Probable Sgr 1833-0832: Swift-XRT refined analysis.}},
	Volume = 10531,
	Year = 2010}

@article{gelfand05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...634L..89G},
	Author = {{Gelfand}, J.~D. and {Lyubarsky}, Y.~E. and {Eichler}, D. and {Gaensler}, B.~M. and {Taylor}, G.~B. and {Granot}, J. and {Newton-McGee}, K.~J. and {Ramirez-Ruiz}, E. and {Kouveliotou}, C. and {Wijers}, R.~A.~M.~J.},
	Doi = {10.1086/498643},
	Eprint = {arXiv:astro-ph/0503269},
	Journal = {\apjl},
	Month = nov,
	Pages = {L89-L92},
	Title = {{A Rebrightening of the Radio Nebula Associated with the 2004 December 27 Giant Flare from SGR 1806-20}},
	Volume = 634,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498643}}

@article{gelfand07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...667.1111G},
	Archiveprefix = {arXiv},
	Author = {{Gelfand}, J.~D. and {Gaensler}, B.~M.},
	Doi = {10.1086/520526},
	Eprint = {0706.1054},
	Journal = {\apj},
	Keywords = {ISM: individual (G327.24-0.13), Stars: Neutron, ISM: Supernova Remnants, X-rays: individual (1E 1547.0-5408), X-Rays: Stars},
	Month = oct,
	Pages = {1111-1118},
	Title = {{The Compact X-Ray Source 1E 1547.0-5408 and the Radio Shell G327.24-0.13: A New Proposed Association between a Candidate Magnetar and a Candidate Supernova Remnant}},
	Volume = 667,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/520526}}

@article{genzel10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010RvMP...82.3121G},
	Archiveprefix = {arXiv},
	Author = {{Genzel}, R. and {Eisenhauer}, F. and {Gillessen}, S.},
	Doi = {10.1103/RevModPhys.82.3121},
	Eprint = {1006.0064},
	Journal = {Reviews of Modern Physics},
	Keywords = {Galactic center, bar, circumnuclear matter, and bulge},
	Month = oct,
	Pages = {3121-3195},
	Primaryclass = {astro-ph.GA},
	Title = {{The Galactic Center massive black hole and nuclear star cluster}},
	Volume = 82,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/RevModPhys.82.3121}}

@ARTICLE{geppert02,
   author = {{Geppert}, U. and {Rheinhardt}, M.},
    title = "{Non-linear magnetic field decay in neutron stars. Theory and observations}",
  journal = {\aap},
   eprint = {astro-ph/0207065},
 keywords = {stars: neutron, stars: magnetic fields, stars: evolution, stars: pulsars: general},
     year = 2002,
    month = sep,
   volume = 392,
    pages = {1015-1024},
      doi = {10.1051/0004-6361:20020978},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...392.1015G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{geppert06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2006A%26A...456..639G&db_key=AST},
	Author = {{Geppert}, U. and {Rheinhardt}, M.},
	Doi = {10.1051/0004-6361:20065144},
	Eprint = {astro-ph/0606120},
	Journal = {\aap},
	Month = sep,
	Pages = {639-649},
	Title = {{Magnetars versus radio pulsars. MHD stability in newborn highly magnetized neutron stars}},
	Volume = 456,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065144}}

@article{ghez08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...689.1044G},
	Archiveprefix = {arXiv},
	Author = {{Ghez}, A.~M. and {Salim}, S. and {Weinberg}, N.~N. and {Lu}, J.~R. and {Do}, T. and {Dunn}, J.~K. and {Matthews}, K. and {Morris}, M.~R. and {Yelda}, S. and {Becklin}, E.~E. and {Kremenek}, T. and {Milosavljevic}, M. and {Naiman}, J.},
	Doi = {10.1086/592738},
	Eprint = {0808.2870},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Galaxy: Center, Galaxy: Kinematics and Dynamics, Infrared: Stars, Techniques: High Anular Resolution},
	Month = dec,
	Pages = {1044-1062},
	Title = {{Measuring Distance and Properties of the Milky Way's Central Supermassive Black Hole with Stellar Orbits}},
	Volume = 689,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/592738}}

@article{ghosh79,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...232..259G},
	Author = {{Ghosh}, P. and {Lamb}, F.~K.},
	Doi = {10.1086/157285},
	Journal = {\apj},
	Keywords = {MAGNETIC STARS, NEUTRON STARS, STELLAR MASS ACCRETION, BOUNDARY LAYER FLOW, BOUNDARY LAYERS, DISKS (SHAPES), EARTH MAGNETOSPHERE, KELVIN-HELMHOLTZ INSTABILITY, KEPLER LAWS, STELLAR MAGNETIC FIELDS, STELLAR ROTATION, TURBULENT DIFFUSION},
	Month = aug,
	Pages = {259-276},
	Title = {{Accretion by rotating magnetic neutron stars. II - Radial and vertical structure of the transition zone in disk accretion}},
	Volume = 232,
	Year = 1979,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/157285}}

@article{gl79,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...234..296G},
	Author = {{Ghosh}, P. and {Lamb}, F.~K.},
	Doi = {10.1086/157498},
	Journal = {\apj},
	Keywords = {MAGNETIC STARS, NEUTRON STARS, STELLAR MASS ACCRETION, STELLAR ROTATION, X RAY SOURCES, ANGULAR VELOCITY, KEPLER LAWS, MAGNETOHYDRODYNAMICS, NUMERICAL ANALYSIS, PERIODIC VARIATIONS, SPIN REDUCTION, STELLAR LUMINOSITY, STELLAR MAGNETIC FIELDS, STELLAR WINDS, TORQUE},
	Month = nov,
	Pages = {296-316},
	Title = {{Accretion by rotating magnetic neutron stars. III - Accretion torques and period changes in pulsating X-ray sources}},
	Volume = 234,
	Year = 1979,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/157498}}

@article{ghosh09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.3263G},
	Archiveprefix = {arXiv},
	Author = {{Ghosh}, K.~K. and {Saripalli}, L. and {Gandhi}, P. and {Foellmi}, C. and {Guti{\'e}rrez}, C.~M. and {L{\'o}pez-Corredoira}, M.},
	Doi = {10.1088/0004-6256/137/2/3263},
	Eprint = {0810.5393},
	Journal = {\aj},
	Keywords = {binaries: general, black hole physics, galaxies: interactions, X-rays: individual: NGC 5774 and NGC 5775},
	Month = feb,
	Pages = {3263-3285},
	Title = {{Multiwavelength Study of the Bright X-Ray Source Population in the Interacting Galaxies NGC 5774/NGC 5775}},
	Volume = 137,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/137/2/3263}}

@ARTICLE{Giacconi1962,
       author = {{Giacconi}, Riccardo and {Gursky}, Herbert and {Paolini}, Frank R. and {Rossi}, Bruno B.},
        title = "{Evidence for x Rays From Sources Outside the Solar System}",
      journal = {\prl},
         year = 1962,
        month = dec,
       volume = {9},
       number = {11},
        pages = {439-443},
          doi = {10.1103/PhysRevLett.9.439},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1962PhRvL...9..439G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{giacconi65,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1965SSRv....4..151G&db_key=AST},
	Author = {{Giacconi}, R. and {Gursky}, H.},
	Journal = {Space Science Reviews},
	Pages = {151},
	Title = {{Observation of X-Ray Sources Outside the Solar System}},
	Volume = 4,
	Year = 1965}

@article{giacconi67,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1967ApJ...148L.119G},
	Author = {{Giacconi}, R. and {Gorenstein}, P. and {Gursky}, H. and {Waters}, J.~R.},
	Doi = {10.1086/180028},
	Journal = {\apjl},
	Month = jun,
	Pages = {L119},
	Title = {{An X-Ray Survey of the Cygnus Region}},
	Volume = 148,
	Year = 1967,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/180028}}

@article{giacconi71,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1971ApJ...165L..27G&db_key=AST},
	Author = {{Giacconi}, R. and {Kellogg}, E. and {Gorenstein}, P. and {Gursky}, H. and {Tananbaum}, H.},
	Journal = {\apjl},
	Month = apr,
	Pages = {L27},
	Title = {{An X-Ray Scan of the Galactic Plane from UHURU}},
	Volume = 165,
	Year = 1971}

@article{ggk71,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...167L..67G},
	Author = {{Giacconi}, R. and {Gursky}, H. and {Kellogg}, E. and {Schreier}, E. and {Tananbaum}, H.},
	Doi = {10.1086/180762},
	Journal = {\apjl},
	Month = jul,
	Pages = {L67},
	Title = {{Discovery of Periodic X-Ray Pulsations in Centaurus X-3 from UHURU}},
	Volume = 167,
	Year = 1971,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/180762}}

@ARTICLE{giacconi79,
       author = {{Giacconi}, R. and {Branduardi}, G. and {Briel}, U. and {Epstein}, A. and {Fabricant}, D. and {Feigelson}, E. and {Forman}, W. and {Gorenstein}, P. and {Grindlay}, J. and {Gursky}, H. and {Harnden}, F.~R. and {Henry}, J.~P. and {Jones}, C. and {Kellogg}, E. and {Koch}, D. and {Murray}, S. and {Schreier}, E. and {Seward}, F. and {Tananbaum}, H. and {Topka}, K. and {Van Speybroeck}, L. and {Holt}, S.~S. and {Becker}, R.~H. and {Boldt}, E.~A. and {Serlemitsos}, P.~J. and {Clark}, G. and {Canizares}, C. and {Markert}, T. and {Novick}, R. and {Helfand}, D. and {Long}, K.},
        title = "{The Einstein (HEAO 2) X-ray Observatory.}",
      journal = {\apj},
     keywords = {Heao 2, Spaceborne Astronomy, X Ray Astronomy, Cameras, Focal Plane Devices, High Resolution, Proportional Counters, Spaceborne Telescopes, Spacecraft Instruments, Spectrometers, Astronomy, X-Ray Telescopes},
         year = 1979,
        month = jun,
       volume = {230},
        pages = {540-550},
          doi = {10.1086/157110},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...230..540G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{giesers19,
       author = {{Giesers}, Benjamin and {Kamann}, Sebastian and {Dreizler}, Stefan and
         {Husser}, Tim-Oliver and {Askar}, Abbas and {G{\"o}ttgens}, Fabian and
         {Brinchmann}, Jarle and {Latour}, Marilyn and {Weilbacher}, Peter M. and
         {Wendt}, Martin and {Roth}, Martin M.},
        title = "{A stellar census in globular clusters with MUSE: Binaries in NGC 3201}",
      journal = {\aap},
     keywords = {binaries: general, blue stragglers, stars: black holes, techniques: radial velocities, techniques: imaging spectroscopy, globular clusters: individual: NGC 3201, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = dec,
       volume = {632},
          eid = {A3},
        pages = {A3},
          doi = {10.1051/0004-6361/201936203},
archivePrefix = {arXiv},
       eprint = {1909.04050},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A...3G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gilfanov04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.349..146G},
	Author = {{Gilfanov}, M.},
	Doi = {10.1111/j.1365-2966.2004.07473.x},
	Eprint = {arXiv:astro-ph/0309454},
	Journal = {\mnras},
	Keywords = {galaxies: elliptical and lenticular, cD, galaxies: fundamental parameters, galaxies: spiral, X-rays: binaries, X-rays: galaxies},
	Month = mar,
	Pages = {146-168},
	Title = {{Low-mass X-ray binaries as a stellar mass indicator for the host galaxy}},
	Volume = 349,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07473.x}}

@article{gillessen09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...692.1075G},
	Archiveprefix = {arXiv},
	Author = {{Gillessen}, S. and {Eisenhauer}, F. and {Trippe}, S. and {Alexander}, T. and {Genzel}, R. and {Martins}, F. and {Ott}, T.},
	Doi = {10.1088/0004-637X/692/2/1075},
	Eprint = {0810.4674},
	Journal = {\apj},
	Keywords = {black hole physics, astrometry, Galaxy: center, infrared: stars},
	Month = feb,
	Pages = {1075-1109},
	Title = {{Monitoring Stellar Orbits Around the Massive Black Hole in the Galactic Center}},
	Volume = 692,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/692/2/1075}}

@ARTICLE{gillessen12,
   author = {{Gillessen}, S. and {Genzel}, R. and {Fritz}, T.~K. and {Quataert}, E. and 
	{Alig}, C. and {Burkert}, A. and {Cuadra}, J. and {Eisenhauer}, F. and 
	{Pfuhl}, O. and {Dodds-Eden}, K. and {Gammie}, C.~F. and {Ott}, T.
	},
    title = "{A gas cloud on its way towards the supermassive black hole at the Galactic Centre}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1112.3264},
 primaryClass = "astro-ph.GA",
     year = 2012,
    month = jan,
   volume = 481,
    pages = {51-54},
      doi = {10.1038/nature10652},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.481...51G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gillessen13,
   author = {{Gillessen}, S. and {Genzel}, R. and {Fritz}, T.~K. and {Eisenhauer}, F. and 
	{Pfuhl}, O. and {Ott}, T. and {Cuadra}, J. and {Schartmann}, M. and 
	{Burkert}, A.},
    title = "{New Observations of the Gas Cloud G2 in the Galactic Center}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.2272},
 keywords = {accretion, accretion disks, black hole physics, Galaxy: center, infrared: general, ISM: clouds},
     year = 2013,
    month = feb,
   volume = 763,
      eid = {78},
    pages = {78},
      doi = {10.1088/0004-637X/763/2/78},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763...78G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gilmozzi87,
   author = {{Gilmozzi}, R. and {Cassatella}, A. and {Clavel}, J. and {Fransson}, C. and 
	{Gonzalez}, R. and {Gry}, C. and {Panagia}, N. and {Talavera}, A. and 
	{Wamsteker}, W.},
    title = "{The progenitor of SN1987A}",
  journal = {\nat},
 keywords = {Astronomical Spectroscopy, Iue, Magellanic Clouds, Supernovae, B Stars, Spatial Distribution, Stellar Spectra},
     year = 1987,
    month = jul,
   volume = 328,
    pages = {318-320},
      doi = {10.1038/328318a0},
   adsurl = {http://adsabs.harvard.edu/abs/1987Natur.328..318G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{giustini20,
       author = {{Giustini}, Margherita and {Miniutti}, Giovanni and {Saxton}, Richard D.},
        title = "{X-ray quasi-periodic eruptions from the galactic nucleus of RX J1301.9+2747}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: nuclei, quasars: general, quasars: supermassive black holes, X-rays: individuals: RX J1301.9+2747, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = apr,
       volume = {636},
          eid = {L2},
        pages = {L2},
          doi = {10.1051/0004-6361/202037610},
archivePrefix = {arXiv},
       eprint = {2002.08967},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...636L...2G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gladstone09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.397..124G},
	Archiveprefix = {arXiv},
	Author = {{Gladstone}, J.~C. and {Roberts}, T.~P.},
	Doi = {10.1111/j.1365-2966.2009.14937.x},
	Eprint = {0904.3852},
	Journal = {\mnras},
	Keywords = {black hole physics , galaxies: individual: NGC 4485 , galaxies: individual: NGC 4490 , X-rays: binaries , X-rays: galaxies},
	Month = jul,
	Pages = {124-134},
	Primaryclass = {astro-ph.HE},
	Title = {{The ultraluminous X-ray source population of NGC 4485/4490}},
	Volume = 397,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14937.x}}

@article{grd09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397.1836G},
	Archiveprefix = {arXiv},
	Author = {{Gladstone}, J.~C. and {Roberts}, T.~P. and {Done}, C.},
	Doi = {10.1111/j.1365-2966.2009.15123.x},
	Eprint = {0905.4076},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , black hole physics , X-rays: binaries , X-rays: galaxies},
	Month = aug,
	Pages = {1836-1851},
	Primaryclass = {astro-ph.CO},
	Title = {{The ultraluminous state}},
	Volume = 397,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15123.x}}

@article{gladstone13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..206...14G},
	Archiveprefix = {arXiv},
	Author = {{Gladstone}, J.~C. and {Copperwheat}, C. and {Heinke}, C.~O. and {Roberts}, T.~P. and {Cartwright}, T.~F. and {Levan}, A.~J. and {Goad}, M.~R.},
	Doi = {10.1088/0067-0049/206/2/14},
	Eid = {14},
	Eprint = {1303.1213},
	Journal = {\apjs},
	Keywords = {accretion, accretion disks, binaries: general, black hole physics, X-rays: binaries},
	Month = jun,
	Pages = {14},
	Primaryclass = {astro-ph.HE},
	Title = {{Optical Counterparts of the Nearest Ultraluminous X-Ray Sources}},
	Volume = 206,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/206/2/14}}

@ARTICLE{glampedakis06,
   author = {{Glampedakis}, K. and {Samuelsson}, L. and {Andersson}, N.},
    title = "{Elastic or magnetic? A toy model for global magnetar oscillations with implications for quasi-periodic oscillations during flares}",
  journal = {\mnras},
   eprint = {astro-ph/0605461},
 keywords = {MHD: stars: neutron: stars: oscillations, MHD, stars: neutron, stars: oscillations},
     year = 2006,
    month = sep,
   volume = 371,
    pages = {L74-L77},
      doi = {10.1111/j.1745-3933.2006.00211.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371L..74G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{glampedakis11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.2021G},
	Archiveprefix = {arXiv},
	Author = {{Glampedakis}, K. and {Jones}, D.~I. and {Samuelsson}, L.},
	Doi = {10.1111/j.1365-2966.2011.18278.x},
	Eprint = {1010.1153},
	Journal = {\mnras},
	Keywords = {stars: magnetars, stars: magnetic field, stars: neutron},
	Month = may,
	Pages = {2021-2030},
	Primaryclass = {astro-ph.SR},
	Title = {{Ambipolar diffusion in superfluid neutron stars}},
	Volume = 413,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.18278.x}}

@ARTICLE{glampedakis14,
   author = {{Glampedakis}, K. and {Jones}, D.~I.},
    title = "{Three evolutionary paths for magnetar oscillations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1307.7078},
 primaryClass = "astro-ph.SR",
 keywords = {dense matter, stars: magnetars, stars: neutron, stars: oscillations},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {1522-1535},
      doi = {10.1093/mnras/stu017},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.1522G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gnedin74,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974A%26A....36..379G&db_key=AST},
	Author = {{Gnedin}, I.~N. and {Sunyaev}, R.~A.},
	Journal = {\aap},
	Month = dec,
	Pages = {379-394},
	Title = {{Polarization of optical and X-radiation from compact thermal sources with magnetic field}},
	Volume = 36,
	Year = 1974}

@article{goad06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365..191G},
	Author = {{Goad}, M.~R. and {Roberts}, T.~P. and {Reeves}, J.~N. and {Uttley}, P.},
	Doi = {10.1111/j.1365-2966.2005.09702.x},
	Eprint = {arXiv:astro-ph/0510185},
	Journal = {\mnras},
	Keywords = {black hole physics, X-rays: binaries, X-rays: galaxies},
	Month = jan,
	Pages = {191-198},
	Title = {{A deep XMM-Newton observation of the ultraluminous X-ray source Holmberg II X-1: the case against a 1000-M$_{solar}$ black hole}},
	Volume = 365,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09702.x}}

@article{gbb06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006GCN..4985....1G},
	Author = {{Goad}, M.~R. and {Barbier}, L.~M. and {Barthelmy}, S.~D. and {Beardmore}, A.~P. and {Brown}, P.~J. and {Burrows}, D.~N. and {Cummings}, J.~R. and {Gehrels}, N. and {Holland}, S.~T. and {Kennea}, J.~A. and {Palmer}, D.~M.},
	Journal = {GCN Circ.},
	Title = {{GRB(?) 060421: swift detection of a burst.}},
	Volume = 4985,
	Year = 2006}

@ARTICLE{gogus99,
   author = {{G{\"o}{\v g}{\"u}{\c s} }, E. and {Woods}, P.~M. and {Kouveliotou}, C. and 
	{van Paradijs}, J. and {Briggs}, M.~S. and {Duncan}, R.~C. and 
	{Thompson}, C.},
    title = "{Statistical Properties of SGR 1900+14 Bursts}",
  journal = {\apjl},
   eprint = {astro-ph/9910062},
 keywords = {GAMMA RAYS: BURSTS, STARS: INDIVIDUAL: ALPHANUMERIC: SGR 1900+14, X-RAYS: BURSTS, Gamma Rays: Bursts, Stars: Individual: Alphanumeric: SGR 1900+14, X-Rays: Bursts},
     year = 1999,
    month = dec,
   volume = 526,
    pages = {L93-L96},
      doi = {10.1086/312380},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...526L..93G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gogus00,
   author = {{G{\"o}{\v g}{\"u}{\c s}}, E. and {Woods}, P.~M. and {Kouveliotou}, C. and 
	{van Paradijs}, J. and {Briggs}, M.~S. and {Duncan}, R.~C. and 
	{Thompson}, C.},
    title = "{Statistical Properties of SGR 1806-20 Bursts}",
  journal = {\apjl},
   eprint = {astro-ph/0002181},
 keywords = {GAMMA RAYS: BURSTS, STARS: INDIVIDUAL: ALPHANUMERIC: SGR 1806-20, X-RAYS: BURSTS},
     year = 2000,
    month = apr,
   volume = 532,
    pages = {L121-L124},
      doi = {10.1086/312583},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...532L.121G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gogus01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...558..228G&amp;db_key=AST},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C. and {Woods}, P.~M. and {Thompson}, C. and {Duncan}, R.~C. and {Briggs}, M.~S.},
	Journal = {\apj},
	Month = sep,
	Pages = {228-236},
	Title = {{Temporal and Spectral Characteristics of Short Bursts from the Soft Gamma Repeaters 1806-20 and 1900+14}},
	Volume = 558,
	Year = 2001}

@article{gogus02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...577..929G&db_key=AST},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C. and {Woods}, P.~M. and {Finger}, M.~H. and {van der Klis}, M.},
	Journal = {\apj},
	Month = oct,
	Pages = {929-939},
	Title = {{A Comprehensive Study of Pulse Profile Evolution in SGR 1806-20 and SGR 1900+14 with the Rossi X-Ray Timing Explorer Proportional Counter Array}},
	Volume = 577,
	Year = 2002}

@article{gogus05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...632.1069G&db_key=AST},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Patel}, S.~K. and {Wilson}, C.~A. and {Woods}, P.~M. and {Finger}, M.~H. and {Kouveliotou}, C.},
	Doi = {10.1086/444373},
	Journal = {\apj},
	Month = oct,
	Pages = {1069-1074},
	Title = {{Chandra Localization of XTE J1906+090 and Discovery of its Optical and Infrared Counterparts}},
	Volume = 632,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/444373}}

@article{gogus_atel2076_09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2076....1G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Woods}, P. and {Kouveliotou}, C.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients},
	Month = jun,
	Title = {{RXTE Discovery of Pulsations from SGR 0418+5729}},
	Volume = 2076,
	Year = 2009}

@article{gogus_atel2121_09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2121....1G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C. and {Woods}, P.~M.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients},
	Month = jul,
	Title = {{Swift XRT Observations of SGR 0418+4729}},
	Volume = 2121,
	Year = 2009}

@article{gogus10atel,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ATel.2493....1G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Strohmayer}, T. and {Kouveliotou}, C. and {Woods}, P.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Pulsars, Soft Gamma-ray Repeaters},
	Month = mar,
	Title = {{Discovery of the Spin Period of SGR 1833-0832}},
	Volume = 2493,
	Year = 2010}

@article{gogus10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1005.3029G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Cusumano}, G. and {Levan}, A.~J. and {Kouveliotou}, C. and {Sakamoto}, T. and {Barthelmy}, S.~D. and {Campana}, S. and {Kaneko}, Y. and {Stappers}, B.~W. and {de Ugarte-Postigo}, A. and {Strohmayer}, T. and {Palmer}, D.~M. and {Gelbord}, J. and {Burrows}, D.~N. and {van der Horst}, A.~J. and {Munoz-Darias}, T. and {Gehrels}, N. and {Hessels}, J.~W.~T. and {Kamble}, A.~P. and {Wachter}, S. and {Wiersema}, K. and {Wijers}, R.~A.~M.~J. and {Woods}, P.~M.},
	Journal = {\apj},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = jul,
	Pages = {331-339},
	Title = {{Discovery of a new Soft Gamma Repeater, SGR J1833-0832}},
	Volume = 718,
	Year = 2010}

@article{gogus11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3542....1G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Star, Soft Gamma-ray Repeater, Pulsar},
	Month = aug,
	Title = {{RXTE Discovery of the Spin Period of Swift J1834.9-0846}},
	Volume = 3542,
	Year = 2011}

@article{gsk11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3503....1G},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Strohmayer}, T. and {Kouveliotou}, C.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Star, Soft Gamma-ray Repeater},
	Month = jul,
	Title = {{SGR 1822-1606 (Swift 1822.3-1606): Spin-down rate and inferred dipole field strength}},
	Volume = 3503,
	Year = 2011}

@article{gkb11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525L...6G},
	Archiveprefix = {arXiv},
	Author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Kreykenbohm}, I. and {Belloni}, T.~M.},
	Doi = {10.1051/0004-6361/201015905},
	Eid = {L6},
	Eprint = {1011.3899},
	Journal = {\aap},
	Keywords = {X-rays: stars, pulsars: individual: GX 301-2},
	Month = jan,
	Pages = {L6},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of a peculiar dip from GX 301-2}},
	Volume = 525,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201015905}}

@ARTICLE{gwk11,
   author = {{G{\"o}{\v g}{\"u}{\c s}}, E. and {Woods}, P.~M. and {Kouveliotou}, C. and 
	{Finger}, M.~H. and {Pal'shin}, V. and {Kaneko}, Y. and {Golenetskii}, S. and 
	{Frederiks}, D. and {Airhart}, C.},
    title = "{Extended Tails from SGR 1806-20 Bursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.4050},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: SGR 1806{\ndash}20, X-rays: bursts},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {55},
    pages = {55},
      doi = {10.1088/0004-637X/740/2/55},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740...55G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gogus16,
   author = {{G{\"o}{\u g}{\"u}{\c s}}, E. and {Lin}, L. and {Kaneko}, Y. and 
	{Kouveliotou}, C. and {Watts}, A.~L. and {Chakraborty}, M. and 
	{Alpar}, M.~A. and {Huppenkothen}, D. and {Roberts}, O.~J. and 
	{Younes}, G. and {van der Horst}, A.~J.},
    title = "{Magnetar-like X-Ray Bursts from a Rotation-powered Pulsar, PSR J1119-6127}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1608.07133},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: PSR J1119{\ndash}6127, stars: magnetars, X-rays: bursts},
     year = 2016,
    month = oct,
   volume = 829,
      eid = {L25},
    pages = {L25},
      doi = {10.3847/2041-8205/829/2/L25},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...829L..25G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{goldoni95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...299..751G&db_key=AST},
	Author = {{Goldoni}, P. and {Mereghetti}, S.},
	Eprint = {astro-ph/9502044},
	Journal = {\aap},
	Month = jul,
	Pages = {751},
	Title = {{X-ray observations of the peculiar Be star LSI +61 303.}},
	Volume = 299,
	Year = 1995}

@article{goldreich69,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1969ApJ...156...59G},
	Author = {{Goldreich}, P. and {Lynden-Bell}, D.},
	Doi = {10.1086/149947},
	Journal = {\apj},
	Month = apr,
	Pages = {59-78},
	Title = {{Io, a jovian unipolar inductor}},
	Volume = 156,
	Year = 1969,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/149947}}

@article{goldreich92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...395..250G},
	Author = {{Goldreich}, P. and {Reisenegger}, A.},
	Doi = {10.1086/171646},
	Journal = {\apj},
	Keywords = {CHARGED PARTICLES, MAGNETIC FLUX, MAGNETIC STARS, NEUTRON STARS, STELLAR MAGNETIC FIELDS, DECAY, EARLY STARS, PULSARS, X RAY BINARIES},
	Month = aug,
	Pages = {250-258},
	Title = {{Magnetic field decay in isolated neutron stars}},
	Volume = 395,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/171646}}

@article{golenetskii87,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1987SvAL...13..166G&db_key=AST},
	Author = {{Golenetskii}, S.~V. and {Aptekar}, R.~L. and {Guryan}, Y.~A. and {Ilinskii}, V.~N. and {Mazets}, E.~P.},
	Journal = {Soviet Astronomy Letters},
	Month = may,
	Pages = {166},
	Title = {{The Recurrent Gamma-Ray Burster GBS:0526-66}},
	Volume = 13,
	Year = 1987}

@article{golenetskii04_gcn1,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2665....1G&db_key=AST},
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'Shin}, V. and {Frederiks}, D. and {Cline}, T. and {Rau}, A. and {von Kienlin}, A. and {Lichti}, G.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Increase of Sgr 1806-20 activity.}},
	Volume = 2665,
	Year = 2004}

@article{golenetskii04_gcn2,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2769....1G&db_key=AST},
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'Shin}, V. and {Frederiks}, D. and {Cline}, T.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Konus-wind observation of a series Sgr 1806-20 bursts on 041005.}},
	Volume = 2769,
	Year = 2004}

@article{golenetskii04_gcn3,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2923....1G&db_key=AST},
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'Shin}, V. and {Frederiks}, D. and {Cline}, T.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Detection of the Sgr 1806-20 giant outburst back-scattered by the.}},
	Volume = 2923,
	Year = 2004}

@article{golenetskii06_gcn1,
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'shin}, V. and {Frederiks}, D. and {Cline}, T.},
	Journal = {GRB Circular Network},
	Title = {{SGR 1900+14: bright burst detected by Konus-Wind on March 28}},
	Volume = 4936,
	Year = 2006}

@article{golenetskii06_gcn2,
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'shin}, V. and {Frederiks}, D. and {Cline}, T.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Konus-Wind observation of the recent SGR 1900+14 activity. Will}},
	Volume = 4946,
	Year = 2006}

@article{golenetskii07,
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'shin}, V. and {Frederiks}, D. and {Cline}, T. and {Kienlin}, A.~v. and {Lichti}, G. and {Rau}, A. and {G\"otz}, D. and {Mereghetti}, S. and {Yamaoka}, K. and {Uehara}, T. and {Ohno}, M. and {Fukazawa}, Y. and {Takahashi}, T. and {Tashiro}, M. and {Terada}, Y. and {Murakami}, T. and {Makishima}, K. and {Hurley}, K. and {Smith}, D.~M. and {Lin}, R.~P. and {McTiernan}, J. and {Schwartz}, R. and {Wigger}, C. and {Hajdas}, W. and {Zehnder}, A.},
	Journal = {GCN Circ. 6684},
	Title = {{Intense burst from SGR 1806-20 detected on July 27}},
	Year = 2007}

@article{golenetskii08,
	Author = {{Golenetskii}, S. and {Aptekar}, R. and {Mazets}, E. and {Pal'shin}, V. and {Frederiks}, D. and {Oleynik}, P. and {Ulanov}, M. and {Cline}, T.},
	Journal = {GCN Circ.},
	Title = {{Konus-Wind observation of reactivation of SGR 1627-41}},
	Volume = 7778,
	Year = 2008}

@book{gombrich95,
  title={The Story of Art},
  author={Gombrich, E.~H.},
  isbn={9780714832470},
  lccn={96140698},
  series={16th Edition},
  url={https://books.google.co.in/books?id=LEMfwo7LQoMC},
  year={1995},
  publisher={Phaidon Press (London)}
}

@article{gonzalez05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005ApJ...630..489G&db_key=AST},
	Author = {{Gonzalez}, M.~E. and {Kaspi}, V.~M. and {Camilo}, F. and {Gaensler}, B.~M. and {Pivovaroff}, M.~J.},
	Doi = {10.1086/432032},
	Eprint = {astro-ph/0505332},
	Journal = {\apj},
	Month = sep,
	Pages = {489-494},
	Title = {{Unusual Pulsed X-Ray Emission from the Young, High Magnetic Field Pulsar PSR J1119-6127}},
	Volume = 630,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432032}}

@ARTICLE{gonzalez10,
   author = {{Gonzalez}, D. and {Reisenegger}, A.},
    title = "{Internal heating of old neutron stars: contrasting different mechanisms}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1005.5699},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, dense matter, stars: rotation, pulsars: general, pulsars: individual: PSR J0437-4715, pulsars: individual: PSR B0950+08},
     year = 2010,
    month = nov,
   volume = 522,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201015084},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...522A..16G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{gorosabel11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3496....1G},
	Author = {{Gorosabel}, J. and {de Ugarte Postigo}, A. and {Mottola}, S. and {Hellmich}, S. and {Ferrero}, P. and {Sanchez-Ramirez}, R. and {Tello}, J.~C. and {Casanova}, V. and {Marti}, R. and {Castro-Tirado}, A.~J.},
	Journal = {Astron. Tel.},
	Keywords = {Infra-Red, Optical, Gamma-Ray Burst, Neutron Star, Soft Gamma-ray Repeater, Transient},
	Month = jul,
	Title = {{Swift J1822.3-1606: Optical/NIR counterpart candidate}},
	Volume = 3496,
	Year = 2011}

@article{gotthelf97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...486L.133G&db_key=AST},
	Author = {{Gotthelf}, E.~V. and {Vasisht}, G.},
	Doi = {10.1086/310846},
	Journal = {\apjl},
	Month = sep,
	Pages = {L133},
	Title = {{Kes 73: A Young Supernova Remnant with an X-Ray--bright, Radio-quiet Central Source}},
	Volume = 486,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310846}}

@article{gph97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...487L.175G},
	Author = {{Gotthelf}, E.~V. and {Petre}, R. and {Hwang}, U.},
	Doi = {10.1086/310900},
	Eprint = {arXiv:astro-ph/9707035},
	Journal = {\apjl},
	Keywords = {STARS: NEUTRON, STARS: INDIVIDUAL ALPHANUMERIC: 1E 161348-5055, STARS: INDIVIDUAL ALPHANUMERIC: RCW 103, ISM: SUPERNOVA REMNANTS, X-RAYS: STARS},
	Month = oct,
	Pages = {L175},
	Title = {{The Nature of the Radio-quiet Compact X-Ray Source in SNR RCW 103}},
	Volume = 487,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310900}}

@article{gotthelf98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998NewA....3..293G},
	Author = {{Gotthelf}, E.~V. and {Vasisht}, G.},
	Doi = {10.1016/S1384-1076(98)00014-1},
	Eprint = {arXiv:astro-ph/9804025},
	Journal = {\na},
	Keywords = {PULSARS: GENERAL, PULSARS: INDIVIDUAL: AX J1845-0258, X-RAYS: GENERAL, SUPERNOVA REMNANTS},
	Month = jul,
	Pages = {293-300},
	Title = {{Discovery of a 7 second anomalous X-ray pulsar in the distant Milky Way}},
	Volume = 3,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/S1384-1076(98)00014-1}}

@article{gotthelf99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...514L.107G},
	Author = {{Gotthelf}, E.~V. and {Petre}, R. and {Vasisht}, G.},
	Doi = {10.1086/311948},
	Eprint = {arXiv:astro-ph/9901371},
	Journal = {\apjl},
	Keywords = {STARS: INDIVIDUAL: ALPHANUMERIC: 1E 161348-5055, STARS: NEUTRON, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: INDIVIDUAL: ALPHANUMERIC: RCW 103, X-RAYS: STARS},
	Month = apr,
	Pages = {L107-L110},
	Title = {{X-Ray Variability from the Compact Source in the Supernova Remnant RCW 103}},
	Volume = 514,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311948}}

@article{gvd99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...522L..49G},
	Author = {{Gotthelf}, E.~V. and {Vasisht}, G. and {Dotani}, T.},
	Doi = {10.1086/312220},
	Eprint = {arXiv:astro-ph/9906122},
	Journal = {\apjl},
	Keywords = {STARS: INDIVIDUAL: ALPHANUMERIC: KES 73, STARS: INDIVIDUAL: ALPHANUMERIC: 1E 1841-045, STARS: NEUTRON, ISM: SUPERNOVA REMNANTS, X-RAYS: STARS},
	Month = sep,
	Pages = {L49-L52},
	Title = {{On the Spin History of the X-Ray Pulsar in Kes 73: Further Evidence for an Ultramagnetized Neutron Star}},
	Volume = 522,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312220}}

@article{gotthelf00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542L..37G},
	Author = {{Gotthelf}, E.~V. and {Vasisht}, G. and {Boylan-Kolchin}, M. and {Torii}, K.},
	Doi = {10.1086/312923},
	Eprint = {arXiv:astro-ph/0008097},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: PSR J1846-0258, Stars: Individual: Alphanumeric: AX J184624.5-025828, Stars: Neutron, Stars: Supernovae: Individual: Name: Kesteven 75, X-Rays: General},
	Month = oct,
	Pages = {L37-L40},
	Title = {{A 700 Year-old Pulsar in the Supernova Remnant Kesteven 75}},
	Volume = 542,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312923}}

@article{gotthelf02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...567L.125G&db_key=AST},
	Author = {{Gotthelf}, E.~V. and {Halpern}, J.~P. and {Dodson}, R.},
	Doi = {10.1086/340109},
	Eprint = {astro-ph/0201161},
	Journal = {\apjl},
	Month = mar,
	Pages = {L125-L128},
	Title = {{Detection of Pulsed X-Ray Emission from PSR B1706-44}},
	Volume = 567,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340109}}

@article{gotthelf03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003ApJ...591..361G&db_key=AST},
	Author = {{Gotthelf}, E.~V.},
	Doi = {10.1086/375124},
	Eprint = {astro-ph/0303155},
	Journal = {\apj},
	Month = jul,
	Pages = {361-365},
	Title = {{X-Ray Spectra of Young Pulsars and Their Wind Nebulae: Dependence on Spin-Down Energy Loss Rate}},
	Volume = 591,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375124}}

@article{gotthelf04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...605..368G&db_key=AST},
	Author = {{Gotthelf}, E.~V. and {Halpern}, J.~P. and {Buxton}, M. and {Bailyn}, C.},
	Doi = {10.1086/382232},
	Eprint = {astro-ph/0309745},
	Journal = {\apj},
	Month = apr,
	Pages = {368-377},
	Title = {{Imaging X-Ray, Optical, and Infrared Observations of the Transient Anomalous X-Ray Pulsar XTE J1810-197}},
	Volume = 605,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/382232}}

@article{ghs05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...627..390G},
	Author = {{Gotthelf}, E.~V. and {Halpern}, J.~P. and {Seward}, F.~D.},
	Doi = {10.1086/430300},
	Eprint = {arXiv:astro-ph/0503424},
	Journal = {\apj},
	Month = jul,
	Pages = {390-396},
	Title = {{Discovery of a 105 ms X-Ray Pulsar in Kesteven 79: On the Nature of Compact Central Objects in Supernova Remnants}},
	Volume = 627,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430300}}

@article{gotthelf07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...664L..35G},
	Author = {{Gotthelf}, E.~V. and {Halpern}, J.~P.},
	Doi = {10.1086/520637},
	Eprint = {arXiv:0704.2255},
	Journal = {\apjl},
	Month = jul,
	Pages = {L35-L38},
	Title = {{Precise Timing of the X-ray Pulsar 1E 1207.4-5209: A Steady Neutron Star Weakly Magnetized at Birth}},
	Volume = 664,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/520637}}

@article{gh07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.308...79G},
	Author = {{Gotthelf}, E.~V. and {Halpern}, J.~P.},
	Doi = {10.1007/s10509-007-9327-9},
	Eprint = {arXiv:astro-ph/0608473},
	Journal = {\apss},
	Month = apr,
	Pages = {79-87},
	Title = {{The anatomy of a magnetar: XMM monitoring of the transient anomalous X-ray pulsar XTE J1810-197}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9327-9}}

@article{gotthelf10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...724.1316G},
	Archiveprefix = {arXiv},
	Author = {{Gotthelf}, E.~V. and {Perna}, R. and {Halpern}, J.~P.},
	Doi = {10.1088/0004-637X/724/2/1316},
	Eprint = {1009.4473},
	Journal = {\apj},
	Keywords = {pulsars: individual: PSR J0821{\ndash}4300, stars: neutron, X-rays: stars},
	Month = dec,
	Pages = {1316-1324},
	Primaryclass = {astro-ph.HE},
	Title = {{Modeling the Surface X-ray Emission and Viewing Geometry of PSR J0821-4300 in Puppis A}},
	Volume = 724,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/724/2/1316}}

@article{gotz04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004A%26A...417L..45G&db_key=AST},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S. and {Mirabel}, I.~F. and {Hurley}, K.},
	Doi = {10.1051/0004-6361:20040080},
	Eprint = {astro-ph/0403018},
	Journal = {\aap},
	Month = apr,
	Pages = {L45-L48},
	Title = {{Spectral evolution of weak bursts from SGR 1806-20 observed with INTEGRAL}},
	Volume = 417,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20040080}}

@article{gotz04_gcn,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2764....1G&db_key=AST},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S. and {Mirabel}, F.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Bursts from Sgr 1806-20: preliminary INTEGRAL results.}},
	Volume = 2764,
	Year = 2004}

@article{gmm06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2006A%26A...445..313G&db_key=AST},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S. and {Molkov}, S. and {Hurley}, K. and {Mirabel}, I.~F. and {Sunyaev}, R. and {Weidenspointner}, G. and {Brandt}, S. and {del Santo}, M. and {Feroci}, M. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {von Kienlin}, A. and {van der Klis}, M. and {Kouveliotou}, C. and {Lund}, N. and {Pizzichini}, G. and {Ubertini}, P. and {Winkler}, C. and {Woods}, P.~M.},
	Doi = {10.1051/0004-6361:20053648},
	Journal = {\aap},
	Month = jan,
	Pages = {313-321},
	Title = {{Two years of INTEGRAL monitoring of the soft gamma-ray repeater SGR 1806-20: from quiescence to frenzy}},
	Volume = 445,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053648}}

@article{gotz06_gcn,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006GCN..5490....1G},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S.},
	Journal = {GCN Circ. 5490},
	Title = {{Two bright bursts from Sgr 1806-20 detected with IBAS.}},
	Year = 2006}

@article{gotz07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007Ap%26SS.308...51G},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S. and {Hurley}, K.},
	Doi = {10.1007/s10509-007-9379-x},
	Eprint = {arXiv:astro-ph/0609404},
	Journal = {\apss},
	Month = apr,
	Pages = {51-59},
	Title = {{Unveiling soft gamma-ray repeaters with INTEGRAL}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9379-x}}

@article{gri07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...475..317G},
	Author = {{G{\"o}tz}, D. and {Rea}, N. and {Israel}, G.~L. and {Zane}, S. and {Esposito}, P. and {Gotthelf}, E.~V. and {Mereghetti}, S. and {Tiengo}, A. and {Turolla}, R.},
	Doi = {10.1051/0004-6361:20078291},
	Eprint = {arXiv:0709.3712},
	Journal = {\aap},
	Month = nov,
	Pages = {317-321},
	Title = {{Long term hard X-ray variability of the anomalous X-ray pulsar 1RXS J170849.0-400910 discovered with INTEGRAL}},
	Volume = 475,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078291}}

@inproceedings{gotz08aip,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007arXiv0710.5822G},
	Author = {{G{\"o}tz}, D. and {Mereghetti}, S. and {Hurley}, K. and {Esposito}, P. and {Gotthelf}, E.~V. and {Israel}, G.~L. and {Rea}, N. and {Tiengo}, A. and {Turolla}, R. and {Zane}, S.},
	Booktitle = {{Bassa} C., {Wang} Z., {Cumming} A., {Kaspi} V.~M., eds., 40 years of pulsars: Millisecond Pulsars, Magnetars and More.},
	Month = feb,
	Pages = {289},
	Series = {AIP Conference Proceedings, Melville NY},
	Title = {{Hard X-ray variability of Magnetar's Tails observed with INTEGRAL}},
	Volume = 983,
	Year = 2008}

@article{gotz08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008arXiv0801.2465G},
	Author = {{G{\"o}tz}, D.},
	Eprint = {0801.2465},
	Journal = {Mem. S.A.It., in press [arXiv: astro-ph/0801.2465]},
	Month = jan,
	Title = {{Hard X-ray Emission from Magnetars : A Case Study for Simbol X}},
	Year = 2008}

@article{gotz13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.3550G},
	Archiveprefix = {arXiv},
	Author = {{G{\"o}tz}, D. and {Covino}, S. and {Fern{\'a}ndez-Soto}, A. and {Laurent}, P. and {Bo{\v s}njak}, {\v Z}.},
	Doi = {10.1093/mnras/stt439},
	Eprint = {1303.4186},
	Journal = {\mnras},
	Keywords = {gravitation, polarization, gamma-ray burst: general, gamma-ray burst: individual: GRB 061122, galaxies: photometry},
	Month = jun,
	Pages = {3550-3556},
	Primaryclass = {astro-ph.HE},
	Title = {{The polarized gamma-ray burst GRB 061122}},
	Volume = 431,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt439}}
	
@ARTICLE{gourgouliatos15,
   author = {{Gourgouliatos}, K.~N. and {Cumming}, A.},
    title = "{Hall drift and the braking indices of young pulsars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1406.3640},
 primaryClass = "astro-ph.SR",
 keywords = {MHD, methods: analytical, methods: numerical, stars: neutron},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {1121-1128},
      doi = {10.1093/mnras/stu2140},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.1121G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{granot04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...609L..17G},
	Author = {{Granot}, J. and {M{\'e}sz{\'a}ros}, P.},
	Doi = {10.1086/422637},
	Eprint = {arXiv:astro-ph/0403260},
	Journal = {\apjl},
	Month = jul,
	Pages = {L17-L20},
	Title = {{High-Energy Emission from the Double Pulsar System J0737-3039}},
	Volume = 609,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422637}}

@ARTICLE{granot06,
   author = {{Granot}, J. and {Ramirez-Ruiz}, E. and {Taylor}, G.~B. and 
	{Eichler}, D. and {Lyubarsky}, Y.~E. and {Wijers}, R.~A.~M.~J. and 
	{Gaensler}, B.~M. and {Gelfand}, J.~D. and {Kouveliotou}, C.
	},
    title = "{Diagnosing the Outflow from the SGR 1806-20 Giant Flare with Radio Observations}",
  journal = {\apj},
   eprint = {astro-ph/0503251},
 keywords = {Hydrodynamics, ISM: Bubbles, Stars: Pulsars: Individual: Alphanumeric: SGR 1806-20, Stars: Flare, Stars: Neutron, Stars: Winds, Outflows},
     year = 2006,
    month = feb,
   volume = 638,
    pages = {391-396},
      doi = {10.1086/497680},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...638..391G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{graves05,
   author = {{Graves}, G.~J.~M. and {Challis}, P.~M. and {Chevalier}, R.~A. and 
	{Crotts}, A. and {Filippenko}, A.~V. and {Fransson}, C. and 
	{Garnavich}, P. and {Kirshner}, R.~P. and {Li}, W. and {Lundqvist}, P. and 
	{McCray}, R. and {Panagia}, N. and {Phillips}, M.~M. and {Pun}, C.~J.~S. and 
	{Schmidt}, B.~P. and {Sonneborn}, G. and {Suntzeff}, N.~B. and 
	{Wang}, L. and {Wheeler}, J.~C.},
    title = "{Limits from the Hubble Space Telescope on a Point Source in SN 1987A}",
  journal = {\apj},
   eprint = {astro-ph/0505066},
 keywords = {Accretion, Accretion Disks, Stars: Neutron, Stars: Supernovae: Individual: Alphanumeric: SN 1987A},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {944-959},
      doi = {10.1086/431422},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..944G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@incollection{gray09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ssc..book.....G},
	Author = {{Gray}, R.~O. and {Corbally}, J., C.},
	Booktitle = {Princeton Series in Astrophysics},
	Editor = {David N. Spergel},
	Publisher = {Princeton University Press},
	Series = {Stellar Spectral Classification},
	Year = 2009}

@ARTICLE{grebenev12,
   author = {{Grebenev}, S.~A. and {Lutovinov}, A.~A. and {Tsygankov}, S.~S. and 
	{Winkler}, C.},
    title = "{Hard-X-ray emission lines from the decay of $^{44}$Ti in the remnant of supernova 1987A}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1211.2656},
 primaryClass = "astro-ph.HE",
     year = 2012,
    month = oct,
   volume = 490,
    pages = {373-375},
      doi = {10.1038/nature11473},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.490..373G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{green09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009BASI...37...45G},
	Archiveprefix = {arXiv},
	Author = {{Green}, D.~A.},
	Eprint = {0905.3699},
	Journal = {Bulletin of the Astronomical Society of India},
	Keywords = {supernova remnants, catalogues, radio continuum: ISM, ISM: general},
	Month = mar,
	Pages = {45},
	Title = {{A revised Galactic supernova remnant catalogue}},
	Volume = 37,
	Year = 2009}

@article{gregory78,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978Natur.272..704G&db_key=AST},
	Author = {{Gregory}, P.~C. and {Taylor}, A.~R.},
	Journal = {\nat},
	Month = apr,
	Pages = {704-706},
	Title = {{New highly variable radio source, possible counterpart of gamma-ray source CG135+1}},
	Volume = 272,
	Year = 1978}

@article{gregory99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999ApJ...520..361G&db_key=AST},
	Author = {{Gregory}, P.~C.},
	Doi = {10.1086/307433},
	Journal = {\apj},
	Month = jul,
	Pages = {361-375},
	Title = {{Bayesian Periodic Signal Detection. I. Analysis of 20 Years of Radio Flux Measurements of the X-Ray Binary LS I +61 deg303}},
	Volume = 520,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307433}}

@article{gpt99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999ApJ...520..376G&db_key=AST},
	Author = {{Gregory}, P.~C. and {Peracaula}, M. and {Taylor}, A.~R.},
	Doi = {10.1086/307432},
	Journal = {\apj},
	Month = jul,
	Pages = {376-390},
	Title = {{Bayesian Periodic Signal Detection. II. Discovery of Periodic Phase Modulation in LS I +61 deg303 Radio Outbursts}},
	Volume = 520,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307432}}

@article{gregory02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...575..427G&db_key=AST},
	Author = {{Gregory}, P.~C.},
	Doi = {10.1086/341257},
	Journal = {\apj},
	Month = aug,
	Pages = {427-434},
	Title = {{Bayesian Analysis of Radio Observations of the Be X-Ray Binary LS I +61{\deg}303}},
	Volume = 575,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/341257}}

@article{greiner01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001A%26A...375..145G&db_key=AST},
	Author = {{Greiner}, J. and {Rau}, A.},
	Doi = {10.1051/0004-6361:20010826},
	Eprint = {astro-ph/0105304},
	Journal = {\aap},
	Month = aug,
	Pages = {145-148},
	Title = {{The X-ray spectrum of LSI+61{\deg} 303}},
	Volume = 375,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20010826}}

@article{greisen66,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1966PhRvL..16..748G&db_key=PHY},
	Author = {{Greisen}, K.},
	Journal = {Physical Review Letters},
	Month = apr,
	Pages = {748-750},
	Title = {{End to the Cosmic-Ray Spectrum?}},
	Volume = 16,
	Year = 1966}

@article{grimm03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339..793G},
	Author = {{Grimm}, H.-J. and {Gilfanov}, M. and {Sunyaev}, R.},
	Doi = {10.1046/j.1365-8711.2003.06224.x},
	Eprint = {arXiv:astro-ph/0205371},
	Journal = {\mnras},
	Keywords = {galaxies: starburst, X-rays: binaries, X-rays: galaxies},
	Month = mar,
	Pages = {793-809},
	Title = {{High-mass X-ray binaries as a star formation rate indicator in distant galaxies}},
	Volume = 339,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06224.x}}

@article{grindlay76,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...205L.127G},
	Author = {{Grindlay}, J. and {Gursky}, H. and {Schnopper}, H. and {Parsignault}, D.~R. and {Heise}, J. and {Brinkman}, A.~C. and {Schrijver}, J.},
	Doi = {10.1086/182105},
	Journal = {\apjl},
	Keywords = {BLACK HOLES (ASTRONOMY), GLOBULAR CLUSTERS, SATELLITE OBSERVATION, X RAY SOURCES, ASTRONOMICAL MODELS, ASTRONOMICAL NETHERLANDS SATELLITE, COSMIC RAYS, ENERGY SPECTRA, RADIANT FLUX DENSITY, SPACEBORNE ASTRONOMY},
	Month = may,
	Pages = {L127-L130},
	Title = {{Discovery of intense X-ray bursts from the globular cluster NGC 6624}},
	Volume = 205,
	Year = 1976,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/182105}}

@article{grindlay01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001Sci...292.2290G},
	Author = {{Grindlay}, J.~E. and {Heinke}, C. and {Edmonds}, P.~D. and {Murray}, S.~S.},
	Doi = {10.1126/science.1061135},
	Eprint = {astro-ph/0105528},
	Journal = {Science},
	Month = jun,
	Pages = {2290-2295},
	Title = {{High-Resolution X-ray Imaging of a Globular Cluster Core: Compact Binaries in 47Tuc}},
	Volume = 292,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1061135}}

@article{groth75,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1975ApJS...29..285G},
	Author = {{Groth}, E.~J.},
	Journal = {\apjs},
	Month = jun,
	Pages = {285-302},
	Title = {{Probability distributions related to power spectra.}},
	Volume = 29,
	Year = 1975}

@article{gruber99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...520..124G&db_key=AST},
	Author = {{Gruber}, D.~E. and {Matteson}, J.~L. and {Peterson}, L.~E. and {Jung}, G.~V.},
	Doi = {10.1086/307450},
	Eprint = {astro-ph/9903492},
	Journal = {\apj},
	Month = jul,
	Pages = {124-129},
	Title = {{The Spectrum of Diffuse Cosmic Hard X-Rays Measured with HEAO 1}},
	Volume = 520,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307450}}

@article{gruendl93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...413L..81G},
	Author = {{Gruendl}, R.~A. and {Vogel}, S.~N. and {Davis}, D.~S. and {Mulchaey}, J.~S.},
	Doi = {10.1086/186964},
	Journal = {\apjl},
	Keywords = {H Alpha Line, Interacting Galaxies, Rosat Mission, Spiral Galaxies, X Ray Astronomy, Fabry-Perot Interferometers, Intergalactic Media, Velocity Distribution},
	Month = aug,
	Pages = {L81-L84},
	Title = {{Interaction of NGC 2276 with the NGC 2300 group - Fabry-Perot observations of the H-alpha velocity field}},
	Volume = 413,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/186964}}

@article{grundstrom07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...656..437G},
	Author = {{Grundstrom}, E.~D. and {Caballero-Nieves}, S.~M. and {Gies}, D.~R. and {Huang}, W. and {McSwain}, M.~V. and {Rafter}, S.~E. and {Riddle}, R.~L. and {Williams}, S.~J. and {Wingert}, D.~W.},
	Doi = {10.1086/510509},
	Eprint = {arXiv:astro-ph/0610608},
	Journal = {\apj},
	Month = feb,
	Pages = {437-443},
	Title = {{Joint H{$\alpha$} and X-Ray Observations of Massive X-Ray Binaries. II. The Be X-Ray Binary and Microquasar LS I +61 303}},
	Volume = 656,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/510509}}

@article{guainazzi99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.310...10G},
	Author = {{Guainazzi}, M. and {Matt}, G. and {Antonelli}, L.~A. and {Bassani}, L. and {Fabian}, A.~C. and {Maiolino}, R. and {Marconi}, A. and {Fiore}, F. and {Iwasawa}, K. and {Piro}, L.},
	Doi = {10.1046/j.1365-8711.1999.02803.x},
	Eprint = {astro-ph/9905261},
	Journal = {\mnras},
	Keywords = {LINE: FORMATION, GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: NGC 1068, GALAXIES: INDIVIDUAL: CIRCINUS GALAXY, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	Month = nov,
	Pages = {10-20},
	Title = {{Soft X-ray spectroscopy of Compton-thick Seyfert 2 galaxies with BeppoSAX}},
	Volume = 310,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1999.02803.x}}

@article{gualandris05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618..845G},
	Author = {{Gualandris}, A. and {Colpi}, M. and {Portegies Zwart}, S. and {Possenti}, A.},
	Doi = {10.1086/426126},
	Eprint = {arXiv:astro-ph/0407502},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Close, Black Hole Physics, Stars: Individual: Alphanumeric: XTE J1118+480, X-Rays: Binaries},
	Month = jan,
	Pages = {845-851},
	Title = {{Has the Black Hole in XTE J1118+480 Experienced an Asymmetric Natal Kick?}},
	Volume = 618,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426126}}

@article{guerrero08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..177..216G},
	Archiveprefix = {arXiv},
	Author = {{Guerrero}, M.~A. and {Chu}, Y.-H.},
	Doi = {10.1086/587059},
	Eprint = {0802.0503},
	Journal = {\apjs},
	Keywords = {Galaxies: Magellanic Clouds, Stars: Wolf-Rayet, Surveys, X-Rays: Stars},
	Month = jul,
	Pages = {216-237},
	Title = {{An X-Ray Survey of Wolf-Rayet Stars in the Magellanic Clouds. I. The Chandra ACIS Data Set}},
	Volume = 177,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587059}}

@article{guidorzi01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001GCN..1041....1G&db_key=AST},
	Author = {{Guidorzi}, C. and {Montanari}, E. and {Frontera}, F. and {Costa}, E. and {Gandolfi}, G. and {Feroci}, M. and {Piro}, L. and {Amati}, L. and {in't Zand}, J.~J.~M. and {D'Andreta}, G. and {Kaptein}, R. and {Reboa}, L.},
	Journal = {GCN Circ. 1041},
	Title = {{Giant flare from SGR1900+14.}},
	Year = 2001}

@article{guidorzi04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004A%26A...416..297G&db_key=AST},
	Author = {{Guidorzi}, C. and {Frontera}, F. and {Montanari}, E. and {Feroci}, M. and {Amati}, L. and {Costa}, E. and {Orlandini}, M.},
	Journal = {\aap},
	Month = mar,
	Pages = {297-310},
	Title = {{Comparative study of the two large flares from SGR1900+14 with the BeppoSAX Gamma-Ray Burst Monitor}},
	Volume = 416,
	Year = 2004}
	
@ARTICLE{guillochon13,
       author = {{Guillochon}, James and {Ramirez-Ruiz}, Enrico},
        title = "{Hydrodynamical Simulations to Determine the Feeding Rate of Black Holes by the Tidal Disruption of Stars: The Importance of the Impact Parameter and Stellar Structure}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, gravitation, hydrodynamics, methods: numerical, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {25},
        pages = {25},
          doi = {10.1088/0004-637X/767/1/25},
archivePrefix = {arXiv},
       eprint = {1206.2350},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...25G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guillon14,
   author = {{Gull{\'o}n}, M. and {Miralles}, J.~A. and {Vigan{\`o}}, D. and 
	{Pons}, J.~A.},
    title = "{Population synthesis of isolated neutron stars with magneto-rotational evolution}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1406.6794},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetic field, stars: neutron, pulsars: general},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {1891-1899},
      doi = {10.1093/mnras/stu1253},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.1891G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guillon15,
   author = {{Gull{\'o}n}, M. and {Pons}, J.~A. and {Miralles}, J.~A. and 
	{Vigan{\`o}}, D. and {Rea}, N. and {Perna}, R.},
    title = "{Population synthesis of isolated neutron stars with magneto-rotational evolution - II. From radio-pulsars to magnetars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1507.05452},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetic field, stars: neutron, pulsars: general},
     year = 2015,
    month = nov,
   volume = 454,
    pages = {615-625},
      doi = {10.1093/mnras/stv1644},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.454..615G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{guver07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...667L..73G},
	Archiveprefix = {arXiv},
	Author = {{G{\"u}ver}, T. and {{\"O}zel}, F. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C.},
	Doi = {10.1086/522047},
	Eprint = {0705.3713},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: General, Stars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron, X-Rays: Stars},
	Month = sep,
	Pages = {L73-L76},
	Title = {{The Magnetar Nature and the Outburst Mechanism of a Transient Anomalous X-Ray Pulsar}},
	Volume = 667,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/522047}}

@article{guver11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418.2773G},
	Archiveprefix = {arXiv},
	Author = {{G{\"u}ver}, T. and {G{\"o}{\v g}{\"u}{\c s}}, E. and {{\"O}zel}, F.},
	Doi = {10.1111/j.1365-2966.2011.19677.x},
	Eprint = {1103.3024},
	Journal = {\mnras},
	Keywords = {stars: magnetars, stars: neutron, X-rays: individual: SGR 0418+5729},
	Month = dec,
	Pages = {2773-2778},
	Primaryclass = {astro-ph.HE},
	Title = {{A magnetar strength surface magnetic field for the slowly spinning down SGR 0418+5729}},
	Volume = 418,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19677.x}}

@article{haberl91,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...252..272H},
	Author = {{Haberl}, F.},
	Journal = {\aap},
	Keywords = {Stellar Winds, Supergiant Stars, X Ray Binaries, X Ray Scattering, X Ray Spectroscopy, Early Stars, Monte Carlo Method, Neutron Stars, Thomson Scattering},
	Month = dec,
	Pages = {272-277},
	Title = {{Scattering of X-rays on the winds of supergiant X-ray binaries}},
	Volume = 252,
	Year = 1991}

@article{haberl08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...485..177H},
	Archiveprefix = {arXiv},
	Author = {{Haberl}, F. and {Eger}, P. and {Pietsch}, W. and {Corbet}, R.~H.~D. and {Sasaki}, M.},
	Doi = {10.1051/0004-6361:200809540},
	Eprint = {0803.2473},
	Journal = {\aap},
	Keywords = {galaxies: individual: small Magellanic Cloud, galaxy: stellar content, stars: emission-line, Be, stars: neutron, X-rays: binaries},
	Month = jul,
	Pages = {177-181},
	Title = {{XMM-Newton observations of the Small Magellanic Cloud: XMMU J004814.1-731003, a 25.55 s Be/X-ray binary pulsar}},
	Volume = 485,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200809540}}

@article{hep08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...489..327H},
	Archiveprefix = {arXiv},
	Author = {{Haberl}, F. and {Eger}, P. and {Pietsch}, W.},
	Doi = {10.1051/0004-6361:200810100},
	Eprint = {0806.4132},
	Journal = {\aap},
	Keywords = {galaxies: individual: Small Magellanic Cloud, galaxies: stellar content, stars: emission-line, Be, stars: neutron, X-rays: binaries},
	Month = oct,
	Pages = {327-348},
	Title = {{XMM-Newton observations of the Small Magellanic Cloud: Be/X-ray binary pulsars active between October 2006 and June 2007}},
	Volume = 489,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810100}}

@ARTICLE{haberl12,
   author = {{Haberl}, F. and {Sturm}, R. and {Filipovi{\'c}}, M.~D. and 
	{Pietsch}, W. and {Crawford}, E.~J.},
    title = "{SXP 1062, a young Be X-ray binary pulsar with long spin period. Implications for the neutron star birth spin}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.0491},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, X-rays: binaries, Magellanic Clouds, stars: emission-line, Be},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {L1},
    pages = {L1},
      doi = {10.1051/0004-6361/201118369},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537L...1H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hailey95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...455L.151H},
	Author = {{Hailey}, C.~J. and {Craig}, W.~W.},
	Doi = {10.1086/309825},
	Journal = {\apjl},
	Month = dec,
	Pages = {L151},
	Title = {{Discovery of a Candidate Isolated Neutron Star in a New Supernova Remnant near CTB 1}},
	Volume = 455,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/309825}}

@article{hakala03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.343L..10H},
	Author = {{Hakala}, P. and {Ramsay}, G. and {Wu}, K. and {Hjalmarsdotter}, L. and {J{\"a}rvinen}, S. and {J{\"a}rvinen}, A. and {Cropper}, M.},
	Doi = {10.1046/j.1365-8711.2003.06830.x},
	Eprint = {arXiv:astro-ph/0305283},
	Journal = {\mnras},
	Keywords = {binaries: general, stars: individual: RX J0806+15, stars: neutron, novae, cataclysmic variables},
	Month = jul,
	Pages = {L10-L14},
	Title = {{Spin up in RX J0806+15: the shortest period binary}},
	Volume = 343,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06830.x}}

@article{hakala04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353..453H},
	Author = {{Hakala}, P. and {Ramsay}, G. and {Byckling}, K.},
	Doi = {10.1111/j.1365-2966.2004.08074.x},
	Journal = {\mnras},
	Keywords = {binaries: close, stars: individual: RX J0806+15, stars: neutron, novae, cataclysmic variables},
	Month = sep,
	Pages = {453-456},
	Title = {{Monitoring the spin up in RX J0806+15}},
	Volume = 353,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08074.x}}

@article{halpern05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...618..874H&db_key=AST},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V.},
	Doi = {10.1086/426130},
	Journal = {\apj},
	Month = jan,
	Pages = {874-882},
	Title = {{The Fading of Transient Anomalous X-Ray Pulsar XTE J1810-197}},
	Volume = 618,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426130}}

@article{hgb05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...632L..29H},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V. and {Becker}, R.~H. and {Helfand}, D.~J. and {White}, R.~L.},
	Doi = {10.1086/497537},
	Eprint = {arXiv:astro-ph/0508534},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: XTE J1810-197, pulsars: individual (AX J1844.8-0256), Radio Continuum: Stars, X-Rays: Stars},
	Month = oct,
	Pages = {L29-L32},
	Title = {{Discovery of Radio Emission from the Transient Anomalous X-Ray Pulsar XTE J1810-197}},
	Volume = 632,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/497537}}

@article{halpern07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1304H},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V. and {Camilo}, F. and {Seward}, F.~D.},
	Doi = {10.1086/519557},
	Eprint = {arXiv:0705.0978},
	Journal = {\apj},
	Month = aug,
	Pages = {1304-1310},
	Title = {{X-Ray Timing of PSR J1852+0040 in Kesteven 79: Evidence of Neutron Stars Weakly Magnetized at Birth}},
	Volume = 665,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/519557}}

@article{halpern08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...676.1178H},
	Archiveprefix = {arXiv},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V. and {Reynolds}, J. and {Ransom}, S.~M. and {Camilo}, F.},
	Doi = {10.1086/527293},
	Eprint = {0711.3780},
	Journal = {\apj},
	Keywords = {ISM: individual (G327.24-0.13), pulsars: individual (1E 1547.0-5408), pulsars: individual (PSR J1550-5418), Stars: Pulsars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron},
	Month = apr,
	Pages = {1178-1183},
	Title = {{Outburst of the 2 s Anomalous X-Ray Pulsar 1E 1547.0-5408}},
	Volume = 676,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/527293}}

@article{halpern09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0912.4985H},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V.},
	Journal = {\apj, in press, preprint (arXiv:astro-ph/0912.4985)},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = dec,
	Title = {{Two Magnetar Candidates in HESS Supernova Remnants}},
	Year = 2009}

@article{hg10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...709..436H},
	Archiveprefix = {arXiv},
	Author = {{Halpern}, J.~P. and {Gotthelf}, E.~V.},
	Doi = {10.1088/0004-637X/709/1/436},
	Eprint = {0911.0093},
	Journal = {\apj},
	Keywords = {ISM: individual objects: Kes 79, pulsars: individual: PSR J0821-4300 1E 1207.4-5209 PSR J1852+0040, stars: neutron},
	Month = jan,
	Pages = {436-446},
	Primaryclass = {astro-ph.HE},
	Title = {{Spin-Down Measurement of PSR J1852+0040 in Kesteven 79: Central Compact Objects as Anti-Magnetars}},
	Volume = 709,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/709/1/436}}

@article{halpern11,
	Author = {{Halpern},J.~P.},
	Journal = {GCN Circ.},
	Title = {{Swift J1822.3-1606: Transient Magnetar or Be X-ray Binary?}},
	Volume = 12170,
	Year = 2011}

@article{halpern12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.4240....1H},
	Author = {{Halpern}, J.~P.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Gamma Ray, Neutron Star, Pulsar},
	Month = jul,
	Title = {{Discovery of 46.6 s X-ray Pulsations from the Candidate for IGR J22534+6243}},
	Volume = 4240,
	Year = 2012}

@article{hambly08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.384..637H},
	Archiveprefix = {arXiv},
	Author = {{Hambly}, N.~C. and {Collins}, R.~S. and {Cross}, N.~J.~G. and {Mann}, R.~G. and {Read}, M.~A. and {Sutorius}, E.~T.~W. and {Bond}, I. and {Bryant}, J. and {Emerson}, J.~P. and {Lawrence}, A. and {Rimoldini}, L. and {Stewart}, J.~M. and {Williams}, P.~M. and {Adamson}, A. and {Hirst}, P. and {Dye}, S. and {Warren}, S.~J.},
	Doi = {10.1111/j.1365-2966.2007.12700.x},
	Eprint = {0711.3593},
	Journal = {\mnras},
	Keywords = {astronomical data bases: miscellaneous , surveys , stars: general , galaxies: general , cosmology: observations , infrared: general},
	Month = feb,
	Pages = {637-662},
	Title = {{The WFCAM Science Archive}},
	Volume = 384,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12700.x}}

@article{hamuy92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992PASP..104..533H},
	Author = {{Hamuy}, M. and {Walker}, A.~R. and {Suntzeff}, N.~B. and {Gigoux}, P. and {Heathcote}, S.~R. and {Phillips}, M.~M.},
	Doi = {10.1086/133028},
	Journal = {\pasp},
	Keywords = {ASTROMETRY, ASTRONOMICAL PHOTOMETRY, ASTRONOMICAL SPECTROSCOPY, SOUTHERN SKY, STELLAR SPECTROPHOTOMETRY, CALIBRATING, CHARGE COUPLED DEVICES, SPECTRAL BANDS, SPECTRAL ENERGY DISTRIBUTION, SPECTROGRAPHS, STELLAR MAGNITUDE},
	Month = jul,
	Pages = {533-552},
	Title = {{Southern spectrophotometric standards.}},
	Volume = 104,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133028}}

@article{hamuy94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994PASP..106..566H},
	Author = {{Hamuy}, M. and {Suntzeff}, N.~B. and {Heathcote}, S.~R. and {Walker}, A.~R. and {Gigoux}, P. and {Phillips}, M.~M.},
	Doi = {10.1086/133417},
	Journal = {\pasp},
	Keywords = {ASTRONOMICAL PHOTOMETRY, CALIBRATING, FLUX DENSITY, INFRARED SPECTRA, SOUTHERN HEMISPHERE, SPECTROPHOTOMETRY, VISIBLE SPECTRUM, CHARGE COUPLED DEVICES, COMPUTATIONAL GRIDS, DATA REDUCTION, NORTHERN HEMISPHERE, SPECTRAL ENERGY DISTRIBUTION, SPECTROGRAPHS, STELLAR MAGNITUDE, TELESCOPES, ULTRAVIOLET SPECTRA},
	Month = jun,
	Pages = {566-589},
	Title = {{Southern spectrophotometric standards, 2}},
	Volume = 106,
	Year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133417}}

@article{hannikainen03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003IAUC.8088....4H},
	Author = {{Hannikainen}, D.~C. and {Rodriguez}, J. and {Pottschmidt}, K.},
	Journal = {\iaucirc},
	Month = mar,
	Title = {{Igr J19140+098}},
	Volume = 8088,
	Year = 2003}

@article{hanuschik96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...308..170H},
	Author = {{Hanuschik}, R.~W.},
	Journal = {\aap},
	Keywords = {LINE: PROFILES, STARS: BE, CIRCUMSTELLAR MATTER},
	Month = apr,
	Pages = {170-179},
	Title = {{On the structure of Be star disks.}},
	Volume = 308,
	Year = 1996}

@article{hhs96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..116..309H},
	Author = {{Hanuschik}, R.~W. and {Hummel}, W. and {Sutorius}, E. and {Dietle}, O. and {Thimm}, G.},
	Journal = {\aaps},
	Keywords = {ATLAS, STARS: BE, LINES: PROFILES},
	Month = apr,
	Pages = {309-358},
	Title = {{Atlas of high-resolution emission and shell lines in Be stars. Line profiles and short-term variability.}},
	Volume = 116,
	Year = 1996}

@article{harding02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...576..366H},
	Author = {{Harding}, A.~K. and {Muslimov}, A.~G. and {Zhang}, B.},
	Doi = {10.1086/341633},
	Eprint = {arXiv:astro-ph/0205077},
	Journal = {\apj},
	Month = sep,
	Pages = {366-375},
	Title = {{Regimes of Pulsar Pair Formation and Particle Energetics}},
	Volume = 576,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/341633}}

@article{hm02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...568..862H},
	Author = {{Harding}, A.~K. and {Muslimov}, A.~G.},
	Doi = {10.1086/338985},
	Eprint = {arXiv:astro-ph/0112392},
	Journal = {\apj},
	Month = apr,
	Pages = {862-877},
	Title = {{Pulsar Polar Cap Heating and Surface Thermal X-Ray Emission. II. Inverse Compton Radiation Pair Fronts}},
	Volume = 568,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/338985}}

@ARTICLE{harding13,
   author = {{Harding}, A.~K.},
    title = "{The neutron star zoo}",
  journal = {Frontiers of Physics},
archivePrefix = "arXiv",
   eprint = {1302.0869},
 primaryClass = "astro-ph.HE",
 keywords = {stars, neutron stars, pulsars, binary stars},
     year = 2013,
    month = dec,
   volume = 8,
    pages = {679-692},
      doi = {10.1007/s11467-013-0285-0},
   adsurl = {http://adsabs.harvard.edu/abs/2013FrPhy...8..679H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{harris96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1996AJ....112.1487H},
	Author = {{Harris}, W.~E.},
	Doi = {10.1086/118116},
	Journal = {\aj},
	Keywords = {GLOBULAR CLUSTERS: GENERAL, CATALOGS},
	Month = oct,
	Pages = {1487},
	Title = {{A Catalog of Parameters for Globular Clusters in the Milky Way}},
	Volume = 112,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/118116}}

@article{harrison00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000ApJ...528..454H&db_key=AST},
	Author = {{Harrison}, F.~A. and {Ray}, P.~S. and {Leahy}, D.~A. and {Waltman}, E.~B. and {Pooley}, G.~G.},
	Doi = {10.1086/308157},
	Eprint = {astro-ph/9908076},
	Journal = {\apj},
	Month = jan,
	Pages = {454-461},
	Title = {{Simultaneous X-Ray and Radio Monitoring of the Unusual Binary LS I +61 deg303: Measurements of the Light Curve and High-Energy Spectrum}},
	Volume = 528,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308157}}

@article{harrison13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770..103H},
	Archiveprefix = {arXiv},
	Author = {{Harrison}, F.~A. and {Craig}, W.~W. and {Christensen}, F.~E. and {Hailey}, C.~J. and {Zhang}, W.~W. and {Boggs}, S.~E. and {Stern}, D. and {Cook}, W.~R. and {Forster}, K. and {Giommi}, P. and {Grefenstette}, B.~W. and {Kim}, Y. and {Kitaguchi}, T. and {Koglin}, J.~E. and {Madsen}, K.~K. and {Mao}, P.~H. and {Miyasaka}, H. and {Mori}, K. and {Perri}, M. and {Pivovaroff}, M.~J. and {Puccetti}, S. and {Rana}, V.~R. and {Westergaard}, N.~J. and {Willis}, J. and {Zoglauer}, A. and {An}, H. and {Bachetti}, M. and {Barri{\`e}re}, N.~M. and {Bellm}, E.~C. and {Bhalerao}, V. and {Brejnholt}, N.~F. and {Fuerst}, F. and {Liebe}, C.~C. and {Markwardt}, C.~B. and {Nynka}, M. and {Vogel}, J.~K. and {Walton}, D.~J. and {Wik}, D.~R. and {Alexander}, D.~M. and {Cominsky}, L.~R. and {Hornschemeier}, A.~E. and {Hornstrup}, A. and {Kaspi}, V.~M. and {Madejski}, G.~M. and {Matt}, G. and {Molendi}, S. and {Smith}, D.~M. and {Tomsick}, J.~A. and {Ajello}, M. and {Ballantyne}, D.~R. and {Balokovi{\'c}}, M. and {Barret}, D. and {Bauer}, F.~E. and {Blandford}, R.~D. and {Brandt}, W.~N. and {Brenneman}, L.~W. and {Chiang}, J. and {Chakrabarty}, D. and {Chenevez}, J. and {Comastri}, A. and {Dufour}, F. and {Elvis}, M. and {Fabian}, A.~C. and {Farrah}, D. and {Fryer}, C.~L. and {Gotthelf}, E.~V. and {Grindlay}, J.~E. and {Helfand}, D.~J. and {Krivonos}, R. and {Meier}, D.~L. and {Miller}, J.~M. and {Natalucci}, L. and {Ogle}, P. and {Ofek}, E.~O. and {Ptak}, A. and {Reynolds}, S.~P. and {Rigby}, J.~R. and {Tagliaferri}, G. and {Thorsett}, S.~E. and {Treister}, E. and {Urry}, C.~M.},
	Doi = {10.1088/0004-637X/770/2/103},
	Eid = {103},
	Eprint = {1301.7307},
	Journal = {\apj},
	Keywords = {space vehicles: instruments, X-rays: general},
	Month = jun,
	Pages = {103},
	Primaryclass = {astro-ph.IM},
	Title = {{The Nuclear Spectroscopic Telescope Array (NuSTAR) High-energy X-Ray Mission}},
	Volume = 770,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/770/2/103}}

@article{hartman99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999ApJS..123...79H&db_key=AST},
	Author = {{Hartman}, R.~C. and {Bertsch}, D.~L. and {Bloom}, S.~D. and {Chen}, A.~W. and {Deines-Jones}, P. and {Esposito}, J.~A. and {Fichtel}, C.~E. and {Friedlander}, D.~P. and {Hunter}, S.~D. and {McDonald}, L.~M. and {Sreekumar}, P. and {Thompson}, D.~J. and {Jones}, B.~B. and {Lin}, Y.~C. and {Michelson}, P.~F. and {Nolan}, P.~L. and {Tompkins}, W.~F. and {Kanbach}, G. and {Mayer-Hasselwander}, H.~A. and {M{\"u}cke}, A. and {Pohl}, M. and {Reimer}, O. and {Kniffen}, D.~A. and {Schneid}, E.~J. and {von Montigny}, C. and {Mukherjee}, R. and {Dingus}, B.~L.},
	Doi = {10.1086/313231},
	Journal = {\apjs},
	Month = jul,
	Pages = {79-202},
	Title = {{The Third EGRET Catalog of High-Energy Gamma-Ray Sources}},
	Volume = 123,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/313231}}

@article{hartman08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...675.1468H},
	Archiveprefix = {arXiv},
	Author = {{Hartman}, J.~M. and {Patruno}, A. and {Chakrabarty}, D. and {Kaplan}, D.~L. and {Markwardt}, C.~B. and {Morgan}, E.~H. and {Ray}, P.~S. and {van der Klis}, M. and {Wijnands}, R.},
	Doi = {10.1086/527461},
	Eprint = {0708.0211},
	Journal = {\apj},
	Keywords = {stars: individual (SAX J1808.4-3658), Stars: Neutron, X-Rays: Stars},
	Month = mar,
	Pages = {1468-1486},
	Title = {{The Long-Term Evolution of the Spin, Pulse Shape, and Orbit of the Accretion-powered Millisecond Pulsar SAX J1808.4-3658}},
	Volume = 675,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/527461}}

@article{hasinger93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...275....1H},
	Author = {{Hasinger}, G. and {Burg}, R. and {Giacconi}, R. and {Hartner}, G. and {Schmidt}, M. and {Trumper}, J. and {Zamorani}, G.},
	Journal = {\aap},
	Month = aug,
	Pages = {1},
	Title = {{A Deep X-Ray Survey in the Lockman-Hole and the Soft X-Ray N-Log}},
	Volume = 275,
	Year = 1993}

@article{heard13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.3462H},
	Archiveprefix = {arXiv},
	Author = {{Heard}, V. and {Warwick}, R.~S.},
	Doi = {10.1093/mnras/sts284},
	Eprint = {1210.6808},
	Journal = {\mnras},
	Keywords = {Galaxy: centre, X-rays: binaries, X-rays: ISM},
	Month = feb,
	Pages = {3462-3477},
	Primaryclass = {astro-ph.HE},
	Title = {{XMM-Newton observations of the Galactic Centre Region - I. The distribution of low-luminosity X-ray sources}},
	Volume = 428,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts284}}

@ARTICLE{heger05,
   author = {{Heger}, A. and {Woosley}, S.~E. and {Spruit}, H.~C.},
    title = "{Presupernova Evolution of Differentially Rotating Massive Stars Including Magnetic Fields}",
  journal = {\apj},
   eprint = {astro-ph/0409422},
 keywords = {Stars: Pulsars: General, Stars: Evolution, Stars: Magnetic Fields, Stars: Rotation},
     year = 2005,
    month = jun,
   volume = 626,
    pages = {350-363},
      doi = {10.1086/429868},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...626..350H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{heil09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397.1061H},
	Archiveprefix = {arXiv},
	Author = {{Heil}, L.~M. and {Vaughan}, S. and {Roberts}, T.~P.},
	Doi = {10.1111/j.1365-2966.2009.15068.x},
	Eprint = {0905.1265},
	Journal = {\mnras},
	Keywords = {black hole physics , X-rays: binaries , X-rays: galaxies , X-rays: general},
	Month = aug,
	Pages = {1061-1072},
	Primaryclass = {astro-ph.HE},
	Title = {{A systematic study of variability in a sample of ultraluminous X-ray sources}},
	Volume = 397,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15068.x}}

@incollection{heindl04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004AIPC..714..323H},
	Author = {{Heindl}, W.~A. and {Rothschild}, R.~E. and {Coburn}, W. and {Staubert}, R. and {Wilms}, J. and {Kreykenbohm}, I. and {Kretschmar}, P.},
	Booktitle = {X-ray Timing 2003: Rossi and Beyond},
	Doi = {10.1063/1.1781049},
	Editor = {{Kaaret}, P. and {Lamb}, F.~K. and {Swank}, J.~H.},
	Eprint = {arXiv:astro-ph/0403197},
	Keywords = {X-ray, Pulsars, Cyclotrons, Synchrotron radiation},
	Month = jul,
	Pages = {323-330},
	Publisher = {AIP Melville},
	Series = {American Institute of Physics Conference Series},
	Title = {{Timing and Spectroscopy of Accreting X-ray Pulsars: the State of Cyclotron Line Studies}},
	Volume = 714,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.1781049}}

@article{heinke05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...625..796H},
	Author = {{Heinke}, C.~O. and {Grindlay}, J.~E. and {Edmonds}, P.~D. and {Cohn}, H.~N. and {Lugger}, P.~M. and {Camilo}, F. and {Bogdanov}, S. and {Freire}, P.~C.},
	Doi = {10.1086/429899},
	Eprint = {astro-ph/0503132},
	Journal = {\apj},
	Keywords = {Galaxy: Globular Clusters: Individual: NGC Number: NGC 104, Stars: Novae, Cataclysmic Variables, Stars: Pulsars: General, Stars: Neutron, X-Rays: Binaries},
	Month = jun,
	Pages = {796-824},
	Title = {{A Deep Chandra Survey of the Globular Cluster 47 Tucanae: Catalog of Point Sources}},
	Volume = 625,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429899}}

@article{hge05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..556H},
	Author = {{Heinke}, C.~O. and {Grindlay}, J.~E. and {Edmonds}, P.~D.},
	Doi = {10.1086/427795},
	Eprint = {astro-ph/0412137},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Binaries: Eclipsing, Galaxy: Globular Clusters: Individual: NGC Number: NGC 104, Stars: Neutron, X-Rays: Binaries},
	Month = mar,
	Pages = {556-564},
	Title = {{Three Additional Quiescent Low-Mass X-Ray Binary Candidates in 47 Tucanae}},
	Volume = 622,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/427795}}

@ARTICLE{heinz15,
   author = {{Heinz}, S. and {Burton}, M. and {Braiding}, C. and {Brandt}, W.~N. and 
	{Jonker}, P.~G. and {Sell}, P. and {Fender}, R.~P. and {Nowak}, M.~A. and 
	{Schulz}, N.~S.},
    title = "{Lord of the Rings: A Kinematic Distance to Circinus X-1 from a Giant X-Ray Light Echo}",
  journal = {\apj},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, stars: distances, stars: individual: Circinus X-1, stars: neutron, techniques: radial velocities, X-rays: binaries},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {265},
    pages = {265},
      doi = {10.1088/0004-637X/806/2/265},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806..265H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{helfand84,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1984Natur.307..215H},
	Author = {{Helfand}, D.~J. and {Becker}, R.~H.},
	Journal = {\nat},
	Month = jan,
	Pages = {215-221},
	Title = {{Observation of stellar remnants from recent supernovae}},
	Volume = 307,
	Year = 1984}

@article{h84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984PASP...96..913H},
	Author = {{Helfand}, D.~J.},
	Doi = {10.1086/131455},
	Journal = {\pasp},
	Keywords = {GALACTIC CLUSTERS, LOCAL GROUP (ASTRONOMY), STELLAR EVOLUTION, X RAY SOURCES, ASTRONOMICAL SPECTROSCOPY, BINARY STARS, CONSTRAINTS, GALACTIC EVOLUTION, MAGELLANIC CLOUDS, MILKY WAY GALAXY, SUPERNOVA REMNANTS, X RAY BINARIES},
	Month = dec,
	Pages = {913-931},
	Title = {{Endpoints of stellar evolution - X-ray surveys of the Local Group}},
	Volume = 96,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/131455}}

@article{helfand01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...556..380H&db_key=AST},
	Author = {{Helfand}, D.~J. and {Gotthelf}, E.~V. and {Halpern}, J.~P.},
	Doi = {10.1086/321533},
	Eprint = {astro-ph/0007310},
	Journal = {\apj},
	Month = jul,
	Pages = {380-391},
	Title = {{Vela Pulsar and Its Synchrotron Nebula}},
	Volume = 556,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321533}}

@article{helfand03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003ApJ...582..783H&db_key=AST},
	Author = {{Helfand}, D.~J. and {Collins}, B.~F. and {Gotthelf}, E.~V.},
	Doi = {10.1086/344725},
	Eprint = {astro-ph/0209348},
	Journal = {\apj},
	Month = jan,
	Pages = {783-792},
	Title = {{Chandra X-Ray Imaging Spectroscopy of the Young Supernova Remnant Kesteven 75}},
	Volume = 582,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/344725}}

@article{helfand07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662.1198H},
	Author = {{Helfand}, D.~J. and {Chatterjee}, S. and {Brisken}, W.~F. and {Camilo}, F. and {Reynolds}, J. and {van Kerkwijk}, M.~H. and {Halpern}, J.~P. and {Ransom}, S.~M.},
	Doi = {10.1086/518028},
	Eprint = {arXiv:astro-ph/0703336},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General, Stars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron, X-Rays: Stars},
	Month = jun,
	Pages = {1198-1203},
	Title = {{VLBA Measurement of the Transverse Velocity of the Magnetar XTE J1810-197}},
	Volume = 662,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518028}}

@article{hellier94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.271L..21H},
	Author = {{Hellier}, C.},
	Journal = {\mnras},
	Keywords = {X-Ray Pulsars: X-Ray Light Curves, X-Ray Pulsars: X-Ray Binaries},
	Month = nov,
	Pages = {L21-L24},
	Title = {{A ROSAT observation of the X-ray pulsars X0142+614 and X0146+612.}},
	Volume = 271,
	Year = 1994}

@article{hellier97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.291...71H},
	Author = {{Hellier}, C.},
	Eprint = {astro-ph/9708076},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, BINARIES: ECLIPSING, STARS: INDIVIDUAL: XY ARI, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
	Month = oct,
	Pages = {71-80},
	Title = {{The size of the accretion region in intermediate polars: eclipses of XY ARIETIS observed with RXTE}},
	Volume = 291,
	Year = 1997}

@article{hmb97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.292..397H},
	Author = {{Hellier}, C. and {Mukai}, K. and {Beardmore}, A.~P.},
	Eprint = {astro-ph/9708077},
	Journal = {\mnras},
	Keywords = {Magnetic Stars, Cataclysmic Variables, Stellar Radiation, X Ray Spectra, Accretion Disks, Stellar Oscillations, Particle Flux Density, X Ray Telescopes, Particle Spin, Ultraviolet Astronomy, Dwarf Novae},
	Month = dec,
	Pages = {397},
	Title = {{An outburst of the magnetic cataclysmic variable XY ARIETIS observed with RXTE}},
	Volume = 292,
	Year = 1997}

@article{hellier98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.299..851H},
	Author = {{Hellier}, C. and {Beardmore}, A.~P. and {Buckley}, D.~A.~H.},
	Doi = {10.1046/j.1365-8711.1998.01850.x},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, STARS: INDIVIDUAL: RXJ1238-38, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
	Month = sep,
	Pages = {851-854},
	Title = {{X-ray confirmation of the new intermediate polar RXJ1238-38}},
	Volume = 299,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.01850.x}}

@inproceedings{hellier14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014EPJWC..6407001H},
	Archiveprefix = {arXiv},
	Author = {{Hellier}, C.},
	Booktitle = {European Physical Journal Web of Conferences},
	Doi = {10.1051/epjconf/20136407001},
	Eid = {07001},
	Eprint = {1312.4779},
	Month = jan,
	Pages = {7001},
	Primaryclass = {astro-ph.SR},
	Series = {European Physical Journal Web of Conferences},
	Title = {{The Magnetospheric Boundary in Cataclysmic Variables}},
	Volume = 64,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/epjconf/20136407001}}

@ARTICLE{henault12,
   author = {{H{\'e}nault-Brunet}, V. and {Oskinova}, L.~M. and {Guerrero}, M.~A. and 
	{Sun}, W. and {Chu}, Y.-H. and {Evans}, C.~J. and {Gallagher}, III, J.~S. and 
	{Gruendl}, R.~A. and {Reyes-Iturbide}, J.},
    title = "{Discovery of a Be/X-ray pulsar binary and associated supernova remnant in the Wing of the Small Magellanic Cloud}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1110.6404},
 primaryClass = "astro-ph.SR",
 keywords = {stars: emission-line, Be, ISM: supernova remnants, Magellanic Clouds, X-rays: binaries},
     year = 2012,
    month = feb,
   volume = 420,
    pages = {L13-L17},
      doi = {10.1111/j.1745-3933.2011.01183.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420L..13H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hendrick05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622L.117H},
	Author = {{Hendrick}, S.~P. and {Reynolds}, S.~P. and {Borkowski}, K.~J.},
	Doi = {10.1086/429862},
	Journal = {\apjl},
	Keywords = {ISM: Individual: Alphanumeric: B0049-73.6, ISM: Supernova Remnants, X-Rays: ISM},
	Month = apr,
	Pages = {L117-L120},
	Title = {{An Fe-Ni Bubble in the Small Magellanic Cloud Supernova Remnant B0049-73.6}},
	Volume = 622,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429862}}

@article{henze12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.3890....1H},
	Author = {{Henze}, M. and {Pietsch}, W. and {Haberl}, F.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Transient},
	Month = jan,
	Title = {{XMMU J004243.6+412519 - a new X-ray transient in M 31 seen with XMM-Newton}},
	Volume = 3890,
	Year = 2012}

@article{hph12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.3921....1H},
	Author = {{Henze}, M. and {Pietsch}, W. and {Haberl}, F.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Transient},
	Month = feb,
	Title = {{XMMU J004243.6+412519 becomes the second ultraluminous X-ray source in M 31}},
	Volume = 3921,
	Year = 2012}

@article{hepiha12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.3959....1H},
	Author = {{Henze}, M. and {Pietsch}, W. and {Haberl}, F.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Transient},
	Month = mar,
	Title = {{Swift XRT observations of the M 31 ULX XMMU J004243.6+412519}},
	Volume = 3959,
	Year = 2012}

@article{hphg12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.4125....1H},
	Author = {{Henze}, M. and {Pietsch}, W. and {Haberl}, F. and {Greiner}, J.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Transient},
	Month = may,
	Title = {{Swift XRT finds the M 31 ULX XMMU J004243.6+412519 still active after Sun block}},
	Volume = 4125,
	Year = 2012}

@article{hermsen77,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1977Natur.269..494H&db_key=AST},
	Author = {{Hermsen}, W. and {Swanenburg}, B.~N. and {Bignami}, G.~F. and {Boella}, G. and {Buccheri}, R. and {Scarsi}, L. and {Kanbach}, G. and {Mayer-Hasselwander}, H.~A. and {Masnou}, J.~L. and {Paul}, J.~A.},
	Journal = {\nat},
	Month = oct,
	Pages = {494},
	Title = {{New high energy gamma-ray sources observed by COS B}},
	Volume = 269,
	Year = 1977}

@ARTICLE{herold79,
   author = {{Herold}, H.},
    title = "{Compton and Thomson scattering in strong magnetic fields}",
  journal = {\prd},
     year = 1979,
    month = may,
   volume = 19,
    pages = {2868-2875},
      doi = {10.1103/PhysRevD.19.2868},
   adsurl = {http://adsabs.harvard.edu/abs/1979PhRvD..19.2868H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hertz78,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...224..614H},
	Author = {{Hertz}, P. and {Joss}, P.~C. and {Rappaport}, S.},
	Doi = {10.1086/156410},
	Journal = {\apj},
	Keywords = {BINARY STARS, LIGHT CURVE, MONTE CARLO METHOD, RADIATIVE TRANSFER, STELLAR MODELS, X RAY SOURCES, COMPANION STARS, COMPTON EFFECT, GRAPHS (CHARTS), PHOTOIONIZATION, STEADY STATE, STELLAR ENVELOPES, STELLAR OCCULTATION, STELLAR WINDS, X RAY SPECTRA, X RAY STARS},
	Month = sep,
	Pages = {614-624},
	Title = {{X-ray transfer in binary systems - A Monte Carlo study}},
	Volume = 224,
	Year = 1978,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/156410}}

@article{hester02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...577L..49H},
	Author = {{Hester}, J.~J. and {Mori}, K. and {Burrows}, D. and {Gallagher}, J.~S. and {Graham}, J.~R. and {Halverson}, M. and {Kader}, A. and {Michel}, F.~C. and {Scowen}, P.},
	Doi = {10.1086/344132},
	Journal = {\apjl},
	Month = sep,
	Pages = {L49-L52},
	Title = {{Hubble Space Telescope and Chandra Monitoring of the Crab Synchrotron Nebula}},
	Volume = 577,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/344132}}

@article{heyl97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...489L..67H},
	Author = {{Heyl}, J.~S. and {Hernquist}, L.},
	Doi = {10.1086/310964},
	Eprint = {arXiv:astro-ph/9708179},
	Journal = {\apjl},
	Month = nov,
	Pages = {L67+},
	Title = {{Powering Anomalous X-Ray Pulsars by Neutron Star Cooling}},
	Volume = 489,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310964}}

@article{hilditch05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.357..304H},
	Author = {{Hilditch}, R.~W. and {Howarth}, I.~D. and {Harries}, T.~J.},
	Doi = {10.1111/j.1365-2966.2005.08653.x},
	Eprint = {arXiv:astro-ph/0411672},
	Journal = {\mnras},
	Keywords = {binaries: close, binaries: eclipsing, binaries: general, binaries: spectroscopic, Magellanic Clouds},
	Month = feb,
	Pages = {304-324},
	Title = {{Forty eclipsing binaries in the Small Magellanic Cloud: fundamental parameters and Cloud distance}},
	Volume = 357,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.08653.x}}

@inproceedings{hill04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004SPIE.5165..217H},
	Author = {{Hill}, J.~E. and {Burrows}, D.~N. and {Nousek}, J.~A. and {Abbey}, A.~F. and {Ambrosi}, R.~M. and {Br{\"a}uninger}, H.~W. and {Burkert}, W. and {Campana}, S. and {Cheruvu}, C. and {Cusumano}, G. and {Freyberg}, M.~J. and {Hartner}, G.~D. and {Klar}, R. and {Mangels}, C. and {Moretti}, A. and {Mori}, K. and {Morris}, D.~C. and {Short}, A.~D.~T. and {Tagliaferri}, G. and {Watson}, D.~J. and {Wood}, P. and {Wells}, A.~A.},
	Booktitle = {X-Ray and Gamma-Ray Instrumentation for Astronomy XIII.},
	Doi = {10.1117/12.505728},
	Editor = {{Flanagan}, K.~A. and {Siegmund}, O.~H.~W.},
	Month = feb,
	Pages = {217-231},
	Publisher = {SPIE, Bellingham},
	Series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	Title = {{Readout modes and automated operation of the Swift X-ray Telescope}},
	Volume = 5165,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.505728}}

@inproceedings{hillas85,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985ICRC....3..445H&db_key=AST},
	Author = {{Hillas}, A.~M.},
	Booktitle = {International Cosmic Ray Conference},
	Editor = {{Jones}, F.~C.},
	Month = aug,
	Pages = {445-448},
	Title = {{Cerenkov light images of EAS produced by primary gamma}},
	Year = 1985}

@ARTICLE{hillebrandt87,
   author = {{Hillebrandt}, W. and {Hoeflich}, P. and {Weiss}, A. and {Truran}, J.~W.
	},
    title = "{Explosion of a blue supergiant - A model for supernova SN1987A}",
  journal = {\nat},
 keywords = {Blue Stars, Stellar Models, Supergiant Stars, Supernova 1987a, Magellanic Clouds, Spectrum Analysis, Stellar Evolution, Stellar Magnitude, Stellar Temperature},
     year = 1987,
    month = jun,
   volume = 327,
    pages = {597-600},
      doi = {10.1038/327597a0},
   adsurl = {http://adsabs.harvard.edu/abs/1987Natur.327..597H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hinton04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004NewAR..48..331H&db_key=AST},
	Author = {{Hinton}, J.~A.},
	Doi = {10.1016/j.newar.2003.12.004},
	Eprint = {astro-ph/0403052},
	Journal = {New Astronomy Review},
	Month = apr,
	Pages = {331-337},
	Title = {{The status of the HESS project}},
	Volume = 48,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.newar.2003.12.004}}
	
@ARTICLE{hirata87,
   author = {{Hirata}, K. and {Kajita}, T. and {Koshiba}, M. and {Nakahata}, M. and 
	{Oyama}, Y.},
    title = "{Observation of a neutrino burst from the supernova SN1987A}",
  journal = {Physical Review Letters},
 keywords = {Neutrinos, Stellar Radiation, Supernova 1987a, Cerenkov Radiation, Electron Energy, Magellanic Clouds, Radiation Detectors},
     year = 1987,
    month = apr,
   volume = 58,
    pages = {1490-1493},
      doi = {10.1103/PhysRevLett.58.1490},
   adsurl = {http://adsabs.harvard.edu/abs/1987PhRvL..58.1490H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ho01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001MNRAS.327.1081H&db_key=AST},
	Author = {{Ho}, W.~C.~G. and {Lai}, D.},
	Doi = {10.1046/j.1365-8711.2001.04801.x},
	Eprint = {astro-ph/0104199},
	Journal = {\mnras},
	Month = nov,
	Pages = {1081-1096},
	Title = {{Atmospheres and spectra of strongly magnetized neutron stars}},
	Volume = 327,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04801.x}}

@article{ho03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003MNRAS.338..233H&db_key=AST},
	Author = {{Ho}, W.~C.~G. and {Lai}, D.},
	Doi = {10.1046/j.1365-8711.2003.06047.x},
	Eprint = {astro-ph/0201380},
	Journal = {\mnras},
	Month = jan,
	Pages = {233-252},
	Title = {{Atmospheres and spectra of strongly magnetized neutron stars - II. The effect of vacuum polarization}},
	Volume = 338,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06047.x}}

@article{hlp03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...599.1293H},
	Author = {{Ho}, W.~C.~G. and {Lai}, D. and {Potekhin}, A.~Y. and {Chabrier}, G.},
	Doi = {10.1086/379507},
	Eprint = {arXiv:astro-ph/0309261},
	Journal = {\apj},
	Keywords = {Magnetic Fields, Radiative Transfer, Stars: Atmospheres, Stars: Magnetic Fields, Stars: Neutron, X-Rays: Stars},
	Month = dec,
	Pages = {1293-1301},
	Title = {{Atmospheres and Spectra of Strongly Magnetized Neutron Stars. III. Partially Ionized Hydrogen Models}},
	Volume = 599,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379507}}

@article{ho04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607..420H},
	Author = {{Ho}, W.~C.~G. and {Lai}, D.},
	Doi = {10.1086/383341},
	Eprint = {arXiv:astro-ph/0402088},
	Journal = {\apj},
	Keywords = {Magnetic Fields, Stars: Atmospheres, Stars: Magnetic Fields, Stars: Neutron, X-Rays: Stars},
	Month = may,
	Pages = {420-425},
	Title = {{Spectral Features in the Thermal Emission from Isolated Neutron Stars: Dependence on Magnetic Field Strengths}},
	Volume = 607,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/383341}}

@ARTICLE{ho11,
   author = {{Ho}, W.~C.~G.},
    title = "{Evolution of a buried magnetic field in the central compact object neutron stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.4870},
 primaryClass = "astro-ph.HE",
 keywords = {stars: evolution, stars: magnetic field, stars: neutron, pulsars: individual: 1E 1207.4-5209, pulsars: individual: PSR J0821-4300, pulsars: individual: PSR J1852+0040},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2567-2575},
      doi = {10.1111/j.1365-2966.2011.18576.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2567H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}}

@article{hog00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...355L..27H},
	Author = {{H{\o}g}, E. and {Fabricius}, C. and {Makarov}, V.~V. and {Urban}, S. and {Corbin}, T. and {Wycoff}, G. and {Bastian}, U. and {Schwekendiek}, P. and {Wicenec}, A.},
	Journal = {\aap},
	Month = mar,
	Pages = {L27-L30},
	Title = {{The Tycho-2 catalogue of the 2.5 million brightest stars}},
	Volume = 355,
	Year = 2000}

@article{holder06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006APh....25..391H&db_key=AST},
	Author = {{Holder}, J. and {Atkins}, R.~W. and {Badran}, H.~M. and {Blaylock}, G. and {Bradbury}, S.~M. and {Buckley}, J.~H. and {Byrum}, K.~L. and {Carter-Lewis}, D.~A. and {Celik}, O. and {Chow}, Y.~C.~K. and {Cogan}, P. and {Cui}, W. and {Daniel}, M.~K. and {de La Calle Perez}, I. and {Dowdall}, C. and {Dowkontt}, P. and {Duke}, C. and {Falcone}, A.~D. and {Fegan}, S.~J. and {Finley}, J.~P. and {Fortin}, P. and {Fortson}, L.~F. and {Gibbs}, K. and {Gillanders}, G. and {Glidewell}, O.~J. and {Grube}, J. and {Gutierrez}, K.~J. and {Gyuk}, G. and {Hall}, J. and {Hanna}, D. and {Hays}, E. and {Horan}, D. and {Hughes}, S.~B. and {Humensky}, T.~B. and {Imran}, A. and {Jung}, I. and {Kaaret}, P. and {Kenny}, G.~E. and {Kieda}, D. and {Kildea}, J. and {Knapp}, J. and {Krawczynski}, H. and {Krennrich}, F. and {Lang}, M.~J. and {Lebohec}, S. and {Linton}, E. and {Little}, E.~K. and {Maier}, G. and {Manseri}, H. and {Milovanovic}, A. and {Moriarty}, P. and {Mukherjee}, R. and {Ogden}, P.~A. and {Ong}, R.~A. and {Petry}, D. and {Perkins}, J.~S. and {Pizlo}, F. and {Pohl}, M. and {Quinn}, J. and {Ragan}, K. and {Reynolds}, P.~T. and {Roache}, E.~T. and {Rose}, H.~J. and {Schroedter}, M. and {Sembroski}, G.~H. and {Sleege}, G. and {Steele}, D. and {Swordy}, S.~P. and {Syson}, A. and {Toner}, J.~A. and {Valcarcel}, L. and {Vassiliev}, V.~V. and {Wakely}, S.~P. and {Weekes}, T.~C. and {White}, R.~J. and {Williams}, D.~A. and {Wagner}, R.},
	Doi = {10.1016/j.astropartphys.2006.04.002},
	Eprint = {astro-ph/0604119},
	Journal = {Astroparticle Physics},
	Month = jul,
	Pages = {391-401},
	Title = {{The first VERITAS telescope}},
	Volume = 25,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.astropartphys.2006.04.002}}

@article{holland98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1916H},
	Author = {{Holland}, S.},
	Doi = {10.1086/300348},
	Eprint = {arXiv:astro-ph/9802088},
	Journal = {\aj},
	Keywords = {GALAXIES: DISTANCES AND REDSHIFTS, GALAXIES: INDIVIDUAL: MESSIER NUMBER: M31, GALAXIES: STAR CLUSTERS},
	Month = may,
	Pages = {1916-1920},
	Title = {{The Distance to the M31 Globular Cluster System}},
	Volume = 115,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/300348}}

@article{hvdbg12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746..165H},
	Archiveprefix = {arXiv},
	Author = {{Hong}, J. and {van den Berg}, M. and {Grindlay}, J.~E. and {Servillat}, M. and {Zhao}, P.},
	Doi = {10.1088/0004-637X/746/2/165},
	Eid = {165},
	Eprint = {1103.2477},
	Journal = {\apj},
	Keywords = {Galaxy: bulge, novae, cataclysmic variables, X-rays: binaries},
	Month = feb,
	Pages = {165},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of a Significant Magnetic Cataclysmic Variable Population in the Limiting Window}},
	Volume = 746,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/746/2/165}}

@article{hong12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.1633H},
	Archiveprefix = {arXiv},
	Author = {{Hong}, J.},
	Doi = {10.1111/j.1365-2966.2012.22079.x},
	Eprint = {1209.1725},
	Journal = {\mnras},
	Keywords = {Galaxy: bulge, X-rays: binaries, X-rays: diffuse background},
	Month = dec,
	Pages = {1633-1650},
	Primaryclass = {astro-ph.HE},
	Title = {{Dominance of magnetic cataclysmic variables in the resolved Galactic ridge X-ray emission of the limiting window}},
	Volume = 427,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.22079.x}}

@article{hopkins06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...651..142H},
	Author = {{Hopkins}, A.~M. and {Beacom}, J.~F.},
	Doi = {10.1086/506610},
	Eprint = {astro-ph/0601463},
	Journal = {\apj},
	Keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: Starburst, Neutrinos, Stars: Supernovae: General},
	Month = nov,
	Pages = {142-154},
	Title = {{On the Normalization of the Cosmic Star Formation History}},
	Volume = 651,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506610}}

@article{horne86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986PASP...98..609H},
	Author = {{Horne}, K.},
	Doi = {10.1086/131801},
	Journal = {\pasp},
	Keywords = {ASTRONOMICAL SPECTROSCOPY, CHARGE COUPLED DEVICES, DATA REDUCTION, SPECTRUM ANALYSIS, IMAGE PROCESSING, ITERATION, OPTIMIZATION, SPATIAL RESOLUTION, STELLAR SPECTRA, VARIANCE (STATISTICS)},
	Month = jun,
	Pages = {609-617},
	Title = {{An optimal extraction algorithm for CCD spectroscopy}},
	Volume = 98,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/131801}}

@article{hb86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...302..757H},
	Author = {{Horne}, J.~H. and {Baliunas}, S.~L.},
	Doi = {10.1086/164037},
	Journal = {\apj},
	Keywords = {COMPUTATIONAL ASTROPHYSICS, PERIODIC FUNCTIONS, TIME SERIES ANALYSIS, FOURIER ANALYSIS, PROBABILITY DISTRIBUTION FUNCTIONS, SAMPLING, SIGNAL TO NOISE RATIOS, VARIANCE (STATISTICS)},
	Month = mar,
	Pages = {757-763},
	Title = {{A prescription for period analysis of unevenly sampled time series}},
	Volume = 302,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/164037}}

@article{hotan04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004PASA...21..302H},
	Author = {{Hotan}, A.~W. and {van Straten}, W. and {Manchester}, R.~N.},
	Doi = {10.1071/AS04022},
	Eprint = {arXiv:astro-ph/0404549},
	Journal = {\pasa},
	Keywords = {pulsars: general, methods: data analysis},
	Pages = {302-309},
	Title = {{PSRCHIVE and PSRFITS: An Open Approach to Radio Pulsar Data Storage and Analysis}},
	Volume = 21,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1071/AS04022}}

@article{hou09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...499..473H},
	Archiveprefix = {arXiv},
	Author = {{Hou}, L.~G. and {Han}, J.~L. and {Shi}, W.~B.},
	Doi = {10.1051/0004-6361/200809692},
	Eprint = {0903.0721},
	Journal = {\aap},
	Keywords = {Galaxy: structure, Galaxy: kinematics and dynamics, ISM: HII regions},
	Month = may,
	Pages = {473-482},
	Title = {{The spiral structure of our Milky Way Galaxy}},
	Volume = 499,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200809692}}

@article{hoversten11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011GCN..12316...1H},
	Author = {{Hoversten}, E.~A. and {Barthelmy}, S.~D. and {Baumgartner}, W.~H. and {Cummings}, J.~R. and {Gronwall}, C. and {Grupe}, D. and {Kennea}, J.~A. and {Krimm}, H.~A. and {Palmer}, D.~M. and {Saxton}, C.~J. and {Swenson}, C.~A. and {Troja}, E. and {Wolf}, C.~A. and {Zhang}, B.-B.},
	Journal = {GCN Circ.},
	Title = {{Swift detection of an Sgr burst from Swift J1834.9-0846.}},
	Volume = 12316,
	Year = 2011}

@ARTICLE{hoyle64,
   author = {{Hoyle}, F. and {Narlikar}, J.~V. and {Wheeler}, J.~A.},
    title = "{Electromagnetic Waves from Very Dense Stars}",
  journal = {\nat},
     year = 1964,
    month = aug,
   volume = 203,
    pages = {914-916},
      doi = {10.1038/203914a0},
   adsurl = {http://adsabs.harvard.edu/abs/1964Natur.203..914H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hubble29,
   author = {{Hubble}, E.~P.},
    title = "{A spiral nebula as a stellar system, Messier 31.}",
  journal = {\apj},
     year = 1929,
    month = mar,
   volume = 69,
    pages = {103},
      doi = {10.1086/143167},
   adsurl = {http://adsabs.harvard.edu/abs/1929ApJ....69..103H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hulleman00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000Natur.408..689H&db_key=AST},
	Author = {{Hulleman}, F. and {van Kerkwijk}, M.~H. and {Kulkarni}, S.~R.},
	Journal = {\nat},
	Month = dec,
	Pages = {689-692},
	Title = {{An optical counterpart to the anomalous X-ray pulsar 4U0142+61}},
	Volume = 408,
	Year = 2000}

@ARTICLE{hulleman04,
   author = {{Hulleman}, F. and {van Kerkwijk}, M.~H. and {Kulkarni}, S.~R.
	},
    title = "{The Anomalous X-ray Pulsar 4U 0142+61: Variability in the infrared and a spectral break in the optical}",
  journal = {\aap},
 keywords = {pulsars: individual: 4U 0142+61, stars: neutron, stars: magnetic fields, X-rays: general},
     year = 2004,
    month = mar,
   volume = 416,
    pages = {1037-1045},
      doi = {10.1051/0004-6361:20031756},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...416.1037H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hummel97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...320..852H},
	Author = {{Hummel}, W. and {Hanuschik}, R.~W.},
	Journal = {\aap},
	Keywords = {LINE: PROFILES, LINE: FORMATION, RADIATIVE TRANSFER, STARS: BE, CIRCUMSTELLAR MATTER},
	Month = apr,
	Pages = {852-864},
	Title = {{Line formation in Be star envelopes. II. Disk oscillations.}},
	Volume = 320,
	Year = 1997}

@ARTICLE{huppenkothen13,
   author = {{Huppenkothen}, D. and {Watts}, A.~L. and {Uttley}, P. and {van der Horst}, A.~J. and 
	{van der Klis}, M. and {Kouveliotou}, C. and {G{\"o}{\v g}{\"u}{\c s}}, E. and 
	{Granot}, J. and {Vaughan}, S. and {Finger}, M.~H.},
    title = "{Quasi-periodic Oscillations and Broadband Variability in Short Magnetar Bursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.1011},
 primaryClass = "astro-ph.HE",
 keywords = {methods: data analysis, methods: statistical, pulsars: individual: SGR 0501+4516, stars: magnetic field, stars: neutron, X-rays: bursts },
     year = 2013,
    month = may,
   volume = 768,
      eid = {87},
    pages = {87},
      doi = {10.1088/0004-637X/768/1/87},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768...87H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{huppenkothen14,
   author = {{Huppenkothen}, D. and {D'Angelo}, C. and {Watts}, A.~L. and 
	{Heil}, L. and {van der Klis}, M. and {van der Horst}, A.~J. and 
	{Kouveliotou}, C. and {Baring}, M.~G. and {G{\"o}{\u g}{\"u}{\c s}}, E. and 
	{Granot}, J. and {Kaneko}, Y. and {Lin}, L. and {von Kienlin}, A. and 
	{Younes}, G.},
    title = "{Quasi-periodic Oscillations in Short Recurring Bursts of the Soft Gamma Repeater J1550-5418}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1404.2756},
 primaryClass = "astro-ph.HE",
 keywords = {methods: data analysis, methods: statistical, pulsars: individual: SGR J1550{\ndash}5418, stars: magnetic field, stars: neutron, X-rays: bursts},
     year = 2014,
    month = jun,
   volume = 787,
      eid = {128},
    pages = {128},
      doi = {10.1088/0004-637X/787/2/128},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787..128H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hhw14,
   author = {{Huppenkothen}, D. and {Heil}, L.~M. and {Watts}, A.~L. and 
	{G{\"o}{\u g}{\"u}{\c s}}, E.},
    title = "{Quasi-periodic Oscillations in Short Recurring Bursts of Magnetars SGR 1806-20 and SGR 1900+14 Observed with RXTE}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1409.7642},
 primaryClass = "astro-ph.HE",
 keywords = {methods: statistical, pulsars: individual: SGR 1806{\ndash}20 SGR 1900+14, stars: magnetic field, stars: neutron, X-rays: bursts},
     year = 2014,
    month = nov,
   volume = 795,
      eid = {114},
    pages = {114},
      doi = {10.1088/0004-637X/795/2/114},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...795..114H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{huppenkothen15,
   author = {{Huppenkothen}, D. and {Brewer}, B.~J. and {Hogg}, D.~W. and 
	{Murray}, I. and {Frean}, M. and {Elenbaas}, C. and {Watts}, A.~L. and 
	{Levin}, Y. and {van der Horst}, A.~J. and {Kouveliotou}, C.
	},
    title = "{Dissecting Magnetar Variability with Bayesian Hierarchical Models}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.05251},
 primaryClass = "astro-ph.HE",
 keywords = {methods: data analysis, methods: statistical, pulsars: individual: SGR J1550{\ndash}5418, stars: magnetars, stars: magnetic field, X-rays: bursts},
     year = 2015,
    month = sep,
   volume = 810,
      eid = {66},
    pages = {66},
      doi = {10.1088/0004-637X/810/1/66},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...810...66H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hurley99_4sgr,
	Adsurl = {http://it.arXiv.org/find/astro-ph/1/hurley%3B+review/0/1/0/1999/1/0},
	Author = {{Hurley}, K.},
	Eprint = {astro-ph/9912061},
	Journal = {ArXiv Astrophysics e-prints (astro-ph/9912061)},
	Month = dec,
	Title = {{The 4.5 $\pm 0.5$ Soft Gamma Repeaters in Review}},
	Year = 1999}

@article{hkm99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...510L.111H&db_key=AST},
	Author = {{Hurley}, K. and {Li}, P. and {Kouveliotou}, C. and {Murakami}, T. and {Ando}, M. and {Strohmayer}, T. and {van Paradijs}, J. and {Vrba}, F. and {Luginbuhl}, C. and {Yoshida}, A. and {Smith}, I.},
	Journal = {\apjl},
	Month = jan,
	Pages = {L111-L114},
	Title = {{ASCA Discovery of an X-Ray Pulsar in the Error Box of SGR 1900+14}},
	Volume = 510,
	Year = 1999}

@article{hurley99_1627,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...519L.143H&db_key=AST},
	Author = {{Hurley}, K. and {Kouveliotou}, C. and {Woods}, P. and {Mazets}, E. and {Golenetskii}, S. and {Frederiks}, D.~D. and {Cline}, T. and {van Paradijs}, J.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L143-L145},
	Title = {{Precise Interplanetary Network Localization of a New Soft Gamma Repeater, SGR 1627-41}},
	Volume = 519,
	Year = 1999}

@article{hkc99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...523L..37H&db_key=AST},
	Author = {{Hurley}, K. and {Kouveliotou}, C. and {Cline}, T. and {Mazets}, E. and {Golenetskii}, S. and {Frederiks}, D.~D. and {van Paradijs}, J.},
	Journal = {\apjl},
	Month = sep,
	Pages = {L37-L40},
	Title = {{Where is SGR 1806-20?}},
	Volume = 523,
	Year = 1999}

@article{hkw99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...510L.107H&db_key=AST},
	Author = {{Hurley}, K. and {Kouveliotou}, C. and {Woods}, P. and {Cline}, T. and {Butterworth}, P. and {Mazets}, E. and {Golenetskii}, S. and {Frederics}, D.},
	Journal = {\apjl},
	Month = jan,
	Pages = {L107-L109},
	Title = {{Reactivation and Precise Interplanetary Network Localization of the Soft Gamma Repeater SGR 1900+14}},
	Volume = 510,
	Year = 1999}

@article{hurley00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...528L..21H&db_key=AST},
	Author = {{Hurley}, K. and {Strohmayer}, T. and {Li}, P. and {Kouveliotou}, C. and {Woods}, P. and {van Paradijs}, J. and {Murakami}, T. and {Hartmann}, D. and {Smith}, I. and {Ando}, M. and {Yoshida}, A. and {Sugizaki}, M.},
	Journal = {\apjl},
	Month = jan,
	Pages = {L21-L23},
	Title = {{ASCA Observation of the Quiescent X-Ray Counterpart to SGR 1627-41}},
	Volume = 528,
	Year = 2000}

@article{hurley02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002GCN..1715....1H&db_key=AST},
	Author = {{Hurley}, K. and {Mazets}, E. and {Golenetskii}, S. and {Cline}, T.},
	Journal = {GCN Circ. 1715},
	Title = {{IPN detection of continued SGR1900+14 activity.}},
	Year = 2002}

@inproceedings{hurley03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003AIPC..662..473H&db_key=AST},
	Author = {{Hurley}, K. and {Cline}, T. and {Mitrofanov}, I. and {Mazets}, E. and {Golenetskii}, S. and {Frontera}, F. and {Montanari}, E. and {Guidorzi}, C. and {Feroci}, M.},
	Booktitle = {AIP Conference Proceedings 662: Gamma-Ray Burst and Afterglow Astronomy 2001: A Workshop Celebrating the First Year of the HETE Mission},
	Month = apr,
	Pages = {473-476},
	Title = {{The Current Performance of the Third Interplanetary Network}},
	Year = 2003}

@article{hutchings81,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PASP...93..486H&db_key=AST},
	Author = {{Hutchings}, J.~B. and {Crampton}, D.},
	Journal = {\pasp},
	Month = aug,
	Pages = {486-489},
	Title = {{Spectroscopy of the unique degenerate binary star LSI + 61 deg 303}},
	Volume = 93,
	Year = 1981}

@article{ibrahim01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...558..237I&db_key=AST},
	Author = {{Ibrahim}, A.~I. and {Strohmayer}, T.~E. and {Woods}, P.~M. and {Kouveliotou}, C. and {Thompson}, C. and {Duncan}, R.~C. and {Dieters}, S. and {Swank}, J.~H. and {van Paradijs}, J. and {Finger}, M.},
	Journal = {\apj},
	Month = sep,
	Pages = {237-252},
	Title = {{An Unusual Burst from Soft Gamma Repeater SGR 1900+14: Comparisons with Giant Flares and Implications for the Magnetar Model}},
	Volume = 558,
	Year = 2001}

@article{ibrahim02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...574L..51I&db_key=AST},
	Author = {{Ibrahim}, A.~I. and {Safi-Harb}, S. and {Swank}, J.~H. and {Parke}, W. and {Zane}, S. and {Turolla}, R.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L51-L55},
	Title = {{Discovery of Cyclotron Resonance Features in the Soft Gamma Repeater SGR 1806-20}},
	Volume = 574,
	Year = 2002}

@article{ibrahim03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...584L..17I&db_key=AST},
	Author = {{Ibrahim}, A.~I. and {Swank}, J.~H. and {Parke}, W.},
	Journal = {\apjl},
	Month = feb,
	Pages = {L17-L21},
	Title = {{New Evidence of Proton-Cyclotron Resonance in a Magnetar Strength Field from SGR 1806-20}},
	Volume = 584,
	Year = 2003}

@article{ibrahim04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...609L..21I&db_key=AST},
	Author = {{Ibrahim}, A.~I. and {Markwardt}, C.~B. and {Swank}, J.~H. and {Ransom}, S. and {Roberts}, M. and {Kaspi}, V. and {Woods}, P.~M. and {Safi-Harb}, S. and {Balman}, S. and {Parke}, W.~C. and {Kouveliotou}, C. and {Hurley}, K. and {Cline}, T.},
	Doi = {10.1086/422636},
	Eprint = {astro-ph/0310665},
	Journal = {\apjl},
	Month = jul,
	Pages = {L21-L24},
	Title = {{Discovery of a Transient Magnetar: XTE J1810-197}},
	Volume = 609,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422636}}

@article{illarionov75,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1975A%26A....39..185I},
	Author = {{Illarionov}, A.~F. and {Sunyaev}, R.~A.},
	Journal = {\aap},
	Month = feb,
	Pages = {185},
	Title = {{Why the Number of Galactic X-ray Stars Is so Small?}},
	Volume = 39,
	Year = 1975}

@article{illarionov90,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.247..219I},
	Author = {{Illarionov}, A.~F. and {Kompaneets}, D.~A.},
	Journal = {\mnras},
	Month = nov,
	Pages = {219},
	Title = {{A Spin-Down Mechanism for Accreting Neutron Stars}},
	Volume = 247,
	Year = 1990}

@inproceedings{immler03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003LNP...598...91I},
	Author = {{Immler}, S. and {Lewin}, W.~H.~G.},
	Booktitle = {Supernovae and Gamma-Ray Bursters},
	Editor = {{Weiler}, K.},
	Eprint = {arXiv:astro-ph/0202231},
	Pages = {91-111},
	Series = {Lecture Notes in Physics, Berlin Springer Verlag},
	Title = {{X-Ray Supernovae}},
	Volume = 598,
	Year = 2003}

@article{inan99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999GeoRL..26.3357I&db_key=AST},
	Author = {{Inan}, U.~S. and {Lehtinen}, N.~G. and {Lev-Tov}, S.~J. and {Johnson}, M.~P. and {Bell}, T.~F. and {Hurley}, K.},
	Journal = {Geophys. Res. Lett.},
	Month = nov,
	Pages = {3357-3360},
	Title = {{Ionization of the lower ionosphere by {$\gamma$}-rays from a magnetar: Detection of a low energy (3-10 keV) component}},
	Volume = 26,
	Year = 1999}

@ARTICLE{inan07,
   author = {{Inan}, U.~S. and {Lehtinen}, N.~G. and {Moore}, R.~C. and {Hurley}, K. and 
	{Boggs}, S. and {Smith}, D.~M. and {Fishman}, G.~J.},
    title = "{Massive disturbance of the daytime lower ionosphere by the giant {$\gamma$}-ray flare from magnetar SGR 1806-20}",
  journal = {Geophys. Res. Lett.},
 keywords = {Atmospheric Composition and Structure: Ion chemistry of the atmosphere (2419, 2427), Ionosphere: Ionization processes (7823), Ionosphere: Ionospheric disturbances, Solar Physics, Astrophysics, and Astronomy: X-rays, gamma rays, and neutrinos},
     year = 2007,
    month = apr,
   volume = 34,
      eid = {L08103},
    pages = {L08103},
      doi = {10.1029/2006GL029145},
   adsurl = {http://adsabs.harvard.edu/abs/2007GeoRL..34.8103I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ingram21,
       author = {{Ingram}, Adam and {Motta}, Sara E. and {Aigrain}, Suzanne and {Karastergiou}, Aris},
        title = "{A self-lensing binary massive black hole interpretation of quasi-periodic eruptions}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational lensing: micro, gravitational waves, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {503},
       number = {2},
        pages = {1703-1716},
          doi = {10.1093/mnras/stab609},
archivePrefix = {arXiv},
       eprint = {2103.00017},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.1703I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{inoue84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984PASJ...36..709I},
	Author = {{Inoue}, H. and {Ogawara}, Y. and {Waki}, I. and {Ohashi}, T. and {Hayakawa}, S. and {Kunieda}, H. and {Nagase}, F. and {Tsunemi}, H.},
	Journal = {\pasj},
	Keywords = {Eclipsing Binary Stars, Pulsars, Radiant Flux Density, Stellar Radiation, X Ray Binaries, X Ray Spectra, Astronomical Satellites, Stellar Models, Variable Stars},
	Pages = {709-713},
	Title = {{Sudden disappearance of VELA X-1 pulses}},
	Volume = 36,
	Year = 1984}

@article{intzand98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998ApJ...496..386I&db_key=AST},
	Author = {{in't Zand}, J.~J.~M. and {Baykal}, A. and {Strohmayer}, T.~E.},
	Doi = {10.1086/305362},
	Journal = {\apj},
	Month = mar,
	Pages = {386},
	Title = {{Recent X-Ray Measurements of the Accretion-powered Pulsar 4U 1907+09}},
	Volume = 496,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/305362}}

@article{intzand02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002A%26A...394..553I&db_key=AST},
	Author = {{in't Zand}, J.~J.~M. and {Miller}, J.~M. and {Oosterbroek}, T. and {Parmar}, A.~N.},
	Journal = {\aap},
	Month = nov,
	Pages = {553-560},
	Title = {{Broad-band X-ray measurements of the black hole candidate XTE J1908+094}},
	Volume = 394,
	Year = 2002}

@inproceedings{intzand04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ESASP.552..427I},
	Author = {{in't Zand}, J. and {Heise}, J. and {Ubertini}, P. and {Bazzano}, A. and {Markwardt}, C.},
	Booktitle = {5th INTEGRAL Workshop on the INTEGRAL Universe},
	Editor = {{Schoenfelder}, V. and {Lichti}, G. and {Winkler}, C.},
	Eprint = {astro-ph/0407085},
	Month = oct,
	Pages = {427},
	Series = {ESA Special Publication},
	Title = {{A BeppoSAX-WFC Viewpoint of New INTEGRAL Sources, Particularly IGR J17544-2619}},
	Volume = 552,
	Year = 2004}

@article{intzand06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...448.1101I},
	Author = {{in't Zand}, J.~J.~M. and {Jonker}, P.~G. and {Nelemans}, G. and {Steeghs}, D. and {O'Brien}, K.},
	Doi = {10.1051/0004-6361:20053411},
	Eprint = {astro-ph/0505256},
	Journal = {\aap},
	Keywords = {X-rays: binaries, X-rays: individuals: EXO 1912+098, IGR J19140+0951, , 2MASS 19140422+0952577},
	Month = mar,
	Pages = {1101-1106},
	Title = {{Optical identification of IGR J19140+0951}},
	Volume = 448,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053411}}

@article{irwin06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.371.1903I},
	Author = {{Irwin}, J.~A.},
	Doi = {10.1111/j.1365-2966.2006.10822.x},
	Eprint = {arXiv:astro-ph/0607395},
	Journal = {\mnras},
	Keywords = {binaries: close: galaxies: elliptical and lenticular, cD: X-rays: binaries: X-rays: galaxies, binaries: close, galaxies: elliptical and lenticular, cD, X-rays: binaries, X-rays: galaxies},
	Month = oct,
	Pages = {1903-1911},
	Title = {{The remarkable stability of probable black hole low-mass X-ray binaries in nearby galaxies}},
	Volume = 371,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10822.x}}

@ARTICLE{irwin10,
       author = {{Irwin}, Jimmy A. and {Brink}, Thomas G. and {Bregman}, Joel N. and
         {Roberts}, Timothy P.},
        title = "{Evidence for a Stellar Disruption by an Intermediate-mass Black Hole in an Extragalactic Globular Cluster}",
      journal = {\apjl},
     keywords = {galaxies: individual: NGC 1399, galaxies: star clusters: general, globular clusters: general, X-rays: binaries, X-rays: galaxies: clusters, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = mar,
       volume = {712},
       number = {1},
        pages = {L1-L4},
          doi = {10.1088/2041-8205/712/1/L1},
archivePrefix = {arXiv},
       eprint = {0908.1115},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...712L...1I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{irwin16,
       author = {{Irwin}, Jimmy A. and {Maksym}, W. Peter and {Sivakoff}, Gregory R. and {Romanowsky}, Aaron J. and {Lin}, Dacheng and {Speegle}, Tyler and {Prado}, Ian and {Mildebrath}, David and {Strader}, Jay and {Liu}, Jifeng and {Miller}, Jon M.},
        title = "{Ultraluminous X-ray bursts in two ultracompact companions to nearby elliptical galaxies}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {538},
       number = {7625},
        pages = {356-358},
          doi = {10.1038/nature19822},
archivePrefix = {arXiv},
       eprint = {1610.05781},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Natur.538..356I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ishida94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994PASJ...46L..81I},
	Author = {{Ishida}, M. and {Mukai}, K. and {Osborne}, J.~P.},
	Journal = {\pasj},
	Keywords = {Cataclysmic Variables, Dwarf Stars, Stellar Radiation, X Ray Spectra, Abundance, Spectrum Analysis, Stellar Spectra, Temperature Effects},
	Month = jun,
	Pages = {L81-L85},
	Title = {{Observation of EX Hydrae with ASCA}},
	Volume = 46,
	Year = 1994}

@article{iskudaryan67,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1967Ap......3...67I},
	Author = {{Iskudaryan}, S.~G. and {Shakhbazyan}, R.~K.},
	Doi = {10.1007/BF01006031},
	Journal = {Astrophysics},
	Month = mar,
	Pages = {67-67},
	Title = {{A supernova in NGC 2276}},
	Volume = 3,
	Year = 1967,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/BF01006031}}

@article{israel94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994ApJ...433L..25I&db_key=AST},
	Author = {{Israel}, G.~L. and {Mereghetti}, S. and {Stella}, L.},
	Journal = {\apjl},
	Month = sep,
	Pages = {L25-L28},
	Title = {{The discovery of 8.7 second pulsations from the ultrasoft X-ray source 4U 0142+61}},
	Volume = 433,
	Year = 1994}

@article{israel96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...468..369I},
	Author = {{Israel}, G.~L. and {Stella}, L.},
	Doi = {10.1086/177697},
	Eprint = {arXiv:astro-ph/9603038},
	Journal = {\apj},
	Keywords = {METHODS: NUMERICAL, METHODS: STATISTICAL, STARS: OSCILLATIONS, X-RAYS: STARS},
	Month = sep,
	Pages = {369},
	Title = {{A New Technique for the Detection of Periodic Signals in ``Colored'' Power Spectra}},
	Volume = 468,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177697}}

@article{israel97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...474L..53I},
	Author = {{Israel}, G.~L. and {Stella}, L. and {Angelini}, L. and {White}, N.~E. and {Kallman}, T.~R. and {Giommi}, P. and {Treves}, A.},
	Doi = {10.1086/310418},
	Eprint = {astro-ph/9610139},
	Journal = {\apjl},
	Keywords = {STARS: BINARIES: SPECTROSCOPIC, STARS: PULSARS: INDIVIDUAL ALPHANUMERIC: HD 49798, STARS: ROTATION, STARS: SUBDWARFS, X-RAYS: STARS, Stars: Binaries: Spectroscopic, Stars: Pulsars: Individual: Alphanumeric: HD 49798, Stars: Rotation, Stars: Subdwarfs, X-Rays: Stars},
	Month = jan,
	Pages = {L53-L56},
	Title = {{The Discovery of 13 Second X-Ray Pulsations from the Hydrogen-depleted Subdwarf O6 Star Binary HD 49798}},
	Volume = 474,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310418}}

@article{israel99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999A%26A...346..929I&db_key=AST},
	Author = {{Israel}, G.~L. and {Oosterbroek}, T. and {Angelini}, L. and {Campana}, S. and {Mereghetti}, S. and {Parmar}, A.~N. and {Segreto}, A. and {Stella}, L. and {van Paradijs}, J. and {White}, N.~E.},
	Journal = {\aap},
	Month = jun,
	Pages = {929-935},
	Title = {{BeppoSAX monitoring of the ``anomalous'' X-ray pulsar 4U 0142+61}},
	Volume = 346,
	Year = 1999}

@article{ics99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1999ApJ...518L.107I},
	Author = {{Israel}, G.~L. and {Covino}, S. and {Stella}, L. and {Campana}, S. and {Haberl}, F. and {Mereghetti}, S.},
	Doi = {10.1086/312077},
	Eprint = {arXiv:astro-ph/9904212},
	Journal = {\apjl},
	Month = jun,
	Pages = {L107-L110},
	Title = {{Further Evidence that 1RXS J170849.0-400910 Is an Anomalous X-Ray Pulsar}},
	Volume = 518,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312077}}

@article{ipc99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...349L...1I},
	Author = {{Israel}, G.~L. and {Panzera}, M.~R. and {Campana}, S. and {Lazzati}, D. and {Covino}, S. and {Tagliaferri}, G. and {Stella}, L.},
	Journal = {\aap},
	Keywords = {STARS: INDIVIDUAL: RX J0806.3+1527, STARS: NOVAE, CATACLYSMIC VARIABLES, STARS: PULSARS: GENERAL, STARS: ROTATION, X-RAYS: STARS},
	Month = sep,
	Pages = {L1-L4},
	Title = {{The discovery of 321 S pulsations in the ROSAT HRI light curves of 1BMW J080622.8+152732 = RX J0806.3+1527}},
	Volume = 349,
	Year = 1999}

@article{israel01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001ApJ...560L..65I},
	Author = {{Israel}, G. and {Oosterbroek}, T. and {Stella}, L. and {Campana}, S. and {Mereghetti}, S. and {Parmar}, A.~N.},
	Doi = {10.1086/324169},
	Eprint = {arXiv:astro-ph/0108506},
	Journal = {\apjl},
	Month = oct,
	Pages = {L65-L69},
	Title = {{The Pulse-Phase-dependent Spectrum of the Anomalous X-Ray Pulsar 1RXS J170849-400910}},
	Volume = 560,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324169}}

@article{israel02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...386L..13I},
	Author = {{Israel}, G.~L. and {Hummel}, W. and {Covino}, S. and {Campana}, S. and {Appenzeller}, I. and {G{\"a}ssler}, W. and {Mantel}, {K.-H.} and {Marconi}, G. and {Mauche}, C.~W. and {Munari}, U. and {Negueruela}, I. and {Nicklas}, H. and {Rupprecht}, G. and {Smart}, R.~L. and {Stahl}, O. and {Stella}, L.},
	Doi = {10.1051/0004-6361:20020314},
	Eprint = {arXiv:astro-ph/0203043},
	Journal = {\aap},
	Keywords = {Stars: Individual: RRX J0806.3+1527, Binaries: Close, Stars: White Dwarfs, Stars: Emission-Line, X-rays: Stars},
	Month = may,
	Pages = {L13-L17},
	Title = {{RX J0806.3+1527: A double degenerate binary with the shortest known orbital period (321s)}},
	Volume = 386,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020314}}

@article{israel03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598..492I},
	Author = {{Israel}, G.~L. and {Covino}, S. and {Stella}, L. and {Mauche}, C.~W. and {Campana}, S. and {Marconi}, G. and {Hummel}, W. and {Mereghetti}, S. and {Munari}, U. and {Negueruela}, I.},
	Doi = {10.1086/378803},
	Eprint = {arXiv:astro-ph/0308045},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Close, Stars: Binaries: General, Stars: Novae, Cataclysmic Variables, Stars: Individual: Alphanumeric: RX J0806.3+1527, Stars: Individual: Alphanumeric: RX J1914.4+2456, Stars: White Dwarfs, X-Rays: Binaries},
	Month = nov,
	Pages = {492-500},
	Title = {{Unveiling the Nature of the 321 Second Modulation in RX J0806.3+1527: Near-Simultaneous Chandra and Very Large Telescope Observations}},
	Volume = 598,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378803}}

@article{icd04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MSAIS...5..148I},
	Author = {{Israel}, G.~L. and {Covino}, S. and {Dall'Osso}, S. and {Fugazza}, D. and {Mouche}, C.~W. and {Stella}, L. and {Campana}, S. and {Mangano}, V. and {Marconi}, G. and {Bagnulo}, S. and {Munari}, U.},
	Eprint = {arXiv:astro-ph/0410453},
	Journal = {Mem. S. A. It. Suppl.},
	Keywords = {cataclysmic variables, white dwarfs, ultracompact binaries, X-rays binaries},
	Pages = {148},
	Title = {{Taking the pulse of the shortest orbital period binary system RX J0806.3+1527}},
	Volume = 5,
	Year = 2004}

@inproceedings{israel04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004IAUS..218..247I&db_key=AST},
	Author = {{Israel}, G. and {Stella}, L. and {Covino}, S. and {Campana}, S. and {Angelini}, L. and {Mignani}, R. and {Mereghetti}, S. and {Marconi}, G. and {Perna}, R.},
	Booktitle = {Young Neutron Stars and Their Environments, IAU Symposium no. 218},
  Publisher={Astronomical Society of the Pacific (san Francisco)},
	Editor = {{Camilo}, F. and {Gaensler}, B.~M.},
	Pages = {247},
	Title = {{Unveiling the Multi-wavelength Phenomenology of Anomalous X-ray Pulsars}},
	Year = 2004}

@article{irm04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...603L..97I},
	Author = {{Israel}, G.~L. and {Rea}, N. and {Mangano}, V. and {Testa}, V. and {Perna}, R. and {Hummel}, W. and {Mignani}, R. and {Ageorges}, N. and {Lo Curto}, G. and {Marco}, O. and {Angelini}, L. and {Campana}, S. and {Covino}, S. and {Marconi}, G. and {Mereghetti}, S. and {Stella}, L.},
	Doi = {10.1086/382875},
	Eprint = {arXiv:astro-ph/0401334},
	Journal = {\apjl},
	Keywords = {Infrared: Stars, Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: XTE J1810-197, Stars: Neutron, X-Rays: Stars},
	Month = mar,
	Pages = {L97-L100},
	Title = {{Accurate X-Ray Position of the Anomalous X-Ray Pulsar XTE J1810-197 and Identification of Its Likely Infrared Counterpart}},
	Volume = 603,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/382875}}

@article{israel05_atel,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005ATel..378....1I&db_key=AST},
	Author = {{Israel}, G.~L. and {Covino}, S. and {Mereghetti}, S. and {Mignani}, R. and {Stella}, L. and {Testa}, V. and {Marconi}, G.},
	Journal = {Astron.~Tel.~378},
	Month = jan,
	Title = {{Possible identification of the IR counterpart of SGR 1806-20}},
	Year = 2005}

@article{ibs05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005ApJ...628L..53I&db_key=AST},
	Author = {{Israel}, G.~L. and {Belloni}, T. and {Stella}, L. and {Rephaeli}, Y. and {Gruber}, D.~E. and {Casella}, P. and {Dall'Osso}, S. and {Rea}, N. and {Persic}, M. and {Rothschild}, R.~E.},
	Doi = {10.1086/432615},
	Eprint = {astro-ph/0505255},
	Journal = {\apjl},
	Month = jul,
	Pages = {L53-L56},
	Title = {{The Discovery of Rapid X-Ray Oscillations in the Tail of the SGR 1806-20 Hyperflare}},
	Volume = 628,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432615}}

@inproceedings{idm05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005AIPC..797..307I},
	Author = {{Israel}, G.~L. and {dall'Osso}, S. and {Mangano}, V. and {Stella}, L. and {Covino}, S. and {Fugazza}, D. and {Campana}, S. and {Marconi}, G. and {Mereghetti}, S. and {Munari}, U.},
	Booktitle = {Interacting Binaries: Accretion, Evolution, and Outcomes},
	Doi = {10.1063/1.2130248},
	Editor = {{Burderi}, L. and {Antonelli}, L.~A. and {D'Antona}, F. and {di Salvo}, T. and {Israel}, G.~L. and {Piersanti}, L. and {Tornamb{\`e}}, A. and {Straniero}, O.},
	Keywords = {white dwarfs, cataclysmic binary stars, X-ray binary stars, astronomical telescopes, X-ray sources (astronomical), Faint blue stars , white dwarfs, degenerate stars, nuclei of planetary nebulae, Spectroscopic binaries; close binaries, Cataclysmic binaries ; symbiotic stars, X-ray binaries, X-ray},
	Month = oct,
	Pages = {307-312},
	Publisher = {AIP, Melville},
	Series = {AIP Conference Series},
	Title = {{RX J0806.3-1527: Ten Years of Phase Coherent Monitoring in the Optical and X-ray Bands}},
	Volume = 797,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2130248}}

@article{israel07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...476L...9I},
	Archiveprefix = {arXiv},
	Author = {{Israel}, G.~L. and {G{\"o}tz}, D. and {Zane}, S. and {Dall'Osso}, S. and {Rea}, N. and {Stella}, L.},
	Doi = {10.1051/0004-6361:20078215},
	Eprint = {0707.0485},
	Journal = {\aap},
	Keywords = {stars: individual: 1RXS J170849-400910, stars: neutron, stars: X-rays,},
	Month = dec,
	Pages = {L9-L12},
	Title = {{Linking the X-ray timing and spectral properties of the glitching AXP 1RXS J170849-400910}},
	Volume = 476,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078215}}

@article{icd07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...664..448I},
	Author = {{Israel}, G.~L. and {Campana}, S. and {Dall'Osso}, S. and {Muno}, M.~P. and {Cummings}, J. and {Perna}, R. and {Stella}, L.},
	Doi = {10.1086/518224},
	Eprint = {arXiv:astro-ph/0703684},
	Journal = {\apj},
	Keywords = {pulsars: individual (CXOU J164710.2-455216), Stars: Neutron, X-Rays: Bursts},
	Month = jul,
	Pages = {448-457},
	Title = {{The Post-Burst Awakening of the Anomalous X-Ray Pulsar in Westerlund 1}},
	Volume = 664,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518224}}

@inproceedings{ibb08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008AIPC..983..311D},
	Author = {{Israel}, G. and {Bernardini}, F. and {Burgay}, M. and {Rea}, N. and {Possenti}, A. and {Dall'Osso}, S.},
	Booktitle = {{Bassa} C., {Wang} Z., {Cumming} A., {Kaspi} V.~M., eds., 40 years of pulsars: Millisecond Pulsars, Magnetars and More.},
	Doi = {10.1063/1.2900173},
	Keywords = {supernova remnants, neutron stars, X-ray sources (astronomical), pulsars},
	Month = feb,
	Pages = {244},
	Series = {AIP Conference Proceedings, Melville NY},
	Title = {{Transient Phenomena in Anomalous X-ray Pulsars}},
	Volume = 983,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2900173}}

@article{israel08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...685.1114I},
	Archiveprefix = {arXiv},
	Author = {{Israel}, G.~L. and {Romano}, P. and {Mangano}, V. and {Dall'Osso}, S. and {Chincarini}, G. and {Stella}, L. and {Campana}, S. and {Belloni}, T. and {Tagliaferri}, G. and {Blustin}, A.~J. and {Sakamoto}, T. and {Hurley}, K. and {Zane}, S. and {Moretti}, A. and {Palmer}, D. and {Guidorzi}, C. and {Burrows}, D.~N. and {Gehrels}, N. and {Krimm}, H.~A.},
	Doi = {10.1086/590486},
	Eprint = {0805.3919},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: SGR 1900+14, Stars: Flare, Stars: Neutron, X-Rays: Bursts},
	Month = oct,
	Pages = {1114-1128},
	Title = {{A Swift Gaze into the 2006 March 29 Burst Forest of SGR 1900+14}},
	Volume = 685,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/590486}}

@article{israel08_atel,
	Author = {{Israel}, G.~L. and {Esposito}, P. and {Rea}, N. and {Krimm}, H.~A. and {Palmer}, D.~M. and {Gehrels}, N. and {Mereghetti}, S. and {Tiengo}, A. and {Senziani}, F. and {G\"otz}, D. and {Zane}, S.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients, Variables},
	Month = oct,
	Title = {{Swift phase-coherent P-Pdot solution for the 1E1547.0-5408 outburst}},
	Volume = 1770,
	Year = 2008}

@article{iwd08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ATel.1837....1I},
	Author = {{Israel}, G.~L. and {Woods}, P. and {Dall'Osso}, S. and {Esposito}, P. and {Rea}, N. and {Kouveliotou}, C. and {Mangano}, E.~G.~V. and {Romano}, P. and {Palmer}, D. and {Gehrels}, N. and {Stella}, L. and {Zane}, S.},
	Journal = {Astron. Tel.},
	Keywords = {Soft Gamma-ray Repeaters},
	Month = nov,
	Title = {{Swift detection of the second period derivative in the timing evolution of SGR0501+4516}},
	Volume = 1837,
	Year = 2008}

@inproceedings{israel09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ASSL..359..281I},
	Author = {{Israel}, G.~L. and {Dall'Osso}, S.},
	Booktitle = {Physics of Relativistic Objects in Compact Binaries: From Birth to Coalescence},
	Doi = {10.1007/978-1-4020-9264-0_8},
	Editor = {{M.~Colpi, P.~Casella, V.~Gorini, U.~Moschella, \& A.~Possenti }},
	Pages = {281},
	Publisher = {Springer, Dordrecht},
	Series = {Astrophysics and Space Science Library.},
	Title = {{White Dwarfs in Ultrashort Binary Systems}},
	Volume = 359,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-1-4020-9264-0_8}}

@article{ieg09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2209....1I},
	Author = {{Israel}, G.~L. and {Esposito}, P. and {G\"otz}, D. and {Rea}, N.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients},
	Month = sep,
	Title = {{Evidence for the first period derivative of SGR 0418+4729}},
	Volume = 2209,
	Year = 2009}

@article{israel10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408.1387I},
	Archiveprefix = {arXiv},
	Author = {{Israel}, G.~L. and {Esposito}, P. and {Rea}, N. and {Dall'Osso}, S. and {Senziani}, F. and {Romano}, P. and {Mangano}, V. and {G{\"o}tz}, D. and {Zane}, S. and {Tiengo}, A. and {Palmer}, D.~M. and {Krimm}, H. and {Gehrels}, N. and {Mereghetti}, S. and {Stella}, L. and {Turolla}, R. and {Campana}, S. and {Perna}, R. and {Angelini}, L. and {De Luca}, A.},
	Doi = {10.1111/j.1365-2966.2010.17001.x},
	Eprint = {1006.2950},
	Journal = {\mnras},
	Keywords = {stars: neutron, X-rays: bursts, X-rays: individual: 1E1547.0-5408},
	Month = nov,
	Pages = {1387-1395},
	Primaryclass = {astro-ph.HE},
	Title = {{The 2008 October Swift detection of X-ray bursts/outburst from the transient SGR-like AXP 1E1547.0-5408}},
	Volume = 408,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17001.x}}

@incollection{israel11,
	Author = {{Israel}, G. and {Dall'Osso}, S.},
	Booktitle = {High-Energy Emission from Pulsars and their Systems. Proceedings of the First Session of the Sant Cugat Forum on Astrophysics
},
	Doi = {10.1007/978-3-642-17251-9_23},
	Editor = {Torres, Diego F. and Rea, Nanda},
	Isbn = {978-3-642-17250-2},
	Pages = {279-298},
	Publisher = {Springer, Heidelberg},
	Series = {Astrophysics and Space Science Proceedings},
	Title = {Bursts and Flares from Highly Magnetic Pulsars},
	Year = {2011},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-3-642-17251-9_21}}

@article{israel12,
	Author = {{Israel}, G.~L. and {Esposito}, P. and {Rea}, N. and {Turolla}, R. and {Zane}, S. and {Mereghetti}, S. and {Tiengo}, A.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients, Variables},
	Month = feb,
	Title = {{On the spin-down rate of Swift J1822.3-1606}},
	Volume = 3944,
	Year = 2012}

@article{ir12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.4241....1I},
	Author = {{Israel}, G.~L. and {Rodriguez}, G.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Binary, Neutron Star, Pulsar},
	Month = jul,
	Title = {{Archival ROSAT observations of the newly discovered X-ray Pulsar IGR J22534+6243 and its period derivative}},
	Volume = 4241,
	Year = 2012}
	
@ARTICLE{israel16,
       author = {{Israel}, G.~L. and {Esposito}, P. and {Rodr{\'\i}guez Castillo}, G.~A. and
         {Sidoli}, L.},
        title = "{The Chandra ACIS Timing Survey Project: glimpsing a sample of faint X-ray pulsators}",
      journal = {\mnras},
     keywords = {methods: data analysis, catalogues, stars: oscillations, pulsars: general, X-rays: binaries, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2016",
        month = "Nov",
       volume = {462},
       number = {4},
        pages = {4371-4385},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.4371I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{israel17,
   author = {{Israel}, G.~L. and {Belfiore}, A. and {Stella}, L. and {Esposito}, P. and 
	{Casella}, P. and {De Luca}, A. and {Marelli}, M. and {Papitto}, A. and 
	{Perri}, M. and {Puccetti}, S. and {Castillo}, G.~A.~R. and 
	{Salvetti}, D. and {Tiengo}, A. and {Zampieri}, L. and {D'Agostino}, D. and 
	{Greiner}, J. and {Haberl}, F. and {Novara}, G. and {Salvaterra}, R. and 
	{Turolla}, R. and {Watson}, M. and {Wilms}, J. and {Wolter}, A.
	},
    title = "{An accreting pulsar with extreme properties drives an ultraluminous x-ray source in NGC 5907}",
  journal = {Science},
     year = 2017,
    month = feb,
   volume = 355,
    pages = {817-819},
      doi = {10.1126/science.aai8635},
   adsurl = {http://adsabs.harvard.edu/abs/2017Sci...355..817I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ipe17,
   author = {{Israel}, G.~L. and {Papitto}, A. and {Esposito}, P. and {Stella}, L. and 
	{Zampieri}, L. and {Belfiore}, A. and {Rodr{\'{\i}}guez Castillo}, G.~A. and 
	{De Luca}, A. and {Tiengo}, A. and {Haberl}, F. and {Greiner}, J. and 
	{Salvaterra}, R. and {Sandrelli}, S. and {Lisini}, G.},
    title = "{Discovery of a 0.42-s pulsar in the ultraluminous X-ray source NGC 7793 P13}",
  journal = {\mnras},
 keywords = {galaxies: individual: NGC 7793, X-rays: binaries, X-rays: individual: CXOU J235750.9, 323726 (XMMU J235751.1-323725, NGC 7793 P13)},
     year = 2017,
    month = mar,
   volume = 466,
    pages = {L48-L52},
      doi = {10.1093/mnrasl/slw218},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.466L..48I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ivanova06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636..985I},
	Author = {{Ivanova}, N. and {Kalogera}, V.},
	Doi = {10.1086/498059},
	Eprint = {arXiv:astro-ph/0506471},
	Journal = {\apj},
	Keywords = {Galaxies: Elliptical and Lenticular, cD, Methods: Statistical, X-Rays: Binaries},
	Month = jan,
	Pages = {985-994},
	Title = {{The Brightest Point X-Ray Sources in Elliptical Galaxies and the Mass Spectrum of Accreting Black Holes}},
	Volume = 636,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498059}}

@article{iwazaki05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005PhRvD..72k4003I},
	Author = {{Iwazaki}, A.},
	Doi = {10.1103/PhysRevD.72.114003},
	Eid = {114003},
	Eprint = {arXiv:hep-ph/0508219},
	Journal = {\prd},
	Keywords = {Quark-gluon plasma, Nuclear matter aspects of neutron stars, Quantum Hall effects, Pulsars},
	Month = dec,
	Number = 11,
	Pages = {114003},
	Title = {{Color ferromagnetism of quark matter: A possible origin of a strong magnetic field in magnetars}},
	Volume = 72,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.72.114003}}

@article{iyudin98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998Natur.396..142I},
	Author = {{Iyudin}, A.~F. and {Sch{\"o}nfelder}, V. and {Bennett}, K. and {Bloemen}, H. and {Diehl}, R. and {Hermsen}, W. and {Lichti}, G.~G. and {van der Meulen}, R.~D. and {Ryan}, J. and {Winkler}, C.},
	Doi = {10.1038/24106},
	Journal = {\nat},
	Month = nov,
	Pages = {142-144},
	Title = {{Emission from ^{44}Ti associated with a previously unknown Galactic supernova}},
	Volume = 396,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/24106}}

@article{iyudin05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...429..225I},
	Author = {{Iyudin}, A.~F. and {Aschenbach}, B. and {Becker}, W. and {Dennerl}, K. and {Haberl}, F.},
	Doi = {10.1051/0004-6361:20041779},
	Eprint = {arXiv:astro-ph/0410372},
	Journal = {\aap},
	Keywords = {nuclear reactions, nucleosynthesis, abundances, stars: supernovae: general, ISM: individual, objects: RX J0852.0-4622, ISM: supernova remnants, gamma-rays: observations, X-rays: ISM},
	Month = jan,
	Pages = {225-234},
	Title = {{XMM-Newton observations of the supernova remnant RX J0852.0-4622/GRO J0852-4642}},
	Volume = 429,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041779}}

@article{jackson06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..163..145J},
	Author = {{Jackson}, J.~M. and {Rathborne}, J.~M. and {Shah}, R.~Y. and {Simon}, R. and {Bania}, T.~M. and {Clemens}, D.~P. and {Chambers}, E.~T. and {Johnson}, A.~M. and {Dormody}, M. and {Lavoie}, R. and {Heyer}, M.~H.},
	Doi = {10.1086/500091},
	Eprint = {arXiv:astro-ph/0602160},
	Journal = {\apjs},
	Keywords = {Galaxy: Kinematics and Dynamics, ISM: Clouds, ISM: Molecules, Radio Lines: General, Surveys},
	Month = mar,
	Pages = {145-159},
	Title = {{The Boston University-Five College Radio Astronomy Observatory Galactic Ring Survey}},
	Volume = 163,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500091}}

@inproceedings{jahoda96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996SPIE.2808...59J},
	Author = {{Jahoda}, K. and {Swank}, J.~H. and {Giles}, A.~B. and {Stark}, M.~J. and {Strohmayer}, T. and {Zhang}, W. and {Morgan}, E.~H.},
	Booktitle = {EUV, X-Ray, and Gamma-Ray Instrumentation for Astronomy VII.},
	Editor = {{Siegmund}, O.~H.~W. and {Gummin}, M.~A.},
	Month = oct,
	Pages = {59-70},
	Series = {SPIE Conference Series, Bellingham WA},
	Title = {{In-orbit performance and calibration of the Rossi X-ray Timing Explorer (RXTE) Proportional Counter Array (PCA)}},
	Volume = 2808,
	Year = 1996}

@article{jahoda06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..163..401J},
	Author = {{Jahoda}, K. and {Markwardt}, C.~B. and {Radeva}, Y. and {Rots}, A.~H. and {Stark}, M.~J. and {Swank}, J.~H. and {Strohmayer}, T.~E. and {Zhang}, W.},
	Doi = {10.1086/500659},
	Eprint = {arXiv:astro-ph/0511531},
	Journal = {\apjs},
	Keywords = {Instrumentation: Detectors, Space Vehicles: Instruments},
	Month = apr,
	Pages = {401-423},
	Title = {{Calibration of the Rossi X-Ray Timing Explorer Proportional Counter Array}},
	Volume = 163,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500659}}

@article{james75,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1975CoPhC..10..343J},
	Author = {{James}, F. and {Roos}, M.},
	Doi = {10.1016/0010-4655(75)90039-9},
	Journal = {Computer Physics Communications},
	Month = dec,
	Pages = {343-367},
	Title = {{Minuit - a system for function minimization and analysis of the parameter errors and correlations}},
	Volume = 10,
	Year = 1975,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/0010-4655(75)90039-9}}

@article{james04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...414...23J},
	Author = {{James}, P.~A. and {Shane}, N.~S. and {Beckman}, J.~E. and {Cardwell}, A. and {Collins}, C.~A. and {Etherton}, J. and {de Jong}, R.~S. and {Fathi}, K. and {Knapen}, J.~H. and {Peletier}, R.~F. and {Percival}, S.~M. and {Pollacco}, D.~L. and {Seigar}, M.~S. and {Stedman}, S. and {Steele}, I.~A.},
	Doi = {10.1051/0004-6361:20031568},
	Eprint = {astro-ph/0311030},
	Journal = {\aap},
	Keywords = {galaxies: general, galaxies: spiral, galaxies: irregular, galaxies: fundamental parameters, galaxies: photometry, galaxies: statistics},
	Month = jan,
	Pages = {23-43},
	Title = {{The H{$\alpha$} galaxy survey. I. The galaxy sample, H{$\alpha$} narrow-band observations and star formation parameters for 334 galaxies}},
	Volume = 414,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031568}}

@article{jansen01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001A%26A...365L...1J&db_key=AST},
	Author = {{Jansen}, F. and {Lumb}, D. and {Altieri}, B. and {Clavel}, J. and {Ehle}, M. and {Erd}, C. and {Gabriel}, C. and {Guainazzi}, M. and {Gondoin}, P. and {Much}, R. and {Munoz}, R. and {Santos}, M. and {Schartel}, N. and {Texier}, D. and {Vacanti}, G.},
	Journal = {\aap},
	Month = jan,
	Pages = {L1-L6},
	Title = {{XMM-Newton observatory. I. The spacecraft and operations}},
	Volume = 365,
	Year = 2001}

@book{jaschek87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987clst.book.....J},
	Author = {{Jaschek}, C. and {Jaschek}, M.},
	Keywords = {SPECTRAL CLASSIFICATION, PHOTOMETRIC SYSTEMS, SPECTRAL TYPES},
	Publisher = {Cambridge: University Press, 1987},
	Title = {{The classification of stars}},
	Year = 1987}
	
@ARTICLE{johnson66,
       author = {{Johnson}, Harold L.},
        title = "{Astronomical Measurements in the Infrared}",
      journal = {\araa},
         year = "1966",
        month = "Jan",
       volume = {4},
        pages = {193},
          doi = {10.1146/annurev.aa.04.090166.001205},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1966ARA&A...4..193J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{johnston92,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...387L..37J},
	Author = {{Johnston}, S. and {Manchester}, R.~N. and {Lyne}, A.~G. and {Bailes}, M. and {Kaspi}, V.~M. and {Qiao}, G. and {D'Amico}, N.},
	Doi = {10.1086/186300},
	Journal = {\apjl},
	Month = mar,
	Pages = {L37-L41},
	Title = {{PSR 1259-63 - A binary radio pulsar with a Be star companion}},
	Volume = 387,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/186300}}

@article{johnston94,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.268..430J},
	Author = {{Johnston}, S. and {Manchester}, R.~N. and {Lyne}, A.~G. and {Nicastro}, L. and {Spyromilio}, J.},
	Journal = {\mnras},
	Month = may,
	Pages = {430},
	Title = {{Radio and Optical Observations of the PSR:B1259-63 / SS:2883 Be-Star Binary System}},
	Volume = 268,
	Year = 1994}

@article{jonker01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553L..43J},
	Author = {{Jonker}, P.~G. and {van der Klis}, M.},
	Doi = {10.1086/320510},
	Eprint = {astro-ph/0104356},
	Journal = {\apjl},
	Keywords = {Accretion, Accretion Disks, Stars: Pulsars: Individual: Alphanumeric: 2A 1822-371, Stars: Binaries: Eclipsing, Stars: Neutron, X-Rays: Stars},
	Month = may,
	Pages = {L43-L46},
	Title = {{Discovery of an X-Ray Pulsar in the Low-Mass X-Ray Binary 2A 1822-371}},
	Volume = 553,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320510}}

@ARTICLE{jonker13,
       author = {{Jonker}, P.~G. and {Glennie}, A. and {Heida}, M. and {Maccarone}, T. and {Hodgkin}, S. and {Nelemans}, G. and {Miller-Jones}, J.~C.~A. and {Torres}, M.~A.~P. and {Fender}, R.},
        title = "{Discovery of a New Kind of Explosive X-Ray Transient near M86}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: individual: M86, galaxies: interactions, X-rays: individual: XRT 000519, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = dec,
       volume = {779},
       number = {1},
          eid = {14},
        pages = {14},
          doi = {10.1088/0004-637X/779/1/14},
archivePrefix = {arXiv},
       eprint = {1310.7238},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...779...14J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{joseph15,
       author = {{Joseph}, T.~D. and {Maccarone}, T.~J. and {Kraft}, R.~P. and
         {Sivakoff}, G.~R.},
        title = "{Deep Chandra observations of the NGC 4472 globular cluster black hole XMMU 122939.7+075333: short-term variability from the first globular cluster black hole binary}",
      journal = {\mnras},
     keywords = {galaxies: individual: NGC 4472, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = feb,
       volume = {447},
       number = {2},
        pages = {1460-1470},
          doi = {10.1093/mnras/stu2523},
archivePrefix = {arXiv},
       eprint = {1412.2919},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447.1460J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{joss84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984ARA%26A..22..537J},
	Author = {{Joss}, P.~C. and {Rappaport}, S.~A.},
	Doi = {10.1146/annurev.aa.22.090184.002541},
	Journal = {\araa},
	Pages = {537-592},
	Title = {{Neutron Stars in Interacting Binary Systems}},
	Volume = 22,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.22.090184.002541}}

@article{juett02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...568L..31J},
	Author = {{Juett}, A.~M. and {Marshall}, H.~L. and {Chakrabarty}, D. and {Schulz}, N.~S.},
	Doi = {10.1086/340273},
	Eprint = {arXiv:astro-ph/0202304},
	Journal = {\apjl},
	Month = mar,
	Pages = {L31-L34},
	Title = {{Chandra High-Resolution Spectrum of the Anomalous X-Ray Pulsar 4U 0142+61}},
	Volume = 568,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340273}}

@ARTICLE{just06,
   author = {{Just}, A. and {M{\"o}llenhoff}, C. and {Borch}, A.},
    title = "{An evolutionary disc model of the edge-on galaxy NGC 5907}",
  journal = {\aap},
 keywords = {stellar dynamics, galaxies: kinematics and dynamics, galaxies: evolution, galaxies: stellar content, galaxies: structure},
     year = 2006,
    month = dec,
   volume = 459,
    pages = {703-716},
      doi = {10.1051/0004-6361:20065701},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...459..703J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kaaret02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...578..114K},
	Author = {{Kaaret}, P.},
	Doi = {10.1086/342475},
	Eprint = {astro-ph/0206374},
	Journal = {\apj},
	Keywords = {Galaxies: Individual: Messier Number: M31, Galaxies: Individual: NGC Number: NGC 224, Galaxies: Spiral, X-Rays: Binaries, X-Rays: Galaxies, X-Rays: General},
	Month = oct,
	Pages = {114-125},
	Title = {{A Chandra High Resolution Camera Observation of X-Ray Point Sources in M31}},
	Volume = 578,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342475}}

@article{kaaret04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348L..28K},
	Author = {{Kaaret}, P. and {Alonso-Herrero}, A. and {Gallagher}, J.~S. and {Fabbiano}, G. and {Zezas}, A. and {Rieke}, M.~J.},
	Doi = {10.1111/j.1365-2966.2004.07516.x},
	Eprint = {arXiv:astro-ph/0312568},
	Journal = {\mnras},
	Keywords = {galaxies: individual: M82, galaxies: individual: NGC 1569, galaxies: individual: NGC 5253, galaxies: starburst, galaxies: stellar content, X-rays: galaxies},
	Month = feb,
	Pages = {L28-L32},
	Title = {{Displacement of X-ray sources from star clusters in starburst galaxies}},
	Volume = 348,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07516.x}}

@article{kaaret07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669..106K},
	Archiveprefix = {arXiv},
	Author = {{Kaaret}, P. and {Feng}, H.},
	Doi = {10.1086/521598},
	Eprint = {0707.2055},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Galaxies: Individual: Messier Number: M82, Galaxies: Stellar Content, X-Rays: Binaries, X-Rays: Galaxies},
	Month = nov,
	Pages = {106-108},
	Title = {{Confirmation of the 62 Day X-Ray Periodicity from M82}},
	Volume = 669,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/521598}}

@article{kaaret13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770...20K},
	Archiveprefix = {arXiv},
	Author = {{Kaaret}, P. and {Feng}, H.},
	Doi = {10.1088/0004-637X/770/1/20},
	Eid = {20},
	Eprint = {1304.6731},
	Journal = {\apj},
	Keywords = {black hole physics, galaxies: individual: blue compact dwarf I Zw 18, X-rays: binaries, X-rays: galaxies},
	Month = jun,
	Pages = {20},
	Primaryclass = {astro-ph.HE},
	Title = {{A State Transition of the Luminous X-Ray Binary in the Low-metallicity Blue Compact Dwarf Galaxy I Zw 18}},
	Volume = 770,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/770/1/20}}

@ARTICLE{kaaret17,
   author = {{Kaaret}, P. and {Feng}, H. and {Roberts}, T.~P.},
    title = "{Ultraluminous X-Ray Sources}",
  journal = {\araa},
     year = 2017,
    month = aug,
   volume = 55,
    pages = {303-341},
      doi = {10.1146/annurev-astro-091916-055259},
   adsurl = {http://adsabs.harvard.edu/abs/2017ARA%26A..55..303K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kajava09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398.1450K},
	Archiveprefix = {arXiv},
	Author = {{Kajava}, J.~J.~E. and {Poutanen}, J.},
	Doi = {10.1111/j.1365-2966.2009.15215.x},
	Eprint = {0906.1485},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , black hole physics , X-rays: binaries , X-rays: galaxies},
	Month = sep,
	Pages = {1450-1460},
	Primaryclass = {astro-ph.HE},
	Title = {{Spectral variability of ultraluminous X-ray sources}},
	Volume = 398,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15215.x}}

@article{kalberla05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...440..775K},
	Author = {{Kalberla}, P.~M.~W. and {Burton}, W.~B. and {Hartmann}, D. and {Arnal}, E.~M. and {Bajaja}, E. and {Morras}, R. and {P{\"o}ppel}, W.~G.~L.},
	Doi = {10.1051/0004-6361:20041864},
	Journal = {\aap},
	Month = sep,
	Pages = {775-782},
	Title = {{The Leiden/Argentine/Bonn (LAB) Survey of Galactic HI. Final data release of the combined LDS and IAR surveys with improved stray-radiation corrections}},
	Volume = 440,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041864}}

@article{kanbach88,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988SSRv...49...69K&db_key=AST},
	Author = {{Kanbach}, G. and {Bertsch}, D.~L. and {Fichtel}, C.~E. and {Hartman}, R.~C. and {Hunter}, S.~D. and {Kniffen}, D.~A. and {Hughlock}, B.~W. and {Favale}, A. and {Hofstadter}, R. and {Hughes}, E.~B.},
	Journal = {Space Science Reviews},
	Pages = {69-84},
	Title = {{The project EGRET (Energetic Gamma-Ray Experiment Telescope) on NASA's Gamma-Ray Observatory (GRO)}},
	Volume = 49,
	Year = 1988}

@article{kaneko10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710.1335K},
	Archiveprefix = {arXiv},
	Author = {{Kaneko}, Y. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C. and {Granot}, J. and {Ramirez-Ruiz}, E. and {van der Horst}, A.~J. and {Watts}, A.~L. and {Finger}, M.~H. and {Gehrels}, N. and {Pe'er}, A. and {van der Klis}, M. and {von Kienlin}, A. and {Wachter}, S. and {Wilson-Hodge}, C.~A. and {Woods}, P.~M.},
	Doi = {10.1088/0004-637X/710/2/1335},
	Eprint = {0911.4636},
	Journal = {\apj},
	Keywords = {pulsars: individual: SGR J1550{\ndash}5418 1E 1547.0{\ndash}5408 PSR J1550-5418, stars: neutron, X-rays: bursts},
	Month = feb,
	Pages = {1335-1342},
	Primaryclass = {astro-ph.HE},
	Title = {{Magnetar Twists: Fermi/Gamma-Ray Burst Monitor Detection of SGR J1550-5418}},
	Volume = 710,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/710/2/1335}}

@article{kaplan01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...556..399K&db_key=AST},
	Author = {{Kaplan}, D.~L. and {Kulkarni}, S.~R. and {van Kerkwijk}, M.~H. and {Rothschild}, R.~E. and {Lingenfelter}, R.~L. and {Marsden}, D. and {Danner}, R. and {Murakami}, T.},
	Doi = {10.1086/323516},
	Eprint = {astro-ph/0103179},
	Journal = {\apj},
	Month = jul,
	Pages = {399-407},
	Title = {{Hubble Space Telescope Observations of SGR 0526-66: New Constraints on Accretion and Magnetar Models}},
	Volume = 556,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323516}}

@article{kaplan02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...564..935K&db_key=AST},
	Author = {{Kaplan}, D.~L. and {Fox}, D.~W. and {Kulkarni}, S.~R. and {Gotthelf}, E.~V. and {Vasisht}, G. and {Frail}, D.~A.},
	Journal = {\apj},
	Month = jan,
	Pages = {935-940},
	Title = {{Precise Chandra Localization of the Soft Gamma-Ray Repeater SGR 1806-20}},
	Volume = 564,
	Year = 2002}

@inproceedings{kaplan08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008AIPC..983..331K},
	Author = {{Kaplan}, D.~L.},
	Booktitle = {40 Years of Pulsars: Millisecond Pulsars, Magnetars and More},
	Doi = {10.1063/1.2900177},
	Editor = {{C.~Bassa, Z.~Wang, A.~Cumming, \& V.~M.~Kaspi}},
	Keywords = {neutron stars, pulsars, X-ray sources (astronomical)},
	Month = feb,
	Pages = {331-339},
	Series = {American Institute of Physics Conference Series, Melville NY},
	Title = {{Nearby, Thermally Emitting Neutron Stars}},
	Volume = 983,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2900177}}

@article{kaplan09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137..354K},
	Archiveprefix = {arXiv},
	Author = {{Kaplan}, D.~L. and {Chatterjee}, S. and {Hales}, C.~A. and {Gaensler}, B.~M. and {Slane}, P.~O.},
	Doi = {10.1088/0004-6256/137/1/354},
	Eprint = {0810.4184},
	Journal = {\aj},
	Keywords = {astrometry, pulsars: general, stars: individual: SGR 1900+14 1E2259+58.6, stars: neutron, X-rays: stars},
	Month = jan,
	Pages = {354-366},
	Title = {{Constraining the Proper Motions of Two Magnetars}},
	Volume = 137,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/137/1/354}}

@article{kvk09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705..798K},
	Archiveprefix = {arXiv},
	Author = {{Kaplan}, D.~L. and {van Kerkwijk}, M.~H.},
	Doi = {10.1088/0004-637X/705/1/798},
	Eprint = {0909.5218},
	Journal = {\apj},
	Keywords = {magnetic fields, stars: individual: RX J0806.4-4123, stars: neutron, X-rays: stars},
	Month = nov,
	Pages = {798-808},
	Primaryclass = {astro-ph.HE},
	Title = {{Constraining the Spin-down of the Nearby Isolated Neutron Star RX J0806.4-4123, and Implications for the Population of Nearby Neutron Stars}},
	Volume = 705,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/705/1/798}}

@article{kaplan12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758...64K},
	Archiveprefix = {arXiv},
	Author = {{Kaplan}, D.~L. and {Bildsten}, L. and {Steinfadt}, J.~D.~R.},
	Doi = {10.1088/0004-637X/758/1/64},
	Eid = {64},
	Eprint = {1208.6320},
	Journal = {\apj},
	Keywords = {nuclear reactions, nucleosynthesis, abundances, supernovae: individual: Type Ia, white dwarfs},
	Month = oct,
	Pages = {64},
	Primaryclass = {astro-ph.SR},
	Title = {{Orbital Evolution of Compact White Dwarf Binaries}},
	Volume = 758,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/758/1/64}}

@article{karachentsev03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...404...93K},
	Author = {{Karachentsev}, I.~D. and {Grebel}, E.~K. and {Sharina}, M.~E. and {Dolphin}, A.~E. and {Geisler}, D. and {Guhathakurta}, P. and {Hodge}, P.~W. and {Karachentseva}, V.~E. and {Sarajedini}, A. and {Seitzer}, P.},
	Doi = {10.1051/0004-6361:20030170},
	Eprint = {astro-ph/0302045},
	Journal = {\aap},
	Keywords = {galaxies: dwarf, galaxies: distances and redshifts, galaxies: kinematics and dynamics},
	Month = jun,
	Pages = {93-111},
	Title = {{Distances to nearby galaxies in Sculptor}},
	Volume = 404,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030170}}

@article{kargaltsev02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...580.1060K},
	Author = {{Kargaltsev}, O. and {Pavlov}, G.~G. and {Sanwal}, D. and {Garmire}, G.~P.},
	Doi = {10.1086/343852},
	Eprint = {arXiv:astro-ph/0207602},
	Journal = {\apj},
	Keywords = {ISM: Individual: Alphanumeric: G266.2-1.2, Stars: Neutron, ISM: Supernova Remnants, X-Rays: Individual: Alphanumeric: CXOU J085201.4-461753},
	Month = dec,
	Pages = {1060-1064},
	Title = {{The Compact Central Object in the Supernova Remnant G266.2-1.2}},
	Volume = 580,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/343852}}

@article{kargaltsev06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646.1139K},
	Author = {{Kargaltsev}, O. and {Pavlov}, G.~G. and {Garmire}, G.~P.},
	Doi = {10.1086/504837},
	Eprint = {arXiv:astro-ph/0603853},
	Journal = {\apj},
	Month = aug,
	Pages = {1139-1148},
	Title = {{X-Ray Emission from the Double Neutron Star Binary B1534+12: Powered by the Pulsar Wind?}},
	Volume = 646,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/504837}}

@inproceedings{kargaltsev08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008AIPC..983..311D},
	Author = {{Kargaltsev}, O. and {Pavlov}, G.~G.},
	Booktitle = {{Bassa} C., {Wang} Z., {Cumming} A., {Kaspi} V.~M., eds., 40 years of pulsars: Millisecond Pulsars, Magnetars and More.},
	Doi = {10.1063/1.2900173},
	Keywords = {supernova remnants, neutron stars, X-ray sources (astronomical), pulsars},
	Month = feb,
	Pages = {171},
	Series = {AIP Conference Proceedings, Melville NY},
	Title = {{Pulsar Wind Nebulae in the Chandra Era}},
	Volume = 983,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.2900173}}

@article{kargaltsev12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...26K},
	Archiveprefix = {arXiv},
	Author = {{Kargaltsev}, O. and {Kouveliotou}, C. and {Pavlov}, G.~G. and {G{\"o}{\v g}{\"u}{\c s}}, E. and {Lin}, L. and {Wachter}, S. and {Griffith}, R.~L. and {Kaneko}, Y. and {Younes}, G.},
	Doi = {10.1088/0004-637X/748/1/26},
	Eid = {26},
	Eprint = {1201.1894},
	Journal = {\apj},
	Keywords = {gamma-ray burst: individual: HESS J1834{\ndash}087, ISM: individual objects: W41, stars: neutron, X-rays: individuals: Swift J1834.9{\ndash}0846, X-rays: ISM},
	Month = mar,
	Pages = {26},
	Primaryclass = {astro-ph.HE},
	Title = {{X-Ray Observations of the New Unusual Magnetar Swift J1834.9-0846}},
	Volume = 748,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/748/1/26}}

@article{kdm12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012Sci...337..946K},
	Archiveprefix = {arXiv},
	Author = {{Kargaltsev}, O. and {Durant}, M. and {Misanovic}, Z. and {Pavlov}, G.~G.},
	Doi = {10.1126/science.1221378},
	Eprint = {1208.5400},
	Journal = {Science},
	Month = aug,
	Pages = {946-949},
	Primaryclass = {astro-ph.HE},
	Title = {{Absorption Features in the X-ray Spectrum of an Ordinary Radio Pulsar}},
	Volume = 337,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1221378}}

@ARTICLE{kdpg12,
   author = {{Kargaltsev}, O. and {Durant}, M. and {Pavlov}, G.~G. and {Garmire}, G.
	},
    title = "{Chandra Pulsar Survey (ChaPS)}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1202.3838},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, X-rays: general},
     year = 2012,
    month = aug,
   volume = 201,
      eid = {37},
    pages = {37},
      doi = {10.1088/0067-0049/201/2/37},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..201...37K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{karino16,
   author = {{Karino}, S.},
    title = "{The nature of the X-ray pulsar in M 31: An intermediate-mass X-ray binary?}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {1608.05276},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries, X-rays: individual (3XMM J004301.4+413017)},
     year = 2016,
    month = dec,
   volume = 68,
      eid = {93},
    pages = {93},
      doi = {10.1093/pasj/psw084},
   adsurl = {http://adsabs.harvard.edu/abs/2016PASJ...68...93K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kaspi95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...453..424K},
	Author = {{Kaspi}, V.~M. and {Tavani}, M. and {Nagase}, F. and {Hirayama}, M. and {Hoshino}, M. and {Aoki}, T. and {Kawai}, N. and {Arons}, J.},
	Doi = {10.1086/176403},
	Journal = {\apj},
	Month = nov,
	Pages = {424},
	Title = {{X-Ray Detection of PSR B1259-63 at Periastron}},
	Volume = 453,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/176403}}

@article{kaspi00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2000ApJ...537L..31K},
	Author = {{Kaspi}, V.~M. and {Lackey}, J.~R. and {Chakrabarty}, D.},
	Doi = {10.1086/312758},
	Eprint = {arXiv:astro-ph/0005326},
	Journal = {\apjl},
	Month = jul,
	Pages = {L31-L34},
	Title = {{A Glitch in an Anomalous X-Ray Pulsar}},
	Volume = 537,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312758}}

@incollection{kaspi01,
	Author = {{Kaspi}, V.~M.},
	Booktitle = {Astrophysical Ages and Times Scales},
	Editor = {{von Hippel}, T. and {Simpson}, C. and {Manset}, N.},
	Pages = {44-56},
	Publisher = {ASP San Francisco},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {Precision Pulsar Timing},
	Volume = 245,
	Year = {2001}}

@article{kaspi03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...588L..93K&db_key=AST},
	Author = {{Kaspi}, V.~M. and {Gavriil}, F.~P. and {Woods}, P.~M. and {Jensen}, J.~B. and {Roberts}, M.~S.~E. and {Chakrabarty}, D.},
	Journal = {\apjl},
	Month = may,
	Pages = {L93-L96},
	Title = {{A Major Soft Gamma Repeater-like Outburst and Rotation Glitch in the No-longer-so-anomalous X-Ray Pulsar 1E 2259+586}},
	Volume = 588,
	Year = 2003}

@article{kg03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...596L..71K},
	Author = {{Kaspi}, V.~M. and {Gavriil}, F.~P.},
	Doi = {10.1086/379093},
	Eprint = {arXiv:astro-ph/0307225},
	Journal = {\apjl},
	Month = oct,
	Pages = {L71-L74},
	Title = {{A Second Glitch from the ``Anomalous'' X-Ray Pulsar 1RXS J170849.0-4000910}},
	Volume = 596,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379093}}

@article{kaspi05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618L..41K},
	Author = {{Kaspi}, V.~M. and {McLaughlin}, M.~A.},
	Doi = {10.1086/427628},
	Eprint = {arXiv:astro-ph/0411615},
	Journal = {\apjl},
	Keywords = {Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: PSR J1718-3718, Stars: Neutron},
	Month = jan,
	Pages = {L41-L44},
	Title = {{Chandra X-Ray Detection of the High Magnetic Field Radio Pulsar PSR J1718-3718}},
	Volume = 618,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/427628}}

@inbook{kaspi06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006csxs.book..279K&db_key=AST},
	Author = {{Kaspi}, V.~M. and {Roberts}, M.~S.~E. and {Harding}, A.~K.},
	Month = apr,
	Pages = {279},
	Publisher = {Cambridge: Cambridge University Press},
	Title = {{in Compact stellar X-ray sources, ed. W. H. G. Levin and M. van der Klis}},
	Year = 2006}

@article{kaspi07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007Ap%26SS.308....1K},
	Author = {{Kaspi}, V.~M.},
	Doi = {10.1007/s10509-007-9309-y},
	Eprint = {arXiv:astro-ph/0610304},
	Journal = {\apss},
	Month = apr,
	Pages = {1-4},
	Title = {{Recent progress on anomalous X-ray pulsars}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9309-y}}

@article{kaspi10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010PNAS..107.7147K},
	Author = {{Kaspi}, V.~M.},
	Doi = {10.1073/pnas.1000812107},
	Journal = {Proc.~of the National Academy of Science},
	Month = apr,
	Pages = {7147-7152},
	Title = {{Grand unification of neutron stars}},
	Volume = 107,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1073/pnas.1000812107}}

@ARTICLE{kb10,
   author = {{Kaspi}, V.~M. and {Boydstun}, K.},
    title = "{On the X-Ray Spectra of Anomalous X-Ray Pulsars and Soft Gamma Repeaters}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.3847},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, stars: magnetic field, stars: neutron, X-rays: stars},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {L115-L120},
      doi = {10.1088/2041-8205/710/2/L115},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710L.115K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inProceedings{kaspi16,
   author = {{Kaspi}, V.~M. and {Kramer}, M.},
    title = "{Radio Pulsars: The Neutron Star Population {\&} Fundamental Physics}",
booktitle = {Astrophysics and Cosmology},
   series = {Proceedings of the 26th Solvay Conference on Physics},
   editor = {{Blandford}, R. and {Gross}, D. and {Sevrin}, A.},
	Publisher = {World Scientific, Singapore},
     year = 2016,
    month = jun,
    pages = {22-61},
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160207738K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaspi17,
   author = {{Kaspi}, V.~M. and {Beloborodov}, A.~M.},
    title = "{Magnetars}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1703.00068},
 primaryClass = "astro-ph.HE",
     year = 2017,
    month = aug,
   volume = 55,
    pages = {261-301},
      doi = {10.1146/annurev-astro-081915-023329},
   adsurl = {http://adsabs.harvard.edu/abs/2017ARA%26A..55..261K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kassim92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992AJ....103..943K},
	Author = {{Kassim}, N.~E.},
	Doi = {10.1086/116116},
	Journal = {\aj},
	Keywords = {MILKY WAY GALAXY, RADIO SOURCES (ASTRONOMY), SUPERNOVA REMNANTS, VERY LARGE ARRAY (VLA), ANGULAR RESOLUTION, ASTRONOMICAL CATALOGS, EMISSION SPECTRA, STELLAR LUMINOSITY},
	Month = mar,
	Pages = {943-952},
	Title = {{330 MHz VLA observations of 20 galactic supernova remnants}},
	Volume = 103,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/116116}}

@article{kato07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007PASJ...59..615K},
	Author = {{Kato}, D. and {Nagashima}, C. and {Nagayama}, T. and {Kurita}, M. and {Koerwer}, J.~F. and {Kawai}, T. and {Yamamuro}, T. and {Zenno}, T. and {Nishiyama}, S. and {Baba}, D. and {Kadowaki}, R. and {Haba}, Y. and {Hatano}, H. and {Shimizu}, H. and {Nishimura}, M. and {Nagata}, T. and {Sato}, S. and {Murai}, Y. and {Kawazu}, T. and {Nakajima}, Y. and {Nakaya}, H. and {Kandori}, R. and {Kusakabe}, N. and {Ishihara}, A. and {Kaneyasu}, N. and {Hashimoto}, J. and {Tamura}, M. and {Tanab{\'e}}, T. and {Ita}, Y. and {Matsunaga}, N. and {Nakada}, Y. and {Sugitani}, K. and {Wakamatsu}, K.-I. and {Glass}, I.~S. and {Feast}, M.~W. and {Menzies}, J.~W. and {Whitelock}, P.~A. and {Fourie}, P. and {Stoffels}, J. and {Evans}, G.~P. and {Hasegawa}, T.},
	Journal = {\pasj},
	Keywords = {catalogs, galaxies: Magellanic Clouds, infrared: stars, surveys},
	Month = jun,
	Pages = {615-641},
	Title = {{The IRSF Magellanic Clouds Point Source Catalog}},
	Volume = 59,
	Year = 2007}

@article{kaur12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..49K},
	Archiveprefix = {arXiv},
	Author = {{Kaur}, A. and {Henze}, M. and {Haberl}, F. and {Pietsch}, W. and {Greiner}, J. and {Rau}, A. and {Hartmann}, D.~H. and {Sala}, G. and {Hernanz}, M.},
	Doi = {10.1051/0004-6361/201118025},
	Eid = {A49},
	Eprint = {1109.1547},
	Journal = {\aap},
	Keywords = {X-rays: binaries, X-rays: stars, galaxies: individual: M 31},
	Month = feb,
	Pages = {A49},
	Primaryclass = {astro-ph.HE},
	Title = {{CXOM31 J004253.1+411422: the first ultraluminous X-ray transient in M 31}},
	Volume = 538,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201118025}}

@article{keller06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...642..834K},
	Author = {{Keller}, S.~C. and {Wood}, P.~R.},
	Doi = {10.1086/501115},
	Eprint = {arXiv:astro-ph/0601225},
	Journal = {\apj},
	Month = may,
	Pages = {834-841},
	Title = {{Bump Cepheids in the Magellanic Clouds: Metallicities, the Distances to the LMC and SMC, and the Pulsation-Evolution Mass Discrepancy}},
	Volume = 642,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/501115}}

@article{kennea13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770L..24K},
	Archiveprefix = {arXiv},
	Author = {{Kennea}, J.~A. and {Burrows}, D.~N. and {Kouveliotou}, C. and {Palmer}, D.~M. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kaneko}, Y. and {Evans}, P.~A. and {Degenaar}, N. and {Reynolds}, M.~T. and {Miller}, J.~M. and {Wijnands}, R. and {Mori}, K. and {Gehrels}, N.},
	Doi = {10.1088/2041-8205/770/2/L24},
	Eid = {L24},
	Eprint = {1305.2128},
	Journal = {\apjl},
	Keywords = {pulsars: general, pulsars: individual: SGR J1745-29, stars: neutron, X-rays: bursts},
	Month = jun,
	Pages = {L24},
	Primaryclass = {astro-ph.HE},
	Title = {{Swift Discovery of a New Soft Gamma Repeater, SGR J1745--29, near Sagittarius A*}},
	Volume = 770,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/770/2/L24}}

@article{kennea16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016ATel.9274....1K},
	Author = {{Kennea}, J.~A. and {Lien}, A.~Y. and {Marshall}, F.~E. and {Palmer}, D.~M. and {Roegiers}, T.~G.~R. and {Sbarufatti}, B.},
	Journal = {Astron. Tel.},
	Keywords = {Neutron Star, Transient},
	Month = jul,
	Title = {{Swift detection of a SGR burst from PSR 1119-6127}},
	Volume = 9274,
	Year = 2016}

@article{kennel84,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1984ApJ...283..694K},
	Author = {{Kennel}, C.~F. and {Coroniti}, F.~V.},
	Doi = {10.1086/162356},
	Journal = {\apj},
	Month = aug,
	Pages = {694-709},
	Title = {{Confinement of the Crab pulsar's wind by its supernova remnant}},
	Volume = 283,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/162356}}

@article{kc84,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1984ApJ...283..710K},
	Author = {{Kennel}, C.~F. and {Coroniti}, F.~V.},
	Doi = {10.1086/162357},
	Journal = {\apj},
	Month = aug,
	Pages = {710-730},
	Title = {{Magnetohydrodynamic model of Crab nebula radiation}},
	Volume = 283,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/162357}}

@article{kennicutt83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...272...54K},
	Author = {{Kennicutt}, Jr., R.~C.},
	Doi = {10.1086/161261},
	Journal = {\apj},
	Keywords = {Disk Galaxies, Galactic Evolution, Spiral Galaxies, Star Formation, Stellar Spectrophotometry, Emission Spectra, Galactic Structure, H Alpha Line, Interstellar Gas, Photoionization, Star Distribution, Star Formation Rate, Stellar Models, Ubv Spectra},
	Month = sep,
	Pages = {54-67},
	Title = {{The rate of star formation in normal disk galaxies}},
	Volume = 272,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/161261}}

@article{kennicutt87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987AJ.....93.1011K},
	Author = {{Kennicutt}, Jr., R.~C. and {Roettiger}, K.~A. and {Keel}, W.~C. and {van der Hulst}, J.~M. and {Hummel}, E.},
	Doi = {10.1086/114384},
	Journal = {\aj},
	Keywords = {GALACTIC EVOLUTION, INTERACTING GALAXIES, SPIRAL GALAXIES, STAR DISTRIBUTION, STAR FORMATION, STAR FORMATION RATE, GALACTIC STRUCTURE, H ALPHA LINE, INFRARED ASTRONOMY SATELLITE, LUMINOSITY},
	Month = may,
	Pages = {1011-1023},
	Title = {{The effects of interactions on spiral galaxies. II - Disk star-formation rates}},
	Volume = 93,
	Year = 1987,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/114384}}

@article{kennicutt94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...435...22K},
	Author = {{Kennicutt}, Jr., R.~C. and {Tamblyn}, P. and {Congdon}, C.~E.},
	Doi = {10.1086/174790},
	Journal = {\apj},
	Keywords = {Astronomical Models, Galactic Evolution, Spiral Galaxies, Star Formation, Stellar Luminosity, Time Measurement, Ultraviolet Spectra, Astronomical Photometry, H Alpha Line, Stellar Mass, Ultraviolet Astronomy},
	Month = nov,
	Pages = {22-36},
	Title = {{Past and future star formation in disk galaxies}},
	Volume = 435,
	Year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/174790}}

@ARTICLE{kern02,
   author = {{Kern}, B. and {Martin}, C.},
    title = "{Optical pulsations from the anomalous X-ray pulsar 4U0142+61}",
  journal = {\nat},
     year = 2002,
    month = may,
   volume = 417,
    pages = {527-529},
      doi = {10.1038/417527a},
   adsurl = {http://adsabs.harvard.edu/abs/2002Natur.417..527K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kim03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...584..985K},
	Author = {{Kim}, C. and {Kalogera}, V. and {Lorimer}, D.~R.},
	Doi = {10.1086/345740},
	Eprint = {astro-ph/0207408},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Close, Gravitational Waves, Stars: Neutron},
	Month = feb,
	Pages = {985-995},
	Title = {{The Probability Distribution of Binary Pulsar Coalescence Rates. I. Double Neutron Star Systems in the Galactic Field}},
	Volume = 584,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345740}}

@article{kim04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611..846K},
	Author = {{Kim}, D.-W. and {Fabbiano}, G.},
	Doi = {10.1086/422210},
	Eprint = {arXiv:astro-ph/0312104},
	Journal = {\apj},
	Keywords = {Galaxies: Elliptical and Lenticular, cD, X-Rays: Binaries, X-Rays: Galaxies},
	Month = aug,
	Pages = {846-857},
	Title = {{X-Ray Luminosity Function and Total Luminosity of Low-Mass X-Ray Binaries in Early-Type Galaxies}},
	Volume = 611,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422210}}

@article{king62,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1962AJ.....67..274K},
	Author = {{King}, I.},
	Doi = {10.1086/108714},
	Journal = {\aj},
	Month = jun,
	Pages = {274-275},
	Title = {{Density Law in Spherical Stellar Systems.}},
	Volume = 67,
	Year = 1962,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/108714}}

@article{king00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.312L..39K},
	Author = {{King}, A.~R.},
	Doi = {10.1046/j.1365-8711.2000.03328.x},
	Eprint = {arXiv:astro-ph/0002286},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, BINARIES: CLOSE, STARS: INDIVIDUAL: GRO J1655-40},
	Month = mar,
	Pages = {L39-L41},
	Title = {{Black hole transients and the Eddington limit}},
	Volume = 312,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03328.x}}

@article{king01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...552L.109K},
	Author = {{King}, A.~R. and {Davies}, M.~B. and {Ward}, M.~J. and {Fabbiano}, G. and {Elvis}, M.},
	Doi = {10.1086/320343},
	Eprint = {arXiv:astro-ph/0104333},
	Journal = {\apjl},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, X-Rays: Stars},
	Month = may,
	Pages = {L109-L112},
	Title = {{Ultraluminous X-Ray Sources in External Galaxies}},
	Volume = 552,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320343}}

@article{king09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393L..41K},
	Archiveprefix = {arXiv},
	Author = {{King}, A.~R.},
	Doi = {10.1111/j.1745-3933.2008.00594.x},
	Eprint = {0811.1473},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, binaries: close, galaxies: active, BL Lacertae objects: general, X-rays: binaries},
	Month = feb,
	Pages = {L41-L44},
	Title = {{Masses, beaming and Eddington ratios in ultraluminous X-ray sources}},
	Volume = 393,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2008.00594.x}}

@ARTICLE{king20,
       author = {{King}, Andrew},
        title = "{GSN 069 - A tidal disruption near miss}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, X-rays: galaxies, supermassive black holes, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = mar,
       volume = {493},
       number = {1},
        pages = {L120-L123},
          doi = {10.1093/mnrasl/slaa020},
archivePrefix = {arXiv},
       eprint = {2002.00970},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493L.120K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{kirsch04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004SPIE.5488..103K},
	Author = {{Kirsch}, M.~G.~F. and {Altieri}, B. and {Chen}, B. and {Haberl}, F. and {Metcalfe}, L. and {Pollock}, A.~M. and {Read}, A.~M. and {Saxton}, R.~D. and {Sembay}, S. and {Smith}, M.~J.},
	Booktitle = {UV and Gamma-Ray Space Telescope Systems. Proceedings of the SPIE. SPIE, Bellingham WA},
	Doi = {10.1117/12.549276},
	Editor = {{Hasinger}, G. and {Turner}, M.~J.~L.},
	Month = oct,
	Pages = {103},
	Title = {{XMM-Newton (cross)-calibration}},
	Volume = 5488,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.549276}}

@inproceedings{kirsch04timing,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004SPIE.5165...85K},
	Author = {{Kirsch}, M.~G.~F. and {Becker}, W. and {Benlloch-Garcia}, S. and {Jansen}, F.~A. and {Kendziorra}, E. and {Kuster}, M. and {Lammers}, U. and {Pollock}, A.~M.~T. and {Possanzini}, F. and {Serpell}, E. and {Talavera}, A.},
	Booktitle = {X-Ray and Gamma-Ray Instrumentation for Astronomy XIII. Edited by Flanagan, Kathryn A.; Siegmund, Oswald H. W. Proceedings of the SPIE. SPIE, Bellingham WA},
	Doi = {10.1117/12.503559},
	Editor = {{Flanagan}, K.~A. and {Siegmund}, O.~H.~W.},
	Month = feb,
	Pages = {85-95},
	Series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	Title = {{Timing accuracy and capabilities of XMM-Newton}},
	Volume = 5165,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.503559}}

@inproceedings{kirsch05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005SPIE.5898...22K&db_key=AST},
	Author = {{Kirsch}, M.~G. and {Briel}, U.~G. and {Burrows}, D. and {Campana}, S. and {Cusumano}, G. and {Ebisawa}, K. and {Freyberg}, M.~J. and {Guainazzi}, M. and {Haberl}, F. and {Jahoda}, K. and {Kaastra}, J. and {Kretschmar}, P. and {Larsson}, S. and {Lubinski}, P. and {Mori}, K. and {Plucinsky}, P. and {Pollock}, A.~M. and {Rothschild}, R. and {Sembay}, S. and {Wilms}, J. and {Yamamoto}, M.},
	Booktitle = {UV, X-Ray, and Gamma-Ray Space Instrumentation for Astronomy XIV. Edited by Siegmund, Oswald H. W. Proceedings of the SPIE, Volume 5898},
	Doi = {10.1117/12.616893},
	Month = aug,
	Pages = {22-33},
	Title = {{Crab: the standard x-ray candle with all (modern) x-ray satellites}},
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.616893}}

@article{klein83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...121..150K},
	Author = {{Klein}, U.},
	Journal = {\aap},
	Keywords = {CONTINUOUS SPECTRA, GALACTIC CLUSTERS, GALACTIC RADIO WAVES, HYDROGEN CLOUDS, INTERACTING GALAXIES, RADIO GALAXIES, STELLAR EVOLUTION, CENTIMETER WAVES, H ALPHA LINE, LYMAN SPECTRA, NONTHERMAL RADIATION, O STARS, PHOTON DENSITY, STAR FORMATION RATE, THERMAL EMISSION},
	Month = may,
	Pages = {150-152},
	Title = {{Observations of the interacting galaxy pair NGC 4490/85}},
	Volume = 121,
	Year = 1983}

@article{kniffen97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...486..126K&db_key=AST},
	Author = {{Kniffen}, D.~A. and {Alberts}, W.~C.~K. and {Bertsch}, D.~L. and {Dingus}, B.~L. and {Esposito}, J.~A. and {Fichtel}, C.~E. and {Foster}, R.~S. and {Hartman}, R.~C. and {Hunter}, S.~D. and {Kanbach}, G. and {Lin}, Y.~C. and {Mattox}, J.~R. and {Mayer-Hasselwander}, H.~A. and {Michelson}, P.~F. and {von Montigny}, C. and {Mukherjee}, R. and {Nolan}, P.~L. and {Paredes}, J.~M. and {Ray}, P.~S. and {Schneid}, E.~J. and {Sreekumar}, P. and {Tavani}, M. and {Thompson}, D.~J.},
	Doi = {10.1086/304490},
	Journal = {\apj},
	Month = sep,
	Pages = {126},
	Title = {{EGRET Observations of the Gamma-Ray Source 2CG 135+01}},
	Volume = 486,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/304490}}

@article{knigge06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.373..484K},
	Author = {{Knigge}, C.},
	Doi = {10.1111/j.1365-2966.2006.11096.x},
	Eprint = {astro-ph/0609671},
	Journal = {\mnras},
	Keywords = {accretion, accretion disks, stars: distances, stars: fundamental parameters, novae, cataclysmic variables},
	Month = dec,
	Pages = {484-502},
	Title = {{The donor stars of cataclysmic variables}},
	Volume = 373,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.11096.x}}

@article{knigge11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..194...28K},
	Archiveprefix = {arXiv},
	Author = {{Knigge}, C. and {Baraffe}, I. and {Patterson}, J.},
	Doi = {10.1088/0067-0049/194/2/28},
	Eid = {28},
	Eprint = {1102.2440},
	Journal = {\apjs},
	Keywords = {novae, cataclysmic variables, stars: fundamental parameters},
	Month = jun,
	Pages = {28},
	Primaryclass = {astro-ph.SR},
	Title = {{The Evolution of Cataclysmic Variables as Revealed by Their Donor Stars}},
	Volume = 194,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/194/2/28}}

@article{kokubun07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2007PASJ...59S..53K&db_key=AST},
	Author = {{Kokubun}, M. and {Makishima}, K. and {Takahashi}, T. and {Murakami}, T. and {Tashiro}, M. and {Fukazawa}, Y. and {Kamae}, T. and {Madejski}, G.~M. and {Nakazawa}, K. and {Yamaoka}, K. and {Terada}, Y. and {Yonetoku}, D. and {Watanabe}, S. and {Tamagawa}, T. and {Mizuno}, T. and {Kubota}, A. and {Isobe}, N. and {Takahashi}, I. and {Sato}, G. and {Takahashi}, H. and {Hong}, S. and {Kawaharada}, M. and {Kawano}, N. and {Mitani}, T. and {Murashima}, M. and {Suzuki}, M. and {Abe}, K. and {Miyawaki}, R. and {Ohno}, M. and {Tanaka}, T. and {Yanagida}, T. and {Itoh}, T. and {Ohnuki}, K. and {Tamura}, K.-I. and {Endo}, Y. and {Hirakuri}, S. and {Hiruta}, T. and {Kitaguchi}, T. and {Kishishita}, T. and {Sugita}, S. and {Takahashi}, T. and {Takeda}, S. and {Enoto}, T. and {Hirasawa}, A. and {Katsuta}, J. and {Matsumura}, S. and {Onda}, K. and {Sato}, M. and {Ushio}, M. and {Ishikawa}, S.-N. and {Murase}, K. and {Odaka}, H. and {Suzuki}, M. and {Yaji}, Y. and {Yamada}, S. and {Yamasaki}, T. and {Yuasa}, T. and {The Hxd Team}},
	Eprint = {astro-ph/0611233},
	Journal = {\pasj},
	Month = jan,
	Pages = {53-76},
	Title = {{In-Orbit Performance of the Hard X-Ray Detector on Board Suzaku}},
	Volume = 59,
	Year = 2007}

@article{komissarov07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1029K},
	Archiveprefix = {arXiv},
	Author = {{Komissarov}, S.~S. and {Barkov}, M.~V.},
	Doi = {10.1111/j.1365-2966.2007.12485.x},
	Eprint = {0707.0264},
	Journal = {\mnras},
	Keywords = {MHD, relativity, methods: numerical, stars: neutron, supernovae: general, gamma-rays: bursts},
	Month = dec,
	Pages = {1029-1040},
	Title = {{Magnetar-energized supernova explosions and gamma-ray burst jets}},
	Volume = 382,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12485.x}}
	
@ARTICLE{kong03,
       author = {{Kong}, A.~K.~H. and {Di Stefano}, R.},
        title = "{A Luminous Recurrent Supersoft X-Ray Source in NGC 300}",
      journal = {\apjl},
     keywords = {Galaxies: Individual: NGC Number: NGC 300, X-Rays: Binaries, X-Rays: Galaxies, Astrophysics},
         year = "2003",
        month = "Jun",
       volume = {590},
       number = {1},
        pages = {L13-L16},
          doi = {10.1086/376552},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304510},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...590L..13K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kong04,
   author = {{Kong}, A.~K.~H. and {Di Stefano}, R. and {Yuan}, F.},
    title = "{Evidence of an Intermediate-Mass Black Hole: Chandra and XMM-Newton Observations of the Ultraluminous Supersoft X-Ray Source in M101 during Its 2004 Outburst}",
  journal = {\apjl},
   eprint = {astro-ph/0410671},
 keywords = {Black Hole Physics, Galaxies: Individual: Messier Number: M101, X-Rays: Binaries, X-Rays: Galaxies},
     year = 2004,
    month = dec,
   volume = 617,
    pages = {L49-L52},
      doi = {10.1086/427025},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...617L..49K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kosec18,
   author = {{Kosec}, P. and {Pinto}, C. and {Walton}, D.~J. and {Fabian}, A.~C. and 
	{Bachetti}, M. and {Brightman}, M. and {F{\"u}rst}, F. and {Grefenstette}, B.~W.
	},
    title = "{Evidence for a variable Ultrafast Outflow in the newly discovered Ultraluminous Pulsar NGC 300 ULX-1}",
  journal = {\mnras},
 keywords = {accretion, accretion discs, stars: neutron, X-rays:binaries, X-rays: individual: NGC 300 ULX-1},
     year = 2018,
    month = sep,
   volume = 479,
    pages = {3978-3986},
      doi = {10.1093/mnras/sty1626},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.479.3978K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kosugi05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...623L.125K},
	Author = {{Kosugi}, G. and {Ogasawara}, R. and {Terada}, H.},
	Doi = {10.1086/430171},
	Eprint = {arXiv:astro-ph/0503280},
	Journal = {\apjl},
	Month = apr,
	Pages = {L125-L128},
	Title = {{A Variable Infrared Counterpart to the Soft Gamma-Ray Repeater SGR 1806-20}},
	Volume = 623,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430171}}

@article{kouveliotou93,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1993Natur.362..728K&db_key=AST},
	Author = {{Kouveliotou}, C. and {Fishman}, G.~J. and {Meegan}, C.~A. and {Paciesas}, W.~S. and {Wilson}, R.~B. and {van Paradijs}, J. and {Preece}, R.~D. and {Briggs}, M.~S. and {Pendleton}, G.~N. and {Brock}, M.~N.},
	Journal = {\nat},
	Month = apr,
	Pages = {728-730},
	Title = {{Recurrent burst activity from the soft gamma-ray repeater SGR 1900 + 14}},
	Volume = 362,
	Year = 1993}

@article{kouveliotou98_1627,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998IAUC.6944....2K&db_key=AST},
	Author = {{Kouveliotou}, C. and {Kippen}, M. and {Woods}, P. and {Richardson}, G. and {Connaughton}, V. and {McCollough}, M.},
	Journal = {\iaucirc},
	Month = jun,
	Pages = {2},
	Title = {{SGR 1627-41}},
	Volume = 6944,
	Year = 1998}

@article{kouveliotou99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...510L.115K&db_key=AST},
	Author = {{Kouveliotou}, C. and {Strohmayer}, T. and {Hurley}, K. and {van Paradijs}, J. and {Finger}, M.~H. and {Dieters}, S. and {Woods}, P. and {Thompson}, C. and {Duncan}, R.~C.},
	Journal = {\apjl},
	Month = jan,
	Pages = {L115-L118},
	Title = {{Discovery of a Magnetar Associated with the Soft Gamma Repeater SGR 1900+14}},
	Volume = 510,
	Year = 1999}

@article{kouveliotou01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...558L..47K&db_key=AST},
	Author = {{Kouveliotou}, C. and {Tennant}, A. and {Woods}, P.~M. and {Weisskopf}, M.~C. and {Hurley}, K. and {Fender}, R.~P. and {Garrington}, S.~T. and {Patel}, S.~K. and {G{\"o}{\u g}{\"u}{\c s}}, E.},
	Journal = {\apjl},
	Month = sep,
	Pages = {L47-L50},
	Title = {{Multiwavelength Observations of the Soft Gamma Repeater SGR 1900+14 during Its 2001 April Activation}},
	Volume = 558,
	Year = 2001}

@article{kouveliotou03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...596L..79K&db_key=AST},
	Author = {{Kouveliotou}, C. and {Eichler}, D. and {Woods}, P.~M. and {Lyubarsky}, Y. and {Patel}, S.~K. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {van der Klis}, M. and {Tennant}, A. and {Wachter}, S. and {Hurley}, K.},
	Journal = {\apjl},
	Month = oct,
	Pages = {L79-L82},
	Title = {{Unraveling the Cooling Trend of the Soft Gamma Repeater SGR 1627-41}},
	Volume = 596,
	Year = 2003}

@article{koyama97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997PASJ...49L...7K},
	Author = {{Koyama}, K. and {Kinugasa}, K. and {Matsuzaki}, K. and {Nishiuchi}, M. and {Sugizaki}, M. and {Torii}, K. and {Yamauchi}, S. and {Aschenbach}, B.},
	Eprint = {arXiv:astro-ph/9704140},
	Journal = {\pasj},
	Keywords = {INTERSTELLAR : INDIVIDUAL (RX J17137-3946), RADIATION MECHANISM, SUPERNOVA REMNANTS, X-RAYS: SOURCES, X-RAYS: SPECTRA},
	Month = jun,
	Pages = {L7-L11},
	Title = {{Discovery of Non-Thermal X-Rays from the Northwest Shell of the New SNR RX J1713.7-3946: The Second SN 1006?}},
	Volume = 49,
	Year = 1997}

@article{koyama07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2007PASJ...59S..23K&db_key=AST},
	Author = {{Koyama}, K. and {Tsunemi}, H. and {Dotani}, T. and {Bautz}, M.~W. and {Hayashida}, K. and {Tsuru}, T.~G. and {Matsumoto}, H. and {Ogawara}, Y. and {Ricker}, G.~R. and {Doty}, J. and {Kissel}, S.~E. and {Foster}, R. and {Nakajima}, H. and {Yamaguchi}, H. and {Mori}, H. and {Sakano}, M. and {Hamaguchi}, K. and {Nishiuchi}, M. and {Miyata}, E. and {Torii}, K. and {Namiki}, M. and {Katsuda}, S. and {Matsuura}, D. and {Miyauchi}, T. and {Anabuki}, N. and {Tawa}, N. and {Ozaki}, M. and {Murakami}, H. and {Maeda}, Y. and {Ichikawa}, Y. and {Prigozhin}, G.~Y. and {Boughan}, E.~A. and {Lamarr}, B. and {Miller}, E.~D. and {Burke}, B.~E. and {Gregory}, J.~A. and {Pillsbury}, A. and {Bamba}, A. and {Hiraga}, J.~S. and {Senda}, A. and {Katayama}, H. and {Kitamoto}, S. and {Tsujimoto}, M. and {Kohmura}, T. and {Tsuboi}, Y. and {Awaki}, H.},
	Journal = {\pasj},
	Month = jan,
	Pages = {23-33},
	Title = {{X-Ray Imaging Spectrometer (XIS) on Board Suzaku}},
	Volume = 59,
	Year = 2007}

@ARTICLE{Kozai62,
       author = {{Kozai}, Yoshihide},
        title = "{Secular perturbations of asteroids with high inclination and eccentricity}",
      journal = {\aj},
         year = 1962,
        month = nov,
       volume = {67},
        pages = {591-598},
          doi = {10.1086/108790},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1962AJ.....67..591K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kraft91,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...374..344K},
	Author = {{Kraft}, R.~P. and {Burrows}, D.~N. and {Nousek}, J.~A.},
	Doi = {10.1086/170124},
	Journal = {\apj},
	Keywords = {BAYES THEOREM, CONFIDENCE LIMITS, PHOTON DENSITY, POISSON DENSITY FUNCTIONS, SUPERNOVA 1987A, CHARGE COUPLED DEVICES, ERROR ANALYSIS, GAMMA RAY ASTRONOMY, PROBABILITY DISTRIBUTION FUNCTIONS},
	Month = jun,
	Pages = {344-355},
	Title = {{Determination of confidence limits for experiments with low numbers of counts}},
	Volume = 374,
	Year = 1991,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/170124}}

@article{kramer06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006Sci...314...97K},
	Author = {{Kramer}, M. and {Stairs}, I.~H. and {Manchester}, R.~N. and {McLaughlin}, M.~A. and {Lyne}, A.~G. and {Ferdman}, R.~D. and {Burgay}, M. and {Lorimer}, D.~R. and {Possenti}, A. and {D'Amico}, N. and {Sarkissian}, J.~M. and {Hobbs}, G.~B. and {Reynolds}, J.~E. and {Freire}, P.~C.~C. and {Camilo}, F.},
	Doi = {10.1126/science.1132305},
	Eprint = {arXiv:astro-ph/0609417},
	Journal = {Science},
	Month = oct,
	Pages = {97-102},
	Title = {{Tests of General Relativity from Timing the Double Pulsar}},
	Volume = 314,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1132305}}

@article{kramer07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.377..107K},
	Author = {{Kramer}, M. and {Stappers}, B.~W. and {Jessner}, A. and {Lyne}, A.~G. and {Jordan}, C.~A.},
	Doi = {10.1111/j.1365-2966.2007.11622.x},
	Eprint = {arXiv:astro-ph/0702365},
	Journal = {\mnras},
	Keywords = {polarization , radiation mechanisms: non-thermal , stars: individual: AXPJ1810-197 , stars: neutron , pulsars: general},
	Month = may,
	Pages = {107-119},
	Title = {{Polarized radio emission from a magnetar}},
	Volume = 377,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11622.x}}

@article{krause05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005Sci...308.1604K},
	Author = {{Krause}, O. and {Rieke}, G.~H. and {Birkmann}, S.~M. and {Le Floc'h}, E. and {Gordon}, K.~D. and {Egami}, E. and {Bieging}, J. and {Hughes}, J.~P. and {Young}, E.~T. and {Hinz}, J.~L. and {Quanz}, S.~P. and {Hines}, D.~C.},
	Doi = {10.1126/science.1112035},
	Eprint = {arXiv:astro-ph/0506186},
	Journal = {Science},
	Month = jun,
	Pages = {1604-1606},
	Title = {{Infrared Echoes near the Supernova Remnant Cassiopeia A}},
	Volume = 308,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1112035}}

@article{krautter99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1999A%26A...350..743K},
	Author = {{Krautter}, J. and {Zickgraf}, F.-J. and {Appenzeller}, I. and {Thiering}, I. and {Voges}, W. and {Chavarria}, C. and {Kneer}, R. and {Mujica}, R. and {Pakull}, M.~W. and {Serrano}, A. and {Ziegler}, B.},
	Eprint = {arXiv:astro-ph/9910514},
	Journal = {\aap},
	Month = oct,
	Pages = {743-752},
	Title = {{Identification of a complete sample of northern ROSAT All-Sky Survey X-ray sources. IV. Statistical analysis}},
	Volume = 350,
	Year = 1999}

@inproceedings{kretschmar04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ESASP.552..329K},
	Author = {{Kretschmar}, P. and {Wilms}, J. and {Staubert}, R. and {Kreykenbohm}, I. and {Heindl}, W.~A.},
	Booktitle = {ESA Special Publication},
	Editor = {{Schoenfelder}, V. and {Lichti}, G. and {Winkler}, C.},
	Month = oct,
	Pages = {329},
	Title = {{XMM-Newton Observations of the Be/X-Ray Transient A0538-66 in Quiescence}},
	Volume = 552,
	Year = 2004}

@inproceedings{kretschmar12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012int..workE..16K},
	Archiveprefix = {arXiv},
	Author = {{Kretschmar}, P. and {Nespoli}, E. and {Reig}, P. and {Anders}, F.},
	Booktitle = {An INTEGRAL view of the high-energy sky (the first 10 years)},
	Editor = {{Lebrun}, F. and {Goldwurm}, A. and {Winkler}, C.},
	Eid = {16},
	Eprint = {1302.3434},
	Pages = {16},
	Primaryclass = {astro-ph.HE},
	Publisher = {Proc. Sci.},
	Title = {{The Be X-ray Binary Outburst Zoo}},
	Volume = 176,
	Year = 2012}

@article{kreykenbohm99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...341..141K},
	Author = {{Kreykenbohm}, I. and {Kretschmar}, P. and {Wilms}, J. and {Staubert}, R. and {Kendziorra}, E. and {Gruber}, D.~E. and {Heindl}, W.~A. and {Rothschild}, R.~E.},
	Eprint = {astro-ph/9810282},
	Journal = {\aap},
	Keywords = {X-RAYS: STARS, STARS: MAGNETIC FIELDS, STARS: NEUTRON, STARS: PULSARS: INDIVIDUAL: VELA X-1},
	Month = jan,
	Pages = {141-150},
	Title = {{VELA X-1 as seen by RXTE}},
	Volume = 341,
	Year = 1999}

@article{kreykenbohm08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...492..511K},
	Archiveprefix = {arXiv},
	Author = {{Kreykenbohm}, I. and {Wilms}, J. and {Kretschmar}, P. and {Torrej{\'o}n}, J.~M. and {Pottschmidt}, K. and {Hanke}, M. and {Santangelo}, A. and {Ferrigno}, C. and {Staubert}, R.},
	Doi = {10.1051/0004-6361:200809956},
	Eprint = {0810.2981},
	Journal = {\aap},
	Keywords = {X-rays: stars, stars: flare, stars:, pulsars: individual: Vela X-1, stars: magnetic fields},
	Month = dec,
	Pages = {511-525},
	Title = {{High variability in Vela X-1: giant flares and off states}},
	Volume = 492,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200809956}}

@article{krimm08_gcn8311,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008GCN..8311....1K},
	Author = {{Krimm}, H.~A. and {Beardmore}, A.~P. and {Burrows}, D.~N. and {Capalbi}, M. and {Evans}, P.~A. and {Gehrels}, N. and {Godet}, O. and {Guidorzi}, C. and {}et~al.},
	Journal = {GRB Coordinates Network},
	Pages = {1},
	Title = {{Trigger 330353: Swift detection of a galactic short soft burst.}},
	Volume = 8311,
	Year = 2008}

@article{krimm08_gcn8312,
	Author = {{Krimm}, H.~A. and {Beardmore}, A.~P. and {Gehrels}, N. and {Page}, K.~L. and {Palmer}, D.~M. and {Starling}, R.~L.~C. and {Ukwatta}, T.~N.},
	Journal = {GCN Circ.},
	Title = {{Swift discovery of a new Soft Gamma Repeater SGR 1550-5418}},
	Volume = 8312,
	Year = 2008}

@article{krivonos12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A..27K},
	Archiveprefix = {arXiv},
	Author = {{Krivonos}, R. and {Tsygankov}, S. and {Lutovinov}, A. and {Revnivtsev}, M. and {Churazov}, E. and {Sunyaev}, R.},
	Doi = {10.1051/0004-6361/201219617},
	Eid = {A27},
	Eprint = {1205.3941},
	Journal = {\aap},
	Keywords = {surveys, X-rays: general, catalogs},
	Month = sep,
	Pages = {A27},
	Primaryclass = {astro-ph.IM},
	Title = {{INTEGRAL/IBIS nine-year Galactic hard X-ray survey}},
	Volume = 545,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201219617}}

@book{krolik98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998agn..book.....K&db_key=AST},
	Author = {{Krolik}, J.~H.},
	Publisher = {Princeton: Princeton University Press},
	Title = {{Active Galactic Nuclei: From the Central Black Hole to the Galactic Environment}},
	Year = 1998}

@article{kubo04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004NewAR..48..323K&db_key=AST},
	Author = {{Kubo}, H. and {Asahara}, A. and {Bicknell}, G.~V. and {Clay}, R.~W. and {Doi}, Y. and {Edwards}, P.~G. and {Enomoto}, R. and {Gunji}, S. and {Hara}, S. and {Hara}, T. and {Hattori}, T. and {Hayashi}, S. and {Itoh}, C. and {Kabuki}, S. and {Kajino}, F. and {Katagiri}, H. and {Kawachi}, A. and {Kifune}, T. and {Ksenofontov}, L.~T. and {Kurihara}, T. and {Kurosaka}, R. and {Kushida}, J. and {Matsubara}, Y. and {Miyashita}, Y. and {Mizumoto}, Y. and {Mori}, M. and {Moro}, H. and {Muraishi}, H. and {Muraki}, Y. and {Naito}, T. and {Nakase}, T. and {Nishida}, D. and {Nishijima}, K. and {Ohishi}, M. and {Okumura}, K. and {Patterson}, J.~R. and {Protheroe}, R.~J. and {Sakamoto}, N. and {Sakurazawa}, K. and {Swaby}, D.~L. and {Tanimori}, T. and {Tanimura}, H. and {Thornton}, G. and {Tokanai}, F. and {Tsuchiya}, K. and {Uchida}, T. and {Watanabe}, S. and {Yamaoka}, T. and {Yanagita}, S. and {Yoshida}, T. and {Yoshikoshi}, T.},
	Doi = {10.1016/j.newar.2003.12.002},
	Journal = {New Astronomy Review},
	Month = apr,
	Pages = {323-329},
	Title = {{Status of the CANGAROO-III project}},
	Volume = 48,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.newar.2003.12.002}}

@article{kubota04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353..980K},
	Author = {{Kubota}, A. and {Done}, C.},
	Doi = {10.1111/j.1365-2966.2004.08134.x},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: individual: XTE J1550: 564},
	Month = sep,
	Pages = {980-990},
	Title = {{The very high state accretion disc structure from the Galactic black hole transient XTE J1550 - 564}},
	Volume = 353,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08134.x}}

@article{kudritzki00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ARA%26A..38..613K},
	Author = {{Kudritzki}, R.-P. and {Puls}, J.},
	Doi = {10.1146/annurev.astro.38.1.613},
	Journal = {\araa},
	Keywords = {MASS LOSS, STELLAR WINDS, MASSIVE STARS, CENTRAL STARS OF PLANETARY NEBULAE, STELLAR EVOLUTION},
	Pages = {613-666},
	Title = {{Winds from Hot Stars}},
	Volume = 38,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.38.1.613}}

@article{kuijken11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011Msngr.146....8K},
	Author = {{Kuijken}, K.},
	Journal = {The Messenger},
	Month = dec,
	Pages = {8-11},
	Title = {{OmegaCAM: ESO's Newest Imager}},
	Volume = 146,
	Year = 2011}

@article{kuiper02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...577..917K},
	Author = {{Kuiper}, L. and {Hermsen}, W. and {Verbunt}, F. and {Ord}, S. and {Stairs}, I. and {Lyne}, A.},
	Doi = {10.1086/342220},
	Eprint = {arXiv:astro-ph/0206081},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: PSR J0218+4232, X-Rays: Stars},
	Month = oct,
	Pages = {917-922},
	Title = {{High-Resolution Spatial and Timing Observations of Millisecond Pulsar PSR J0218+4232 with Chandra}},
	Volume = 577,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342220}}

@article{kuiper03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003A%26A...411L..31K&db_key=AST},
	Author = {{Kuiper}, L. and {Hermsen}, W. and {Walter}, R. and {Foschini}, L.},
	Journal = {\aap},
	Month = nov,
	Pages = {L31-L36},
	Title = {{Absolute timing with IBIS, SPI and JEM-X aboard INTEGRAL. Crab main-pulse arrival times in radio, X-rays and high-energy gamma -rays}},
	Volume = 411,
	Year = 2003}

@article{kuiper04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...613.1173K&db_key=AST},
	Author = {{Kuiper}, L. and {Hermsen}, W. and {Mendez}, M.},
	Doi = {10.1086/423129},
	Journal = {\apj},
	Month = oct,
	Pages = {1173-1178},
	Title = {{Discovery of Hard Nonthermal Pulsed X-Ray Emission from the Anomalous X-Ray Pulsar 1E 1841-045}},
	Volume = 613,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423129}}

@article{kuiper09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2151....1K},
	Author = {{Kuiper}, L. and {Hermsen}, W.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Soft Gamma-ray Repeaters, Transients},
	Month = aug,
	Title = {{RXTE timing observations of SGR 0418+5729}},
	Volume = 2151,
	Year = 2009}

@article{kuiper11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3577....1K},
	Author = {{Kuiper}, L. and {Hermsen}, W.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Gamma Ray, Neutron Star, Soft Gamma-ray Repeater, Transient, Pulsar},
	Month = aug,
	Title = {{The spin-down of Swift J1834.9-0846: confirmation as magnetar}},
	Volume = 3577,
	Year = 2011}

@article{kulkarni93,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1993Natur.365...33K&db_key=AST},
	Author = {{Kulkarni}, S.~R. and {Frail}, D.~A.},
	Journal = {\nat},
	Month = sep,
	Pages = {33-35},
	Title = {{Identification of a supernova remnant coincident with the soft gamma-ray repeater SGR1806-20}},
	Volume = 365,
	Year = 1993}

@article{kulkarni03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...585..948K&db_key=AST},
	Author = {{Kulkarni}, S.~R. and {Kaplan}, D.~L. and {Marshall}, H.~L. and {Frail}, D.~A. and {Murakami}, T. and {Yonetoku}, D.},
	Journal = {\apj},
	Month = mar,
	Pages = {948-954},
	Title = {{The Quiescent Counterpart of the Soft Gamma-Ray Repeater SGR 0526-66}},
	Volume = 585,
	Year = 2003}

@article{kuulkers13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A..32K},
	Archiveprefix = {arXiv},
	Author = {{Kuulkers}, E. and {Kouveliotou}, C. and {Belloni}, T. and {Cadolle Bel}, M. and {Chenevez}, J. and {D{\'{\i}}az Trigo}, M. and {Homan}, J. and {Ibarra}, A. and {Kennea}, J.~A. and {Mu{\~n}oz-Darias}, T. and {Ness}, J.-U. and {Parmar}, A.~N. and {Pollock}, A.~M.~T. and {van den Heuvel}, E.~P.~J. and {van der Horst}, A.~J.},
	Doi = {10.1051/0004-6361/201219447},
	Eid = {A32},
	Eprint = {1204.5840},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, binaries: close, stars: individual: MAXI J1659-152, X-rays: binaries},
	Month = apr,
	Pages = {A32},
	Primaryclass = {astro-ph.HE},
	Title = {{MAXI J1659-152: the shortest orbital period black-hole transient in outburst}},
	Volume = 552,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201219447}}

@article{lai12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757L...3L},
	Archiveprefix = {arXiv},
	Author = {{Lai}, D.},
	Doi = {10.1088/2041-8205/757/1/L3},
	Eid = {L3},
	Eprint = {1206.3723},
	Journal = {\apjl},
	Keywords = {binaries: close, gravitational waves, planetary systems, stars: magnetic field, stars: neutron},
	Month = sep,
	Pages = {L3},
	Primaryclass = {astro-ph.HE},
	Title = {{DC Circuit Powered by Orbital Motion: Magnetic Interactions in Compact Object Binaries and Exoplanetary Systems}},
	Volume = 757,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/757/1/L3}}

@article{lamb81,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1981ApJ...244...94L},
	Author = {{Lamb}, R.~C. and {Markert}, T.~H.},
	Doi = {10.1086/158688},
	Journal = {\apj},
	Keywords = {GAMMA RAY ASTRONOMY, NEBULAE, SUPERNOVA REMNANTS, X RAY SOURCES, NEUTRON STARS, POINT SOURCES, PROPORTIONAL COUNTERS, X RAY TELESCOPES},
	Month = feb,
	Pages = {94-101},
	Title = {{X-ray emission from supernova remnants near gamma-ray sources}},
	Volume = 244,
	Year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/158688}}

@article{lamb02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...567L.129L},
	Author = {{Lamb}, R.~C. and {Macomb}, D.~J. and {Prince}, T.~A. and {Majid}, W.~A.},
	Doi = {10.1086/340001},
	Eprint = {astro-ph/0112360},
	Journal = {\apjl},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: General, Stars: Pulsars: General, X-Rays: General},
	Month = mar,
	Pages = {L129-L132},
	Title = {{Discovery of 16.6 and 25.5 Second Pulsations from the Small Magellanic Cloud}},
	Volume = 567,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340001}}

@article{lfm02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...574L..29L&db_key=AST},
	Author = {{Lamb}, R.~C. and {Fox}, D.~W. and {Macomb}, D.~J. and {Prince}, T.~A.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L29-L32},
	Title = {{Discovery of a Possible Anomalous X-Ray Pulsar in the Small Magellanic Cloud}},
	Volume = 574,
	Year = 2002}

@article{lamb03errata,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...599L.115L},
	Author = {{Lamb}, R.~C. and {Fox}, D.~W. and {Macomb}, D.~J. and {Prince}, T.~A.},
	Doi = {10.1086/381175},
	Journal = {\apjl},
	Month = dec,
	Pages = {L115-L115},
	Title = {{Addendum: ``Discovery of a Possible Anomalous X-Ray Pulsar in the Small Magellanic Cloud'' (<A href=''/abs/2002ApJ...574L..29L''>ApJ, 574, L29 [2002]</A>)}},
	Volume = 599,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/381175}}

@article{lamb03,
	Adsurl = {http://gcn.gsfc.nasa.gov/gcn/gcn3/2351.gcn3},
	Author = {{Lamb}, D. and {Graziani}, C. and {Shirasaki}, Y. and {Atteia}, J-L. and {Barraud}, C. and {Hurley}, K and {Crew}, G.},
	Journal = {GCN Circ. 2351},
	Title = {{SGR 1808-20 (=H2802): A Possible new SGR}},
	Year = 2003}

@ARTICLE{lander15,
   author = {{Lander}, S.~K. and {Andersson}, N. and {Antonopoulou}, D. and 
	{Watts}, A.~L.},
    title = "{Magnetically driven crustquakes in neutron stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1412.5852},
 primaryClass = "astro-ph.HE",
 keywords = {asteroseismology, stars: magnetars, stars: magnetic field, stars: neutron},
     year = 2015,
    month = may,
   volume = 449,
    pages = {2047-2058},
      doi = {10.1093/mnras/stv432},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.2047L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{landi12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.4166....1L},
	Author = {{Landi}, R. and {Bassani}, L. and {Masetti}, N. and {Bazzano}, A. and {Ubertini}, P. and {Bird}, A.~J. and {Goossens}, M.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Gamma Ray, Request for Observations},
	Month = jun,
	Title = {{Search for counterparts of newly discovered INTEGRAL/IBIS sources}},
	Volume = 4166,
	Year = 2012}

@article{landolt83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983AJ.....88..439L},
	Author = {{Landolt}, A.~U.},
	Doi = {10.1086/113329},
	Journal = {\aj},
	Keywords = {ELECTROPHOTOMETRY, REFERENCE STARS, STELLAR SPECTROPHOTOMETRY, UBV SPECTRA, ASTRONOMICAL CATALOGS, ERRORS, STELLAR COLOR},
	Month = mar,
	Pages = {439-460},
	Title = {{UBVRI photometric standard stars around the celestial equator}},
	Volume = 88,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/113329}}

@article{langer89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...210...93L},
	Author = {{Langer}, N.},
	Journal = {\aap},
	Keywords = {Stellar Models, Stellar Structure, Wolf-Rayet Stars, Abundance, Chemical Composition, Mass To Light Ratios, Stellar Evolution, Stellar Mass, Surface Temperature},
	Month = feb,
	Pages = {93-113},
	Title = {{Standard models of Wolf-Rayet stars}},
	Volume = 210,
	Year = 1989}

@ARTICLE{langer12,
   author = {{Langer}, N.},
    title = "{Presupernova Evolution of Massive Single and Binary Stars}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1206.5443},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = sep,
   volume = 50,
    pages = {107-164},
      doi = {10.1146/annurev-astro-081811-125534},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..107L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lanzoni10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...717..653L},
	Archiveprefix = {arXiv},
	Author = {{Lanzoni}, B. and {Ferraro}, F.~R. and {Dalessandro}, E. and {Mucciarelli}, A. and {Beccari}, G. and {Miocchi}, P. and {Bellazzini}, M. and {Rich}, R.~M. and {Origlia}, L. and {Valenti}, E. and {Rood}, R.~T. and {Ransom}, S.~M.},
	Doi = {10.1088/0004-637X/717/2/653},
	Eprint = {1005.2847},
	Journal = {\apj},
	Keywords = {globular clusters: individual: Terzan 5, stars: evolution},
	Month = jul,
	Pages = {653-657},
	Title = {{New Density Profile and Structural Parameters of the Complex Stellar System Terzan 5}},
	Volume = 717,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/717/2/653}}

@article{lapalombara07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...474..137L},
	Archiveprefix = {arXiv},
	Author = {{La Palombara}, N. and {Mereghetti}, S.},
	Doi = {10.1051/0004-6361:20077970},
	Eprint = {0706.3972},
	Journal = {\aap},
	Keywords = {X-rays: binaries, accretion, accretion disks, stars: emission-line, Be, stars: pulsars: individual: X Persei, X-rays: individuals: 4U 0352+309},
	Month = oct,
	Pages = {137-143},
	Title = {{XMM-Newton observation of the persistent Be/neutron star system X Persei at a high-luminosity level}},
	Volume = 474,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077970}}

@article{laros86,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1986Natur.322..152L&db_key=AST},
	Author = {{Laros}, J.~G. and {Fenimore}, E.~E. and {Fikani}, M.~M. and {Klebesadel}, R.~W. and {Barat}, C.},
	Journal = {\nat},
	Month = jul,
	Pages = {152},
	Title = {{The soft gamma-ray burst GB790107}},
	Volume = 322,
	Year = 1986}

@article{lasker08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136..735L},
	Archiveprefix = {arXiv},
	Author = {{Lasker}, B.~M. and {Lattanzi}, M.~G. and {McLean}, B.~J. and {Bucciarelli}, B. and {Drimmel}, R. and {Garcia}, J. and {Greene}, G. and {Guglielmetti}, F. and {Hanley}, C. and {Hawkins}, G. and {Laidler}, V.~G. and {Loomis}, C. and {Meakes}, M. and {Mignani}, R. and {Morbidelli}, R. and {Morrison}, J. and {Pannunzio}, R. and {Rosenberg}, A. and {Sarasso}, M. and {Smart}, R.~L. and {Spagna}, A. and {Sturch}, C.~R. and {Volpicelli}, A. and {White}, R.~L. and {Wolfe}, D. and {Zacchei}, A.},
	Doi = {10.1088/0004-6256/136/2/735},
	Eprint = {0807.2522},
	Journal = {\aj},
	Keywords = {astrometry, astronomical data bases: miscellaneous, catalogs, surveys, techniques: image processing, techniques: photometric},
	Month = aug,
	Pages = {735-766},
	Title = {{The Second-Generation Guide Star Catalog: Description and Properties}},
	Volume = 136,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/136/2/735}}

@article{lasky13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..88j3005L},
	Archiveprefix = {arXiv},
	Author = {{Lasky}, P.~D. and {Melatos}, A.},
	Doi = {10.1103/PhysRevD.88.103005},
	Eid = {103005},
	Eprint = {1310.7633},
	Journal = {\prd},
	Keywords = {Gravitational radiation magnetic fields and other observations, Wave generation and sources, Neutron stars},
	Month = nov,
	Number = 10,
	Pages = {103005},
	Primaryclass = {astro-ph.HE},
	Title = {{Tilted torus magnetic fields in neutron stars and their gravitational wave signatures}},
	Volume = 88,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.88.103005}}

@article{lawrence07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.379.1599L},
	Author = {{Lawrence}, A. and {Warren}, S.~J. and {Almaini}, O. and {Edge}, A.~C. and {Hambly}, N.~C. and {Jameson}, R.~F. and {Lucas}, P. and {Casali}, M. and {Adamson}, A. and {Dye}, S. and {Emerson}, J.~P. and {Foucaud}, S. and {Hewett}, P. and {Hirst}, P. and {Hodgkin}, S.~T. and {Irwin}, M.~J. and {Lodieu}, N. and {McMahon}, R.~G. and {Simpson}, C. and {Smail}, I. and {Mortlock}, D. and {Folger}, M.},
	Doi = {10.1111/j.1365-2966.2007.12040.x},
	Eprint = {arXiv:astro-ph/0604426},
	Journal = {\mnras},
	Keywords = {surveys, infrared: general},
	Month = aug,
	Pages = {1599-1617},
	Title = {{The UKIRT Infrared Deep Sky Survey (UKIDSS)}},
	Volume = 379,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12040.x}}

@article{laycock05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634L..53L},
	Author = {{Laycock}, S. and {Grindlay}, J. and {van den Berg}, M. and {Zhao}, P. and {Hong}, J. and {Koenig}, X. and {Schlegel}, E.~M. and {Persson}, S.~E.},
	Doi = {10.1086/498821},
	Eprint = {arXiv:astro-ph/0509783},
	Journal = {\apjl},
	Keywords = {Galaxy: Center, X-Rays: Binaries},
	Month = nov,
	Pages = {L53-L56},
	Title = {{Constraining the Nature of the Galactic Center X-Ray Source Population}},
	Volume = 634,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498821}}

@article{laycock10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2010ApJ...716.1217L},
	Archiveprefix = {arXiv},
	Author = {{Laycock}, S. and {Zezas}, A. and {Hong}, J. and {Drake}, J.~J. and {Antoniou}, V.},
	Doi = {10.1088/0004-637X/716/2/1217},
	Eprint = {0809.1738},
	Journal = {\apj},
	Keywords = {Magellanic Clouds, stars: emission-line, Be, stars: neutron, X-rays: binaries},
	Month = jun,
	Pages = {1217-1240},
	Title = {{Exploring the Small Magellanic Cloud to the Faintest X-ray Fluxes: Source Catalog, Timing, and Spectral Analysis}},
	Volume = 716,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/716/2/1217}}

@article{laycock15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.1399L},
	Archiveprefix = {arXiv},
	Author = {{Laycock}, S.~G.~T. and {Cappallo}, R.~C. and {Moro}, M.~J.},
	Doi = {10.1093/mnras/stu2151},
	Eprint = {1410.3417},
	Journal = {\mnras},
	Keywords = {binaries: eclipsing, stars: black holes, stars: Wolf-Rayet, X-rays: binaries},
	Month = jan,
	Pages = {1399-1410},
	Primaryclass = {astro-ph.HE},
	Title = {{Chandra and XMM monitoring of the black hole X-ray binary IC 10 X-1}},
	Volume = 446,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu2151}}

@article{lazendic03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...593L..27L},
	Author = {{Lazendic}, J.~S. and {Slane}, P.~O. and {Gaensler}, B.~M. and {Plucinsky}, P.~P. and {Hughes}, J.~P. and {Galloway}, D.~K. and {Crawford}, F.},
	Doi = {10.1086/378183},
	Eprint = {arXiv:astro-ph/0306057},
	Journal = {\apjl},
	Month = aug,
	Pages = {L27-L30},
	Title = {{X-Ray Observations of the Compact Central Object in Supernova Remnant G347.3-0.5}},
	Volume = 593,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378183}}

@article{lazendic04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...602..271L},
	Author = {{Lazendic}, J.~S. and {Slane}, P.~O. and {Gaensler}, B.~M. and {Reynolds}, S.~P. and {Plucinsky}, P.~P. and {Hughes}, J.~P.},
	Doi = {10.1086/380956},
	Eprint = {arXiv:astro-ph/0310696},
	Journal = {\apj},
	Month = feb,
	Pages = {271-285},
	Title = {{A High-Resolution Study of Nonthermal Radio and X-Ray Emission from Supernova Remnant G347.3-0.5}},
	Volume = 602,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/380956}}

@article{lazendic05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...618..733L},
	Author = {{Lazendic}, J.~S. and {Slane}, P.~O. and {Hughes}, J.~P. and {Chen}, Y. and {Dame}, T.~M.},
	Doi = {10.1086/426114},
	Eprint = {arXiv:astro-ph/0409592},
	Journal = {\apj},
	Month = jan,
	Pages = {733-743},
	Title = {{Chandra Detection of Ejecta in the Small-Diameter Supernova Remnant G349.7+0.2}},
	Volume = 618,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426114}}

@article{leahy83_ray,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...272..256L},
	Author = {{Leahy}, D.~A. and {Elsner}, R.~F. and {Weisskopf}, M.~C.},
	Doi = {10.1086/161288},
	Journal = {\apj},
	Month = sep,
	Pages = {256-258},
	Title = {{On searches for periodic pulsed emission - The Rayleigh test compared to epoch folding}},
	Volume = 272,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/161288}}

@article{leahy83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1983ApJ...266..160L},
	Author = {{Leahy}, D.~A. and {Darbro}, W. and {Elsner}, R.~F. and {Weisskopf}, M.~C. and {Kahn}, S. and {Sutherland}, P.~G. and {Grindlay}, J.~E.},
	Doi = {10.1086/160766},
	Journal = {\apj},
	Month = mar,
	Pages = {160-170},
	Title = {{On searches for pulsed emission with application to four globular cluster X-ray sources - NGC 1851, 6441, 6624, and 6712}},
	Volume = 266,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160766}}

@article{leahy87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...180..275L},
	Author = {{Leahy}, D.~A.},
	Journal = {\aap},
	Keywords = {MONTE CARLO METHOD, PARAMETER IDENTIFICATION, PULSED RADIATION, SIGNAL DETECTION, SINE WAVES, STATISTICAL ANALYSIS, AMPLITUDES, PERIODIC VARIATIONS, SEARCHING, SIGNAL TO NOISE RATIOS, TIME MEASUREMENT},
	Month = jun,
	Pages = {275-277},
	Title = {{Searches for pulsed emission - Improved determination of period and amplitude from epoch folding for sinusoidal signals}},
	Volume = 180,
	Year = 1987}

@article{leahy97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997ApJ...475..823L&db_key=AST},
	Author = {{Leahy}, D.~A. and {Harrison}, F.~A. and {Yoshida}, A.},
	Doi = {10.1086/303557},
	Journal = {\apj},
	Month = feb,
	Pages = {823},
	Title = {{The ASCA X-Ray Spectrum of the Unusual Binary LSI +61 degrees 303}},
	Volume = 475,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/303557}}

@article{leahy01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...380..516L},
	Author = {{Leahy}, D.~A.},
	Doi = {10.1051/0004-6361:20011390},
	Journal = {\aap},
	Month = dec,
	Pages = {516-519},
	Title = {{The gamma-ray source LSI +61deg303. I. RXTE/ASM observations}},
	Volume = 380,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20011390}}

@article{leahy04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...413.1019L},
	Author = {{Leahy}, D.~A.},
	Doi = {10.1051/0004-6361:20031545},
	Journal = {\aap},
	Month = jan,
	Pages = {1019-1028},
	Title = {{The gamma-ray source {\l}si. II. Multiwavelength emission model}},
	Volume = 413,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031545}}

@article{lebrun03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.141L},
	Author = {{Lebrun}, F. and {Leray}, J.~P. and {Lavocat}, P. and {Cr{\'e}tolle}, J. and {Arqu{\`e}s}, M. and {Blondel}, C. and {Bonnin}, C. and {Bou{\`e}re}, A. and {Cara}, C. and {Chaleil}, T. and {Daly}, F. and {Desages}, F. and {Dzitko}, H. and {Horeau}, B. and {Laurent}, P. and {Limousin}, O. and {Mathy}, F. and {Mauguen}, V. and {Meignier}, F. and {Molini{\'e}}, F. and {Poindron}, E. and {Rouger}, M. and {Sauvageon}, A. and {Tourrette}, T.},
	Doi = {10.1051/0004-6361:20031367},
	Eprint = {arXiv:astro-ph/0310362},
	Journal = {\aap},
	Month = nov,
	Pages = {L141-L148},
	Title = {{ISGRI: The INTEGRAL Soft Gamma-Ray Imager}},
	Volume = 411,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031367}}

@article{lebrun04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004Natur.428..293L&db_key=AST},
	Author = {{Lebrun}, F. and {Terrier}, R. and {Bazzano}, A. and {B{\'e}langer}, G. and {Bird}, A. and {Bouchet}, L. and {Dean}, A. and {Del Santo}, M. and {Goldwurm}, A. and {Lund}, N. and {Morand}, H. and {Parmar}, A. and {Paul}, J. and {Roques}, J.-P. and {Sch{\"o}nfelder}, V. and {Strong}, A.~W. and {Ubertini}, P. and {Walter}, R. and {Winkler}, C.},
	Doi = {10.1038/nature02407},
	Journal = {\nat},
	Month = mar,
	Pages = {293-296},
	Title = {{Compact sources as the origin of the soft {$\gamma$}-ray emission of the Milky Way}},
	Volume = 428,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature02407}}

@ARTICLE{leibowitz20,
       author = {{Leibowitz}, Elia},
        title = "{Possible Evidence from the Flaring Activity of Sgr A* for a Star at a Distance of {\ensuremath{\sim}}3.3 Schwarzschild Radii from the Black Hole}",
      journal = {\apj},
     keywords = {159, 565, 1814, 793, 1822, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jun,
       volume = {896},
       number = {1},
          eid = {74},
        pages = {74},
          doi = {10.3847/1538-4357/ab93c5},
archivePrefix = {arXiv},
       eprint = {2005.07256},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...896...74L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lenters03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...587..761L&db_key=AST},
	Author = {{Lenters}, G.~T. and {Woods}, P.~M. and {Goupell}, J.~E. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Hurley}, K. and {Frederiks}, D. and {Golenetskii}, S. and {Swank}, J.},
	Journal = {\apj},
	Month = apr,
	Pages = {761-770},
	Title = {{An Extended Burst Tail from SGR 1900+14 with a Thermal X-Ray Spectrum}},
	Volume = 587,
	Year = 2003}

@inproceedings{lenzen03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://esoads.eso.org/abs/2003SPIE.4841..944L},
	Author = {{Lenzen}, R. and {Hartung}, M. and {Brandner}, W. and {Finger}, G. and {Hubin}, N.~N. and {Lacombe}, F. and {Lagrange}, A.-M. and {Lehnert}, M.~D. and {Moorwood}, A.~F.~M. and {Mouillet}, D.},
	Booktitle = {Instrument Design and Performance for Optical/Infrared Ground-based Telescopes.},
	Doi = {10.1117/12.460044},
	Editor = {{Iye}, M. and {Moorwood}, A.~F.~M.},
	Month = mar,
	Pages = {944-952},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{NAOS-CONICA first on sky results in a variety of observing modes}},
	Volume = 4841,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.460044}}

@ARTICLE{levin06,
   author = {{Levin}, Y.},
    title = "{QPOs during magnetar flares are not driven by mechanical normal modes of the crust}",
  journal = {\mnras},
   eprint = {astro-ph/0601020},
 keywords = {stars: magnetic fields, stars: neutron, stars: oscillations, quasars: general},
     year = 2006,
    month = may,
   volume = 368,
    pages = {L35-L38},
      doi = {10.1111/j.1745-3933.2006.00155.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368L..35L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{levin07,
   author = {{Levin}, Y.},
    title = "{On the theory of magnetar QPOs}",
  journal = {\mnras},
   eprint = {astro-ph/0612725},
 keywords = {MHD, stars: neutron},
     year = 2007,
    month = may,
   volume = 377,
    pages = {159-167},
      doi = {10.1111/j.1365-2966.2007.11582.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.377..159L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{levin11,
   author = {{Levin}, Y. and {van Hoven}, M.},
    title = "{On the excitation of f modes and torsional modes by magnetar giant flares}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.0880},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron},
     year = 2011,
    month = nov,
   volume = 418,
    pages = {659-663},
      doi = {10.1111/j.1365-2966.2011.19515.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418..659L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{levin12,
   author = {{Levin}, L. and {Bailes}, M. and {Bates}, S.~D. and {Bhat}, N.~D.~R. and 
	{Burgay}, M. and {Burke-Spolaor}, S. and {D'Amico}, N. and {Johnston}, S. and 
	{Keith}, M.~J. and {Kramer}, M. and {Milia}, S. and {Possenti}, A. and 
	{Stappers}, B. and {van Straten}, W.},
    title = "{Radio emission evolution, polarimetry and multifrequency single pulse analysis of the radio magnetar PSR J1622-4950}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1204.2045},
 primaryClass = "astro-ph.HE",
 keywords = {stars: magnetars, pulsars: individual: PSR J1622-4950},
     year = 2012,
    month = may,
   volume = 422,
    pages = {2489-2500},
      doi = {10.1111/j.1365-2966.2012.20807.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.2489L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lewin93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993SSRv...62..223L},
	Author = {{Lewin}, W.~H.~G. and {van Paradijs}, J. and {Taam}, R.~E.},
	Doi = {10.1007/BF00196124},
	Journal = {\ssr},
	Month = sep,
	Pages = {223-389},
	Title = {{X-Ray Bursts}},
	Volume = 62,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/BF00196124}}

@article{lewin71,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...169L..17L},
	Author = {{Lewin}, W.~H.~G. and {Ricker}, G.~R. and {McClintock}, J.~E.},
	Doi = {10.1086/180805},
	Journal = {\apjl},
	Month = oct,
	Pages = {L17},
	Title = {{X-Rays from a New Variable Source GX 1+4}},
	Volume = 169,
	Year = 1971,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/180805}}

@ARTICLE{li04,
   author = {{Li}, J. and {Kastner}, J.~H. and {Prigozhin}, G.~Y. and {Schulz}, N.~S. and 
	{Feigelson}, E.~D. and {Getman}, K.~V.},
    title = "{Chandra ACIS Subpixel Event Repositioning: Further Refinements and Comparison between Backside- and Frontside-illuminated X-Ray CCDs}",
  journal = {\apj},
   eprint = {astro-ph/0401592},
 keywords = {Instrumentation: Detectors, Methods: Data Analysis, Techniques: Image Processing, X-Rays: General},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {1204-1212},
      doi = {10.1086/421866},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610.1204L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{li07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...666L..81L},
	Archiveprefix = {arXiv},
	Author = {{Li}, {X.-D.}},
	Doi = {10.1086/521791},
	Eprint = {0708.0060},
	Journal = {\apjl},
	Keywords = {Stars: Individual: Alphanumeric: 1E 161348-5055, Stars: Individual: Alphanumeric: SS 433, Stars: Neutron, ISM: Supernova Remnants, Stars: Supernovae: Individual: Alphanumeric: RCW 103, X-Rays: Stars},
	Month = sep,
	Pages = {L81-L84},
	Title = {{The Nature of the Compact X-Ray Source in Supernova Remnant RCW 103}},
	Volume = 666,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/521791}}

@ARTICLE{li08,
   author = {{Li}, X.-H. and {Lu}, F.-J. and {Li}, Z.},
    title = "{Nonthermal X-Ray Properties of Rotation-powered Pulsars and Their Wind Nebulae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0707.4279},
 keywords = {pulsars: general, radiation mechanisms: non-thermal, stars: neutron, X-rays: general },
     year = 2008,
    month = aug,
   volume = 682,
      eid = {1166-1176},
    pages = {1166-1176},
      doi = {10.1086/589495},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682.1166L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{li16,
   author = {{Li}, T. and {Shao}, Y. and {Li}, X.-D.},
    title = "{Can the Subsonic Accretion Model Explain the Spin Period Distribution of Wind-fed X-Ray Pulsars?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1605.03669},
 primaryClass = "astro-ph.HE",
 keywords = {stars: early-type, stars: evolution, stars: neutron, X-rays: binaries},
     year = 2016,
    month = jun,
   volume = 824,
      eid = {143},
    pages = {143},
      doi = {10.3847/0004-637X/824/2/143},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...824..143L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{li17,
   author = {{Li}, J. and {Rea}, N. and {Torres}, D.~F. and {de O{\~n}a-Wilhelmi}, E.
	},
    title = "{Gamma-ray Upper Limits on Magnetars with Six Years of Fermi-LAT Observations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1607.03778},
 primaryClass = "astro-ph.HE",
 keywords = {gamma-rays: stars, stars: magnetars, X-rays: stars},
     year = 2017,
    month = jan,
   volume = 835,
      eid = {30},
    pages = {30},
      doi = {10.3847/1538-4357/835/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835...30L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{liedahl95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...438L.115L},
	Author = {{Liedahl}, D.~A. and {Osterheld}, A.~L. and {Goldstein}, W.~H.},
	Doi = {10.1086/187729},
	Journal = {\apjl},
	Month = jan,
	Pages = {L115-L118},
	Title = {{New calculations of Fe L-shell X-ray spectra in high-temperature plasmas}},
	Volume = 438,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/187729}}

@ARTICLE{lidov62,
       author = {{Lidov}, M.~L.},
        title = "{The evolution of orbits of artificial satellites of planets under the action of gravitational perturbations of external bodies}",
      journal = {\planss},
         year = 1962,
        month = oct,
       volume = {9},
       number = {10},
        pages = {719-759},
          doi = {10.1016/0032-0633(62)90129-0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1962P&SS....9..719L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lin14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...780...39L},
	Archiveprefix = {arXiv},
	Author = {{Lin}, D. and {Webb}, N.~A. and {Barret}, D.},
	Doi = {10.1088/0004-637X/780/1/39},
	Eid = {39},
	Eprint = {1309.0509},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, galaxies: nuclei, X-rays: binaries},
	Month = jan,
	Pages = {39},
	Primaryclass = {astro-ph.HE},
	Title = {{Classification of X-Ray Sources in the XMM-Newton Serendipitous Source Catalog: Objects of Special Interest}},
	Volume = 780,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/780/1/39}}

@article{linden10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725.1984L},
	Archiveprefix = {arXiv},
	Author = {{Linden}, T. and {Kalogera}, V. and {Sepinsky}, J.~F. and {Prestwich}, A. and {Zezas}, A. and {Gallagher}, J.~S.},
	Doi = {10.1088/0004-637X/725/2/1984},
	Eprint = {1005.1639},
	Journal = {\apj},
	Keywords = {galaxies: starburst, supernovae: general, X-rays: binaries},
	Month = dec,
	Pages = {1984-1994},
	Primaryclass = {astro-ph.CO},
	Title = {{The Effect of Starburst Metallicity on Bright X-ray Binary Formation Pathways}},
	Volume = 725,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/725/2/1984}}

@article{linden12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748..114L},
	Archiveprefix = {arXiv},
	Author = {{Linden}, T. and {Valsecchi}, F. and {Kalogera}, V.},
	Doi = {10.1088/0004-637X/748/2/114},
	Eid = {114},
	Eprint = {1111.5012},
	Journal = {\apj},
	Keywords = {galaxies: starburst, stars: emission-line, Be, stars: Wolf-Rayet, X-rays: binaries},
	Month = apr,
	Pages = {114},
	Primaryclass = {astro-ph.GA},
	Title = {{On the Rarity of X-Ray Binaries with Naked Helium Donors}},
	Volume = 748,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/748/2/114}}

@article{liu00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000A%26AS..147...25L&db_key=AST},
	Author = {{Liu}, Q.~Z. and {van Paradijs}, J. and {van den Heuvel}, E.~P.~J.},
	Journal = {\aaps},
	Month = nov,
	Pages = {25-49},
	Title = {{A catalogue of high-mass X-ray binaries}},
	Volume = 147,
	Year = 2000}

@article{liu05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJS..157...59L},
	Author = {{Liu}, J.-F. and {Bregman}, J.~N.},
	Doi = {10.1086/427170},
	Eprint = {arXiv:astro-ph/0501309},
	Journal = {\apjs},
	Keywords = {Catalogs, Galaxies: General, X-Rays: Binaries, X-Rays: Galaxies},
	Month = mar,
	Pages = {59-125},
	Title = {{Ultraluminous X-Ray Sources in Nearby Galaxies from ROSAT High Resolution Imager Observations I. Data Analysis}},
	Volume = 157,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/427170}}

@article{lm05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...429.1125L},
	Author = {{Liu}, Q.~Z. and {Mirabel}, I.~F.},
	Doi = {10.1051/0004-6361:20041878},
	Journal = {\aap},
	Keywords = {X-rays: galaxies, X-rays: binaries, galaxies: general, catalogs},
	Month = jan,
	Pages = {1125-1129},
	Title = {{A catalogue of ultraluminous X-ray sources in external galaxies}},
	Volume = 429,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041878}}

@article{liu07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..807L},
	Archiveprefix = {arXiv},
	Author = {{Liu}, Q.~Z. and {van Paradijs}, J. and {van den Heuvel}, E.~P.~J.},
	Doi = {10.1051/0004-6361:20077303},
	Eprint = {0707.0544},
	Journal = {\aap},
	Keywords = {binaries: close, stars: late-type, X-rays: binaries, catalogs},
	Month = jul,
	Pages = {807-810},
	Title = {{A catalogue of low-mass X-ray binaries in the Galaxy, LMC, and SMC (Fourth edition)}},
	Volume = 469,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077303}}

@article{liu09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690L..39L},
	Author = {{Liu}, J. and {Bregman}, J.~N. and {McClintock}, J.~E.},
	Doi = {10.1088/0004-637X/690/1/L39},
	Journal = {\apjl},
	Keywords = {galaxies: individual: NGC 1313, X-rays: binaries},
	Month = jan,
	Pages = {L39-L42},
	Title = {{Hubble Space Telescope Monitoring Reveals a 6.1 Day Period for an Ultraluminous X-Ray Source in NGC 1313}},
	Volume = 690,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/1/L39}}

@article{liu11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..192...10L},
	Archiveprefix = {arXiv},
	Author = {{Liu}, J.},
	Doi = {10.1088/0067-0049/192/1/10},
	Eid = {10},
	Eprint = {0811.0804},
	Journal = {\apjs},
	Keywords = {catalogs, galaxies: general, X-rays: binaries, X-rays: galaxies},
	Month = jan,
	Pages = {10},
	Title = {{Chandra ACIS Survey of X-ray Point Sources in 383 Nearby Galaxies. I. The Source Catalog}},
	Volume = 192,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/192/1/10}}

@article{liu12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...747....1L},
	Archiveprefix = {arXiv},
	Author = {{Liu}, K. and {Wex}, N. and {Kramer}, M. and {Cordes}, J.~M. and {Lazio}, T.~J.~W.},
	Doi = {10.1088/0004-637X/747/1/1},
	Eid = {1},
	Eprint = {1112.2151},
	Journal = {\apj},
	Keywords = {black hole physics, Galaxy: center, pulsars: general},
	Month = mar,
	Pages = {1},
	Primaryclass = {astro-ph.HE},
	Title = {{Prospects for Probing the Spacetime of Sgr A* with Pulsars}},
	Volume = 747,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/747/1/1}}

@article{liu13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013Natur.503..500L},
	Archiveprefix = {arXiv},
	Author = {{Liu}, J.-F. and {Bregman}, J.~N. and {Bai}, Y. and {Justham}, S. and {Crowther}, P.},
	Doi = {10.1038/nature12762},
	Eprint = {1312.0337},
	Journal = {\nat},
	Month = nov,
	Pages = {500-503},
	Primaryclass = {astro-ph.HE},
	Title = {{Puzzling accretion onto a black hole in the ultraluminous X-ray source M 101 ULX-1}},
	Volume = 503,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature12762}}

@article{liu15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..233L},
	Archiveprefix = {arXiv},
	Author = {{Liu}, X.~W. and {Xu}, R.~X. and {van den Heuvel}, E.~P.~J. and {Qiao}, G.~J. and {Han}, J.~L. and {Han}, Z.~W. and {Li}, X.~D.},
	Doi = {10.1088/0004-637X/799/2/233},
	Eid = {233},
	Eprint = {1207.4687},
	Journal = {\apj},
	Keywords = {ISM: supernova remnants, stars: evolution, stars: individual: 1E161348-5055, stars: neutron},
	Month = feb,
	Pages = {233},
	Primaryclass = {astro-ph.HE},
	Title = {{The Extremely Long-period X-Ray Source in a Young Supernova Remnant: A Thorne-{\.Z}ytkow Object Descendant?}},
	Volume = 799,
	Year = 2015,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/799/2/233}}

@article{livingstone07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.308..317L},
	Author = {{Livingstone}, M.~A. and {Kaspi}, V.~M. and {Gavriil}, F.~P. and {Manchester}, R.~N. and {Gotthelf}, E.~V.~G. and {Kuiper}, L.},
	Doi = {10.1007/s10509-007-9320-3},
	Eprint = {arXiv:astro-ph/0702196},
	Journal = {\apss},
	Month = apr,
	Pages = {317-323},
	Title = {{New phase-coherent measurements of pulsar braking indices}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9320-3}}

@article{livingstone11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743L..38L},
	Archiveprefix = {arXiv},
	Author = {{Livingstone}, M.~A. and {Scholz}, P. and {Kaspi}, V.~M. and {Ng}, C.-Y. and {Gavriil}, F.~P.},
	Doi = {10.1088/2041-8205/743/2/L38},
	Eid = {L38},
	Eprint = {1109.5715},
	Journal = {\apjl},
	Keywords = {pulsars: individual: Swift J1822.3-1606, stars: magnetars, stars: neutron, X-rays: bursts},
	Month = dec,
	Pages = {L38},
	Primaryclass = {astro-ph.HE},
	Title = {{The Spin-down of Swift J1822.3-1606: A New Galactic Magnetar}},
	Volume = 743,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/743/2/L38}}

@article{livio87,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1987Natur.327..398L&db_key=AST},
	Author = {{Livio}, M. and {Taam}, R.~E.},
	Journal = {\nat},
	Month = jun,
	Pages = {398-400},
	Title = {{Possible models for the high-energy transient GB790107}},
	Volume = 327,
	Year = 1987}

@article{lodders03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591.1220L},
	Author = {{Lodders}, K.},
	Doi = {10.1086/375492},
	Journal = {\apj},
	Keywords = {Astrochemistry, Meteors, Meteoroids, Solar System: Formation- Sun: Abundances, Sun: Photosphere},
	Month = jul,
	Pages = {1220-1247},
	Title = {{Solar System Abundances and Condensation Temperatures of the Elements}},
	Volume = 591,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/375492}}

@article{lommen05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...443..231L},
	Author = {{Lommen}, D. and {Yungelson}, L. and {van den Heuvel}, E. and {Nelemans}, G. and {Portegies Zwart}, S.},
	Doi = {10.1051/0004-6361:20052824},
	Eprint = {arXiv:astro-ph/0507304},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, stars: individual: Cyg X-3, stars: binaries: close, stars: binaries: general, stars: Wolf-Rayet},
	Month = nov,
	Pages = {231-241},
	Title = {{Cygnus X-3 and the problem of the missing Wolf-Rayet X-ray binaries}},
	Volume = 443,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052824}}

@inproceedings{long83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983adsx.conf..141L},
	Author = {{Long}, K.~S. and {van Speybroeck}, L.~P.},
	Booktitle = {Accretion-Driven Stellar X-ray Sources, Cambridge University Press, Cambridge.},
	Editor = {{Lewin}, W.~H.~G. and {van den Heuvel}, E.~P.~J.},
	Pages = {141},
	Title = {{Very Bright Non-Nuclear Sources}},
	Year = 1983}

@BOOK{longair11,
   author = {{Longair}, M.~S.},
    title = "{High Energy Astrophysics}",
     year = 2011,
    month = feb,
	Publisher = {Cambridge, UK: Cambridge University Press},
   adsurl = {http://adsabs.harvard.edu/abs/2011hea..book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lorenzin09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.394.1588L},
	Author = {{Lorenzin}, A. and {Zampieri}, L.},
	Doi = {10.1111/j.1365-2966.2009.14435.x},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , black hole physics , X-rays: binaries},
	Month = apr,
	Pages = {1588-1596},
	Title = {{A comparative analysis of standard accretion discs spectra: an application to ultraluminous X-ray sources}},
	Volume = 394,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14435.x}}

@book{lorimer04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004hpa..book.....L},
	Author = {{Lorimer}, D.~R. and {Kramer}, M.},
	Month = dec,
	Publisher = {Cambridge, UK: Cambridge University Press},
	Title = {{Handbook of Pulsar Astronomy}},
	Year = 2004}

@article{lorimer06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006MNRAS.372..777L&db_key=AST},
	Author = {{Lorimer}, D.~R. and {Faulkner}, A.~J. and {Lyne}, A.~G. and {Manchester}, R.~N. and {Kramer}, M. and {McLaughlin}, M.~A. and {Hobbs}, G. and {Possenti}, A. and {Stairs}, I.~H. and {Camilo}, F. and {Burgay}, M. and {D'Amico}, N. and {Corongiu}, A. and {Crawford}, F.},
	Doi = {10.1111/j.1365-2966.2006.10887.x},
	Eprint = {astro-ph/0607640},
	Journal = {\mnras},
	Month = oct,
	Pages = {777-800},
	Title = {{The Parkes Multibeam Pulsar Survey - VI. Discovery and timing of 142 pulsars and a Galactic population analysis}},
	Volume = 372,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10887.x}}

@article{lorimer09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2096....1L},
	Author = {{Lorimer}, D.~R. and {Edel}, S. and {Kondratiev}, V.~I. and {McLaughlin}, M.~A. and {Boyles}, J.~R. and {Ludovici}, D.~A. and {Ridley}, J.~P.},
	Journal = {Astron. Tel.},
	Keywords = {Radio, Soft Gamma-ray Repeaters},
	Month = jun,
	Title = {{No radio emission from soft gamma repeater SGR 0418+5729}},
	Volume = 2096,
	Year = 2009}

@article{lovelace95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.275..244L},
	Author = {{Lovelace}, R.~V.~E. and {Romanova}, M.~M. and {Bisnovatyi-Kogan}, G.~S.},
	Eprint = {arXiv:astro-ph/9412030},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, STARS: MAGNETIC FIELDS, STARS: NEUTRON, STARS: ROTATION, ISM: JETS AND OUTFLOWS},
	Month = jul,
	Pages = {244-254},
	Title = {{Spin-up/spin-down of magnetized stars with accretion discs and outflows}},
	Volume = 275,
	Year = 1995}

@article{lu09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1463L},
	Archiveprefix = {arXiv},
	Author = {{Lu}, J.~R. and {Ghez}, A.~M. and {Hornstein}, S.~D. and {Morris}, M.~R. and {Becklin}, E.~E. and {Matthews}, K.},
	Doi = {10.1088/0004-637X/690/2/1463},
	Eprint = {0808.3818},
	Journal = {\apj},
	Keywords = {black hole physics, Galaxy: center, infrared: stars, techniques: high angular resolution},
	Month = jan,
	Pages = {1463-1487},
	Title = {{A Disk of Young Stars at the Galactic Center as Determined by Individual Stellar Orbits}},
	Volume = 690,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/690/2/1463}}

@article{lund03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411L.231L},
	Author = {{Lund}, N. and {Budtz-J{\o}rgensen}, C. and {Westergaard}, N.~J. and {Brandt}, S. and {Rasmussen}, I.~L. and {Hornstrup}, A. and {Oxborrow}, C.~A. and {Chenevez}, J. and {Jensen}, P.~A. and {Laursen}, S. and {Andersen}, K.~H. and {Mogensen}, P.~B. and {Rasmussen}, I. and {Om{\o}}, K. and {Pedersen}, S.~M. and {Polny}, J. and {Andersson}, H. and {Andersson}, T. and {K{\"a}m{\"a}r{\"a}inen}, V. and {Vilhu}, O. and {Huovelin}, J. and {Maisala}, S. and {Morawski}, M. and {Juchnikowski}, G. and {Costa}, E. and {Feroci}, M. and {Rubini}, A. and {Rapisarda}, M. and {Morelli}, E. and {Carassiti}, V. and {Frontera}, F. and {Pelliciari}, C. and {Loffredo}, G. and {Mart{\'{\i}}nez N{\'u}{\~n}ez}, S. and {Reglero}, V. and {Velasco}, T. and {Larsson}, S. and {Svensson}, R. and {Zdziarski}, A.~A. and {Castro-Tirado}, A. and {Attina}, P. and {Goria}, M. and {Giulianelli}, G. and {Cordero}, F. and {Rezazad}, M. and {Schmidt}, M. and {Carli}, R. and {Gomez}, C. and {Jensen}, P.~L. and {Sarri}, G. and {Tiemon}, A. and {Orr}, A. and {Much}, R. and {Kretschmar}, P. and {Schnopper}, H.~W.},
	Doi = {10.1051/0004-6361:20031358},
	Journal = {\aap},
	Month = nov,
	Pages = {L231-L238},
	Title = {{JEM-X: The X-ray monitor aboard INTEGRAL}},
	Volume = 411,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031358}}

@article{luna13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...559A...6L},
	Archiveprefix = {arXiv},
	Author = {{Luna}, G.~J.~M. and {Sokoloski}, J.~L. and {Mukai}, K. and {Nelson}, T.},
	Doi = {10.1051/0004-6361/201220792},
	Eid = {A6},
	Eprint = {1211.6082},
	Journal = {\aap},
	Keywords = {binaries: symbiotic, accretion, accretion disks, X-rays: binaries},
	Month = nov,
	Pages = {A6},
	Primaryclass = {astro-ph.SR},
	Title = {{Symbiotic stars in X-rays}},
	Volume = 559,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201220792}}

@ARTICLE{lynch15,
   author = {{Lynch}, R.~S. and {Archibald}, R.~F. and {Kaspi}, V.~M. and 
	{Scholz}, P.},
    title = "{Green Bank Telescope and Swift X-Ray Telescope Observations of the Galactic Center Radio Magnetar SGR J1745-2900}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1412.0610},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: SGR J1745{\ndash}2900, stars: magnetars},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {266},
    pages = {266},
      doi = {10.1088/0004-637X/806/2/266},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806..266L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lyne04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004Sci...303.1153L},
	Author = {{Lyne}, A.~G. and {Burgay}, M. and {Kramer}, M. and {Possenti}, A. and {Manchester}, R.~N. and {Camilo}, F. and {McLaughlin}, M.~A. and {Lorimer}, D.~R. and {D'Amico}, N. and {Joshi}, B.~C. and {Reynolds}, J. and {Freire}, P.~C.~C.},
	Doi = {10.1126/science.1094645},
	Eprint = {arXiv:astro-ph/0401086},
	Journal = {Science},
	Month = feb,
	Pages = {1153-1157},
	Title = {{A Double-Pulsar System: A Rare Laboratory for Relativistic Gravity and Plasma Physics}},
	Volume = 303,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1094645}}

@article{lyne09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400.1439L},
	Archiveprefix = {arXiv},
	Author = {{Lyne}, A.~G. and {McLaughlin}, M.~A. and {Keane}, E.~F. and {Kramer}, M. and {Espinoza}, C.~M. and {Stappers}, B.~W. and {Palliyaguru}, N.~T. and {Miller}, J.},
	Doi = {10.1111/j.1365-2966.2009.15668.x},
	Eprint = {0909.1165},
	Journal = {\mnras},
	Keywords = {pulsars: general},
	Month = dec,
	Pages = {1439-1444},
	Primaryclass = {astro-ph.SR},
	Title = {{Unusual glitch activity in the RRAT J1819-1458: an exhausted magnetar?}},
	Volume = 400,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15668.x}}

@ARTICLE{lyne10,
   author = {{Lyne}, A. and {Hobbs}, G. and {Kramer}, M. and {Stairs}, I. and 
	{Stappers}, B.},
    title = "{Switched Magnetospheric Regulation of Pulsar Spin-Down}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1006.5184},
 primaryClass = "astro-ph.GA",
     year = 2010,
    month = jul,
   volume = 329,
    pages = {408},
      doi = {10.1126/science.1186683},
   adsurl = {http://adsabs.harvard.edu/abs/2010Sci...329..408L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{lyubarsky01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001ApJ...547..437L},
	Author = {{Lyubarsky}, Y. and {Kirk}, J.~G.},
	Doi = {10.1086/318354},
	Eprint = {arXiv:astro-ph/0009270},
	Journal = {\apj},
	Month = jan,
	Pages = {437-448},
	Title = {{Reconnection in a Striped Pulsar Wind}},
	Volume = 547,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/318354}}

@article{lyubarsky02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002MNRAS.332..199L&db_key=AST},
	Author = {{Lyubarsky}, Y.~E.},
	Doi = {10.1046/j.1365-8711.2002.05290.x},
	Journal = {\mnras},
	Month = may,
	Pages = {199-204},
	Title = {{On the X-ray spectra of soft gamma repeaters}},
	Volume = 332,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05290.x}}

@article{let02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...580L..69L&db_key=AST},
	Author = {{Lyubarsky}, Y. and {Eichler}, D. and {Thompson}, C.},
	Journal = {\apjl},
	Month = nov,
	Pages = {L69-L72},
	Title = {{Diagnosing Magnetars with Transient Cooling}},
	Volume = 580,
	Year = 2002}

@article{lyutikov02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...580L..65L&db_key=AST},
	Author = {{Lyutikov}, M.},
	Journal = {\apjl},
	Month = nov,
	Pages = {L65-L68},
	Title = {{Radio Emission from Magnetars}},
	Volume = 580,
	Year = 2002}

@article{lyutikov03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003MNRAS.346..540L&db_key=AST},
	Author = {{Lyutikov}, M.},
	Journal = {\mnras},
	Month = dec,
	Pages = {540-554},
	Title = {{Explosive reconnection in magnetars}},
	Volume = 346,
	Year = 2003}

@article{lyutikov04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353.1095L},
	Author = {{Lyutikov}, M.},
	Doi = {10.1111/j.1365-2966.2004.08129.x},
	Eprint = {arXiv:astro-ph/0403076},
	Journal = {\mnras},
	Month = oct,
	Pages = {1095-1106},
	Title = {{On the nature of eclipses in binary pulsar J0737-3039}},
	Volume = 353,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.08129.x}}

@article{lyutikov05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362.1078L},
	Author = {{Lyutikov}, M.},
	Doi = {10.1111/j.1365-2966.2005.09388.x},
	Eprint = {arXiv:astro-ph/0502503},
	Journal = {\mnras},
	Month = sep,
	Pages = {1078-1084},
	Title = {{Orbital modulation of emission of the binary pulsar J0737-3039B}},
	Volume = 362,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09388.x}}

@article{lt05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1223L},
	Author = {{Lyutikov}, M. and {Thompson}, C.},
	Doi = {10.1086/432252},
	Eprint = {arXiv:astro-ph/0502333},
	Journal = {\apj},
	Month = dec,
	Pages = {1223-1241},
	Title = {{Magnetospheric Eclipses in the Double Pulsar System PSR J0737-3039}},
	Volume = 634,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432252}}

@article{lyutikov06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368..690L},
	Author = {{Lyutikov}, M. and {Gavriil}, F.~P.},
	Doi = {10.1111/j.1365-2966.2006.10140.x},
	Eprint = {arXiv:astro-ph/0507557},
	Journal = {\mnras},
	Month = may,
	Pages = {690-706},
	Title = {{Resonant cyclotron scattering and Comptonization in neutron star magnetospheres}},
	Volume = 368,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10140.x}}

@ARTICLE{maccarone05,
       author = {{Maccarone}, Thomas J.},
        title = "{An explanation for long flares from extragalactic globular cluster X-ray sources}",
      journal = {\mnras},
     keywords = {stellar dynamics, binaries: close, galaxies: star clusters, X-rays: binaries, Astrophysics},
         year = 2005,
        month = dec,
       volume = {364},
       number = {3},
        pages = {971-976},
          doi = {10.1111/j.1365-2966.2005.09623.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0509619},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.364..971M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{maccarone07,
       author = {{Maccarone}, Thomas J. and {Kundu}, Arunav and {Zepf}, Stephen E. and
         {Rhode}, Katherine L.},
        title = "{A black hole in a globular cluster}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = "2007",
        month = "Jan",
       volume = {445},
       number = {7124},
        pages = {183-185},
          doi = {10.1038/nature05434},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701310},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007Natur.445..183M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mk07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26G....48e..12M},
	Archiveprefix = {arXiv},
	Author = {{Maccarone}, T. and {Knigge}, C.},
	Doi = {10.1111/j.1468-4004.2007.48512.x},
	Eprint = {0709.3732},
	Journal = {Astronomy and Geophysics},
	Month = oct,
	Number = 5,
	Pages = {050000-5},
	Title = {{Compact objects in globular clusters}},
	Volume = 48,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1468-4004.2007.48512.x}}

@ARTICLE{maccarone10,
       author = {{Maccarone}, Thomas J. and {Kundu}, Arunav and {Zepf}, Stephen E. and
         {Rhode}, Katherine L.},
        title = "{Fading of the X-ray flux from the black hole in the NGC 4472 globular cluster RZ 2109}",
      journal = {\mnras},
     keywords = {globular clusters: general, galaxies: star clusters: individual: NGC 4472, X-rays: binaries, stars: binaries, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = nov,
       volume = {409},
       number = {1},
        pages = {L84-L88},
          doi = {10.1111/j.1745-3933.2010.00953.x},
archivePrefix = {arXiv},
       eprint = {1009.2827},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.409L..84M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{maccarone14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.3064M},
	Archiveprefix = {arXiv},
	Author = {{Maccarone}, T.~J. and {Lehmer}, B.~D. and {Leyder}, J.~C. and {Antoniou}, V. and {Hornschemeier}, A. and {Ptak}, A. and {Wik}, D. and {Zezas}, A.},
	Doi = {10.1093/mnras/stu167},
	Eprint = {1401.5425},
	Journal = {\mnras},
	Keywords = {stars: Wolf-Rayet, galaxies: individual: NGC 253, galaxies: starburst, X-rays: binaries},
	Month = apr,
	Pages = {3064-3072},
	Primaryclass = {astro-ph.HE},
	Title = {{A new candidate Wolf-Rayet X-ray binary in NGC 253}},
	Volume = 439,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu167}}

@article{maeda02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...570..671M},
	Author = {{Maeda}, Y. and {Baganoff}, F.~K. and {Feigelson}, E.~D. and {Morris}, M. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Burrows}, D.~N. and {Doty}, J.~P. and {Garmire}, G.~P. and {Pravdo}, S.~H. and {Ricker}, G.~R. and {Townsley}, L.~K.},
	Doi = {10.1086/339773},
	Eprint = {arXiv:astro-ph/0102183},
	Journal = {\apj},
	Keywords = {Galaxy: Center, ISM: Individual: Name: Sagittarius A East, ISM: Supernova Remnants, X-Rays: ISM},
	Month = may,
	Pages = {671-687},
	Title = {{A Chandra Study of Sagittarius A East: A Supernova Remnant Regulating the Activity of Our Galactic Center?}},
	Volume = 570,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/339773}}

@article{magnier92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992A%26AS...96..379M},
	Author = {{Magnier}, E.~A. and {Lewin}, W.~H.~G. and {van Paradijs}, J. and {Hasinger}, G. and {Jain}, A. and {Pietsch}, W. and {Truemper}, J.},
	Journal = {\aaps},
	Keywords = {ANDROMEDA GALAXY, ASTRONOMICAL PHOTOMETRY, CHARGE COUPLED DEVICES, ASTRONOMICAL CATALOGS, COLOR-MAGNITUDE DIAGRAM, SKY SURVEYS (ASTRONOMY), STAR FORMATION, STELLAR MAGNITUDE, X RAY BINARIES},
	Month = dec,
	Pages = {379-388},
	Title = {{BV RI CCD photometry of 361,281 objects in the field of M 31}},
	Volume = 96,
	Year = 1992}

@article{majid04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...609..133M},
	Author = {{Majid}, W.~A. and {Lamb}, R.~C. and {Macomb}, D.~J.},
	Doi = {10.1086/420925},
	Eprint = {arXiv:astro-ph/0312034},
	Journal = {\apj},
	Month = jul,
	Pages = {133-143},
	Title = {{X-Ray Pulsars in the Small Magellanic Cloud}},
	Volume = 609,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/420925}}

@ARTICLE{majid17,
   author = {{Majid}, W.~A. and {Pearlman}, A.~B. and {Dobreva}, T. and {Horiuchi}, S. and 
	{Kocz}, J. and {Lippuner}, J. and {Prince}, T.~A.},
    title = "{Post-outburst Radio Observations of the High Magnetic Field Pulsar PSR J1119-6127}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1612.02868},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: G292.2-0.5, ISM: supernova remnants, pulsars: individual: PSR J1119-6127, stars: magnetars, stars: neutron},
     year = 2017,
    month = jan,
   volume = 834,
      eid = {L2},
    pages = {L2},
      doi = {10.3847/2041-8213/834/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...834L...2M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{makishima84,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1984PASJ...36..679M&db_key=AST},
	Author = {{Makishima}, K. and {Kawai}, N. and {Koyama}, K. and {Shibazaki}, N. and {Nagase}, F. and {Nakagawa}, M.},
	Journal = {\pasj},
	Pages = {679-689},
	Title = {{Discovery of a 437.5-s X-ray pulsation from 4U 1907 + 09}},
	Volume = 36,
	Year = 1984}

@article{makishima90,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1990PASJ...42..295M},
	Author = {{Makishima}, K. and {Ohashi}, T. and {Kawai}, N. and {Matsuoka}, M. and {Koyama}, K. and {Kunieda}, H. and {Tawara}, Y. and {Ushimaru}, N. and {Corbet}, R.~H.~D. and {Inoue}, H. and {Kii}, T. and {Makino}, F. and {Mitsuda}, K. and {Murakami}, T. and {Nagase}, F. and {Ogawara}, Y. and {Tanaka}, Y. and {Kitamoto}, S. and {Miyamoto}, S. and {Tsunemi}, H. and {Yamashita}, K.},
	Journal = {\pasj},
	Keywords = {B STARS, PULSARS, X RAY BINARIES, X RAY SOURCES, ANNUAL VARIATIONS, SPACEBORNE ASTRONOMY, X RAY ASTRONOMY, X RAY SPECTRA},
	Month = apr,
	Pages = {295-315},
	Title = {{Observations of the peculiar hard X-ray transient X0331+53 (V0332+53)}},
	Volume = 42,
	Year = 1990}

@article{makishima00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...535..632M},
	Author = {{Makishima}, K. and {Kubota}, A. and {Mizuno}, T. and {Ohnishi}, T. and {Tashiro}, M. and {Aruga}, Y. and {Asai}, K. and {Dotani}, T. and {Mitsuda}, K. and {Ueda}, Y. and {Uno}, S. and {Yamaoka}, K. and {Ebisawa}, K. and {Kohmura}, Y. and {Okada}, K.},
	Doi = {10.1086/308868},
	Eprint = {arXiv:astro-ph/0001009},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Galaxies: Spiral, X-Rays: Galaxies},
	Month = jun,
	Pages = {632-643},
	Title = {{The Nature of Ultraluminous Compact X-Ray Sources in Nearby Spiral Galaxies}},
	Volume = 535,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308868}}

@article{malheiro12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012PASJ...64...56M},
	Archiveprefix = {arXiv},
	Author = {{Malheiro}, M. and {Rueda}, J.~A. and {Ruffini}, R.},
	Eprint = {1102.0653},
	Journal = {\pasj},
	Keywords = {stars: anomalous X-ray pulsars, stars: magnetars, stars: massive fast rotating highly magnetized white dwarfs, stars: soft gamma ray repeaters},
	Month = jun,
	Pages = {56},
	Primaryclass = {astro-ph.SR},
	Title = {{SGRs and AXPs as Rotation-Powered Massive White Dwarfs}},
	Volume = 64,
	Year = 2012}

@article{manchester95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...445L.137M},
	Author = {{Manchester}, R.~N. and {Johnston}, S. and {Lyne}, A.~G. and {D'Amico}, N. and {Bailes}, M. and {Nicastro}, L.},
	Doi = {10.1086/187908},
	Journal = {\apjl},
	Month = jun,
	Pages = {L137-L140},
	Title = {{Period evolution of PSR B1259-63: Evidence for propeller-torque spindown}},
	Volume = 445,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/187908}}

@article{manchester01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.328...17M},
	Author = {{Manchester}, R.~N. and {Lyne}, A.~G. and {Camilo}, F. and {Bell}, J.~F. and {Kaspi}, V.~M. and {D'Amico}, N. and {McKay}, N.~P.~F. and {Crawford}, F. and {Stairs}, I.~H. and {Possenti}, A. and {Kramer}, M. and {Sheppard}, D.~C.},
	Doi = {10.1046/j.1365-8711.2001.04751.x},
	Eprint = {arXiv:astro-ph/0106522},
	Journal = {\mnras},
	Keywords = {METHODS: OBSERVATIONAL, PULSARS: GENERAL},
	Month = nov,
	Pages = {17-35},
	Title = {{The Parkes multi-beam pulsar survey - I. Observing and data analysis systems, discovery and timing of 100 pulsars}},
	Volume = 328,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2001.04751.x}}

@article{manchester04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004Sci...304..542M},
	Author = {{Manchester}, R.~N.},
	Doi = {10.1126/science.1097649},
	Journal = {Science},
	Month = apr,
	Pages = {542-547},
	Title = {{Observational Properties of Pulsars}},
	Volume = 304,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1097649}}

@article{mkp05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005ApJ...621L..49M},
	Author = {{Manchester}, R.~N. and {Kramer}, M. and {Possenti}, A. and {Lyne}, A.~G. and {Burgay}, M. and {Stairs}, I.~H. and {Hotan}, A.~W. and {McLaughlin}, M.~A. and {Lorimer}, D.~R. and {Hobbs}, G.~B. and {Sarkissian}, J.~M. and {D'Amico}, N. and {Camilo}, F. and {Joshi}, B.~C. and {Freire}, P.~C.~C.},
	Doi = {10.1086/429128},
	Eprint = {arXiv:astro-ph/0501665},
	Journal = {\apjl},
	Month = mar,
	Pages = {L49-L52},
	Title = {{The Mean Pulse Profile of PSR J0737-3039A}},
	Volume = 621,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/429128}}

@INPROCEEDINGS{manchester07,
   author = {{Manchester}, R.~N.},
    title = "{Searching for a Pulsar in SN1987A}",
 keywords = {Supernovae, Pulsars, Neutron stars},
booktitle = {Supernova 1987A: 20 Years After: Supernovae and Gamma-Ray Bursters},
     year = 2007,
	Publisher = {AIP, Melville},
   series = {American Institute of Physics Conference Series},
   volume = 937,
archivePrefix = "arXiv",
   eprint = {0708.2372},
   editor = {{Immler}, S. and {Weiler}, K. and {McCray}, R.},
    month = oct,
    pages = {134-143},
      doi = {10.1063/1.3682894},
   adsurl = {http://adsabs.harvard.edu/abs/2007AIPC..937..134M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mandea06,
   author = {{Mandea}, M. and {Balasis}, G.},
    title = "{FAST TRACK PAPER: The SGR 1806-20 magnetar signature on the Earth's magnetic field}",
  journal = {Geophysical Journal International},
archivePrefix = "arXiv",
   eprint = {0710.2793},
 keywords = {geomagnetic field, magnetar, wavelet analysis},
     year = 2006,
    month = nov,
   volume = 167,
    pages = {586-591},
      doi = {10.1111/j.1365-246X.2006.03125.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006GeoJI.167..586M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{manousakis11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A..62M},
	Archiveprefix = {arXiv},
	Author = {{Manousakis}, A. and {Walter}, R.},
	Doi = {10.1051/0004-6361/201015707},
	Eid = {A62},
	Eprint = {1008.5362},
	Journal = {\aap},
	Keywords = {X-rays: binaries, stars: winds, outflows, pulsars: individual: IGR J17252-3616, supergiants},
	Month = feb,
	Pages = {A62},
	Primaryclass = {astro-ph.HE},
	Title = {{X-ray wind tomography of the highly absorbed HMXB IGR J17252-3616}},
	Volume = 526,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201015707}}

@article{mapelli09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.395L..71M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Colpi}, M. and {Zampieri}, L.},
	Doi = {10.1111/j.1745-3933.2009.00645.x},
	Eprint = {0902.3540},
	Journal = {\mnras},
	Keywords = {black hole physics, galaxies: individual: Cartwheel, galaxies: starburst, X-rays: binaries, X-rays: galaxies},
	Month = may,
	Pages = {L71-L75},
	Primaryclass = {astro-ph.HE},
	Title = {{Low metallicity and ultra-luminous X-ray sources in the Cartwheel galaxy}},
	Volume = 395,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2009.00645.x}}

@article{mapelli10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408..234M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Ripamonti}, E. and {Zampieri}, L. and {Colpi}, M. and {Bressan}, A.},
	Doi = {10.1111/j.1365-2966.2010.17048.x},
	Eprint = {1005.3548},
	Journal = {\mnras},
	Keywords = {black hole physics, galaxies: starburst, X-rays: binaries, X-rays: galaxies},
	Month = oct,
	Pages = {234-253},
	Primaryclass = {astro-ph.CO},
	Title = {{Ultra-luminous X-ray sources and remnants of massive metal-poor stars}},
	Volume = 408,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17048.x}}

@article{mhm10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...719..987M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Huwyler}, C. and {Mayer}, L. and {Jetzer}, P. and {Vecchio}, A.},
	Doi = {10.1088/0004-637X/719/2/987},
	Eprint = {1006.1664},
	Journal = {\apj},
	Keywords = {binaries: general, black hole physics, galaxies: star clusters: general, gravitational waves, stars: kinematics and dynamics},
	Month = aug,
	Pages = {987-995},
	Title = {{Gravitational Waves from Intermediate-mass Black Holes in Young Clusters}},
	Volume = 719,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/719/2/987}}

@article{mapelli11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416.1756M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Ripamonti}, E. and {Zampieri}, L. and {Colpi}, M.},
	Doi = {10.1111/j.1365-2966.2011.18991.x},
	Eprint = {1105.0681},
	Journal = {\mnras},
	Keywords = {black hole physics, binaries: general, galaxies: star clusters: general, X-rays: binaries},
	Month = sep,
	Pages = {1756-1763},
	Primaryclass = {astro-ph.CO},
	Title = {{Dynamics of massive stellar black holes in young star clusters and the displacement of ultra-luminous X-ray sources}},
	Volume = 416,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.18991.x}}

@article{mrzc11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AN....332..414M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Ripamonti}, E. and {Zampieri}, L. and {Colpi}, M.},
	Doi = {10.1002/asna.201011511},
	Eprint = {1009.5706},
	Journal = {Astronomische Nachrichten},
	Keywords = {black hole physics, galaxies: starburst, X-rays: binaries, X-rays: galaxies},
	Month = may,
	Pages = {414},
	Primaryclass = {astro-ph.CO},
	Title = {{Remnants of massive metal-poor stars: Viable engines for ultra-luminous X-ray sources}},
	Volume = 332,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.201011511}}

@article{mapelli12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...542A.102M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Ripamonti}, E. and {Vecchio}, A. and {Graham}, A.~W. and {Gualandris}, A.},
	Doi = {10.1051/0004-6361/201118444},
	Eid = {A102},
	Eprint = {1205.2702},
	Journal = {\aap},
	Keywords = {gravitational waves, black hole physics, galaxies: nuclei, galaxies: star clusters: general, cosmology: theory},
	Month = jun,
	Pages = {A102},
	Primaryclass = {astro-ph.CO},
	Title = {{A cosmological view of extreme mass-ratio inspirals in nuclear star clusters}},
	Volume = 542,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201118444}}

@article{mapelli13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.429.2298M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Zampieri}, L. and {Ripamonti}, E. and {Bressan}, A.},
	Doi = {10.1093/mnras/sts500},
	Eprint = {1211.6441},
	Journal = {\mnras},
	Keywords = {black hole physics, methods: numerical, binaries: general, stars: kinematics and dynamics, galaxies: star clusters: general, X-rays: binaries},
	Month = mar,
	Pages = {2298-2314},
	Primaryclass = {astro-ph.HE},
	Title = {{Dynamics of stellar black holes in young star clusters with different metallicities - I. Implications for X-ray binaries}},
	Volume = 429,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts500}}

@article{mapelli14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794....7M},
	Archiveprefix = {arXiv},
	Author = {{Mapelli}, M. and {Zampieri}, L.},
	Doi = {10.1088/0004-637X/794/1/7},
	Eid = {7},
	Eprint = {1408.1406},
	Journal = {\apj},
	Keywords = {binaries: general, black hole physics, galaxies: star clusters: general, methods: numerical, stars: kinematics and dynamics, X-rays: binaries},
	Month = oct,
	Pages = {7},
	Primaryclass = {astro-ph.HE},
	Title = {{Roche-lobe Overflow Systems Powered by Black Holes in Young Star Clusters: The Importance of Dynamical Exchanges}},
	Volume = 794,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/794/1/7}}

@article{maraschi81,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981MNRAS.194P...1M&db_key=AST},
	Author = {{Maraschi}, L. and {Treves}, A.},
	Journal = {\mnras},
	Month = jan,
	Pages = {1P-5P},
	Title = {{A model for LSI61 deg 303}},
	Volume = 194,
	Year = 1981}

@ARTICLE{marelli17,
   author = {{Marelli}, M. and {Tiengo}, A. and {De Luca}, A. and {Salvetti}, D. and 
	{Saronni}, L. and {Sidoli}, L. and {Paizis}, A. and {Salvaterra}, R. and 
	{Belfiore}, A. and {Israel}, G. and {Haberl}, F. and {D'Agostino}, D.
	},
    title = "{Discovery of Periodic Dips in the Brightest Hard X-Ray Source of M31 with EXTraS}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1711.05540},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: bulges, galaxies: individual: M31, pulsars: general, stars: neutron, X-rays: binaries },
     year = 2017,
    month = dec,
   volume = 851,
      eid = {L27},
    pages = {L27},
      doi = {10.3847/2041-8213/aa9b2e},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...851L..27M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{marlborough69,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1969ApJ...156..135M},
	Author = {{Marlborough}, J.~M.},
	Doi = {10.1086/149954},
	Journal = {\apj},
	Month = apr,
	Pages = {135},
	Title = {{Models for the Envelopes of be Stars}},
	Volume = 156,
	Year = 1969,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/149954}}

@article{marsden98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998ApJ...502L.129M&db_key=AST},
	Author = {{Marsden}, D. and {Gruber}, D.~E. and {Heindl}, W.~A. and {Pelling}, M.~R. and {Rothschild}, R.~E.},
	Doi = {10.1086/311510},
	Journal = {\apjl},
	Month = aug,
	Pages = {L129},
	Title = {{Discovery of a New 89 Second X-Ray Pulsar: XTE J1906+09}},
	Volume = 502,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311510}}

@article{marsden01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...551L.155M&db_key=AST},
	Author = {{Marsden}, D. and {White}, N.~E.},
	Journal = {\apjl},
	Month = apr,
	Pages = {L155-L158},
	Title = {{Correlations between Spectral Properties and Spin-down Rate in Soft Gamma-Ray Repeaters and Anomalous X-Ray Pulsars}},
	Volume = 551,
	Year = 2001}

@article{marsh02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.331L...7M},
	Author = {{Marsh}, T.~R. and {Steeghs}, D.},
	Doi = {10.1046/j.1365-8711.2002.05346.x},
	Eprint = {arXiv:astro-ph/0201309},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, gravitational waves, binaries: close, stars: individual: V407 Vul, novae, cataclysmic variables, white dwarfs},
	Month = mar,
	Pages = {L7-L11},
	Title = {{V407 Vul: a direct impact accretor}},
	Volume = 331,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05346.x}}

@article{martayan10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...509A..11M},
	Archiveprefix = {arXiv},
	Author = {{Martayan}, C. and {Baade}, D. and {Fabregat}, J.},
	Doi = {10.1051/0004-6361/200911672},
	Eid = {A11},
	Eprint = {0909.2303},
	Journal = {\aap},
	Keywords = {stars: early-type, stars: emission-line, Be, stars: fundamental parameters, stars: evolution, magellanic clouds, catalogs},
	Month = jan,
	Pages = {A11},
	Primaryclass = {astro-ph.CO},
	Title = {{A slitless spectroscopic survey for H{$\alpha$} emission-line objects in SMC clusters}},
	Volume = 509,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200911672}}

@article{marti95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...298..151M&db_key=AST},
	Author = {{Marti}, J. and {Paredes}, J.~M.},
	Journal = {\aap},
	Month = jun,
	Pages = {151},
	Title = {{Modelling of LSI+61 303 from near infrared data.}},
	Volume = 298,
	Year = 1995}

@ARTICLE{martin14,
   author = {{Martin}, J. and {Rea}, N. and {Torres}, D.~F. and {Papitto}, A.
	},
    title = "{Comparing supernova remnants around strongly magnetized and canonical pulsars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.1027},
 primaryClass = "astro-ph.HE",
 keywords = {line: identification, stars: magnetars, pulsars: general, ISM: supernova remnants, X-rays: general},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {2910-2924},
      doi = {10.1093/mnras/stu1594},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.2910M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{masada10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010PASJ...62.1093M},
	Author = {{Masada}, Y. and {Nagataki}, S. and {Shibata}, K. and {Terasawa}, T.},
	Journal = {\pasj},
	Keywords = {stars: individual (SGR 1806-20), stars: magnetic fields, stars: neutron},
	Month = aug,
	Pages = {1093-1102},
	Title = {{Solar-Type Magnetic Reconnection Model for Magnetar Giant Flares}},
	Volume = 62,
	Year = 2010}

@article{masetti06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...459...21M},
	Author = {{Masetti}, N. and {Morelli}, L. and {Palazzi}, E. and {Galaz}, G. and {Bassani}, L. and {Bazzano}, A. and {Bird}, A.~J. and {Dean}, A.~J. and {Israel}, G.~L. and {Landi}, R. and {Malizia}, A. and {Minniti}, D. and {Schiavone}, F. and {Stephen}, J.~B. and {Ubertini}, P. and {Walter}, R.},
	Doi = {10.1051/0004-6361:20066055},
	Eprint = {arXiv:astro-ph/0608394},
	Journal = {\aap},
	Keywords = {galaxies: Seyfert, stars: novae, cataclysmic variables, X-rays: binaries, techniques: spectroscopic, X-rays: general},
	Month = nov,
	Pages = {21-30},
	Title = {{Unveiling the nature of INTEGRAL objects through optical spectroscopy. V. Identification and properties of 21 southern hard X-ray sources}},
	Volume = 459,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066055}}

@article{mop06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...453..295M},
	Author = {{Masetti}, N. and {Orlandini}, M. and {Palazzi}, E. and {Amati}, L. and {Frontera}, F.},
	Doi = {10.1051/0004-6361:20065025},
	Eprint = {astro-ph/0603227},
	Journal = {\aap},
	Keywords = {astrometry, stars: binaries: general, X-rays: binaries, stars: neutron, stars: individuals: 4U 1700+24, stars: individual: 4U 1954+319},
	Month = jul,
	Pages = {295-299},
	Title = {{M-type giants as optical counterparts of X-ray sources 4U 1700+24 and 4U 1954+319}},
	Volume = 453,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065025}}

@article{masetti12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ATel.4248....1M},
	Author = {{Masetti}, N. and {Jimenez-Bailon}, E. and {Chavushyan}, V. and {Parisi}, P. and {Bazzano}, A. and {Landi}, R. and {Bird}, A.~J.},
	Journal = {Astron. Tel.},
	Keywords = {Optical, X-ray, Binary, Neutron Star, Star, Pulsar},
	Month = jul,
	Title = {{Optical spectroscopy of X-ray source IGR J22534+6243}},
	Volume = 4248,
	Year = 2012}

@article{mason82,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...262..253M},
	Author = {{Mason}, K.~O. and {Cordova}, F.~A.},
	Doi = {10.1086/160416},
	Journal = {\apj},
	Keywords = {BINARY STARS, INFRARED ASTRONOMY, INFRARED PHOTOMETRY, LIGHT CURVE, STELLAR MODELS, STELLAR SPECTROPHOTOMETRY, ULTRAVIOLET SPECTRA, VISIBLE SPECTRUM, X RAY SOURCES, EMISSION SPECTRA, FAR ULTRAVIOLET RADIATION, NEAR INFRARED RADIATION, OPTICAL EMISSION SPECTROSCOPY, SPECTRAL BANDS, STELLAR MASS ACCRETION},
	Month = nov,
	Pages = {253-262},
	Title = {{Infrared photometry of the X-ray binary 2A 1822-371 - A model for the ultraviolet, optical, and infrared light curve}},
	Volume = 262,
	Year = 1982,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160416}}

@article{mason01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...365L..36M},
	Author = {{Mason}, K.~O. and {Breeveld}, A. and {Much}, R. and {Carter}, M. and {Cordova}, F.~A. and {Cropper}, M.~S. and {Fordham}, J. and {Huckle}, H. and {Ho}, C. and {Kawakami}, H. and {Kennea}, J. and {Kennedy}, T. and {Mittaz}, J. and {Pandel}, D. and {Priedhorsky}, W.~C. and {Sasseen}, T. and {Shirey}, R. and {Smith}, P. and {Vreux}, J.-M.},
	Doi = {10.1051/0004-6361:20000044},
	Eprint = {astro-ph/0011216},
	Journal = {\aap},
	Keywords = {SPACE VEHICLES: INSTRUMENTS, INSTRUMENTATION: DETECTORS, ULTRAVIOLET: GENERAL},
	Month = jan,
	Pages = {L36-L44},
	Title = {{The XMM-Newton optical/UV monitor telescope}},
	Volume = 365,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000044}}

@article{mason10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1003.1986M},
	Archiveprefix = {arXiv},
	Author = {{Mason}, E. and {Israel}, G.~L. and {Dall'Osso}, S. and {Stella}, L. and {Munari}, U. and {Marconi}, G. and {O'Brian}, K. and {Covino}, S. and {Fugazza}, D.},
	Eprint = {1003.1986},
	Journal = {eprint: astro-ph/1003.1986},
	Keywords = {Astrophysics - Galaxy Astrophysics},
	Month = mar,
	Title = {{VLT Phase Resolved Optical Spectroscopy of the Ultra-Compact Binary HM Cnc}},
	Year = 2010}

@article{massaro06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...455..153M},
	Author = {{Massaro}, F. and {Bianchi}, S. and {Matt}, G. and {D'Onofrio}, E. and {Nicastro}, F.},
	Doi = {10.1051/0004-6361:20054772},
	Journal = {\aap},
	Keywords = {galaxies: nuclei, galaxies: Seyfert, X-rays: individuals: Circinus Galaxy},
	Month = aug,
	Pages = {153-159},
	Title = {{The properties of the circumnuclear regions in the Circinus galaxy}},
	Volume = 455,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054772}}

@article{massey03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ARA%26A..41...15M},
	Author = {{Massey}, P.},
	Doi = {10.1146/annurev.astro.41.071601.170033},
	Journal = {\araa},
	Pages = {15-56},
	Title = {{MASSIVE STARS IN THE LOCAL GROUP: Implications for Stellar Evolution and Star Formation}},
	Volume = 41,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.41.071601.170033}}

@article{massey06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.2478M},
	Author = {{Massey}, P. and {Olsen}, K.~A.~G. and {Hodge}, P.~W. and {Strong}, S.~B. and {Jacoby}, G.~H. and {Schlingman}, W. and {Smith}, R.~C.},
	Doi = {10.1086/503256},
	Eprint = {astro-ph/0602128},
	Journal = {\aj},
	Keywords = {Catalogs, Galaxies: Individual: Messier Number: M31, Galaxies: Individual: Messier Number: M33, Galaxies: Stellar Content, Stars: Early-Type, Stars: Supergiants, Surveys},
	Month = may,
	Pages = {2478-2496},
	Title = {{A Survey of Local Group Galaxies Currently Forming Stars. I. UBVRI Photometry of Stars in M31 and M33}},
	Volume = 131,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/503256}}

@article{massi01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001A%26A...376..217M&db_key=AST},
	Author = {{Massi}, M. and {Rib{\'o}}, M. and {Paredes}, J.~M. and {Peracaula}, M. and {Estalella}, R.},
	Doi = {10.1051/0004-6361:20010953},
	Eprint = {astro-ph/0107093},
	Journal = {\aap},
	Month = sep,
	Pages = {217-223},
	Title = {{One-sided jet at milliarcsecond scales in <ASTROBJ>LS I +61deg303</ASTROBJ>}},
	Volume = 376,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20010953}}

@article{massi04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004A%26A...414L...1M},
	Author = {{Massi}, M. and {Rib{\'o}}, M. and {Paredes}, J.~M. and {Garrington}, S.~T. and {Peracaula}, M. and {Mart{\'{\i}}}, J.},
	Doi = {10.1051/0004-6361:20031760},
	Eprint = {arXiv:astro-ph/0312091},
	Journal = {\aap},
	Month = jan,
	Pages = {L1-L4},
	Title = {{Hints for a fast precessing relativistic radio jet in LS I +61^{$\,^{\circ}$}303}},
	Volume = 414,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031760}}

@article{massi04rn,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004A%26A...422..267M&db_key=AST},
	Author = {{Massi}, M.},
	Doi = {10.1051/0004-6361:20047145},
	Eprint = {astro-ph/0404605},
	Journal = {\aap},
	Month = jul,
	Pages = {267-270},
	Title = {{LS I +61{\deg}303 in the context of microquasars}},
	Volume = 422,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20047145}}

@article{massi05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005astro.ph..6731M},
	Author = {{Massi}, M.},
	Eprint = {astro-ph/0506731},
	Journal = {preprint (astro-ph/0506731)},
	Month = jun,
	Title = {{Introduction to Astrophysics of Microquasars}},
	Year = 2005}

@article{mrpg04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004A%26A...414L...1M&db_key=AST},
	Author = {{Massi}, M. and {Rib{\'o}}, M. and {Paredes}, J.~M. and {Garrington}, S.~T. and {Peracaula}, M. and {Mart{\'{\i}}}, J.},
	Doi = {10.1051/0004-6361:20031760},
	Eprint = {astro-ph/0312091},
	Journal = {\aap},
	Month = jan,
	Pages = {L1-L4},
	Title = {{Hints for a fast precessing relativistic radio jet in LS I +61^{$\,^{\circ}$}303}},
	Volume = 414,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20031760}}

@article{mathewson83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJS...51..345M},
	Author = {{Mathewson}, D.~S. and {Ford}, V.~L. and {Dopita}, M.~A. and {Tuohy}, I.~R. and {Long}, K.~S. and {Helfand}, D.~J.},
	Doi = {10.1086/190854},
	Journal = {\apjs},
	Keywords = {ASTRONOMICAL CATALOGS, LIGHT (VISIBLE RADIATION), MAGELLANIC CLOUDS, RADIO SOURCES (ASTRONOMY), SUPERNOVA REMNANTS, X RAY SOURCES, HIGH RESOLUTION, PROPORTIONAL COUNTERS, SPECTRAL RESOLUTION, STELLAR EVOLUTION},
	Month = apr,
	Pages = {345-355},
	Title = {{Supernova remnants in the Magellanic Clouds}},
	Volume = 51,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/190854}}

@article{mathis77,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
	Author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
	Doi = {10.1086/155591},
	Journal = {\apj},
	Keywords = {COSMIC DUST, INTERSTELLAR EXTINCTION, INTERSTELLAR MATTER, PARTICLE SIZE DISTRIBUTION, ENSTATITE, GRAPHITE, MAGNETITE, OLIVINE, POLARIZATION CHARACTERISTICS, ULTRAVIOLET ASTRONOMY},
	Month = oct,
	Pages = {425-433},
	Title = {{The size distribution of interstellar grains}},
	Volume = 217,
	Year = 1977,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/155591}}

@ARTICLE{mathis91,
   author = {{Mathis}, J.~S. and {Lee}, C.-W.},
    title = "{X-ray halos as diagnostics of interstellar grains}",
  journal = {\apj},
 keywords = {Halos, Interstellar Matter, X Ray Sources, Galactic Structure, Grains},
     year = 1991,
    month = aug,
   volume = 376,
    pages = {490-499},
      doi = {10.1086/170297},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...376..490M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{matsuura11,
   author = {{Matsuura}, M. and {Dwek}, E. and {Meixner}, M. and {Otsuka}, M. and 
	{Babler}, B. and {Barlow}, M.~J. and {Roman-Duval}, J. and {Engelbracht}, C. and 
	{Sandstrom}, K. and {Laki{\'c}evi{\'c}}, M. and {van Loon}, J.~T. and 
	{Sonneborn}, G. and {Clayton}, G.~C. and {Long}, K.~S. and {Lundqvist}, P. and 
	{Nozawa}, T. and {Gordon}, K.~D. and {Hony}, S. and {Panuzzo}, P. and 
	{Okumura}, K. and {Misselt}, K.~A. and {Montiel}, E. and {Sauvage}, M.
	},
    title = "{Herschel Detects a Massive Dust Reservoir in Supernova 1987A}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1107.1477},
 primaryClass = "astro-ph.SR",
     year = 2011,
    month = sep,
   volume = 333,
    pages = {1258},
      doi = {10.1126/science.1205983},
   adsurl = {http://adsabs.harvard.edu/abs/2011Sci...333.1258M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{matsuura17,
   author = {{Matsuura}, M. and {Indebetouw}, R. and {Woosley}, S. and {Bujarrabal}, V. and 
	{Abellan}, F.~J. and {McCray}, R. and {Kamenetzky}, J. and {Fransson}, C. and 
	{Barlow}, M.~J. and {Gomez}, H.~L. and {Cigan}, P. and {De Looze}, I and 
	{Spyromilio}, J. and {Staveley-Smith}, L. and {Zanardo}, G. and 
	{Roche}, P. and {Larsson}, J. and {Viti}, S. and {van Loon}, J.~T. and 
	{Wheeler}, J.~C. and {Baes}, M. and {Chevalier}, R. and {Lundqvist}, P. and 
	{Marcaide}, J.~M. and {Dwek}, E. and {Meixner}, M. and {Ng}, C.-Y. and 
	{Sonneborn}, G. and {Yates}, J.},
    title = "{ALMA spectral survey of Supernova 1987A --- molecular inventory, chemistry, dynamics and explosive nucleosynthesis}",
  journal = {\mnras, in press (preprint: astro-ph/1704.02324)},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
     year = 2017,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170402324M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{matt96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.281L..69M},
	Author = {{Matt}, G. and {Fiore}, F. and {Perola}, G.~C. and {Piro}, L. and {Fink}, H.~H. and {Grandi}, P. and {Matsuoka}, M. and {Oliva}, E. and {Salvati}, M.},
	Journal = {\mnras},
	Keywords = {LINE: FORMATION, LINE: IDENTIFICATION, GALAXIES: INDIVIDUAL: CIRCINUS, GALAXIES: SEYFERT, X-RAYS: GALAXIES},
	Month = aug,
	Pages = {L69-L73},
	Title = {{A reflection-dominated X-ray spectrum discovered by ASCA in the Circinus galaxy}},
	Volume = 281,
	Year = 1996}

@article{mattana06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460L...1M},
	Author = {{Mattana}, F. and {G{\"o}tz}, D. and {Falanga}, M. and {Senziani}, F. and {de Luca}, A. and {Esposito}, P. and {Caraveo}, P.~A.},
	Doi = {10.1051/0004-6361:20066154},
	Eprint = {astro-ph/0610158},
	Journal = {\aap},
	Keywords = {binaries: close, pulsars: individual: 4U 1954+319, stars: neutron, X-rays: binaries},
	Month = dec,
	Pages = {L1-L4},
	Title = {{A new symbiotic low mass X-ray binary system: 4U 1954+319}},
	Volume = 460,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066154}}

@article{mattana09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...694...12M},
	Archiveprefix = {arXiv},
	Author = {{Mattana}, F. and {Falanga}, M. and {G{\"o}tz}, D. and {Terrier}, R. and {Esposito}, P. and {Pellizzoni}, A. and {De Luca}, A. and {Marandon}, V. and {Goldwurm}, A. and {Caraveo}, P.~A.},
	Doi = {10.1088/0004-637X/694/1/12},
	Eprint = {0811.0327},
	Journal = {\apj},
	Keywords = {gamma rays: observations, pulsars: general, radiation mechanisms: non-thermal, supernova remnants, X-rays: stars},
	Month = mar,
	Pages = {12-17},
	Title = {{The Evolution of the {$\gamma$}- and X-Ray Luminosities of Pulsar Wind Nebulae}},
	Volume = 694,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/694/1/12}}

@article{mgg79,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1979SvAL....5..343M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Golenetskii}, S.~V. and {Guryan}, Y.~A.},
	Journal = {Soviet Astronomy Letters},
	Month = dec,
	Pages = {343},
	Title = {{Soft gamma-ray bursts from the source B1900+14}},
	Volume = 5,
	Year = 1979}

@article{mazets79,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979Natur.282..587M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Golentskii}, S.~V. and {Ilinskii}, V.~N. and {Aptekar}, R.~L. and {Guryan}, I.~A.},
	Journal = {\nat},
	Month = dec,
	Pages = {587-589},
	Title = {{Observations of a flaring X-ray pulsar in Dorado}},
	Volume = 282,
	Year = 1979}

@article{mazets82,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1982Ap%26SS..84..173M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Golenetskii}, S.~V. and {Gurian}, I.~A. and {Ilinskii}, V.~N.},
	Journal = {\apss},
	Month = may,
	Pages = {173-189},
	Title = {{The 5 March 1979 event and the distinct class of short gamma bursts Are they of the same origin}},
	Volume = 84,
	Year = 1982}

@article{mazets99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...519L.151M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Aptekar}, R.~L. and {Butterworth}, P.~S. and {Cline}, T.~L. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Hurley}, K. and {Il'Inskii}, V.~N.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L151-L153},
	Title = {{Unusual Burst Emission from the New Soft Gamma Repeater SGR 1627-41}},
	Volume = 519,
	Year = 1999}

@article{mca99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999AstL...25..628M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Cline}, T.~L. and {Aptekar}, R.~L. and {Butterworth}, P.~S. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Il'Inskii}, V.~N. and {Pal'Shin}, V.~D.},
	Journal = {Astron.~Lett.},
	Month = oct,
	Pages = {628-634},
	Title = {{Activity of the soft gamma repeater SGR 1900 + 14 in 1998 from Konus-Wind observations: 1. Short recurrent bursts}},
	Volume = 25,
	Year = 1999}

@article{mca99_2,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999AstL...25..635M&db_key=AST},
	Author = {{Mazets}, E.~P. and {Cline}, T.~L. and {Aptekar'}, R.~L. and {Butterworth}, P.~S. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Il'Inskii}, V.~N. and {Pal'Shin}, V.~D.},
	Eprint = {astro-ph/9905196},
	Journal = {Astron.~Lett.},
	Month = oct,
	Pages = {635-648},
	Title = {{Activity of the soft gamma repeater SGR 1900 + 14 in 1998 from Konus-Wind observations: 2. The giant August 27 outburst}},
	Volume = 25,
	Year = 1999}

@article{mazets04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2922....1M&db_key=AST},
	Author = {{Mazets}, E. and {Golenetskii}, S. and {Aptekar}, R. and {Frederiks}, D. and {Pal'Shin}, V. and {Cline}, T.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{The giant outburst from Sgr 1806-20.}},
	Volume = 2922,
	Year = 2004}

@article{mazets05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005astro.ph..2541M&db_key=PRE},
	Author = {{Mazets}, E.~P. and {Cline}, T.~L. and {Aptekar}, R.~L. and {Frederiks}, D.~D. and {Golenetskii}, S.~V. and {Il'inskii}, V.~N. and {Pal'shin}, V.~D.},
	Eprint = {astro-ph/0502541},
	Journal = {ArXiv Astrophysics e-prints, [ArXiv: astro-ph/0502541]},
	Month = feb,
	Title = {{The Konus-Wind and Helicon-Coronas-F detection of the giant \$$\backslash$gamma\$-ray flare from the soft \$$\backslash$gamma\$-ray repeater SGR 1806-20}},
	Year = 2005}

@article{mcbride08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1198M},
	Archiveprefix = {arXiv},
	Author = {{McBride}, V.~A. and {Coe}, M.~J. and {Negueruela}, I. and {Schurch}, M.~P.~E. and {McGowan}, K.~E.},
	Doi = {10.1111/j.1365-2966.2008.13410.x},
	Eprint = {0805.0008},
	Journal = {\mnras},
	Keywords = {binaries: general , emission-line, Be , Magellanic Clouds},
	Month = aug,
	Pages = {1198-1204},
	Title = {{Spectral distribution of Be/X-ray binaries in the Small Magellanic Cloud}},
	Volume = 388,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13410.x}}

@inbook{mcclintock06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006csxs.book..157M&db_key=AST},
	Author = {{McClintock}, J.~E. and {Remillard}, R.~A.},
	Month = apr,
	Pages = {157},
	Publisher = {Cambridge: Cambridge University Press},
	Title = {{in Compact stellar X-ray sources, ed. W. H. G. Levin and M. van der Klis}},
	Year = 2006}

@article{mcclure05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...630L.161M&db_key=AST},
	Author = {{McClure-Griffiths}, N.~M. and {Gaensler}, B.~M.},
	Doi = {10.1086/496879},
	Journal = {\apjl},
	Month = sep,
	Pages = {L161-L163},
	Title = {{Constraints on the Distance to SGR 1806-20 from H I Absorption}},
	Volume = 630,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/496879}}

@ARTICLE{mccray93,
   author = {{McCray}, R.},
    title = "{Supernova 1987A revisited}",
  journal = {\araa},
 keywords = {Light Curve, Stellar Envelopes, Stellar Spectra, Supernova 1987a, Electromagnetic Spectra, Gamma Ray Spectra, X Ray Sources},
     year = 1993,
   volume = 31,
    pages = {175-216},
      doi = {10.1146/annurev.aa.31.090193.001135},
   adsurl = {http://adsabs.harvard.edu/abs/1993ARA%26A..31..175M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{mccray07,
   author = {{McCray}, R.},
    title = "{Supernova 1987A at Age 20}",
 keywords = {Supernova remnants, Astronomical observations, Supernovae},
booktitle = {Supernova 1987A: 20 Years After: Supernovae and Gamma-Ray Bursters},
     year = 2007,
	Publisher = {AIP, Melville},
   series = {American Institute of Physics Conference Series},
   volume = 937,
   editor = {{Immler}, S. and {Weiler}, K. and {McCray}, R.},
    month = oct,
    pages = {3-14},
      doi = {10.1063/1.3682877},
   adsurl = {http://adsabs.harvard.edu/abs/2007AIPC..937....3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mccray16,
   author = {{McCray}, R. and {Fransson}, C.},
    title = "{The Remnant of Supernova 1987A}",
  journal = {\araa},
     year = 2016,
    month = sep,
   volume = 54,
    pages = {19-52},
      doi = {10.1146/annurev-astro-082615-105405},
   adsurl = {http://adsabs.harvard.edu/abs/2016ARA%26A..54...19M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mcgarry05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...627L.137M&db_key=AST},
	Author = {{McGarry}, M.~B. and {Gaensler}, B.~M. and {Ransom}, S.~M. and {Kaspi}, V.~M. and {Veljkovik}, S.},
	Doi = {10.1086/432441},
	Journal = {\apjl},
	Month = jul,
	Pages = {L137-L140},
	Title = {{X-Ray Timing, Spectroscopy, and Photometry of the Anomalous X-Ray Pulsar Candidate CXOU J010043.1-721134}},
	Volume = 627,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/432441}}

@article{mcgowan04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...600..343M},
	Author = {{McGowan}, K.~E. and {Zane}, S. and {Cropper}, M. and {Kennea}, J.~A. and {C{\'o}rdova}, F.~A. and {Ho}, C. and {Sasseen}, T. and {Vestrand}, W.~T.},
	Doi = {10.1086/379787},
	Eprint = {arXiv:astro-ph/0309445},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: Individual: Alphanumeric: PSR B1706-44, Stars: Neutron, X-Rays: Stars},
	Month = jan,
	Pages = {343-350},
	Title = {{XMM-Newton Observations of PSR B1706-44}},
	Volume = 600,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379787}}

@inproceedings{mchardy96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..110..293M},
	Author = {{McHardy}, I.},
	Booktitle = {Blazar Continuum Variability},
	Editor = {{Miller}, H.~R. and {Webb}, J.~R. and {Noble}, J.~C.},
	Pages = {293},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{X-ray Variability of Blazars}},
	Volume = 110,
	Year = 1996}

@article{mchardy06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006Natur.444..730M},
	Author = {{McHardy}, I.~M. and {Koerding}, E. and {Knigge}, C. and {Uttley}, P. and {Fender}, R.~P.},
	Doi = {10.1038/nature05389},
	Eprint = {arXiv:astro-ph/0612273},
	Journal = {\nat},
	Month = dec,
	Pages = {730-732},
	Title = {{Active galactic nuclei as scaled-up Galactic black holes}},
	Volume = 444,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature05389}}

@inproceedings{mclaughlin00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2000ASPC..202..359M},
	Author = {{McLaughlin}, M. and {Cordes}, J.},
	Booktitle = {IAU Colloq. 177: Pulsar Astronomy - 2000 and Beyond},
	Editor = {{Kramer}, M. and {Wex}, N. and {Wielebinski}, R.},
	Pages = {359},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{Gamma Ray Pulsar Luminosities}},
	Volume = 202,
	Year = 2000}

@article{mclaughlin02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...564..333M},
	Author = {{McLaughlin}, M.~A. and {Arzoumanian}, Z. and {Cordes}, J.~M. and {Backer}, D.~C. and {Lommen}, A.~N. and {Lorimer}, D.~R. and {Zepka}, A.~F.},
	Doi = {10.1086/324151},
	Eprint = {arXiv:astro-ph/0106371},
	Journal = {\apj},
	Month = jan,
	Pages = {333-342},
	Title = {{PSR J1740+1000: A Young Pulsar Well Out of the Galactic Plane}},
	Volume = 564,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324151}}

@article{mclaughlin04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605L..41M},
	Author = {{McLaughlin}, M.~A. and {Camilo}, F. and {Burgay}, M. and {D'Amico}, N. and {Joshi}, B.~C. and {Kramer}, M. and {Lorimer}, D.~R. and {Lyne}, A.~G. and {Manchester}, R.~N. and {Possenti}, A.},
	Doi = {10.1086/392511},
	Eprint = {arXiv:astro-ph/0402518},
	Journal = {\apjl},
	Month = apr,
	Pages = {L41-L44},
	Title = {{X-Ray Emission from the Double Pulsar System J0737-3039}},
	Volume = 605,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/392511}}

@article{mclaughlin04a,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616L.131M},
	Author = {{McLaughlin}, M.~A. and {Lyne}, A.~G. and {Lorimer}, D.~R. and {Possenti}, A. and {Manchester}, R.~N. and {Camilo}, F. and {Stairs}, I.~H. and {Kramer}, M. and {Burgay}, M. and {D'Amico}, N. and {Freire}, P.~C.~C. and {Joshi}, B.~C. and {Bhat}, N.~D.~R.},
	Doi = {10.1086/426813},
	Eprint = {arXiv:astro-ph/0408297},
	Journal = {\apjl},
	Month = dec,
	Pages = {L131-L134},
	Title = {{The Double Pulsar System J0737-3039: Modulation of A by B at Eclipse}},
	Volume = 616,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426813}}

@article{mclaughlin04b,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613L..57M},
	Author = {{McLaughlin}, M.~A. and {Kramer}, M. and {Lyne}, A.~G. and {Lorimer}, D.~R. and {Stairs}, I.~H. and {Possenti}, A. and {Manchester}, R.~N. and {Freire}, P.~C.~C. and {Joshi}, B.~C. and {Burgay}, M. and {Camilo}, F. and {D'Amico}, N.},
	Doi = {10.1086/424998},
	Eprint = {arXiv:astro-ph/0407265},
	Journal = {\apjl},
	Month = sep,
	Pages = {L57-L60},
	Title = {{The Double Pulsar System J0737-3039: Modulation of the Radio Emission from B by Radiation from A}},
	Volume = 613,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/424998}}

@article{mam06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..166..249M},
	Author = {{McLaughlin}, D.~E. and {Anderson}, J. and {Meylan}, G. and {Gebhardt}, K. and {Pryor}, C. and {Minniti}, D. and {Phinney}, S.},
	Doi = {10.1086/505692},
	Eprint = {astro-ph/0607597},
	Journal = {\apjs},
	Keywords = {Astrometry, Galaxy: Globular Clusters: Individual: NGC Number: NGC 104, Stellar Dynamics},
	Month = sep,
	Pages = {249-297},
	Title = {{Hubble Space Telescope Proper Motions and Stellar Dynamics in the Core of the Globular Cluster 47 Tucanae}},
	Volume = 166,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505692}}

@article{mclaughlin06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006Natur.439..817M},
	Author = {{McLaughlin}, M.~A. and {Lyne}, A.~G. and {Lorimer}, D.~R. and {Kramer}, M. and {Faulkner}, A.~J. and {Manchester}, R.~N. and {Cordes}, J.~M. and {Camilo}, F. and {Possenti}, A. and {Stairs}, I.~H. and {Hobbs}, G. and {D'Amico}, N. and {Burgay}, M. and {O'Brien}, J.~T.},
	Doi = {10.1038/nature04440},
	Eprint = {arXiv:astro-ph/0511587},
	Journal = {\nat},
	Month = feb,
	Pages = {817-820},
	Title = {{Transient radio bursts from rotating neutron stars}},
	Volume = 439,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature04440}}

@article{mclaughlin07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...670.1307M},
	Archiveprefix = {arXiv},
	Author = {{McLaughlin}, M.~A. and {Rea}, N. and {Gaensler}, B.~M. and {Chatterjee}, S. and {Camilo}, F. and {Kramer}, M. and {Lorimer}, D.~R. and {Lyne}, A.~G. and {Israel}, G.~L. and {Possenti}, A.},
	Doi = {10.1086/522335},
	Eprint = {0708.1149},
	Journal = {\apj},
	Keywords = {pulsars: individual (J1819-1458), Radio Continuum: Stars, Stars: Flare, Stars: Neutron, X-Rays: Stars},
	Month = dec,
	Pages = {1307-1313},
	Title = {{Discovery of Pulsations and a Possible Spectral Feature in the X-Ray Emission from Rotating Radio Transient J1819-1458}},
	Volume = 670,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/522335}}

@article{mclaughlin09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400.1431M},
	Archiveprefix = {arXiv},
	Author = {{McLaughlin}, M.~A. and {Lyne}, A.~G. and {Keane}, E.~F. and {Kramer}, M. and {Miller}, J.~J. and {Lorimer}, D.~R. and {Manchester}, R.~N. and {Camilo}, F. and {Stairs}, I.~H.},
	Doi = {10.1111/j.1365-2966.2009.15584.x},
	Eprint = {0908.3813},
	Journal = {\mnras},
	Keywords = {stars: neutron , pulsars: general , Galaxy: stellar content},
	Month = dec,
	Pages = {1431-1438},
	Title = {{Timing observations of rotating radio transients}},
	Volume = 400,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15584.x}}

@ARTICLE{McLeod2014,
       author = {{MacLeod}, Morgan and {Goldstein}, Jacqueline and {Ramirez-Ruiz}, Enrico and {Guillochon}, James and {Samsing}, Johan},
        title = "{Illuminating Massive Black Holes with White Dwarfs: Orbital Dynamics and High-energy Transients from Tidal Interactions}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, galaxies: nuclei, stars: kinematics and dynamics, white dwarfs, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = oct,
       volume = {794},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0004-637X/794/1/9},
archivePrefix = {arXiv},
       eprint = {1405.1426},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...794....9M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{medin08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383..161M},
	Archiveprefix = {arXiv},
	Author = {{Medin}, Z. and {Lai}, D. and {Potekhin}, A.~Y.},
	Doi = {10.1111/j.1365-2966.2007.12518.x},
	Eprint = {0704.1598},
	Journal = {\mnras},
	Keywords = {atomic processes , magnetic fields , stars: atmospheres , stars: neutron},
	Month = jan,
	Pages = {161-172},
	Title = {{Radiative transitions of the helium atom in highly magnetized neutron star atmospheres}},
	Volume = 383,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12518.x}}

@article{melatos95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.275..381M},
	Author = {{Melatos}, A. and {Johnston}, S. and {Melrose}, D.~B.},
	Journal = {\mnras},
	Month = jul,
	Pages = {381-397},
	Title = {{Stellar wind and stellar disc models of dispersion and rotation measure variations in the PSR B1259 - 63/SS2883 binary system}},
	Volume = 275,
	Year = 1995}

@article{melia01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ARA%26A..39..309M},
	Author = {{Melia}, F. and {Falcke}, H.},
	Doi = {10.1146/annurev.astro.39.1.309},
	Eprint = {arXiv:astro-ph/0106162},
	Journal = {\araa},
	Keywords = {ACCRETION, BLACK HOLE PHYSICS, GAS DYNAMICS, JETS, MAGNETOHYDRODYNAMICS, RADIO SYNCHROTRON, RADIO POLARIZATION, STELLAR KINEMATICS},
	Pages = {309-352},
	Title = {{The Supermassive Black Hole at the Galactic Center}},
	Volume = 39,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.39.1.309}}

@article{mendelson89,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989MNRAS.239..733M&db_key=AST},
	Author = {{Mendelson}, H. and {Mazeh}, T.},
	Journal = {\mnras},
	Month = aug,
	Pages = {733-740},
	Title = {{Discovery of a 26.5-day optical periodicity of LSI+61 deg 303}},
	Volume = 239,
	Year = 1989}

@article{mereghetti95,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1995ApJ...442L..17M&db_key=AST},
	Author = {{Mereghetti}, S. and {Stella}, L.},
	Journal = {\apjl},
	Month = mar,
	Pages = {L17-L20},
	Title = {{The very low mass X-ray binary pulsars: A new class of sources?}},
	Volume = 442,
	Year = 1995}

@article{mereghetti00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000A%26A...361..240M&db_key=AST},
	Author = {{Mereghetti}, S. and {Cremonesi}, D. and {Feroci}, M. and {Tavani}, M.},
	Journal = {\aap},
	Month = sep,
	Pages = {240-244},
	Title = {{BeppoSAX observations of SGR 1806-20}},
	Volume = 361,
	Year = 2000}

@article{mereghetti01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...548L.213M},
	Author = {{Mereghetti}, S.},
	Doi = {10.1086/319115},
	Eprint = {arXiv:astro-ph/0011554},
	Journal = {\apjl},
	Keywords = {ISM: Individual: Alphanumeric: G266.2-1.2, Stars: Neutron, ISM: Supernova Remnants, X-Rays: Individual: Alphanumeric: RX J0851.9-4617.4, X-Rays: Individual: Alphanumeric: RX J0852.0-4622},
	Month = feb,
	Pages = {L213-L216},
	Title = {{The X-Ray Sources at the Center of the Supernova Remnant RX J0852.0-4622}},
	Volume = 548,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/319115}}

@inproceedings{mci02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002nsps.conf...29M&db_key=AST},
	Author = {{Mereghetti}, S. and {Chiarlone}, L. and {Israel}, G.~L. and {Stella}, L.},
	Booktitle = {Neutron Stars, Pulsars, and Supernova Remnants},
	Editor = {{Becker}, W. and {Lesch}, H. and {Tr{\"u}mper}, J.},
	Title = {{The Anomalous X-ray Pulsars}},
  Publisher={MPE Report 278},
	Pages = {29-43},
	Year = 2002}

@article{mereghetti02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...574..873M&db_key=AST},
	Author = {{Mereghetti}, S. and {Bandiera}, R. and {Bocchino}, F. and {Israel}, G.~L.},
	Doi = {10.1086/340976},
	Eprint = {astro-ph/0204050},
	Journal = {\apj},
	Month = aug,
	Pages = {873-878},
	Title = {{BeppoSAX Observations of the Young Pulsar in the Kes 75 Supernova Remnant}},
	Volume = 574,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340976}}

@article{mereghetti02_sait,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002MmSAI..73..572M&db_key=AST},
	Author = {{Mereghetti}, S. and {Feroci}, M. and {Tavani}, M. and {Woods}, P.},
	Journal = {Memorie della Societa Astronomica Italiana},
	Pages = {572-577},
	Title = {{Beppo-SAX observations of SGR 1806-20}},
	Volume = 73,
	Year = 2002}

@article{mereghetti03_gcn,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003GCN..2415....1M&db_key=AST},
	Author = {{Mereghetti}, S. and {G\"otz}, D. and {Beck}, M. and {Mirabel}, F.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR 1806-20 bursts with INTEGRAL and IBAS announcement on soft.}},
	Volume = 2415,
	Year = 2003}

@article{mereghetti03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003A%26A...411L.291M&db_key=AST},
	Author = {{Mereghetti}, S. and {G{\"o}tz}, D. and {Borkowski}, J. and {Walter}, R. and {Pedersen}, H.},
	Journal = {\aap},
	Month = nov,
	Pages = {L291-L297},
	Title = {{The INTEGRAL Burst Alert System}},
	Volume = 411,
	Year = 2003}

@article{mereghetti04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...608..427M&db_key=AST},
	Author = {{Mereghetti}, S. and {Tiengo}, A. and {Stella}, L. and {Israel}, G.~L. and {Rea}, N. and {Zane}, S. and {Oosterbroek}, T.},
	Journal = {\apj},
	Month = jun,
	Pages = {427-431},
	Title = {{Pronounced Long-Term Flux Variability of the Anomalous X-Ray Pulsar 1E 1048.1-5937}},
	Volume = 608,
	Year = 2004}

@article{mgm04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004astro.ph.11695M&db_key=PRE},
	Author = {{Mereghetti}, S. and {G{\"o}tz}, D. and {Mirabel}, I.~F. and {Hurley}, K.},
	Eprint = {astro-ph/0411695},
	Journal = {ArXiv Astrophysics e-prints (astro-ph/0411695)},
	Month = nov,
	Title = {{INTEGRAL discovery of persistent hard X-ray emission from the Soft Gamma Ray Repeater SGR 1806-20}},
	Year = 2004}

@article{mereghetti04_gcn,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004GCN..2763....1M&db_key=AST},
	Author = {{Mereghetti}, S. and {G\"otz}, D. and {Borkowski}, J. and {Beck}, M. and {Mirabel}, F.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{Very strong outburst from Sgr 1806-20 detected with INTEGRAL.}},
	Volume = 2763,
	Year = 2004}

@article{mereghetti05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005ApJ...624L.105M&db_key=AST},
	Author = {{Mereghetti}, S. and {G{\"o}tz}, D. and {von Kienlin}, A. and {Rau}, A. and {Lichti}, G. and {Weidenspointner}, G. and {Jean}, P.},
	Doi = {10.1086/430669},
	Journal = {\apjl},
	Month = may,
	Pages = {L105-L108},
	Title = {{The First Giant Flare from SGR 1806-20: Observations Using the Anticoincidence Shield of the Spectrometer on INTEGRAL}},
	Volume = 624,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430669}}

@article{mgm05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005A%26A...433L...9M&db_key=AST},
	Author = {{Mereghetti}, S. and {G{\"o}tz}, D. and {Mirabel}, I.~F. and {Hurley}, K.},
	Doi = {10.1051/0004-6361:200500088},
	Journal = {\aap},
	Month = apr,
	Pages = {L9-L12},
	Title = {{INTEGRAL discovery of persistent hard X-ray emission from the Soft Gamma-ray Repeater SGR 1806-20}},
	Volume = 433,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500088}}

@article{mte05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...628..938M&db_key=AST},
	Author = {{Mereghetti}, S. and {Tiengo}, A. and {Esposito}, P. and {G{\"o}tz}, D. and {Stella}, L. and {Israel}, G.~L. and {Rea}, N. and {Feroci}, M. and {Turolla}, R. and {Zane}, S.},
	Doi = {10.1086/430943},
	Journal = {\apj},
	Month = aug,
	Pages = {938-945},
	Title = {{An XMM-Newton View of the Soft Gamma Repeater SGR 1806-20: Long-Term Variability in the Pre-Giant Flare Epoch}},
	Volume = 628,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430943}}

@article{mereghetti06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006A%26A...450..759M&db_key=AST},
	Author = {{Mereghetti}, S. and {Esposito}, P. and {Tiengo}, A. and {Turolla}, R. and {Zane}, S. and {Stella}, L. and {Israel}, G.~L. and {Feroci}, M. and {Treves}, A.},
	Doi = {10.1051/0004-6361:20054210},
	Journal = {\aap},
	Month = may,
	Pages = {759-762},
	Title = {{XMM-Newton observations of the Soft Gamma Ray Repeater SGR 1627-41 in a low luminosity state}},
	Volume = 450,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054210}}

@article{met06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006ApJ...653.1423M&db_key=AST},
	Author = {{Mereghetti}, S. and {Esposito}, P. and {Tiengo}, A. and {Zane}, S. and {Turolla}, R. and {Stella}, L. and {Israel}, G.~L. and {G{\"o}tz}, D. and {Feroci}, M.},
	Doi = {10.1086/508682},
	Eprint = {astro-ph/0608588},
	Journal = {\apj},
	Month = dec,
	Pages = {1423-1428},
	Title = {{The First XMM-Newton Observations of the Soft Gamma-Ray Repeater SGR 1900+14}},
	Volume = 653,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/508682}}

@article{met07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007Ap%26SS.308...13M},
	Author = {{Mereghetti}, S. and {Esposito}, P. and {Tiengo}, A.},
	Doi = {10.1007/s10509-007-9384-0},
	Eprint = {arXiv:astro-ph/0608364},
	Journal = {\apss},
	Month = apr,
	Pages = {13-23},
	Title = {{XMM Newton observations of soft gamma-ray repeaters}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9384-0}}

@article{mereghetti08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26ARv..15..225M},
	Archiveprefix = {arXiv},
	Author = {{Mereghetti}, S.},
	Doi = {10.1007/s00159-008-0011-z},
	Eprint = {0804.0250},
	Journal = {\aapr},
	Keywords = {Stars: neutron, Magnetic fields, X-rays: stars, Gamma rays: bursts, Pulsars: general},
	Month = jul,
	Pages = {225-287},
	Title = {{The strongest cosmic magnets: soft gamma-ray repeaters and anomalous X-ray pulsars}},
	Volume = 15,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s00159-008-0011-z}}

@article{mereghetti09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696L..74M},
	Archiveprefix = {arXiv},
	Author = {{Mereghetti}, S. and {G{\"o}tz}, D. and {Weidenspointner}, G. and {von Kienlin}, A. and {Esposito}, P. and {Tiengo}, A. and {Vianello}, G. and {Israel}, G.~L. and {Stella}, L. and {Turolla}, R. and {Rea}, N. and {Zane}, S.},
	Doi = {10.1088/0004-637X/696/1/L74},
	Eprint = {0903.1974},
	Journal = {\apjl},
	Keywords = {gamma rays: bursts, gamma rays: observations, pulsars: individual: 1E 1547.0-5408, stars: neutron},
	Month = may,
	Pages = {L74-L78},
	Title = {{Strong Bursts from the Anomalous X-Ray Pulsar 1E{\nbsp}1547.0{\ndash}5408 Observed with the INTEGRAL/SPI Anti-Coincidence Shield}},
	Volume = 696,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/696/1/L74}}

@article{mte09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009Sci...325.1222M},
	Archiveprefix = {arXiv},
	Author = {{Mereghetti}, S. and {Tiengo}, A. and {Esposito}, P. and {La Palombara}, N. and {Israel}, G.~L. and {Stella}, L.},
	Doi = {10.1126/science.1176252},
	Eprint = {1003.0997},
	Journal = {Science},
	Month = sep,
	Pages = {1222-},
	Primaryclass = {astro-ph.HE},
	Title = {{An Ultramassive, Fast-Spinning White Dwarf in a Peculiar Binary System}},
	Volume = 325,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1176252}}

@ARTICLE{mereghetti15,
   author = {{Mereghetti}, S. and {Pons}, J.~A. and {Melatos}, A.},
    title = "{Magnetars: Properties, Origin and Evolution}",
  journal = {\ssr},
archivePrefix = "arXiv",
   eprint = {1503.06313},
 primaryClass = "astro-ph.HE",
 keywords = {Neutron star, Magnetic field, Magnetar},
     year = 2015,
    month = oct,
   volume = 191,
    pages = {315-338},
      doi = {10.1007/s11214-015-0146-y},
   adsurl = {http://adsabs.harvard.edu/abs/2015SSRv..191..315M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mereghetti16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.tmp..325M},
	Archiveprefix = {arXiv},
	Author = {{Mereghetti}, S. and {Pintore}, F. and {Esposito}, P. and {Palombara}, N.~L. and {Tiengo}, A. and {Israel}, G.~L. and {Stella}, L.},
	Doi = {10.1093/mnras/stw536},
	Eprint = {1603.01505},
	Journal = {\mnras, in press (preprint: astro-ph/1603.01505)},
	Keywords = {X-rays: binaries.~Stars: neutron, white dwarfs, subdwarfs, individual: HD 49798},
	Month = mar,
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of spin-up in the X-ray pulsar companion of the hot subdwarf HD 49798}},
	Year = 2016,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stw536}}

@ARTICLE{mkt16,
   author = {{Mereghetti}, S. and {Kuiper}, L. and {Tiengo}, A. and {Hessels}, J. and 
	{Hermsen}, W. and {Stovall}, K. and {Possenti}, A. and {Rankin}, J. and 
	{Esposito}, P. and {Turolla}, R. and {Mitra}, D. and {Wright}, G. and 
	{Stappers}, B. and {Horneffer}, A. and {Oslowski}, S. and {Serylak}, M. and 
	{Grie{\ss}meier}, J.-M.},
    title = "{A Deep Campaign to Characterize the Synchronous Radio/X-Ray Mode Switching of PSR B0943+10}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1607.07735},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, stars: neutron, X-rays: individual: PSR B0943+10},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {21},
    pages = {21},
      doi = {10.3847/0004-637X/831/1/21},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...831...21M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{metzger08,
   author = {{Metzger}, B.~D. and {Quataert}, E. and {Thompson}, T.~A.},
    title = "{Short-duration gamma-ray bursts with extended emission from protomagnetar spin-down}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0712.1233},
 keywords = {MHD , stars: neutron , stars: winds, outflows , gamma-rays: bursts},
     year = 2008,
    month = apr,
   volume = 385,
    pages = {1455-1460},
      doi = {10.1111/j.1365-2966.2008.12923.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.1455M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{metzger11,
   author = {{Metzger}, B.~D. and {Giannios}, D. and {Thompson}, T.~A. and 
	{Bucciantini}, N. and {Quataert}, E.},
    title = "{The protomagnetar model for gamma-ray bursts}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.0001},
 primaryClass = "astro-ph.HE",
 keywords = {MHD, gamma-ray burst: general, stars: neutron, stars: winds, outflows},
     year = 2011,
    month = may,
   volume = 413,
    pages = {2031-2056},
      doi = {10.1111/j.1365-2966.2011.18280.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.2031M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{metzger21,
       author = {{Metzger}, Brian D. and {Stone}, Nicholas C. and {Gilbaum}, Shmuel},
        title = "{Interacting Stellar EMRIs as Sources of Quasi-Periodic Eruptions in Galactic Nuclei}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jul,
          eid = {arXiv:2107.13015},
        pages = {arXiv:2107.13015},
archivePrefix = {arXiv},
       eprint = {2107.13015},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210713015M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mewe85,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1985A%26AS...62..197M},
	Author = {{Mewe}, R. and {Gronenschild}, E.~H.~B.~M. and {van den Oord}, G.~H.~J.},
	Journal = {\aaps},
	Month = nov,
	Pages = {197-254},
	Title = {{Calculated X-radiation from optically thin plasmas. V}},
	Volume = 62,
	Year = 1985}

@article{mewe86,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986A%26AS...65..511M},
	Author = {{Mewe}, R. and {Lemen}, J.~R. and {van den Oord}, G.~H.~J.},
	Journal = {\aaps},
	Month = sep,
	Pages = {511-536},
	Title = {{Calculated X-radiation from optically thin plasmas. VI - Improved calculations for continuum emission and approximation formulae for nonrelativistic average Gaunt factors}},
	Volume = 65,
	Year = 1986}

@article{mezcua13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.3128M},
	Archiveprefix = {arXiv},
	Author = {{Mezcua}, M. and {Roberts}, T.~P. and {Sutton}, A.~D. and {Lobanov}, A.~P.},
	Doi = {10.1093/mnras/stt1794},
	Eprint = {1309.5721},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, ISM: jets and outflows, radio continuum: general, X-rays: binaries},
	Month = dec,
	Pages = {3128-3134},
	Primaryclass = {astro-ph.HE},
	Title = {{Radio observations of extreme ULXs: revealing the most powerful ULX radio nebula ever or the jet of an intermediate-mass black hole?}},
	Volume = 436,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt1794}}

@article{mezger89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...209..337M},
	Author = {{Mezger}, P.~G. and {Zylka}, R. and {Salter}, C.~J. and {Wink}, J.~E. and {Chini}, R. and {Kreysa}, E. and {Tuffs}, R.},
	Journal = {\aap},
	Keywords = {ASTRONOMICAL SPECTROSCOPY, INFRARED ASTRONOMY, MILLIMETER WAVES, MOLECULAR CLOUDS, RADIO SOURCES (ASTRONOMY), SUBMILLIMETER WAVES, COSMIC DUST, EMISSION SPECTRA, OPTICAL THICKNESS, STELLAR MASS, STELLAR WINDS, SUPERNOVA REMNANTS},
	Month = jan,
	Pages = {337-348},
	Title = {{Continuum observations of SGR A at mm/submm wavelengths}},
	Volume = 209,
	Year = 1989}

@article{meynet05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...429..581M},
	Author = {{Meynet}, G. and {Maeder}, A.},
	Doi = {10.1051/0004-6361:20047106},
	Eprint = {astro-ph/0408319},
	Journal = {\aap},
	Keywords = {stars: evolution, stars: rotation, stars: Wolf-Rayet},
	Month = jan,
	Pages = {581-598},
	Title = {{Stellar evolution with rotation. XI. Wolf-Rayet star populations at different metallicities}},
	Volume = 429,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20047106}}

@article{mhlahlo07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.378..211M},
	Archiveprefix = {arXiv},
	Author = {{Mhlahlo}, N. and {Buckley}, D.~A.~H. and {Dhillon}, V.~S. and {Potter}, S.~B. and {Warner}, B. and {Woudt}, P.~A.},
	Doi = {10.1111/j.1365-2966.2007.11762.x},
	Eprint = {0704.0017},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, novae, cataclysmic variables},
	Month = jun,
	Pages = {211-220},
	Title = {{Spectroscopic observations of the intermediate polar EX Hydrae in quiescence}},
	Volume = 378,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11762.x}}

@ARTICLE{michael02,
   author = {{Michael}, E. and {Zhekov}, S. and {McCray}, R. and {Hwang}, U. and 
	{Burrows}, D.~N. and {Park}, S. and {Garmire}, G.~P. and {Holt}, S.~S. and 
	{Hasinger}, G.},
    title = "{The X-Ray Spectrum of Supernova Remnant 1987A}",
  journal = {\apj},
   eprint = {astro-ph/0112261},
 keywords = {Shock Waves, ISM: Supernova Remnants, Stars: Supernovae: Individual: Alphanumeric: SN 1987A, X-Rays: ISM},
     year = 2002,
    month = jul,
   volume = 574,
    pages = {166-178},
      doi = {10.1086/340591},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...574..166M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{middleton11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417..464M},
	Archiveprefix = {arXiv},
	Author = {{Middleton}, M.~J. and {Sutton}, A.~D. and {Roberts}, T.~P.},
	Doi = {10.1111/j.1365-2966.2011.19285.x},
	Eprint = {1106.3900},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, X-rays: binaries, X-rays: individual: M33 X-8},
	Month = oct,
	Pages = {464-471},
	Primaryclass = {astro-ph.CO},
	Title = {{X-ray spectral evolution in the ultraluminous X-ray source M33 X-8}},
	Volume = 417,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19285.x}}

@article{middleton12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.2969M},
	Archiveprefix = {arXiv},
	Author = {{Middleton}, M.~J. and {Sutton}, A.~D. and {Roberts}, T.~P. and {Jackson}, F.~E. and {Done}, C.},
	Doi = {10.1111/j.1365-2966.2011.20145.x},
	Eprint = {1111.1188},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, X-rays: binaries},
	Month = mar,
	Pages = {2969-2977},
	Primaryclass = {astro-ph.HE},
	Title = {{The missing link: a low-mass X-ray binary in M31 seen as an ultraluminous X-ray source}},
	Volume = 420,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.20145.x}}

@article{middleton13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013Natur.493..187M},
	Archiveprefix = {arXiv},
	Author = {{Middleton}, M.~J. and {Miller-Jones}, J.~C.~A. and {Markoff}, S. and {Fender}, R. and {Henze}, M. and {Hurley-Walker}, N. and {Scaife}, A.~M.~M. and {Roberts}, T.~P. and {Walton}, D. and {Carpenter}, J. and {Macquart}, J.-P. and {Bower}, G.~C. and {Gurwell}, M. and {Pietsch}, W. and {Haberl}, F. and {Harris}, J. and {Daniel}, M. and {Miah}, J. and {Done}, C. and {Morgan}, J.~S. and {Dickinson}, H. and {Charles}, P. and {Burwitz}, V. and {Della Valle}, M. and {Freyberg}, M. and {Greiner}, J. and {Hernanz}, M. and {Hartmann}, D.~H. and {Hatzidimitriou}, D. and {Riffeser}, A. and {Sala}, G. and {Seitz}, S. and {Reig}, P. and {Rau}, A. and {Orio}, M. and {Titterington}, D. and {Grainge}, K.},
	Doi = {10.1038/nature11697},
	Eprint = {1212.4698},
	Journal = {\nat},
	Month = jan,
	Pages = {187-190},
	Primaryclass = {astro-ph.HE},
	Title = {{Bright radio emission from an ultraluminous stellar-mass microquasar in M 31}},
	Volume = 493,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature11697}}

@article{mignani07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...473..883M},
	Author = {{Mignani}, R.~P. and {De Luca}, A. and {Zaggia}, S. and {Sester}, D. and {Pellizzoni}, A. and {Mereghetti}, S. and {Caraveo}, P.~A.},
	Doi = {10.1051/0004-6361:20077768},
	Eprint = {arXiv:0707.0937},
	Journal = {\aap},
	Keywords = {stars: neutron, X-rays: individuals: CXO J085201.4-461753, ISM: supernova remnants},
	Month = oct,
	Pages = {883-889},
	Title = {{VLT observations of the central compact object in the Vela Jr. supernova remnant}},
	Volume = 473,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077768}}

@article{mignani08,
   author = {{Mignani}, R.~P. and {Zaggia}, S. and {de Luca}, A. and {Perna}, R. and 
	{Bassan}, N. and {Caraveo}, P.~A.},
    title = "{Optical and infrared observations of the X-ray source 1WGA J1713.4-3949 in the G347.3-0.5 SNR}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0803.3722},
 keywords = {stars: neutron, stars: individual: 1WGA J1713.4-3949},
     year = 2008,
    month = jun,
   volume = 484,
    pages = {457-461},
      doi = {10.1051/0004-6361:20079076},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...484..457M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mignani08_atel,
	Author = {{Mignani}, R.~P. and {Rea}, N. and {Israel}, G.~L. and {Testa}, V. and {Esposito}, P.},
	Journal = {Astron. Tel.},
	Keywords = {Infra-Red, Request for Observations, Pulsars, Transients},
	Month = oct,
	Title = {{Possible NIR counterpart to the AXP 1E 1547.0-5408}},
	Volume = 1758,
	Year = 2008}

@article{mrt09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2244....1M},
	Author = {{Mignani}, R.~P. and {Rea}, N. and {Testa}, V. and {Israel}, G.~L. and {Covino}, S. and {Stella}, L. and {Mereghetti}, S. and {Burgay}, M. and {Possenti}, A. and {Chaty}, S. and {Jonker}, P. and {Lo Curto}, G. and {Perna}, R. and {Turolla}, R. and {Zane}, S.},
	Journal = {Astron. Tel.},
	Keywords = {Optical, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters},
	Month = oct,
	Title = {{GTC optical observations of SGR 0418+5729}},
	Volume = 2244,
	Year = 2009}

@article{mignani11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AdSpR..47.1281M},
	Archiveprefix = {arXiv},
	Author = {{Mignani}, R.~P.},
	Doi = {10.1016/j.asr.2009.12.011},
	Eprint = {0912.2931},
	Journal = {Advances in Space Research},
	Month = apr,
	Pages = {1281-1293},
	Primaryclass = {astro-ph.HE},
	Title = {{Optical, ultraviolet, and infrared observations of isolated neutron stars}},
	Volume = 47,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.asr.2009.12.011}}

@article{miller03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...583L..99M},
	Author = {{Miller}, J.~M. and {Wijnands}, R. and {M{\'e}ndez}, M. and {Kendziorra}, E. and {Tiengo}, A. and {van der Klis}, M. and {Chakrabarty}, D. and {Gaensler}, B.~M. and {Lewin}, W.~H.~G.},
	Doi = {10.1086/368105},
	Eprint = {arXiv:astro-ph/0208166},
	Journal = {\apjl},
	Month = feb,
	Pages = {L99-L102},
	Title = {{XMM-Newton Spectroscopy of the Accretion-driven Millisecond X-Ray Pulsar XTE J1751-305 in Outburst}},
	Volume = 583,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/368105}}

@article{miller04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004IJMPD..13....1M},
	Author = {{Miller}, M.~C. and {Colbert}, E.~J.~M.},
	Doi = {10.1142/S0218271804004426},
	Journal = {International Journal of Modern Physics D},
	Keywords = {Black hole physics, (galaxy) globular clusters: general, gravitational waves, stellar dynamics, X-rays: binaries},
	Month = jan,
	Pages = {1-64},
	Title = {{Intermediate-Mass Black Holes}},
	Volume = 13,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1142/S0218271804004426}}

@ARTICLE{mj15,
       author = {{Miller-Jones}, J.~C.~A. and {Strader}, J. and {Heinke}, C.~O. and
         {Maccarone}, T.~J. and {van den Berg}, M. and {Knigge}, C. and
         {Chomiuk}, L. and {Noyola}, E. and {Russell}, T.~D. and {Seth}, A.~C. and
         {Sivakoff}, G.~R.},
        title = "{Deep radio imaging of 47 Tuc identifies the peculiar X-ray source X9 as a new black hole candidate}",
      journal = {\mnras},
     keywords = {stars: black holes, globular clusters: individual: 47 Tuc, radio continuum: general, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = nov,
       volume = {453},
       number = {4},
        pages = {3918-3931},
          doi = {10.1093/mnras/stv1869},
archivePrefix = {arXiv},
       eprint = {1509.02579},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.453.3918M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mineo12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.2095M},
	Archiveprefix = {arXiv},
	Author = {{Mineo}, S. and {Gilfanov}, M. and {Sunyaev}, R.},
	Doi = {10.1111/j.1365-2966.2011.19862.x},
	Eprint = {1105.4610},
	Journal = {\mnras},
	Keywords = {stars: formation, galaxies: irregular, galaxies: spiral, galaxies: starburst, X-rays: binaries, X-rays: galaxies},
	Month = jan,
	Pages = {2095-2115},
	Primaryclass = {astro-ph.HE},
	Title = {{X-ray emission from star-forming galaxies - I. High-mass X-ray binaries}},
	Volume = 419,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19862.x}}

@article{mingo12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...758...95M},
	Archiveprefix = {arXiv},
	Author = {{Mingo}, B. and {Hardcastle}, M.~J. and {Croston}, J.~H. and {Evans}, D.~A. and {Kharb}, P. and {Kraft}, R.~P. and {Lenc}, E.},
	Doi = {10.1088/0004-637X/758/2/95},
	Eid = {95},
	Eprint = {1209.0348},
	Journal = {\apj},
	Keywords = {galaxies: individual: Circinus, galaxies: jets, galaxies: Seyfert, shock waves, X-rays: galaxies},
	Month = oct,
	Pages = {95},
	Primaryclass = {astro-ph.CO},
	Title = {{Shocks, Seyferts, and the Supernova Remnant Connection: A Chandra Observation of the Circinus Galaxy}},
	Volume = 758,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/758/2/95}}

@ARTICLE{miniutti19,
       author = {{Miniutti}, G. and {Saxton}, R.~D. and {Giustini}, M. and {Alexand
        er}, K.~D. and {Fender}, R.~P. and {Heywood}, I. and {Monageng}, I. and
         {Coriat}, M. and {Tzioumis}, A.~K. and {Read}, A.~M. and {Knigge}, C. and
         {Gandhi}, P. and {Pretorius}, M.~L. and {Ag{\'\i}s-Gonz{\'a}lez}, B.},
        title = "{Nine-hour X-ray quasi-periodic eruptions from a low-mass black hole galactic nucleus}",
      journal = {\nat},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = sep,
       volume = {573},
       number = {7774},
        pages = {381-384},
          doi = {10.1038/s41586-019-1556-x},
archivePrefix = {arXiv},
       eprint = {1909.04693},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Natur.573..381M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mirabel98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998Natur.392..673M&db_key=AST},
	Author = {{Mirabel}, I.~F. and {Rodr{\'{\i}}guez}, L.~F.},
	Doi = {10.1038/33603},
	Journal = {\nat},
	Month = apr,
	Pages = {673-676},
	Title = {{Microquasars in our Galaxy}},
	Volume = 392,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/33603}}

@article{mirabel99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999ARA%26A..37..409M},
	Author = {{Mirabel}, I.~F. and {Rodr{\'{\i}}guez}, L.~F.},
	Doi = {10.1146/annurev.astro.37.1.409},
	Eprint = {arXiv:astro-ph/9902062},
	Journal = {\araa},
	Pages = {409-443},
	Title = {{Sources of Relativistic Jets in the Galaxy}},
	Volume = 37,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.37.1.409}}

@inproceedings{mirabel00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000AIPC..526..814M&db_key=AST},
	Author = {{Mirabel}, I.~F. and {Fuchs}, Y. and {Chaty}, S.},
	Booktitle = {AIP Conference Proceedings 526: Gamma-ray Bursts, 5th Huntsville Symposium},
	Pages = {814},
	Title = {{Soft Gamma-Ray Repeaters in Clusters of Massive Stars}},
	Year = 2000}

@article{mirabel06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006Sci...312.1759M},
	Author = {{Mirabel}, I.~F.},
	Eprint = {arXiv:astro-ph/0606393},
	Journal = {Science},
	Month = jun,
	Pages = {1759},
	Title = {{Very energetic gamma-rays from microquasars and binary pulsars}},
	Volume = 312,
	Year = 2006}

@article{misanovic11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...735...33M},
	Archiveprefix = {arXiv},
	Author = {{Misanovic}, Z. and {Kargaltsev}, O. and {Pavlov}, G.~G.},
	Doi = {10.1088/0004-637X/735/1/33},
	Eprint = {1101.1342},
	Journal = {\apj},
	Keywords = {stars: neutron, X-rays: individual: CXOU J183434.9{\ndash}084443 XMMU J183435.3{\ndash}084443 HESS J1834{\ndash}087 1FGL J1834.3{\ndash}0842c SNR W41=G23.3{\ndash}0.3},
	Month = jul,
	Pages = {33},
	Primaryclass = {astro-ph.HE},
	Title = {{Chandra Observation of the TeV Source HESS J1834-087}},
	Volume = 735,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/735/1/33}}

@article{mitsuda84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984PASJ...36..741M},
	Author = {{Mitsuda}, K. and {Inoue}, H. and {Koyama}, K. and {Makishima}, K. and {Matsuoka}, M. and {Ogawara}, Y. and {Suzuki}, K. and {Tanaka}, Y. and {Shibazaki}, N. and {Hirano}, T.},
	Journal = {\pasj},
	Keywords = {ACCRETION DISKS, ENERGY SPECTRA, NEUTRON STARS, X RAY BINARIES, X RAY SPECTRA, ASTRONOMICAL SATELLITES, BLACK BODY RADIATION, PERIODIC VARIATIONS, PULSE AMPLITUDE, RADIANT FLUX DENSITY, SPECTRUM ANALYSIS},
	Pages = {741-759},
	Title = {{Energy spectra of low-mass binary X-ray sources observed from TENMA}},
	Volume = 36,
	Year = 1984}

@article{mitsuda07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007PASJ...59S...1M},
	Author = {{Mitsuda}, K. and {Bautz}, M. and {Inoue}, H. and {Kelley}, R.~L. and {Koyama}, K. and {Kunieda}, H. and {Makishima}, K. and {Ogawara}, Y. and {Petre}, R. and {Takahashi}, T. and {Tsunemi}, H. and {White}, N.~E. and {Anabuki}, N. and {Angelini}, L. and {Arnaud}, K. and {Awaki}, H. and {Bamba}, A. and {Boyce}, K. and {Brown}, G.~V. and {Chan}, K.-W. and {Cottam}, J. and {Dotani}, T. and {Doty}, J. and {Ebisawa}, K. and {Ezoe}, Y. and {Fabian}, A.~C. and {Figueroa}, E. and {Fujimoto}, R. and {Fukazawa}, Y. and {Furusho}, T. and {Furuzawa}, A. and {Gendreau}, K. and {Griffiths}, R.~E. and {Haba}, Y. and {Hamaguchi}, K. and {Harrus}, I. and {Hasinger}, G. and {Hatsukade}, I. and {Hayashida}, K. and {Henry}, P.~J. and {Hiraga}, J.~S. and {Holt}, S.~S. and {Hornschemeier}, A. and {Hughes}, J.~P. and {Hwang}, U. and {Ishida}, M. and {Ishisaki}, Y. and {Isobe}, N. and {Itoh}, M. and {Iyomoto}, N. and {Kahn}, S.~M. and {Kamae}, T. and {Katagiri}, H. and {Kataoka}, J. and {Katayama}, H. and {Kawai}, N. and {Kilbourne}, C. and {Kinugasa}, K. and {Kissel}, S. and {Kitamoto}, S. and {Kohama}, M. and {Kohmura}, T. and {Kokubun}, M. and {Kotani}, T. and {Kotoku}, J. and {Kubota}, A. and {Madejski}, G.~M. and {Maeda}, Y. and {Makino}, F. and {Markowitz}, A. and {Matsumoto}, C. and {Matsumoto}, H. and {Matsuoka}, M. and {Matsushita}, K. and {McCammon}, D. and {Mihara}, T. and {Misaki}, K. and {Miyata}, E. and {Mizuno}, T. and {Mori}, K. and {Mori}, H. and {Morii}, M. and {Moseley}, H. and {Mukai}, K. and {Murakami}, H. and {Murakami}, T. and {Mushotzky}, R. and {Nagase}, F. and {Namiki}, M. and {Negoro}, H. and {Nakazawa}, K. and {Nousek}, J.~A. and {Okajima}, T. and {Ogasaka}, Y. and {Ohashi}, T. and {Oshima}, T. and {Ota}, N. and {Ozaki}, M. and {Ozawa}, H. and {Parmar}, A.~N. and {Pence}, W.~D. and {Porter}, F.~S. and {Reeves}, J.~N. and {Ricker}, G.~R. and {Sakurai}, I. and {Sanders}, W.~T. and {Senda}, A. and {Serlemitsos}, P. and {Shibata}, R. and {Soong}, Y. and {Smith}, R. and {Suzuki}, M. and {Szymkowiak}, A.~E. and {Takahashi}, H. and {Tamagawa}, T. and {Tamura}, K. and {Tamura}, T. and {Tanaka}, Y. and {Tashiro}, M. and {Tawara}, Y. and {Terada}, Y. and {Terashima}, Y. and {Tomida}, H. and {Torii}, K. and {Tsuboi}, Y. and {Tsujimoto}, M. and {Tsuru}, T.~G. and {Turner}, M.~J.~L.~. and {Ueda}, Y. and {Ueno}, S. and {Ueno}, M. and {Uno}, S. and {Urata}, Y. and {Watanabe}, S. and {Yamamoto}, N. and {Yamaoka}, K. and {Yamasaki}, N.~Y. and {Yamashita}, K. and {Yamauchi}, M. and {Yamauchi}, S. and {Yaqoob}, T. and {Yonetoku}, D. and {Yoshida}, A.},
	Journal = {\pasj},
	Month = jan,
	Pages = {1-7},
	Title = {{The X-Ray Observatory Suzaku}},
	Volume = 59,
	Year = 2007}

@article{molendi03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003MNRAS.343L...1M},
	Author = {{Molendi}, S. and {Bianchi}, S. and {Matt}, G.},
	Doi = {10.1046/j.1365-8711.2003.06783.x},
	Eprint = {astro-ph/0305217},
	Journal = {\mnras},
	Keywords = {galaxies: active, galaxies: individual: Circinus galaxy, X-rays: galaxies},
	Month = jul,
	Pages = {L1-L4},
	Title = {{Iron and nickel line properties in the X-ray-reflecting region of the Circinus galaxy}},
	Volume = 343,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06783.x}}

@ARTICLE{molendi09,
       author = {{Molendi}, S. and {Gastaldello}, F.},
        title = "{Non-thermal emission in the core of Perseus: results from a long XMM-Newton observation}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, galaxies: clusters: individual: Perseus, X-rays: galaxies: clusters, Astrophysics},
         year = 2009,
        month = Jan,
       volume = {493},
        pages = {13-21},
          doi = {10.1051/0004-6361:200810138},
archivePrefix = {arXiv},
       eprint = {0807.2653},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2009A&A...493...13M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{molkov04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004AstL...30..534M&db_key=AST},
	Author = {{Molkov}, S.~V. and {Cherepashchuk}, A.~M. and {Lutovinov}, A.~A. and {Revnivtsev}, M.~G. and {Postnov}, K.~A. and {Sunyaev}, R.~A.},
	Journal = {Astron.~Lett.},
	Month = aug,
	Pages = {534-539},
	Title = {{A Hard X-ray Survey of the Sagittarius Arm Tangent with the IBIS Telescope of the INTEGRAL Observatory: A Catalog of Sources}},
	Volume = 30,
	Year = 2004}

@article{molkov05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005A%26A...433L..13M&db_key=AST},
	Author = {{Molkov}, S. and {Hurley}, K. and {Sunyaev}, R. and {Shtykovsky}, P. and {Revnivtsev}, M. and {Kouveliotou}, C.},
	Doi = {10.1051/0004-6361:200500087},
	Journal = {\aap},
	Month = apr,
	Pages = {L13-L16},
	Title = {{The broad-band spectrum of the persistent emission from SGR 1806-20}},
	Volume = 433,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500087}}

@article{monet03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125..984M},
	Author = {{Monet}, D.~G. and {Levine}, S.~E. and {Canzian}, B. and {Ables}, H.~D. and {Bird}, A.~R. and {Dahn}, C.~C. and {Guetter}, H.~H. and {Harris}, H.~C. and {Henden}, A.~A. and {Leggett}, S.~K. and {Levison}, H.~F. and {Luginbuhl}, C.~B. and {Martini}, J. and {Monet}, A.~K.~B. and {Munn}, J.~A. and {Pier}, J.~R. and {Rhodes}, A.~R. and {Riepe}, B. and {Sell}, S. and {Stone}, R.~C. and {Vrba}, F.~J. and {Walker}, R.~L. and {Westerhout}, G. and {Brucato}, R.~J. and {Reid}, I.~N. and {Schoening}, W. and {Hartley}, M. and {Read}, M.~A. and {Tritton}, S.~B.},
	Doi = {10.1086/345888},
	Eprint = {arXiv:astro-ph/0210694},
	Journal = {\aj},
	Month = feb,
	Pages = {984-993},
	Title = {{The USNO-B Catalog}},
	Volume = 125,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345888}}

@inproceedings{moretti05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005SPIE.5898..348M},
	Author = {{Moretti}, A. and {Campana}, S. and {Mineo}, T. and {Romano}, P. and {Abbey}, A.~F. and {Angelini}, L. and {Beardmore}, A. and {Burkert}, W. and {Burrows}, D.~N. and {Capalbi}, M. and {Chincarini}, G. and {Citterio}, O. and {Cusumano}, G. and {Freyberg}, M.~J. and {Giommi}, P. and {Goad}, M.~R. and {Godet}, O. and {Hartner}, G.~D. and {Hill}, J.~E. and {Kennea}, J. and {La Parola}, V. and {Mangano}, V. and {Morris}, D. and {Nousek}, J.~A. and {Osborne}, J. and {Page}, K. and {Pagani}, C. and {Perri}, M. and {Tagliaferri}, G. and {Tamburelli}, F. and {Wells}, A.},
	Booktitle = {{UV, X-Ray, and Gamma-Ray Space Instrumentation for Astronomy XIV}},
	Doi = {10.1117/12.617164},
	Editor = {{Siegmund}, O.~H.~W.},
	Month = jan,
	Pages = {348-356},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{In-flight calibration of the Swift XRT Point Spread Function}},
	Volume = 5898,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.617164}}

@INPROCEEDINGS{mori01,
   author = {{Mori}, K. and {Tsunemi}, H. and {Miyata}, E. and {Baluta}, C.~J. and 
	{Burrows}, D.~N. and {Garmire}, G.~P. and {Chartas}, G.},
    title = "{Improvement of the Chandra ACIS Spatial Resolution by Selecting the Split Pixel Events}",
booktitle = {New Century of X-ray Astronomy},
     year = 2001,
	Publisher = {ASP, San Francisco},
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 251,
   editor = {{Inoue}, H. and {Kunieda}, H.},
    pages = {576},
   adsurl = {http://adsabs.harvard.edu/abs/2001ASPC..251..576M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mori07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.377..905M},
	Author = {{Mori}, K. and {Ho}, W.~C.~G.},
	Doi = {10.1111/j.1365-2966.2007.11663.x},
	Eprint = {arXiv:astro-ph/0611145},
	Journal = {\mnras},
	Keywords = {atomic processes, magnetic fields, stars: atmospheres, stars: neutron},
	Month = may,
	Pages = {905-919},
	Title = {{Modelling mid-Z element atmospheres for strongly magnetized neutron stars}},
	Volume = 377,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11663.x}}

@article{mori13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770L..23M},
	Archiveprefix = {arXiv},
	Author = {{Mori}, K. and {Gotthelf}, E.~V. and {Zhang}, S. and {An}, H. and {Baganoff}, F.~K. and {Barri{\`e}re}, N.~M. and {Beloborodov}, A.~M. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Dufour}, F. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Harrison}, F.~A. and {Hong}, J. and {Kaspi}, V.~M. and {Kennea}, J.~A. and {Madsen}, K.~K. and {Markwardt}, C.~B. and {Nynka}, M. and {Stern}, D. and {Tomsick}, J.~A. and {Zhang}, W.~W.},
	Doi = {10.1088/2041-8205/770/2/L23},
	Eid = {L23},
	Eprint = {1305.1945},
	Journal = {\apjl},
	Keywords = {Galaxy: center, pulsars: general, pulsars: individual: SGR J1745-29, stars: neutron},
	Month = jun,
	Pages = {L23},
	Primaryclass = {astro-ph.HE},
	Title = {{NuSTAR Discovery of a 3.76 s Transient Magnetar Near Sagittarius A*}},
	Volume = 770,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/770/2/L23}}

@article{morii03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003PASJ...55L..45M&db_key=AST},
	Author = {{Morii}, M. and {Sato}, R. and {Kataoka}, J. and {Kawai}, N.},
	Journal = {\pasj},
	Month = jun,
	Pages = {L45-L48},
	Title = {{Chandra Observation of the Anomalous X-Ray Pulsar 1E 1841-045}},
	Volume = 55,
	Year = 2003}

@ARTICLE{morris07,
   author = {{Morris}, T. and {Podsiadlowski}, P.},
    title = "{The Triple-Ring Nebula Around SN 1987A: Fingerprint of a Binary Merger}",
  journal = {Science},
   eprint = {astro-ph/0703317},
     year = 2007,
    month = feb,
   volume = 315,
    pages = {1103},
      doi = {10.1126/science.1136351},
   adsurl = {http://adsabs.harvard.edu/abs/2007Sci...315.1103M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{morrison83,
   author = {{Morrison}, R. and {McCammon}, D.},
    title = "{Interstellar photoelectric absorption cross sections, 0.03-10 keV}",
  journal = {\apj},
 keywords = {Absorption Cross Sections, Cosmic Dust, Interstellar Chemistry, Interstellar Matter, X Ray Astronomy, Abundance, Electrophotometry, Ionization, Molecules},
     year = 1983,
    month = jul,
   volume = 270,
    pages = {119-122},
      doi = {10.1086/161102},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..119M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{morscher15,
       author = {{Morscher}, Meagan and {Pattabiraman}, Bharath and {Rodriguez}, Carl and
         {Rasio}, Frederic A. and {Umbreit}, Stefan},
        title = "{The Dynamical Evolution of Stellar Black Holes in Globular Clusters}",
      journal = {\apj},
     keywords = {binaries: close, globular clusters: general, gravitational waves, methods: numerical, stars: black holes, stars: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {800},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0004-637X/800/1/9},
archivePrefix = {arXiv},
       eprint = {1409.0866},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...800....9M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{motta09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400.1603M},
	Archiveprefix = {arXiv},
	Author = {{Motta}, S. and {Belloni}, T. and {Homan}, J.},
	Doi = {10.1111/j.1365-2966.2009.15566.x},
	Eprint = {0908.2451},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , black hole physics , stars: individual: GX 339-4 , X-rays: binaries},
	Month = dec,
	Pages = {1603-1612},
	Title = {{The evolution of the high-energy cut-off in the X-ray spectrum of GX 339-4 across a hard-to-soft transition}},
	Volume = {400},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15566.x}}

@article{motta12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Author = {{Motta}, S. and {Homan}, J. and {Mu\~{n}oz-Darias}, T. and {Casella}, P. and {Belloni}, T.~M. and {Hiemstra}, B. and {M\`endez, M}.},
	Journal = {\mnras, in press (eprint: astro-ph.HE/1209.0327)},
	Month = sep,
	Title = {{Discovery of two simultaneous non-harmonically related Quasi-Periodic Oscillations in the 2005 outburst of the black-hole binary GRO J1655-40}},
	Year = {2012}}

@ARTICLE{motta20,
       author = {{Motta}, S.~E. and {Marelli}, M. and {Pintore}, F. and {Esposito}, P. and
         {Salvaterra}, R. and {De Luca}, A. and {Israel}, G.~L. and
         {Tiengo}, A. and {Castillo}, G.~A. Rodr{\'\i}guez},
        title = "{The Slow Heartbeats of an Ultraluminous X-Ray Source in NGC 3621}",
      journal = {\apj},
     keywords = {Black holes, Neutron stars, Accretion, X-ray point sources, Compact objects, Extragalactic astronomy, 162, 1108, 14, 1270, 288, 506, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = aug,
       volume = {898},
       number = {2},
          eid = {174},
        pages = {174},
          doi = {10.3847/1538-4357/ab9b81},
archivePrefix = {arXiv},
       eprint = {2006.05384},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...898..174M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mucciarelli06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365.1123M},
	Author = {{Mucciarelli}, P. and {Casella}, P. and {Belloni}, T. and {Zampieri}, L. and {Ranalli}, P.},
	Doi = {10.1111/j.1365-2966.2005.09754.x},
	Eprint = {arXiv:astro-ph/0509796},
	Journal = {\mnras},
	Keywords = {stars: oscillations, galaxies: individual: M82, X-rays: binaries, X-rays: individual: M82 X-1, X-rays: stars},
	Month = feb,
	Pages = {1123-1130},
	Title = {{A variable Quasi-Periodic Oscillation in M82 X-1. Timing and spectral analysis of XMM-Newton and RossiXTE observations}},
	Volume = 365,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09754.x}}

@article{mukai93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993Legac...3...21M},
	Author = {{Mukai}, K.},
	Journal = {Legacy, vol.~3, p.21-31},
	Month = may,
	Pages = {21-31},
	Title = {{PIMMS and Viewing: proposal preparation tools}},
	Volume = 3,
	Year = 1993}

@article{mukherjee09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691.1707M},
	Archiveprefix = {arXiv},
	Author = {{Mukherjee}, R. and {Gotthelf}, E.~V. and {Halpern}, J.~P.},
	Doi = {10.1088/0004-637X/691/2/1707},
	Eprint = {0810.1605},
	Journal = {\apj},
	Keywords = {gamma rays: observations, pulsars: individual: PSR J1833{\ndash}0827 XMMU J183435.3{\ndash}084443},
	Month = feb,
	Pages = {1707-1711},
	Title = {{On the Origin of TeV Gamma-Ray Emission from HESS J1834-087}},
	Volume = 691,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/691/2/1707}}

@article{mulchaey93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...404L...9M},
	Author = {{Mulchaey}, J.~S. and {Davis}, D.~S. and {Mushotzky}, R.~F. and {Burstein}, D.},
	Doi = {10.1086/186731},
	Journal = {\apjl},
	Keywords = {Dark Matter, Diffuse Radiation, Galactic Evolution, Galactic Structure, X Ray Astronomy, Elliptical Galaxies, Lenticular Bodies},
	Month = feb,
	Pages = {L9-L12},
	Title = {{Diffuse X-ray emission from the NGC 2300 group of galaxies - Implications for dark matter and galaxy evolution in small groups}},
	Volume = 404,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/186731}}

@article{muno03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...589..225M},
	Author = {{Muno}, M.~P. and {Baganoff}, F.~K. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Broos}, P.~S. and {Feigelson}, E.~D. and {Garmire}, G.~P. and {Morris}, M.~R. and {Ricker}, G.~R. and {Townsley}, L.~K.},
	Doi = {10.1086/374639},
	Eprint = {astro-ph/0301371},
	Journal = {\apj},
	Keywords = {Catalogs, Galaxy: Center, X-Rays: General},
	Month = may,
	Pages = {225-241},
	Title = {{A Deep Chandra Catalog of X-Ray Point Sources toward the Galactic Center}},
	Volume = 589,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/374639}}

@article{mbb03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...599..465M},
	Author = {{Muno}, M.~P. and {Baganoff}, F.~K. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Garmire}, G.~P. and {Ricker}, G.~R.},
	Doi = {10.1086/379244},
	Eprint = {astro-ph/0308335},
	Journal = {\apj},
	Keywords = {Stars: Novae, Cataclysmic Variables, Stars: Pulsars: General, Stars: Rotation, X-Rays: Binaries},
	Month = dec,
	Pages = {465-474},
	Title = {{X-Ray Sources with Periodic Variability in a Deep Chandra Image of the Galactic Center}},
	Volume = 599,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379244}}

@article{muno04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613.1179M},
	Author = {{Muno}, M.~P. and {Arabadjis}, J.~S. and {Baganoff}, F.~K. and {Bautz}, M.~W. and {Brandt}, W.~N. and {Broos}, P.~S. and {Feigelson}, E.~D. and {Garmire}, G.~P. and {Morris}, M.~R. and {Ricker}, G.~R.},
	Doi = {10.1086/423164},
	Eprint = {astro-ph/0403463},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Galaxy: Center, Stars: Novae, Cataclysmic Variables, X-Rays: Binaries, X-Rays: Stars},
	Month = oct,
	Pages = {1179-1201},
	Title = {{The Spectra and Variability of X-Ray Sources in a Deep Chandra Observation of the Galactic Center}},
	Volume = 613,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423164}}

@article{muno06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...636L..41M},
	Author = {{Muno}, M.~P. and {Clark}, J.~S. and {Crowther}, P.~A. and {Dougherty}, S.~M. and {de Grijs}, R. and {Law}, C. and {McMillan}, S.~L.~W. and {Morris}, M.~R. and {Negueruela}, I. and {Pooley}, D. and {Portegies Zwart}, S. and {Yusef-Zadeh}, F.},
	Doi = {10.1086/499776},
	Eprint = {arXiv:astro-ph/0509408},
	Journal = {\apjl},
	Keywords = {open clusters and associations: individual (Westerlund 1), Stars: Neutron, X-Rays: Stars},
	Month = jan,
	Pages = {L41-L44},
	Title = {{A Neutron Star with a Massive Progenitor in Westerlund 1}},
	Volume = 636,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/499776}}

@article{mbb06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..165..173M},
	Author = {{Muno}, M.~P. and {Bauer}, F.~E. and {Bandyopadhyay}, R.~M. and {Wang}, Q.~D.},
	Doi = {10.1086/504798},
	Eprint = {astro-ph/0601627},
	Journal = {\apjs},
	Keywords = {Catalogs, Galaxy: Center, X-Rays: General},
	Month = jul,
	Pages = {173-187},
	Title = {{A Chandra Catalog of X-Ray Sources in the Central 150 pc of the Galaxy}},
	Volume = 165,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/504798}}

@article{muno07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...656L..69M},
	Author = {{Muno}, M.~P. and {Baganoff}, F.~K. and {Brandt}, W.~N. and {Park}, S. and {Morris}, M.~R.},
	Doi = {10.1086/512236},
	Eprint = {arXiv:astro-ph/0611651},
	Journal = {\apjl},
	Keywords = {Galaxy: Center, ISM: Clouds, X-Rays: ISM},
	Month = feb,
	Pages = {L69-L72},
	Title = {{Discovery of Variable Iron Fluorescence from Reflection Nebulae in the Galactic Center}},
	Volume = 656,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/512236}}

@article{muno08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...680..639M},
	Archiveprefix = {arXiv},
	Author = {{Muno}, M.~P. and {Gaensler}, B.~M. and {Nechita}, A. and {Miller}, J.~M. and {Slane}, P.~O.},
	Doi = {10.1086/527316},
	Eprint = {0711.0988},
	Journal = {\apj},
	Keywords = {Stars: Neutron, Stars: Statistics, X-Rays: Stars},
	Month = jun,
	Pages = {639-653},
	Title = {{A Search for New Galactic Magnetars in Archival Chandra and XMM-Newton Observations}},
	Volume = 680,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/527316}}

@article{muno09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJS..181..110M},
	Archiveprefix = {arXiv},
	Author = {{Muno}, M.~P. and {Bauer}, F.~E. and {Baganoff}, F.~K. and {Bandyopadhyay}, R.~M. and {Bower}, G.~C. and {Brandt}, W.~N. and {Broos}, P.~S. and {Cotera}, A. and {Eikenberry}, S.~S. and {Garmire}, G.~P. and {Hyman}, S.~D. and {Kassim}, N.~E. and {Lang}, C.~C. and {Lazio}, T.~J.~W. and {Law}, C. and {Mauerhan}, J.~C. and {Morris}, M.~R. and {Nagata}, T. and {Nishiyama}, S. and {Park}, S. and {Ram{\`\i}rez}, S.~V. and {Stolovy}, S.~R. and {Wijnands}, R. and {Wang}, Q.~D. and {Wang}, Z. and {Yusef-Zadeh}, F.},
	Doi = {10.1088/0067-0049/181/1/110},
	Eprint = {0809.1105},
	Journal = {\apjs},
	Keywords = {Galaxy: center, X-rays: stars},
	Month = mar,
	Pages = {110-128},
	Title = {{A Catalog of X-Ray Point Sources from Two Megaseconds of Chandra Observations of the Galactic Center}},
	Volume = 181,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/181/1/110}}

@article{murakami94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994Natur.368..127M&db_key=AST},
	Author = {{Murakami}, T. and {Tanaka}, Y. and {Kulkarni}, S.~R. and {Ogasaka}, Y. and {Sonobe}, T. and {Ogawara}, Y. and {Aoki}, T. and {Yoshida}, A.},
	Journal = {\nat},
	Month = mar,
	Pages = {127},
	Title = {{X-Ray Identification of the Soft Gamma-Ray Repeater 1806-20}},
	Volume = 368,
	Year = 1994}

@article{murakami99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999ApJ...510L.119M&db_key=AST},
	Author = {{Murakami}, T. and {Kubo}, S. and {Shibazaki}, N. and {Takeshima}, T. and {Yoshida}, A. and {Kawai}, N.},
	Journal = {\apjl},
	Month = jan,
	Pages = {L119-L122},
	Title = {{Accurate Position of SGR 1900+14 by Bursts and Changes in Pulse Period and Folded Pulse Profile with ASCA}},
	Volume = 510,
	Year = 1999}

@article{murphy07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382..382M},
	Archiveprefix = {arXiv},
	Author = {{Murphy}, T. and {Mauch}, T. and {Green}, A. and {Hunstead}, R.~W. and {Piestrzynska}, B. and {Kels}, A.~P. and {Sztajer}, P.},
	Doi = {10.1111/j.1365-2966.2007.12379.x},
	Eprint = {0708.3092},
	Journal = {\mnras},
	Keywords = {methods: data analysis , catalogues , surveys , Galaxy: general , radio continuum: ISM},
	Month = nov,
	Pages = {382-392},
	Title = {{The second epoch Molonglo Galactic Plane Survey: compact source catalogue}},
	Volume = 382,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12379.x}}

@inproceedings{murray00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000SPIE.4012...68M&db_key=AST},
	Author = {{Murray}, S.~S. and {Austin}, G.~K. and {Chappell}, J.~H. and {Gomes}, J.~J. and {Kenter}, A.~T. and {Kraft}, R.~P. and {Meehan}, G.~R. and {Zombeck}, M.~V. and {Fraser}, G.~W. and {Serio}, S.},
	Booktitle = {Proc. SPIE Vol. 4012, X-Ray Optics, Instruments, and Missions III},
	Editor = {{Truemper}, J.~E. and {Aschenbach}, B.},
	Publisher = {SPIE, Bellingham},
	Month = jul,
	Pages = {68},
	Title = {{In-flight performance of the Chandra high-resolution camera}},
	Year = 2000}

@article{mushotzky04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004PThPS.155...27M},
	Author = {{Mushotzky}, R.},
	Doi = {10.1143/PTPS.155.27},
	Eprint = {astro-ph/0411040},
	Journal = {Progress of Theoretical Physics Supplement},
	Pages = {27-44},
	Title = {{Ultra-Luminous Sources in Nearby Galaxies}},
	Volume = 155,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1143/PTPS.155.27}}

@ARTICLE{mushtukov15,
   author = {{Mushtukov}, A.~A. and {Suleimanov}, V.~F. and {Tsygankov}, S.~S. and 
	{Poutanen}, J.},
    title = "{On the maximum accretion luminosity of magnetized neutron stars: connecting X-ray pulsars and ultraluminous X-ray sources}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1506.03600},
 primaryClass = "astro-ph.HE",
 keywords = {scattering, stars: neutron, pulsars: general, X-rays: binaries},
     year = 2015,
    month = dec,
   volume = 454,
    pages = {2539-2548},
      doi = {10.1093/mnras/stv2087},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.454.2539M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{nakagawa07_gcn,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007GCN..6264....1N},
	Author = {{Nakagawa}, Y.~E. and {Yamaoka}, K. and {Yoshida}, A. and {Sugita}, S. and {Mihara}, T. and {Suzuki}, M. and {Murakami}, T. and {Yonetoku}, D. and {Nakajima}, M. and {Tashiro}, M. and {Nakazawa}, K.},
	Journal = {GCN Circ. 6264},
	Title = {{Suzaku ToO observation of Sgr 1806-20.}},
	Year = 2007}

@article{nakagawa07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007astro.ph..1701N},
	Author = {{Nakagawa}, Y.~E. and {Yoshida}, A. and {Hurley}, K. and {Atteia}, J.-L. and {Maetou}, M. and {Tamagawa}, T. and {Suzuki}, M. and {Yamazaki}, T. and {Tanaka}, K. and {Kawai}, N. and {Shirasaki}, Y. and {Pelangeon}, A. and {Matsuoka}, M. and {Vanderspek}, R. and {Crew}, G.~B. and {Villasenor}, J.~S. and {Sato}, R. and {Sugita}, S. and {Kotoku}, J. and {Arimoto}, M. and {Pizzichini}, G. and {Doty}, J.~P. and {Ricker}, G.~R.},
	Eprint = {astro-ph/0701701},
	Journal = {\pasj},
	Month = apr,
	Pages = {653-678},
	Title = {{A Comprehensive Study of Short Bursts from SGR 1806-20 and SGR 1900+14 Detected by HETE-2}},
	Volume = 59,
	Year = 2007}

@article{nakagawa08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007arXiv0710.3816N},
	Author = {{Nakagawa}, Y.~E. and {Yoshida}, A. and {Yamaoka}, K. and {Shibazaki}, N.},
	Eprint = {0710.3816},
	Journal = {preprint (astro-ph/0710.3816)},
	Month = oct,
	Title = {{A Spectral Unified Scheme of Steady Emission and Short Bursts for Magnetar Candidates}},
	Year = 2007}

@ARTICLE{nandra13,
       author = {{Nandra}, Kirpal and {Barret}, Didier and {Barcons}, Xavier and {Fabian}, Andy and {den Herder}, Jan-Willem and {Piro}, Luigi and {Watson}, Mike and {Adami}, Christophe and {Aird}, James and {Afonso}, Jose Manuel and {Alexander}, Dave and {Argiroffi}, Costanza and {Amati}, Lorenzo and {Arnaud}, Monique and {Atteia}, Jean-Luc and {Audard}, Marc and {Badenes}, Carles and {Ballet}, Jean and {Ballo}, Lucia and {Bamba}, Aya and {Bhardwaj}, Anil and {Stefano Battistelli}, Elia and {Becker}, Werner and {De Becker}, Micha{\"e}l and {Behar}, Ehud and {Bianchi}, Stefano and {Biffi}, Veronica and {B{\^\i}rzan}, Laura and {Bocchino}, Fabrizio and {Bogdanov}, Slavko and {Boirin}, Laurence and {Boller}, Thomas and {Borgani}, Stefano and {Borm}, Katharina and {Bouch{\'e}}, Nicolas and {Bourdin}, Herv{\'e} and {Bower}, Richard and {Braito}, Valentina and {Branchini}, Enzo and {Branduardi-Raymont}, Graziella and {Bregman}, Joel and {Brenneman}, Laura and {Brightman}, Murray and {Br{\"u}ggen}, Marcus and {Buchner}, Johannes and {Bulbul}, Esra and {Brusa}, Marcella and {Bursa}, Michal and {Caccianiga}, Alessandro and {Cackett}, Ed and {Campana}, Sergio and {Cappelluti}, Nico and {Cappi}, Massimo and {Carrera}, Francisco and {Ceballos}, Maite and {Christensen}, Finn and {Chu}, You-Hua and {Churazov}, Eugene and {Clerc}, Nicolas and {Corbel}, Stephane and {Corral}, Amalia and {Comastri}, Andrea and {Costantini}, Elisa and {Croston}, Judith and {Dadina}, Mauro and {D'Ai}, Antonino and {Decourchelle}, Anne and {Della Ceca}, Roberto and {Dennerl}, Konrad and {Dolag}, Klaus and {Done}, Chris and {Dovciak}, Michal and {Drake}, Jeremy and {Eckert}, Dominique and {Edge}, Alastair and {Ettori}, Stefano and {Ezoe}, Yuichiro and {Feigelson}, Eric and {Fender}, Rob and {Feruglio}, Chiara and {Finoguenov}, Alexis and {Fiore}, Fabrizio and {Galeazzi}, Massimiliano and {Gallagher}, Sarah and {Gandhi}, Poshak and {Gaspari}, Massimo and {Gastaldello}, Fabio and {Georgakakis}, Antonis and {Georgantopoulos}, Ioannis and {Gilfanov}, Marat and {Gitti}, Myriam and {Gladstone}, Randy and {Goosmann}, Rene and {Gosset}, Eric and {Grosso}, Nicolas and {Guedel}, Manuel and {Guerrero}, Martin and {Haberl}, Frank and {Hardcastle}, Martin and {Heinz}, Sebastian and {Alonso Herrero}, Almudena and {Herv{\'e}}, Anthony and {Holmstrom}, Mats and {Iwasawa}, Kazushi and {Jonker}, Peter and {Kaastra}, Jelle and {Kara}, Erin and {Karas}, Vladimir and {Kastner}, Joel and {King}, Andrew and {Kosenko}, Daria and {Koutroumpa}, Dimita and {Kraft}, Ralph and {Kreykenbohm}, Ingo and {Lallement}, Rosine and {Lanzuisi}, Giorgio and {Lee}, J. and {Lemoine-Goumard}, Marianne and {Lobban}, Andrew and {Lodato}, Giuseppe and {Lovisari}, Lorenzo and {Lotti}, Simone and {McCharthy}, Ian and {McNamara}, Brian and {Maggio}, Antonio and {Maiolino}, Roberto and {De Marco}, Barbara and {de Martino}, Domitilla and {Mateos}, Silvia and {Matt}, Giorgio and {Maughan}, Ben and {Mazzotta}, Pasquale and {Mendez}, Mariano and {Merloni}, Andrea and {Micela}, Giuseppina and {Miceli}, Marco and {Mignani}, Robert and {Miller}, Jon and {Miniutti}, Giovanni and {Molendi}, Silvano and {Montez}, Rodolfo and {Moretti}, Alberto and {Motch}, Christian and {Naz{\'e}}, Ya{\"e}l and {Nevalainen}, Jukka and {Nicastro}, Fabrizio and {Nulsen}, Paul and {Ohashi}, Takaya and {O'Brien}, Paul and {Osborne}, Julian and {Oskinova}, Lida and {Pacaud}, Florian and {Paerels}, Frederik and {Page}, Mat and {Papadakis}, Iossif and {Pareschi}, Giovanni and {Petre}, Robert and {Petrucci}, Pierre-Olivier and {Piconcelli}, Enrico and {Pillitteri}, Ignazio and {Pinto}, C. and {de Plaa}, Jelle and {Pointecouteau}, Etienne and {Ponman}, Trevor and {Ponti}, Gabriele and {Porquet}, Delphine and {Pounds}, Ken and {Pratt}, Gabriel and {Predehl}, Peter and {Proga}, Daniel and {Psaltis}, Dimitrios and {Rafferty}, David and {Ramos-Ceja}, Miriam and {Ranalli}, Piero and {Rasia}, Elena and {Rau}, Arne and {Rauw}, Gregor and {Rea}, Nanda and {Read}, Andy and {Reeves}, James and {Reiprich}, Thomas and {Renaud}, Matthieu and {Reynolds}, Chris and {Risaliti}, Guido and {Rodriguez}, Jerome and {Rodriguez Hidalgo}, Paola and {Roncarelli}, Mauro and {Rosario}, David and {Rossetti}, Mariachiara and {Rozanska}, Agata and {Rovilos}, Emmanouil and {Salvaterra}, Ruben and {Salvato}, Mara and {Di Salvo}, Tiziana and {Sanders}, Jeremy and {Sanz-Forcada}, Jorge and {Schawinski}, Kevin and {Schaye}, Joop and {Schwope}, Axel and {Sciortino}, Salvatore and {Severgnini}, Paola and {Shankar}, Francesco and {Sijacki}, Debora and {Sim}, Stuart and {Schmid}, Christian and {Smith}, Randall and {Steiner}, Andrew and {Stelzer}, Beate and {Stewart}, Gordon and {Strohmayer}, Tod and {Str{\"u}der}, Lothar and {Sun}, Ming and {Takei}, Yoh and {Tatischeff}, V. and {Tiengo}, Andreas and {Tombesi}, Francesco and {Trinchieri}, Ginevra and {Tsuru}, T.~G. and {Ud-Doula}, Asif and {Ursino}, Eugenio and {Valencic}, Lynne and {Vanzella}, Eros and {Vaughan}, Simon and {Vignali}, Cristian and {Vink}, Jacco and {Vito}, Fabio and {Volonteri}, Marta and {Wang}, Daniel and {Webb}, Natalie and {Willingale}, Richard and {Wilms}, Joern and {Wise}, Michael and {Worrall}, Diana and {Young}, Andrew and {Zampieri}, Luca and {In't Zand}, Jean and {Zane}, Silvia and {Zezas}, Andreas and {Zhang}, Yuying and {Zhuravleva}, Irina},
        title = "{The Hot and Energetic Universe: A White Paper presenting the science theme motivating the Athena+ mission}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = jun,
          eid = {arXiv:1306.2307},
        pages = {arXiv:1306.2307},
archivePrefix = {arXiv},
       eprint = {1306.2307},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013arXiv1306.2307N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{nauenberg72,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...175..417N},
	Author = {{Nauenberg}, M.},
	Doi = {10.1086/151568},
	Journal = {\apj},
	Month = jul,
	Pages = {417},
	Title = {{Analytic Approximations to the Mass-Radius Relation and Energy of Zero-Temperature Stars}},
	Volume = 175,
	Year = 1972,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/151568}}

@article{navarro97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...490..493N},
	Author = {{Navarro}, J.~F. and {Frenk}, C.~S. and {White}, S.~D.~M.},
	Eprint = {astro-ph/9611107},
	Journal = {\apj},
	Keywords = {Cosmology: Theory, Cosmology: Dark Matter, Galaxies: Halos, Methods: Numerical},
	Month = dec,
	Pages = {493-508},
	Title = {{A Universal Density Profile from Hierarchical Clustering}},
	Volume = 490,
	Year = 1997}

@article{naze04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...608..208N},
	Author = {{Naz{\'e}}, Y. and {Manfroid}, J. and {Stevens}, I.~R. and {Corcoran}, M.~F. and {Flores}, A.},
	Doi = {10.1086/386323},
	Eprint = {arXiv:astro-ph/0402629},
	Journal = {\apj},
	Month = jun,
	Pages = {208-219},
	Title = {{An X-Ray Investigation of the NGC 346 Field in the Small Magellanic Cloud. III. XMM-Newton Data}},
	Volume = 608,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/386323}}

@INPROCEEDINGS{neiner15,
   author = {{Neiner}, C. and {Morin}, J. and {Alecian}, E.},
    title = "{The ``Binarity and Magnetic Interactions in various classes of stars'' (BinaMIcS) project}",
 keywords = {stars: magnetic field, binaries: spectroscopic, binaries: close, techniques: polarimetric},
booktitle = {SF2A-2015: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
     year = 2015,
archivePrefix = "arXiv",
   eprint = {1510.02121},
 primaryClass = "astro-ph.SR",
   editor = {{Martins}, F. and {Boissier}, S. and {Buat}, V. and {Cambr{\'e}sy}, L. and 
	{Petit}, P.},
    month = dec,
    pages = {213-216},
   adsurl = {http://adsabs.harvard.edu/abs/2015sf2a.conf..213N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ng09,
   author = {{Ng}, C.-Y. and {Gaensler}, B.~M. and {Murray}, S.~S. and {Slane}, P.~O. and 
	{Park}, S. and {Staveley-Smith}, L. and {Manchester}, R.~N. and 
	{Burrows}, D.~N.},
    title = "{High-Resolution X-Ray Imaging of Supernova Remnant 1987A}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0910.3610},
 primaryClass = "astro-ph.HE",
 keywords = {circumstellar matter, shock waves, stars: neutron, supernova remnants, supernovae: individual: SN 1987A, X-rays: general},
     year = 2009,
    month = nov,
   volume = 706,
    pages = {L100-L105},
      doi = {10.1088/0004-637X/706/1/L100},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...706L.100N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{negueruela98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...336..251N},
	Author = {{Negueruela}, I. and {Reig}, P. and {Coe}, M.~J. and {Fabregat}, J.},
	Eprint = {arXiv:astro-ph/9804307},
	Journal = {\aap},
	Keywords = {STARS: CIRCUMSTELLAR MATTER, STARS: EMISSION LINE, BE, BINARIES: CLOSE, STARS: NEUTRON, X-RAYS: STARS},
	Month = aug,
	Pages = {251-262},
	Title = {{Large-scale perturbations in the circumstellar envelopes of Be/X-ray binaries}},
	Volume = 336,
	Year = 1998}

@article{nelemans01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...368..939N},
	Author = {{Nelemans}, G. and {Portegies Zwart}, S.~F. and {Verbunt}, F. and {Yungelson}, L.~R.},
	Doi = {10.1051/0004-6361:20010049},
	Eprint = {arXiv:astro-ph/0101123},
	Journal = {\aap},
	Keywords = {STARS: WHITE DWARFS, STARS: STATISTICS, BINARIES: CLOSE, BINARIES: EVOLUTION},
	Month = mar,
	Pages = {939-949},
	Title = {{Population synthesis for double white dwarfs. II. Semi-detached systems: AM CVn stars}},
	Volume = 368,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20010049}}

@article{nelemans04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.349..181N},
	Author = {{Nelemans}, G. and {Yungelson}, L.~R. and {Portegies Zwart}, S.~F.},
	Doi = {10.1111/j.1365-2966.2004.07479.x},
	Eprint = {arXiv:astro-ph/0312193},
	Journal = {\mnras},
	Keywords = {gravitational waves, binaries: close, white dwarfs},
	Month = mar,
	Pages = {181-192},
	Title = {{Short-period AM CVn systems as optical, X-ray and gravitational-wave sources}},
	Volume = 349,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2004.07479.x}}

@article{nelemans09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009CQGra..26i4030N},
	Archiveprefix = {arXiv},
	Author = {{Nelemans}, G.},
	Doi = {10.1088/0264-9381/26/9/094030},
	Eprint = {0901.1778},
	Journal = {Classical and Quantum Gravity},
	Month = may,
	Number = 9,
	Pages = {094030},
	Primaryclass = {astro-ph.SR},
	Title = {{The Galactic gravitational wave foreground}},
	Volume = 26,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0264-9381/26/9/094030}}

@inproceedings{nelemans13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ASPC..467...27N},
	Archiveprefix = {arXiv},
	Author = {{Nelemans}, G.},
	Booktitle = {The 9th LISA Symposium},
	Editor = {{Auger}, G. and {Bin{\'e}truy}, P. and {Plagnol}, E.},
	Eprint = {1302.0138},
	Month = jan,
	Pages = {27},
	Primaryclass = {astro-ph.HE},
	Publisher = {ASP, San Francisco},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{Galactic Binaries with eLISA}},
	Volume = 467,
	Year = 2013}

@article{neronov07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007astro.ph..1144N},
	Author = {{Neronov}, A. and {Chernyakova}, M.},
	Eprint = {astro-ph/0701144},
	Journal = {submitted to \mnras, (astro-ph/0701144)},
	Month = jan,
	Title = {{Compactified pulsar wind nebula model of gamma-ray loud binary LSI +61 303}},
	Year = 2007}

@article{nespoli08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...486..911N},
	Archiveprefix = {arXiv},
	Author = {{Nespoli}, E. and {Fabregat}, J. and {Mennickent}, R.~E.},
	Doi = {10.1051/0004-6361:200809645},
	Eprint = {0806.0295},
	Journal = {\aap},
	Keywords = {X-rays: binaries, stars: supergiants, accretion, accretion disks, infrared: stars},
	Month = aug,
	Pages = {911-917},
	Title = {{Unveiling the nature of six HMXBs through IR spectroscopy}},
	Volume = 486,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200809645}}

@article{nevalainen10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...523A..22N},
	Archiveprefix = {arXiv},
	Author = {{Nevalainen}, J. and {David}, L. and {Guainazzi}, M.},
	Doi = {10.1051/0004-6361/201015176},
	Eid = {A22},
	Eprint = {1008.2102},
	Journal = {\aap},
	Keywords = {instrumentation: miscellaneous, techniques: spectroscopic, galaxies: clusters: intracluster medium, X-rays: galaxies: clusters},
	Month = nov,
	Pages = {A22},
	Primaryclass = {astro-ph.IM},
	Title = {{Cross-calibrating X-ray detectors with clusters of galaxies: an IACHEC study}},
	Volume = 523,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201015176}}

@ARTICLE{newman05,
   author = {{Newman}, M.~E.~J.},
    title = "{Power laws, Pareto distributions and Zipf's law}",
  journal = {Contemporary Physics},
   eprint = {cond-mat/0412004},
     year = 2005,
    month = sep,
   volume = 46,
    pages = {323-351},
      doi = {10.1080/00107510500052444},
   adsurl = {http://adsabs.harvard.edu/abs/2005ConPh..46..323N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ng12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...761...65N},
	Archiveprefix = {arXiv},
	Author = {{Ng}, C.-Y. and {Kaspi}, V.~M. and {Ho}, W.~C.~G. and {Weltevrede}, P. and {Bogdanov}, S. and {Shannon}, R. and {Gonzalez}, M.~E.},
	Doi = {10.1088/0004-637X/761/1/65},
	Eid = {65},
	Eprint = {1211.2761},
	Journal = {\apj},
	Keywords = {ISM: individual objects: G292.2{\ndash}0.5, ISM: supernova remnants, pulsars: individual: PSR J1119{\ndash}6127, stars: neutron, X-rays: ISM},
	Month = dec,
	Pages = {65},
	Primaryclass = {astro-ph.HE},
	Title = {{Deep X-Ray Observations of the Young High-magnetic-field Radio Pulsar J1119-6127 and Supernova Remnant G292.2-0.5}},
	Volume = 761,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/761/1/65}}

@article{nichelli09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2354....1N},
	Author = {{Nichelli}, E. and {Israel}, G.~L. and {Moretti}, A. and {Campana}, S. and {Bernabei}, S. and {Mason}, E. and {G{\"o}tz}, D. and {Stella}, L.},
	Journal = {Astron.~Tel.},
	Keywords = {Optical, X-ray, Binaries, Cataclysmic Variables},
	Month = dec,
	Title = {{Swift-XRT detection of x-ray pulsations from IGR J18173-2509 and SWIFT J2138.8+5544}},
	Volume = 2354,
	Year = 2009}

@article{nichelli11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3205....1N},
	Author = {{Nichelli}, E. and {Israel}, G.~L. and {Moretti}, A. and {Campana}, S. and {G{\"o}tz}, D. and {Stella}, L.},
	Journal = {Astron.~Tel.},
	Keywords = {X-ray, Binary, Star, Pulsar},
	Month = mar,
	Title = {{Swift discovery of 328s coherent pulsations from the HMXB IGR J17200-3116}},
	Volume = 3205,
	Year = 2011}

@inproceedings{nichelli11b,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011sssf.confE..39N},
	Author = {{Nichelli}, E. and {Israel}, G. and {Moretti}, A. and {Stella}, L. and {Mason}, E. and {Campana}, S. and {G{\"o}tz}, D. and {Kunder}, A. and {Testa}, V. and {Belloni}, T.},
	Booktitle = {Swift and the Surprising Sky: The First Seven Years of Swift. Online at: http://www.brera.inaf.it/docM/OAB/Research/SWIFT/Swift7 /Presentations/Nichelli.pdf},
	Eid = {39},
	Month = nov,
	Pages = {39},
	Title = {{The Swift Gaze to the Milky Way}},
	Year = 2011}

@article{nicholl13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013Natur.502..346N},
	Archiveprefix = {arXiv},
	Author = {{Nicholl}, M. and {Smartt}, S.~J. and {Jerkstrand}, A. and {Inserra}, C. and {McCrum}, M. and {Kotak}, R. and {Fraser}, M. and {Wright}, D. and {Chen}, T.-W. and {Smith}, K. and {Young}, D.~R. and {Sim}, S.~A. and {Valenti}, S. and {Howell}, D.~A. and {Bresolin}, F. and {Kudritzki}, R.~P. and {Tonry}, J.~L. and {Huber}, M.~E. and {Rest}, A. and {Pastorello}, A. and {Tomasella}, L. and {Cappellaro}, E. and {Benetti}, S. and {Mattila}, S. and {Kankare}, E. and {Kangas}, T. and {Leloudas}, G. and {Sollerman}, J. and {Taddia}, F. and {Berger}, E. and {Chornock}, R. and {Narayan}, G. and {Stubbs}, C.~W. and {Foley}, R.~J. and {Lunnan}, R. and {Soderberg}, A. and {Sanders}, N. and {Milisavljevic}, D. and {Margutti}, R. and {Kirshner}, R.~P. and {Elias-Rosa}, N. and {Morales-Garoffolo}, A. and {Taubenberger}, S. and {Botticella}, M.~T. and {Gezari}, S. and {Urata}, Y. and {Rodney}, S. and {Riess}, A.~G. and {Scolnic}, D. and {Wood-Vasey}, W.~M. and {Burgett}, W.~S. and {Chambers}, K. and {Flewelling}, H.~A. and {Magnier}, E.~A. and {Kaiser}, N. and {Metcalfe}, N. and {Morgan}, J. and {Price}, P.~A. and {Sweeney}, W. and {Waters}, C.},
	Doi = {10.1038/nature12569},
	Eprint = {1310.4446},
	Journal = {\nat},
	Month = oct,
	Pages = {346-349},
	Primaryclass = {astro-ph.CO},
	Title = {{Slowly fading super-luminous supernovae that are not pair-instability explosions}},
	Volume = 502,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature12569}}

@article{nishimura00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000PASJ...52..167N&db_key=AST},
	Author = {{Nishimura}, O. and {Sumiyoshi}, K. and {Ebisuzaki}, T.},
	Journal = {\pasj},
	Month = feb,
	Pages = {167},
	Title = {{The Absence of Cyclotron Lines in Neutron-Star Atmospheres with Super-Strong Magnetic Fields}},
	Volume = 52,
	Year = 2000}

@article{nobili08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386.1527N},
	Archiveprefix = {arXiv},
	Author = {{Nobili}, L. and {Turolla}, R. and {Zane}, S.},
	Doi = {10.1111/j.1365-2966.2008.13125.x},
	Eprint = {0802.2647},
	Journal = {\mnras},
	Keywords = {radiation mechanisms: non-thermal , stars: neutron , X-rays: stars},
	Month = may,
	Pages = {1527-1542},
	Title = {{X-ray spectra from magnetar candidates - I. Monte Carlo simulations in the non-relativistic regime}},
	Volume = 386,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13125.x}}

@ARTICLE{norris91,
   author = {{Norris}, J.~P. and {Hertz}, P. and {Wood}, K.~S. and {Kouveliotou}, C.
	},
    title = "{On the nature of soft gamma repeaters}",
  journal = {\apj},
 keywords = {Gamma Ray Astronomy, Gamma Ray Bursts, Neutron Stars, Compton Effect, Cyclotron Resonance, Magellanic Clouds, Spatial Distribution, Starquakes, Synchrotron Radiation},
     year = 1991,
    month = jan,
   volume = 366,
    pages = {240-252},
      doi = {10.1086/169556},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...366..240N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{norton89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989MNRAS.237..853N},
	Author = {{Norton}, A.~J. and {Watson}, M.~G.},
	Journal = {\mnras},
	Keywords = {Cataclysmic Variables, Stellar Models, Stellar Spectra, X Ray Astronomy, Absorption Spectra, Exosat Satellite, Stellar Mass Accretion, White Dwarf Stars, X Ray Sources},
	Month = apr,
	Pages = {853-874},
	Title = {{Spin modulated X-ray emission from intermediate polars}},
	Volume = 237,
	Year = 1989}

@article{norton04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...419.1025N},
	Author = {{Norton}, A.~J. and {Haswell}, C.~A. and {Wynn}, G.~A.},
	Doi = {10.1051/0004-6361:20035906},
	Eprint = {arXiv:astro-ph/0206013},
	Journal = {\aap},
	Keywords = {stars: novae, cataclysmic variables, X-rays: stars, stars: individual: RX J1914.4+2456, stars: individual: V407 Vul, stars: individual: RX J0806.3+1527, stars: magnetic fields, stars: binaries},
	Month = jun,
	Pages = {1025-1033},
	Title = {{Face-on, stream-fed intermediate polars: An alternative model for RX J1914.4+2456 and RX J0806.3+1527}},
	Volume = 419,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20035906}}

@article{nws04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...614..349N},
	Author = {{Norton}, A.~J. and {Wynn}, G.~A. and {Somerscales}, R.~V.},
	Doi = {10.1086/423333},
	Eprint = {astro-ph/0406363},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Novae, Cataclysmic Variables, Stars: Magnetic Fields, Stars: White Dwarfs},
	Month = oct,
	Pages = {349-357},
	Title = {{The Spin Periods and Magnetic Moments of White Dwarfs in Magnetic Cataclysmic Variables}},
	Volume = 614,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/423333}}

@article{nowak12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...759...95N},
	Archiveprefix = {arXiv},
	Author = {{Nowak}, M.~A. and {Neilsen}, J. and {Markoff}, S.~B. and {Baganoff}, F.~K. and {Porquet}, D. and {Grosso}, N. and {Levin}, Y. and {Houck}, J. and {Eckart}, A. and {Falcke}, H. and {Ji}, L. and {Miller}, J.~M. and {Wang}, Q.~D.},
	Doi = {10.1088/0004-637X/759/2/95},
	Eid = {95},
	Eprint = {1209.6354},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, radiation mechanisms: non-thermal},
	Month = nov,
	Pages = {95},
	Primaryclass = {astro-ph.HE},
	Title = {{Chandra/HETGS Observations of the Brightest Flare Seen from Sgr A*}},
	Volume = 759,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/759/2/95}}

@article{nucita09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...504..973N},
	Archiveprefix = {arXiv},
	Author = {{Nucita}, A.~A. and {Maiolo}, B.~M.~T. and {Carpano}, S. and {Belanger}, G. and {Coia}, D. and {Guainazzi}, M. and {de Paolis}, F. and {Ingrosso}, G.},
	Doi = {10.1051/0004-6361/200811461},
	Eprint = {0907.4897},
	Journal = {\aap},
	Keywords = {stars: binaries: general, stars: white dwarfs, X-rays: binaries, stars: novae, cataclysmic variables},
	Month = sep,
	Pages = {973-979},
	Primaryclass = {astro-ph.HE},
	Title = {{The X-ray eclipse of the dwarf nova HT Cassiopeiae observed by the XMM-Newton satellite: spectral and timing analysis}},
	Volume = 504,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200811461}}

@article{nucita11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..75N},
	Author = {{Nucita}, A.~A. and {Kuulkers}, E. and {Maiolo}, B.~M.~T. and {de Paolis}, F. and {Ingrosso}, G. and {Vetrugno}, D.},
	Doi = {10.1051/0004-6361/201117572},
	Eid = {A75},
	Journal = {\aap},
	Keywords = {X-rays: binaries, white dwarfs, novae, cataclysmic variables},
	Month = dec,
	Pages = {A75},
	Title = {{The XMM-Newton view of the eclipse and dips of the dwarf nova Z Chamaleontis}},
	Volume = 536,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201117572}}

@article{nucita12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012JPhCS.354a2013N},
	Author = {{Nucita}, A.~A. and {De Paolis}, F. and {Ingrosso}, G.},
	Doi = {10.1088/1742-6596/354/1/012013},
	Eid = {012013},
	Journal = {Journal of Physics Conference Series},
	Month = mar,
	Number = 1,
	Pages = {012013},
	Title = {{X-rays from eclipsing cataclysmic variable systems: the eclipse profile}},
	Volume = 354,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/1742-6596/354/1/012013}}

@article{nulsen82,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1982MNRAS.198.1007N},
	Author = {{Nulsen}, P.~E.~J.},
	Journal = {\mnras},
	Keywords = {Cosmic Gases, Galactic Clusters, Gas Transport, Gas Viscosity, High Temperature Gases, Thermal Conductivity, Turbulence Effects, Elliptical Galaxies, Galactic Evolution, Intergalactic Media, Interstellar Gas, Ion Motion, Laminar Flow, Mean Free Path, Stripping (Distillation)},
	Month = mar,
	Pages = {1007-1016},
	Title = {{Transport processes and the stripping of cluster galaxies}},
	Volume = 198,
	Year = 1982}

@article{okazaki97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...318..548O},
	Author = {{Okazaki}, A.~T.},
	Journal = {\aap},
	Keywords = {GLOBAL DISC OSCILLATION, HYDRODYNAMICS, RADIATIVE TRANSFER, STARS: CIRCUMSTELLAR MATTER, STARS: EMISSION LINE, BE},
	Month = feb,
	Pages = {548-560},
	Title = {{On the confinement of one-armed oscillations in discs of Be stars.}},
	Volume = 318,
	Year = 1997}

@article{okazaki01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...377..161O},
	Author = {{Okazaki}, A.~T. and {Negueruela}, I.},
	Doi = {10.1051/0004-6361:20011083},
	Eprint = {arXiv:astro-ph/0108037},
	Journal = {\aap},
	Keywords = {STARS: CIRCUMSTELLAR MATTER, EMISSION-LINE, BE, BINARIES: CLOSE, NEUTRON, X-RAY: STARS, BURSTS},
	Month = oct,
	Pages = {161-174},
	Title = {{A natural explanation for periodic X-ray outbursts in Be/X-ray binaries}},
	Volume = 377,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20011083}}

@inproceedings{okazaki14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014efxu.conf..202O},
	Archiveprefix = {arXiv},
	Author = {{Okazaki}, A.~T. and {Russell}, C.~M.~P.},
	Booktitle = {Suzaku-MAXI 2014: Expanding the Frontiers of the X-ray Universe},
	Editor = {{Ishida}, M. and {Petre}, R. and {Mitsuda}, K.},
	Eprint = {1405.4808},
	Month = sep,
	Pages = {202},
	Primaryclass = {astro-ph.HE},
	Title = {{3D Dynamical Modeling of Wind Accretion in Cyg X-3}},
	Year = 2014}

@article{oke83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...266..713O},
	Author = {{Oke}, J.~B. and {Gunn}, J.~E.},
	Doi = {10.1086/160817},
	Journal = {\apj},
	Keywords = {REFERENCE STARS, SPECTRAL ENERGY DISTRIBUTION, STELLAR SPECTROPHOTOMETRY, SUBDWARF STARS, CALIBRATING, LINE SPECTRA},
	Month = mar,
	Pages = {713-717},
	Title = {{Secondary standard stars for absolute spectrophotometry}},
	Volume = 266,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160817}}

@article{olausen11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742....4O},
	Archiveprefix = {arXiv},
	Author = {{Olausen}, S.~A. and {Kaspi}, V.~M. and {Ng}, C.-Y. and {Zhu}, W.~W. and {Dib}, R. and {Gavriil}, F.~P. and {Woods}, P.~M.},
	Doi = {10.1088/0004-637X/742/1/4},
	Eid = {4},
	Eprint = {1107.2952},
	Journal = {\apj},
	Keywords = {pulsars: individual: 1E 1547.0{\ndash}5408, stars: neutron, X-rays: stars},
	Month = nov,
	Pages = {4},
	Primaryclass = {astro-ph.HE},
	Title = {{On the Extended Emission around the Anomalous X-Ray Pulsar 1E 1547.0-5408}},
	Volume = 742,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/742/1/4}}

@ARTICLE{olausen13,
   author = {{Olausen}, S.~A. and {Zhu}, W.~W. and {Vogel}, J.~K. and {Kaspi}, V.~M. and 
	{Lyne}, A.~G. and {Espinoza}, C.~M. and {Stappers}, B.~W. and 
	{Manchester}, R.~N. and {McLaughlin}, M.~A.},
    title = "{X-Ray Observations of High-B Radio Pulsars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1211.5387},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, pulsars: individual: PSR B1845{\ndash}19 PSR J1001{\ndash}5939 PSR J1734{\ndash}3333, stars: neutron, X-rays: stars},
     year = 2013,
    month = feb,
   volume = 764,
      eid = {1},
    pages = {1},
      doi = {10.1088/0004-637X/764/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...764....1O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oliva89,
   author = {{Oliva}, E. and {Moorwood}, A.~F.~M. and {Danziger}, I.~J.},
    title = "{Infrared spectroscopy of supernova remnants}",
  journal = {\aap},
 keywords = {Crab Nebula, Hydrogen Recombinations, Infrared Spectroscopy, Magellanic Clouds, Supernova Remnants, Astronomical Maps, H Ii Regions, Spatial Distribution},
     year = 1989,
    month = apr,
   volume = 214,
    pages = {307-320},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...214..307O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{olive04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...616.1148O&db_key=AST},
	Author = {{Olive}, J.-F. and {Hurley}, K. and {Sakamoto}, T. and {Atteia}, J.-L. and {Crew}, G. and {Ricker}, G. and {Pizzichini}, G. and {Barraud}, C. and {Kawai}, N.},
	Journal = {\apj},
	Month = dec,
	Pages = {1148-1158},
	Title = {{Time-resolved X-Ray Spectral Modeling of an Intermediate Burst from SGR 1900+14 Observed by HETE-2 FREGATE and WXM}},
	Volume = 616,
	Year = 2004}

@article{oosterbroek97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...327..215O},
	Author = {{Oosterbroek}, T. and {Parmar}, A.~N. and {Martin}, D.~D.~E. and {Lammers}, U.},
	Eprint = {astro-ph/9706188},
	Journal = {\aap},
	Keywords = {STARS: INDIVIDUAL: HER X-1, NEUTRON STARS, X-RAYS: STARS},
	Month = nov,
	Pages = {215-218},
	Title = {{The BeppoSAX LECS X-ray spectrum of Hercules X-1.}},
	Volume = 327,
	Year = 1997}

@article{orlandini98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500L.163O},
	Author = {{Orlandini}, M. and {Dal Fiume}, D. and {Frontera}, F. and {Del Sordo}, S. and {Piraino}, S. and {Santangelo}, A. and {Segreto}, A. and {Oosterbroek}, T. and {Parmar}, A.~N.},
	Doi = {10.1086/311404},
	Eprint = {astro-ph/9804241},
	Journal = {\apjl},
	Keywords = {STARS: BINARIES: CLOSE, STARS: NEUTRON, STARS: PULSARS: INDIVIDUAL ALPHANUMERIC: 4U 1626-67, X-RAYS: STARS, Stars: Binaries: Close, Stars: Pulsars: Individual: Alphanumeric: 4U 1626-67, Stars: Neutron, X-Rays: Stars},
	Month = jun,
	Pages = {L163-L166},
	Title = {{BEPPOSAX Observation of 4U 1626-67: Discovery of an Absorption Cyclotron Resonance Feature}},
	Volume = 500,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311404}}

@article{oskinova12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421.2820O},
	Archiveprefix = {arXiv},
	Author = {{Oskinova}, L.~M. and {Feldmeier}, A. and {Kretschmar}, P.},
	Doi = {10.1111/j.1365-2966.2012.20507.x},
	Eprint = {1201.1915},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, instabilities, stars: neutron, X-rays: binaries, X-rays: stars},
	Month = apr,
	Pages = {2820-2831},
	Primaryclass = {astro-ph.SR},
	Title = {{Clumped stellar winds in supergiant high-mass X-ray binaries: X-ray variability and photoionization}},
	Volume = 421,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.20507.x}}

@article{ostriker69,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1969ApJ...157.1395O&db_key=AST},
	Author = {{Ostriker}, J.~P. and {Gunn}, J.~E.},
	Journal = {\apj},
	Month = sep,
	Pages = {1395},
	Title = {{On the Nature of Pulsars. I. Theory}},
	Volume = 157,
	Year = 1969}

@article{ouyed02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...390L..39O},
	Author = {{Ouyed}, R. and {Dey}, J. and {Dey}, M.},
	Doi = {10.1051/0004-6361:20020982},
	Eprint = {arXiv:astro-ph/0105109},
	Journal = {\aap},
	Keywords = {dense matter, gamma ray: bursts, stars: interior},
	Month = jul,
	Pages = {L39-L42},
	Title = {{Quark-Nova}},
	Volume = 390,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020982}}

@article{ouyed04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...420.1025O},
	Author = {{Ouyed}, R. and {Elgar{\o}y}, {\O}. and {Dahle}, H. and {Ker{\"a}nen}, P.},
	Doi = {10.1051/0004-6361:20034180},
	Eprint = {arXiv:astro-ph/0308166},
	Journal = {\aap},
	Keywords = {gamma rays: bursts, X-rays: stars, stars: magnetic fields, stars: neutron, stars: quark star},
	Month = jun,
	Pages = {1025-1032},
	Title = {{Meissner effect and vortex dynamics in quark stars. A model for soft gamma-ray repeaters}},
	Volume = 420,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20034180}}

@article{ouyed07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...473..357O},
	Author = {{Ouyed}, R. and {Leahy}, D. and {Niebergal}, B.},
	Doi = {10.1051/0004-6361:20077412},
	Eprint = {arXiv:astro-ph/0608536},
	Journal = {\aap},
	Keywords = {dense matter, accretion, accretion disks, stars: pulsars: general, X-rays: bursts, elementary particles},
	Month = oct,
	Pages = {357-368},
	Title = {{Quark-nova remnants. I. The leftover debris with applications to SGRs, AXPs, and XDINs}},
	Volume = 473,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077412}}

@article{oln07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475...63O},
	Author = {{Ouyed}, R. and {Leahy}, D. and {Niebergal}, B.},
	Doi = {10.1051/0004-6361:20077426},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, stars: pulsars: general, dense matter, X-rays: bursts, elementary particles},
	Month = nov,
	Pages = {63-70},
	Title = {{Quark-nova remnants. II. The degenerate torus case with applications to AXPs}},
	Volume = 475,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077426}}

@ARTICLE{Oppenheimer1939,
       author = {{Oppenheimer}, J.~R. and {Volkoff}, G.~M.},
        title = "{On Massive Neutron Cores}",
      journal = {Physical Review},
         year = 1939,
        month = feb,
       volume = {55},
       number = {4},
        pages = {374-381},
          doi = {10.1103/PhysRev.55.374},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1939PhRv...55..374O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ouyed09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.1058O},
	Archiveprefix = {arXiv},
	Author = {{Ouyed}, R. and {Leahy}, D. and {Niebergal}, B. and {Yue}, Y.},
	Doi = {10.1111/j.1365-2966.2009.14773.x},
	Eprint = {0802.3929},
	Journal = {\mnras},
	Keywords = {stars: evolution , stars: neutron , supernovae: general},
	Month = jun,
	Pages = {1058-1065},
	Title = {{Quark-nova remnants: application to RRATs}},
	Volume = 396,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14773.x}}

@article{ouyed10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...516A..88O},
	Author = {{Ouyed}, R. and {Leahy}, D. and {Niebergal}, B.},
	Doi = {10.1051/0004-6361/200811114},
	Eid = {A88},
	Journal = {\aap},
	Keywords = {stars: evolution, accretion, accretion disks, magnetic fields, pulsars: general},
	Month = jun,
	Pages = {A88},
	Title = {{Quark-nova remnants. IV. Application to radio emitting anomalous X-ray pulsars transients}},
	Volume = 516,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200811114}}

@article{ouyed11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.415.1590O},
	Archiveprefix = {arXiv},
	Author = {{Ouyed}, R. and {Leahy}, D. and {Niebergal}, B.},
	Doi = {10.1111/j.1365-2966.2011.18804.x},
	Eprint = {1012.4510},
	Journal = {\mnras},
	Keywords = {stars: neutron, stars: magnetic fields},
	Month = aug,
	Pages = {1590-1596},
	Primaryclass = {astro-ph.HE},
	Title = {{SGR 0418+5729 as an evolved Quark-Nova compact remnant}},
	Volume = 415,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.18804.x}}

@article{overbeck65,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1965ApJ...141..864O},
	Author = {{Overbeck}, J.~W.},
	Doi = {10.1086/148180},
	Journal = {\apj},
	Month = apr,
	Pages = {864},
	Title = {{Small-Angle Scattering of Celestial X-Rays by Interstellar Grains.}},
	Volume = 141,
	Year = 1965,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/148180}}

@article{ozel01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...563..255O},
	Author = {{{\"O}zel}, F. and {Psaltis}, D. and {Kaspi}, V.~M.},
	Doi = {10.1086/323777},
	Eprint = {arXiv:astro-ph/0105372},
	Journal = {\apj},
	Month = dec,
	Pages = {255-266},
	Title = {{Constraints on Thermal Emission Models of Anomalous X-Ray Pulsars}},
	Volume = 563,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323777}}

@article{ozel07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...659L.141O},
	Author = {{{\"O}zel}, F. and {G{\"u}ver}, T.},
	Doi = {10.1086/517933},
	Eprint = {arXiv:astro-ph/0612561},
	Journal = {\apjl},
	Keywords = {Stars: Neutron, X-Rays: Stars},
	Month = apr,
	Pages = {L141-L144},
	Title = {{Hardness-Intensity Correlations in Magnetar Afterglows}},
	Volume = 659,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/517933}}

@article{ozel10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725.1918O},
	Archiveprefix = {arXiv},
	Author = {{{\"O}zel}, F. and {Psaltis}, D. and {Narayan}, R. and {McClintock}, J.~E.},
	Doi = {10.1088/0004-637X/725/2/1918},
	Eprint = {1006.2834},
	Journal = {\apj},
	Keywords = {black hole physics, X-rays: binaries},
	Month = dec,
	Pages = {1918-1927},
	Primaryclass = {astro-ph.GA},
	Title = {{The Black Hole Mass Distribution in the Galaxy}},
	Volume = 725,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/725/2/1918}}

@ARTICLE{ozel13,
   author = {{{\"O}zel}, F.},
    title = "{Surface emission from neutron stars and implications for the physics of their interiors}",
  journal = {Reports on Progress in Physics},
archivePrefix = "arXiv",
   eprint = {1210.0916},
 primaryClass = "astro-ph.HE",
     year = 2013,
    month = jan,
   volume = 76,
   number = 1,
      eid = {016901},
    pages = {016901},
      doi = {10.1088/0034-4885/76/1/016901},
   adsurl = {http://adsabs.harvard.edu/abs/2013RPPh...76a6901O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pacini67,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1967Natur.216..567P},
	Author = {{Pacini}, F.},
	Doi = {10.1038/216567a0},
	Journal = {\nat},
	Month = nov,
	Pages = {567-568},
	Title = {{Energy Emission from a Neutron Star}},
	Volume = 216,
	Year = 1967,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/216567a0}}

@article{paczynski71,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1971ARA%26A...9..183P},
	Author = {{Paczy{\'n}ski}, B.},
	Doi = {10.1146/annurev.aa.09.090171.001151},
	Journal = {\araa},
	Pages = {183},
	Title = {{Evolutionary Processes in Close Binary Systems}},
	Volume = 9,
	Year = 1971,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.09.090171.001151}}

@article{paczynski92,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1992AcA....42..145P&amp;db_key=AST},
	Author = {{Paczynski}, B.},
	Journal = {Acta Astronomica},
	Pages = {145-153},
	Title = {{GB 790305 as a very strongly magnetized neutron star}},
	Volume = 42,
	Year = 1992}

@article{pagani11,
	Author = {{Pagani}, C. and {Beardmore}, A.~P. and {Kennea}, J.~A.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Pulsars, Soft Gamma-ray Repeaters},
	Month = jul,
	Title = {{Swift J1822.3-1606: Enhanced Swift-XRT position}},
	Volume = 3493,
	Year = 2011}

@ARTICLE{page09,
   author = {{Page}, D. and {Lattimer}, J.~M. and {Prakash}, M. and {Steiner}, A.~W.
	},
    title = "{Neutrino Emission from Cooper Pairs and Minimal Cooling of Neutron Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0906.1621},
 primaryClass = "astro-ph.SR",
 keywords = {dense matter, equation of state, neutrinos, stars: neutron},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {1131-1140},
      doi = {10.1088/0004-637X/707/2/1131},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707.1131P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{page12,
       author = {{Page}, M.~J. and {Brindle}, C. and {Talavera}, A. and {Still}, M. and
         {Rosen}, S.~R. and {Yershov}, V.~N. and {Ziaeepour}, H. and
         {Mason}, K.~O. and {Cropper}, M.~S. and {Breeveld}, A.~A. and
         {Loiseau}, N. and {Mignani}, R. and {Smith}, A. and {Murdin}, P.},
        title = "{The XMM-Newton serendipitous ultraviolet source survey catalogue}",
      journal = {\mnras},
     keywords = {catalogues, astrometry, stars: general, galaxies: photometry, ultraviolet: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Oct",
       volume = {426},
       number = {2},
        pages = {903-926},
          doi = {10.1111/j.1365-2966.2012.21706.x},
archivePrefix = {arXiv},
       eprint = {1207.5182},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.426..903P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{paizis14,
   author = {{Paizis}, A. and {Sidoli}, L.},
    title = "{Cumulative luminosity distributions of supergiant fast X-ray transients in hard X-rays}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1401.6861},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, stars: neutron, X-rays: binaries, X-rays: individual: IGR J17544-2619, X-rays: individual: SAX J1818.6-1703, X-rays: individual: XTE J1739-302},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {3439-3452},
      doi = {10.1093/mnras/stu191},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.3439P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{pakull02,
   author = {{Pakull}, M.~W. and {Mirioni}, L.},
    title = "{Optical Counterparts of Ultraluminous X-Ray Sources}",
    booktitle = {New Visions of the X-ray Universe in the XMM-Newton and Chandra Era, 26-30 November 2001, ESTEC,
The Netherlands},
  series = {ArXiv Astrophysics e-prints: astro-ph/0202488},
 keywords = {Astrophysics},
     year = 2002,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2002astro.ph..2488P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{pakull03,
   author = {{Pakull}, M.~W. and {Mirioni}, L.},
    title = "{Bubble Nebulae around Ultraluminous X-Ray Sources}",
 keywords = {H II regions, ISM: Jets and outflows, Stars: Mass loss, X-rays: binaries},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2003,
   series = {Revista Mexicana de Astronomia y Astrofisica, vol.~27},
   volume = 15,
   editor = {{Arthur}, J. and {Henney}, W.~J.},
    month = jan,
    pages = {197-199},
   adsurl = {http://adsabs.harvard.edu/abs/2003RMxAC..15..197P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{pakull08,
   author = {{Pakull}, M.~W. and {Gris{\'e}}, F.},
    title = "{Ultraluminous X-ray Sources: Beambags and Optical Counterparts}",
 keywords = {X-ray sources, X-ray bursts, Interstellar medium  and nebulae in external galaxies, Intracluster matter, cooling flows},
booktitle = {A Population Explosion: The Nature \& Evolution of X-ray Binaries in Diverse Environments},
     year = 2008,
   series = {American Institute of Physics Conference Series},
   volume = 1010,
   editor = {{Bandyopadhyay}, R.~M. and {Wachter}, S. and {Gelino}, D. and 
	{Gelino}, C.~R.},
    month = may,
    pages = {303-307},
      doi = {10.1063/1.2945062},
   adsurl = {http://adsabs.harvard.edu/abs/2008AIPC.1010..303P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pakull10,
   author = {{Pakull}, M.~W. and {Soria}, R. and {Motch}, C.},
    title = "{A 300-parsec-long jet-inflated bubble around a powerful microquasar in the galaxy NGC 7793}",
  journal = {\nat},
     year = 2010,
    month = jul,
   volume = 466,
    pages = {209-212},
      doi = {10.1038/nature09168},
   adsurl = {http://adsabs.harvard.edu/abs/2010Natur.466..209P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{palmer02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002MmSAI..73..578P&db_key=AST},
	Author = {{Palmer}, D.~M.},
	Journal = {Memorie della Societa Astronomica Italiana},
	Pages = {578-583},
	Title = {{Rapid spindown of SGR 1900+14 following its superburst.}},
	Volume = 73,
	Year = 2002}

@article{palmer05_gcn,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005GCN..2945....1P&db_key=AST},
	Author = {{Palmer}, D. and {Barthelmy}, S. and {Barbier}, L. and {Cummings}, J. and {Fenimore}, E. and {Fink}, R. and {Gehrels}, N. and {Hullinger}, D. and {Hunsberger}, S. and {Krimm}, H. and {Markwardt}, C. and {Matteo}, P. and {McLean}, K. and {Nousek}, J. and {Meszaros}, P. and {Parsons}, A. and {Sakamoto}, T. and {Sato}, G. and {Suzuki}, M. and {Tueller}, J.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR1806-20: Swift-BAT observations of two additional bursts.}},
	Volume = 2945,
	Year = 2005}

@article{palmer05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005Natur.434.1107P&db_key=AST},
	Author = {{Palmer}, D.~M. and {Barthelmy}, S. and {Gehrels}, N. and {Kippen}, R.~M. and {Cayton}, T. and {Kouveliotou}, C. and {Eichler}, D. and {Wijers}, R.~A.~M.~J. and {Woods}, P.~M. and {Granot}, J. and {Lyubarsky}, Y.~E. and {Ramirez-Ruiz}, E. and {Barbier}, L. and {Chester}, M. and {Cummings}, J. and {Fenimore}, E.~E. and {Finger}, M.~H. and {Gaensler}, B.~M. and {Hullinger}, D. and {Krimm}, H. and {Markwardt}, C.~B. and {Nousek}, J.~A. and {Parsons}, A. and {Patel}, S. and {Sakamoto}, T. and {Sato}, G. and {Suzuki}, M. and {Tueller}, J.},
	Doi = {10.1038/nature03525},
	Journal = {\nat},
	Month = apr,
	Pages = {1107-1109},
	Title = {{A giant {$\gamma$}-ray flare from the magnetar SGR 1806 - 20}},
	Volume = 434,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03525}}

@article{palmer06,
	Author = {{Palmer}, D. and {Sakamoto}, T. and {Barthelmy}, S. and {Cummings}, J. and {Gehrels}, N. and {Krimm}, H. and {Markwardt}, C. and {Tueller}, J.},
	Journal = {Astron.~Tel.~789},
	Title = {{SGR 1900+14: BAT observations}},
	Year = 2006}

@article{palmer08,
	Author = {{Palmer}, D. and {Esposito}, P. and {Barthelmy}, S. and {Cummings}, J.~R. and {Gehrels}, N. and {Israel}, G.~L. and {Krimm}, H. and {Sakamoto}, T. and {Starling}, R.},
	Journal = {GCN Circ.},
	Title = {{Reactivation of SGR 1627-41}},
	Volume = 7777,
	Year = 2008}

@article{palmer10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010GCN.10537....1P},
	Author = {{Palmer}, D. and {Gelbord}, J.~M.},
	Journal = {GCN Circ.},
	Title = {{SGR 1833-0832 is pulsed at 7.56 seconds.}},
	Volume = 10537,
	Year = 2010}

@ARTICLE{papitto11,
   author = {{Papitto}, A. and {D'A{\`i}}, A. and {Motta}, S. and {Riggio}, A. and 
	{Burderi}, L. and {di Salvo}, T. and {Belloni}, T. and {Iaria}, R.
	},
    title = "{The spin and orbit of the newly discovered pulsar IGR J17480-2446}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1010.4793},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, stars: rotation, X-rays: binaries, pulsars: individual: IGR J17480-2446},
     year = 2011,
    month = feb,
   volume = 526,
      eid = {L3},
    pages = {L3},
      doi = {10.1051/0004-6361/201015974},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526L...3P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{papitto12,
   author = {{Papitto}, A. and {Di Salvo}, T. and {Burderi}, L. and {Belloni}, T.~M. and 
	{Stella}, L. and {Bozzo}, E. and {D'A{\`i}}, A. and {Ferrigno}, C. and 
	{Iaria}, R. and {Motta}, S. and {Riggio}, A. and {Tramacere}, A.
	},
    title = "{The pulse profile and spin evolution of the accreting pulsar in Terzan 5, IGR J17480-2446, during its 2010 outburst}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.4096},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, stars: neutron, pulsars: individual: IGR J17480-2446, X-rays: binaries},
     year = 2012,
    month = jun,
   volume = 423,
    pages = {1178-1193},
      doi = {10.1111/j.1365-2966.2012.20945.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423.1178P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{paredes86,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...154L..30P&db_key=AST},
	Author = {{Paredes}, J.~M. and {Figueras}, F.},
	Journal = {\aap},
	Month = jan,
	Pages = {L30-L32},
	Title = {{Detection of optical variability of LSI + 61 deg 303}},
	Volume = 154,
	Year = 1986}

@article{paredes94,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...288..519P},
	Author = {{Paredes}, J.~M. and {Marziani}, P. and {Marti}, J. and {Fabregat}, J. and {Coe}, M.~J. and {Everall}, C. and {Figueras}, F. and {Jordi}, C. and {Norton}, A.~J. and {Prince}, T. and {Reglero}, V. and {Roche}, P. and {Torra}, J. and {Unger}, S.~J. and {Zamanov}, R.},
	Eprint = {arXiv:astro-ph/9402016},
	Journal = {\aap},
	Month = aug,
	Pages = {519-528},
	Title = {{Photometric and H{$\alpha$} observations of LSI+61 303: detection of a \~{}26 day V and JHK band modulation}},
	Volume = 288,
	Year = 1994}

@article{paredes97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...320L..25P},
	Author = {{Paredes}, J.~M. and {Marti}, J. and {Peracaula}, M. and {Ribo}, M.},
	Journal = {\aap},
	Month = apr,
	Pages = {L25-L28},
	Title = {{Evidence of X-ray periodicity in LSI+61 303.}},
	Volume = 320,
	Year = 1997}

@article{paredes00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000Sci...288.2340P&db_key=AST},
	Author = {{Paredes}, J.~M. and {Mart{\'{\i}}}, J. and {Rib{\'o}}, M. and {Massi}, M.},
	Doi = {10.1126/science.288.5475.2340},
	Eprint = {astro-ph/0102235},
	Journal = {Science},
	Month = jun,
	Pages = {2340-2342},
	Title = {{Discovery of a High-Energy Gamma-Ray-Emitting Persistent Microquasar}},
	Volume = 288,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.288.5475.2340}}

@article{paredes06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2006A%26A...451..259P&db_key=AST},
	Author = {{Paredes}, J.~M. and {Bosch-Ramon}, V. and {Romero}, G.~E.},
	Doi = {10.1051/0004-6361:20054155},
	Eprint = {astro-ph/0509095},
	Journal = {\aap},
	Month = may,
	Pages = {259-266},
	Title = {{Spectral energy distribution of the {$\gamma$}-ray microquasar LS 5039}},
	Volume = 451,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054155}}

@article{paredes07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...664L..39P},
	Author = {{Paredes}, J.~M. and {Rib{\'o}}, M. and {Bosch-Ramon}, V. and {West}, J.~R. and {Butt}, Y.~M. and {Torres}, D.~F. and {Mart{\'{\i}}}, J.},
	Doi = {10.1086/520674},
	Eprint = {arXiv:0706.0877},
	Journal = {\apjl},
	Month = jul,
	Pages = {L39-L42},
	Title = {{Chandra Observations of the Gamma-Ray Binary LS I +61 303: Extended X-Ray Structure?}},
	Volume = 664,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/520674}}

@article{park03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586..210P},
	Author = {{Park}, S. and {Burrows}, D.~N. and {Garmire}, G.~P. and {Nousek}, J.~A. and {Hughes}, J.~P. and {Williams}, R.~M.},
	Doi = {10.1086/367619},
	Eprint = {arXiv:astro-ph/0211552},
	Journal = {\apj},
	Keywords = {ISM: Individual: Alphanumeric: N49, Stars: Neutron, ISM: Supernova Remnants, X-Rays: Individual: Alphanumeric: SGR 0526-66, X-Rays: ISM, X-Rays: Stars},
	Month = mar,
	Pages = {210-223},
	Title = {{X-Ray Emission from Multiphase Shock in the Large Magellanic Cloud Supernova Remnant N49}},
	Volume = 586,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/367619}}

@ARTICLE{park04,
   author = {{Park}, S. and {Zhekov}, S.~A. and {Burrows}, D.~N. and {Garmire}, G.~P. and 
	{McCray}, R.},
    title = "{A Chandra View of the Morphological and Spectral Evolution of Supernova Remnant 1987A}",
  journal = {\apj},
   eprint = {astro-ph/0404145},
 keywords = {ISM: Supernova Remnants, Stars: Supernovae: General, Stars: Supernovae: Individual: Alphanumeric: SN 1987A, X-Rays: General, X-Rays: Stars},
     year = 2004,
    month = jul,
   volume = 610,
    pages = {275-284},
      doi = {10.1086/421701},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..275P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pmm04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..378P},
	Author = {{Park}, S.~Q. and {Miller}, J.~M. and {McClintock}, J.~E. and {Remillard}, R.~A. and {Orosz}, J.~A. and {Shrader}, C.~R. and {Hunstead}, R.~W. and {Campbell-Wilson}, D. and {Ishwara-Chandra}, C.~H. and {Rao}, A.~P. and {Rupen}, M.~P.},
	Doi = {10.1086/421511},
	Eprint = {arXiv:astro-ph/0308363},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Black Hole Physics, Stars: Individual: Constellation Name: IL Lupi, Stars: Individual: Alphanumeric: 4U 1543-47, X-Rays: Stars},
	Month = jul,
	Pages = {378-389},
	Title = {{Spectral and Timing Evolution of the Black Hole X-Ray Nova 4U 1543-47 during Its 2002 Outburst}},
	Volume = 610,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/421511}}

@ARTICLE{park05,
   author = {{Park}, S. and {Zhekov}, S.~A. and {Burrows}, D.~N. and {Garmire}, G.~P. and 
	{McCray}, D.},
    title = "{Supernova remnant 1987A: The latest report from the Chandra X-ray Observatory}",
  journal = {Advances in Space Research},
   eprint = {astro-ph/0501561},
     year = 2005,
   volume = 35,
    pages = {991-995},
      doi = {10.1016/j.asr.2005.01.075},
   adsurl = {http://adsabs.harvard.edu/abs/2005AdSpR..35..991P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{park06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...653L..37P},
	Author = {{Park}, S. and {Mori}, K. and {Kargaltsev}, O. and {Slane}, P.~O. and {Hughes}, J.~P. and {Burrows}, D.~N. and {Garmire}, G.~P. and {Pavlov}, G.~G.},
	Doi = {10.1086/510366},
	Eprint = {arXiv:astro-ph/0610004},
	Journal = {\apjl},
	Month = dec,
	Pages = {L37-L40},
	Title = {{Discovery of a Candidate Central Compact Object in the Galactic Nonthermal SNR G330.2+1.0}},
	Volume = 653,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/510366}}

@article{parker05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439..213P},
	Author = {{Parker}, T.~L. and {Norton}, A.~J. and {Mukai}, K.},
	Doi = {10.1051/0004-6361:20052887},
	Eprint = {astro-ph/0503658},
	Journal = {\aap},
	Keywords = {stars: novae, cataclysmic variables, X-rays: stars, stars: magnetic, fields, stars: binaries: close},
	Month = aug,
	Pages = {213-225},
	Title = {{X-ray orbital modulations in intermediate polars}},
	Volume = 439,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052887}}

@article{parmar86,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...308..199P},
	Author = {{Parmar}, A.~N. and {White}, N.~E. and {Giommi}, P. and {Gottwald}, M.},
	Doi = {10.1086/164490},
	Journal = {\apj},
	Keywords = {ECLIPSING BINARY STARS, PERIODIC VARIATIONS, X RAY BINARIES, ABUNDANCE, ACCRETION DISKS, COMPANION STARS, INTERSTELLAR MATTER, METALLICITY},
	Month = sep,
	Pages = {199-212},
	Title = {{The discovery of 3.8 hour periodic intensity dips and eclipses from the transient low-mass X-ray binary EXO 0748-676}},
	Volume = 308,
	Year = 1986,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/164490}}

@article{parmar89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...338..359P},
	Author = {{Parmar}, A.~N. and {White}, N.~E. and {Stella}, L. and {Izzo}, C. and {Ferri}, P.},
	Doi = {10.1086/167204},
	Journal = {\apj},
	Keywords = {EARLY STARS, PULSARS, STELLAR LUMINOSITY, X RAY BINARIES, CHARGE COUPLED DEVICES, EXOSAT SATELLITE, LIGHT CURVE, STELLAR FLARES, STELLAR MASS ACCRETION},
	Month = mar,
	Pages = {359-372},
	Title = {{The transient 42 second X-ray pulsar EXO 2030+375. I - The discovery and the luminosity dependence of the pulse period variations}},
	Volume = 338,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/167204}}

@article{parmar97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26AS..122..309P&db_key=AST},
	Author = {{Parmar}, A.~N. and {Martin}, D.~D.~E. and {Bavdaz}, M. and {Favata}, F. and {Kuulkers}, E. and {Vacanti}, G. and {Lammers}, U. and {Peacock}, A. and {Taylor}, B.~G.},
	Journal = {\aaps},
	Month = apr,
	Pages = {309-326},
	Title = {{The low-energy concentrator spectrometer on-board the BeppoSAX X-ray astronomy satellite}},
	Volume = 122,
	Year = 1997}

@article{parmar98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998A%26A...330..175P&db_key=AST},
	Author = {{Parmar}, A.~N. and {Oosterbroek}, T. and {Favata}, F. and {Pightling}, S. and {Coe}, M.~J. and {Mereghetti}, S. and {Israel}, G.~L.},
	Journal = {\aap},
	Month = feb,
	Pages = {175-180},
	Title = {{A BeppoSAX observation of the X-ray pulsar 1E2259+586 and the supernova remnant (CTB109)}},
	Volume = 330,
	Year = 1998}

@article{patel04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...602L..45P&db_key=AST},
	Author = {{Patel}, S.~K. and {Kouveliotou}, C. and {Tennant}, A. and {Woods}, P.~M. and {King}, A. and {Finger}, M.~H. and {Ubertini}, P. and {Winkler}, C. and {Courvoisier}, T.~J.-L. and {van der Klis}, M. and {Wachter}, S. and {Gaensler}, B.~M. and {Phillips}, C.~J.},
	Journal = {\apjl},
	Month = feb,
	Pages = {L45-L48},
	Title = {{The Peculiar X-Ray Transient IGR J16358-4726}},
	Volume = 602,
	Year = 2004}

@article{pz08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..543P},
	Archiveprefix = {arXiv},
	Author = {{Patruno}, A. and {Zampieri}, L.},
	Doi = {10.1111/j.1365-2966.2008.13063.x},
	Eprint = {0710.2815},
	Journal = {\mnras},
	Keywords = {galaxies: individual: M81 , galaxies: individual: NGC1313 , galaxies: individual: NGC4559 , galaxies: individual: Holmberg II , X-rays: binaries , X-rays: galaxies},
	Month = may,
	Pages = {543-552},
	Title = {{Optical emission from massive donors in ultraluminous X-ray source binary systems}},
	Volume = 386,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13063.x}}

@article{pz10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403L..69P},
	Archiveprefix = {arXiv},
	Author = {{Patruno}, A. and {Zampieri}, L.},
	Doi = {10.1111/j.1745-3933.2010.00817.x},
	Eprint = {1001.3315},
	Journal = {\mnras},
	Keywords = {galaxies: X-rays: binaries, X-rays: galaxies},
	Month = mar,
	Pages = {L69-L73},
	Primaryclass = {astro-ph.HE},
	Title = {{The black hole in NGC 1313 X-2: constraints on the mass from optical observations}},
	Volume = 403,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2010.00817.x}}

@ARTICLE{patruno12,
   author = {{Patruno}, A. and {Alpar}, M.~A. and {van der Klis}, M. and 
	{van den Heuvel}, E.~P.~J.},
    title = "{The Peculiar Evolutionary History of IGR J17480-2446 in Terzan 5}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.5315},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, X-rays: binaries, X-rays: stars},
     year = 2012,
    month = jun,
   volume = 752,
      eid = {33},
    pages = {33},
      doi = {10.1088/0004-637X/752/1/33},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...752...33P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{patterson94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994PASP..106..209P},
	Author = {{Patterson}, J.},
	Doi = {10.1086/133375},
	Journal = {\pasp},
	Keywords = {Cataclysmic Variables, Cosmic X Rays, Pulsars, Stellar Mass Accretion, White Dwarf Stars, Circular Polarization, Magnetic Moments, Synchronism},
	Month = mar,
	Pages = {209-238},
	Title = {{The DQ Herculis stars}},
	Volume = 106,
	Year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/133375}}

@article{pavlov01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...552L.129P&db_key=AST},
	Author = {{Pavlov}, G.~G. and {Zavlin}, V.~E. and {Sanwal}, D. and {Burwitz}, V. and {Garmire}, G.~P.},
	Doi = {10.1086/320342},
	Eprint = {astro-ph/0103171},
	Journal = {\apjl},
	Month = may,
	Pages = {L129-L133},
	Title = {{The X-Ray Spectrum of the Vela Pulsar Resolved with the Chandra X-Ray Observatory}},
	Volume = 552,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320342}}

@article{pavlov01vjr,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...559L.131P},
	Author = {{Pavlov}, G.~G. and {Sanwal}, D. and {K{\i}z{\i}ltan}, B. and {Garmire}, G.~P.},
	Doi = {10.1086/323975},
	Journal = {\apjl},
	Keywords = {ISM: Individual: Alphanumeric: RX J0852.0-4622, Stars: Neutron, X-Rays: Individual: Alphanumeric: CXOU J085201.4-461753},
	Month = oct,
	Pages = {L131-L134},
	Title = {{The Compact Central Object in the RX J0852.0-4622 Supernova Remnant}},
	Volume = 559,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323975}}

@inproceedings{pavlov02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ASPC..271..247P&db_key=AST},
	Author = {{Pavlov}, G.~G. and {Sanwal}, D. and {Garmire}, G.~P. and {Zavlin}, V.~E.},
	Booktitle = {Astronomical Society of the Pacific Conference Series,},
	Pages = {247},
	Title = {{The Puzzling Compact Objects in Supernova Remnants}},
	Year = 2002}

@inproceedings{pavlov04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004IAUS..218..239P},
	Author = {{Pavlov}, G.~G. and {Sanwal}, D. and {Teter}, M.~A.},
	Booktitle = {Young Neutron Stars and Their Environments},
	Editor = {{Camilo}, F. and {Gaensler}, B.~M.},
	Pages = {239},
	Series = {IAU Symposium},
	Title = {{Central Compact Objects in Supernova Remnants}},
	Volume = 218,
	Year = 2004}

@article{peacock83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983MNRAS.202..615P},
	Author = {{Peacock}, J.~A.},
	Journal = {\mnras},
	Keywords = {ASTRONOMY, GOODNESS OF FIT, STATISTICAL DISTRIBUTIONS, MONTE CARLO METHOD, POWER SPECTRA, PROBABILITY DISTRIBUTION FUNCTIONS, QUASARS, SAMPLING, SIGNIFICANCE, VIRGO GALACTIC CLUSTER},
	Month = feb,
	Pages = {615-627},
	Title = {{Two-dimensional goodness-of-fit testing in astronomy}},
	Volume = 202,
	Year = 1983}

@ARTICLE{peacock12,
       author = {{Peacock}, Mark B. and {Zepf}, Stephen E. and {Kundu}, Arunav and
         {Maccarone}, Thomas J. and {Rhode}, Katherine L. and {Salzer}, John J. and
         {Waters}, Christopher Z. and {Ciardullo}, Robin and {Gronwall}, Caryl and
         {Stern}, Daniel},
        title = "{Spatially Resolved Spectroscopy of the Globular Cluster RZ 2109 and the Nature of its Black Hole}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 4472, galaxies: star clusters: general, galaxies: star clusters: individual: RZ 2109, globular clusters: general, X-rays: binaries, X-rays: galaxies: clusters, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = nov,
       volume = {759},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.1088/0004-637X/759/2/126},
archivePrefix = {arXiv},
       eprint = {1209.6253},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...759..126P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pellizzoni02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...393L..65P},
	Author = {{Pellizzoni}, A. and {Mereghetti}, S. and {De Luca}, A.},
	Doi = {10.1051/0004-6361:20021036},
	Eprint = {arXiv:astro-ph/0208393},
	Journal = {\aap},
	Keywords = {stars: individual: AX J0851.9-4617.4, stars: neutron, HII regions},
	Month = oct,
	Pages = {L65-L68},
	Title = {{An H{$\alpha$} nebula possibly associated with the central X-ray source in the G 266.2-1.2 supernova remnant}},
	Volume = 393,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20021036}}

@article{pellizzoni04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...612L..49P},
	Author = {{Pellizzoni}, A. and {De Luca}, A. and {Mereghetti}, S. and {Tiengo}, A. and {Mattana}, F. and {Caraveo}, P. and {Tavani}, M. and {Bignami}, G.~F.},
	Doi = {10.1086/424038},
	Eprint = {arXiv:astro-ph/0407312},
	Journal = {\apjl},
	Month = sep,
	Pages = {L49-L52},
	Title = {{A First XMM-Newton Look at the Relativistic Double Pulsar PSR J0737-3039}},
	Volume = 612,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/424038}}

@article{pellizzoni04agile,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004AdSpR..33..625P&db_key=AST},
	Author = {{Pellizzoni}, A. and {Chen}, A. and {Conti}, M. and {Giuliani}, A. and {Mereghetti}, S. and {Tavani}, M. and {Vercellone}, S.},
	Doi = {10.1016/j.asr.2003.07.029},
	Journal = {Advances in Space Research},
	Pages = {625-629},
	Title = {{Prospects for high energy studies of pulsars with the AGILE {$\gamma$}-ray telescope}},
	Volume = 33,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.asr.2003.07.029}}

@article{pellizzoni08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...679..664P},
	Author = {{Pellizzoni}, A. and {Tiengo}, A. and {De Luca}, A. and {Esposito}, P. and {Mereghetti}, S.},
	Doi = {10.1086/587053},
	Eprint = {arXiv:0802.0350},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: PSR J0737-3039A, Stars: Pulsars: Individual: Alphanumeric: PSR J0737-3039B, Stars: Neutron, X-Rays: Stars},
	Month = may,
	Pages = {664-674},
	Title = {{PSR J0737-3039: Interacting Pulsars in X-Rays}},
	Volume = 679,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587053}}

@ARTICLE{pena12,
       author = {{Pe{\~n}a}, M. and {Reyes-P{\'e}rez}, J. and
         {Hern{\'a}ndez-Mart{\'\i}nez}, L. and {P{\'e}rez-Guill{\'e}n}, M.},
        title = "{A catalog of planetary nebula candidates in the Sculptor spiral galaxy NGC 300}",
      journal = {\aap},
     keywords = {galaxies: individual: NGC 300, planetary nebulae: general, HII regions, galaxies: distances and redshifts, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Nov",
       volume = {547},
          eid = {A78},
        pages = {A78},
          doi = {10.1051/0004-6361/201219490},
archivePrefix = {arXiv},
       eprint = {1208.5541},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...547A..78P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pennucci15,
   author = {{Pennucci}, T.~T. and {Possenti}, A. and {Esposito}, P. and 
	{Rea}, N. and {Haggard}, D. and {Baganoff}, F.~K. and {Burgay}, M. and 
	{Coti Zelati}, F. and {Israel}, G.~L. and {Minter}, A.},
    title = "{Simultaneous Multi-band Radio and X-Ray Observations of the Galactic Center Magnetar SGR 1745-2900}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1505.00836},
 primaryClass = "astro-ph.HE",
 keywords = {Galaxy: center, pulsars: individual: PSR J1745{\ndash}2900, SGR 1745{\ndash}2900, stars: magnetars},
     year = 2015,
    month = jul,
   volume = 808,
      eid = {81},
    pages = {81},
      doi = {10.1088/0004-637X/808/1/81},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...808...81P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{perego15,
   author = {{Perego}, A. and {Hempel}, M. and {Fr{\"o}hlich}, C. and {Ebinger}, K. and 
	{Eichler}, M. and {Casanova}, J. and {Liebend{\"o}rfer}, M. and 
	{Thielemann}, F.-K.},
    title = "{PUSHing Core-collapse Supernovae to Explosions in Spherical Symmetry I: the Model and the Case of SN 1987A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.02845},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, stars: neutron, supernovae: general, supernovae: individual: SN 1987},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {275},
    pages = {275},
      doi = {10.1088/0004-637X/806/2/275},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806..275P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{perna01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...557...18P},
	Author = {{Perna}, R. and {Heyl}, J.~S. and {Hernquist}, L.~E. and {Juett}, A.~M. and {Chakrabarty}, D.},
	Doi = {10.1086/321569},
	Eprint = {arXiv:astro-ph/0103273},
	Journal = {\apj},
	Month = aug,
	Pages = {18-23},
	Title = {{Anomalous X-Ray Pulsars and Soft Gamma-Ray Repeaters: Spectral Fits and the Magnetar Model}},
	Volume = 557,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321569}}

@article{perna06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...639..363P},
	Author = {{Perna}, R. and {Bozzo}, E. and {Stella}, L.},
	Doi = {10.1086/499227},
	Eprint = {arXiv:astro-ph/0511285},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Magnetic Fields, Stars: Neutron, Stars: Pulsars: General},
	Month = mar,
	Pages = {363-376},
	Title = {{On the Spin-up/Spin-down Transitions in Accreting X-Ray Binaries}},
	Volume = 639,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/499227}}

@ARTICLE{perna08,
   author = {{Perna}, R. and {Soria}, R. and {Pooley}, D. and {Stella}, L.
	},
    title = "{How rapidly do neutron stars spin at birth? Constraints from archival X-ray observations of extragalactic supernovae}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0712.1040},
 keywords = {supernova remnants , pulsars: general , X-rays: stars},
     year = 2008,
    month = mar,
   volume = 384,
    pages = {1638-1648},
      doi = {10.1111/j.1365-2966.2007.12821.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.384.1638P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pg08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...681..522P},
	Archiveprefix = {arXiv},
	Author = {{Perna}, R. and {Gotthelf}, E.~V.},
	Doi = {10.1086/588211},
	Eprint = {0803.2042},
	Journal = {\apj},
	Keywords = {pulsars: individual (XTE J1810-197), Stars: Neutron, X-Rays: Stars},
	Month = jul,
	Pages = {522-529},
	Title = {{Constraints on the Emission and Viewing Geometry of the Transient Anomalous X-Ray Pulsar XTE J1810-197}},
	Volume = 681,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588211}}

@article{perna11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...727L..51P},
	Archiveprefix = {arXiv},
	Author = {{Perna}, R. and {Pons}, J.~A.},
	Doi = {10.1088/2041-8205/727/2/L51},
	Eid = {L51},
	Eprint = {1101.1098},
	Journal = {\apjl},
	Keywords = {stars: neutron, X-rays: stars},
	Month = feb,
	Pages = {L51},
	Primaryclass = {astro-ph.HE},
	Title = {{A Unified Model of the Magnetar and Radio Pulsar Bursting Phenomenology}},
	Volume = 727,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/727/2/L51}}

@ARTICLE{perna14,
   author = {{Perna}, R. and {Duffell}, P. and {Cantiello}, M. and {MacFadyen}, A.~I.
	},
    title = "{The Fate of Fallback Matter around Newly Born Compact Objects}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.4981},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, stars: evolution, stars: neutron, supernovae: general},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {119},
    pages = {119},
      doi = {10.1088/0004-637X/781/2/119},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781..119P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{perotti07,
	Author = {{Perotti}, F. and {Giuliani}, A. and {Mereghetti}, S. and {Fiorini}, M. and {Vercellone}, S. and {Chen}, A. and {Pellizzoni}, A. and {Labanti}, C. and {Trifoglio}, M. and {Cocco}, G.~D. and {Tavani}, M. and {Feroci}, M. and {Argan}, A. and {Trois}, A. and {Picozza}, G. and {Longo}, F. and {Barbiellini}, G. and {Giommi}, P. and {Antonelli}, L.~A. and {Pittori}, C. and {Salotti}, L.},
	Journal = {GCN Circ. 6688},
	Title = {{AGILE-ACS position for the SGR 1806-20 July 27 burst}},
	Year = 2007}

@article{peters64,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1964PhRv..136.1224P},
	Author = {{Peters}, P.~C.},
	Doi = {10.1103/PhysRev.136.B1224},
	Journal = {Physical Review},
	Month = nov,
	Pages = {1224-1232},
	Title = {{Gravitational Radiation and the Motion of Two Point Masses}},
	Volume = 136,
	Year = 1964,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRev.136.B1224}}

@ARTICLE{petit08,
   author = {{Petit}, V. and {Wade}, G.~A. and {Drissen}, L. and {Montmerle}, T. and 
	{Alecian}, E.},
    title = "{Discovery of two magnetic massive stars in the Orion Nebula Cluster: a clue to the origin of neutron star magnetic fields?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0803.2691},
 keywords = {stars: early-type, stars: magnetic fields, stars: neutron, pulsars: general},
     year = 2008,
    month = jun,
   volume = 387,
    pages = {L23-L27},
      doi = {10.1111/j.1745-3933.2008.00474.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.387L..23P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{petre96,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1996ApJ...465L..43P},
	Author = {{Petre}, R. and {Becker}, C.~M. and {Winkler}, P.~F.},
	Doi = {10.1086/310141},
	Journal = {\apjl},
	Month = jul,
	Pages = {L43},
	Title = {{A Central Stellar Remnant in Puppis A}},
	Volume = 465,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310141}}

@article{petrov11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2011AJ....142...35P},
	Archiveprefix = {arXiv},
	Author = {{Petrov}, L. and {Kovalev}, Y.~Y. and {Fomalont}, E.~B. and {Gordon}, D.},
	Doi = {10.1088/0004-6256/142/2/35},
	Eid = {35},
	Eprint = {1101.1460},
	Journal = {\aj},
	Keywords = {astrometry, catalogs, surveys},
	Month = aug,
	Pages = {35},
	Primaryclass = {astro-ph.CO},
	Title = {{The Very Long Baseline Array Galactic Plane Survey---VGaPS}},
	Volume = 142,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/142/2/35}}

@article{pfahl02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...574..364P},
	Author = {{Pfahl}, E. and {Rappaport}, S. and {Podsiadlowski}, P. and {Spruit}, H.},
	Doi = {10.1086/340794},
	Eprint = {arXiv:astro-ph/0109521},
	Journal = {\apj},
	Keywords = {Stars: Neutron, Stars: Supernovae: General, X-Rays: Stars},
	Month = jul,
	Pages = {364-376},
	Title = {{A New Class of High-Mass X-Ray Binaries: Implications for Core Collapse and Neutron Star Recoil}},
	Volume = 574,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/340794}}

@article{prp02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...571L..37P},
	Author = {{Pfahl}, E. and {Rappaport}, S. and {Podsiadlowski}, P.},
	Doi = {10.1086/341197},
	Eprint = {arXiv:astro-ph/0203266},
	Journal = {\apjl},
	Keywords = {Stars: Neutron, X-Rays: Stars},
	Month = may,
	Pages = {L37-L40},
	Title = {{On the Population of Wind-accreting Neutron Stars in the Galaxy}},
	Volume = 571,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/341197}}

@inproceedings{pfeffermann87,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1987SPIE..733..519P},
	Author = {{Pfeffermann}, E. and {Briel}, U.~G. and {Hippmann}, H. and {Kettenring}, G. and {Metzner}, G. and {Predehl}, P. and {Reger}, G. and {Stephan}, K.-H. and {Zombeck}, M. and {Chappell}, J. and {Murray}, S.~S.},
	Booktitle = {Soft X-ray optics and technology. Edited by E.-E.~Koch \& G.~Schmahl},
	Pages = {519-532},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{The focal plane instrumentation of the ROSAT Telescope}},
	Volume = 733,
	Year = 1987}

@inproceedings{pfeffermann96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996rftu.proc..267P},
	Author = {{Pfeffermann}, E. and {Aschenbach}, B.},
	Booktitle = {{Zimmermann}, H.~U. and {Tr{\"u}mper}, J. and {Yorke}, H., eds., Roentgenstrahlung from the Universe.},
	Keywords = {Supernova Remnants: Discoveries, Supernova Remnants: X-Ray Images, Supernova Remnants: Morphology, X-Ray Sources: Wolf-Rayet Stars},
	Month = feb,
	Pages = {267},
	Series = {MPE Report, MPI Garching Germany},
	Title = {{ROSAT observation of a new supernova remnant in the constellation Scorpius}},
	Volume = 263,
	Year = 1996}

@ARTICLE{pfuhl15,
   author = {{Pfuhl}, O. and {Gillessen}, S. and {Eisenhauer}, F. and {Genzel}, R. and 
	{Plewa}, P.~M. and {Ott}, T. and {Ballone}, A. and {Schartmann}, M. and 
	{Burkert}, A. and {Fritz}, T.~K. and {Sari}, R. and {Steinberg}, E. and 
	{Madigan}, A.-M.},
    title = "{The Galactic Center Cloud G2 and its Gas Streamer}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1407.4354},
 keywords = {black hole physics, Galaxy: center, ISM: clouds},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {111},
    pages = {111},
      doi = {10.1088/0004-637X/798/2/111},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798..111P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{phifer13,
   author = {{Phifer}, K. and {Do}, T. and {Meyer}, L. and {Ghez}, A.~M. and 
	{Witzel}, G. and {Yelda}, S. and {Boehle}, A. and {Lu}, J.~R. and 
	{Morris}, M.~R. and {Becklin}, E.~E. and {Matthews}, K.},
    title = "{Keck Observations of the Galactic Center Source G2: Gas Cloud or Star?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1304.5280},
 keywords = {accretion, accretion disks, black hole physics, Galaxy: center, Galaxy: kinematics and dynamics, infrared: general },
     year = 2013,
    month = aug,
   volume = 773,
      eid = {L13},
    pages = {L13},
      doi = {10.1088/2041-8205/773/1/L13},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...773L..13P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{phinney92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992RSPTA.341...39P},
	Author = {{Phinney}, E.~S.},
	Doi = {10.1098/rsta.1992.0084},
	Journal = {Royal Society of London Philosophical Transactions Series A},
	Month = oct,
	Pages = {39-75},
	Title = {{Pulsars as Probes of Newtonian Dynamical Systems}},
	Volume = 341,
	Year = 1992,
	Bdsk-Url-1 = {http://dx.doi.org/10.1098/rsta.1992.0084}}

@article{pian02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...392..407P},
	Author = {{Pian}, E. and {Falomo}, R. and {Hartman}, R.~C. and {Maraschi}, L. and {Tavecchio}, F. and {Tornikoski}, M. and {Treves}, A. and {Urry}, C.~M. and {Ballo}, L. and {Mukherjee}, R. and {Scarpa}, R. and {Thompson}, D.~J. and {Pesce}, J.~E.},
	Doi = {10.1051/0004-6361:20020881},
	Eprint = {astro-ph/0207355},
	Journal = {\aap},
	Keywords = {galaxies: active, BL Lacertae objects: individual: PKS 0537-441, ultraviolet: galaxies, X-ray: galaxies, gamma rays: observations},
	Month = sep,
	Pages = {407-415},
	Title = {{Broad-band continuum and line emission of the gamma-ray blazar PKS 0537-441}},
	Volume = 392,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020881}}

@article{pian07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...664..106P},
	Archiveprefix = {arXiv},
	Author = {{Pian}, E. and {Romano}, P. and {Treves}, A. and {Ghisellini}, G. and {Covino}, S. and {Cucchiara}, A. and {Dolcini}, A. and {Tagliaferri}, G. and {Markwardt}, C. and {Campana}, S. and {Chincarini}, G. and {Gehrels}, N. and {Giommi}, P. and {Maraschi}, L. and {Vergani}, S.~D. and {Zerbi}, F.~M. and {Molinari}, E. and {Testa}, V. and {Tosti}, G. and {Vitali}, F. and {Antonelli}, L.~A. and {Conconi}, P. and {Malaspina}, G. and {Nicastro}, L. and {Palazzi}, E. and {Meurs}, E.~J.~A. and {Norci}, L.},
	Doi = {10.1086/518469},
	Eprint = {0704.0958},
	Journal = {\apj},
	Keywords = {Galaxies: BL Lacertae Objects: Individual: Alphanumeric: PKS 0537-441, Galaxies: Active, Gamma Rays: Observations, Radiation Mechanisms: Nonthermal},
	Month = jul,
	Pages = {106-116},
	Title = {{Simultaneous Swift and REM Monitoring of the Blazar PKS 0537-441 in 2005}},
	Volume = 664,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518469}}

@article{pietsch05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...434..483P},
	Author = {{Pietsch}, W. and {Freyberg}, M. and {Haberl}, F.},
	Doi = {10.1051/0004-6361:20041990},
	Eprint = {astro-ph/0410117},
	Journal = {\aap},
	Keywords = {galaxies: individual: <ASTROBJ>M 31</ASTROBJ>, X-rays: galaxies},
	Month = may,
	Pages = {483-496},
	Title = {{An XMM-Newton survey of M 31}},
	Volume = 434,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20041990}}

@article{pilyugin07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669..299P},
	Archiveprefix = {arXiv},
	Author = {{Pilyugin}, L.~S. and {Thuan}, T.~X.},
	Doi = {10.1086/521597},
	Eprint = {0707.2856},
	Journal = {\apj},
	Keywords = {Galaxies: Abundances, ISM: H II Regions, ISM: Abundances},
	Month = nov,
	Pages = {299-314},
	Title = {{The Oxygen Abundance of Nearby Galaxies from Sloan Digital Sky Survey Spectra}},
	Volume = 669,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/521597}}

@ARTICLE{pinto16,
   author = {{Pinto}, C. and {Middleton}, M.~J. and {Fabian}, A.~C.},
    title = "{Resolved atomic lines reveal outflows in two ultraluminous X-ray sources}",
  journal = {\nat},
     year = 2016,
    month = may,
   volume = 533,
    pages = {64-67},
      doi = {10.1038/nature17417},
   adsurl = {http://adsabs.harvard.edu/abs/2016Natur.533...64P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pintore12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.1107P},
	Archiveprefix = {arXiv},
	Author = {{Pintore}, F. and {Zampieri}, L.},
	Doi = {10.1111/j.1365-2966.2011.20072.x},
	Eprint = {1110.6277},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, X-rays: binaries, X-rays: galaxies, X-rays: individual: NGC 1313 X-1, X-rays: individual: NGC 1313 X-2},
	Month = feb,
	Pages = {1107-1114},
	Primaryclass = {astro-ph.HE},
	Title = {{X-ray spectral states and metallicity in the ultraluminous X-ray sources NGC 1313 X-1 and X-2}},
	Volume = 420,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.20072.x}}

@ARTICLE{pintore17,
   author = {{Pintore}, F. and {Mereghetti}, S. and {Tiengo}, A. and {Vianello}, G. and 
	{Costantini}, E. and {Esposito}, P.},
    title = "{The effect of X-ray dust scattering on a bright burst from the magnetar 1E 1547.0-5408}",
  journal = {\mnras},
 keywords = {stars: magnetars, stars: neutron, pulsars: individual: 1E 1547.0 - 5408, infrared: stars, X-rays: stars},
     year = 2017,
    month = may,
   volume = 467,
    pages = {3467-3474},
      doi = {10.1093/mnras/stx368},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.467.3467P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pintore18,
   author = {{Pintore}, F. and {Belfiore}, A. and {Novara}, G. and {Salvaterra}, R. and 
	{Marelli}, M. and {De Luca}, A. and {Rigoselli}, M. and {Israel}, G. and 
	{Rodriguez}, G. and {Mereghetti}, S. and {Wolter}, A. and {Walton}, D.~J. and 
	{Fuerst}, F. and {Ambrosi}, E. and {Zampieri}, L. and {Tiengo}, A. and 
	{Salvaggio}, C.},
    title = "{A new ultraluminous X-ray source in the galaxy NGC 5907}",
  journal = {\mnras},
 keywords = {accretion, accretion discs, X-rays: binaries, X-rays: galaxies, X-rays: individual: NGC 5907 ULX-2},
     year = 2018,
    month = jun,
   volume = 477,
    pages = {L90-L95},
      doi = {10.1093/mnrasl/sly048},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.477L..90P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pizzolato08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...681..530P},
	Archiveprefix = {arXiv},
	Author = {{Pizzolato}, F. and {Colpi}, M. and {De Luca}, A. and {Mereghetti}, S. and {Tiengo}, A.},
	Doi = {10.1086/588084},
	Eprint = {0803.1373},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Stars: Magnetic Fields, Stars: Neutron, Stars: Novae, Cataclysmic Variables, Stars: Supernovae: Individual: Alphanumeric: RCW 103, X-Rays: Binaries},
	Month = jul,
	Pages = {530-542},
	Title = {{1E 161348-5055 in the Supernova Remnant RCW 103: A Magnetar in a Young Low-Mass Binary System?}},
	Volume = 681,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588084}}

@article{pizzolato10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.1116P},
	Author = {{Pizzolato}, F. and {Wolter}, A. and {Trinchieri}, G.},
	Doi = {10.1111/j.1365-2966.2010.16735.x},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, galaxies: individual: Cartwheel, X-rays: binaries, X-rays: galaxies},
	Month = aug,
	Pages = {1116-1124},
	Title = {{Chandra observations of the ULX N10 in the Cartwheel galaxy}},
	Volume = 406,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.16735.x}}

@ARTICLE{plewa17,
   author = {{Plewa}, P.~M. and {Gillessen}, S. and {Pfuhl}, O. and {Eisenhauer}, F. and 
	{Genzel}, R. and {Burkert}, A. and {Dexter}, J. and {Habibi}, M. and 
	{George}, E. and {Ott}, T. and {Waisberg}, I. and {von Fellenberg}, S.
	},
    title = "{The Post-pericenter Evolution of the Galactic Center Source G2}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1704.05351},
 keywords = {black hole physics, Galaxy: center, ISM: clouds},
     year = 2017,
    month = may,
   volume = 840,
      eid = {50},
    pages = {50},
      doi = {10.3847/1538-4357/aa6e00},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...840...50P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{pons07,
	Author = {{Pons}, J.~A. and {Link}, B. and {Miralles}, J.~A. and {Geppert}, U.},
	Journal = {\prl},
	Month = feb,
	Pages = {071101},
	Title = {{Evidence for Heating of Neutron Stars by Magnetic Field Decay}},
	Volume = 98,
	Year = 2007}

@article{pg07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...470..303P},
	Author = {{Pons}, J.~A. and {Geppert}, U.},
	Doi = {10.1051/0004-6361:20077456},
	Eprint = {arXiv:astro-ph/0703267},
	Journal = {\aap},
	Keywords = {stars: neutron, stars: magnetic fields, stars: evolution},
	Month = jul,
	Pages = {303-315},
	Title = {{Magnetic field dissipation in neutron star crusts: from magnetars to isolated neutron stars}},
	Volume = 470,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077456}}

@article{pons09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...496..207P},
	Archiveprefix = {arXiv},
	Author = {{Pons}, J.~A. and {Miralles}, J.~A. and {Geppert}, U.},
	Doi = {10.1051/0004-6361:200811229},
	Eprint = {0812.3018},
	Journal = {\aap},
	Keywords = {stars: neutron, stars: evolution, stars: magnetic fields},
	Month = mar,
	Pages = {207-216},
	Title = {{Magneto-thermal evolution of neutron stars}},
	Volume = 496,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200811229}}

@article{pons11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741..123P},
	Archiveprefix = {arXiv},
	Author = {{Pons}, J.~A. and {Perna}, R.},
	Doi = {10.1088/0004-637X/741/2/123},
	Eid = {123},
	Eprint = {1109.5184},
	Journal = {\apj},
	Keywords = {stars: magnetars, stars: neutron, X-rays: bursts},
	Month = nov,
	Pages = {123},
	Primaryclass = {astro-ph.HE},
	Title = {{Magnetars versus High Magnetic Field Pulsars: A Theoretical Interpretation of the Apparent Dichotomy}},
	Volume = 741,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/741/2/123}}

@article{ponti10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714..732P},
	Archiveprefix = {arXiv},
	Author = {{Ponti}, G. and {Terrier}, R. and {Goldwurm}, A. and {Belanger}, G. and {Trap}, G.},
	Doi = {10.1088/0004-637X/714/1/732},
	Eprint = {1003.2001},
	Journal = {\apj},
	Keywords = {Galaxy: center, ISM: clouds, X-rays: ISM},
	Month = may,
	Pages = {732-747},
	Primaryclass = {astro-ph.HE},
	Title = {{Discovery of a Superluminal Fe K Echo at the Galactic Center: The Glorious Past of Sgr A* Preserved by Molecular Clouds}},
	Volume = 714,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/1/732}}

@incollection{ponti12,
	Author = {{Ponti}, G. and {Morris}, M.~R. and {Terrier}, R. and {Goldwurm}, A.},
	Booktitle = {Cosmic Rays in Star-Forming Environments},
	Editor = {Torres, Diego F. and Reimer, Olaf},
	Isbn = {978-3-642-35409-0},
	Pages = {331-370},
	Publisher = {Springer, Heidelberg},
	Series = {Astrophysics and Space Science Proceedings},
	Title = {Traces of past activity in the Galactic Centre},
	Volume = {34},
	Year = {2013}}

@ARTICLE{ponti15,
   author = {{Ponti}, G. and {De Marco}, B. and {Morris}, M.~R. and {Merloni}, A. and 
	{Mu{\~n}oz-Darias}, T. and {Clavel}, M. and {Haggard}, D. and 
	{Zhang}, S. and {Nandra}, K. and {Gillessen}, S. and {Mori}, K. and 
	{Neilsen}, J. and {Rea}, N. and {Degenaar}, N. and {Terrier}, R. and 
	{Goldwurm}, A.},
    title = "{Fifteen years of XMM-Newton and Chandra monitoring of Sgr A$^{???}$: evidence for a recent increase in the bright flaring rate}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1507.02690},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, black hole physics, methods: data analysis, Galaxy: centre, X-rays: binaries, X-rays: individual: Sgr A$^{???}$},
     year = 2015,
    month = dec,
   volume = 454,
    pages = {1525-1544},
      doi = {10.1093/mnras/stv1537},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.454.1525P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{poole08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383..627P},
	Archiveprefix = {arXiv},
	Author = {{Poole}, T.~S. and {Breeveld}, A.~A. and {Page}, M.~J. and {Landsman}, W. and {Holland}, S.~T. and {Roming}, P. and {Kuin}, N.~P.~M. and {Brown}, P.~J. and {Gronwall}, C. and {Hunsberger}, S. and {Koch}, S. and {Mason}, K.~O. and {Schady}, P. and {vanden Berk}, D. and {Blustin}, A.~J. and {Boyd}, P. and {Broos}, P. and {Carter}, M. and {Chester}, M.~M. and {Cucchiara}, A. and {Hancock}, B. and {Huckle}, H. and {Immler}, S. and {Ivanushkina}, M. and {Kennedy}, T. and {Marshall}, F. and {Morgan}, A. and {Pandey}, S.~B. and {de Pasquale}, M. and {Smith}, P.~J. and {Still}, M.},
	Doi = {10.1111/j.1365-2966.2007.12563.x},
	Eprint = {0708.2259},
	Journal = {\mnras},
	Keywords = {instrumentation: photometers, techniques: photometric, ultraviolet: general},
	Month = jan,
	Pages = {627-645},
	Title = {{Photometric calibration of the Swift ultraviolet/optical telescope}},
	Volume = 383,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.12563.x}}

@article{pooley10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010PNAS..107.7164P},
	Author = {{Pooley}, D.},
	Doi = {10.1073/pnas.0913903107},
	Journal = {Proc. of the National Academy of Science},
	Month = apr,
	Pages = {7164-7167},
	Title = {{Globular cluster x-ray sources}},
	Volume = 107,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1073/pnas.0913903107}}

@article{popham95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...442..337P},
	Author = {{Popham}, R. and {Narayan}, R.},
	Doi = {10.1086/175444},
	Journal = {\apj},
	Keywords = {Accretion Disks, Black Body Radiation, Boundary Layers, Cataclysmic Variables, Luminosity, Mathematical Models, Optical Thickness, White Dwarf Stars, Angular Momentum, Angular Velocity, Energy Distribution, Mass Flow Rate, Opacity, Radiative Transfer},
	Month = mar,
	Pages = {337-357},
	Title = {{Accretion disk boundary layers in cataclysmic variables. 1: Optically thick boundary layers}},
	Volume = 442,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/175444}}

@article{popov12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421L.127P},
	Archiveprefix = {arXiv},
	Author = {{Popov}, S.~B. and {Turolla}, R.},
	Doi = {10.1111/j.1745-3933.2012.01220.x},
	Eprint = {1112.2507},
	Journal = {\mnras},
	Keywords = {stars: neutron, X-rays: binaries},
	Month = mar,
	Pages = {L127-L131},
	Primaryclass = {astro-ph.HE},
	Title = {{Probing the neutron star spin evolution in the young Small Magellanic Cloud Be/X-ray binary SXP 1062}},
	Volume = 421,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1745-3933.2012.01220.x}}

@ARTICLE{popov15,
   author = {{Popov}, S.~B. and {Kaurov}, A.~A. and {Kaminker}, A.~D.},
    title = "{Central Compact Objects in Kes 79 and RCW 103 as `Hidden' Magnetars with Crustal Activity}",
  journal = {\pasa},
 primaryClass = "astro-ph.HE",
 keywords = {stars:individual (Kes 79, RCW 103), stars:magnetars, stars:neutron.},
     year = 2015,
    month = may,
   volume = 32,
      pages = {e018}
}

@article{possenti02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002A%26A...387..993P&db_key=AST},
	Author = {{Possenti}, A. and {Cerutti}, R. and {Colpi}, M. and {Mereghetti}, S.},
	Doi = {10.1051/0004-6361:20020472},
	Eprint = {astro-ph/0109452},
	Journal = {\aap},
	Month = jun,
	Pages = {993-1002},
	Title = {{Re-examining the X-ray versus spin-down luminosity correlation of rotation powered pulsars}},
	Volume = 387,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020472}}

@article{potekhin98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998JPhB...31...49P},
	Author = {{Potekhin}, A.~Y.},
	Doi = {10.1088/0953-4075/31/1/008},
	Eprint = {arXiv:physics/9710046},
	Journal = {Journal of Physics B: Atomic, Molecular and Optical Physics},
	Month = jan,
	Pages = {49-63},
	Title = {{Hydrogen atom moving across a strong magnetic field: analytical approximations}},
	Volume = 31,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0953-4075/31/1/008}}

@article{potekhin10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518A..24P},
	Archiveprefix = {arXiv},
	Author = {{Potekhin}, A.~Y.},
	Doi = {10.1051/0004-6361/201014781},
	Eid = {A24},
	Eprint = {1003.5106},
	Journal = {\aap},
	Keywords = {stars: neutron, stars: atmospheres, opacity, magnetic fields, X-rays: stars},
	Month = jul,
	Pages = {A24},
	Primaryclass = {astro-ph.HE},
	Title = {{Cyclotron harmonics in opacities of isolated neutron star atmospheres}},
	Volume = 518,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201014781}}

@article{poutanen06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.373..836P},
	Author = {{Poutanen}, J. and {Beloborodov}, A.~M.},
	Doi = {10.1111/j.1365-2966.2006.11088.x},
	Eprint = {arXiv:astro-ph/0608663},
	Journal = {\mnras},
	Keywords = {stars: neutron, pulsars: general, X-rays: binaries},
	Month = dec,
	Pages = {836-844},
	Title = {{Pulse profiles of millisecond pulsars and their Fourier amplitudes}},
	Volume = 373,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.11088.x}}

@article{poutanen13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432..506P},
	Archiveprefix = {arXiv},
	Author = {{Poutanen}, J. and {Fabrika}, S. and {Valeev}, A.~F. and {Sholukhova}, O. and {Greiner}, J.},
	Doi = {10.1093/mnras/stt487},
	Eprint = {1210.1210},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, galaxies: individual: NGC 4038, galaxies: individual: NGC4039, galaxies: star clusters: general, X-rays: galaxies},
	Month = jun,
	Pages = {506-519},
	Primaryclass = {astro-ph.HE},
	Title = {{On the association of the ultraluminous X-ray sources in the Antennae galaxies with young stellar clusters}},
	Volume = 432,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stt487}}

@article{predehl95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1995A%26A...293..889P},
	Author = {{Predehl}, P. and {Schmitt}, J.~H.~M.~M.},
	Journal = {\aap},
	Month = jan,
	Pages = {889-905},
	Title = {{X-raying the interstellar medium: ROSAT observations of dust scattering halos.}},
	Volume = 293,
	Year = 1995}

@book{press92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992nrca.book.....P},
	Author = {{Press}, W.~H. and {Teukolsky}, S.~A. and {Vetterling}, W.~T. and {Flannery}, B.~P.},
	Publisher = {Cambridge: University Press, 2nd ed.},
	Title = {{Numerical recipes in C. The art of scientific computing}},
	Year = 1992}

@article{prestwich03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...595..719P},
	Author = {{Prestwich}, A.~H. and {Irwin}, J.~A. and {Kilgard}, R.~E. and {Krauss}, M.~I. and {Zezas}, A. and {Primini}, F. and {Kaaret}, P. and {Boroson}, B.},
	Doi = {10.1086/377366},
	Eprint = {arXiv:astro-ph/0206127},
	Journal = {\apj},
	Keywords = {Galaxies: Spiral, Galaxies: Starburst, Surveys, X-Rays: Galaxies, X-Rays: General},
	Month = oct,
	Pages = {719-726},
	Title = {{Classifying X-Ray Sources in External Galaxies from X-Ray Colors}},
	Volume = 595,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/377366}}

@article{prestwich07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669L..21P},
	Archiveprefix = {arXiv},
	Author = {{Prestwich}, A.~H. and {Kilgard}, R. and {Crowther}, P.~A. and {Carpano}, S. and {Pollock}, A.~M.~T. and {Zezas}, A. and {Saar}, S.~H. and {Roberts}, T.~P. and {Ward}, M.~J.},
	Doi = {10.1086/523755},
	Eprint = {0709.2892},
	Journal = {\apjl},
	Keywords = {Galaxies: Starburst, Stars: Wolf-Rayet, X-Rays: Binaries, X-Rays: Galaxies},
	Month = nov,
	Pages = {L21-L24},
	Title = {{The Orbital Period of the Wolf-Rayet Binary IC 10 X-1: Dynamic Evidence that the Compact Object Is a Black Hole}},
	Volume = 669,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/523755}}

@article{prestwich13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769...92P},
	Archiveprefix = {arXiv},
	Author = {{Prestwich}, A.~H. and {Tsantaki}, M. and {Zezas}, A. and {Jackson}, F. and {Roberts}, T.~P. and {Foltz}, R. and {Linden}, T. and {Kalogera}, V.},
	Doi = {10.1088/0004-637X/769/2/92},
	Eid = {92},
	Eprint = {1302.6203},
	Journal = {\apj},
	Keywords = {stars: formation, X-rays: binaries},
	Month = jun,
	Pages = {92},
	Primaryclass = {astro-ph.HE},
	Title = {{Ultra-luminous X-Ray Sources in the Most Metal Poor Galaxies}},
	Volume = 769,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/769/2/92}}

@article{protassov02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...571..545P&db_key=AST},
	Author = {{Protassov}, R. and {van Dyk}, D.~A. and {Connors}, A. and {Kashyap}, V.~L. and {Siemiginowska}, A.},
	Journal = {\apj},
	Month = may,
	Pages = {545-559},
	Title = {{Statistics, Handle with Care: Detecting Multiple Model Components with the Likelihood Ratio Test}},
	Volume = 571,
	Year = 2002}

@article{ptak06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJS..166..154P},
	Author = {{Ptak}, A. and {Colbert}, E. and {van der Marel}, R.~P. and {Roye}, E. and {Heckman}, T. and {Towne}, B.},
	Doi = {10.1086/505218},
	Eprint = {astro-ph/0605561},
	Journal = {\apjs},
	Keywords = {Catalogs, X-Rays: Binaries, X-Rays: Galaxies},
	Month = sep,
	Pages = {154-187},
	Title = {{Optical Counterparts of Ultraluminous X-Ray Sources Identified from Archival HST WFPC2 Images}},
	Volume = 166,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/505218}}

@article{ramsay00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.311...75R},
	Author = {{Ramsay}, G. and {Cropper}, M. and {Wu}, K. and {Mason}, K.~O. and {Hakala}, P.},
	Doi = {10.1046/j.1365-8711.2000.03065.x},
	Eprint = {arXiv:astro-ph/9908042},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, STARS: INDIVIDUAL: RX J1914+24, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
	Month = jan,
	Pages = {75-84},
	Title = {{Detection of the optical counterpart of the proposed double degenerate polar RX J1914+24}},
	Volume = 311,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03065.x}}

@article{ramsay02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.332L...7R},
	Author = {{Ramsay}, G. and {Hakala}, P. and {Cropper}, M.},
	Doi = {10.1046/j.1365-8711.2002.05471.x},
	Eprint = {arXiv:astro-ph/0203053},
	Journal = {\mnras},
	Keywords = {binaries: general, stars: individual: RX J086+15, stars: neutron, X-rays: binaries},
	Month = may,
	Pages = {L7-L10},
	Title = {{RX J0806+15: the shortest period binary?}},
	Volume = 332,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05471.x}}
	
@ARTICLE{ramsay17,
       author = {{Ramsay}, Gavin and {Schreiber}, Matthias R. and
         {G{\"a}nsicke}, Boris T. and {Wheatley}, Peter J.},
        title = "{Distances of cataclysmic variables and related objects derived from Gaia Data Release 1}",
      journal = {\aap},
     keywords = {stars: dwarf novae, stars: distances, accretion, accretion disks, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Aug",
       volume = {604},
          eid = {A107},
        pages = {A107},
          doi = {10.1051/0004-6361/201730679},
archivePrefix = {arXiv},
       eprint = {1704.00496},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...604A.107R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ranalli03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...399...39R},
	Author = {{Ranalli}, P. and {Comastri}, A. and {Setti}, G.},
	Doi = {10.1051/0004-6361:20021600},
	Eprint = {arXiv:astro-ph/0211304},
	Journal = {\aap},
	Keywords = {X-rays: galaxies, radio continuum: galaxies, galaxies: high-redshift, infrared: galaxies -, galaxies: fundamental parameters, galaxies: starburst},
	Month = feb,
	Pages = {39-50},
	Title = {{The 2-10 keV luminosity as a Star Formation Rate indicator}},
	Volume = 399,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20021600}}

@article{rappaport77,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217L..29R},
	Author = {{Rappaport}, S. and {Markert}, T. and {Li}, F.~K. and {Clark}, G.~W. and {Jernigan}, J.~G. and {McClintock}, J.~E.},
	Doi = {10.1086/182532},
	Journal = {\apjl},
	Keywords = {Pulsars, Sas, X Ray Sources, Astronomical Spectroscopy, Pulse Duration, Spaceborne Astronomy},
	Month = oct,
	Pages = {L29-L33},
	Title = {{Discovery of a 7.68 second X-ray periodicity in 3U 1626-67}},
	Volume = 217,
	Year = 1977,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/182532}}

@INPROCEEDINGS{rappaport81,
   author = {{Rappaport}, S. and {Joss}, P.~C.},
    title = "{Binary X-Ray Pulsars}",
booktitle = {X-ray Astronomy with the Einstein Satellite},
     year = 1981,
   series = {Astrophysics and Space Science Library},
   volume = 87,
   editor = {{Giacconi}, R.},
   publisher = {Springer, Dordrecht},
    month = nov,
    pages = {123},
      doi = {10.1007/978-94-009-8459-2_8},
   adsurl = {http://adsabs.harvard.edu/abs/1981ASSL...87..123R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{rappaport83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...275..713R},
	Author = {{Rappaport}, S. and {Verbunt}, F. and {Joss}, P.~C.},
	Doi = {10.1086/161569},
	Journal = {\apj},
	Keywords = {Binary Stars, Stellar Evolution, Stellar Magnetic Fields, Stellar Systems, Computer Programs, Polytropic Processes, Stellar Mass Ejection, Stellar Models},
	Month = dec,
	Pages = {713-731},
	Title = {{A new technique for calculations of binary stellar evolution, with application to magnetic braking}},
	Volume = 275,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/161569}}

@inproceedings{rasilla08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008SPIE.7014E.107R},
	Author = {{Rasilla}, J.~L. and {L{\'o}pez L{\'o}pez}, R. and {Tejada}, C.},
	Booktitle = {{Ground-based and Airborne Instrumentation for Astronomy II}},
	Doi = {10.1117/12.789093},
	Month = aug,
	Pages = {701438},
	Series = {SPIE Conference Series, Bellingham, WA},
	Title = {{OSIRIS optical integration and tests}},
	Volume = 7014,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.789093}}

@article{rasmussen06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370..453R},
	Author = {{Rasmussen}, J. and {Ponman}, T.~J. and {Mulchaey}, J.~S.},
	Doi = {10.1111/j.1365-2966.2006.10492.x},
	Eprint = {astro-ph/0604549},
	Journal = {\mnras},
	Keywords = {galaxies: evolution , galaxies: individual: NGC 2276 , galaxies: interactions , galaxies: spiral , X-rays: galaxies , X-rays: galaxies: clusters},
	Month = jul,
	Pages = {453-467},
	Title = {{Gas stripping in galaxy groups - the case of the starburst spiral NGC 2276}},
	Volume = 370,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10492.x}}

@article{ratti09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2169....1R},
	Author = {{Ratti}, E. and {Steeghs}, D. and {Jonker}, P.~G.},
	Journal = {Astron. Tel.},
	Keywords = {Optical, Binaries, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters},
	Month = aug,
	Title = {{Optical observations of the field containing SGR 0418+5729}},
	Volume = 2169,
	Year = 2009}

@article{raymond77,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1977ApJS...35..419R},
	Author = {{Raymond}, J.~C. and {Smith}, B.~W.},
	Journal = {\apjs},
	Month = dec,
	Pages = {419-439},
	Title = {{Soft X-ray spectrum of a hot plasma}},
	Volume = 35,
	Year = 1977}

@article{rea03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...586L..65R&db_key=AST},
	Author = {{Rea}, N. and {Israel}, G.~L. and {Stella}, L. and {Oosterbroek}, T. and {Mereghetti}, S. and {Angelini}, L. and {Campana}, S. and {Covino}, S.},
	Doi = {10.1086/374585},
	Journal = {\apjl},
	Month = mar,
	Pages = {L65-L69},
	Title = {{Evidence of a Cyclotron Feature in the Spectrum of the Anomalous X-Ray Pulsar 1RXS J170849-400910}},
	Volume = 586,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/374585}}

@article{rea04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425L...5R},
	Author = {{Rea}, N. and {Testa}, V. and {Israel}, G.~L. and {Mereghetti}, S. and {Perna}, R. and {Stella}, L. and {Tiengo}, A. and {Mangano}, V. and {Oosterbroek}, T. and {Mignani}, R. and {Lo Curto}, G. and {Campana}, S. and {Covino}, S.},
	Doi = {10.1051/0004-6361:200400052},
	Eprint = {arXiv:astro-ph/0408087},
	Journal = {\aap},
	Keywords = {stars: pulsars: individual: XTE J1810-197, stars: neutron, X-rays: stars},
	Month = oct,
	Pages = {L5-L8},
	Title = {{Correlated Infrared and X-ray variability of the transient Anomalous X-ray Pulsar XTE J1810-197}},
	Volume = 425,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200400052}}

@article{rea05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ApJ...627L.133R&db_key=AST},
	Author = {{Rea}, N. and {Tiengo}, A. and {Mereghetti}, S. and {Israel}, G.~L. and {Zane}, S. and {Turolla}, R. and {Stella}, L.},
	Doi = {10.1086/431951},
	Journal = {\apjl},
	Month = jul,
	Pages = {L133-L136},
	Title = {{A First Look with Chandra at SGR 1806-20 after the Giant Flare: Significant Spectral Softening and Rapid Flux Decay}},
	Volume = 627,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/431951}}

@article{roz05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005MNRAS.361..710R},
	Author = {{Rea}, N. and {Oosterbroek}, T. and {Zane}, S. and {Turolla}, R. and {M{\'e}ndez}, M. and {Israel}, G.~L. and {Stella}, L. and {Haberl}, F.},
	Doi = {10.1111/j.1365-2966.2005.09201.x},
	Eprint = {arXiv:astro-ph/0505400},
	Journal = {\mnras},
	Month = aug,
	Pages = {710-718},
	Title = {{Post-glitch variability in the anomalous X-ray pulsar 1RXSJ170849.0-400910}},
	Volume = 361,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09201.x}}

@article{rea05_atel,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005ATel..645....1R&db_key=AST},
	Author = {{Rea}, N. and {Israel}, G. and {Covino}, S. and {Tiengo}, A. and {Nichelli}, E. and {Turolla}, R. and {Zane}, S. and {Mereghetti}, S. and {Esposito}, P. and {Stella}, L.},
	Journal = {Astron. Tel. 645},
	Month = oct,
	Title = {{SGR 1806-20: X-ray and IR post-Giant Flare monitoring}},
	Year = 2005}

@article{rea07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...661L..65R},
	Author = {{Rea}, N. and {Turolla}, R. and {Zane}, S. and {Tramacere}, A. and {Stella}, L. and {Israel}, G.~L. and {Campana}, R.},
	Doi = {10.1086/518434},
	Eprint = {arXiv:astro-ph/0703128},
	Journal = {\apjl},
	Month = may,
	Pages = {L65-L68},
	Title = {{Spectral Modeling of the High-Energy Emission of the Magnetar 4U 0142+614}},
	Volume = 661,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/518434}}

@article{rio07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007Ap%26SS.308..505R},
	Author = {{Rea}, N. and {Israel}, G.~L. and {Oosterbroek}, T. and {Campana}, S. and {Zane}, S. and {Turolla}, R. and {Testa}, V. and {M{\'e}ndez}, M. and {Stella}, L.},
	Doi = {10.1007/s10509-007-9310-5},
	Eprint = {arXiv:astro-ph/0610594},
	Journal = {\apss},
	Month = apr,
	Pages = {505-511},
	Title = {{X-ray intensity-hardness correlation and deep IR observations of the anomalous X-ray pulsar 1RXS J170849-400910}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9310-5}}

@article{rzl07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.308...61R},
	Author = {{Rea}, N. and {Zane}, S. and {Lyutikov}, M. and {Turolla}, R.},
	Doi = {10.1007/s10509-007-9306-1},
	Eprint = {arXiv:astro-ph/0608650},
	Journal = {\apss},
	Month = apr,
	Pages = {61-65},
	Title = {{Our distorted view of magnetars: application of the resonant cyclotron scattering model}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9306-1}}

@article{rea08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...686.1245R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Zane}, S. and {Turolla}, R. and {Lyutikov}, M. and {G{\"o}tz}, D.},
	Doi = {10.1086/591264},
	Eprint = {0802.1923},
	Journal = {\apj},
	Keywords = {Radiation Mechanisms: Nonthermal, Stars: Magnetic Fields, Stars: Neutron, X-rays: individual (4U 0142+614), X-rays: individual (1RXS J1708-4009), X-rays: individual (1E 1841-045), X-Rays: Individual: Alphanumeric: 1E 2259+586, X-rays: individual (1E 1048-5937), X-rays: individual (XTE J1810-197), X-rays: individual (1E 1547.0-5408), X-rays: individual (CXOU J1647-4552), X-rays: individual (SGR 1806-20), X-rays: individual (SGR 1900+14)},
	Month = oct,
	Pages = {1245-1260},
	Title = {{Resonant Cyclotron Scattering in Magnetars' Emission}},
	Volume = 686,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591264}}

@article{rea09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.2419R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Israel}, G.~L. and {Turolla}, R. and {Esposito}, P. and {Mereghetti}, S. and {G{\"o}tz}, D. and {Zane}, S. and {Tiengo}, A. and {Hurley}, K. and {Feroci}, M. and {Still}, M. and {Yershov}, V. and {Winkler}, C. and {Perna}, R. and {Bernardini}, F. and {Ubertini}, P. and {Stella}, L. and {Campana}, S. and {van der Klis}, M. and {Woods}, P.},
	Doi = {10.1111/j.1365-2966.2009.14920.x},
	Eprint = {0904.2413},
	Journal = {\mnras},
	Keywords = {pulsars: general , pulsars: individual: SGR0501+4516},
	Month = jul,
	Pages = {2419-2432},
	Title = {{The first outburst of the new magnetar candidate SGR0501+4516}},
	Volume = 396,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.14920.x}}

@article{rea10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010Sci...330..944R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Esposito}, P. and {Turolla}, R. and {Israel}, G.~L. and {Zane}, S. and {Stella}, L. and {Mereghetti}, S. and {Tiengo}, A. and {G{\"o}tz}, D. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C.},
	Doi = {10.1126/science.1196088},
	Eprint = {1010.2781},
	Journal = {Science},
	Month = nov,
	Pages = {944},
	Primaryclass = {astro-ph.HE},
	Title = {{A Low-Magnetic-Field Soft Gamma Repeater}},
	Volume = 330,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1126/science.1196088}}

@article{rct10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.1887R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Curto}, G.~L. and {Testa}, V. and {Israel}, G.~L. and {Possenti}, A. and {McLaughlin}, M. and {Camilo}, F. and {Gaensler}, B.~M. and {Burgay}, M.},
	Doi = {10.1111/j.1365-2966.2010.17032.x},
	Eprint = {1003.2085},
	Journal = {\mnras},
	Keywords = {pulsars: general, pulsars: individual: RRATJ1819-1458, pulsars: individual: RRATJ1317-5759},
	Month = sep,
	Pages = {1887-1894},
	Primaryclass = {astro-ph.GA},
	Title = {{Near-infrared observations of rotating radio transients}},
	Volume = 407,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17032.x}}

@incollection{rea11,
	Author = {Rea, Nanda and Esposito, Paolo},
	Booktitle = {High-Energy Emission from Pulsars and their Systems. Proceedings of the First Session of the Sant Cugat Forum on Astrophysics
},
	Doi = {10.1007/978-3-642-17251-9_21},
	Editor = {Torres, Diego F. and Rea, Nanda},
	Isbn = {978-3-642-17250-2},
	Pages = {247-273},
	Publisher = {Springer, Heidelberg},
	Series = {Astrophysics and Space Science Proceedings},
	Title = {Magnetar outbursts: an observational review},
	Year = {2011},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/978-3-642-17251-9_21}}

@article{rmi11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3515....1R},
	Author = {{Rea}, N. and {Mignani}, R.~P. and {Israel}, G.~L. and {Esposito}, P.},
	Journal = {Astron. Tel.},
	Keywords = {Optical, X-ray, Soft Gamma-ray Repeater, Transient},
	Month = jul,
	Title = {{Optical observations of Swift J1822.3-1606 with the 10.4m Gran Telescopio Canarias}},
	Volume = 3515,
	Year = 2011}

@article{rei11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ATel.3501....1R},
	Author = {{Rea}, N. and {Esposito}, P. and {Israel}, G.~L. and {Tiengo}, A. and {Zan}, S.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Soft Gamma-ray Repeater},
	Month = jul,
	Title = {{Swift J1822.3-1606: refined X-ray timing and spectral parameters}},
	Volume = 3501,
	Year = 2011}

@article{rea12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748L..12R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Pons}, J.~A. and {Torres}, D.~F. and {Turolla}, R.},
	Doi = {10.1088/2041-8205/748/1/L12},
	Eid = {L12},
	Eprint = {1202.3069},
	Journal = {\apjl},
	Keywords = {stars: magnetars, stars: neutron, X-rays: stars},
	Month = mar,
	Pages = {L12},
	Primaryclass = {astro-ph.GA},
	Title = {{The Fundamental Plane for Radio Magnetars}},
	Volume = 748,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/748/1/L12}}

@article{rie12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754...27R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Israel}, G.~L. and {Esposito}, P. and {Pons}, J.~A. and {Camero-Arranz}, A. and {Mignani}, R.~P. and {Turolla}, R. and {Zane}, S. and {Burgay}, M. and {Possenti}, A. and {Campana}, S. and {Enoto}, T. and {Gehrels}, N. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {G{\"o}tz}, D. and {Kouveliotou}, C. and {Makishima}, K. and {Mereghetti}, S. and {Oates}, S.~R. and {Palmer}, D.~M. and {Perna}, R. and {Stella}, L. and {Tiengo}, A.},
	Doi = {10.1088/0004-637X/754/1/27},
	Eid = {27},
	Eprint = {1203.6449},
	Journal = {\apj},
	Keywords = {stars: individual: Swift J1822.3{\ndash}1606, stars: magnetars, stars: neutron, X-rays: bursts, X-rays: stars},
	Month = jul,
	Pages = {27},
	Primaryclass = {astro-ph.GA},
	Title = {{A New Low Magnetic Field Magnetar: The 2011 Outburst of Swift J1822.3-1606}},
	Volume = 754,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/754/1/27}}

@article{rea13,
   author = {{Rea}, N. and {Israel}, G.~L. and {Pons}, J.~A. and {Turolla}, R. and 
	{Vigan{\`o}}, D. and {Zane}, S. and {Esposito}, P. and {Perna}, R. and 
	{Papitto}, A. and {Terreran}, G. and {Tiengo}, A. and {Salvetti}, D. and 
	{Girart}, J.~M. and {Palau}, A. and {Possenti}, A. and {Burgay}, M. and 
	{G{\"o}{\u g}{\"u}{\c s}}, E. and {Caliandro}, G.~A. and {Kouveliotou}, C. and 
	{G{\"o}tz}, D. and {Mignani}, R.~P. and {Ratti}, E. and {Stella}, L.
	},
    title = "{The Outburst Decay of the Low Magnetic Field Magnetar SGR 0418+5729}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1303.5579},
 primaryClass = "astro-ph.GA",
 keywords = {stars: individual: SGR 0418+5729, stars: magnetic field, stars: neutron},
     year = 2013,
    month = jun,
   volume = 770,
      eid = {65},
    pages = {65},
      doi = {10.1088/0004-637X/770/1/65},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770...65R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{rep13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...775L..34R},
	Archiveprefix = {arXiv},
	Author = {{Rea}, N. and {Esposito}, P. and {Pons}, J.~A. and {Turolla}, R. and {Torres}, D.~F. and {Israel}, G.~L. and {Possenti}, A. and {Burgay}, M. and {Vigan{\`o}}, D. and {Papitto}, A. and {Perna}, R. and {Stella}, L. and {Ponti}, G. and {Baganoff}, F.~K. and {Haggard}, D. and {Camero-Arranz}, A. and {Zane}, S. and {Minter}, A. and {Mereghetti}, S. and {Tiengo}, A. and {Sch{\"o}del}, R. and {Feroci}, M. and {Mignani}, R. and {G{\"o}tz}, D.},
	Doi = {10.1088/2041-8205/775/2/L34},
	Eid = {L34},
	Eprint = {1307.6331},
	Journal = {\apjl},
	Keywords = {Galaxy: center, stars: neutron, X-rays: individual: SGR J1745-2900},
	Month = oct,
	Pages = {L34},
	Primaryclass = {astro-ph.GA},
	Title = {{A Strongly Magnetized Pulsar within the Grasp of the Milky Way's Supermassive Black Hole}},
	Volume = 775,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/775/2/L34}}

@article{read97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.286..626R},
	Author = {{Read}, A.~M. and {Ponman}, T.~J. and {Strickland}, D.~K.},
	Journal = {\mnras},
	Keywords = {SURVEYS, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: ISM, GALAXIES: SPIRAL, GALAXIES: STARBURST, X-RAYS: GALAXIES},
	Month = apr,
	Pages = {626-668},
	Title = {{ROSAT PSPC observations of nearby spiral galaxies - I. The data}},
	Volume = 286,
	Year = 1997}

@ARTICLE{read01,
   author = {{Read}, A.~M. and {Pietsch}, W.},
    title = "{X-ray emission from the Sculptor galaxy NGC 300}",
  journal = {\aap},
   eprint = {astro-ph/0105106},
 keywords = {GALAXIES: CLUSTERS: SCULPTOR, GALAXIES: INDIVIDUAL: NGC 300, GALAXIES: ISM, GALAXIES: SPIRAL, X-RAYS: GALAXIES},
     year = 2001,
    month = jul,
   volume = 373,
    pages = {473-484},
      doi = {10.1051/0004-6361:20010636},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2001A%26A...373..473R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{read14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1403.3555R},
	Archiveprefix = {arXiv},
	Author = {{Read}, A.~M. and {Guainazzi}, M. and {Sembay}, S.},
	Eprint = {1403.3555},
	Journal = {\aap, in press (preprint: astro.ph/1403.3555)},
	Keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
	Month = mar,
	Primaryclass = {astro-ph.IM},
	Title = {{Cross-Calibration of the XMM-Newton EPIC pn {\amp} MOS On-Axis Effective Areas Using 2XMM Sources}},
	Year = 2014}

@ARTICLE{rees88,
       author = {{Rees}, Martin J.},
        title = "{Tidal disruption of stars by black holes of {}10$^{6}$-{}10$^{8}$ solar masses in nearby galaxies}",
      journal = {\nat},
     keywords = {Active Galactic Nuclei, Black Holes (Astronomy), Stellar Mass, Quasars, Red Shift, Star Distribution, Stellar Flares, Tides, Astrophysics},
         year = 1988,
        month = jun,
       volume = {333},
       number = {6173},
        pages = {523-528},
          doi = {10.1038/333523a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988Natur.333..523R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{reig05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...440.1079R},
	Author = {{Reig}, P. and {Negueruela}, I. and {Fabregat}, J. and {Chato}, R. and {Coe}, M.~J.},
	Doi = {10.1051/0004-6361:20053124},
	Eprint = {arXiv:astro-ph/0506230},
	Journal = {\aap},
	Keywords = {stars: individual: <ASTROBJ>RX J0440.9+4431</ASTROBJ>, <ASTROBJ>LS V +44 17</ASTROBJ>, X-rays: binaries, stars: neutron, stars: binaries: close, stars: emission-line, Be},
	Month = sep,
	Pages = {1079-1086},
	Title = {{Long-term optical/IR variability of the Be/X-ray binary <ASTROBJ>LS V +44 17</ASTROBJ>/<ASTROBJ>RX J0440.9+4431</ASTROBJ>}},
	Volume = 440,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053124}}

@article{rln07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...462.1081R},
	Author = {{Reig}, P. and {Larionov}, V. and {Negueruela}, I. and {Arkharov}, A.~A. and {Kudryavtseva}, N.~A.},
	Doi = {10.1051/0004-6361:20066217},
	Eprint = {arXiv:astro-ph/0611516},
	Journal = {\aap},
	Keywords = {stars: pulsars: individual: 4U 0115+63, stars: pulsars: individual: V635 Cas, X-rays: binaries, stars: neutron, stars: binaries: close, stars:, emission line, Be},
	Month = feb,
	Pages = {1081-1089},
	Title = {{The Be/X-ray transient 4U 0115+63/V635 Cassiopeiae. III. Quasi-cyclic variability}},
	Volume = 462,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20066217}}

@article{reig07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.377..867R},
	Author = {{Reig}, P.},
	Doi = {10.1111/j.1365-2966.2007.11657.x},
	Eprint = {arXiv:astro-ph/0703073},
	Journal = {\mnras},
	Keywords = {binaries: close , stars: emission-line, Be , stars: neutron , X-rays: binaries},
	Month = may,
	Pages = {867-873},
	Title = {{On the neutron star-disc interaction in Be/X-ray binaries}},
	Volume = 377,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2007.11657.x}}

@article{remillard06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ARA%26A..44...49R},
	Author = {{Remillard}, R.~A. and {McClintock}, J.~E.},
	Doi = {10.1146/annurev.astro.44.051905.092532},
	Eprint = {arXiv:astro-ph/0606352},
	Journal = {\araa},
	Month = sep,
	Pages = {49-92},
	Title = {{X-Ray Properties of Black-Hole Binaries}},
	Volume = 44,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.astro.44.051905.092532}}

@article{repetto12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2799R},
	Archiveprefix = {arXiv},
	Author = {{Repetto}, S. and {Davies}, M.~B. and {Sigurdsson}, S.},
	Doi = {10.1111/j.1365-2966.2012.21549.x},
	Eprint = {1203.3077},
	Journal = {\mnras},
	Keywords = {black hole physics, binaries: general, stars: neutron, supernovae: general, Galaxy: kinematics and dynamics, X-rays: binaries},
	Month = oct,
	Pages = {2799-2809},
	Primaryclass = {astro-ph.GA},
	Title = {{Investigating stellar-mass black hole kicks}},
	Volume = 425,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21549.x}}

@article{revnivtsev03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003ATel..131....1R&db_key=AST},
	Author = {{Revnivtsev}, M. and {Lutovinov}, A. and {Ebisawa}, K.},
	Journal = {Astron.~Tel.~131},
	Month = mar,
	Title = {{IGR J16358-4726 in archival data of ASCA and BeppoSAX}},
	Year = 2003}

@article{revnivtsev04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004AstL...30..382R&db_key=AST},
	Author = {{Revnivtsev}, M.~G. and {Sunyaev}, R.~A. and {Varshalovich}, D.~A. and {Zheleznyakov}, V.~V. and {Cherepashchuk}, A.~M. and {Lutovinov}, A.~A. and {Churazov}, E.~M. and {Grebenev}, S.~A. and {Gilfanov}, M.~R.},
	Journal = {Astron.~Lett.},
	Month = jun,
	Pages = {382-389},
	Title = {{A Hard X-ray Survey of the Galactic-Center Region with the IBIS Telescope of the INTEGRAL Observatory: A Catalog of Sources}},
	Volume = 30,
	Year = 2004}

@ARTICLE{revnivtsev14,
   author = {{Revnivtsev}, M.~G. and {Sunyaev}, R.~A. and {Krivonos}, R.~A. and 
	{Tsygankov}, S.~S. and {Molkov}, S.~V.},
    title = "{Broadband spectrum of the total X-ray emission from the galaxy M31}",
  journal = {Astronomy Letters},
 keywords = {X-ray sources},
     year = 2014,
    month = jan,
   volume = 40,
    pages = {22-28},
      doi = {10.1134/S1063773714010046},
   adsurl = {http://adsabs.harvard.edu/abs/2014AstL...40...22R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{reynolds06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...639L..71R},
	Author = {{Reynolds}, S.~P. and {Borkowski}, K.~J. and {Gaensler}, B.~M. and {Rea}, N. and {McLaughlin}, M. and {Possenti}, A. and {Israel}, G. and {Burgay}, M. and {Camilo}, F. and {Chatterjee}, S. and {Kramer}, M. and {Lyne}, A. and {Stairs}, I.},
	Doi = {10.1086/502648},
	Eprint = {arXiv:astro-ph/0512379},
	Journal = {\apjl},
	Month = mar,
	Pages = {L71-L74},
	Title = {{Discovery of the X-Ray Counterpart to the Rotating Radio Transient J1819-1458}},
	Volume = 639,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/502648}}

@article{reynolds06cco,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...652L..45R},
	Author = {{Reynolds}, S.~P. and {Borkowski}, K.~J. and {Hwang}, U. and {Harrus}, I. and {Petre}, R. and {Dubner}, G.},
	Doi = {10.1086/510066},
	Eprint = {arXiv:astro-ph/0610323},
	Journal = {\apjl},
	Month = nov,
	Pages = {L45-L48},
	Title = {{A New Young Galactic Supernova Remnant Containing a Compact Object: G15.9+0.2}},
	Volume = 652,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/510066}}

@article{reynoso95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995AJ....110..318R},
	Author = {{Reynoso}, E.~M. and {Dubner}, G.~M. and {Goss}, W.~M. and {Arnal}, E.~M.},
	Doi = {10.1086/117522},
	Journal = {\aj},
	Keywords = {SUPERNOVA REMNANTS, ISM: ABUNDANCES, ISM: KINEMATICS AND DYNAMICS},
	Month = jul,
	Pages = {318},
	Title = {{VLA Observations of Neutral Hydrogen in the Direction of Puppis A}},
	Volume = 110,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/117522}}

@article{reynoso04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004PASA...21...82R},
	Author = {{Reynoso}, E.~M. and {Green}, A.~J. and {Johnston}, S. and {Goss}, W.~M. and {Dubner}, G.~M. and {Giacani}, E.~B.},
	Doi = {10.1071/AS03053},
	Eprint = {arXiv:astro-ph/0310100},
	Journal = {\pasa},
	Keywords = {stars: neutron, supernova remnants, ISM: individual: RCW 103, X-rays: individual: 1E 161348-5055, spectral lines: neutral hydrogen.},
	Pages = {82-88},
	Title = {{Influence of the Neutron Star 1E 161348-5055 in RCW 103 on the Surrounding Medium}},
	Volume = 21,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1071/AS03053}}

@article{reynoso06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...449..243R},
	Author = {{Reynoso}, E.~M. and {Dubner}, G. and {Giacani}, E. and {Johnston}, S. and {Green}, A.~J.},
	Doi = {10.1051/0004-6361:20054236},
	Eprint = {arXiv:astro-ph/0512009},
	Journal = {\aap},
	Month = apr,
	Pages = {243-250},
	Title = {{The interior of the SNR RX J0852.0-4622 (Vela Jr) at radio wavelengths}},
	Volume = 449,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054236}}

@ARTICLE{rhode01,
       author = {{Rhode}, Katherine L. and {Zepf}, Stephen E.},
        title = "{The Globular Cluster System in the Outer Regions of NGC 4472}",
      journal = {\aj},
     keywords = {Galaxies: Formation, Galaxies: Individual: NGC Number: NGC 4472, Galaxies: Star Clusters, Astrophysics},
         year = 2001,
        month = jan,
       volume = {121},
       number = {1},
        pages = {210-224},
          doi = {10.1086/318039},
archivePrefix = {arXiv},
       eprint = {astro-ph/0010065},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001AJ....121..210R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Richards1969,
       author = {{Richards}, D.~W. and {Comella}, J.~M.},
        title = "{The Period of Pulsar NP 0532}",
      journal = {\nat},
         year = 1969,
        month = may,
       volume = {222},
       number = {5193},
        pages = {551-552},
          doi = {10.1038/222551a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969Natur.222..551R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{richings10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2010ApJ...723.1375R},
	Archiveprefix = {arXiv},
	Author = {{Richings}, A.~J. and {Fabbiano}, G. and {Wang}, J. and {Roberts}, T.~P.},
	Doi = {10.1088/0004-637X/723/2/1375},
	Eprint = {1009.4396},
	Journal = {\apj},
	Keywords = {galaxies: individual: NGC 4485/90, galaxies: interactions, galaxies: ISM, X-rays: galaxies, X-rays: ISM},
	Month = nov,
	Pages = {1375-1392},
	Primaryclass = {astro-ph.GA},
	Title = {{The Hot Interstellar Medium of the Interacting Galaxy NGC 4490}},
	Volume = 723,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/723/2/1375}}

@ARTICLE{ripamonti12,
       author = {{Ripamonti}, E. and {Mapelli}, M.},
        title = "{Broad [O III] in the globular cluster RZ 2109: X-ray ionized nova ejecta}",
      journal = {\mnras},
     keywords = {novae, cataclysmic variables, ISM: jets and outflows, galaxies: individual: NGC 4472, galaxies: star clusters: individual: RZ 2109, X-rays: binaries, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = jun,
       volume = {423},
       number = {2},
        pages = {1144-1153},
          doi = {10.1111/j.1365-2966.2012.20942.x},
archivePrefix = {arXiv},
       eprint = {1203.4233},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.423.1144R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ritter03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...404..301R},
	Author = {{Ritter}, H. and {Kolb}, U.},
	Doi = {10.1051/0004-6361:20030330},
	Eprint = {astro-ph/0301444},
	Journal = {\aap},
	Keywords = {catalogs, stars: novae, cataclysmic variables, stars: binaries: close},
	Month = jun,
	Pages = {301-303},
	Title = {{Catalogue of cataclysmic binaries, low-mass X-ray binaries and related objects (Seventh edition)}},
	Volume = 404,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20030330}}

@article{rivera10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..797R},
	Archiveprefix = {arXiv},
	Author = {{Rivera-Ingraham}, A. and {van Kerkwijk}, M.~H.},
	Doi = {10.1088/0004-637X/710/1/797},
	Eprint = {1001.4465},
	Journal = {\apj},
	Keywords = {dust, extinction, scattering, stars: individual: 4U 0142+61 1E 1048.1-5937 1RXS J170849.0-400910, stars: neutron},
	Month = feb,
	Pages = {797-803},
	Primaryclass = {astro-ph.GA},
	Title = {{Extinction and Distance to Anomalous X-ray Pulsars from X-ray Scattering Halos}},
	Volume = 710,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/710/1/797}}

@ARTICLE{rizzuto21,
       author = {{Rizzuto}, Francesco Paolo and {Naab}, Thorsten and {Spurzem}, Rainer and {Giersz}, Mirek and {Ostriker}, J.~P. and {Stone}, N.~C. and {Wang}, Long and {Berczik}, Peter and {Rampp}, M.},
        title = "{Intermediate mass black hole formation in compact young massive star clusters}",
      journal = {\mnras},
     keywords = {gravitational waves, methods: numerical, stars: black holes, stars: mass-loss, galaxies: star clusters: general, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = mar,
       volume = {501},
       number = {4},
        pages = {5257-5273},
          doi = {10.1093/mnras/staa3634},
archivePrefix = {arXiv},
       eprint = {2008.09571},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.5257R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{roberts00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315...98R},
	Author = {{Roberts}, T.~P. and {Warwick}, R.~S.},
	Doi = {10.1046/j.1365-8711.2000.03384.x},
	Eprint = {arXiv:astro-ph/0001209},
	Journal = {\mnras},
	Keywords = {GALAXIES: ACTIVE, GALAXIES: GENERAL, X-RAYS: GALAXIES},
	Month = jun,
	Pages = {98-114},
	Title = {{A ROSAT High Resolution Imager survey of bright nearby galaxies}},
	Volume = 315,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2000.03384.x}}

@article{roberts02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002MNRAS.337..677R},
	Author = {{Roberts}, T.~P. and {Warwick}, R.~S. and {Ward}, M.~J. and {Murray}, S.~S.},
	Doi = {10.1046/j.1365-8711.2002.05950.x},
	Eprint = {arXiv:astro-ph/0208196},
	Journal = {\mnras},
	Keywords = {galaxies: individual: NGC 4485, galaxies: individual: NGC 4490, galaxies: interactions, X-rays: galaxies},
	Month = dec,
	Pages = {677-692},
	Title = {{A Chandra observation of the interacting pair of galaxies NGC 4485/4490}},
	Volume = 337,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05950.x}}

@article{roberts07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.311..203R},
	Archiveprefix = {arXiv},
	Author = {{Roberts}, T.~P.},
	Doi = {10.1007/s10509-007-9547-z},
	Eprint = {0706.2562},
	Journal = {\apss},
	Keywords = {Black hole physics, X-rays: binaries, X-rays: galaxies},
	Month = oct,
	Pages = {203-212},
	Title = {{X-ray observations of ultraluminous X-ray sources}},
	Volume = 311,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9547-z}}

@article{roelofs10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711L.138R},
	Archiveprefix = {arXiv},
	Author = {{Roelofs}, G.~H.~A. and {Rau}, A. and {Marsh}, T.~R. and {Steeghs}, D. and {Groot}, P.~J. and {Nelemans}, G.},
	Doi = {10.1088/2041-8205/711/2/L138},
	Eprint = {1003.0658},
	Journal = {\apjl},
	Keywords = {binaries: close, gravitational waves, stars: individual: HM Cancri V407 Vulpeculae, X-rays: binaries},
	Month = mar,
	Pages = {L138-L142},
	Title = {{Spectroscopic Evidence for a 5.4 Minute Orbital Period in HM Cancri}},
	Volume = 711,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/711/2/L138}}

@article{roming05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005SSRv..120...95R},
	Author = {{Roming}, P.~W.~A. and {Kennedy}, T.~E. and {Mason}, K.~O. and {Nousek}, J.~A. and {Ahr}, L. and {Bingham}, R.~E. and {Broos}, P.~S. and {Carter}, M.~J. and {Hancock}, B.~K. and {Huckle}, H.~E. and {Hunsberger}, S.~D. and {Kawakami}, H. and {Killough}, R. and {Koch}, T.~S. and {McLelland}, M.~K. and {Smith}, K. and {Smith}, P.~J. and {Soto}, J.~C. and {Boyd}, P.~T. and {Breeveld}, A.~A. and {Holland}, S.~T. and {Ivanushkina}, M. and {Pryzby}, M.~S. and {Still}, M.~D. and {Stock}, J.},
	Doi = {10.1007/s11214-005-5095-4},
	Eprint = {arXiv:astro-ph/0507413},
	Journal = {Space Science Reviews},
	Month = oct,
	Pages = {95-142},
	Title = {{The Swift Ultra-Violet/Optical Telescope}},
	Volume = 120,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11214-005-5095-4}}

@ARTICLE{1RXH,
       author = {{ROSAT Scientific Team}},
        title = "{VizieR Online Data Catalog: ROSAT HRI Pointed Observations (1RXH) (ROSAT Team, 2000)}",
      journal = {VizieR Online Data Catalog},
     keywords = {X-ray sources, Surveys},
         year = 2000,
        month = may,
       number = {71},
          eid = {IX/28A},
        pages = {IX/28A},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000yCat.9028....0R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{rosen88,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1988MNRAS.231..549R},
	Author = {{Rosen}, S.~R. and {Mason}, K.~O. and {Cordova}, F.~A.},
	Journal = {\mnras},
	Keywords = {Cataclysmic Variables, Eclipsing Binary Stars, Magnetic Stars, X Ray Astronomy, Companion Stars, Exosat Satellite, Light Curve, Spaceborne Astronomy, Stellar Mass Accretion, Stellar Occultation},
	Month = mar,
	Pages = {549-573},
	Title = {{EXOSAT X-ray observations of the eclipsing magnetic cataclysmic variable EX Hya}},
	Volume = 231,
	Year = 1988}

@article{rosen15,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150407051R},
	Archiveprefix = {arXiv},
	Author = {{Rosen}, S.~R. and {Webb}, N.~A. and {Watson}, M.~G. and {Ballet}, J. and {Barret}, D. and {Braito}, V. and {Carrera}, F.~J. and {Ceballos}, M.~T. and {Coriat}, M. and {Della Ceca}, R. and {Denkinson}, G. and {Esquej}, P. and {Farrell}, S.~A. and {Freyberg}, M. and {Gris{\'e}}, F. and {Guillout}, P. and {Heil}, L. and {Law-Green}, D. and {Lamer}, G. and {Lin}, D. and {Martino}, R. and {Michel}, L. and {Motch}, C. and {Nebot Gomez-Moran}, A. and {Page}, C.~G. and {Page}, K. and {Page}, M. and {Pakull}, M.~W. and {Pye}, J. and {Read}, A. and {Rodriguez}, P. and {Sakano}, M. and {Saxton}, R. and {Schwope}, A. and {Scott}, A.~E. and {Sturm}, R. and {Traulsen}, I. and {Yershov}, V. and {Zolotukhin}, I.},
	Eprint = {1504.07051},
	Journal = {\aap, submitted (preprint: astro-ph/1504.07051)},
	Keywords = {Astrophysics - High Energy Astrophysical Phenomena},
	Month = apr,
	Primaryclass = {astro-ph.HE},
	Title = {{The XMM-Newton serendipitous survey. VII. The third XMM-Newton serendipitous source catalogue}},
	Year = 2015}

@article{rothschild94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994Natur.368..432R&amp;db_key=AST},
	Author = {{Rothschild}, R.~E. and {Kulkarni}, S.~R. and {Lingenfelter}, R.~E.},
	Journal = {\nat},
	Month = mar,
	Pages = {432},
	Title = {{Discovery of an X-Ray Source Coincident with the Soft Gamma-ray Repeater 0525-66}},
	Volume = 368,
	Year = 1994}

@inproceedings{rothschild02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002nssr.conf..257R&db_key=AST},
	Author = {{Rothschild}, R.~E. and {Lingenfelter}, R.~E. and {Marsden}, D.},
	Booktitle = {ASP Conf. Ser. 271: Neutron Stars in Supernova Remnants},
	Pages = {257},
	Title = {{Propeller vs. Magnetar Concepts for SGRs/AXPs}},
	Year = 2002}

@ARTICLE{rousseau78,
   author = {{Rousseau}, J. and {Martin}, N. and {Pr{\'e}vot}, L. and {Rebeirot}, E. and 
	{Robin}, A. and {Brunet}, J.~P.},
    title = "{Studies of the Large Magellanic Cloud stellar content: III. Spectral types and V magnitudes of 1822 members.}",
  journal = {\aaps},
 keywords = {Magellanic Clouds:Spectral Classification, Magellanic Clouds:Stellar Content, Magellanic Clouds:Supergiants},
     year = 1978,
    month = feb,
   volume = 31,
    pages = {243-260},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26AS...31..243R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{rousset03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://esoads.eso.org/abs/2003SPIE.4839..140R},
	Author = {{Rousset}, G. and {Lacombe}, F. and {Puget}, P. and {Hubin}, N.~N. and {Gendron}, E. and {Fusco}, T. and {Arsenault}, R. and {Charton}, J. and {Feautrier}, P. and {Gigan}, P. and {Kern}, P.~Y. and {Lagrange}, A.-M. and {Madec}, P.-Y. and {Mouillet}, D. and {Rabaud}, D. and {Rabou}, P. and {Stadler}, E. and {Zins}, G.},
	Booktitle = {Adaptive Optical System Technologies II.},
	Doi = {10.1117/12.459332},
	Editor = {{Wizinowich}, P.~L. and {Bonaccini}, D.},
	Month = feb,
	Pages = {140-149},
	Publisher = {SPIE, Bellingham},
	Series = {SPIE Conference Series},
	Title = {{NAOS, the first AO system of the VLT: on-sky performance}},
	Volume = 4839,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.459332}}

@article{russeil03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...397..133R},
	Author = {{Russeil}, D.},
	Doi = {10.1051/0004-6361:20021504},
	Journal = {\aap},
	Keywords = {ISM: HII regions, Galaxy: kinematics and dynamics, Galaxy: structure},
	Month = jan,
	Pages = {133-146},
	Title = {{Star-forming complexes and the spiral structure of our Galaxy}},
	Volume = 397,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20021504}}

@article{sambruna01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...546L...9S},
	Author = {{Sambruna}, R.~M. and {Brandt}, W.~N. and {Chartas}, G. and {Netzer}, H. and {Kaspi}, S. and {Garmire}, G.~P. and {Nousek}, J.~A. and {Weaver}, K.~A.},
	Doi = {10.1086/318067},
	Eprint = {astro-ph/0010355},
	Journal = {\apjl},
	Keywords = {Galaxies: Active, Galaxies: Individual: Name: Circinus, Galaxies: Nuclei, Galaxies: Seyfert, X-Rays: Galaxies},
	Month = jan,
	Pages = {L9-L12},
	Title = {{X-Ray Imaging of the Seyfert 2 Galaxy Circinus with Chandra}},
	Volume = 546,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/318067}}

@ARTICLE{sana06,
   author = {{Sana}, H. and {Rauw}, G. and {Naz{\'e}}, Y. and {Gosset}, E. and 
	{Vreux}, J.-M.},
    title = "{An XMM-Newton view of the young open cluster NGC 6231 - II. The OB star population}",
  journal = {\mnras},
   eprint = {astro-ph/0607486},
 keywords = {open clusters and associations: individual: NGC 6231 , stars: fundamental parameters , stars: early-type , X-rays: individuals: NGC 6231 , X-rays: stars},
     year = 2006,
    month = oct,
   volume = 372,
    pages = {661-678},
      doi = {10.1111/j.1365-2966.2006.10847.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..661S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{sanders03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126.1607S},
	Author = {{Sanders}, D.~B. and {Mazzarella}, J.~M. and {Kim}, D.-C. and {Surace}, J.~A. and {Soifer}, B.~T.},
	Doi = {10.1086/376841},
	Eprint = {astro-ph/0306263},
	Journal = {\aj},
	Keywords = {Galaxies: General, Infrared Radiation},
	Month = oct,
	Pages = {1607-1664},
	Title = {{The IRAS Revised Bright Galaxy Sample}},
	Volume = 126,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/376841}}

@inproceedings{sanwal02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002AAS...200.7201S},
	Author = {{Sanwal}, D. and {Garmire}, G.~P. and {Garmire}, A. and {Pavlov}, G.~G. and {Mignani}, R.},
	Booktitle = {200th AAS Meeting,},
	Month = may,
	Pages = {764},
	Series = {Bulletin of the American Astronomical Society, Washington DC},
	Title = {{Accreting Compact Object at the Center of the Supernova Remnant RCW 103}},
	Volume = 34,
	Year = 2002}

@article{sarazin00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...544L.101S},
	Author = {{Sarazin}, C.~L. and {Irwin}, J.~A. and {Bregman}, J.~N.},
	Doi = {10.1086/317308},
	Eprint = {arXiv:astro-ph/0009448},
	Journal = {\apjl},
	Keywords = {Stars: Binaries: Close, Galaxies: Elliptical and Lenticular, cD, Galaxies: ISM, X-Rays: Galaxies, X-Rays: ISM, X-Rays: Stars},
	Month = dec,
	Pages = {L101-L105},
	Title = {{Resolving the Mystery of X-Ray-faint Elliptical Galaxies: Chandra X-Ray Observations of NGC 4697}},
	Volume = 544,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/317308}}

@article{sarma97,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...483..335S&db_key=AST},
	Author = {{Sarma}, A.~P. and {Goss}, W.~M. and {Green}, A.~J. and {Frail}, D.~A.},
	Journal = {\apj},
	Month = jul,
	Pages = {335},
	Title = {{Australia Telescope Observations of the CTB 33 Complex}},
	Volume = 483,
	Year = 1997}

@article{sarraj12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2012IBVS.6030....1S},
	Author = {{Sarraj}, I. and {Sanders}, R.~J. and {Schmidtke}, P.~C.},
	Journal = {Information Bulletin on Variable Stars},
	Keywords = {Be stars, X-ray binaries},
	Month = jul,
	Pages = {1},
	Title = {{Photometric Behavior of Eight Be/X-ray Binaries in the SMC}},
	Volume = 6030,
	Year = 2012}

@article{sasano14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014PASJ...66...35S},
	Archiveprefix = {arXiv},
	Author = {{Sasano}, M. and {Makishima}, K. and {Sakurai}, S. and {Zhang}, Z. and {Enoto}, T.},
	Doi = {10.1093/pasj/psu002},
	Eid = {35},
	Eprint = {1311.4618},
	Journal = {\pasj},
	Keywords = {accretion, accretion disks, stars: magnetic fields, X-rays: binaries},
	Month = apr,
	Pages = {35},
	Primaryclass = {astro-ph.HE},
	Title = {{Suzaku view of the neutron star in the dipping source 4U 1822-37}},
	Volume = 66,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/pasj/psu002}}

@article{sato05,
	Author = {{Sato}, G. and {Antonelli}, L. and {Barthelmy}, S. and {Barbier}, L. and {Cropper}, M. and {Cummings}, J. and {Fenimore}, E. and {Fink}, R. and {Galassi}, M. and {Gehrels}, N. and {Hullinger}, D. and {Krimm}, H. and {Markwardt}, C. and {Meszaros}, P. and {McLean}, K. and {Palmer}, D. and {Parsons}, A. and {Sakamoto}, T. and {Suzuki}, M. and {Tueller}, J.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR1806-20: Swift-BAT detection of a large normal burst.}},
	Volume = 3002,
	Year = 2005}

@ARTICLE{saxton20,
       author = {{Saxton}, R. and {Komossa}, S. and {Auchettl}, K. and {Jonker}, P.~G.},
        title = "{X-Ray Properties of TDEs}",
      journal = {\ssr},
     keywords = {X-ray, TDE, Black holes, Accretion disks},
         year = 2020,
        month = jul,
       volume = {216},
       number = {5},
          eid = {85},
        pages = {85},
          doi = {10.1007/s11214-020-00708-4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SSRv..216...85S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{sazonov06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...450..117S},
	Author = {{Sazonov}, S. and {Revnivtsev}, M. and {Gilfanov}, M. and {Churazov}, E. and {Sunyaev}, R.},
	Doi = {10.1051/0004-6361:20054297},
	Eprint = {astro-ph/0510049},
	Journal = {\aap},
	Keywords = {stars: luminosity function, mass function, Galaxy: structure, X-rays: binaries, X-rays: galaxies, X-rays: stars},
	Month = apr,
	Pages = {117-128},
	Title = {{X-ray luminosity function of faint point sources in the Milky Way}},
	Volume = 450,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20054297}}

@article{scargle82,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...263..835S},
	Author = {{Scargle}, J.~D.},
	Doi = {10.1086/160554},
	Journal = {\apj},
	Keywords = {ASTRONOMY, SIGNAL DETECTION, SPECTRUM ANALYSIS, STATISTICAL DISTRIBUTIONS, TIME SERIES ANALYSIS, FOURIER TRANSFORMATION, FREQUENCY RESPONSE, POWER SPECTRA, SIGNAL TO NOISE RATIOS},
	Month = dec,
	Pages = {835-853},
	Title = {{Studies in astronomical time series analysis. II - Statistical aspects of spectral analysis of unevenly spaced data}},
	Volume = 263,
	Year = 1982,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160554}}

@article{scargle98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...504..405S},
	Author = {{Scargle}, J.~D.},
	Doi = {10.1086/306064},
	Journal = {\apj},
	Keywords = {METHODS: DATA ANALYSIS, GAMMA RAYS: BURSTS, METHODS: NUMERICAL, METHODS: STATISTICAL},
	Month = sep,
	Pages = {405},
	Title = {{Studies in Astronomical Time Series Analysis. V. Bayesian Blocks, a New Method to Analyze Structure in Photon Counting Data}},
	Volume = 504,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/306064}}
	
@ARTICLE{schild03,
       author = {{Schild}, H. and {Crowther}, P.~A. and {Abbott}, J.~B. and {Schmutz}, W.},
        title = "{A large Wolf-Rayet population in NGC 300 uncovered by VLT-FORS2}",
      journal = {\aap},
     keywords = {galaxies: individual: NGC 300, stars: Wolf-Rayet, stars: fundamental parameters, Astrophysics},
         year = "2003",
        month = "Jan",
       volume = {397},
        pages = {859-870},
          doi = {10.1051/0004-6361:20021555},
archivePrefix = {arXiv},
       eprint = {astro-ph/0209259},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...397..859S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schlafly11,
   author = {{Schlafly}, E.~F. and {Finkbeiner}, D.~P.},
    title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.4804},
 primaryClass = "astro-ph.GA",
 keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {103},
    pages = {103},
      doi = {10.1088/0004-637X/737/2/103},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737..103S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{schlegel98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..525S},
	Author = {{Schlegel}, D.~J. and {Finkbeiner}, D.~P. and {Davis}, M.},
	Doi = {10.1086/305772},
	Eprint = {arXiv:astro-ph/9710327},
	Journal = {\apj},
	Keywords = {COSMOLOGY: DIFFUSE RADIATION, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, INFRARED: ISM: CONTINUUM},
	Month = jun,
	Pages = {525},
	Title = {{Maps of Dust Infrared Emission for Use in Estimation of Reddening and Cosmic Microwave Background Radiation Foregrounds}},
	Volume = 500,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/305772}}

@article{schodel09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...502...91S},
	Archiveprefix = {arXiv},
	Author = {{Sch{\"o}del}, R. and {Merritt}, D. and {Eckart}, A.},
	Doi = {10.1051/0004-6361/200810922},
	Eprint = {0902.3892},
	Journal = {\aap},
	Keywords = {instrumentation: adaptive optics, techniques: high angular resolution, stars: kinematics, Galaxy: center, Galaxy: structure},
	Month = jul,
	Pages = {91-111},
	Primaryclass = {astro-ph.GA},
	Title = {{The nuclear star cluster of the Milky Way: proper motions and mass}},
	Volume = 502,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200810922}}

@article{schodel10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...511A..18S},
	Author = {{Sch{\"o}del}, R. and {Najarro}, F. and {Muzic}, K. and {Eckart}, A.},
	Doi = {10.1051/0004-6361/200913183},
	Eid = {A18},
	Journal = {\aap},
	Keywords = {Galaxy: nucleus, dust, extinction, Galaxy: center, stars: horizontal-branch},
	Month = feb,
	Pages = {A18},
	Title = {{Peering through the veil: near-infrared photometry and extinction for the Galactic nuclear star cluster. Accurate near infrared H, Ks, and L' photometry and the near-infrared extinction-law toward the central parsec of the Galaxy}},
	Volume = 511,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913183}}

@article{schoenberner95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...294..509S},
	Author = {{Schoenberner}, D. and {Harmanec}, P.},
	Journal = {\aap},
	Keywords = {Brightness, Early Stars, Eclipsing Binary Stars, Stellar Mass, Stellar Models, Calibrating, Solar Neighborhood, Star Clusters, Stellar Evolution, Stellar Temperature},
	Month = feb,
	Pages = {509-514},
	Title = {{On the absolute brightnesses and masses of early-type stars}},
	Volume = 294,
	Year = 1995}

@inproceedings{schoenfelder00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000AIPC..510...54S},
	Author = {{Sch{\"o}nfelder}, V. and {Bloemen}, H. and {Collmar}, W. and {Diehl}, R. and {Hermsen}, W. and {Kn{\"o}dlseder}, J. and {Lichti}, G.~G. and {Pl{\"u}schke}, S. and {Ryan}, J. and {Strong}, A. and {Winkler}, C.},
	Booktitle = {{McConnell}, M.~L. and {Ryan}, J.~M., eds., The Fifth Compton Symposium.},
	Pages = {54},
	Series = {AIP Conference Proceedings, Melville NY},
	Title = {{$^{44}$Ti Gamma-Ray Line Emission from Cas A and RXJ0852-4622/GROJ0852-4642}},
	Volume = 510,
	Year = 2000}

@article{scholz12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...761...66S},
	Archiveprefix = {arXiv},
	Author = {{Scholz}, P. and {Ng}, C.-Y. and {Livingstone}, M.~A. and {Kaspi}, V.~M. and {Cumming}, A. and {Archibald}, R.~F.},
	Doi = {10.1088/0004-637X/761/1/66},
	Eid = {66},
	Eprint = {1204.1034},
	Journal = {\apj},
	Keywords = {pulsars: individual: Swift J1822.3{\ndash}1606, stars: neutron, X-rays: bursts, X-rays: general},
	Month = dec,
	Pages = {66},
	Primaryclass = {astro-ph.HE},
	Title = {{Post-outburst X-Ray Flux and Timing Evolution of Swift J1822.3-1606}},
	Volume = 761,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/761/1/66}}

@ARTICLE{scholz17,
   author = {{Scholz}, P. and {Camilo}, F. and {Sarkissian}, J. and {Reynolds}, J.~E. and 
	{Levin}, L. and {Bailes}, M. and {Burgay}, M. and {Johnston}, S. and 
	{Kramer}, M. and {Possenti}, A.},
    title = "{Spin-down Evolution and Radio Disappearance of the Magnetar PSR J1622-4950}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1705.04899},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, pulsars: individual: PSR J1622{\ndash}4950, stars: magnetars, stars: neutron},
     year = 2017,
    month = jun,
   volume = 841,
      eid = {126},
    pages = {126},
      doi = {10.3847/1538-4357/aa73de},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...841..126S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{schraerer92,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1992A%26A...263..129S},
	Author = {{Schaerer}, D. and {Maeder}, A.},
	Journal = {\aap},
	Keywords = {Stellar Models, Wolf-Rayet Stars, Abundance, Stellar Composition, Stellar Cores, Stellar Luminosity, Stellar Mass Ejection, Stellar Temperature},
	Month = sep,
	Pages = {129-136},
	Title = {{Basic relations between physical parameters of Wolf-Rayet stars}},
	Volume = 263,
	Year = 1992}

@article{schwartzschild59,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1959ApJ...129..637S&db_key=AST},
	Author = {{Schwarzschild}, M. and {H{\"a}rm}, R.},
	Journal = {\apj},
	Month = may,
	Pages = {637},
	Title = {{On the Maximum Mass of Stable Stars.}},
	Volume = 129,
	Year = 1959}

@ARTICLE{seiradakis04,
   author = {{Seiradakis}, J.~H. and {Wielebinski}, R.},
    title = "{Morphology and characteristics of radio pulsars}",
  journal = {\aapr},
   eprint = {hep-ph/0410022},
 keywords = {Radio pulsar morphology: pulse shapes, spectra, polarization, distributions},
     year = 2004,
    month = dec,
   volume = 12,
    pages = {239-271},
      doi = {10.1007/s00159-004-0022-3},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26ARv..12..239S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{serim17,
   author = {{Serim}, M.~M. and {{\c S}ahiner}, {\c S}. and {{\c C}erri-Serim}, D. and 
	{{\.I}nam}, S.~{\c C}. and {Baykal}, A.},
    title = "{Comprehensive timing and X-ray spectral analysis of GX 1+4}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1701.04328},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion discs, stars: neutron, pulsars: individual: GX 1+4, X-rays: binaries},
     year = 2017,
    month = aug,
   volume = 469,
    pages = {2509-2516},
      doi = {10.1093/mnras/stx1045},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.469.2509S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{serlemitsos07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007PASJ...59S...9S},
	Author = {{Serlemitsos}, P.~J. and {Soong}, Y. and {Chan}, K.-W. and {Okajima}, T. and {Lehan}, J.~P. and {Maeda}, Y. and {Itoh}, K. and {Mori}, H. and {Iizuka}, R. and {Itoh}, A. and {Inoue}, H. and {Okada}, S. and {Yokoyama}, Y. and {Itoh}, Y. and {Ebara}, M. and {Nakamura}, R. and {Suzuki}, K. and {Ishida}, M. and {Hayakawa}, A. and {Inoue}, C. and {Okuma}, S. and {Kubota}, R. and {Suzuki}, M. and {Osawa}, T. and {Yamashita}, K. and {Kunieda}, H. and {Tawara}, Y. and {Ogasaka}, Y. and {Furuzawa}, A. and {Tamura}, K. and {Shibata}, R. and {Haba}, Y. and {Naitou}, M. and {Misaki}, K.},
	Journal = {\pasj},
	Month = jan,
	Pages = {9-21},
	Title = {{The X-Ray Telescope onboard Suzaku}},
	Volume = 59,
	Year = 2007}

@ARTICLE{seward88,
   author = {{Seward}, F.~D. and {Wang}, Z.-R.},
    title = "{Pulsars, X-ray synchrotron nebulae, and guest stars}",
  journal = {\apj},
 keywords = {Neutron Stars, Pulsars, Stellar Coronas, Stellar Rotation, Supernova Remnants, X Ray Astronomy, Charged Particles, Energy Dissipation, Magnetic Dipoles, Radio Sources (Astronomy), Relativistic Particles},
     year = 1988,
    month = sep,
   volume = 332,
    pages = {199-205},
      doi = {10.1086/166646},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...332..199S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{seward03,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...584..414S},
	Author = {{Seward}, F.~D. and {Slane}, P.~O. and {Smith}, R.~K. and {Sun}, M.},
	Doi = {10.1086/345600},
	Eprint = {arXiv:astro-ph/0210496},
	Journal = {\apj},
	Month = feb,
	Pages = {414-417},
	Title = {{A Compact Central Object in the Supernova Remnant Kesteven 79}},
	Volume = 584,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/345600}}

@article{sguera05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005A%26A...444..221S&db_key=AST},
	Author = {{Sguera}, V. and {Barlow}, E.~J. and {Bird}, A.~J. and {Clark}, D.~J. and {Dean}, A.~J. and {Hill}, A.~B. and {Moran}, L. and {Shaw}, S.~E. and {Willis}, D.~R. and {Bazzano}, A. and {Ubertini}, P. and {Malizia}, A.},
	Doi = {10.1051/0004-6361:20053103},
	Eprint = {astro-ph/0509018},
	Journal = {\aap},
	Month = dec,
	Pages = {221-231},
	Title = {{INTEGRAL observations of recurrent fast X-ray transient sources}},
	Volume = 444,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20053103}}

@article{shabaltas12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748..148S},
	Archiveprefix = {arXiv},
	Author = {{Shabaltas}, N. and {Lai}, D.},
	Doi = {10.1088/0004-637X/748/2/148},
	Eid = {148},
	Eprint = {1110.3129},
	Journal = {\apj},
	Keywords = {magnetic fields, pulsars: individual: PSR J1852+0040, radiative transfer, stars: neutron, X-rays: stars},
	Month = apr,
	Pages = {148},
	Primaryclass = {astro-ph.HE},
	Title = {{The Hidden Magnetic Field of the Young Neutron Star in Kesteven 79}},
	Volume = 748,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/748/2/148}}

@article{shakura12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420..216S},
	Archiveprefix = {arXiv},
	Author = {{Shakura}, N. and {Postnov}, K. and {Kochetkova}, A. and {Hjalmarsdotter}, L.},
	Doi = {10.1111/j.1365-2966.2011.20026.x},
	Eprint = {1110.3701},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, pulsars: general, X-rays: binaries},
	Month = feb,
	Pages = {216-236},
	Primaryclass = {astro-ph.HE},
	Title = {{Theory of quasi-spherical accretion in X-ray pulsars}},
	Volume = 420,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.20026.x}}

@article{shakura13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428..670S},
	Archiveprefix = {arXiv},
	Author = {{Shakura}, N. and {Postnov}, K. and {Hjalmarsdotter}, L.},
	Doi = {10.1093/mnras/sts062},
	Eprint = {1209.4962},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, pulsars: general, X-rays: binaries},
	Month = jan,
	Pages = {670-677},
	Primaryclass = {astro-ph.HE},
	Title = {{On the nature of `off' states in slowly rotating low-luminosity X-ray pulsars}},
	Volume = 428,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/sts062}}

@article{shannon13,
   author = {{Shannon}, R.~M. and {Johnston}, S.},
    title = "{Radio properties of the magnetar near Sagittarius A* from observations with the Australia Telescope Compact Array}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.3036},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: PSR J1745-2900, ISM: structure, Galaxy: centre},
     year = 2013,
    month = aug,
   volume = 435,
    pages = {L29-L32},
      doi = {10.1093/mnrasl/slt088},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435L..29S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{shapiro83,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1983bhwd.book.....S&db_key=AST},
	Author = {{Shapiro}, S.~L. and {Teukolsky}, S.~A.},
	Publisher = {Research supported by the National Science Foundation.~New York, Wiley-Interscience, 1983, 663 p.},
	Title = {{Black holes, white dwarfs, and neutron stars: The physics of compact objects}},
	Year = 1983}

@article{shaposhnikov09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699..453S},
	Archiveprefix = {arXiv},
	Author = {{Shaposhnikov}, N. and {Titarchuk}, L.},
	Doi = {10.1088/0004-637X/699/1/453},
	Eprint = {0902.2852},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, radiation mechanisms: non-thermal, stars: individual: XTE J1550 {\ndash} 564 H 1743 {\ndash} 322 GX 339 {\ndash} 4 4U 1630 {\ndash} 47 GRS 1915+105 XTE 1650 {\ndash} 500 XTE 1859+226 4U 1543 {\ndash} 47},
	Month = jul,
	Pages = {453-468},
	Primaryclass = {astro-ph.HE},
	Title = {{Determination of Black Hole Masses in Galactic Black Hole Binaries Using Scaling of Spectral and Variability Characteristics}},
	Volume = 699,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/699/1/453}}

@article{shaw09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...495..733S},
	Archiveprefix = {arXiv},
	Author = {{Shaw Greening}, L. and {Barnard}, R. and {Kolb}, U. and {Tonkin}, C. and {Osborne}, J.~P.},
	Doi = {10.1051/0004-6361/200809864},
	Eprint = {0806.0074},
	Journal = {\aap},
	Keywords = {galaxies: individual: M 31, X-rays: general, X-rays: binaries},
	Month = mar,
	Pages = {733-741},
	Title = {{An X-ray spectral survey of the disc of M 31 with XMM-Newton}},
	Volume = 495,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200809864}}

@ARTICLE{shen19,
       author = {{Shen}, >Rong-Feng},
        title = "{Fast, Ultraluminous X-Ray Bursts from Tidal Stripping of White Dwarfs by Intermediate-mass Black Holes}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, hydrodynamics, stars: black holes, white dwarfs, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2019,
        month = jan,
       volume = {871},
       number = {1},
          eid = {L17},
        pages = {L17},
          doi = {10.3847/2041-8213/aafc64},
archivePrefix = {arXiv},
       eprint = {1809.09359},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...871L..17S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sheng21,
       author = {{Sheng}, Zhenfeng and {Wang}, Tinggui and {Ferland}, Gary and {Shu}, Xinwen and {Yang}, Chenwei and {Jiang}, Ning and {Chen}, Yang},
        title = "{Evidence of a Tidal-disruption Event in GSN 069 from the Abnormal Carbon and Nitrogen Abundance Ratio}",
      journal = {\apjl},
     keywords = {Active galactic nuclei, Active galaxies, 16, 17, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = oct,
       volume = {920},
       number = {1},
          eid = {L25},
        pages = {L25},
          doi = {10.3847/2041-8213/ac2251},
archivePrefix = {arXiv},
       eprint = {2109.01683},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920L..25S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shibata16,
   author = {{Shibata}, S. and {Watanabe}, E. and {Yatsu}, Y. and {Enoto}, T. and 
	{Bamba}, A.},
    title = "{X-Ray and Rotational Luminosity Correlation and Magnetic Heating of Radio Pulsars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1610.01705},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, stars: neutron, X-rays: general},
     year = 2016,
    month = dec,
   volume = 833,
      eid = {59},
    pages = {59},
      doi = {10.3847/1538-4357/833/1/59},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...833...59S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{shitov99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999IAUC.7110....2S&db_key=AST},
	Author = {{Shitov}, Y.~P.},
	Journal = {\iaucirc},
	Month = feb,
	Pages = {2},
	Title = {{SGR 1900+14 = PSR J1907+0919}},
	Volume = 7110,
	Year = 1999}

@article{shrader10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...718..488S},
	Archiveprefix = {arXiv},
	Author = {{Shrader}, C.~R. and {Titarchuk}, L. and {Shaposhnikov}, N.},
	Doi = {10.1088/0004-637X/718/1/488},
	Eprint = {1005.5362},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, radiation mechanisms: non-thermal, stars: individual: Cygnus X-3 GRS 1915+105},
	Month = jul,
	Pages = {488-493},
	Primaryclass = {astro-ph.HE},
	Title = {{New Evidence for a Black Hole in the Compact Binary Cygnus X-3}},
	Volume = 718,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/718/1/488}}

@ARTICLE{Shklovsky1967,
       author = {{Shklovsky}, I.~S.},
        title = "{On the Nature of the Source of X-Ray Emission of Sco XR-1.}",
      journal = {\apjl},
         year = 1967,
        month = apr,
       volume = {148},
        pages = {L1},
          doi = {10.1086/180001},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967ApJ...148L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shtykovskiy05,
   author = {{Shtykovskiy}, P.~E. and {Lutovinov}, A.~A. and {Gilfanov}, M.~R. and 
	{Sunyaev}, R.~A.},
    title = "{Constraints on the Luminosity of the Central Source in SNR 1987A}",
  journal = {Astronomy Letters},
   eprint = {astro-ph/0411731},
 keywords = {supernovae - pulsars},
     year = 2005,
    month = apr,
   volume = 31,
    pages = {258-262},
      doi = {10.1134/1.1896069},
   adsurl = {http://adsabs.harvard.edu/abs/2005AstL...31..258S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{sg05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362..879S},
	Author = {{Shtykovskiy}, P. and {Gilfanov}, M.},
	Doi = {10.1111/j.1365-2966.2005.09320.x},
	Eprint = {arXiv:astro-ph/0503477},
	Journal = {\mnras},
	Keywords = {stars: neutron, Magellanic Clouds, X-rays: binaries, X-rays: galaxies},
	Month = sep,
	Pages = {879-890},
	Title = {{High-mass X-ray binaries in the Small Magellanic Cloud: the luminosity function}},
	Volume = 362,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2005.09320.x}}

@article{shu11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...738..147S},
	Archiveprefix = {arXiv},
	Author = {{Shu}, X.~W. and {Yaqoob}, T. and {Wang}, J.~X.},
	Doi = {10.1088/0004-637X/738/2/147},
	Eid = {147},
	Eprint = {1107.0195},
	Journal = {\apj},
	Keywords = {galaxies: active, line: profiles, X-rays: galaxies},
	Month = sep,
	Pages = {147},
	Primaryclass = {astro-ph.CO},
	Title = {{Chandra High-energy Grating Observations of the Fe K{$\alpha$} Line Core in Type II Seyfert Galaxies: A Comparison with Type I Nuclei}},
	Volume = 738,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/738/2/147}}

@article{sidoli05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...440.1033S},
	Author = {{Sidoli}, L. and {Mereghetti}, S. and {Larsson}, S. and {Chernyakova}, M. and {Kreykenbohm}, I. and {Kretschmar}, P. and {Paizis}, A. and {Santangelo}, A. and {Ferrigno}, C. and {Falanga}, M.},
	Doi = {10.1051/0004-6361:20052961},
	Eprint = {arXiv:astro-ph/0505532},
	Journal = {\aap},
	Keywords = {X-rays: individuals: SAX J2103.5+4545, X-rays: binaries, stars: neutron, accretion, accretion disks},
	Month = sep,
	Pages = {1033-1039},
	Title = {{A large spin-up rate measured with INTEGRAL in the high mass X-ray binary pulsar SAX J2103.5+4545}},
	Volume = 440,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052961}}

@article{sidoli06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2006A%26A...459..901S&db_key=AST},
	Author = {{Sidoli}, L. and {Pellizzoni}, A. and {Vercellone}, S. and {Moroni}, M. and {Mereghetti}, S. and {Tavani}, M.},
	Doi = {10.1051/0004-6361:20065933},
	Eprint = {astro-ph/0606722},
	Journal = {\aap},
	Month = dec,
	Pages = {901-907},
	Title = {{XMM-Newton observation of a spectral state transition in the peculiar radio/X-ray/{$\gamma$}-ray source LS I +61 303}},
	Volume = 459,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20065933}}

@ARTICLE{sidoli17,
   author = {{Sidoli}, L. and {Israel}, G.~L. and {Esposito}, P. and {Rodr{\'{\i}}guez Castillo}, G.~A. and 
	{Postnov}, K.},
    title = "{AX J1910.7+0917: the slowest X-ray pulsar}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1705.01791},
 primaryClass = "astro-ph.HE",
 keywords = {stars: neutron, pulsars: general, X-rays: binaries, X-rays: individual: AX J1910.7+0917, CXOU J191043.7+091629, 2XMM J191043.4+091629, pulsars: general - X-rays: binaries},
     year = 2017,
    month = aug,
   volume = 469,
    pages = {3056-3061},
      doi = {10.1093/mnras/stx1105},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.469.3056S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{silverman08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678L..17S},
	Archiveprefix = {arXiv},
	Author = {{Silverman}, J.~M. and {Filippenko}, A.~V.},
	Doi = {10.1086/588096},
	Eprint = {0802.2716},
	Journal = {\apjl},
	Keywords = {Black Hole Physics, Galaxies: Starburst, Stars: Wolf-Rayet, X-Rays: Binaries},
	Month = may,
	Pages = {L17-L20},
	Title = {{On IC 10 X-1, the Most Massive Known Stellar-Mass Black Hole}},
	Volume = 678,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/588096}}

@ARTICLE{sivakoff05,
       author = {{Sivakoff}, Gregory R. and {Sarazin}, Craig L. and {Jord{\'a}n}, Andr{\'e}s},
        title = "{Luminous X-Ray Flares from Low-Mass X-Ray Binary Candidates in the Early-Type Galaxy NGC 4697}",
      journal = {\apjl},
     keywords = {Stars: Binaries: Close, Galaxies: Elliptical and Lenticular, cD, Galaxies: Individual: NGC Number: NGC 4697, X-Rays: Binaries, X-Rays: Bursts, X-Rays: Galaxies, Astrophysics},
         year = 2005,
        month = may,
       volume = {624},
       number = {1},
        pages = {L17-L20},
          doi = {10.1086/430374},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503195},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...624L..17S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{sivakoff08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677L..27S},
	Archiveprefix = {arXiv},
	Author = {{Sivakoff}, G.~R. and {Kraft}, R.~P. and {Jord{\'a}n}, A. and {Juett}, A.~M. and {Evans}, D.~A. and {Forman}, W.~R. and {Hardcastle}, M.~J. and {Sarazin}, C.~L. and {Birkinshaw}, M. and {Brassington}, N.~J. and {Croston}, J.~H. and {Harris}, W.~E. and {Jones}, C. and {Murray}, S.~S. and {Raychaudhury}, S. and {Woodley}, K.~A. and {Worrall}, D.~M.},
	Doi = {10.1086/587960},
	Eprint = {0803.0549},
	Journal = {\apjl},
	Keywords = {Stars: Binaries: Close, Galaxies: Elliptical and Lenticular, cD, Galaxies: Individual: Name: Centaurus A, Galaxies: Individual: NGC Number: NGC 5128, X-Rays: Binaries},
	Month = apr,
	Pages = {L27-L30},
	Title = {{A Transient Black Hole Low-Mass X-Ray Binary Candidate in Centaurus A}},
	Volume = 677,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587960}}

@article{siwek17,
   author = {{Siwek}, M. and {S{\c a}dowski}, A. and {Narayan}, R. and {Roberts}, T.~P. and 
	{Soria}, R.},
    title = "{Optical and X-ray luminosities of expanding nebulae around ultraluminous X-ray sources}",
  journal = {\mnras},
 keywords = {accretion, accretion discs, black hole physics, relativistic processes, methods: numerical, ISM: bubbles, X-rays: binaries},
     year = 2017,
    month = sep,
   volume = 470,
    pages = {361-371},
      doi = {10.1093/mnras/stx1185},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.470..361S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{skinner80,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1980Natur.288..141S},
	Author = {{Skinner}, G.~K.},
	Journal = {\nat},
	Month = nov,
	Pages = {141-143},
	Title = {{Observations of optical flares in the recurrent X-ray transient A0538-66}},
	Volume = 288,
	Year = 1980}

@article{skinner82,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1982Natur.297..568S},
	Author = {{Skinner}, G.~K. and {Bedford}, D.~K. and {Elsner}, R.~F. and {Leahy}, D. and {Weisskopf}, M.~C. and {Grindlay}, J.},
	Journal = {\nat},
	Month = jun,
	Pages = {568-570},
	Title = {{Discovery of 69 MS periodic X-ray pulsations in A0538-66}},
	Volume = 297,
	Year = 1982}

@article{skrutskie06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006AJ....131.1163S},
	Author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and {Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and {Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and {Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and {Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and {Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and {Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and {Wheelock}, S.},
	Doi = {10.1086/498708},
	Journal = {\aj},
	Month = feb,
	Pages = {1163-1183},
	Title = {{The Two Micron All Sky Survey (2MASS)}},
	Volume = 131,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/498708}}

@article{slane99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1999ApJ...525..357S},
	Author = {{Slane}, P. and {Gaensler}, B.~M. and {Dame}, T.~M. and {Hughes}, J.~P. and {Plucinsky}, P.~P. and {Green}, A.},
	Doi = {10.1086/307893},
	Eprint = {arXiv:astro-ph/9906364},
	Journal = {\apj},
	Month = nov,
	Pages = {357-367},
	Title = {{Nonthermal X-Ray Emission from the Shell-Type Supernova Remnant G347.3-0.5}},
	Volume = 525,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/307893}}

@article{slane01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...548..814S},
	Author = {{Slane}, P. and {Hughes}, J.~P. and {Edgar}, R.~J. and {Plucinsky}, P.~P. and {Miyata}, E. and {Tsunemi}, H. and {Aschenbach}, B.},
	Doi = {10.1086/319033},
	Eprint = {arXiv:astro-ph/0010510},
	Journal = {\apj},
	Keywords = {ISM: Individual: Alphanumeric: G266.2-1.2, Radiation Mechanisms: Nonthermal, ISM: Supernova Remnants, X-Rays: ISM},
	Month = feb,
	Pages = {814-819},
	Title = {{RX J0852.0-4622: Another Nonthermal Shell-Type Supernova Remnant (G266.2-1.2)}},
	Volume = 548,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/319033}}

@article{slane05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005AdSpR..35.1092S&db_key=AST},
	Author = {{Slane}, P.},
	Doi = {10.1016/j.asr.2005.04.029},
	Eprint = {astro-ph/0504108},
	Journal = {Advances in Space Research},
	Pages = {1092-1098},
	Title = {{The devil is in the details: Compact structures in pulsar wind nebulae}},
	Volume = 35,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.asr.2005.04.029}}

@article{smith98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301..767S},
	Author = {{Smith}, D.~A. and {Dhillon}, V.~S.},
	Doi = {10.1046/j.1365-8711.1998.02065.x},
	Eprint = {astro-ph/9808217},
	Journal = {\mnras},
	Keywords = {BINARIES: CLOSE, STARS: LATE-TYPE, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
	Month = dec,
	Pages = {767-781},
	Title = {{The secondary stars in cataclysmic variables and low-mass X-ray binaries}},
	Volume = 301,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.02065.x}}

@article{smith99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...519L.147S&db_key=AST},
	Author = {{Smith}, D.~A. and {Bradt}, H.~V. and {Levine}, A.~M.},
	Doi = {10.1086/312121},
	Journal = {\apjl},
	Month = jul,
	Pages = {L147-L150},
	Title = {{Rossi X-Ray Timing Explorer All-Sky Monitor Localization of SGR 1627-41}},
	Volume = 519,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312121}}

@article{smith01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556L..91S},
	Author = {{Smith}, R.~K. and {Brickhouse}, N.~S. and {Liedahl}, D.~A. and {Raymond}, J.~C.},
	Doi = {10.1086/322992},
	Eprint = {arXiv:astro-ph/0106478},
	Journal = {\apjl},
	Month = aug,
	Pages = {L91-L95},
	Title = {{Collisional Plasma Models with APEC/APED: Emission-Line Diagnostics of Hydrogen-like and Helium-like Ions}},
	Volume = 556,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/322992}}

@article{sw01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...557..180S},
	Author = {{Smith}, D.~A. and {Wilson}, A.~S.},
	Doi = {10.1086/321667},
	Eprint = {astro-ph/0104252},
	Journal = {\apj},
	Keywords = {Galaxies: Active, Galaxies: Individual: Name: Circinus, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, X-Rays: Galaxies},
	Month = aug,
	Pages = {180-192},
	Title = {{A Chandra Observation of the Circinus Galaxy}},
	Volume = 557,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/321667}}

@article{smith06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ConPh..47..363S},
	Author = {{Smith}, R.~C.},
	Doi = {10.1080/00107510601181175},
	Journal = {Contemporary Physics},
	Month = nov,
	Pages = {363-386},
	Title = {{Cataclysmic variables}},
	Volume = 47,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1080/00107510601181175}}

@article{smith12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012AJ....143..144S},
	Archiveprefix = {arXiv},
	Author = {{Smith}, B.~J. and {Swartz}, D.~A. and {Miller}, O. and {Burleson}, J.~A. and {Nowak}, M.~A. and {Struck}, C.},
	Doi = {10.1088/0004-6256/143/6/144},
	Eid = {144},
	Eprint = {1204.3194},
	Journal = {\aj},
	Keywords = {galaxies: interactions, galaxies: starburst, ultraviolet: galaxies, X-rays: galaxies},
	Month = jun,
	Pages = {144},
	Primaryclass = {astro-ph.CO},
	Title = {{ChAInGeS: The Chandra Arp Interacting Galaxies Survey}},
	Volume = 143,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/143/6/144}}

@ARTICLE{sniegowska20,
       author = {{Sniegowska}, M. and {Czerny}, B. and {Bon}, E. and {Bon}, N.},
        title = "{Possible mechanism for multiple changing-look phenomena in active galactic nuclei}",
      journal = {\aap},
     keywords = {accretion, accretion disks, galaxies: active, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A167},
        pages = {A167},
          doi = {10.1051/0004-6361/202038575},
archivePrefix = {arXiv},
       eprint = {2007.06441},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A.167S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{snowden02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2002astro.ph..3311S},
	Author = {{Snowden}, S.~L.},
	Eprint = {astro-ph/0203311},
	Journal = {preprint: astro-ph/0203311},
	Month = mar,
	Title = {{Comparison of XMM-Newton EPIC, Chandra ACIS-S3, ASCA SIS and GIS, and ROSAT PSPC Results for G21.5-0.9, 1E0102.2-7219, and MS1-54.4-0321}},
	Year = 2002}

@article{sofue09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..227S},
	Archiveprefix = {arXiv},
	Author = {{Sofue}, Y. and {Honma}, M. and {Omodaka}, T.},
	Eprint = {0811.0859},
	Journal = {\pasj},
	Keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: rotation curve, Galaxy: structure},
	Month = feb,
	Pages = {227-},
	Title = {{Unified Rotation Curve of the Galaxy -- Decomposition into de Vaucouleurs Bulge, Disk, Dark Halo, and the 9-kpc Rotation Dip --}},
	Volume = 61,
	Year = 2009}

@article{solheim10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010PASP..122.1133S},
	Author = {{Solheim}, J.-E.},
	Doi = {10.1086/656680},
	Journal = {\pasp},
	Keywords = {Reviews (Invited or Regular)},
	Month = oct,
	Pages = {1133-1163},
	Title = {{AM CVn Stars: Status and Challenges}},
	Volume = 122,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/656680}}

@article{somero12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A.111S},
	Archiveprefix = {arXiv},
	Author = {{Somero}, A. and {Hakala}, P. and {Muhli}, P. and {Charles}, P. and {Vilhu}, O.},
	Doi = {10.1051/0004-6361/201118439},
	Eid = {A111},
	Eprint = {1201.3461},
	Journal = {\aap},
	Keywords = {stars: individual: X1822-371, accretion, accretion disks, X-rays: binaries},
	Month = mar,
	Pages = {A111},
	Primaryclass = {astro-ph.SR},
	Title = {{Phase-resolved optical and X-ray spectroscopy of low-mass X-ray binary X1822-371}},
	Volume = 539,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201118439}}

@ARTICLE{sonneborn87,
   author = {{Sonneborn}, G. and {Altner}, B. and {Kirshner}, R.~P.},
    title = "{The progenitor of SN 1987A - Spatially resolved ultraviolet spectroscopy of the supernova field}",
  journal = {\apjl},
 keywords = {Astronomical Spectroscopy, Iue, Supernova 1987a, Gravitational Collapse, Spatial Resolution, Temporal Distribution, Ultraviolet Spectra},
     year = 1987,
    month = dec,
   volume = 323,
    pages = {L35-L39},
      doi = {10.1086/185052},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...323L..35S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{sonobe94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994ApJ...436L..23S&amp;db_key=AST},
	Author = {{Sonobe}, T. and {Murakami}, T. and {Kulkarni}, S.~R. and {Aoki}, T. and {Yoshida}, A.},
	Journal = {\apjl},
	Month = nov,
	Pages = {L23-L25},
	Title = {{Characteristics of the persistent emission of SGR 1806-20}},
	Volume = 436,
	Year = 1994}

@article{soria12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750..152S},
	Archiveprefix = {arXiv},
	Author = {{Soria}, R. and {Kuntz}, K.~D. and {Winkler}, P.~F. and {Blair}, W.~P. and {Long}, K.~S. and {Plucinsky}, P.~P. and {Whitmore}, B.~C.},
	Doi = {10.1088/0004-637X/750/2/152},
	Eid = {152},
	Eprint = {1203.2335},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, galaxies: individual: M83, X-rays: binaries},
	Month = may,
	Pages = {152},
	Primaryclass = {astro-ph.HE},
	Title = {{The Birth of an Ultraluminous X-Ray Source in M83}},
	Volume = 750,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/750/2/152}}

@ARTICLE{soria14,
   author = {{Soria}, R. and {Long}, K.~S. and {Blair}, W.~P. and {Godfrey}, L. and 
	{Kuntz}, K.~D. and {Lenc}, E. and {Stockdale}, C. and {Winkler}, P.~F.
	},
    title = "{Super-Eddington Mechanical Power of an Accreting Black Hole in M83}",
  journal = {Science},
     year = 2014,
    month = mar,
   volume = 343,
    pages = {1330-1333},
      doi = {10.1126/science.1248759},
   adsurl = {http://adsabs.harvard.edu/abs/2014Sci...343.1330S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{spitkovsky06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...648L..51S},
	Author = {{Spitkovsky}, A.},
	Doi = {10.1086/507518},
	Eprint = {arXiv:astro-ph/0603147},
	Journal = {\apjl},
	Keywords = {Magnetohydrodynamics: MHD, Stars: Pulsars: General, Stars: Magnetic Fields, Stars: Neutron},
	Month = sep,
	Pages = {L51-L54},
	Title = {{Time-dependent Force-free Pulsar Magnetospheres: Axisymmetric and Oblique Rotators}},
	Volume = 648,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507518}}

@article{springel01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001NewA....6...79S},
	Author = {{Springel}, V. and {Yoshida}, N. and {White}, S.~D.~M.},
	Doi = {10.1016/S1384-1076(01)00042-2},
	Eprint = {astro-ph/0003162},
	Journal = {\na},
	Month = apr,
	Pages = {79-117},
	Title = {{GADGET: a code for collisionless and gasdynamical cosmological simulations}},
	Volume = 6,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/S1384-1076(01)00042-2}}

@INPROCEEDINGS{spruit08,
   author = {{Spruit}, H.~C.},
    title = "{Origin of neutron star magnetic fields}",
 keywords = {Neutron stars, Gravitational radiation magnetic fields and other observations, Pulsars, Origin and evolution, Supernovae},
booktitle = {40 Years of Pulsars: Millisecond Pulsars, Magnetars and More},
     year = 2008,
   series = {American Institute of Physics Conference Series},
   volume = 983,
archivePrefix = "arXiv",
   eprint = {0711.3650},
   editor = {{Bassa}, C. and {Wang}, Z. and {Cumming}, A. and {Kaspi}, V.~M.
	},
    month = feb,
    pages = {391-398},
      doi = {10.1063/1.2900262},
   adsurl = {http://adsabs.harvard.edu/abs/2008AIPC..983..391S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{staff06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645L.145S},
	Author = {{Staff}, J.~E. and {Ouyed}, R. and {Jaikumar}, P.},
	Doi = {10.1086/506255},
	Eprint = {arXiv:astro-ph/0603743},
	Journal = {\apjl},
	Keywords = {Dense Matter, Equation of State, Magnetic Fields, Stars: Neutron},
	Month = jul,
	Pages = {L145-L148},
	Title = {{Quark Deconfinement in Neutron Star Cores: The Effects of Spin-down}},
	Volume = 645,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506255}}

@article{stanek98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...503L.131S},
	Author = {{Stanek}, K.~Z. and {Garnavich}, P.~M.},
	Doi = {10.1086/311539},
	Eprint = {arXiv:astro-ph/9802121},
	Journal = {\apjl},
	Keywords = {GALAXY: CENTER, GALAXIES: INDIVIDUAL MESSIER NUMBER: M31, GALAXIES: DISTANCES AND REDSHIFTS, SOLAR SYSTEM: GENERAL, STARS: HORIZONTAL-BRANCH},
	Month = aug,
	Pages = {L131},
	Title = {{Distance to M31 with the Hubble Space Telescope and HIPPARCOS Red Clump Stars}},
	Volume = 503,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/311539}}
	
@ARTICLE{stasinska13,
       author = {{Stasi{\'n}ska}, G. and {Pe{\~n}a}, M. and {Bresolin}, F. and
         {Tsamis}, Y.~G.},
        title = "{Planetary nebulae and H ii regions in the spiral galaxy NGC 300. Clues on the evolution of abundance gradients and on AGB nucleosynthesis}",
      journal = {\aap},
     keywords = {planetary nebulae: general, Hiiregions, stars: AGB and post-AGB, galaxies: abundances, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2013",
        month = "Apr",
       volume = {552},
          eid = {A12},
        pages = {A12},
          doi = {10.1051/0004-6361/201220345},
archivePrefix = {arXiv},
       eprint = {1301.5280},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...552A..12S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{staubert07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...465L..25S},
	Author = {{Staubert}, R. and {Shakura}, N.~I. and {Postnov}, K. and {Wilms}, J. and {Rothschild}, R.~E. and {Coburn}, W. and {Rodina}, L. and {Klochkov}, D.},
	Doi = {10.1051/0004-6361:20077098},
	Eprint = {arXiv:astro-ph/0702490},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, binaries: eclipsing, stars: neutron, X-rays: binaries, X-rays: stars},
	Month = apr,
	Pages = {L25-L28},
	Title = {{Discovery of a flux-related change of the cyclotron line energy in Hercules X-1}},
	Volume = 465,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20077098}}

@article{staveley96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996PASA...13..243S},
	Author = {{Staveley-Smith}, L. and {Wilson}, W.~E. and {Bird}, T.~S. and {Disney}, M.~J. and {Ekers}, R.~D. and {Freeman}, K.~C. and {Haynes}, R.~F. and {Sinclair}, M.~W. and {Vaile}, R.~A. and {Webster}, R.~L. and {Wright}, A.~E.},
	Journal = {Publications of the Astronomical Society of Australia},
	Keywords = {INSTRUMENTATION, RECEIVERS},
	Month = nov,
	Pages = {243-248},
	Title = {{The Parkes 21 CM multibeam receiver}},
	Volume = 13,
	Year = 1996}

@article{stephen05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...432L..49S},
	Author = {{Stephen}, J.~B. and {Bassani}, L. and {Molina}, M. and {Malizia}, A. and {Bazzano}, A. and {Ubertini}, P. and {Dean}, A.~J. and {Bird}, A.~J. and {Lebrun}, F. and {Much}, R. and {Walter}, R.},
	Doi = {10.1051/0004-6361:200500017},
	Eprint = {arXiv:astro-ph/0502158},
	Journal = {\aap},
	Keywords = {catalogues, surveys, gamma-rays: observations},
	Month = mar,
	Pages = {L49-L52},
	Title = {{Using the ROSAT Bright Source Catalogue to find counterparts for IBIS/ISGRI survey sources}},
	Volume = 432,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500017}}

@article{stiele11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A..55S},
	Archiveprefix = {arXiv},
	Author = {{Stiele}, H. and {Pietsch}, W. and {Haberl}, F. and {Hatzidimitriou}, D. and {Barnard}, R. and {Williams}, B.~F. and {Kong}, A.~K.~H. and {Kolb}, U.},
	Doi = {10.1051/0004-6361/201015270},
	Eid = {A55},
	Eprint = {1106.4755},
	Journal = {\aap},
	Keywords = {galaxies: individual:M 31, X-rays: galaxies},
	Month = oct,
	Pages = {A55},
	Primaryclass = {astro-ph.HE},
	Title = {{The deep XMM-Newton Survey of M 31}},
	Volume = 534,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201015270}}

@ARTICLE{stiele19,
       author = {{Stiele}, H. and {Kong}, A.~K.~H.},
        title = "{Peculiar Outbursts of an Ultra-luminous Source: Likely Signs of an Aperiodic Disk-wind}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 4472, X-rays: binaries, X-rays: individual: XMMU 122939.7+075333},
         year = 2019,
        month = jun,
       volume = {877},
       number = {2},
          eid = {115},
        pages = {115},
          doi = {10.3847/1538-4357/ab1e4b},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...877..115S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{stobbart06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368..397S},
	Author = {{Stobbart}, A.-M. and {Roberts}, T.~P. and {Wilms}, J.},
	Doi = {10.1111/j.1365-2966.2006.10112.x},
	Eprint = {arXiv:astro-ph/0601651},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, X-rays: binaries, X-rays: galaxies},
	Month = may,
	Pages = {397-413},
	Title = {{XMM-Newton observations of the brightest ultraluminous X-ray sources}},
	Volume = 368,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2006.10112.x}}

@article{strohmayer00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...537L.111S&db_key=AST},
	Author = {{Strohmayer}, T.~E. and {Ibrahim}, A.~I.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L111-L114},
	Title = {{Discovery of a 6.4 KEV Emission Line in a Burst from SGR 1900+14}},
	Volume = 537,
	Year = 2000}

@article{strohmayer02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...581..577S},
	Author = {{Strohmayer}, T.~E.},
	Doi = {10.1086/344101},
	Eprint = {arXiv:astro-ph/0204128},
	Journal = {\apj},
	Keywords = {Stars: Binaries: General, Stars: Novae, Cataclysmic Variables, Stars: Individual: Alphanumeric: RX J1914.4+2456, Stars: White Dwarfs, X-Rays: Binaries, X-Rays: Stars},
	Month = dec,
	Pages = {577-584},
	Title = {{Evidence for Orbital Decay of RX J1914.4+2456: Gravitational Radiation and the Nature of the X-Ray Emission}},
	Volume = 581,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/344101}}

@article{strohmayer03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...593L..39S},
	Author = {{Strohmayer}, T.~E.},
	Doi = {10.1086/378061},
	Eprint = {arXiv:astro-ph/0306593},
	Journal = {\apjl},
	Keywords = {Stars: Binaries: Close, Gravitational Waves, Stars: Individual: Alphanumeric: RX J0806.3+1527, Stars: Individual: Alphanumeric: RX J1914.4+2456, Stars: White Dwarfs, X-Rays: Binaries},
	Month = aug,
	Pages = {L39-L42},
	Title = {{Phase Coherent Timing of RX J0806.3+1527 with ROSAT and Chandra}},
	Volume = 593,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/378061}}

@article{sm03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586L..61S},
	Author = {{Strohmayer}, T.~E. and {Mushotzky}, R.~F.},
	Doi = {10.1086/374732},
	Eprint = {arXiv:astro-ph/0303665},
	Journal = {\apjl},
	Keywords = {Black Hole Physics, Galaxies: Individual: Messier Number: M82, Galaxies: Starburst, Stars: Oscillations, X-Rays: Galaxies, X-Rays: Stars},
	Month = mar,
	Pages = {L61-L64},
	Title = {{Discovery of X-Ray Quasi-periodic Oscillations from an Ultraluminous X-Ray Source in M82: Evidence against Beaming}},
	Volume = 586,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/374732}}

@article{strohmayer05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...627..920S},
	Author = {{Strohmayer}, T.~E.},
	Doi = {10.1086/430439},
	Eprint = {arXiv:astro-ph/0504150},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Close, Gravitational Waves, Stars: Individual: Alphanumeric: RX J0806.3+1527, Stars: Individual: Constellation Name: V407 Vulpeculae, Stars: White Dwarfs, X-Rays: Binaries},
	Month = jul,
	Pages = {920-925},
	Title = {{Precision X-Ray Timing of RX J0806.3+1527 with Chandra: Evidence for Gravitational Radiation from an Ultracompact Binary}},
	Volume = 627,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/430439}}

@ARTICLE{sw05,
   author = {{Strohmayer}, T.~E. and {Watts}, A.~L.},
    title = "{Discovery of Fast X-Ray Oscillations during the 1998 Giant Flare from SGR 1900+14}",
  journal = {\apjl},
   eprint = {astro-ph/0508206},
 keywords = {Stars: Pulsars: Individual: Alphanumeric: SGR 1900+14, Stars: Magnetic Fields, Stars: Neutron, Stars: Oscillations, Stars: Rotation, X-Rays: Stars},
     year = 2005,
    month = oct,
   volume = 632,
    pages = {L111-L114},
      doi = {10.1086/497911},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...632L.111S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{strohmayer06,
   author = {{Strohmayer}, T.~E. and {Watts}, A.~L.},
    title = "{The 2004 Hyperflare from SGR 1806-20: Further Evidence for Global Torsional Vibrations}",
  journal = {\apj},
   eprint = {astro-ph/0608463},
 keywords = {Stars: Pulsars: Individual: Alphanumeric: SGR 1806-20, Stars: Magnetic Fields, Stars: Neutron, Stars: Oscillations, Stars: Rotation, X-Rays: Stars},
     year = 2006,
    month = dec,
   volume = 653,
    pages = {593-601},
      doi = {10.1086/508703},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653..593S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{strohmayer07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660..580S},
	Author = {{Strohmayer}, T.~E. and {Mushotzky}, R.~F. and {Winter}, L. and {Soria}, R. and {Uttley}, P. and {Cropper}, M.},
	Doi = {10.1086/512723},
	Eprint = {arXiv:astro-ph/0701390},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Galaxies: Individual: NGC Number: NGC 5408, Stars: Oscillations, X-Rays: Galaxies, X-Rays: Stars},
	Month = may,
	Pages = {580-586},
	Title = {{Quasi-periodic Variability in NGC 5408 X-1}},
	Volume = 660,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/512723}}

@article{strohmayer08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...679L.109S},
	Author = {{Strohmayer}, T.~E.},
	Doi = {10.1086/589439},
	Journal = {\apjl},
	Keywords = {Stars: Binaries: Close, Gravitational Waves, Stars: Individual: Alphanumeric: RX J0806.3+1527, Stars: Individual: Constellation Name: V407 Vulpeculae, Stars: White Dwarfs, X-Rays: Binaries},
	Month = jun,
	Pages = {L109-L112},
	Title = {{High-Resolution X-Ray Spectroscopy of RX J0806.3+1527 with Chandra}},
	Volume = 679,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/589439}}

@article{strohmayer09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...703.1386S},
	Archiveprefix = {arXiv},
	Author = {{Strohmayer}, T.~E. and {Mushotzky}, R.~F.},
	Doi = {10.1088/0004-637X/703/2/1386},
	Eprint = {0911.1076},
	Journal = {\apj},
	Keywords = {black hole physics, galaxies: individual: NGC 5408, stars: oscillations, X-rays: stars, X-rays: galaxies},
	Month = oct,
	Pages = {1386-1393},
	Primaryclass = {astro-ph.HE},
	Title = {{Evidence for an Intermediate-mass Black Hole in NGC 5408 X-1}},
	Volume = 703,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/703/2/1386}}

@article{struder01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001A%26A...365L..18S&db_key=AST},
	Author = {{Str{\"u}der}, L. and {Briel}, U. and {Dennerl}, K. and {Hartmann}, R. and {Kendziorra}, E. and {Meidinger}, N. and {Pfeffermann}, E. and {Reppin}, C. and {Aschenbach}, B. and {Bornemann}, W. and {Br{\"a}uninger}, H. and {Burkert}, W. and {Elender}, M. and {Freyberg}, M. and {Haberl}, F. and {Hartner}, G. and {Heuschmann}, F. and {Hippmann}, H. and {Kastelic}, E. and {Kemmer}, S. and {Kettenring}, G. and {Kink}, W. and {Krause}, N. and {M{\"u}ller}, S. and {Oppitz}, A. and {Pietsch}, W. and {Popp}, M. and {Predehl}, P. and {Read}, A. and {Stephan}, K.~H. and {St{\"o}tter}, D. and {Tr{\"u}mper}, J. and {Holl}, P. and {Kemmer}, J. and {Soltau}, H. and {St{\"o}tter}, R. and {Weber}, U. and {Weichert}, U. and {von Zanthier}, C. and {Carathanassis}, D. and {Lutz}, G. and {Richter}, R.~H. and {Solc}, P. and {B{\"o}ttcher}, H. and {Kuster}, M. and {Staubert}, R. and {Abbey}, A. and {Holland}, A. and {Turner}, M. and {Balasini}, M. and {Bignami}, G.~F. and {La Palombara}, N. and {Villa}, G. and {Buttler}, W. and {Gianini}, F. and {Lain{\'e}}, R. and {Lumb}, D. and {Dhez}, P.},
	Doi = {10.1051/0004-6361:20000066},
	Journal = {\aap},
	Month = jan,
	Pages = {L18-L26},
	Title = {{The European Photon Imaging Camera on XMM-Newton: The pn-CCD camera}},
	Volume = 365,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000066}}

@article{struve31,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1931ApJ....73...94S},
	Author = {{Struve}, O.},
	Doi = {10.1086/143298},
	Journal = {\apj},
	Month = mar,
	Pages = {94},
	Title = {{On the Origin of Bright Lines in Spectra of Stars of Class B}},
	Volume = 73,
	Year = 1931,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/143298}}

@article{suchkov04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...612..437S},
	Author = {{Suchkov}, A.~A. and {Hanisch}, R.~J.},
	Doi = {10.1086/422544},
	Journal = {\apj},
	Keywords = {Galaxy: Globular Clusters: General, Methods: Statistical, Surveys, X-Rays: Binaries, X-Rays: General, X-Rays: Stars},
	Month = sep,
	Pages = {437-446},
	Title = {{ClassX Detection of Candidate Low-Luminosity Hard X-Ray Binaries}},
	Volume = 612,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422544}}

@article{sugizaki97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1997PASJ...49L..25S},
	Author = {{Sugizaki}, M. and {Nagase}, F. and {Torii}, K. and {Kinugasa}, K. and {Asanuma}, T. and {Matsuzaki}, K. and {Koyama}, K. and {Yamauchi}, S.},
	Journal = {\pasj},
	Month = oct,
	Pages = {L25-L30},
	Title = {{Discovery of an 11-s X-Ray Pulsar in the Galactic-Plane Section of the Scorpius Constellation}},
	Volume = 49,
	Year = 1997}

@article{sugizaki01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJS..134...77S&db_key=AST},
	Author = {{Sugizaki}, M. and {Mitsuda}, K. and {Kaneda}, H. and {Matsuzaki}, K. and {Yamauchi}, S. and {Koyama}, K.},
	Doi = {10.1086/320358},
	Journal = {\apjs},
	Month = may,
	Pages = {77-102},
	Title = {{Faint X-Ray Sources Resolved in the ASCA Galactic Plane Survey and Their Contribution to the Galactic Ridge X-Ray Emission}},
	Volume = 134,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/320358}}

@article{suleimanov10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714..630S},
	Archiveprefix = {arXiv},
	Author = {{Suleimanov}, V.~F. and {Pavlov}, G.~G. and {Werner}, K.},
	Doi = {10.1088/0004-637X/714/1/630},
	Eprint = {1001.0973},
	Journal = {\apj},
	Keywords = {pulsars: individual: 1E 1207.4-5209 PSR J1852+0040 PSR J0821-4300, radiative transfer, stars: magnetic field, stars: neutron},
	Month = may,
	Pages = {630-635},
	Primaryclass = {astro-ph.HE},
	Title = {{Quantum Nature of Cyclotron Harmonics in Thermal Spectra of Neutron Stars}},
	Volume = 714,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/714/1/630}}

@article{shp10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...522A.111S},
	Archiveprefix = {arXiv},
	Author = {{Suleimanov}, V. and {Hambaryan}, V. and {Potekhin}, A.~Y. and {van Adelsberg}, M. and {Neuh{\"a}user}, R. and {Werner}, K.},
	Doi = {10.1051/0004-6361/200913641},
	Eid = {A111},
	Eprint = {1006.3292},
	Journal = {\aap},
	Keywords = {radiative transfer, scattering, methods: numerical, stars: neutron, stars: atmospheres, X-rays: stars},
	Month = nov,
	Pages = {A111},
	Primaryclass = {astro-ph.HE},
	Title = {{Radiative properties of highly magnetized isolated neutron star surfaces and approximate treatment of absorption features in their spectra}},
	Volume = 522,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200913641}}

@article{suleimanov12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...15S},
	Archiveprefix = {arXiv},
	Author = {{Suleimanov}, V.~F. and {Pavlov}, G.~G. and {Werner}, K.},
	Doi = {10.1088/0004-637X/751/1/15},
	Eid = {15},
	Eprint = {1201.5527},
	Journal = {\apj},
	Keywords = {pulsars: individual: 1E 1207.4-5209 PSR J1210 5226 PSR J1852+0040 PSR J0822-4300, radiation mechanisms: thermal, radiative transfer, stars: magnetic field, stars: neutron},
	Month = may,
	Pages = {15},
	Primaryclass = {astro-ph.HE},
	Title = {{Magnetized Neutron Star Atmospheres: Beyond the Cold Plasma Approximation}},
	Volume = 751,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/751/1/15}}

@article{sunyaev93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...407..606S},
	Author = {{Sunyaev}, R.~A. and {Markevitch}, M. and {Pavlinsky}, M.},
	Doi = {10.1086/172542},
	Journal = {\apj},
	Keywords = {GALACTIC NUCLEI, INTERSTELLAR GAS, MILKY WAY GALAXY, SPACEBORNE ASTRONOMY, ASTRONOMICAL SPECTROSCOPY, BREMSSTRAHLUNG, EMISSION SPECTRA, ENERGY BANDS, MOLECULAR GASES, X RAY SPECTRA},
	Month = apr,
	Pages = {606-610},
	Title = {{The center of the Galaxy in the recent past - A view from GRANAT}},
	Volume = 407,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/172542}}

@article{sunyaev98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.297.1279S},
	Author = {{Sunyaev}, R. and {Churazov}, E.},
	Doi = {10.1046/j.1365-8711.1998.01684.x},
	Eprint = {arXiv:astro-ph/9805038},
	Journal = {\mnras},
	Keywords = {LINE: FORMATION, ISM: INDIVIDUAL: SGR B, GALAXY: CENTRE, X-RAYS: GENERAL},
	Month = jul,
	Pages = {1279-1291},
	Title = {{Equivalent width, shape and proper motion of the iron fluorescent line emission from molecular clouds as an indicator of the illuminating source X-ray flux history}},
	Volume = 297,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.1998.01684.x}}

@article{supper01,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...373...63S},
	Author = {{Supper}, R. and {Hasinger}, G. and {Lewin}, W.~H.~G. and {Magnier}, E.~A. and {van Paradijs}, J. and {Pietsch}, W. and {Read}, A.~M. and {Tr{\"u}mper}, J.},
	Doi = {10.1051/0004-6361:20010495},
	Eprint = {astro-ph/0104297},
	Journal = {\aap},
	Keywords = {GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: INDIVIDUAL: M 31, GALAXIES: SPIRAL, X-RAYS: GALAXIES},
	Month = jul,
	Pages = {63-99},
	Title = {{The second ROSAT PSPC survey of M 31 and the complete ROSAT PSPC source list}},
	Volume = 373,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20010495}}

@article{sutton12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423.1154S},
	Archiveprefix = {arXiv},
	Author = {{Sutton}, A.~D. and {Roberts}, T.~P. and {Walton}, D.~J. and {Gladstone}, J.~C. and {Scott}, A.~E.},
	Doi = {10.1111/j.1365-2966.2012.20944.x},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, black hole physics, X rays: binaries, X rays: galaxies},
	Month = jun,
	Pages = {1154-1177},
	Title = {{The most extreme ultraluminous X-ray sources: evidence for intermediate-mass black holes?}},
	Volume = 423,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.20944.x}}

@article{swanenburg81,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...243L..69S},
	Author = {{Swanenburg}, B.~N. and {Bennett}, K. and {Bignami}, G.~F. and {Buccheri}, R. and {Caraveo}, P. and {Hermsen}, W. and {Kanbach}, G. and {Lichti}, G.~G. and {Masnou}, J.~L. and {Mayer-Hasselwander}, H.~A. and {Paul}, J.~A. and {Sacco}, B. and {Scarsi}, L. and {Wills}, R.~D.},
	Doi = {10.1086/183445},
	Journal = {\apjl},
	Month = jan,
	Pages = {L69-L73},
	Title = {{Second COS B catalog of high-energy gamma-ray sources}},
	Volume = 243,
	Year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/183445}}

@article{swartz04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154..519S},
	Author = {{Swartz}, D.~A. and {Ghosh}, K.~K. and {Tennant}, A.~F. and {Wu}, K.},
	Doi = {10.1086/422842},
	Eprint = {astro-ph/0405498},
	Journal = {\apjs},
	Keywords = {Galaxies: General, Surveys, X-Rays: Binaries, X-Rays: Galaxies, X-Rays: General},
	Month = oct,
	Pages = {519-539},
	Title = {{The Ultraluminous X-Ray Source Population from the Chandra Archive of Galaxies}},
	Volume = 154,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/422842}}

@article{swartz11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...49S},
	Archiveprefix = {arXiv},
	Author = {{Swartz}, D.~A. and {Soria}, R. and {Tennant}, A.~F. and {Yukita}, M.},
	Doi = {10.1088/0004-637X/741/1/49},
	Eid = {49},
	Eprint = {1108.1372},
	Journal = {\apj},
	Keywords = {galaxies: general, surveys, X-rays: binaries, X-rays: galaxies, X-rays: general},
	Month = nov,
	Pages = {49},
	Primaryclass = {astro-ph.HE},
	Title = {{A Complete Sample of Ultraluminous X-ray Source Host Galaxies}},
	Volume = 741,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/741/1/49}}

@article{szostek08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..593S},
	Archiveprefix = {arXiv},
	Author = {{Szostek}, A. and {Zdziarski}, A.~A.},
	Doi = {10.1111/j.1365-2966.2008.13073.x},
	Eprint = {0710.5591},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , binaries: general , stars: individual: Cyg X-3 , X-rays: binaries , X-rays: individual: Cyg X-3 , X-rays: stars},
	Month = may,
	Pages = {593-607},
	Title = {{Effects of the stellar wind on X-ray spectra of Cygnus X-3}},
	Volume = 386,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13073.x}}

@article{szm08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1001S},
	Archiveprefix = {arXiv},
	Author = {{Szostek}, A. and {Zdziarski}, A.~A. and {McCollough}, M.~L.},
	Doi = {10.1111/j.1365-2966.2008.13479.x},
	Eprint = {0803.2217},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , binaries: general , stars: individual: Cyg X-3 , radio continuum: stars , X-rays: binaries , X-rays: stars},
	Month = aug,
	Pages = {1001-1010},
	Title = {{A classification of the X-ray and radio states of Cyg X-3 and their long-term correlations}},
	Volume = 388,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2008.13479.x}}

@article{taam88,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...331L.117T},
	Author = {{Taam}, R.~E. and {Brown}, D.~A. and {Fryxell}, B.~A.},
	Doi = {10.1086/185248},
	Journal = {\apjl},
	Keywords = {PULSARS, STELLAR FLARES, STELLAR MODELS, X RAY BINARIES, B STARS, NEUTRON STARS, PERIODIC VARIATIONS, STELLAR MASS EJECTION},
	Month = aug,
	Pages = {L117-L120},
	Title = {{A model for the recurrent flares in EXO 2030 + 375}},
	Volume = 331,
	Year = 1988,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/185248}}

@article{takahashi07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2007PASJ...59S..35T&db_key=AST},
	Author = {{Takahashi}, T. and {Abe}, K. and {Endo}, M. and {Endo}, Y. and {Ezoe}, Y. and {Fukazawa}, Y. and {Hamaya}, M. and {Hirakuri}, S. and {Hong}, S. and {Horii}, M. and {Inoue}, H. and {Isobe}, N. and {Itoh}, T. and {Iyomoto}, N. and {Kamae}, T. and {Kasama}, D. and {Kataoka}, J. and {Kato}, H. and {Kawaharada}, M. and {Kawano}, N. and {Kawashima}, K. and {Kawasoe}, S. and {Kishishita}, T. and {Kitaguchi}, T. and {Kobayashi}, Y. and {Kokubun}, M. and {Kotoku}, J. and {Kouda}, M. and {Kubota}, A. and {Kuroda}, Y. and {Madejski}, G. and {Makishima}, K. and {Masukawa}, K. and {Matsumoto}, Y. and {Mitani}, T. and {Miyawaki}, R. and {Mizuno}, T. and {Mori}, K. and {Mori}, M. and {Murashima}, M. and {Murakami}, T. and {Nakazawa}, K. and {Niko}, H. and {Nomachi}, M. and {Okada}, Y. and {Ohno}, M. and {Oonuki}, K. and {Ota}, N. and {Ozawa}, H. and {Sato}, G. and {Shinoda}, S. and {Sugiho}, M. and {Suzuki}, M. and {Taguchi}, K. and {Takahashi}, H. and {Takahashi}, I. and {Takeda}, S. and {Tamura}, K.-I. and {Tamura}, T. and {Tanaka}, T. and {Tanihata}, C. and {Tashiro}, M. and {Terada}, Y. and {Tominaga}, S. and {Uchiyama}, Y. and {Watanabe}, S. and {Yamaoka}, K. and {Yanagida}, T. and {Yonetoku}, D.},
	Eprint = {astro-ph/0611232},
	Journal = {\pasj},
	Month = jan,
	Pages = {35-51},
	Title = {{Hard X-Ray Detector (HXD) on Board Suzaku}},
	Volume = 59,
	Year = 2007}

@ARTICLE{tam04,
   author = {{Tam}, C.~R. and {Kaspi}, V.~M. and {van Kerkwijk}, M.~H. and 
	{Durant}, M.},
    title = "{Correlated Infrared and X-Ray Flux Changes Following the 2002 June Outburst of the Anomalous X-Ray Pulsar 1E 2259+586}",
  journal = {\apjl},
   eprint = {astro-ph/0409351},
 keywords = {Infrared: Stars, Stars: Pulsars: General, Stars: Pulsars: Individual: Alphanumeric: 1E 2259+586, Stars: Magnetic Fields, Stars: Neutron},
     year = 2004,
    month = dec,
   volume = 617,
    pages = {L53-L56},
      doi = {10.1086/426963},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...617L..53T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{tam06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652..548T},
	Author = {{Tam}, C.~R. and {Kaspi}, V.~M. and {Gaensler}, B.~M. and {Gotthelf}, E.~V.},
	Doi = {10.1086/507262},
	Eprint = {arXiv:astro-ph/0602522},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General, pulsars: individual (AX J1845.0-0258), Stars: Neutron, X-rays: individual (CXOU J184454.6-025653)},
	Month = nov,
	Pages = {548-553},
	Title = {{Chandra Observations of the Transient 7 s X-ray Pulsar AX J1845.0-0258}},
	Volume = 652,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507262}}

@article{tanaka93,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1993IAUC.5880....1T&db_key=AST},
	Author = {{Tanaka}, Y. and {Kouveliotou}, C.},
	Journal = {\iaucirc},
	Month = oct,
	Pages = {1},
	Title = {{SGR 1806-20}},
	Volume = 5880,
	Year = 1993}

@article{tanaka94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994PASJ...46L..37T&db_key=AST},
	Author = {{Tanaka}, Y. and {Inoue}, H. and {Holt}, S.~S.},
	Journal = {\pasj},
	Month = jun,
	Pages = {L37-L41},
	Title = {{The X-ray astronomy satellite ASCA}},
	Volume = 46,
	Year = 1994}

@article{tananbaum99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1999IAUC.7246....1T},
	Author = {{Tananbaum}, H.},
	Journal = {\iaucirc},
	Month = sep,
	Pages = {1},
	Title = {{Cassiopeia A}},
	Volume = 7246,
	Year = 1999}

@ARTICLE{tauris12,
   author = {{Tauris}, T.~M. and {Langer}, N. and {Kramer}, M.},
    title = "{Formation of millisecond pulsars with CO white dwarf companions - II. Accretion, spin-up, true ages and comparison to MSPs with He white dwarf companions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.1862},
 primaryClass = "astro-ph.SR",
 keywords = {stars: neutron, pulsars: general, pulsars: individual: PSR J1614-2230, stars: rotation, white dwarfs, X-rays: binaries },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {1601-1627},
      doi = {10.1111/j.1365-2966.2012.21446.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.1601T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{tavani96,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..120C.243T},
	Author = {{Tavani}, M. and {Hermsen}, W. and {van Dijk}, R. and {Strickman}, M. and {Zhang}, S.~N. and {Foster}, R.~S. and {Ray}, P.~S. and {Mattox}, J. and {Ulmer}, M. and {Purcell}, W. and {Coe}, M.},
	Eprint = {arXiv:astro-ph/9611200},
	Journal = {\aaps},
	Month = dec,
	Pages = {C243},
	Title = {{Monitoring the gamma-ray source 2CG 135+1 and the radio star LSI +61 303.}},
	Volume = 120,
	Year = 1996}

@inproceedings{tavani06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006SPIE.6266E...2T},
	Author = {{Tavani}, M. and {Barbiellini}, G. and {Argan}, A. and {Basset}, M. and {Boffelli}, F. and {Bulgarelli}, A. and {Caraveo}, P. and {Chen}, A. and {Costa}, E. and {De Paris}, G. and {Del Monte}, E. and {Di Cocco}, G. and {Donnarumma}, I. and {Feroci}, M. and {Fiorini}, M. and {Foggetta}, L. and {Froysland}, T. and {Frutti}, M. and {Fuschino}, F. and {Galli}, M. and {Gianotti}, F. and {Giuliani}, A. and {Labanti}, C. and {Lapshov}, I. and {Lazzarotto}, F. and {Liello}, F. and {Lipari}, P. and {Longo}, F. and {Marisaldi}, M. and {Mastropietro}, M. and {Mattaini}, E. and {Mauri}, F. and {Mereghetti}, S. and {Morelli}, E. and {Morselli}, A. and {Pacciani}, L. and {Pellizzoni}, A. and {Perotti}, F. and {Picozza}, P. and {Pittori}, C. and {Pontoni}, C. and {Porrovecchio}, G. and {Prest}, M. and {Pucella}, G. and {Rapisarda}, M. and {Rossi}, E. and {Rubini}, A. and {Soffitta}, P. and {Traci}, A. and {Trifoglio}, M. and {Trois}, A. and {Vallazza}, E. and {Vercellone}, S. and {Zambra}, A. and {Zanello}, D.},
	Booktitle = {Space Telescopes and Instrumentation II: Ultraviolet to Gamma Ray. Edited by Turner, Martin J. L.; Hasinger, G{\"u}nther. Proceedings of the SPIE, Volume 6266, pp. 626603 (2006).},
	Doi = {10.1117/12.673207},
	Month = jul,
	Series = {Presented at the Society of Photo-Optical Instrumentation Engineers (SPIE) Conference},
	Title = {{The AGILE mission and its scientific instrument}},
	Volume = 6266,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1117/12.673207}}

@article{taylor93,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...411..674T&db_key=AST},
	Author = {{Taylor}, J.~H. and {Cordes}, J.~M.},
	Doi = {10.1086/172870},
	Journal = {\apj},
	Month = jul,
	Pages = {674-684},
	Title = {{Pulsar distances and the galactic distribution of free electrons}},
	Volume = 411,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/172870}}

@article{tml93,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJS...88..529T&db_key=AST},
	Author = {{Taylor}, J.~H. and {Manchester}, R.~N. and {Lyne}, A.~G.},
	Doi = {10.1086/191832},
	Journal = {\apjs},
	Month = oct,
	Pages = {529-568},
	Title = {{Catalog of 558 pulsars}},
	Volume = 88,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/191832}}

@article{taylor96,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...305..817T&db_key=AST},
	Author = {{Taylor}, A.~R. and {Young}, G. and {Peracaula}, M. and {Kenny}, H.~T. and {Gregory}, P.~C.},
	Journal = {\aap},
	Month = jan,
	Pages = {817},
	Title = {{An X-ray outburst. from the radio emitting X-ray binary LSI+61 303}},
	Volume = 305,
	Year = 1996}

@article{taylor05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634L..93T},
	Author = {{Taylor}, G.~B. and {Gelfand}, J.~D. and {Gaensler}, B.~M. and {Granot}, J. and {Kouveliotou}, C. and {Fender}, R.~P. and {Ramirez-Ruiz}, E. and {Eichler}, D. and {Lyubarsky}, Y.~E. and {Garrett}, M. and {Wijers}, R.~A.~M.~J.},
	Doi = {10.1086/491648},
	Eprint = {arXiv:astro-ph/0504363},
	Journal = {\apjl},
	Month = nov,
	Pages = {L93-L96},
	Title = {{The Growth, Polarization, and Motion of the Radio Afterglow from the Giant Flare from SGR 1806-20}},
	Volume = 634,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/491648}}

@article{tendulkar12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...761...76T},
	Archiveprefix = {arXiv},
	Author = {{Tendulkar}, S.~P. and {Cameron}, P.~B. and {Kulkarni}, S.~R.},
	Doi = {10.1088/0004-637X/761/1/76},
	Eid = {76},
	Eprint = {1210.8151},
	Journal = {\apj},
	Keywords = {proper motions, stars: individual: SGR 1806{\ndash}20 SGR 1900+14, stars: magnetars, stars: neutron},
	Month = dec,
	Pages = {76},
	Primaryclass = {astro-ph.HE},
	Title = {{Proper Motions and Origins of SGR 1806-20 and SGR 1900+14}},
	Volume = 761,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/761/1/76}}

@ARTICLE{tendulkar13,
   author = {{Tendulkar}, S.~P. and {Cameron}, P.~B. and {Kulkarni}, S.~R.
	},
    title = "{Proper Motions and Origins of AXP 1E 2259+586 and AXP 4U 0142+61}",
  journal = {\apj},
 keywords = {instrumentation: adaptive optics, ISM: individual objects: CTB 109, stars: individual: AXP 1E 2259+586 AXP 4U 0142+61, stars: magnetars, techniques: high angular resolution},
     year = 2013,
    month = jul,
   volume = 772,
      eid = {31},
    pages = {31},
      doi = {10.1088/0004-637X/772/1/31},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772...31T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tendulkar15,
   author = {{Tendulkar}, S.~P. and {Hasc{\"o}et}, R. and {Yang}, C. and 
	{Kaspi}, V.~M. and {Beloborodov}, A.~M. and {An}, H. and {Bachetti}, M. and 
	{Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and 
	{Guillot}, S. and {Hailey}, C.~A. and {Harrison}, F.~A. and 
	{Stern}, D. and {Zhang}, W.},
    title = "{Phase-resolved NuSTAR and Swift-XRT Observations of Magnetar 4U 0142+61}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1506.03098},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: 4U 0142+61, stars: magnetars, stars: neutron},
     year = 2015,
    month = jul,
   volume = 808,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-637X/808/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...808...32T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ttt05,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005astro.ph..2315T&db_key=PRE},
	Author = {{Terasawa}, T. and {Tanaka}, Y. and {Takei}, Y. and {Kawai}, N. and {Yoshida}, A. and {Nomoto}, K. and {Yoshikawa}, I. and {Saito}, Y. and {Kasaba}, Y. and {Takashima}, T. and {Mukai}, T. and {Noda}, H. and {Murakami}, T. and {Watanabe}, K. and {Muraki}, Y. and {Yokoyama}, T. and {Hoshino}, M.},
	Eprint = {astro-ph/0502315},
	Journal = {ArXiv Astrophysics e-prints (astro-ph/0502315)},
	Month = feb,
	Title = {{GEOTAIL observation of the SGR1806-20 Giant Flare: The first 600 ms}},
	Year = 2005}

@article{terasawa05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005Natur.434.1110T&db_key=AST},
	Author = {{Terasawa}, T. and {Tanaka}, Y.~T. and {Takei}, Y. and {Kawai}, N. and {Yoshida}, A. and {Nomoto}, K. and {Yoshikawa}, I. and {Saito}, Y. and {Kasaba}, Y. and {Takashima}, T. and {Mukai}, T. and {Noda}, H. and {Murakami}, T. and {Watanabe}, K. and {Muraki}, Y. and {Yokoyama}, T. and {Hoshino}, M.},
	Doi = {10.1038/nature03573},
	Journal = {\nat},
	Month = apr,
	Pages = {1110-1111},
	Title = {{Repeated injections of energy in the first 600ms of the giant flare of SGR1806 - 20}},
	Volume = 434,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature03573}}

@article{terrell80,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1980Natur.285..383T&db_key=AST},
	Author = {{Terrell}, J. and {Evans}, W.~D. and {Klebesadel}, R.~W. and {Laros}, J.~G.},
	Journal = {\nat},
	Month = jun,
	Pages = {383-385},
	Title = {{Periodicity of the gamma-ray transient event of 5 March 1979}},
	Volume = 285,
	Year = 1980}

@article{testa08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..607T},
	Archiveprefix = {arXiv},
	Author = {{Testa}, V. and {Rea}, N. and {Mignani}, R.~P. and {Israel}, G.~L. and {Perna}, R. and {Chaty}, S. and {Stella}, L. and {Covino}, S. and {Turolla}, R. and {Zane}, S. and {Lo Curto}, G. and {Campana}, S. and {Marconi}, G. and {Mereghetti}, S.},
	Doi = {10.1051/0004-6361:20078692},
	Eprint = {0712.4171},
	Journal = {\aap},
	Keywords = {stars: pulsars: individual: XTE J1810-197, stars: pulsars: individual: 1RXS J1708-4009, stars: pulsars: individual: 1E 1841-045, stars: pulsars: individual: SGR 1900+14, stars: pulsars: general, stars: neutron},
	Month = may,
	Pages = {607-615},
	Title = {{Adaptive optics, near-infrared observations of magnetars}},
	Volume = 482,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20078692}}

@article{thompson93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...408..194T},
	Author = {{Thompson}, C. and {Duncan}, R.~C.},
	Doi = {10.1086/172580},
	Journal = {\apj},
	Month = may,
	Pages = {194-217},
	Title = {{Neutron star dynamos and the origins of pulsar magnetism}},
	Volume = 408,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/172580}}

@article{thompson00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000ApJ...543..340T&db_key=AST},
	Author = {{Thompson}, C. and {Duncan}, R.~C. and {Woods}, P.~M. and {Kouveliotou}, C. and {Finger}, M.~H. and {van Paradijs}, J.},
	Journal = {\apj},
	Month = nov,
	Pages = {340-350},
	Title = {{Physical Mechanisms for the Variable Spin-down and Light Curve of SGR 1900+14}},
	Volume = 543,
	Year = 2000}

@article{thompson01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2001ApJ...561..980T},
	Author = {{Thompson}, C. and {Duncan}, R.~C.},
	Doi = {10.1086/323256},
	Eprint = {arXiv:astro-ph/0110675},
	Journal = {\apj},
	Month = nov,
	Pages = {980-1005},
	Title = {{The Giant Flare of 1998 August 27 from SGR 1900+14. II. Radiative Mechanism and Physical Constraints on the Source}},
	Volume = 561,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/323256}}

@article{thompson02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002MmSAI..73..572M&db_key=AST},
	Author = {{Thompson}, C},
	Journal = {Memorie della Societa Astronomica Italiana},
	Pages = {572-577},
	Title = {{Nature of the Soft Gamma Repeaters and Anomalous X-ray Pulsars}},
	Volume = 73,
	Year = 2002}

@article{tlk02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJ...574..332T&db_key=AST},
	Author = {{Thompson}, C. and {Lyutikov}, M. and {Kulkarni}, S.~R.},
	Journal = {\apj},
	Month = jul,
	Pages = {332-355},
	Title = {{Electrodynamics of Magnetars: Implications for the Persistent X-Ray Emission and Spin-down of the Soft Gamma Repeaters and Anomalous X-Ray Pulsars}},
	Volume = 574,
	Year = 2002}

@inproceedings{thompson04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ASSL..304..149T},
	Author = {{Thompson}, D.~J.},
	Booktitle = {Cosmic Gamma-Ray Sources},
	Editor = {{Cheng}, K.~S. and {Romero}, G.~E.},
	Month = oct,
	Pages = {149},
	Series = {Astrophysics and Space Science Library},
	Title = {{Gamma ray pulsars}},
	Volume = 304,
	Year = 2004}

@article{thompson08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...688..499T},
	Archiveprefix = {arXiv},
	Author = {{Thompson}, C.},
	Doi = {10.1086/592061},
	Eprint = {0802.2572},
	Journal = {\apj},
	Keywords = {Plasmas, Radiation Mechanisms: Nonthermal, Stars: Magnetic Fields, Stars: Neutron},
	Month = nov,
	Pages = {499-526},
	Title = {{Electrodynamics of Magnetars. IV. Self-Consistent Model of the Inner Accelerator with Implications for Pulsed Radio Emission}},
	Volume = 688,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/592061}}

@article{thorne77,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1977ApJ...212..832T&db_key=AST},
	Author = {{Thorne}, K.~S. and {Zytkow}, A.~N.},
	Journal = {\apj},
	Month = mar,
	Pages = {832-858},
	Title = {{Stars with degenerate neutron cores. I - Structure of equilibrium models}},
	Volume = 212,
	Year = 1977}

@article{thronson89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...339..803T},
	Author = {{Thronson}, Jr., H.~A. and {Hunter}, D.~A. and {Casey}, S. and {Latter}, W.~B. and {Harper}, D.~A.},
	Doi = {10.1086/167337},
	Journal = {\apj},
	Keywords = {ASTRONOMICAL SPECTROSCOPY, INTERACTING GALAXIES, INTERSTELLAR MATTER, STAR FORMATION, COSMIC DUST, EMISSION SPECTRA, H ALPHA LINE, INFRARED SPECTRA, SPECTRAL ENERGY DISTRIBUTION, VISIBLE SPECTRUM},
	Month = apr,
	Pages = {803-811},
	Title = {{The interacting galaxy pair NGC 4485 and NGC 4490 - Star formation and the interstellar medium}},
	Volume = 339,
	Year = 1989,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/167337}}

@article{tian07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...657L..25T},
	Author = {{Tian}, W.~W. and {Li}, Z. and {Leahy}, D.~A. and {Wang}, Q.~D.},
	Doi = {10.1086/512544},
	Eprint = {arXiv:astro-ph/0612296},
	Journal = {\apjl},
	Keywords = {Gamma Rays: Observations, ISM: Molecules, Radio Continuum: Galaxies, Radio Lines: Galaxies, ISM: Supernova Remnants, X-Rays: Galaxies},
	Month = mar,
	Pages = {L25-L28},
	Title = {{VLA and XMM-Newton Observations of the SNR W41/TeV Gamma-Ray Source HESS J1834-087}},
	Volume = 657,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/512544}}

@article{tmt05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005A%26A...437..997T&db_key=AST},
	Author = {{Tiengo}, A. and {Mereghetti}, S. and {Turolla}, R. and {Zane}, S. and {Rea}, N. and {Stella}, L. and {Israel}, G.~L.},
	Doi = {10.1051/0004-6361:20052633},
	Journal = {\aap},
	Month = jul,
	Pages = {997-1005},
	Title = {{Three XMM-Newton observations of the anomalous X-ray pulsar 1E 1048.1-5937: Long term variations in spectrum and pulsed fraction}},
	Volume = 437,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052633}}

@article{tiengo05,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2005A%26A...440L..63T&db_key=AST},
	Author = {{Tiengo}, A. and {Esposito}, P. and {Mereghetti}, S. and {Rea}, N. and {Stella}, L. and {Israel}, G.~L. and {Turolla}, R. and {Zane}, S.},
	Doi = {10.1051/0004-6361:200500170},
	Journal = {\aap},
	Month = sep,
	Pages = {L63-L66},
	Title = {{The calm after the storm: XMM-Newton observation of SGR 1806-20 two months after the Giant Flare of 2004 December 27}},
	Volume = 440,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200500170}}

@article{tiengo07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007Ap%26SS.308...33T},
	Author = {{Tiengo}, A. and {Esposito}, P. and {Mereghetti}, S. and {Sidoli}, L. and {G{\"o}tz}, D. and {Feroci}, M. and {Turolla}, R. and {Zane}, S. and {Israel}, G.~L. and {Stella}, L. and {Woods}, P.},
	Doi = {10.1007/s10509-007-9300-7},
	Eprint = {arXiv:astro-ph/0609319},
	Journal = {\apss},
	Month = apr,
	Pages = {33-37},
	Title = {{Long term spectral variability in the soft gamma-ray repeater SGR 1900+14}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9300-7}}

@article{tiengo08atel1559,
	Author = {{Tiengo}, A. and {Rea}, N. and {Klein-Wolt}, M. and {Wijnands}, R. and {Israel}, G.~L. and {Esposito}, P. and {Zane}, S. and {Starling}, R. and {Mereghetti}, S. and {De~Luca}, A. and {G\"otz}, D.},
	Journal = {Astron. Tel.},
	Title = {{RXTE Observations of Renewed Burst Activity from SGR 1627-41}},
	Volume = 1559,
	Year = 2008}

@article{tiengo10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..227T},
	Archiveprefix = {arXiv},
	Author = {{Tiengo}, A. and {Vianello}, G. and {Esposito}, P. and {Mereghetti}, S. and {Giuliani}, A. and {Costantini}, E. and {Israel}, G.~L. and {Stella}, L. and {Turolla}, R. and {Zane}, S. and {Rea}, N. and {G{\"o}tz}, D. and {Bernardini}, F. and {Moretti}, A. and {Romano}, P. and {Ehle}, M. and {Gehrels}, N.},
	Doi = {10.1088/0004-637X/710/1/227},
	Journal = {\apj},
	Keywords = {dust, extinction, stars: neutron, X-rays: individual: 1E 1547.0-5408, X-rays: stars},
	Month = feb,
	Pages = {227-235},
	Title = {{The Dust-scattering X-ray Rings of the Anomalous X-ray Pulsar 1E 1547.0-5408}},
	Volume = 710,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/710/1/227}}

@inproceedings{tody93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...52..173T},
	Author = {{Tody}, D.},
	Booktitle = {Astronomical Data Analysis Software and Systems II},
	Editor = {{Hanisch}, R.~J. and {Brissenden}, R.~J.~V. and {Barnes}, J.},
	Month = jan,
	Pages = {173-183},
	Publisher = {ASP, San Francisco},
	Series = {Astronomical Society of the Pacific Conference Series},
	Title = {{IRAF in the Nineties}},
	Volume = 52,
	Year = 1993}

@article{tomsick08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...685.1143T},
	Archiveprefix = {arXiv},
	Author = {{Tomsick}, J.~A. and {Chaty}, S. and {Rodriguez}, J. and {Walter}, R. and {Kaaret}, P.},
	Doi = {10.1086/591040},
	Eprint = {0807.2278},
	Journal = {\apj},
	Keywords = {Black Hole Physics, Infrared: Stars, stars: individual (IGR J00234+6141), stars: individual (IGR J01363+6610), stars: individual (IGR J06074+2205), stars: individual (IGR J09026-4812), stars: individual (IGR J10101-5654), stars: individual (IGR J11305-6256), stars: individual (IGR J11435-6109), stars: individual (IGR J14515-5542), stars: individual (IGR J17200-3116), stars: individual (IGR J17285-2922), stars: individual (IGR J17331-2406), stars: individual (IGR J17407-2808), stars: individual (IGR J17445-2747), stars: individual (IGR J17507-2856), stars: individual (IGR J18193-2542), stars: individual (IGR J18214-1318), stars: individual (IGR J18256-1035), stars: individual (IGR J18259-0706), stars: individual (IGR J18325-0756), stars: individual (IGR J18539+0727), Stars: Neutron, Stars: White Dwarfs, X-Rays: Stars},
	Month = oct,
	Pages = {1143-1156},
	Title = {{Chandra Localizations and Spectra of INTEGRAL Sources in the Galactic Plane}},
	Volume = 685,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/591040}}

@ARTICLE{tong16,
   author = {{Tong}, H. and {Wang}, W. and {Liu}, X.~W. and {Xu}, R.~X.},
    title = "{Rotational Evolution of Magnetars in the Presence of a Fallback Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1608.02113},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, pulsars: individual: 1E 161348-5055, stars: magnetars},
     year = 2016,
    month = dec,
   volume = 833,
      eid = {265},
    pages = {265},
      doi = {10.3847/1538-4357/833/2/265},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...833..265T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{torii98,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...503..843T},
	Author = {{Torii}, K. and {Kinugasa}, K. and {Katayama}, K. and {Tsunemi}, H. and {Yamauchi}, S.},
	Doi = {10.1086/306038},
	Journal = {\apj},
	Keywords = {X-RAYS: STARS, STARS: PULSARS: INDIVIDUAL ALPHANUMERIC: AX J1845.0-, 300, STARS: NEUTRON},
	Month = aug,
	Pages = {843},
	Title = {{Discovery of a 7 Second X-Ray Pulsar, AX J1845.0-0300}},
	Volume = 503,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/306038}}

@ARTICLE{torne15,
   author = {{Torne}, P. and {Eatough}, R.~P. and {Karuppusamy}, R. and {Kramer}, M. and 
	{Paubert}, G. and {Klein}, B. and {Desvignes}, G. and {Champion}, D.~J. and 
	{Wiesemeyer}, H. and {Kramer}, C. and {Spitler}, L.~G. and {Thum}, C. and 
	{G{\"u}sten}, R. and {Schuster}, K.~F. and {Cognard}, I.},
    title = "{Simultaneous multifrequency radio observations of the Galactic Centre magnetar SGR J1745-2900}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1504.07241},
 primaryClass = "astro-ph.HE",
 keywords = {radiation mechanisms: non-thermal, stars: magnetars, stars: neutron, pulsars: general, pulsars: individual: SGR J1745-2900, Galaxy: centre},
     year = 2015,
    month = jul,
   volume = 451,
    pages = {L50-L54},
      doi = {10.1093/mnrasl/slv063},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.451L..50T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{torne17,
   author = {{Torne}, P. and {Desvignes}, G. and {Eatough}, R.~P. and {Karuppusamy}, R. and 
	{Paubert}, G. and {Kramer}, M. and {Cognard}, I. and {Champion}, D.~J. and 
	{Spitler}, L.~G.},
    title = "{Detection of the magnetar SGR J1745-2900 up to 291 GHz with evidence of polarized millimetre emission}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1610.07616},
 primaryClass = "astro-ph.HE",
 keywords = {radiation mechanisms: non-thermal, stars: magnetars, stars: neutron, pulsars: general, pulsars: individual: SGR J1745-2900},
     year = 2017,
    month = feb,
   volume = 465,
    pages = {242-247},
      doi = {10.1093/mnras/stw2757},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465..242T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{torrejon10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...510A..61T},
	Archiveprefix = {arXiv},
	Author = {{Torrej{\'o}n}, J.~M. and {Negueruela}, I. and {Smith}, D.~M. and {Harrison}, T.~E.},
	Doi = {10.1051/0004-6361/200912619},
	Eid = {A61},
	Eprint = {0910.5603},
	Journal = {\aap},
	Keywords = {binaries: close, supergiants, infrared: stars, X-rays: binaries},
	Month = feb,
	Pages = {A61},
	Primaryclass = {astro-ph.SR},
	Title = {{Near-infrared survey of high mass X-ray binary candidates}},
	Volume = 510,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200912619}}

@article{torres12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...744..106T},
	Archiveprefix = {arXiv},
	Author = {{Torres}, D.~F. and {Rea}, N. and {Esposito}, P. and {Li}, J. and {Chen}, Y. and {Zhang}, S.},
	Doi = {10.1088/0004-637X/744/2/106},
	Eid = {106},
	Eprint = {1109.5008},
	Journal = {\apj},
	Keywords = {stars: magnetars, X-rays: binaries, X-rays: individual: LSI+61303},
	Month = jan,
	Pages = {106},
	Primaryclass = {astro-ph.HE},
	Title = {{A Magnetar-like Event from LS I +61{$^\circ$}303 and Its Nature as a Gamma-Ray Binary}},
	Volume = 744,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/744/2/106}}

@article{treffers93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993IAUC.5850....1T},
	Author = {{Treffers}, R.~R. and {Filippenko}, A.~V. and {Leibundgut}, B. and {Paik}, Y. and {Lee}, L.~F.~M. and {Richmond}, M.~W.},
	Journal = {\iaucirc},
	Month = aug,
	Title = {{Supernova 1993X in NGC 2276}},
	Volume = 5850,
	Year = 1993}

@article{treves00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000PASP..112..297T&db_key=AST},
	Author = {{Treves}, A. and {Turolla}, R. and {Zane}, S. and {Colpi}, M.},
	Journal = {\pasp},
	Month = mar,
	Pages = {297-314},
	Title = {{Isolated Neutron Stars: Accretors and Coolers}},
	Volume = 112,
	Year = 2000}

@article{trudolyubov04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616..821T},
	Author = {{Trudolyubov}, S. and {Priedhorsky}, W.},
	Doi = {10.1086/425033},
	Eprint = {astro-ph/0402619},
	Journal = {\apj},
	Keywords = {Galaxies: Individual: Messier Number: M31, Galaxies: Star Clusters, Galaxy: Globular Clusters: General, X-Rays: Galaxies},
	Month = dec,
	Pages = {821-844},
	Title = {{M31 Globular Cluster X-Ray Sources: XMM-Newton and Chandra Results}},
	Volume = 616,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/425033}}

@ARTICLE{trudolyubov05,
   author = {{Trudolyubov}, S. and {Kotov}, O. and {Priedhorsky}, W. and 
	{Cordova}, F. and {Mason}, K.},
    title = "{XMM-Newton Observations of the M31 Northern Disk: Properties of Selected X-Ray Sources and Unresolved Emission}",
  journal = {\apj},
   eprint = {astro-ph/0401227},
 keywords = {Galaxies: Individual: Messier Number: M31, X-Rays: Galaxies, X-Rays: Stars},
     year = 2005,
    month = nov,
   volume = 634,
    pages = {314-331},
      doi = {10.1086/496940},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634..314T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{truemper73,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....25..445T},
	Author = {{Tr{\"u}mper}, J. and {Sch{\"o}nfelder}, V.},
	Journal = {\aap},
	Month = jun,
	Pages = {445},
	Title = {{Distance Determination of Variable X-ray Sources}},
	Volume = 25,
	Year = 1973}

@article{truemper78,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...219L.105T&db_key=AST},
	Author = {{Truemper}, J. and {Pietsch}, W. and {Reppin}, C. and {Voges}, W. and {Staubert}, R. and {Kendziorra}, E.},
	Journal = {\apjl},
	Month = feb,
	Pages = {L105-L110},
	Title = {{Evidence for strong cyclotron line emission in the hard X-ray spectrum of Hercules X-1}},
	Volume = 219,
	Year = 1978}

@article{truemper10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518A..46T},
	Archiveprefix = {arXiv},
	Author = {{Tr{\"u}mper}, J.~E. and {Zezas}, A. and {Ertan}, {\"U}. and {Kylafis}, N.~D.},
	Doi = {10.1051/0004-6361/200911834},
	Eid = {A46},
	Eprint = {1004.3391},
	Journal = {\aap},
	Keywords = {pulsars: individual: 1E 1841-045, pulsars: individual: 1RXS J1708-4009, pulsars: individual: 4U 0142+61, X-rays: stars, stars: magnetic fields},
	Month = jul,
	Pages = {A46},
	Primaryclass = {astro-ph.HE},
	Title = {{The energy spectrum of anomalous X-ray pulsars and soft gamma-ray repeaters}},
	Volume = 518,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200911834}}

@article{tsunemi00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000PASJ...52..887T},
	Author = {{Tsunemi}, H. and {Miyata}, E. and {Aschenbach}, B. and {Hiraga}, J. and {Akutsu}, D.},
	Eprint = {arXiv:astro-ph/0005452},
	Journal = {\pasj},
	Keywords = {ISM: INDIVIDUAL (RX J0852-4622), SUPERNOVA REMNANTS, X-RAYS: SOURCES, X-RAYS: SPECTRA},
	Month = oct,
	Pages = {887-893},
	Title = {{Overabundance of Calcium in the Young SNR RX J0852-4622: Evidence of Over-Production of ^{44}Ti}},
	Volume = 52,
	Year = 2000}

@article{tueller10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..186..378T},
	Archiveprefix = {arXiv},
	Author = {{Tueller}, J. and {Baumgartner}, W.~H. and {Markwardt}, C.~B. and {Skinner}, G.~K. and {Mushotzky}, R.~F. and {Ajello}, M. and {Barthelmy}, S. and {Beardmore}, A. and {Brandt}, W.~N. and {Burrows}, D. and {Chincarini}, G. and {Campana}, S. and {Cummings}, J. and {Cusumano}, G. and {Evans}, P. and {Fenimore}, E. and {Gehrels}, N. and {Godet}, O. and {Grupe}, D. and {Holland}, S. and {Kennea}, J. and {Krimm}, H.~A. and {Koss}, M. and {Moretti}, A. and {Mukai}, K. and {Osborne}, J.~P. and {Okajima}, T. and {Pagani}, C. and {Page}, K. and {Palmer}, D. and {Parsons}, A. and {Schneider}, D.~P. and {Sakamoto}, T. and {Sambruna}, R. and {Sato}, G. and {Stamatikos}, M. and {Stroh}, M. and {Ukwata}, T. and {Winter}, L.},
	Doi = {10.1088/0067-0049/186/2/378},
	Eprint = {0903.3037},
	Journal = {\apjs},
	Keywords = {catalogs, galaxies: active, gamma rays: observations, novae, cataclysmic variables, surveys, X-rays: binaries},
	Month = feb,
	Pages = {378-405},
	Primaryclass = {astro-ph.HE},
	Title = {{The 22 Month Swift-BAT All-Sky Hard X-ray Survey}},
	Volume = 186,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0067-0049/186/2/378}}

@book{tully88,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1988cng..book.....T},
	Author = {{Tully}, R.~B. and {Fisher}, J.~R.},
	Month = apr,
	Publisher = {Cambridge University Press, Cambridge},
	Title = {{Catalog of Nearby Galaxies}},
	Year = 1988}

@ARTICLE{tully08,
       author = {{Tully}, R. Brent and {Shaya}, Edward J. and {Karachentsev}, Igor D. and
         {Courtois}, H{\'e}l{\`e}ne M. and {Kocevski}, Dale D. and
         {Rizzi}, Luca and {Peel}, Alan},
        title = "{Our Peculiar Motion Away from the Local Void}",
      journal = {\apj},
     keywords = {dark matter, galaxies: distances and redshifts, large-scale structure of universe, Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2008,
        month = mar,
       volume = {676},
       number = {1},
        pages = {184-205},
          doi = {10.1086/527428},
archivePrefix = {arXiv},
       eprint = {0705.4139},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...676..184T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{tully09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009AJ....138..323T},
	Author = {{Tully}, R.~B. and {Rizzi}, L. and {Shaya}, E.~J. and {Courtois}, H.~M. and {Makarov}, D.~I. and {Jacobs}, B.~A.},
	Doi = {10.1088/0004-6256/138/2/323},
	Journal = {\aj},
	Keywords = {astronomical data bases: miscellaneous, catalogs, galaxies: distances and redshifts, galaxies: fundamental parameters},
	Month = aug,
	Pages = {323-331},
	Title = {{The Extragalactic Distance Database}},
	Volume = 138,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/138/2/323}}

@ARTICLE{tully13,
   author = {{Tully}, R.~B. and {Courtois}, H.~M. and {Dolphin}, A.~E. and 
	{Fisher}, J.~R. and {H{\'e}raudeau}, P. and {Jacobs}, B.~A. and 
	{Karachentsev}, I.~D. and {Makarov}, D. and {Makarova}, L. and 
	{Mitronova}, S. and {Rizzi}, L. and {Shaya}, E.~J. and {Sorce}, J.~G. and 
	{Wu}, P.-F.},
    title = "{Cosmicflows-2: The Data}",
  journal = {\aj},
 keywords = {catalogs, galaxies: distances and redshifts},
     year = 2013,
    month = oct,
   volume = 146,
      eid = {86},
    pages = {86},
      doi = {10.1088/0004-6256/146/4/86},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....146...86T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{tuohy80,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1980ApJ...239L.107T},
	Author = {{Tuohy}, I. and {Garmire}, G.},
	Doi = {10.1086/183303},
	Journal = {\apjl},
	Month = aug,
	Pages = {L107-L110},
	Title = {{Discovery of a compact X-ray source at the center of the supernova remnant RCW 103}},
	Volume = 239,
	Year = 1980,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/183303}}

@article{tuohy83,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...268..778T},
	Author = {{Tuohy}, I.~R. and {Dopita}, M.~A. and {Garmire}, G.~P. and {Manchester}, R.~N.},
	Doi = {10.1086/160999},
	Journal = {\apj},
	Keywords = {BINARY STARS, BLACK BODY RADIATION, NEBULAE, NEUTRON STARS, SUPERNOVA REMNANTS, X RAY SOURCES, COOLING, POINT SOURCES, STELLAR LUMINOSITY, STELLAR TEMPERATURE},
	Month = may,
	Pages = {778-781},
	Title = {{The central X-ray source in RCW 103 - Evidence for blackbody emission}},
	Volume = 268,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/160999}}

@article{turner01,
	Author = {{Turner}, M.~J.~L. and {Abbey}, A. and {Arnaud}, M. and {Balasini}, M. and {Barbera}, M. and {Belsole}, E. and {Bennie}, P.~J. and {Bernard}, J.~P. and {Bignami}, G.~F. and {Boer}, M. and {Briel}, U. and {Butler}, I. and {Cara}, C. and {Chabaud}, C. and {Cole}, R. and {Collura}, A. and {Conte}, M. and {Cros}, A. and {Denby}, M. and {Dhez}, P. and {Di Coco}, G. and {Dowson}, J. and {Ferrando}, P. and {Ghizzardi}, S. and {Gianotti}, F. and {Goodall}, C.~V. and {Gretton}, L. and {Griffiths}, R.~G. and {Hainaut}, O. and {Hochedez}, J.~F. and {Holland}, A.~D. and {Jourdain}, E. and {Kendziorra}, E. and {Lagostina}, A. and {Laine}, R. and {La Palombara}, N. and {Lortholary}, M. and {Lumb}, D. and {Marty}, P. and {Molendi}, S. and {Pigot}, C. and {Poindron}, E. and {Pounds}, K.~A. and {Reeves}, J.~N. and {Reppin}, C. and {Rothenflug}, R. and {Salvetat}, P. and {Sauvageot}, J.~L. and {Schmitt}, D. and {Sembay}, S. and {Short}, A.~D.~T. and {Spragg}, J. and {Stephen}, J. and {Str{\"u}der}, L. and {Tiengo}, A. and {Trifoglio}, M. and {Tr{\"u}mper}, J. and {Vercellone}, S. and {Vigroux}, L. and {Villa}, G. and {Ward}, M.~J. and {Whitehead}, S. and {Zonca}, E.},
	Journal = {\aap},
	Month = jan,
	Pages = {L27-L35},
	Title = {{The European Photon Imaging Camera on XMM-Newton: The MOS cameras}},
	Volume = 365,
	Year = 2001}

@article{turolla04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...603..265T},
	Author = {{Turolla}, R. and {Zane}, S. and {Drake}, J.~J.},
	Doi = {10.1086/379113},
	Eprint = {arXiv:astro-ph/0308326},
	Journal = {\apj},
	Keywords = {Radiative Transfer, Stars: Individual: Alphanumeric: RX J0720.4-3125, Stars: Individual: Alphanumeric: RX J1856.5-3754, Stars: Neutron, X-Rays: Stars},
	Month = mar,
	Pages = {265-282},
	Title = {{Bare Quark Stars or Naked Neutron Stars? The Case of RX J1856.5-3754}},
	Volume = 603,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/379113}}

@article{turolla11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740..105T},
	Archiveprefix = {arXiv},
	Author = {{Turolla}, R. and {Zane}, S. and {Pons}, J.~A. and {Esposito}, P. and {Rea}, N.},
	Doi = {10.1088/0004-637X/740/2/105},
	Eid = {105},
	Eprint = {1107.5488},
	Journal = {\apj},
	Keywords = {pulsars: individual: SGR 0418+5729, stars: magnetic field, stars: neutron},
	Month = oct,
	Pages = {105},
	Primaryclass = {astro-ph.HE},
	Title = {{Is SGR 0418+5729 Indeed a Waning Magnetar?}},
	Volume = 740,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/740/2/105}}

@article{ubertini03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003A%26A...411L.131U&db_key=AST},
	Author = {{Ubertini}, P. and {Lebrun}, F. and {Di Cocco}, G. and {Bazzano}, A. and {Bird}, A.~J. and {Broenstad}, K. and {Goldwurm}, A. and {La Rosa}, G. and {Labanti}, C. and {Laurent}, P. and {Mirabel}, I.~F. and {Quadrini}, E.~M. and {Ramsey}, B. and {Reglero}, V. and {Sabau}, L. and {Sacco}, B. and {Staubert}, R. and {Vigroux}, L. and {Weisskopf}, M.~C. and {Zdziarski}, A.~A.},
	Journal = {\aap},
	Month = nov,
	Pages = {L131-L139},
	Title = {{IBIS: The Imager on-board INTEGRAL}},
	Volume = 411,
	Year = 2003}

@article{uchiyama08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008PASJ...60S..35U},
	Archiveprefix = {arXiv},
	Author = {{Uchiyama}, Y. and {Maeda}, Y. and {Ebara}, M. and {Fujimoto}, R. and {Ishisaki}, Y. and {Ishida}, M. and {Iizuka}, R. and {Ushio}, M. and {Inoue}, H. and {Okada}, S. and {Mori}, H. and {Ozaki}, M.},
	Eprint = {0803.3418},
	Journal = {\pasj},
	Keywords = {instrumentation: miscellaneous, space vehicles: instruments, X-rays: general},
	Month = jan,
	Pages = {35},
	Title = {{Restoring the Suzaku Source Position Accuracy and Point-Spread Function}},
	Volume = 60,
	Year = 2008}

@article{urry95,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995PASP..107..803U&db_key=AST},
	Author = {{Urry}, C.~M. and {Padovani}, P.},
	Eprint = {astro-ph/9506063},
	Journal = {\pasp},
	Month = sep,
	Pages = {803},
	Title = {{Unified Schemes for Radio-Loud Active Galactic Nuclei}},
	Volume = 107,
	Year = 1995}

@article{valinia98,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1998ApJ...505..134V&db_key=AST},
	Author = {{Valinia}, A. and {Marshall}, F.~E.},
	Doi = {10.1086/306155},
	Eprint = {astro-ph/9804012},
	Journal = {\apj},
	Month = sep,
	Pages = {134-147},
	Title = {{RXTE Measurement of the Diffuse X-Ray Emission from the Galactic Ridge: Implications for the Energetics of the Interstellar Medium}},
	Volume = 505,
	Year = 1998,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/306155}}

@article{vancura92,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1992ApJ...394..158V&db_key=AST},
	Author = {{Vancura}, O. and {Blair}, W.~P. and {Long}, K.~S. and {Raymond}, J.~C.},
	Journal = {\apj},
	Month = jul,
	Pages = {158-173},
	Title = {{A multiwavelength study of the supernova remnant N49 in the Large Magellanic Cloud}},
	Volume = 394,
	Year = 1992}

@article{vandenberg09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...700.1702V},
	Archiveprefix = {arXiv},
	Author = {{van den Berg}, M. and {Hong}, J.~S. and {Grindlay}, J.~E.},
	Doi = {10.1088/0004-637X/700/2/1702},
	Eprint = {0905.4298},
	Journal = {\apj},
	Keywords = {Galaxy: bulge, novae, cataclysmic variables, surveys, X-rays: binaries},
	Month = aug,
	Pages = {1702-1715},
	Primaryclass = {astro-ph.HE},
	Title = {{ChaMPlane Deep Galactic Bulge Survey. I. Faint Accretion-driven Binaries in the Limiting Window}},
	Volume = 700,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/700/2/1702}}

@article{vandenberg12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...31V},
	Archiveprefix = {arXiv},
	Author = {{van den Berg}, M. and {Penner}, K. and {Hong}, J. and {Grindlay}, J.~E. and {Zhao}, P. and {Laycock}, S. and {Servillat}, M.},
	Doi = {10.1088/0004-637X/748/1/31},
	Eid = {31},
	Eprint = {1201.5038},
	Journal = {\apj},
	Keywords = {novae, cataclysmic variables, stars: flare, stars: individual: CXOPS J154305.5{\ndash}522709 CXOPS J171340.5{\ndash}395213 CXOPS J175900.8{\ndash}334548 HD 9743, surveys, X-rays: binaries, X-rays: stars},
	Month = mar,
	Pages = {31},
	Primaryclass = {astro-ph.HE},
	Title = {{The ChaMPlane Bright X-Ray Sources{\mdash}Galactic Longitudes l = 2{\deg}-358{\deg}}},
	Volume = 748,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/748/1/31}}
	
@ARTICLE{vandenheuvel17,
       author = {{van den Heuvel}, E.~P.~J. and {Portegies Zwart}, S.~F. and
         {de Mink}, S.~E.},
        title = "{Forming short-period Wolf-Rayet X-ray binaries and double black holes through stable mass transfer}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: Wolf-Rayet, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Nov",
       volume = {471},
       number = {4},
        pages = {4256-4264},
          doi = {10.1093/mnras/stx1430},
archivePrefix = {arXiv},
       eprint = {1701.02355},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471.4256V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{vanderhorst10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711L...1V},
	Author = {{van der Horst}, A.~J. and {Connaughton}, V. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kaneko}, Y. and {Wachter}, S. and {Briggs}, M.~S. and {Granot}, J. and {Ramirez-Ruiz}, E. and {Woods}, P.~M. and {Aptekar}, R.~L. and {Barthelmy}, S.~D. and {Cummings}, J.~R. and {Finger}, M.~H. and {Frederiks}, D.~D. and {Gehrels}, N. and {Gelino}, C.~R. and {Gelino}, D.~M. and {Golenetskii}, S. and {Hurley}, K. and {Krimm}, H.~A. and {Mazets}, E.~P. and {McEnery}, J.~E. and {Meegan}, C.~A. and {Oleynik}, P.~P. and {Palmer}, D.~M. and {Pal'shin}, V.~D. and {Pe'er}, A. and {Svinkin}, D. and {Ulanov}, M.~V. and {van der Klis}, M. and {von Kienlin}, A. and {Watts}, A.~L. and {Wilson-Hodge}, C.~A.},
	Doi = {10.1088/2041-8205/711/1/L1},
	Journal = {\apjl},
	Keywords = {pulsars: individual: SGR J0418+5729, stars: neutron, X-rays: bursts},
	Month = mar,
	Pages = {L1-L6},
	Title = {{Discovery of a New Soft Gamma Repeater: SGR J0418 + 5729}},
	Volume = 711,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/2041-8205/711/1/L1}}

@ARTICLE{vanderhorst12,
   author = {{van der Horst}, A.~J. and {Kouveliotou}, C. and {Gorgone}, N.~M. and 
	{Kaneko}, Y. and {Baring}, M.~G. and {Guiriec}, S. and {G{\"o}{\v g}{\"u}{\c s}}, E. and 
	{Granot}, J. and {Watts}, A.~L. and {Lin}, L. and {Bhat}, P.~N. and 
	{Bissaldi}, E. and {Chaplin}, V.~L. and {Finger}, M.~H. and 
	{Gehrels}, N. and {Gibby}, M.~H. and {Giles}, M.~M. and {Goldstein}, A. and 
	{Gruber}, D. and {Harding}, A.~K. and {Kaper}, L. and {von Kienlin}, A. and 
	{van der Klis}, M. and {McBreen}, S. and {Mcenery}, J. and {Meegan}, C.~A. and 
	{Paciesas}, W.~S. and {Pe'er}, A. and {Preece}, R.~D. and {Ramirez-Ruiz}, E. and 
	{Rau}, A. and {Wachter}, S. and {Wilson-Hodge}, C. and {Woods}, P.~M. and 
	{Wijers}, R.~A.~M.~J.},
    title = "{SGR J1550-5418 Bursts Detected with the Fermi Gamma-Ray Burst Monitor during its Most Prolific Activity}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1202.3157},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: SGR J1550{\ndash}5418 1E 1547.0{\ndash}5408 PSR J1550{\ndash}5418, stars: neutron, X-rays: bursts},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {122},
    pages = {122},
      doi = {10.1088/0004-637X/749/2/122},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...749..122V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inbook{vanderklis06,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2006csxs.book...39V},
	Author = {{van der Klis}, M.},
	Month = apr,
	Pages = {39},
	Publisher = {Cambridge: Cambridge University Press},
	Title = {{in Compact stellar X-ray sources, ed. W. H. G. Levin and M. van der Klis}},
	Year = 2006}

@inproceedings{vandermarel04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp...37V},
	Author = {{van der Marel}, R.~P.},
	Booktitle = {Carnegie Observatories Astrophysics Series, Vol.~1: Coevolution of Black Holes and Galaxies.},
	Editor = {L. C. Ho},
	Eprint = {arXiv:astro-ph/0302101},
	Pages = {37},
	Publisher = {Cambridge University Press},
	Title = {{Intermediate-mass Black Holes in the Universe: A Review of Formation Theories and Observational Constraints}},
	Year = 2004}

@article{vanderswaluw04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004A%26A...420..937V&db_key=AST},
	Author = {{van der Swaluw}, E. and {Downes}, T.~P. and {Keegan}, R.},
	Doi = {10.1051/0004-6361:20035700},
	Eprint = {astro-ph/0311388},
	Journal = {\aap},
	Month = jun,
	Pages = {937-944},
	Title = {{An evolutionary model for pulsar-driven supernova remnants. A hydrodynamical model}},
	Volume = 420,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20035700}}

@article{vankerkwijk95,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1995ApJ...444L..33V&db_key=AST},
	Author = {{van Kerkwijk}, M.~H. and {Kulkarni}, S.~R. and {Matthews}, K. and {Neugebauer}, G.},
	Journal = {\apjl},
	Month = may,
	Pages = {L33-L35},
	Title = {{A luminous companion to SGR 1806-20}},
	Volume = 444,
	Year = 1995}

@article{vankerkwijk96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...314..521V},
	Author = {{van Kerkwijk}, M.~H. and {Geballe}, T.~R. and {King}, D.~L. and {van der Klis}, M. and {van Paradijs}, J.},
	Eprint = {arXiv:astro-ph/9604100},
	Journal = {\aap},
	Keywords = {STARS: INDIVIDUAL: CYGNUS X-3, STARS: WOLF-RAYET, X-RAYS: STARS},
	Month = oct,
	Pages = {521-540},
	Title = {{The Wolf-Rayet counterpart of Cygnus X-3.}},
	Volume = 314,
	Year = 1996}

@article{vankerkwijk07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.308..191V},
	Author = {{van Kerkwijk}, M.~H. and {Kaplan}, D.~L.},
	Doi = {10.1007/s10509-007-9343-9},
	Eprint = {arXiv:astro-ph/0607320},
	Journal = {\apss},
	Month = apr,
	Pages = {191-201},
	Title = {{Isolated neutron stars: magnetic fields, distances,and spectra}},
	Volume = 308,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s10509-007-9343-9}}

@inproceedings{vanparadijs84,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1984AIPC..115...49V},
	Author = {{van Paradijs}, J. and {Verbunt}, F.},
	Booktitle = {High Energy Transients in Astrophysics},
	Doi = {10.1063/1.34556},
	Editor = {{Woosley}, S.~E.},
	Keywords = {cosmic x-ray sources, binary stars, transients, visible spectra, star accretion, luminosity, variable stars, dwarf novae, light curves},
	Month = may,
	Pages = {49-62},
	Publisher = {AIP, Melville},
	Series = {AIP Conference Series},
	Title = {{A comparison of soft x-ray transients and dwarf novae}},
	Volume = 115,
	Year = 1984,
	Bdsk-Url-1 = {http://dx.doi.org/10.1063/1.34556}}

@article{vanparadijs94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...281L..17V},
	Author = {{van Paradijs}, J. and {van der Klis}, M.},
	Journal = {\aap},
	Keywords = {Black Holes (Astronomy), Neutron Stars, Stellar Luminosity, X Ray Astronomy, X Ray Binaries, X Ray Spectra, Astronomical Catalogs, Emission Spectra, Heao 1, Stellar Mass, X Ray Spectroscopy},
	Month = jan,
	Pages = {L17-L20},
	Title = {{Luminosity dependence of the hardness of the 13-80 keV X-ray spectra of low-mass X-ray binaries}},
	Volume = 281,
	Year = 1994}

@article{vanparadijs95,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1995A%26A...299L..41V&db_key=AST},
	Author = {{van Paradijs}, J. and {Taam}, R.~E. and {van den Heuvel}, E.~P.~J.},
	Journal = {\aap},
	Month = jul,
	Pages = {L41},
	Title = {{On the nature of the 'anomalous' 6-s X-ray pulsars}},
	Volume = 299,
	Year = 1995}

@ARTICLE{vanputten13,
   author = {{van Putten}, T. and {Watts}, A.~L. and {D'Angelo}, C.~R. and 
	{Baring}, M.~G. and {Kouveliotou}, C.},
    title = "{Models of hydrostatic magnetar atmospheres at high luminosities}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.4212},
 primaryClass = "astro-ph.HE",
 keywords = {stars: atmospheres, stars: magnetars, X-rays: bursts},
     year = 2013,
    month = sep,
   volume = 434,
    pages = {1398-1410},
      doi = {10.1093/mnras/stt1093},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.434.1398V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{vanstraten11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011PASA...28....1V},
	Archiveprefix = {arXiv},
	Author = {{van Straten}, W. and {Bailes}, M.},
	Doi = {10.1071/AS10021},
	Eprint = {1008.3973},
	Journal = {\pasa},
	Keywords = {methods: data analysis, polarisation, pulsars: general, techniques: polarimetric},
	Month = jan,
	Pages = {1-14},
	Primaryclass = {astro-ph.IM},
	Title = {{DSPSR: Digital Signal Processing Software for Pulsar Astronomy}},
	Volume = 28,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1071/AS10021}}

@ARTICLE{vasilopoulos16,
   author = {{Vasilopoulos}, G. and {Petropoulou}, M.},
    title = "{The X-ray dust-scattered rings of the black hole low-mass binary V404 Cyg}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.00932},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, ISM: individual objects: V404 Cygni, X-rays: binaries, X-rays: ISM},
     year = 2016,
    month = feb,
   volume = 455,
    pages = {4426-4441},
      doi = {10.1093/mnras/stv2605},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.455.4426V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{vasisht94,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1994ApJ...431L..35V&amp;db_key=AST},
	Author = {{Vasisht}, G. and {Kulkarni}, S.~R. and {Frail}, D.~A. and {Greiner}, J.},
	Journal = {\apjl},
	Month = aug,
	Pages = {L35-L38},
	Title = {{Supernova remnant candidates for the soft gamma-ray repeater 1900+14}},
	Volume = 431,
	Year = 1994}

@article{vasisht97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1997ApJ...486L.129V&db_key=AST},
	Author = {{Vasisht}, G. and {Gotthelf}, E.~V.},
	Doi = {10.1086/310843},
	Journal = {\apjl},
	Month = sep,
	Pages = {L129+},
	Title = {{The Discovery of an Anomalous X-Ray Pulsar in the Supernova Remnant Kes 73}},
	Volume = 486,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/310843}}

@article{vasisht00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542L..49V},
	Author = {{Vasisht}, G. and {Gotthelf}, E.~V. and {Torii}, K. and {Gaensler}, B.~M.},
	Doi = {10.1086/312910},
	Eprint = {arXiv:astro-ph/0008196},
	Journal = {\apjl},
	Keywords = {ISM: Individual: Alphanumeric: G29.6+0.1, Stars: Pulsars: Individual: Alphanumeric: AX J1845-0258, Stars: Individual: Alphanumeric: AX J184453-025640, Stars: Neutron},
	Month = oct,
	Pages = {L49-L52},
	Title = {{Detection of a Compact X-Ray Source in the Supernova Remnant G29.6+0.1: A Variable Anomalous X-Ray Pulsar?}},
	Volume = 542,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/312910}}

@article{vaughan94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1994ApJ...435..362V},
	Author = {{Vaughan}, B.~A. and {van der Klis}, M. and {Wood}, K.~S. and {Norris}, J.~P. and {Hertz}, P. and {Michelson}, P.~F. and {van Paradijs}, J. and {Lewin}, W.~H.~G. and {Mitsuda}, K. and {Penninx}, W.},
	Doi = {10.1086/174818},
	Journal = {\apj},
	Month = nov,
	Pages = {362-371},
	Title = {{Searches for millisecond pulsations in low-mass X-ray binaries, 2}},
	Volume = 435,
	Year = 1994,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/174818}}

@ARTICLE{vaughan04,
   author = {{Vaughan}, S. and {Willingale}, R. and {O'Brien}, P.~T. and 
	{Osborne}, J.~P. and {Reeves}, J.~N. and {Levan}, A.~J. and 
	{Watson}, M.~G. and {Tedds}, J.~A. and {Watson}, D. and {Santos-Lle{\'o}}, M. and 
	{Rodr{\'{\i}}guez-Pascual}, P.~M. and {Schartel}, N.},
    title = "{The Discovery of an Evolving Dust-scattered X-Ray Halo around GRB 031203}",
  journal = {\apjl},
 keywords = {ISM: Dust, Extinction, Galaxy: Structure, Gamma Rays: Bursts, X-Rays: General},
     year = 2004,
    month = mar,
   volume = 603,
    pages = {L5-L8},
      doi = {10.1086/382785},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...603L...5V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{verbunt93,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1993ARA%26A..31...93V},
	Author = {{Verbunt}, F.},
	Doi = {10.1146/annurev.aa.31.090193.000521},
	Journal = {\araa},
	Keywords = {NEUTRON STARS, PULSARS, RADIO STARS, STELLAR EVOLUTION, X RAY BINARIES, ROCHE LIMIT, STELLAR MASS EJECTION},
	Pages = {93-127},
	Title = {{Origin and evolution of X-ray binaries and binary radio pulsars}},
	Volume = 31,
	Year = 1993,
	Bdsk-Url-1 = {http://dx.doi.org/10.1146/annurev.aa.31.090193.000521}}

@ARTICLE{verstappen13,
   author = {{Verstappen}, J. and {Fritz}, J. and {Baes}, M. and {Smith}, M.~W.~L. and 
	{Allaert}, F. and {Bianchi}, S. and {Blommaert}, J.~A.~D.~L. and 
	{De Geyter}, G. and {De Looze}, I. and {Gentile}, G. and {Gordon}, K.~D. and 
	{Holwerda}, B.~W. and {Viaene}, S. and {Xilouris}, E.~M.},
    title = "{HERschel Observations of Edge-on Spirals (HEROES). I. Far-infrared morphology and dust mass determination}",
  journal = {\aap},
 keywords = {galaxies: structure, infrared: ISM, infrared: galaxies, submillimeter: ISM, submillimeter: galaxies, dust, extinction},
     year = 2013,
    month = aug,
   volume = 556,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201220733},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...556A..54V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{vetere06,
	Author = {{Vetere}, L. and {Barthelmy}, S.~D. and {Kennea}, J.~A. and {Markwardt}, C.~B. and {Palmer}, D.~M.},
	Journal = {GRB Circular Network},
	Pages = {1},
	Title = {{SGR 1900+14: Swift detection of renewed activity}},
	Volume = 4922,
	Year = 2006}

@article{viallefond80,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1980A%26A....82..207V},
	Author = {{Viallefond}, F. and {Allen}, R.~J. and {de Boer}, J.~A.},
	Journal = {\aap},
	Keywords = {CONTINUOUS SPECTRA, GALACTIC STRUCTURE, HYDROGEN, INTERACTING GALAXIES, RADIO GALAXIES, RADIO SPECTRA, ASTRONOMICAL MAPS, CONTINUOUS RADIATION, DATA PROCESSING, GALACTIC RADIATION, H II REGIONS, NEUTRAL GASES, RADIO ASTRONOMY},
	Month = feb,
	Pages = {207-220},
	Title = {{Radio continuum and H I observations of the interacting galaxies NGC 4490/85}},
	Volume = 82,
	Year = 1980}

@article{vietri07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...661.1089V},
	Author = {{Vietri}, M. and {Stella}, L. and {Israel}, G.~L.},
	Doi = {10.1086/517506},
	Eprint = {arXiv:astro-ph/0702598},
	Journal = {\apj},
	Keywords = {Stars: Individual: Alphanumeric: SGR 1806-20, Stars: Magnetic Fields, Stars: Neutron},
	Month = jun,
	Pages = {1089-1093},
	Title = {{SGR 1806-20: Evidence for a Superstrong Magnetic Field from Quasi-Periodic Oscillations}},
	Volume = 661,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/517506}}

@article{vigano12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2487V},
	Archiveprefix = {arXiv},
	Author = {{Vigan{\`o}}, D. and {Pons}, J.~A.},
	Doi = {10.1111/j.1365-2966.2012.21679.x},
	Eprint = {1206.2014},
	Journal = {\mnras},
	Keywords = {stars: magnetic field, stars: neutron, pulsars: general},
	Month = oct,
	Pages = {2487-2492},
	Primaryclass = {astro-ph.SR},
	Title = {{Central compact objects and the hidden magnetic field scenario}},
	Volume = 425,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21679.x}}

@article{vpm12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012CoPhC.183.2042V},
	Archiveprefix = {arXiv},
	Author = {{Vigan{\`o}}, D. and {Pons}, J.~A. and {Miralles}, J.~A.},
	Doi = {10.1016/j.cpc.2012.04.029},
	Eprint = {1204.4707},
	Journal = {Computer Physics Communications},
	Month = oct,
	Pages = {2042-2053},
	Primaryclass = {astro-ph.SR},
	Title = {{A new code for the Hall-driven magnetic evolution of neutron stars}},
	Volume = 183,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.cpc.2012.04.029}}

@article{vilhu09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501..679V},
	Archiveprefix = {arXiv},
	Author = {{Vilhu}, O. and {Hakala}, P. and {Hannikainen}, D.~C. and {McCollough}, M. and {Koljonen}, K.},
	Doi = {10.1051/0004-6361/200811293},
	Eprint = {0904.3967},
	Journal = {\aap},
	Keywords = {black hole physics, accretion, accretion disks, stars: binaries: spectroscopic, stars: winds, outflows, stars: individual: Cygnus X-3, stars: neutron},
	Month = jul,
	Pages = {679-686},
	Primaryclass = {astro-ph.HE},
	Title = {{Orbital modulation of X-ray emission lines in Cygnus X-3}},
	Volume = 501,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/200811293}}

@article{vilhu13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A..48V},
	Archiveprefix = {arXiv},
	Author = {{Vilhu}, O. and {Hannikainen}, D.~C.},
	Doi = {10.1051/0004-6361/201219843},
	Eid = {A48},
	Eprint = {1212.3793},
	Journal = {\aap},
	Keywords = {accretion, accretion disks, black hole physics, binaries: spectroscopic, stars: winds, outflows, X-rays: binaries, gamma rays: stars},
	Month = feb,
	Pages = {A48},
	Primaryclass = {astro-ph.HE},
	Title = {{Modeling the X-ray light curves of Cygnus X-3. Possible role of the jet}},
	Volume = 550,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201219843}}

@article{vink05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...442..587V},
	Author = {{Vink}, J.~S. and {de Koter}, A.},
	Doi = {10.1051/0004-6361:20052862},
	Eprint = {arXiv:astro-ph/0507352},
	Journal = {\aap},
	Keywords = {stars: Wolf-Rayet, stars: early-type, stars: mass-loss, stars: winds, outflows, stars: evolution},
	Month = nov,
	Pages = {587-596},
	Title = {{On the metallicity dependence of Wolf-Rayet winds}},
	Volume = 442,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20052862}}

@ARTICLE{vink06,
   author = {{Vink}, J. and {Kuiper}, L.},
    title = "{Supernova remnant energetics and magnetars: no evidence in favour of millisecond proto-neutron stars}",
  journal = {\mnras},
   eprint = {astro-ph/0604187},
 keywords = {stars: magnetic fields , stars: neutron , ISM: supernova remnants , ISM: individual: N49 , ISM: individual: Kes 73 , ISM: individual: CTB 109},
     year = 2006,
    month = jul,
   volume = 370,
    pages = {L14-L18},
      doi = {10.1111/j.1745-3933.2006.00178.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370L..14V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vogel14,
   author = {{Vogel}, J.~K. and {Hasco{\"e}t}, R. and {Kaspi}, V.~M. and 
	{An}, H. and {Archibald}, R. and {Beloborodov}, A.~M. and {Boggs}, S.~E. and 
	{Christensen}, F.~E. and {Craig}, W.~W. and {Gotthelf}, E.~V. and 
	{Grefenstette}, B.~W. and {Hailey}, C.~J. and {Harrison}, F.~A. and 
	{Kennea}, J.~A. and {Madsen}, K.~K. and {Pivovaroff}, M.~J. and 
	{Stern}, D. and {Zhang}, W.~W.},
    title = "{NuSTAR Observations of the Magnetar 1E 2259+586}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1408.0768},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: individual: 1E 2259+586, stars: magnetars, stars: neutron, X-rays: bursts },
     year = 2014,
    month = jul,
   volume = 789,
      eid = {75},
    pages = {75},
      doi = {10.1088/0004-637X/789/1/75},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...789...75V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{voges99,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...349..389V},
	Author = {{Voges}, W. and {Aschenbach}, B. and {Boller}, T. and {Br{\"a}uninger}, H. and {Briel}, U. and {Burkert}, W. and {Dennerl}, K. and {Englhauser}, J. and {Gruber}, R. and {Haberl}, F. and {Hartner}, G. and {Hasinger}, G. and {K{\"u}rster}, M. and {Pfeffermann}, E. and {Pietsch}, W. and {Predehl}, P. and {Rosso}, C. and {Schmitt}, J.~H.~M.~M. and {Tr{\"u}mper}, J. and {Zimmermann}, H.~U.},
	Eprint = {arXiv:astro-ph/9909315},
	Journal = {\aap},
	Keywords = {CATALOGS, SURVEYS, X-RAYS: GENERAL},
	Month = sep,
	Pages = {389-405},
	Title = {{The ROSAT all-sky survey bright source catalogue}},
	Volume = 349,
	Year = 1999}

@article{voges00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000IAUC.7432....3V},
	Author = {{Voges}, W. and {Aschenbach}, B. and {Boller}, T. and {Brauninger}, H. and {Briel}, U. and {Burkert}, W. and {Dennerl}, K. and {Englhauser}, J. and {Gruber}, R. and {Haberl}, F. and {Hartner}, G. and {Hasinger}, G. and {Pfeffermann}, E. and {Pietsch}, W. and {Predehl}, P. and {Schmitt}, J. and {Trumper}, J. and {Zimmermann}, U.},
	Journal = {\iaucirc},
	Month = may,
	Pages = {3},
	Title = {{Rosat All-Sky Survey Faint Source Catalogue}},
	Volume = 7432,
	Year = 2000}

@article{vrba00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...533L..17V&db_key=AST},
	Author = {{Vrba}, F.~J. and {Henden}, A.~A. and {Luginbuhl}, C.~B. and {Guetter}, H.~H. and {Hartmann}, D.~H. and {Klose}, S.},
	Journal = {\apjl},
	Month = apr,
	Pages = {L17-L20},
	Title = {{The Discovery of an Embedded Cluster of High-Mass Stars near SGR 1900+14}},
	Volume = 533,
	Year = 2000}

@ARTICLE{vulic16,
   author = {{Vulic}, N. and {Gallagher}, S.~C. and {Barmby}, P.},
    title = "{X-rays beware: the deepest Chandra catalogue of point sources in M31}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1607.01772},
 keywords = {catalogues, galaxies: individual: M31, NGC 224, X-rays: binaries, X-rays: galaxies},
     year = 2016,
    month = oct,
   volume = 461,
    pages = {3443-3456},
      doi = {10.1093/mnras/stw1523},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461.3443V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{wachter04,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2004ApJ...615..887W&db_key=AST},
	Author = {{Wachter}, S. and {Patel}, S.~K. and {Kouveliotou}, C. and {Bouchet}, P. and {{\"O}zel}, F. and {Tennant}, A.~F. and {Woods}, P.~M. and {Hurley}, K. and {Becker}, W. and {Slane}, P.},
	Journal = {\apj},
	Month = nov,
	Pages = {887-896},
	Title = {{Precise Localization of the Soft Gamma Repeater SGR 1627-41 and the Anomalous X-Ray Pulsar AXP 1E1841-045 with Chandra}},
	Volume = 615,
	Year = 2004}

@article{wachter09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2164....1W},
	Author = {{Wachter}, S. and {Gelino}, C.~R. and {Gelino}, D.~M. and {Woods}, P. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E.},
	Journal = {Astron. Tel.},
	Keywords = {Infra-Red, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters},
	Month = aug,
	Title = {{Near-IR Observations of the Position of SGR 0418+5729}},
	Volume = 2164,
	Year = 2009}

@ARTICLE{walborn89,
   author = {{Walborn}, N.~R. and {Prevot}, M.~L. and {Prevot}, L. and {Wamsteker}, W. and 
	{Gonzalez}, R. and {Gilmozzi}, R. and {Fitzpatrick}, E.~L.},
    title = "{The spectrograms of Sanduleak -69.202 deg, precursor to supernova 1987A in the Large Magellanic Cloud}",
  journal = {\aap},
 keywords = {Magellanic Clouds, Stellar Spectra, Supergiant Stars, Supernova 1987a, Classifications, Nitrogen, Ubv Spectra},
     year = 1989,
    month = jul,
   volume = 219,
    pages = {229-236},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...219..229W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{walker56,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1956ApJ...123...68W},
	Author = {{Walker}, M.~F.},
	Doi = {10.1086/146132},
	Journal = {\apj},
	Month = jan,
	Pages = {68},
	Title = {{A Photometric Investigation of the Short-Period Eclipsing Binary, Nova DQ Herculis (1934).}},
	Volume = 123,
	Year = 1956,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/146132}}

@article{walter04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ATel..229....1W},
	Author = {{Walter}, R. and {Bodaghee}, A. and {Barlow}, E.~J. and {Bird}, A.~J. and {Dean}, A. and {Hill}, A.~B. and {Shaw}, S. and {Bazzano}, A. and {Ubertini}, P. and {Bassani}, L. and {Malizia}, A. and {Stephen}, J.~B. and {Belanger}, G. and {Lebrun}, F. and {Terrier}, R.},
	Journal = {Astron.~Tel.},
	Keywords = {X-ray, Gamma Ray, Binaries, Black Holes, Neutron Stars},
	Month = feb,
	Title = {{14 New Unidentified INTEGRAL Sources}},
	Volume = 229,
	Year = 2004}

@article{walton13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779..148W},
	Archiveprefix = {arXiv},
	Author = {{Walton}, D.~J. and {Fuerst}, F. and {Harrison}, F. and {Stern}, D. and {Bachetti}, M. and {Barret}, D. and {Bauer}, F. and {Boggs}, S.~E. and {Christensen}, F.~E. and {Craig}, W.~W. and {Fabian}, A.~C. and {Grefenstette}, B.~W. and {Hailey}, C.~J. and {Madsen}, K.~K. and {Miller}, J.~M. and {Ptak}, A. and {Rana}, V. and {Webb}, N.~A. and {Zhang}, W.~W.},
	Doi = {10.1088/0004-637X/779/2/148},
	Eid = {148},
	Journal = {\apj},
	Keywords = {black hole physics, X-rays: binaries, X-rays: individual: Circinus ULX5},
	Month = dec,
	Pages = {148},
	Title = {{An Extremely Luminous and Variable Ultraluminous X-Ray Source in the Outskirts of Circinus Observed with NuSTAR}},
	Volume = 779,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/779/2/148}}

@ARTICLE{walton15,
   author = {{Walton}, D.~J. and {Harrison}, F.~A. and {Bachetti}, M. and 
	{Barret}, D. and {Boggs}, S.~E. and {Christensen}, F.~E. and 
	{Craig}, W.~W. and {Fuerst}, F. and {Grefenstette}, B.~W. and 
	{Hailey}, C.~J. and {Madsen}, K.~K. and {Middleton}, M.~J. and 
	{Rana}, V. and {Roberts}, T.~P. and {Stern}, D. and {Sutton}, A.~D. and 
	{Webb}, N. and {Zhang}, W.},
    title = "{NuSTAR and XMM-Newton Observations of the Extreme Ultraluminous X-Ray Source NGC 5907 ULX1: A Vanishing Act}",
  journal = {\apj},
 keywords = {black hole physics, X-rays: binaries, X-rays: individual: NGC 5907 ULX1},
     year = 2015,
    month = feb,
   volume = 799,
      eid = {122},
    pages = {122},
      doi = {10.1088/0004-637X/799/2/122},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..122W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{walton16,
   author = {{Walton}, D.~J. and {F{\"u}rst}, F. and {Bachetti}, M. and {Barret}, D. and 
	{Brightman}, M. and {Fabian}, A.~C. and {Gehrels}, N. and {Harrison}, F.~A. and 
	{Heida}, M. and {Middleton}, M.~J. and {Rana}, V. and {Roberts}, T.~P. and 
	{Stern}, D. and {Tao}, L. and {Webb}, N.},
    title = "{A 78 Day X-Ray Period Detected from NGC 5907 ULX1 by Swift}",
  journal = {\apjl},
 keywords = {black hole physics, X-rays: binaries, X-rays: individual: NGC 5907 ULX1},
     year = 2016,
    month = aug,
   volume = 827,
      eid = {L13},
    pages = {L13},
      doi = {10.3847/2041-8205/827/1/L13},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...827L..13W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{walton16b,
   author = {{Walton}, D.~J. and {Middleton}, M.~J. and {Pinto}, C. and {Fabian}, A.~C. and 
	{Bachetti}, M. and {Barret}, D. and {Brightman}, M. and {Fuerst}, F. and 
	{Harrison}, F.~A. and {Miller}, J.~M. and {Stern}, D.},
    title = "{An Iron K Component to the Ultrafast Outflow in NGC 1313 X-1}",
  journal = {\apjl},
 keywords = {black hole physics, X-rays: binaries, X-rays: individual: NGC 1313 X-1},
     year = 2016,
    month = aug,
   volume = 826,
      eid = {L26},
    pages = {L26},
      doi = {10.3847/2041-8205/826/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...826L..26W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{wang97,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...318L..59W},
	Author = {{Wang}, Z.~R. and {Qu}, Q.-Y. and {Chen}, Y.},
	Journal = {\aap},
	Keywords = {HISTORY AND PHILOSOPHY OF ASTRONOMY, STARS: SUPERNOVAE: INDIVIDUAL AD393 , ISM: SUPERNOVA REMNANTS},
	Month = feb,
	Pages = {L59-L61},
	Title = {{Is RX J1713.7-3946 the remnant of the AD393 guest star?}},
	Volume = 318,
	Year = 1997}

@article{wang02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...579L..33W&db_key=AST},
	Author = {{Wang}, Z. and {Chakrabarty}, D.},
	Journal = {\apjl},
	Month = nov,
	Pages = {L33-L36},
	Title = {{The Likely Near-Infrared Counterpart to the Anomalous X-Ray Pulsar 1E 1048.1-5937}},
	Volume = 579,
	Year = 2002}

@article{wgl02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002Natur.415..148W},
	Author = {{Wang}, Q.~D. and {Gotthelf}, E.~V. and {Lang}, C.~C.},
	Doi = {10.1038/415148a},
	Journal = {\nat},
	Month = jan,
	Pages = {148-150},
	Title = {{A faint discrete source origin for the highly ionized iron emission from the Galactic Centre region}},
	Volume = 415,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/415148a}}

@ARTICLE{wang06,
   author = {{Wang}, Z. and {Chakrabarty}, D. and {Kaplan}, D.~L.},
    title = "{A debris disk around an isolated young neutron star}",
  journal = {\nat},
   eprint = {astro-ph/0604076},
     year = 2006,
    month = apr,
   volume = 440,
    pages = {772-775},
      doi = {10.1038/nature04669},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.440..772W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{wang08,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...679.1443W},
	Archiveprefix = {arXiv},
	Author = {{Wang}, Z. and {Bassa}, C. and {Kaspi}, V.~M. and {Bryant}, J.~J. and {Morrell}, N.},
	Doi = {10.1086/587505},
	Eprint = {0711.2290},
	Journal = {\apj},
	Keywords = {Infrared: Stars, Stars: Pulsars: Individual: Alphanumeric: 1E 1048.1-5937, Stars: Neutron, X-Rays: Stars},
	Month = jun,
	Pages = {1443-1446},
	Title = {{Optical/Infrared Observations of the Anomalous X-Ray Pulsar 1E 1048.1-5937 During Its 2007 X-Ray Flare}},
	Volume = 679,
	Year = 2008,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/587505}}

@article{wang16,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160308353W},
	Archiveprefix = {arXiv},
	Author = {{Wang}, S. and {Liu}, J. and {Qiu}, Y. and {Bai}, Y. and {Yang}, H. and {Guo}, J. and {Zhang}, P.},
	Eprint = {1603.08353},
	Journal = {\apjs, in press (preprint: astroph/1603.08353)},
	Keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
	Month = mar,
	Primaryclass = {astro-ph.SR},
	Title = {{Chandra ACIS Survey of X-ray Point Sources: The Source Catalog}},
	Year = 2016}
	
@ARTICLE{wang21,
       author = {{Wang}, Yi-Han and {Perna}, Rosalba and {Armitage}, Philip J.},
        title = "{Partial tidal disruption events by stellar mass black holes: Gravitational instability of stream and impact from remnant core}",
      journal = {\mnras},
     keywords = {black hole physics, hydrodynamics, stars: kinematics and dynamics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jun,
       volume = {503},
       number = {4},
        pages = {6005-6015},
          doi = {10.1093/mnras/stab802},
archivePrefix = {arXiv},
       eprint = {2103.09238},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.6005W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{warner87,
       author = {{Warner}, Brian},
        title = "{Absolute magnitudes of cataclysmic variables.}",
      journal = {\mnras},
     keywords = {Accretion Disks, Cataclysmic Variables, Computational Astrophysics, Dwarf Novae, Stellar Magnitude, Mass To Light Ratios, Mass Transfer, Orbital Elements, Stellar Evolution, Astrophysics},
         year = "1987",
        month = "Jul",
       volume = {227},
        pages = {23-73},
          doi = {10.1093/mnras/227.1.23},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987MNRAS.227...23W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{warner95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995Ap%26SS.225..249W},
	Author = {{Warner}, B.},
	Doi = {10.1007/BF00613240},
	Journal = {\apss},
	Month = mar,
	Pages = {249-270},
	Title = {{The AM Canum Venaticorum Stars}},
	Volume = 225,
	Year = 1995,
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/BF00613240}}

@article{warner96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.282..735W},
	Author = {{Warner}, B. and {Livio}, M. and {Tout}, C.~A.},
	Journal = {\mnras},
	Keywords = {ACCRETION, ACCRETION DISCS, INSTABILITIES, METHODS: NUMERICAL, METHODS: OBSERVATIONAL, NOVAE, CATACLYSMIC VARIABLES, WHITE DWARFS},
	Month = oct,
	Pages = {735-738},
	Title = {{Dwarf nova outbursts in truncated accretion discs: down with low alphas}},
	Volume = 282,
	Year = 1996}

@book{warner03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003cvs..book.....W},
	Author = {{Warner}, B.},
	Month = sep,
	Publisher = {Cambridge, UK: Cambridge University Press},
	Title = {{Cataclysmic Variable Stars}},
	Year = 2003}

@article{warner09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397..979W},
	Archiveprefix = {arXiv},
	Author = {{Warner}, B. and {Woudt}, P.~A.},
	Doi = {10.1111/j.1365-2966.2009.15006.x},
	Eprint = {0905.0325},
	Journal = {\mnras},
	Keywords = {binaries: close , stars: individual: V597 Pup , novae, cataclysmic variables , stars: oscillations},
	Month = aug,
	Pages = {979-984},
	Primaryclass = {astro-ph.SR},
	Title = {{The eclipsing intermediate polar V597 Pup (Nova Puppis 2007)}},
	Volume = 397,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15006.x}}

@article{waters88,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...198..200W},
	Author = {{Waters}, L.~B.~F.~M. and {van den Heuvel}, E.~P.~J. and {Taylor}, A.~R. and {Habets}, G.~M.~H.~J. and {Persi}, P.},
	Journal = {\aap},
	Keywords = {B STARS, STELLAR MASS EJECTION, STELLAR WINDS, X RAY BINARIES, INFRARED PHOTOMETRY, INFRARED RADIATION, ULTRAVIOLET RADIATION, VISUAL PHOTOMETRY},
	Month = jun,
	Pages = {200-210},
	Title = {{Evidence for low-velocity winds in Be/X-ray binaries}},
	Volume = 198,
	Year = 1988}

@article{waters89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...223..207W},
	Author = {{Waters}, L.~B.~F.~M. and {de Martino}, D. and {Habets}, G.~M.~H.~J. and {Taylor}, A.~R.},
	Journal = {\aap},
	Keywords = {B STARS, LIGHT CURVE, NEUTRON STARS, X RAY BINARIES, ACCRETION DISKS, STELLAR EVOLUTION, STELLAR LUMINOSITY, STELLAR ORBITS, STELLAR WINDS},
	Month = oct,
	Pages = {207-218},
	Title = {{X-ray light curves of Be/X-ray binaries}},
	Volume = 223,
	Year = 1989}

@article{wvk89,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...223..196W},
	Author = {{Waters}, L.~B.~F.~M. and {van Kerkwijk}, M.~H.},
	Journal = {\aap},
	Keywords = {PULSARS, STELLAR ORBITS, SUPERGIANT STARS, X RAY BINARIES, B STARS, COMPUTATIONAL ASTROPHYSICS, SPIN-ORBIT INTERACTIONS, STELLAR LUMINOSITY, STELLAR MASS, STELLAR WINDS},
	Month = oct,
	Pages = {196-206},
	Title = {{The relation between orbital and spin periods in massive X-ray binaries}},
	Volume = 223,
	Year = 1989}

@article{watson09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...493..339W},
	Archiveprefix = {arXiv},
	Author = {{Watson}, M.~G. and {Schr{\"o}der}, A.~C. and {Fyfe}, D. and {Page}, C.~G. and {Lamer}, G. and {Mateos}, S. and {Pye}, J. and {Sakano}, M. and {Rosen}, S. and {Ballet}, J. and {Barcons}, X. and {Barret}, D. and {Boller}, T. and {Brunner}, H. and {Brusa}, M. and {Caccianiga}, A. and {Carrera}, F.~J. and {Ceballos}, M. and {Della Ceca}, R. and {Denby}, M. and {Denkinson}, G. and {Dupuy}, S. and {Farrell}, S. and {Fraschetti}, F. and {Freyberg}, M.~J. and {Guillout}, P. and {Hambaryan}, V. and {Maccacaro}, T. and {Mathiesen}, B. and {McMahon}, R. and {Michel}, L. and {Motch}, C. and {Osborne}, J.~P. and {Page}, M. and {Pakull}, M.~W. and {Pietsch}, W. and {Saxton}, R. and {Schwope}, A. and {Severgnini}, P. and {Simpson}, M. and {Sironi}, G. and {Stewart}, G. and {Stewart}, I.~M. and {Stobbart}, A.-M. and {Tedds}, J. and {Warwick}, R. and {Webb}, N. and {West}, R. and {Worrall}, D. and {Yuan}, W.},
	Doi = {10.1051/0004-6361:200810534},
	Eprint = {0807.1067},
	Journal = {\aap},
	Keywords = {X-rays: general, catalogs, surveys},
	Month = jan,
	Pages = {339-373},
	Title = {{The XMM-Newton serendipitous survey. V. The Second XMM-Newton serendipitous source catalogue}},
	Volume = 493,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:200810534}}

@ARTICLE{watson11,
   author = {{Watson}, D.},
    title = "{The Galactic dust-to-metals ratio and metallicity using gamma-ray bursts}",
  journal = {\aap},
 keywords = {ISM: abundances, dust, extinction, Galaxy: abundances, X-rays: ISM, gamma-ray burst: general},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201117120},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..16W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{watts06,
   author = {{Watts}, A.~L. and {Strohmayer}, T.~E.},
    title = "{Detection with RHESSI of High-Frequency X-Ray Oscillations in the Tailof the 2004 Hyperflare from SGR 1806-20}",
  journal = {\apjl},
   eprint = {astro-ph/0512630},
 keywords = {Stars: Pulsars: Individual: Alphanumeric: SGR 1806-20, Stars: Magnetic Fields, Stars: Neutron, Stars: Oscillations, Stars: Rotation, X-Rays: Stars},
     year = 2006,
    month = feb,
   volume = 637,
    pages = {L117-L120},
      doi = {10.1086/500735},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...637L.117W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weaver77,
   author = {{Weaver}, R. and {McCray}, R. and {Castor}, J. and {Shapiro}, P. and 
	{Moore}, R.},
    title = "{Interstellar bubbles. II - Structure and evolution}",
  journal = {\apj},
 keywords = {Interstellar Gas, Plasma Interactions, Stellar Winds, Adiabatic Flow, Bubbles, Conductive Heat Transfer, Early Stars, Energy Dissipation, Hydrodynamics, Ion Density (Concentration), Radiative Transfer, Stellar Motions},
     year = 1977,
    month = dec,
   volume = 218,
    pages = {377-395},
      doi = {10.1086/155692},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...218..377W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{wegner94,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.270..229W},
	Author = {{Wegner}, W.},
	Journal = {\mnras},
	Month = sep,
	Pages = {229},
	Title = {{Intrinsic Colour Indices of OB Supergiants Giants and Dwarfs in the UBVRIJHKLM System}},
	Volume = 270,
	Year = 1994}

@inproceedings{weisskopf00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000SPIE.4012....2W},
	Author = {{Weisskopf}, M.~C. and {Tananbaum}, H.~D. and {Van Speybroeck}, L.~P. and {O'Dell}, S.~L.},
	Booktitle = {X-Ray Optics, Instruments, and Missions III. Edited by {Truemper}, J.~E. and {Aschenbach}, B. Proceedings of the SPIE. SPIE, Bellingham WA},
	Month = jul,
	Pages = {2-16},
	Series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
	Title = {{Chandra X-ray Observatory (CXO): overview}},
	Volume = 4012,
	Year = 2000}

@article{weisskopf02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002PASP..114....1W&db_key=AST},
	Author = {{Weisskopf}, M.~C. and {Brinkman}, B. and {Canizares}, C. and {Garmire}, G. and {Murray}, S. and {Van Speybroeck}, L.~P.},
	Journal = {\pasp},
	Month = jan,
	Pages = {1-24},
	Title = {{An Overview of the Performance and Scientific Results from the Chandra X-Ray Observatory}},
	Volume = 114,
	Year = 2002}

@article{weisskopf03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003ExA....16....1W},
	Author = {{Weisskopf}, M.~C. and {Aldcroft}, T.~L. and {Bautz}, M. and {Cameron}, R.~A. and {Dewey}, D. and {Drake}, J.~J. and {Grant}, C.~E. and {Marshall}, H.~L. and {Murray}, S.~S.},
	Doi = {10.1023/B:EXPA.0000038953.49421.54},
	Eprint = {arXiv:astro-ph/0503319},
	Journal = {Experimental Astronomy},
	Keywords = {X-ray astronomy, X-ray missions, X-ray optics, X-ray detectors, X-ray spectroscopy, astrophysics, astronomical objects},
	Month = aug,
	Pages = {1-68},
	Title = {{An Overview of the Performance of the Chandra X-ray Observatory}},
	Volume = 16,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1023/B:EXPA.0000038953.49421.54}}

@article{weisskopf04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605..360W},
	Author = {{Weisskopf}, M.~C. and {Wu}, K. and {Tennant}, A.~F. and {Swartz}, D.~A. and {Ghosh}, K.~K.},
	Doi = {10.1086/381307},
	Eprint = {astro-ph/0311291},
	Journal = {\apj},
	Keywords = {Stars: Binaries: Eclipsing, Black Hole Physics, Galaxies: Individual: Name: Circinus, X-Rays: Binaries, X-Rays: Galaxies},
	Month = apr,
	Pages = {360-367},
	Title = {{On the Nature of the Bright Short-Period X-Ray Source in the Circinus Galaxy Field}},
	Volume = 605,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/381307}}

@article{weltevrede11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.411.1917W},
	Archiveprefix = {arXiv},
	Author = {{Weltevrede}, P. and {Johnston}, S. and {Espinoza}, C.~M.},
	Doi = {10.1111/j.1365-2966.2010.17821.x},
	Eprint = {1010.0857},
	Journal = {\mnras},
	Keywords = {polarization, radiation mechanisms: non-thermal, pulsars: general, pulsars: individual: J1119-6127},
	Month = mar,
	Pages = {1917-1934},
	Primaryclass = {astro-ph.SR},
	Title = {{The glitch-induced identity changes of PSR J1119-6127}},
	Volume = 411,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2010.17821.x}}

@article{wen06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..163..372W},
	Author = {{Wen}, L. and {Levine}, A.~M. and {Corbet}, R.~H.~D. and {Bradt}, H.~V.},
	Doi = {10.1086/500648},
	Eprint = {astro-ph/0512529},
	Journal = {\apjs},
	Keywords = {Stars: Binaries: General, X-Rays: Stars},
	Month = apr,
	Pages = {372-392},
	Title = {{A Systematic Search for Periodicities in RXTE ASM Data}},
	Volume = 163,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/500648}}

@article{wharton12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753..108W},
	Archiveprefix = {arXiv},
	Author = {{Wharton}, R.~S. and {Chatterjee}, S. and {Cordes}, J.~M. and {Deneva}, J.~S. and {Lazio}, T.~J.~W.},
	Doi = {10.1088/0004-637X/753/2/108},
	Eid = {108},
	Eprint = {1111.4216},
	Journal = {\apj},
	Keywords = {Galaxy: center, pulsars: general},
	Month = jul,
	Pages = {108},
	Primaryclass = {astro-ph.HE},
	Title = {{Multiwavelength Constraints on Pulsar Populations in the Galactic Center}},
	Volume = 753,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/753/2/108}}

@article{wheatley03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345.1009W},
	Author = {{Wheatley}, P.~J. and {West}, R.~G.},
	Doi = {10.1046/j.1365-8711.2003.07030.x},
	Eprint = {astro-ph/0307436},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, binaries: eclipsing, stars: individual: OY Car, novae, cataclysmic variables, X-rays: stars},
	Month = nov,
	Pages = {1009-1014},
	Title = {{The X-ray eclipse of OY Car resolved with XMM-Newton: X-ray emission from the polar regions of the white dwarf}},
	Volume = 345,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.07030.x}}

@article{wheaton79,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979Natur.282..240W&db_key=AST},
	Author = {{Wheaton}, W.~A. and {Doty}, J.~P. and {Primini}, F.~A. and {Cooke}, B.~A. and {Dobson}, C.~A. and {Goldman}, A. and {Hecht}, M. and {Howe}, S.~K. and {Hoffman}, J.~A. and {Scheepmaker}, A.},
	Journal = {\nat},
	Month = nov,
	Pages = {240-243},
	Title = {{An absorption feature in the spectrum of the pulsed hard X-ray flux from 4U0115 + 63}},
	Volume = 282,
	Year = 1979}

@article{white76,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1976MNRAS.176..201W},
	Author = {{White}, N.~E. and {Mason}, K.~O. and {Sanford}, P.~W. and {Murdin}, P.},
	Journal = {\mnras},
	Keywords = {SATELLITE-BORNE INSTRUMENTS, STELLAR SPECTRA, TIME RESPONSE, X RAY SOURCES, ARIEL SATELLITES, B STARS, GRAPHS (CHARTS), OAO 3, POWER SPECTRA},
	Month = jul,
	Pages = {201-215},
	Title = {{The X-ray behaviour of 3U 0352+30 (X Per)}},
	Volume = 176,
	Year = 1976}

@article{white78,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1978MNRAS.183P..11W},
	Author = {{White}, N.~E. and {Carpenter}, G.~F.},
	Journal = {\mnras},
	Month = apr,
	Pages = {11P-15P},
	Title = {{The recurrent X-ray transient A0538-66}},
	Volume = 183,
	Year = 1978}

@article{white81,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...247..994W},
	Author = {{White}, N.~E. and {Becker}, R.~H. and {Boldt}, E.~A. and {Holt}, S.~S. and {Serlemitsos}, P.~J. and {Swank}, J.~H.},
	Doi = {10.1086/159109},
	Journal = {\apj},
	Keywords = {Binary Stars, Blue Stars, Modulation, Stellar Radiation, X Ray Sources, Heao 1, Light Curve, Stellar Magnitude, X Ray Spectra},
	Month = aug,
	Pages = {994-1002},
	Title = {{A 5.57 hour modulation of the X-ray flux from 4U 1822-37}},
	Volume = 247,
	Year = 1981,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/159109}}

@article{white82,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...257..318W},
	Author = {{White}, N.~E. and {Holt}, S.~S.},
	Doi = {10.1086/159991},
	Journal = {\apj},
	Keywords = {Eclipsing Binary Stars, Stellar Coronas, Stellar Mass Accretion, X Ray Sources, Compton Effect, Gas Density, Luminosity, Magnitude, Neutron Stars, Optical Thickness, Spectral Emission, Stellar Models, Stellar Spectra, X Rays},
	Month = jun,
	Pages = {318-337},
	Title = {{Accretion disk coronae}},
	Volume = 257,
	Year = 1982,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/159991}}

@article{white83,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...270..711W},
	Author = {{White}, N.~E. and {Swank}, J.~H. and {Holt}, S.~S.},
	Doi = {10.1086/161162},
	Journal = {\apj},
	Month = jul,
	Pages = {711-734},
	Title = {{Accretion powered X-ray pulsars}},
	Volume = 270,
	Year = 1983,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/161162}}

@article{white94,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1994IAUC.6100....1W},
	Author = {{White}, N.~E. and {Giommi}, P. and {Angelini}, L.},
	Journal = {\iaucirc},
	Month = nov,
	Pages = {1},
	Title = {{WGACAT}},
	Volume = 6100,
	Year = 1994}

@article{white97,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/1997ApJ...475..479W},
	Author = {{White}, R.~L. and {Becker}, R.~H. and {Helfand}, D.~J. and {Gregg}, M.~D.},
	Doi = {10.1086/303564},
	Journal = {\apj},
	Month = feb,
	Pages = {479},
	Title = {{A Catalog of 1.4 GHz Radio Sources from the FIRST Survey}},
	Volume = 475,
	Year = 1997,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/303564}}

@article{whiteoak96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..329W},
	Author = {{Whiteoak}, J.~B.~Z. and {Green}, A.~J.},
	Journal = {\aaps},
	Keywords = {ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ATLASES, CATALOGUES, SURVEYS},
	Month = aug,
	Pages = {329-380},
	Title = {{The MOST supernova remnant catalogue (MSC).}},
	Volume = 118,
	Year = 1996}

@article{wieringa10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ATel.2521....1W},
	Author = {{Wieringa}, M.~H. and {Possenti}, A. and {Burgay}, M. and {Esposito}, P. and {Israel}, G.~L. and {Rea}, N. and {Tiengo}, A. and {Turolla}, R. and {Zane}, S. and {G\"otz}, D. and {Mereghetti}, S. and {Stella}, L.},
	Journal = {Astron. Tel.},
	Keywords = {Radio, Pulsars, Soft Gamma-ray Repeaters},
	Month = mar,
	Title = {{ATCA observations of the soft gamma-ray repeater SGR 1833-0832}},
	Volume = 2521,
	Year = 2010}

@article{willingale01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001A%26A...365L.212W&db_key=AST},
	Author = {{Willingale}, R. and {Aschenbach}, B. and {Griffiths}, R.~G. and {Sembay}, S. and {Warwick}, R.~S. and {Becker}, W. and {Abbey}, A.~F. and {Bonnet-Bidaud}, J.-M.},
	Doi = {10.1051/0004-6361:20000114},
	Journal = {\aap},
	Month = jan,
	Pages = {L212-L217},
	Title = {{New light on the X-ray spectrum of the Crab Nebula}},
	Volume = 365,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20000114}}

@article{wilms00,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542..914W},
	Author = {{Wilms}, J. and {Allen}, A. and {McCray}, R.},
	Doi = {10.1086/317016},
	Journal = {\apj},
	Keywords = {Atomic Data, ISM: Dust, Extinction, ISM: Abundances, X-Rays: ISM},
	Month = oct,
	Pages = {914-924},
	Title = {{On the Absorption of X-Rays in the Interstellar Medium}},
	Volume = 542,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/317016}}

@article{wilson02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...565.1150W&db_key=AST},
	Author = {{Wilson}, C.~A. and {Finger}, M.~H. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Woods}, P.~M. and {Kouveliotou}, C.},
	Doi = {10.1086/324707},
	Eprint = {astro-ph/0110084},
	Journal = {\apj},
	Month = feb,
	Pages = {1150-1160},
	Title = {{Serendipitous Detections of XTE J1906+09 with the Rossi X-Ray Timing Explorer}},
	Volume = 565,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/324707}}

@article{winkler03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003A%26A...411L...1W&db_key=AST},
	Author = {{Winkler}, C. and {Courvoisier}, T.~J.-L. and {Di Cocco}, G. and {Gehrels}, N. and {Gim{\'e}nez}, A. and {Grebenev}, S. and {Hermsen}, W. and {Mas-Hesse}, J.~M. and {Lebrun}, F. and {Lund}, N. and {Palumbo}, G.~G.~C. and {Paul}, J. and {Roques}, J.-P. and {Schnopper}, H. and {Sch{\"o}nfelder}, V. and {Sunyaev}, R. and {Teegarden}, B. and {Ubertini}, P. and {Vedrenne}, G. and {Dean}, A.~J.},
	Journal = {\aap},
	Month = nov,
	Pages = {L1-L6},
	Title = {{The INTEGRAL mission}},
	Volume = 411,
	Year = 2003}

@article{winkler07,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...670..635W},
	Author = {{Winkler}, P.~F. and {Petre}, R.},
	Doi = {10.1086/522101},
	Eprint = {arXiv:astro-ph/0608205},
	Journal = {\apj},
	Keywords = {Astrometry, ISM: Individual: Name: Puppis A, Stars: Neutron, ISM: Supernova Remnants, Stars: Supernovae: General, X-rays: individual (RX J0822-4300)},
	Month = nov,
	Pages = {635-642},
	Title = {{Direct Measurement of Neutron Star Recoil in the Oxygen-rich Supernova Remnant Puppis A}},
	Volume = 670,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/522101}}

@article{winter06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649..730W},
	Author = {{Winter}, L.~M. and {Mushotzky}, R.~F. and {Reynolds}, C.~S.},
	Doi = {10.1086/506579},
	Eprint = {arXiv:astro-ph/0512480},
	Journal = {\apj},
	Keywords = {Accretion, Accretion Disks, Galaxies: General, Surveys, X-Rays: Binaries},
	Month = oct,
	Pages = {730-752},
	Title = {{XMM-Newton Archival Study of the Ultraluminous X-Ray Population in Nearby Galaxies}},
	Volume = 649,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/506579}}

@article{wolter04,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...426..787W},
	Author = {{Wolter}, A. and {Trinchieri}, G.},
	Doi = {10.1051/0004-6361:20047110},
	Eprint = {astro-ph/0407446},
	Journal = {\aap},
	Keywords = {galaxies: general, X-rays: galaxies, galaxies: luminosity function, mass function, galaxies: individual: Cartwheel, galaxies: interactions},
	Month = nov,
	Pages = {787-796},
	Title = {{A thorough study of the intriguing X-ray emission from the Cartwheel ring}},
	Volume = 426,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20047110}}

@article{wolter11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011AN....332..358W},
	Archiveprefix = {arXiv},
	Author = {{Wolter}, A. and {Pizzolato}, F. and {Rota}, S. and {Mapelli}, M. and {Ripamonti}, E.},
	Doi = {10.1002/asna.201011499},
	Eprint = {1010.5675},
	Journal = {Astronomische Nachrichten},
	Keywords = {black hole physics, galaxies: peculiar, X-rays: binaries},
	Month = may,
	Pages = {358},
	Primaryclass = {astro-ph.CO},
	Title = {{The population of ULXs in the spiral galaxy NGC 2276}},
	Volume = 332,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1002/asna.201011499}}

@ARTICLE{Woltjer1964,
       author = {{Woltjer}, L.},
        title = "{X-Rays and Type I Supernova Remnants.}",
      journal = {\apj},
         year = 1964,
        month = oct,
       volume = {140},
        pages = {1309-1313},
          doi = {10.1086/148028},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964ApJ...140.1309W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{wkvp99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...527L..47W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {van Paradijs}, J. and {Briggs}, M.~S. and {Hurley}, K. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Preece}, R.~D. and {Giblin}, T.~W. and {Thompson}, C. and {Duncan}, R.~C.},
	Journal = {\apjl},
	Month = dec,
	Pages = {L47-L50},
	Title = {{Hard Burst Emission from the Soft Gamma Repeater SGR 1900+14}},
	Volume = 527,
	Year = 1999}

@article{wkvp99_2,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...518L.103W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {van Paradijs}, J. and {Finger}, M.~H. and {Thompson}, C.},
	Journal = {\apjl},
	Month = jun,
	Pages = {L103-L106},
	Title = {{BEPPOSAX Observations of SGR 1900+14 in Quiescence and during an Active Period}},
	Volume = 518,
	Year = 1999}

@article{woods99,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...519L.139W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {van Paradijs}, J. and {Hurley}, K. and {Kippen}, R.~M. and {Finger}, M.~H. and {Briggs}, M.~S. and {Dieters}, S. and {Fishman}, G.~J.},
	Journal = {\apjl},
	Month = jul,
	Pages = {L139-L142},
	Title = {{Discovery of a New Soft Gamma Repeater, SGR 1627-41}},
	Volume = 519,
	Year = 1999}

@article{wkvp99_3,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1999ApJ...524L..55W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {van Paradijs}, J. and {Finger}, M.~H. and {Thompson}, C. and {Duncan}, R.~C. and {Hurley}, K. and {Strohmayer}, T. and {Swank}, J. and {Murakami}, T.},
	Journal = {\apjl},
	Month = oct,
	Pages = {L55-L58},
	Title = {{Variable Spin-Down in the Soft Gamma Repeater SGR 1900+14 and Correlations with Burst Activity}},
	Volume = 524,
	Year = 1999}

@article{woods00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...535L..55W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {Finger}, M.~H. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Scott}, D.~M. and {Dieters}, S. and {Thompson}, C. and {Duncan}, R.~C. and {Hurley}, K. and {Strohmayer}, T. and {Swank}, J. and {Murakami}, T.},
	Journal = {\apjl},
	Month = may,
	Pages = {L55-L58},
	Title = {{Timing Noise in SGR 1806-20}},
	Volume = 535,
	Year = 2000}

@article{woods01,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...552..748W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Finger}, M.~H. and {Swank}, J. and {Smith}, D.~A. and {Hurley}, K. and {Thompson}, C.},
	Journal = {\apj},
	Month = may,
	Pages = {748-755},
	Title = {{Evidence for a Sudden Magnetic Field Reconfiguration in Soft Gamma Repeater 1900+14}},
	Volume = 552,
	Year = 2001}

@article{woods02,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002ApJ...576..381W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Finger}, M.~H. and {Swank}, J. and {Markwardt}, C.~B. and {Hurley}, K. and {van der Klis}, M.},
	Journal = {\apj},
	Month = sep,
	Pages = {381-390},
	Title = {{Large Torque Variations in Two Soft Gamma Repeaters}},
	Volume = 576,
	Year = 2002}

@article{woods02_iauc,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2002IAUC.7856....1W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {Finger}, M.~H. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Swank}, J. and {Markwardt}, C. and {Strohmayer}, T.},
	Journal = {\iaucirc},
	Month = mar,
	Pages = {1},
	Title = {{XTE J1908+094}},
	Volume = 7856,
	Year = 2002}

@article{woods03,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2003ApJ...596..464W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Finger}, M.~H. and {Feroci}, M. and {Mereghetti}, S. and {Swank}, J.~H. and {Hurley}, K. and {Heise}, J. and {Smith}, D. and {Frontera}, F. and {Guidorzi}, C. and {Thompson}, C.},
	Journal = {\apj},
	Month = oct,
	Pages = {464-469},
	Title = {{The 2001 April Burst Activation of SGR 1900+14: Pulse Properties and Torque}},
	Volume = 596,
	Year = 2003}

@article{woods04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2004ApJ...605..378W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kaspi}, V.~M. and {Thompson}, C. and {Gavriil}, F.~P. and {Marshall}, H.~L. and {Chakrabarty}, D. and {Flanagan}, K. and {Heyl}, J. and {Hernquist}, L.},
	Journal = {\apj},
	Month = apr,
	Pages = {378-399},
	Title = {{Changes in the X-Ray Emission from the Magnetar Candidate 1E 2259+586 during Its 2002 Outburst}},
	Volume = 605,
	Year = 2004}

@article{woods05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..985W},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {Gavriil}, F.~P. and {Kaspi}, V.~M. and {Roberts}, M.~S.~E. and {Ibrahim}, A. and {Markwardt}, C.~B. and {Swank}, J.~H. and {Finger}, M.~H.},
	Doi = {10.1086/431476},
	Eprint = {arXiv:astro-ph/0505039},
	Journal = {\apj},
	Keywords = {Stars: Pulsars: General, Stars: Individual: Alphanumeric: XTE J1810-197, X-Rays: Bursts},
	Month = aug,
	Pages = {985-997},
	Title = {{X-Ray Bursts from the Transient Magnetar Candidate XTE J1810-197}},
	Volume = 629,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/431476}}

@book{woods06,
	Author = {{Woods}, P.~M. and {Thompson}, C.},
	Month = apr,
	Pages = {547},
	Publisher = {Cambridge: Cambridge University Press, p.~547},
	Title = {{in Compact stellar X-ray sources, ed. W. H. G. Levin and M. van der Klis}},
	Year = 2006}

@article{woods07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2007ApJ...654..470W&db_key=AST},
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {Finger}, M.~H. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Wilson}, C.~A. and {Patel}, S.~K. and {Hurley}, K. and {Swank}, J.~H.},
	Doi = {10.1086/507459},
	Eprint = {astro-ph/0602402},
	Journal = {\apj},
	Month = jan,
	Pages = {470-486},
	Title = {{The Prelude to and Aftermath of the Giant Flare of 2004 December 27: Persistent and Pulsed X-Ray Properties of SGR 1806-20 from 1993 to 2005}},
	Volume = 654,
	Year = 2007,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/507459}}

@article{woods08atel1549,
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Hurley}, K.},
	Journal = {Astron. Tel.},
	Title = {{RXTE Observations of Renewed Burst Activity from SGR 1627-41}},
	Volume = 1549,
	Year = 2008}

@article{woods08atel1564,
	Author = {{Woods}, P.~M. and {Kouveliotou}, C. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Hurley}, K. and {Tomsick}, J.},
	Journal = {Astron. Tel.},
	Title = {{Chandra ToO Observation of SGR 1627-41}},
	Volume = 1564,
	Year = 2008}

@article{woods09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2159....1W},
	Author = {{Woods}, P.~M. and {Wachter}, S. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients},
	Month = aug,
	Title = {{Chandra Location of SGR 0418+5729}},
	Volume = 2159,
	Year = 2009}

@article{wgk09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ATel.2152....1W},
	Author = {{Woods}, P.~M. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kouveliotou}, C.},
	Journal = {Astron. Tel.},
	Keywords = {X-ray, Neutron Stars, Pulsars, Soft Gamma-ray Repeaters, Transients},
	Month = aug,
	Title = {{Apparent Glitch in SGR 0418+5729}},
	Volume = 2152,
	Year = 2009}

@ARTICLE{woosley87,
   author = {{Woosley}, S.~E. and {Pinto}, P.~A. and {Martin}, P.~G. and 
	{Weaver}, T.~A.},
    title = "{Supernova 1987A in the Large Magellanic Cloud - The explosion of an approximately 20 solar mass star which has experienced mass loss?}",
  journal = {\apj},
 keywords = {Gravitational Collapse, Magellanic Clouds, Main Sequence Stars, Stellar Mass Ejection, Supernova 1987a, Ubv Spectra, Gamma Ray Spectra, Helium, Light Curve, Stellar Cores, Stellar Spectrophotometry},
     year = 1987,
    month = jul,
   volume = 318,
    pages = {664-673},
      doi = {10.1086/165402},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...318..664W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{woosley95,
   author = {{Woosley}, S.~E. and {Weaver}, T.~A.},
    title = "{The Evolution and Explosion of Massive Stars. II. Explosive Hydrodynamics and Nucleosynthesis}",
  journal = {\apjs},
 keywords = {HYDRODYNAMICS, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: EVOLUTION, STARS: INTERIORS, STARS: SUPERNOVAE: GENERAL},
     year = 1995,
    month = nov,
   volume = 101,
    pages = {181},
      doi = {10.1086/192237},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1995ApJS..101..181W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{woosley02,
   author = {{Woosley}, S.~E. and {Heger}, A. and {Weaver}, T.~A.},
    title = "{The evolution and explosion of massive stars}",
  journal = {Reviews of Modern Physics},
 keywords = {Nucleosynthesis in novae supernovae and other explosive environments, Supernovae, Hydrostatic stellar nucleosynthesis, Elementary particle processes, Stellar structure interiors evolution nucleosynthesis ages, Neutron stars, Relativity and gravitation},
     year = 2002,
    month = nov,
   volume = 74,
    pages = {1015-1071},
      doi = {10.1103/RevModPhys.74.1015},
   adsurl = {http://adsabs.harvard.edu/abs/2002RvMP...74.1015W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{woudt03,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.340.1011W},
	Author = {{Woudt}, P.~A. and {Warner}, B.},
	Doi = {10.1046/j.1365-8711.2003.06367.x},
	Eprint = {astro-ph/0301241},
	Journal = {\mnras},
	Keywords = {techniques: photometric, binaries: close, binaries: eclipsing, novae, cataclysmic variables},
	Month = apr,
	Pages = {1011-1019},
	Title = {{High-speed photometry of faint cataclysmic variables - III. V842 Cen, BY Cir, DD Cir, TV Crv, V655 CrA, CP Cru, V794 Oph, V992 Sco, EU Sct and V373 Sct}},
	Volume = 340,
	Year = 2003,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2003.06367.x}}

@article{wu02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.331..221W},
	Author = {{Wu}, K. and {Cropper}, M. and {Ramsay}, G. and {Sekiguchi}, K.},
	Doi = {10.1046/j.1365-8711.2002.05190.x},
	Eprint = {arXiv:astro-ph/0111358},
	Journal = {\mnras},
	Keywords = {binaries: close, stars: individual: RX J1914+24 stars: magnetic fields, X-rays: stars, binaries: close; stars: individual: RX J1914+24, stars: magnetic fields; X-rays: stars},
	Month = mar,
	Pages = {221-227},
	Title = {{An electrically powered binary star?}},
	Volume = 331,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1046/j.1365-8711.2002.05190.x}}

@article{wu09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009RAA.....9..725W},
	Archiveprefix = {arXiv},
	Author = {{Wu}, K.},
	Doi = {10.1088/1674-4527/9/7/001},
	Eprint = {0906.2091},
	Journal = {Research in Astronomy and Astrophysics},
	Month = jul,
	Pages = {725-744},
	Title = {{Magnetic interaction in ultra-compact binary systems}},
	Volume = 9,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/1674-4527/9/7/001}}

@ARTICLE{xilouris99,
   author = {{Xilouris}, E.~M. and {Byun}, Y.~I. and {Kylafis}, N.~D. and 
	{Paleologou}, E.~V. and {Papamastorakis}, J.},
    title = "{Are spiral galaxies optically thin or thick?}",
  journal = {\aap},
 keywords = {ISM: DUST, EXTINCTION, GALAXIES: ISM, GALAXIES: PHOTOMETRY, GALAXIES: SPIRAL},
     year = 1999,
    month = apr,
   volume = 344,
    pages = {868-878},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...344..868X},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{yakovlev02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...389L..24Y},
	Author = {{Yakovlev}, D.~G. and {Kaminker}, A.~D. and {Haensel}, P. and {Gnedin}, O.~Y.},
	Doi = {10.1051/0004-6361:20020699},
	Eprint = {arXiv:astro-ph/0204233},
	Journal = {\aap},
	Keywords = {pulsars: individual: PSR J0205+6449, stars: neutron, dense matter},
	Month = jul,
	Pages = {L24-L27},
	Title = {{The cooling neutron star in 3C 58}},
	Volume = 389,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361:20020699}}

@article{yamazaki05,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2005astro.ph..2320Y&db_key=PRE},
	Author = {{Yamazaki}, R. and {Ioka}, K. and {Takahara}, F. and {Shibazaki}, N.},
	Eprint = {astro-ph/0502320},
	Journal = {ArXiv Astrophysics e-prints (astro-ph/0502320)},
	Month = feb,
	Title = {{Giant flare of SGR 1806-20 from a relativistic jet}},
	Year = 2005}

@article{yang09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691..131Y},
	Archiveprefix = {arXiv},
	Author = {{Yang}, Y. and {Wilson}, A.~S. and {Matt}, G. and {Terashima}, Y. and {Greenhill}, L.~J.},
	Doi = {10.1088/0004-637X/691/1/131},
	Eprint = {0809.4656},
	Journal = {\apj},
	Keywords = {galaxies: active, galaxies: individual: Circinus, galaxies: Seyfert, X-rays: galaxies},
	Month = jan,
	Pages = {131-139},
	Title = {{Suzaku Observations of the Circinus Galaxy}},
	Volume = 691,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/691/1/131}}

@article{yoshida10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722..760Y},
	Archiveprefix = {arXiv},
	Author = {{Yoshida}, T. and {Ebisawa}, K. and {Matsushita}, K. and {Tsujimoto}, M. and {Kawaguchi}, T.},
	Doi = {10.1088/0004-637X/722/1/760},
	Eprint = {1008.4187},
	Journal = {\apj},
	Keywords = {accretion, accretion disks, black hole physics, galaxies: individual: M 51 NGC 4490 NGC 4485, X-rays: binaries},
	Month = oct,
	Pages = {760-773},
	Primaryclass = {astro-ph.HE},
	Title = {{Long-term Spectral Variations of Ultraluminous X-ray Sources in the Interacting Galaxy Systems M 51 and NGC 4490/85}},
	Volume = 722,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/722/1/760}}

@article{younes12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757...39Y},
	Archiveprefix = {arXiv},
	Author = {{Younes}, G. and {Kouveliotou}, C. and {Kargaltsev}, O. and {Pavlov}, G.~G. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Wachter}, S.},
	Doi = {10.1088/0004-637X/757/1/39},
	Eid = {39},
	Eprint = {1206.3330},
	Journal = {\apj},
	Keywords = {stars: neutron, X-rays: individual: Swift J1834.9{\ndash}0846, X-rays: ISM},
	Month = sep,
	Pages = {39},
	Primaryclass = {astro-ph.HE},
	Title = {{XMM-Newton View of Swift J1834.9-0846 and Its Magnetar Wind Nebula}},
	Volume = 757,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-637X/757/1/39}}

@ARTICLE{younes17,
   author = {{Younes}, G. and {Kouveliotou}, C. and {Jaodand}, A. and {Baring}, M.~G. and 
	{van der Horst}, A.~J. and {Harding}, A.~K. and {Hessels}, J.~W.~T. and 
	{Gehrels}, N. and {Gill}, R. and {Huppenkothen}, D. and {Granot}, J. and 
	{G{\"o}{\u g}{\"u}{\c s}}, E. and {Lin}, L.},
    title = "{X-Ray and Radio Observations of the Magnetar SGR J1935+2154 during Its 2014, 2015, and 2016 Outbursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1702.04370},
 primaryClass = "astro-ph.HE",
 keywords = {radio continuum: stars, stars: individual: SGR J1935+2154, stars: magnetars, stars: neutron, X-rays: stars},
     year = 2017,
    month = oct,
   volume = 847,
      eid = {85},
    pages = {85},
      doi = {10.3847/1538-4357/aa899a},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...847...85Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ybk17,
   author = {{Younes}, G. and {Baring}, M.~G. and {Kouveliotou}, C. and {Harding}, A. and 
	{Donovan}, S. and {G{\"o}{\u g}{\"u}{\c s}}, E. and {Kaspi}, V. and 
	{Granot}, J.},
    title = "{The Sleeping Monster: NuSTAR Observations of SGR 1806-20, 11 Years After the Giant Flare}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1711.00034},
 primaryClass = "astro-ph.HE",
 keywords = {stars: individual: SGR 1806{\ndash}20, stars: magnetars, stars: neutron, X-rays: stars},
     year = 2017,
    month = dec,
   volume = 851,
      eid = {17},
    pages = {17},
      doi = {10.3847/1538-4357/aa96fd},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...851...17Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yukita17,
   author = {{Yukita}, M. and {Ptak}, A. and {Hornschemeier}, A.~E. and {Wik}, D. and 
	{Maccarone}, T.~J. and {Pottschmidt}, K. and {Zezas}, A. and 
	{Antoniou}, V. and {Ballhausen}, R. and {Lehmer}, B.~D. and 
	{Lien}, A. and {Williams}, B. and {Baganoff}, F. and {Boyd}, P.~T. and 
	{Enoto}, T. and {Kennea}, J. and {Page}, K.~L. and {Choi}, Y.
	},
    title = "{Identification of the Hard X-Ray Source Dominating the E $\gt$ 25 keV Emission of the Nearby Galaxy M31}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1703.07318},
 keywords = {galaxies: bulges, galaxies: individual: M31, pulsars: general, stars: neutron, X-rays: binaries},
     year = 2017,
    month = mar,
   volume = 838,
      eid = {47},
    pages = {47},
      doi = {10.3847/1538-4357/aa62a3},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...838...47Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{yukita18,
   author = {{Yukita}, M. and {Tzanavaris}, P. and {Corbet}, R. and {Ptak}, A. and 
	{Hornschemeier}, A. and {Pottschmidt}, K. and {Ballhausen}, R. and 
	{Enoto}, T. and {Antoniou}, V. and {Lehmer}, B. and {Maccarone}, T.~J. and 
	{Wik}, D. and {Williams}, B. and {Zezas}, A.},
    title = "{Detection of potential periodicities in the unique hard X-ray source Swift J0042.6+4112, dominating the hard X-ray emission in M31}",
booktitle = {American Astronomical Society Meeting Abstracts \#231},
     year = 2018,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 231,
    month = jan,
      eid = {333.01},
    pages = {333.01},
   adsurl = {http://adsabs.harvard.edu/abs/2018AAS...23133301Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{zacharias05,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005yCat.1297....0Z},
	Author = {{Zacharias}, N. and {Monet}, D.~G. and {Levine}, S.~E. and {Urban}, S.~E. and {Gaume}, R. and {Wycoff}, G.~L.},
	Journal = {VizieR Online Data Catalog},
	Keywords = {Positional data, Proper motions, Surveys, Photometry: photographic, Photometry: infrared},
	Month = nov,
	Pages = {0},
	Title = {{NOMAD Catalog (Zacharias+ 2005)}},
	Volume = 1297,
	Year = 2005}

@article{zacharias10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.2184Z},
	Archiveprefix = {arXiv},
	Author = {{Zacharias}, N. and {Finch}, C. and {Girard}, T. and {Hambly}, N. and {Wycoff}, G. and {Zacharias}, M.~I. and {Castillo}, D. and {Corbin}, T. and {DiVittorio}, M. and {Dutta}, S. and {Gaume}, R. and {Gauss}, S. and {Germain}, M. and {Hall}, D. and {Hartkopf}, W. and {Hsu}, D. and {Holdenried}, E. and {Makarov}, V. and {Martinez}, M. and {Mason}, B. and {Monet}, D. and {Rafferty}, T. and {Rhodes}, A. and {Siemers}, T. and {Smith}, D. and {Tilleman}, T. and {Urban}, S. and {Wieder}, G. and {Winter}, L. and {Young}, A.},
	Doi = {10.1088/0004-6256/139/6/2184},
	Eprint = {1003.2136},
	Journal = {\aj},
	Keywords = {astrometry, catalogs, reference systems, stars: kinematics and dynamics},
	Month = jun,
	Pages = {2184-2199},
	Primaryclass = {astro-ph.IM},
	Title = {{The Third US Naval Observatory CCD Astrograph Catalog (UCAC3)}},
	Volume = 139,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/139/6/2184}}

@ARTICLE{zalamea10,
       author = {{Zalamea}, I. and {Menou}, K. and {Beloborodov}, A.~M.},
        title = "{White dwarfs stripped by massive black holes: sources of coincident gravitational and electromagnetic radiation}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, white dwarfs, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2010,
        month = nov,
       volume = {409},
       number = {1},
        pages = {L25-L29},
          doi = {10.1111/j.1745-3933.2010.00930.x},
archivePrefix = {arXiv},
       eprint = {1005.3987},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.409L..25Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{zamanov99,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...351..543Z},
	Author = {{Zamanov}, R.~K. and {Mart{\'{\i}}}, J. and {Paredes}, J.~M. and {Fabregat}, J. and {Rib{\'o}}, M. and {Tarasov}, A.~E.},
	Eprint = {arXiv:astro-ph/9909233},
	Journal = {\aap},
	Month = nov,
	Pages = {543-550},
	Title = {{Evidence of H{$\alpha$} periodicities in LS I+61^{deg}303}},
	Volume = 351,
	Year = 1999}

@article{zampieri09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400..677Z},
	Archiveprefix = {arXiv},
	Author = {{Zampieri}, L. and {Roberts}, T.~P.},
	Doi = {10.1111/j.1365-2966.2009.15509.x},
	Eprint = {0909.1017},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs , black hole physics , X-rays: binaries},
	Month = dec,
	Pages = {677-686},
	Primaryclass = {astro-ph.HE},
	Title = {{Low-metallicity natal environments and black hole masses in ultraluminous X-ray sources}},
	Volume = 400,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15509.x}}

@article{zampieri12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.1331Z},
	Archiveprefix = {arXiv},
	Author = {{Zampieri}, L. and {Impiombato}, D. and {Falomo}, R. and {Gris{\'e}}, F. and {Soria}, R.},
	Doi = {10.1111/j.1365-2966.2011.19790.x},
	Eprint = {1109.4437},
	Journal = {\mnras},
	Keywords = {techniques: photometric, stars: individual: NGC 1313 X-2, stars: variables: general, galaxies: individual: NGC 1313, X-rays: binaries, X-rays: individual: NGC 1313 X-2},
	Month = jan,
	Pages = {1331-1337},
	Primaryclass = {astro-ph.HE},
	Title = {{Searching for the orbital period of the ultraluminous X-ray source NGC 1313 X-2}},
	Volume = 419,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2011.19790.x}}

@ARTICLE{zanardo14,
   author = {{Zanardo}, G. and {Staveley-Smith}, L. and {Indebetouw}, R. and 
	{Chevalier}, R.~A. and {Matsuura}, M. and {Gaensler}, B.~M. and 
	{Barlow}, M.~J. and {Fransson}, C. and {Manchester}, R.~N. and 
	{Baes}, M. and {Kamenetzky}, J.~R. and {Laki{\'c}evi{\'c}}, M. and 
	{Lundqvist}, P. and {Marcaide}, J.~M. and {Mart{\'{\i}}-Vidal}, I. and 
	{Meixner}, M. and {Ng}, C.-Y. and {Park}, S. and {Sonneborn}, G. and 
	{Spyromilio}, J. and {van Loon}, J.~T.},
    title = "{Spectral and Morphological Analysis of the Remnant of Supernova 1987A with ALMA and ATCA}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1409.7811},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: supernova remnants, radiation mechanisms: non-thermal, radiation mechanisms: thermal, radio continuum: general, stars: neutron, supernovae: individual: SN 1987A},
     year = 2014,
    month = dec,
   volume = 796,
      eid = {82},
    pages = {82},
      doi = {10.1088/0004-637X/796/2/82},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...796...82Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{zane96,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...471..248Z},
	Author = {{Zane}, S. and {Turolla}, R. and {Treves}, A.},
	Doi = {10.1086/177966},
	Eprint = {arXiv:astro-ph/9605071},
	Journal = {\apj},
	Keywords = {ACCRETION, ACCRETION DISKS, GALAXY: CENTER, STARS: NEUTRON, X-RAYS: STARS},
	Month = nov,
	Pages = {248},
	Title = {{Old Isolated Accreting Neutron Stars: The Diffuse X-Ray Emission from the Galactic Center}},
	Volume = 471,
	Year = 1996,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/177966}}

@article{zane01,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001ApJ...560..384Z&db_key=AST},
	Author = {{Zane}, S. and {Turolla}, R. and {Stella}, L. and {Treves}, A.},
	Doi = {10.1086/322360},
	Eprint = {astro-ph/0103316},
	Journal = {\apj},
	Month = oct,
	Pages = {384-389},
	Title = {{Proton Cyclotron Features in Thermal Spectra of Ultramagnetized Neutron Stars}},
	Volume = 560,
	Year = 2001,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/322360}}

@article{zane09,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398.1403Z},
	Archiveprefix = {arXiv},
	Author = {{Zane}, S. and {Rea}, N. and {Turolla}, R. and {Nobili}, L.},
	Doi = {10.1111/j.1365-2966.2009.15190.x},
	Eprint = {0906.1135},
	Journal = {\mnras},
	Keywords = {radiation mechanisms: non-thermal , stars: neutron , X-rays: stars},
	Month = sep,
	Pages = {1403-1413},
	Title = {{X-ray spectra from magnetar candidates - III. Fitting SGR/AXP soft X-ray emission with non-relativistic Monte Carlo models}},
	Volume = 398,
	Year = 2009,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15190.x}}

@article{zatsepin66,
	Author = {{Zatsepin}, G.T. and {Kuzmin}, V.A.},
	Journal = {Soviet Phys.$-$JETP Lett.},
	Pages = {78},
	Volume = 4,
	Year = 1966}

@article{zavlin95,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...297..441Z},
	Author = {{Zavlin}, V.~E. and {Pavlov}, G.~G. and {Shibanov}, Y.~A. and {Ventura}, J.},
	Journal = {\aap},
	Keywords = {STARS: NEUTRON, MAGNETIC FIELDS, X-RAYS: STARS, PULSARS: INDIVIDUAL: PSR 0656+14, RADIATIVE TRANSFER},
	Month = may,
	Pages = {441},
	Title = {{Thermal radiation from rotating neutron star: effect of the magnetic field and surface temperature distribution.}},
	Volume = 297,
	Year = 1995}

@article{zavlin02,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...569..894Z},
	Author = {{Zavlin}, V.~E. and {Pavlov}, G.~G. and {Sanwal}, D. and {Manchester}, R.~N. and {Tr{\"u}mper}, J. and {Halpern}, J.~P. and {Becker}, W.},
	Doi = {10.1086/339351},
	Eprint = {arXiv:astro-ph/0112544},
	Journal = {\apj},
	Month = apr,
	Pages = {894-902},
	Title = {{X-Radiation from the Millisecond Pulsar J0437-4715}},
	Volume = 569,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/339351}}

@article{zdziarski10,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402..767Z},
	Archiveprefix = {arXiv},
	Author = {{Zdziarski}, A.~A. and {Misra}, R. and {Gierli{\'n}ski}, M.},
	Doi = {10.1111/j.1365-2966.2009.15942.x},
	Eprint = {0905.1086},
	Journal = {\mnras},
	Keywords = {accretion, accretion discs, binaries: general, stars: individual: Cyg X-3, radio continuum: stars, X-rays: binaries, X-rays: stars},
	Month = feb,
	Pages = {767-775},
	Primaryclass = {astro-ph.HE},
	Title = {{Compton scattering as the explanation of the peculiar X-ray properties of Cyg X-3}},
	Volume = 402,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2009.15942.x}}

@article{zdziarski12,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1031Z},
	Archiveprefix = {arXiv},
	Author = {{Zdziarski}, A.~A. and {Maitra}, C. and {Frankowski}, A. and {Skinner}, G.~K. and {Misra}, R.},
	Doi = {10.1111/j.1365-2966.2012.21635.x},
	Eprint = {1205.4402},
	Journal = {\mnras},
	Keywords = {radiation mechanisms: non-thermal, binaries: general, stars: individual: Cyg X-3, stars: winds, outflows, gamma rays: stars, X-rays: binaries},
	Month = oct,
	Pages = {1031-1042},
	Primaryclass = {astro-ph.HE},
	Title = {{Energy-dependent orbital modulation of X-rays and constraints on emission of the jet in Cyg X-3}},
	Volume = 426,
	Year = 2012,
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1365-2966.2012.21635.x}}

@article{zdziarski13,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.429L.104Z},
	Archiveprefix = {arXiv},
	Author = {{Zdziarski}, A.~A. and {Miko{\l}ajewska}, J. and {Belczy{\'n}ski}, K.},
	Doi = {10.1093/mnrasl/sls035},
	Eprint = {1208.5455},
	Journal = {\mnras},
	Keywords = {binaries: close, stars: individual: Cyg X-3, stars: winds, outflows, stars: Wolf-Rayet, X-rays: binaries},
	Month = feb,
	Pages = {L104-L108},
	Primaryclass = {astro-ph.HE},
	Title = {{Cyg X-3: a low-mass black hole or a neutron star}},
	Volume = 429,
	Year = 2013,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnrasl/sls035}}

@ARTICLE{zepf07,
       author = {{Zepf}, Stephen E. and {Maccarone}, Thomas J. and {Bergond}, Gilles and
         {Kundu}, Arunav and {Rhode}, Katherine L. and {Salzer}, John J.},
        title = "{[O III] {\ensuremath{\lambda}}5007 Emission from the Black Hole X-Ray Binary in an NGC 4472 Globular Cluster}",
      journal = {\apjl},
     keywords = {galaxies: individual (NGC 4472), Galaxies: Star Clusters, Galaxy: Globular Clusters: General, X-Rays: Binaries, X-Rays: Galaxies: Clusters, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {L69-L72},
          doi = {10.1086/523797},
archivePrefix = {arXiv},
       eprint = {0709.3103},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669L..69Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zepf08,
       author = {{Zepf}, Stephen E. and {Stern}, Daniel and {Maccarone}, Thomas J. and
         {Kundu}, Arunav and {Kamionkowski}, Marc and {Rhode}, Katherine L. and
         {Salzer}, John J. and {Ciardullo}, Robin and {Gronwall}, Caryl},
        title = "{Very Broad [O III] {\ensuremath{\lambda}}{\ensuremath{\lambda}}4959, 5007 Emission from the NGC 4472 Globular Cluster RZ 2109 and Implications for the Mass of Its Black Hole X-Ray Source}",
      journal = {\apjl},
     keywords = {galaxies: individual: NGC 4472, galaxies: star clusters, globular clusters: general, X-rays: binaries, X-rays: galaxies: clusters, Astrophysics},
         year = 2008,
        month = aug,
       volume = {683},
       number = {2},
        pages = {L139},
          doi = {10.1086/591937},
archivePrefix = {arXiv},
       eprint = {0805.2952},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...683L.139Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{zezas02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...577..710Z},
	Author = {{Zezas}, A. and {Fabbiano}, G. and {Rots}, A.~H. and {Murray}, S.~S.},
	Doi = {10.1086/342160},
	Journal = {\apj},
	Keywords = {Galaxies: Individual: NGC Number: NGC 4038/4039, Galaxies: Interactions, Galaxies: Peculiar, X-Rays: Galaxies},
	Month = oct,
	Pages = {710-725},
	Title = {{Chandra Observations of ``The Antennae'' Galaxies (NGC 4038/4039). III. X-Ray Properties and Multiwavelength Associations of the X-Ray Source Population}},
	Volume = 577,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342160}}

@article{zf02,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...577..726Z},
	Author = {{Zezas}, A. and {Fabbiano}, G.},
	Doi = {10.1086/342135},
	Journal = {\apj},
	Keywords = {Galaxies: Individual: NGC Number: NGC 4038/4039, Galaxies: Interactions, Galaxies: Peculiar, X-Rays: Galaxies},
	Month = oct,
	Pages = {726-737},
	Title = {{Chandra Observations of ``The Antennae'' Galaxies (NGC 4038/4039). IV. The X-Ray Source Luminosity Function and the Nature of Ultraluminous X-Ray Sources}},
	Volume = 577,
	Year = 2002,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/342135}}

@article{zezas06,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..166..211Z},
	Author = {{Zezas}, A. and {Fabbiano}, G. and {Baldi}, A. and {Schweizer}, F. and {King}, A.~R. and {Ponman}, T.~J. and {Rots}, A.~H.},
	Doi = {10.1086/501526},
	Journal = {\apjs},
	Keywords = {galaxies: individual (NGC 4038/39), Galaxies: Interactions, Galaxies: Peculiar, X-Rays: Binaries, X-Rays: Galaxies},
	Month = sep,
	Pages = {211-248},
	Title = {{Chandra Monitoring Observations of The Antennae Galaxies. I. Catalog of Source Properties}},
	Volume = 166,
	Year = 2006,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/501526}}

@article{zhang00,
	Adsnote = {Provided by the NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000ApJ...545L.127Z&db_key=AST},
	Author = {{Zhang}, B. and {Xu}, R.~X. and {Qiao}, G.~J.},
	Journal = {\apjl},
	Month = dec,
	Pages = {L127-L130},
	Title = {{Nature and Nurture: a Model for Soft Gamma-Ray Repeaters}},
	Volume = 545,
	Year = 2000}

@article{zh00,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2000ApJ...532.1150Z},
	Author = {{Zhang}, B. and {Harding}, A.~K.},
	Doi = {10.1086/308598},
	Eprint = {arXiv:astro-ph/9911028},
	Journal = {\apj},
	Month = apr,
	Pages = {1150-1171},
	Title = {{Full Polar Cap Cascade Scenario: Gamma-Ray and X-Ray Luminosities from Spin-powered Pulsars}},
	Volume = 532,
	Year = 2000,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/308598}}

@article{zhang04,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...614L..53Z},
	Author = {{Zhang}, B. and {Loeb}, A.},
	Doi = {10.1086/425339},
	Eprint = {arXiv:astro-ph/0406609},
	Journal = {\apjl},
	Month = oct,
	Pages = {L53-L56},
	Title = {{A Model for the Flaring Radio Emission in the Double Pulsar System J0737-3039}},
	Volume = 614,
	Year = 2004,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/425339}}

@ARTICLE{zhao21,
       author = {{Zhao}, Z.~Y. and {Wang}, Y.~Y. and {Zou}, Y.~C. and {Wang}, F.~Y. and {Dai}, Z.~G.},
        title = "{Quasi-periodic Eruptions from Helium Envelope of Hydrogen-deficient Stars Stripped by Supermassive Black Holes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.03471},
        pages = {arXiv:2109.03471},
archivePrefix = {arXiv},
       eprint = {2109.03471},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210903471Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhekov06,
   author = {{Zhekov}, S.~A. and {McCray}, R. and {Borkowski}, K.~J. and 
	{Burrows}, D.~N. and {Park}, S.},
    title = "{Chandra LETG Observations of Supernova Remnant 1987A}",
  journal = {\apj},
   eprint = {astro-ph/0603305},
 keywords = {ISM: Supernova Remnants, Stars: Supernovae: Individual: Alphanumeric: SNR 1987A, X-Rays: ISM},
     year = 2006,
    month = jul,
   volume = 645,
    pages = {293-302},
      doi = {10.1086/504285},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...645..293Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{ziosi14,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3703Z},
	Archiveprefix = {arXiv},
	Author = {{Ziosi}, B.~M. and {Mapelli}, M. and {Branchesi}, M. and {Tormen}, G.},
	Doi = {10.1093/mnras/stu824},
	Eprint = {1404.7147},
	Journal = {\mnras},
	Keywords = {black hole physics, gravitational waves, methods: numerical, binaries: general, galaxies: star clusters: general},
	Month = jul,
	Pages = {3703-3717},
	Title = {{Dynamics of stellar black holes in young star clusters with different metallicities - II. Black hole-black hole binaries}},
	Volume = 441,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/mnras/stu824}}

@ARTICLE{zolotukhin17,
   author = {{Zolotukhin}, I.~Y. and {Bachetti}, M. and {Sartore}, N. and 
	{Chilingarian}, I.~V. and {Webb}, N.~A.},
    title = "{The Slowest Spinning X-Ray Pulsar in an Extragalactic Globular Cluster}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1602.05191},
 primaryClass = "astro-ph.HE",
 keywords = {astronomical databases: miscellaneous, galaxies: individual: M31, globular clusters: individual: Bol D91, pulsars: individual: 3XMM J004301.4+413017, virtual observatory tools, X-rays: binaries},
     year = 2017,
    month = apr,
   volume = 839,
      eid = {125},
    pages = {125},
      doi = {10.3847/1538-4357/aa689d},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...839..125Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{zombeck07,
	Adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System},
	Adsurl = {http://cdsads.u-strasbg.fr/abs/2007hsaa.book.....Z},
	Author = {{Zombeck}, M.},
	Publisher = {Cambridge University Press, Cambridge, UK},
	Title = {{Handbook of Space Astronomy and Astrophysics: Third Edition}},
	Year = 2007}

@article{zorotovic11,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..42Z},
	Archiveprefix = {arXiv},
	Author = {{Zorotovic}, M. and {Schreiber}, M.~R. and {G{\"a}nsicke}, B.~T.},
	Doi = {10.1051/0004-6361/201116626},
	Eid = {A42},
	Eprint = {1108.4600},
	Journal = {\aap},
	Keywords = {binaries: close, white dwarfs, novae, cataclysmic variables},
	Month = dec,
	Pages = {A42},
	Primaryclass = {astro-ph.SR},
	Title = {{Post common envelope binaries from SDSS. XI. The white dwarf mass distributions of CVs and pre-CVs}},
	Volume = 536,
	Year = 2011,
	Bdsk-Url-1 = {http://dx.doi.org/10.1051/0004-6361/201116626}}

@ARTICLE{zubko04,
   author = {{Zubko}, V. and {Dwek}, E. and {Arendt}, R.~G.},
    title = "{Interstellar Dust Models Consistent with Extinction, Emission, and Abundance Constraints}",
  journal = {\apjs},
 keywords = {ISM: Dust, Extinction, Infrared: ISM, ISM: Abundances, Ultraviolet: ISM},
     year = 2004,
    month = jun,
   volume = 152,
    pages = {211-249},
      doi = {10.1086/382351},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..152..211Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972ApJ...178..347B,
       author = {{Bardeen}, James M. and {Press}, William H. and {Teukolsky}, Saul A.},
        title = "{Rotating Black Holes: Locally Nonrotating Frames, Energy Extraction, and Scalar Synchrotron Radiation}",
      journal = {\apj},
         year = 1972,
        month = dec,
       volume = {178},
        pages = {347-370},
          doi = {10.1086/151796},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...178..347B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dicarlo21,
       author = {{Di Carlo}, Ugo N. and {Mapelli}, Michela and {Pasquato}, Mario and {Rastello}, Sara and {Ballone}, Alessandro and {Dall'Amico}, Marco and {Giacobbo}, Nicola and {Iorio}, Giuliano and {Spera}, Mario and {Torniamenti}, Stefano and {Haardt}, Francesco},
        title = "{Intermediate-mass black holes from stellar mergers in young star clusters}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, methods: numerical, binaries: general, stars: kinematics and dynamics, galaxies: star clusters: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = nov,
       volume = {507},
       number = {4},
        pages = {5132-5143},
          doi = {10.1093/mnras/stab2390},
archivePrefix = {arXiv},
       eprint = {2105.01085},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.507.5132D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021MNRAS.501.5257R,
       author = {{Rizzuto}, Francesco Paolo and {Naab}, Thorsten and {Spurzem}, Rainer and {Giersz}, Mirek and {Ostriker}, J.~P. and {Stone}, N.~C. and {Wang}, Long and {Berczik}, Peter and {Rampp}, M.},
        title = "{Intermediate mass black hole formation in compact young massive star clusters}",
      journal = {\mnras},
     keywords = {gravitational waves, methods: numerical, stars: black holes, stars: mass-loss, galaxies: star clusters: general, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = mar,
       volume = {501},
       number = {4},
        pages = {5257-5273},
          doi = {10.1093/mnras/staa3634},
archivePrefix = {arXiv},
       eprint = {2008.09571},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.5257R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2019ApJ...870L..18Q,
       author = {{Qin}, Ying and {Marchant}, Pablo and {Fragos}, Tassos and {Meynet}, Georges and {Kalogera}, Vicky},
        title = "{On the Origin of Black Hole Spin in High-mass X-Ray Binaries}",
      journal = {\apjl},
     keywords = {binaries: close, stars: black holes, stars: massive, stars: rotation, X-rays: binaries, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jan,
       volume = {870},
       number = {2},
          eid = {L18},
        pages = {L18},
          doi = {10.3847/2041-8213/aaf97b},
archivePrefix = {arXiv},
       eprint = {1810.13016},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...870L..18Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020arXiv200713746A,
       author = {{Arca Sedda}, Manuel and {Amaro Seoane}, Pau and {Chen}, Xian},
        title = "{Merging stellar and intermediate-mass black holes in dense clusters: implications for LIGO, LISA, and the next generation of gravitational wave detectors}",
      journal = {\aap},
     keywords = {black hole physics, gravitational waves, globular clusters: general, Galaxy: general, Astrophysics - Astrophysics of Galaxies, General Relativity and Quantum Cosmology},
         year = 2021,
        month = aug,
       volume = {652},
          eid = {A54},
        pages = {A54},
          doi = {10.1051/0004-6361/202037785},
archivePrefix = {arXiv},
       eprint = {2007.13746},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...652A..54A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MNRAS.432.3250K,
       author = {{Katz}, Harley and {Ricotti}, Massimo},
        title = "{Two epochs of globular cluster formation from deep field luminosity functions: implications for reionization and the Milky Way satellites}",
      journal = {\mnras},
     keywords = {globular clusters: general, galaxies: luminosity function, mass function, cosmology: theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = jul,
       volume = {432},
       number = {4},
        pages = {3250-3261},
          doi = {10.1093/mnras/stt676},
archivePrefix = {arXiv},
       eprint = {1211.6153},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.432.3250K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1962AJ.....67..591K,
       author = {{Kozai}, Yoshihide},
        title = "{Secular perturbations of asteroids with high inclination and eccentricity}",
      journal = {\aj},
         year = 1962,
        month = nov,
       volume = {67},
        pages = {591-598},
          doi = {10.1086/108790},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1962AJ.....67..591K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1962P&SS....9..719L,
       author = {{Lidov}, M.~L.},
        title = "{The evolution of orbits of artificial satellites of planets under the action of gravitational perturbations of external bodies}",
      journal = {\planss},
         year = 1962,
        month = oct,
       volume = {9},
       number = {10},
        pages = {719-759},
          doi = {10.1016/0032-0633(62)90129-0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1962P&SS....9..719L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJS..112..423H,
       author = {{Hollywood}, J.~M. and {Melia}, Fulvio},
        title = "{General Relativistic Effects on the Infrared Spectrum of Thin Accretion Disks in Active Galactic Nuclei: Application to Sagittarius A *}",
      journal = {\apjs},
     keywords = {ACCRETION, ACCRETION DISKS, GALAXIES: ACTIVE, INFRARED: GALAXIES, RELATIVITY, Accretion, Accretion Disks, Galaxies: Active, Infrared: Galaxies, Relativity},
         year = 1997,
        month = oct,
       volume = {112},
       number = {2},
        pages = {423-455},
          doi = {10.1086/313036},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJS..112..423H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2019MNRAS.483..152A,
       author = {{Arca-Sedda}, M. and {Capuzzo-Dolcetta}, R.},
        title = "{The MEGaN project II. Gravitational waves from intermediate-mass and binary black holes around a supermassive black hole}",
      journal = {\mnras},
     keywords = {gravitational waves, galaxies: nuclei, galaxies: star clusters: general, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {483},
       number = {1},
        pages = {152-171},
          doi = {10.1093/mnras/sty3096},
archivePrefix = {arXiv},
       eprint = {1709.05567},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483..152A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2008AJ....135.2398M,
       author = {{Mikkola}, Seppo and {Merritt}, David},
        title = "{Implementing Few-Body Algorithmic Regularization with Post-Newtonian Terms}",
      journal = {\aj},
     keywords = {black hole physics, celestial mechanics, Galaxy: center, methods: N-body simulations, relativity, stellar dynamics, Astrophysics},
         year = 2008,
        month = jun,
       volume = {135},
       number = {6},
        pages = {2398-2405},
          doi = {10.1088/0004-6256/135/6/2398},
archivePrefix = {arXiv},
       eprint = {0709.3367},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AJ....135.2398M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2016ARA&A..54..441N,
       author = {{Naoz}, Smadar},
        title = "{The Eccentric Kozai-Lidov Effect and Its Applications}",
      journal = {\araa},
     keywords = {Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = sep,
       volume = {54},
        pages = {441-489},
          doi = {10.1146/annurev-astro-081915-023315},
archivePrefix = {arXiv},
       eprint = {1601.07175},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ARA&A..54..441N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

